Trusted Hardware Acceleration for Malicious-Secure Function Secret Sharing

Function secret sharing (FSS) underlies two-party private inference and private information retrieval, with cost dominated by generating, moving and evaluating distributed point function (DPF) keys. A trusted GPU-integrated distributed function accelerator (DFA) removed key movement by generating and consuming keys locally, but tolerates only semi-honest adversaries. A malicious host or GPU can tamper with shares, replay one-time material, swap buffers after checking, request early outputs, or abuse the accelerator as a forgery oracle, while malicious FSS ships large authenticated keys or multiplies DPF work. We present VIGOR-DFA, protecting the chain from authorized input to authorized output release with three mechanisms: a fresh authentication epilogue using three field multiplications per DPF output, 3.8-4.0 times faster per gate than per-lane DPF tag trees; a freeze-before-challenge check of every opening with t = 3 independent MAC lanes over F_{2^61-1}; and a role-bound one-time resource ledger with a release guard, in a protected datapath beside the GPU L2 cache. We prove stand-alone static malicious security with abort in a protected-module model, with statistical error Q(2/p)^t approximately 2^-148 for Q less than or equal to 2^32 checked batches. Our DFA-calibrated model shows that, against dealer-based malicious FSS modeled after the protocol family of Shark, VIGOR-DFA removes 21.8-563 GB of per-query offline authenticated material and, mainly by generating it in-module, lowers LAN latency by 10.1-14.0 times (1.5-1.8 times excluding offline distribution) and energy by 3.0-3.9 times. Malicious security costs 2.5-3.5 times LAN latency over semi-honest DFA and 0.145 mm^2 at 7 nm. We have completed the verification of specifications and the functional CPU reference model, including GPU/RTL conformance verification, protected runtime evaluation, and deployment-related tests.

==> qa/draft1/macros.tex <==
% ------------------------------------------------------------------
% Shared packages and macros for the TIFS manuscript.
% Every section/appendix/algorithm/table file relies ONLY on these.
% ------------------------------------------------------------------
\usepackage[T1]{fontenc}
\usepackage{amsmath,amssymb,amsfonts,mathtools}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{graphicx}
\usepackage[dvipsnames,table]{xcolor}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{array}
\usepackage{tabularx}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{setspace}
\let\labelindent\relax
\usepackage[inline]{enumitem}
\usepackage{pifont}
\usepackage{xspace}
\usepackage{stmaryrd}
\usepackage{cite}
\usepackage[hidelinks]{hyperref}
\usepackage[capitalise,noabbrev]{cleveref}

% ---------------- cross-reference names (IEEE style) ----------------
\crefname{section}{Section}{Sections}
\Crefname{section}{Section}{Sections}
\crefname{subsection}{Section}{Sections}
\Crefname{subsection}{Section}{Sections}
\crefname{subsubsection}{Section}{Sections}
\Crefname{subsubsection}{Section}{Sections}
\crefname{appendix}{Appendix}{Appendices}
\Crefname{appendix}{Appendix}{Appendices}
\crefname{figure}{Fig.}{Figs.}
\Crefname{figure}{Fig.}{Figs.}
\crefname{table}{Table}{Tables}
\Crefname{table}{Table}{Tables}
\crefname{algorithm}{Algorithm}{Algorithms}
\Crefname{algorithm}{Algorithm}{Algorithms}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Eq.}{Eqs.}
\crefname{ALC@unique}{line}{lines}
\crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{remark}{Remark}{Remarks}
\crefname{proposition}{Proposition}{Propositions}

% ---------------- theorem environments ----------------
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\theoremstyle{remark}
\newtheorem{remark}{Remark}

% ---------------- algorithm style (FuseFSS / DFA hybrid) ----------------
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) \textit{#1}}
\algnewcommand{\Abort}{\textbf{abort}}
\newcommand{\algstretch}{\setstretch{0.92}}

% ---------------- estimates: RED, to be replaced by measured values ----------------
\newcommand{\est}[1]{\textcolor{red}{#1}}

% ---------------- names ----------------
\newcommand{\sys}{VIGOR-DFA\xspace}
\newcommand{\DFA}{DFA\xspace}
\newcommand{\ProfT}{Profile~$\mathsf{T}$\xspace}
\newcommand{\ProfU}{Profile~$\mathsf{U}$\xspace}

% ---------------- algebra ----------------
\newcommand{\F}{\mathbb{F}}
\newcommand{\Fp}{\mathbb{F}_p}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\bits}[1]{\{0,1\}^{#1}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\getsr}{\xleftarrow{\$}}
\newcommand{\inner}[2]{\langle #1, #2\rangle}
\newcommand{\auth}[1]{[#1]}                  % authenticated sharing
\newcommand{\authb}[2]{[#1]_{#2}}            % party-b tuple (x_b, gamma_{b,1..t})
\newcommand{\tagv}[3]{\gamma_{#1,#2}^{(#3)}} % optional explicit tag notation

% ---------------- FSS objects ----------------
\newcommand{\Gen}{\mathsf{Gen}}
\newcommand{\Eval}{\mathsf{Eval}}
\newcommand{\EvalAll}{\mathsf{EvalAll}}
\newcommand{\DPF}{\mathsf{DPF}}
\newcommand{\DCF}{\mathsf{DCF}}
\newcommand{\CW}{\mathsf{CW}}
\newcommand{\CWout}{\mathsf{CW}^{\mathrm{out}}}
\newcommand{\sCW}{s^{\mathsf{CW}}}
\newcommand{\tCW}[1]{t^{\mathsf{CW},#1}}
\newcommand{\PRG}{G}
\newcommand{\Conv}{H}
\newcommand{\keep}{\mathit{keep}}
\newcommand{\lose}{\mathit{lose}}

% ---------------- crypto ----------------
\newcommand{\PRF}{\mathsf{PRF}}
\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\Hash}{\mathsf{Hash}}
\newcommand{\AEAD}{\mathsf{AEAD}}
\newcommand{\Adv}{\mathcal{A}}
\newcommand{\Sim}{\mathcal{S}}
\newcommand{\Env}{\mathcal{Z}}
\newcommand{\View}{\mathsf{View}}
\newcommand{\Real}{\mathsf{Real}}
\newcommand{\Ideal}{\mathsf{Ideal}}
\newcommand{\Hyb}[1]{\mathsf{H}_{#1}}
\newcommand{\Leak}{\mathcal{L}}
\newcommand{\FC}{\mathcal{F}^{\mathrm{abort}}_{C,\mu}}
\newcommand{\FPIR}{\mathcal{F}^{\mathrm{abort}}_{\mathrm{PIR}}}
\newcommand{\eps}[1]{\epsilon_{\mathsf{#1}}}
\newcommand{\negl}{\mathsf{negl}}

% ---------------- protocol / ledger / commands ----------------
\newcommand{\cmd}[1]{\texttt{\detokenize{#1}}}
\newcommand{\lstate}[1]{\textsf{#1}}
\newcommand{\algname}[1]{\textsf{#1}}
\newcommand{\CheckOpen}{\algname{CheckOpen}\xspace}
\newcommand{\AuthShare}{\algname{AuthShare}\xspace}
\newcommand{\Epilogue}{\algname{Epilogue}\xspace}

% ---------------- marks for tables ----------------
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\pmark}{\ding{109}}   % partial


==> qa/draft1/sections/00_abstract.tex <==
% ==================================================================
% Abstract and index terms (owner: sections/00_abstract.tex)
% Red values are model estimates (\est{}); see Appendix F.
% ==================================================================
\begin{abstract}
Function secret sharing (FSS) underlies some of the fastest two-party protocols for private inference and private information retrieval (PIR), and its cost is dominated by generating, moving and evaluating distributed point function (DPF) keys. A trusted distributed function accelerator (DFA) next to the GPU removed that key movement by generating and consuming keys locally, but it is secure only against semi-honest adversaries. A malicious host, driver or GPU can tamper with shares, replay one-time material, swap buffers between check and use, request outputs early, or abuse the module as a forgery oracle, while known malicious FSS routes ship large authenticated keys or multiply DPF work. We present \sys, which protects the chain from authorized input to authorized output release with three co-designed mechanisms: a fresh authentication epilogue that authenticates each DPF output with three field multiplications instead of extra DPF trees; a freeze-before-challenge check of every opening with $t=3$ independent MAC lanes over $\F_{2^{61}-1}$; and a role-bound one-time resource ledger with a release guard, realized as a protected datapath beside the GPU L2 cache. We prove static malicious security with abort in an explicit protected-module model, with statistical error $Q(2/p)^t\approx 2^{-148}$ for $Q\le 2^{32}$ checked batches. Our model estimates that, against dealer-based malicious FSS, \sys reduces LAN latency by \est{10.1--14.0$\times$} and energy by \est{3.0--3.9$\times$} and removes \est{21.8--563~GB} of offline authenticated material per query. Malicious security costs \est{2.5--3.5$\times$} LAN latency over semi-honest trusted DFA, PIR keeps \est{93\%} of its throughput, and the added area is \est{0.145~mm$^2$} at 7~nm.
\end{abstract}

\begin{IEEEkeywords}
Function secret sharing, distributed point function, malicious security, trusted hardware, hardware accelerator, secure inference, private information retrieval.
\end{IEEEkeywords}


==> qa/draft1/sections/01_introduction.tex <==
% ==================================================================
% Section I: Introduction (owner: sections/01_introduction.tex)
% Labels defined here: sec:intro
% Red values are model estimates (\est{}); black numbers are either
% reproduced from the DFA paper (cited) or executed reference tests.
% ==================================================================
\section{Introduction}\label{sec:intro}

\IEEEPARstart{P}{rivacy}-preserving computation is moving from prototypes into deployments where the data are both valuable and regulated: hospitals that want to run a diagnostic model on records they may not export, cloud providers that serve proprietary models to clients who will not reveal their queries, and lookup services whose queries disclose what a user is interested in. Secure two-party computation (2PC) for private machine-learning (ML) inference~\cite{yao1986generate,goldreich2019play,mohassel2017secureml,rathee2020cryptflow2} and private information retrieval (PIR)~\cite{chor1998private,angel2018pir} address these settings with cryptographic rather than contractual guarantees. Function secret sharing (FSS)~\cite{boyle2015fss,boyle2016function} has become one of the most effective building blocks for both. In FSS-based private inference, the parties open a masked input $x+r$ and evaluate one-time keys for the gate function shifted by the mask, so that a nonlinear layer often costs a single online round~\cite{boyle2021function,gupta2023sigma,jawalkar2024orca}. In two-server PIR, the client splits a point function into two short keys and each server evaluates its key over the entire database~\cite{gilboa2014distributed,wang2017splinter,lam2023gpu}.

The price of this online efficiency is paid in distributed point function (DPF) work. Every comparison, lookup table and interval test in an FSS-compiled model is built from DPFs or from the distributed comparison functions (DCFs) derived from them~\cite{boyle2021function,storrier2023grotto,gupta2023sigma}, and each key is used once. A dealer must therefore generate, ship and store fresh keys for every nonlinear element of every query: 17.1~GB of offline material for a single BERT-Base inference~\cite{dfa2026trusted}, a cost that cannot always be hidden behind the online phase~\cite{huang2026beyond}. PIR, conversely, is dominated by full-domain DPF evaluation, which is AES-bound even on a modern GPU~\cite{lam2023gpu}. The distributed function accelerator (DFA)~\cite{dfa2026trusted} attacked both costs with a small DPF engine integrated next to the GPU L2 cache. In its trusted mode, a protected module in each server attests to its peer, establishes a shared key and plays the dealer locally: it generates its own party's key share on demand and consumes each correction word as soon as it is produced (\emph{generate-and-consume}, GaC), so keys are never distributed, stored or reread. For BERT-Base, trusted DFA reduces LAN latency from 18.8~s to 1.42~s and offline communication from 17.1~GB to 0.1~GB, and it raises PIR throughput by $5.05\times$ for $2^{20}$ records~\cite{dfa2026trusted}.

\textbf{The semi-honest boundary.}
DFA, like Sigma~\cite{gupta2023sigma}, Orca~\cite{jawalkar2024orca} and most GPU-based FSS systems, is secure only against semi-honest adversaries: it assumes that both servers run the prescribed code. In a real deployment, however, the component that is easiest to subvert is not the small protected module but everything around it: the host operating system, the GPU driver and runtime, the kernels running on the streaming multiprocessors (SMs), the DMA buffers in host and GPU memory, and the network stack. These components hold all of the data path and most of the software, and both the attack literature on privileged software and firmware~\cite{xu2015controlled,butterworth2013bios,han2018bad} and GPU isolation designs~\cite{volos2018graviton,jang2019heterogeneous} treat them as potentially adversarial. With its module intact, a single compromised server host can still mount at least five classes of attacks against semi-honest trusted acceleration (\cref{fig:scenarios}):
(i)~\emph{additive attacks}, which add an error to a value share, an opened masked input or a GPU matrix product; the error propagates undetected, biases the result, and, when later behavior depends on whether the shifted value crosses a comparison threshold, leaks secret bits through selective failure;
(ii)~\emph{replay and reset}, which resubmit an old mask, counter or key request, or restart the module and resume old state; reusing one mask $r$ for two openings $x+r$ and $x'+r$ already reveals $x-x'$;
(iii)~\emph{check-to-use substitution}, which modifies a DMA buffer after it has been checked but before it is consumed;
(iv)~\emph{oracle abuse}, which submits a value computed arbitrarily on the GPU to a naive ``authenticate'' interface and obtains valid MAC tags for it, turning the trusted dealer into a forgery oracle; and
(v)~\emph{premature release}, which requests a gate output before any check has completed.
Remote attestation does not close these gaps. It proves which code and configuration run inside the module; it does not prove that the untrusted GPU used a valid key, computed the right product, or released an authorized result. Likewise, a valid MAC on an incorrectly generated multiplication triple does not make the triple correct.

\textbf{Why existing malicious routes are costly.}
FSS can be made maliciously secure, but the known routes give back much of what trusted acceleration gained. Dealer-based actively secure FSS inference, as in Shark~\cite{gupta2025shark}, keeps an external dealer that ships authenticated keys and correlated randomness to both parties. Our model of a dealer-based pipeline in this protocol family (\cref{app:model}) estimates \est{37.6~GB} of offline material per BERT-Base query, \est{2.2$\times$} the semi-honest 17.1~GB~\cite{dfa2026trusted}, and a LAN latency of \est{43.9~s} of which \est{37.6~s} is distribution. Dealer-free malicious preprocessing in the SPDZ family~\cite{damgard2012spdz,keller2016mascot,keller2018overdrive,cramer2018spdz2k} replaces the dealer by oblivious-transfer or homomorphic-encryption based triple generation whose communication typically far exceeds that of the online phase. Verifiable FSS~\cite{decastro2022vfss} lets servers check that client-generated DPF keys are well formed, but a well-formed key does not force an untrusted GPU to return its correct evaluation, nor does it cover the arithmetic around the gate. The direct way to authenticate an FSS output inside an accelerator, one additional DPF tree with payload $\Delta_j\beta$ per MAC lane, multiplies pseudorandom generator (PRG) work by $(1+t)$, that is, $4\times$ for the $t=3$ lanes we use over a 61-bit field; our throughput model gives \est{26.7} instead of \est{106}~M gates/s for 61-bit inputs. Enclave-based designs either run the whole protocol on the CPU (Aramis~\cite{kumar2020cryptflow}) or verify only outsourced linear layers with Freivalds' test~\cite{freivalds1977probabilistic} (Slalom~\cite{tramer2018slalom}).

\textbf{Our key insight} is that a module that already plays the FSS dealer can also be the verifier. The trusted module knows every correlation it generates. It can therefore (1)~generate \emph{authenticated} correlations (input masks, Beaver triples~\cite{beaver1991efficient} and DPF keys) locally at zero network cost, computing every triple product correctly inside its own boundary; (2)~authenticate its own FSS outputs with a fresh resharing epilogue instead of extra DPF trees, because it already holds the raw output shares and the MAC key material; and (3)~check every opening on bytes it has frozen before any challenge exists, so that the GPU remains a fast but untrusted linear-algebra engine whose results are only candidates until verified. What must be protected is thus not a single primitive but an integrity chain:
\begin{center}
\small
\emph{authorized input} $\rightarrow$ \emph{correlated preprocessing} $\rightarrow$ \emph{correct local evaluation} $\rightarrow$ \emph{authenticated arithmetic} $\rightarrow$ \emph{consistent opening} $\rightarrow$ \emph{authorized output release.}
\end{center}
Each link has a concrete failure mode under a malicious host, and each needs its own mechanism. \Cref{fig:flows} places the resulting execution flow next to the semi-honest GPU baseline, trusted DFA and dealer-based malicious FSS.

\textbf{This work.}
We present \sys (Verified Integrity-Gated On-demand Randomness DFA), the malicious-secure successor of trusted DFA. It keeps DFA's placement beside the GPU L2 cache, its local key generation and its generate-and-consume execution. In our main setting, \ProfT, each computing party $P_b$ consists of an untrusted host (CPU, operating system, driver, runtime, GPU SMs and memory, NIC) and a protected module $T_b$; a probabilistic polynomial-time adversary statically corrupts at most one host, which may deviate arbitrarily, abort, delay or replay. Every secret value on a host or GPU is an authenticated share over $\Fp$, $p=2^{61}-1$, with $t=3$ independent SPDZ-style MAC lanes~\cite{damgard2012spdz,damgard2013practical}, or 32 bytes per element per party. Three mechanisms carry the design; we claim their composition, not any of them as an unprecedented primitive. The \emph{fresh authentication epilogue} turns a raw DPF output share $\tilde{y}_b$ into $y_b=\tilde{y}_b+(-1)^b\zeta$ and $\gamma_{b,j}=\Delta_j y_b+(-1)^b\kappa_j$ with fresh joint pads, at three field multiplications and four pads per output, and no command authenticates a host-supplied value. \emph{Freeze-before-challenge} \CheckOpen{} derives independent per-lane challenges only after both modules have frozen the exact submitted bytes, and later consumes exactly those bytes. A \emph{role-bound one-time ledger} labels all randomness by session, epoch, gate and purpose and poisons the epoch on any failure, and its \emph{release guard} lets no output leave a module before the corresponding check is \lstate{VERIFIED}.

\textbf{Scope and limits.}
\sys relocates trust to the modules rather than removing it. Under \ProfT the modules see inputs, so we also evaluate a direct protected gate as a legitimate competitor and let a cost-aware compiler choose among direct, lookup-table and interval FSS gates. Physical attacks (probing, fault injection, power and electromagnetic analysis) and rollback without a trusted monotonic service are outside our theorem, and security holds with abort, without fairness. Where the hardware itself is adversarial, \ProfU is a separate backend that runs the circuit on an established malicious 2PC protocol with the accelerator confined to party-local data. Finally, once the epilogue removes tag trees, the dominant cost of malicious security moves from DPF to four-lane authenticated linear algebra on the GPU and to the doubled round count (\cref{sec:analysis}).

This paper makes the following contributions:
\begin{itemize}[leftmargin=*]
    \item \textbf{Malicious Threat Analysis.}
    We systematize how a malicious host or GPU attacks semi-honest trusted FSS acceleration into eight scenarios, S1 to S8 (\cref{fig:scenarios}), from share tampering and forgery-oracle requests to check-to-use buffer swaps and PIR snapshot substitution. For each we show why semi-honest trusted DFA fails and which \sys mechanism and theorem stop it (\cref{tab:scenarios}), and we make explicit which deviations, input substitution and selective abort, the ideal functionality permits.

    \item \textbf{Protocol Co-Design.}
    We specify the authenticated $\Fp$ representation, the fresh authentication epilogue, freeze-before-challenge \CheckOpen{} with independent per-lane challenges, the one-time ledger and release guard, and malicious generate-and-consume with explicit generator and evaluator states (\cref{sec:protocol}). On top of them we build authenticated lookup-table, interval, polynomial and direct protected gates, exact comparison and truncation, a refactoring rule that preserves the joint (not only the marginal) distribution of DFA's decoupled preprocessing, and versioned-snapshot PIR.

    \item \textbf{Hardware Architecture.}
    We design a protected datapath beside the GPU L2 cache (\cref{sec:arch}) with a frame parser, ledger, page freezer, joint PRF sampler, DPF generation and evaluation contexts, a 128-lane Mersenne-61 field unit array, a check engine, AEAD spill and a release guard, whose 64 AES engines are time-shared among PRG expansion, challenge derivation and AEAD freezing. The additions cost \est{0.145~mm$^2$} and \est{0.508~W} at 7~nm, and the entire \sys occupies \est{0.046\%} of the A100 die.

    \item \textbf{Security Analysis.}
    We give ideal functionalities with explicit leakage and a hybrid proof with an explicit simulator of static malicious security with abort (\cref{sec:security}, \cref{thm:main}), with advantage at most $\eps{setup}+\eps{prf}+\eps{channel}+\eps{bind}+\eps{trace}+Q(2/p)^t$, where the last term is about $2^{-148}$ for $Q\le 2^{32}$ checked batches. We show why shared challenges across lanes and the ring $\Z_{2^{64}}$ break this bound, and we separate what is proved from the implementation obligations that remain (\cref{tab:obligations}).

    \item \textbf{Evaluation.}
    With an analytical model calibrated on DFA (\cref{sec:eval}, \cref{tab:e2e}), we estimate that \sys is \est{11.4$\times$} faster than dealer-based malicious FSS for BERT-Base on a LAN and \est{43.7$\times$} faster at 0.1~GB/s, and that it cuts offline communication from \est{37.6~GB} to \est{under 1~MB} per query. Malicious security costs \est{2.7$\times$} LAN latency over semi-honest trusted DFA for BERT-Base, yet \sys stays \est{4.3--6.1$\times$} faster than the semi-honest GPU-only pipeline across four models, and it keeps \est{0.93$\times$} of DFA's PIR throughput while adding integrity. A CPU reference model of every algorithm passes 22 unit tests with no failures, covering 21,840 exhaustive small-domain DPF cases, 2,728 generate-and-consume equivalence comparisons, 1,364 DCF comparisons and 20,004 checks of the GPU Mersenne multiplication.
\end{itemize}

Throughout, red values are estimates of our analytical model (\cref{app:model}) that await measurement; black values are reproduced from DFA~\cite{dfa2026trusted}, are analytical parameters, or come from executed reference tests.

The rest of this paper is organized as follows. \Cref{sec:bg} reviews FSS, private inference, PIR, trusted DFA and the malicious-security toolbox. \Cref{sec:threat} defines the threat model, the malicious scenarios and the security goal, and \cref{sec:analysis} analyzes where the cost of malicious FSS goes. \Cref{sec:protocol,sec:arch,sec:security} present the \sys protocol, its architecture and its security analysis. \Cref{sec:eval} evaluates \sys, \cref{sec:discussion} discusses its limitations, \cref{sec:related} surveys related work, and \cref{sec:conclusion} concludes. The appendices give the ideal functionalities, the full proofs and the performance model.


==> qa/draft1/sections/02_background.tex <==
% ==================================================================
% Section II: Background
% Owner labels: sec:bg, sec:bg-fss, sec:bg-pi, sec:bg-pir, sec:bg-dfa,
%               sec:bg-mal, fig:flows, eq:dpf, eq:pir
% ==================================================================
\section{Background}
\label{sec:bg}

This section reviews the primitives that \sys builds on and the semi-honest DFA design~\cite{dfa2026trusted} that it extends.
We write $P_0,P_1$ for the two computing parties, $b\in\{0,1\}$ for a party index, $\lambda$ for the seed length of the pseudorandom generator (PRG), and $\one[\cdot]$ for the indicator of a predicate.

% ==================================================================
\subsection{Function Secret Sharing, DPF, and DCF}
\label{sec:bg-fss}

\textbf{Function secret sharing.}
A two-party function secret sharing (FSS) scheme~\cite{boyle2015fss,boyle2016function} for a function class $\mathcal{F}$ with output group $\mathbb{G}$ consists of $\Gen(1^\lambda,\hat f)$, which maps a description of $f\in\mathcal{F}$ to a key pair $(k_0,k_1)$, and $\Eval(k_b,x)$, which returns party $b$'s share $y_b\in\mathbb{G}$.
Correctness requires $\Eval(k_0,x)+\Eval(k_1,x)=f(x)$ for every $x$; security requires that each key alone be simulatable from public information (domain, output group, function class), so that a single key hides $f$.

\textbf{Distributed point function.}
A distributed point function (DPF)~\cite{gilboa2014distributed,boyle2015fss,boyle2016function} shares the point function $f_{\alpha,\beta}$ with target $\alpha\in\bits{n}$ and payload $\beta\in\mathbb{G}$:
\begin{equation}\label{eq:dpf}
\Eval(k_0,x)+\Eval(k_1,x)=\beta\cdot\one[x=\alpha]\quad\text{for all } x\in\bits{n}.
\end{equation}
In this paper $\mathbb{G}=\Fp$ with $p=2^{61}-1$ (\cref{sec:proto-repr}), inputs are read most-significant bit first, and we use the tree-based construction of Boyle et al.~\cite{boyle2016function}.
Each node of a depth-$n$ binary tree carries a state $(s,t)$ of a $\lambda$-bit seed and a control bit; a fixed PRG $\PRG:\bits{\lambda}\rightarrow(\bits{\lambda}\times\bits{})^2$ expands a seed into the states of its two children, and $\Conv:\bits{\lambda}\rightarrow\Fp$ converts a leaf seed into a field element.
Generation walks the target path from two independent root seeds with control bits $t_0=0$ and $t_1=1$; at level $i$ it emits a correction word $\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$ that makes both parties' states identical on the child leaving the path and keeps them pseudorandom with opposite control bits on the child staying on it; an output correction $\CWout$ programs the payload so that the signed outputs $y_b=(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$ sum to $\beta$ at $x=\alpha$ and cancel elsewhere.
Party $b$'s key holds its root seed, its fixed control bit $t_b^{(0)}=b$, the $n$ level correction words, and $\CWout$, i.e., $O(\lambda n)$ bits.
\Cref{sec:analysis-dpf} gives the exact algorithms (\cref{alg:gen,alg:eval}).

\textbf{Evaluation patterns and cost.}
Generation expands two states per level ($2n$ PRG expansions); a single-path $\Eval(k_b,x)$ expands $n$ states; a full-domain $\EvalAll(k_b)$ expands $2^n-1$ internal nodes, and a depth-first traversal keeps only $O(n)$ pending siblings.
All patterns are dominated by the PRG, which DFA, GPU-DPF~\cite{lam2023gpu}, and \sys instantiate with AES-128.
Two properties matter later.
First, keys are \emph{one-time}: a key encodes the mask of one gate instance or the index of one query, and reusing a mask exposes the difference of two masked inputs.
Second, DPF key privacy holds for \emph{arbitrary} $(\alpha,\beta)$~\cite{boyle2016function}; uniform targets come from the application protocol, which masks an input with a uniform value (\cref{sec:bg-pi}), and any refactoring of generation must preserve that application-level distribution (\cref{sec:bg-dfa}).

\textbf{Distributed comparison function.}
A distributed comparison function (DCF) shares $f^{<}_{\alpha,\beta}(x)=\beta\cdot\one[x<\alpha]$.
We use this ``$<$'' orientation throughout; DFA~\cite{dfa2026trusted} uses ``$>$'', and we convert explicitly at interfaces via $\beta\cdot\one[x>\alpha]=\beta-f^{<}_{\alpha+1,\beta}(x)$, treating the threshold $2^n$ as a public constant.
Optimized DCFs evaluate with $O(n)$ PRG expansions~\cite{boyle2021function}, and DCFs can be assembled from DPFs~\cite{storrier2023grotto}.
For its proofs, \sys uses a conservative construction that sums $n$ independent prefix DPFs, with target $\alpha_1\cdots\alpha_{i-1}0$ and payload $\beta\cdot\alpha_i$ for prefix length $i$ (\cref{alg:dcf,thm:dcf}); it costs $n(n+1)/2$ path expansions, i.e., $O(n^2)$, and optimized DCFs are reported only as a projection that \cref{thm:dcf} does not cover.

% ==================================================================
\subsection{FSS-Based Private Inference}
\label{sec:bg-pi}

\textbf{Two-party secure inference.}
Private inference runs a neural network with private input, and possibly private weights, as a secure two-party computation~\cite{yao1986generate,goldreich2019play,mohassel2017secureml,rathee2020cryptflow2,crypten2020,tan2021cryptgpu,watson2022piranha}.
With additive shares $x=x_0+x_1$, linear operations are local, and a multiplication consumes a Beaver triple $(a,b,c=ab)$~\cite{beaver1991efficient}: the parties open $d=x-a$ and $e=y-b$ and locally compute shares of $xy=c+db+ea+de$.
Nonlinear layers (ReLU, GeLU, Softmax, LayerNorm) dominate the cost; earlier systems use multi-round Boolean conversions for them~\cite{demmler2015aby,mohassel2018aby3,wagh2019securenn,wagh2020falcon}.

\textbf{Masked-input FSS gates.}
FSS-based systems~\cite{boyle2021function,ryffel2020ariann,wagh2022pika,gupta2023sigma,jawalkar2024orca} evaluate each nonlinear gate $g$ in the masked-input paradigm.
Offline, a dealer samples a fresh uniform mask $r$, shares it, and generates FSS keys for the offset function $g_r(c)=g(c-r)$, often with an output mask.
Online, the parties open $c=x+r$, which is uniform and independent of $x$, and the outputs $\Eval(k_b,c)$ are shares of $g(x)$.
Comparisons and ReLU use DCFs, spline approximations of GeLU, exponentials, and inverse square roots use DCF-based interval selection plus low-degree polynomials, and small lookup tables use DPFs~\cite{gupta2023sigma,jawalkar2024orca}.
Each gate costs one opening round, so the online phase is round-efficient but compute-intensive.

\textbf{Offline cost and the dealer assumption.}
The price is paid offline.
Semi-honest FSS inference of BERT-Base with 128 tokens moves 17.1\,GB of one-time key material per query and LLaMA2-7B moves 256\,GB, more than 90\% of it DPF keys~\cite{dfa2026trusted}; this cost cannot always be hidden behind online work, and its energy and monetary cost is never hidden~\cite{huang2026beyond}.
Sigma, Orca, and related systems~\cite{gupta2023sigma,jawalkar2024orca,crypten2020} obtain keys from a trusted dealer and assume semi-honest computing parties.
A deviating party can shift its share of $c$ by an arbitrary $e$, so that the gate silently evaluates $g(x+e)$, or add an arbitrary error to its output share; for comparisons, whether $x+e$ crosses a threshold then shapes later behavior and can leak through selective failure.

% ==================================================================
\subsection{DPF-Based Private Information Retrieval}
\label{sec:bg-pir}

PIR lets a client retrieve record $D[\alpha]$ of an $N$-record database $D$ without revealing $\alpha$~\cite{chor1998private}.
Single-server schemes rely on homomorphic encryption and are computationally heavy~\cite{angel2018pir,henzinger2023one}; we focus on the faster two-server DPF-based schemes~\cite{gilboa2014distributed,boyle2016function}.
With $n=\lceil\log_2 N\rceil$, the client sends $k_b$ of $(k_0,k_1)\leftarrow\Gen(1^\lambda,\alpha,1)$ to server $P_b$, which returns
\begin{equation}\label{eq:pir}
y_b=\sum_{x=0}^{N-1}\Eval(k_b,x)\cdot D[x],\qquad b\in\{0,1\},
\end{equation}
and by \cref{eq:dpf} the client obtains $D[\alpha]=y_0+y_1$.
Keys have $O(\lambda\log N)$ bits, but each query costs $O(N)$ PRG expansions plus an $N$-term inner product per server, and the expansion dominates even on GPUs~\cite{lam2023gpu}.
The same full-domain pattern underlies anonymous messaging, private analytics and search, and distributed ORAM~\cite{corrigan2015riposte,wang2017splinter,boneh2021lightweight,dauterman2020dory,dauterman2022waldo,doerner2017scaling,vadapalli2023duoram}.
Standard DPF-based PIR protects the index but not the answer: a malicious server can add an offset $\delta$ to $y_b$, so that the client accepts $D[\alpha]+\delta$, or answer from a stale database.
Conversely, a malicious client can submit a malformed key pair that reconstructs a combination of several records, which verifiable DPFs detect~\cite{decastro2022vfss}.
Authenticated PIR~\cite{colombo2023apir} lets the client verify answers against a database digest at additional server cost; \cref{sec:proto-pir} gives our protected versioned-snapshot design.

% ==================================================================
\subsection{Trusted DFA}
\label{sec:bg-dfa}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_flows.pdf}
    \caption{Execution flows of two-party FSS-based private inference in four configurations, from left to right.
    (1)~GPU without DFA (semi-honest): a trusted party generates FSS keys in an offline phase and ships them over the network, and each party stores them, reads them back, and transfers them to its GPU.
    (2)~Trusted DFA (semi-honest)~\cite{dfa2026trusted}: after a one-time initialization with attestation and key exchange, each on-die module generates its party's keys locally and merges generation with evaluation (generate-and-consume), which removes the offline phase.
    (3)~Dealer-based malicious FSS: the dealer additionally issues authenticated keys and authenticated triples, so larger offline material leaves the dealer and must be stored and reread, while the GPU runs authenticated GEMM and checks MACs online.
    (4)~\sys (malicious): the protected module (red dashed trusted boundary) keeps local generation and generate-and-consume, adds the fresh authentication epilogue, freeze-before-challenge \CheckOpen, and the release guard, and exchanges authenticated shares $\authb{x}{b}$ with a GPU that runs authenticated linear algebra on one value lane and three MAC-tag lanes; the inter-party network carries opened values and check residuals instead of keys.}
    \label{fig:flows}
\end{figure*}

\textbf{Hardware.}
DFA~\cite{dfa2026trusted} integrates 16 DPF units with four pipelined AES-128 engines each (64 in total) next to the L2 slices of a GPU; each 20-stage unit sustains one Gen or Eval iteration per cycle after warm-up.
A Cortex-M3-class security core~\cite{st33tpm12spi,arm_cortex_m3} handles attestation and key management, and a 16-lane vector unit~\cite{cavalcante2019ara} runs protocol-specific pre- and post-processing.
The design runs at 720\,MHz in 28\,nm, delivers about 290\,GB/s of DPF output in Accel-Sim~\cite{khairy2020accel}, and traverses full-domain trees depth-first, needing $O(nm)$ state for $m$ units instead of $O(2^n)$~\cite{dfa2026trusted}.

\textbf{Untrusted and trusted modes.}
In the \emph{untrusted mode}, DFA only expands seeds for keys produced elsewhere, and the protocol is unchanged.
In the \emph{trusted mode}, each party's module replaces the dealer: the modules attest to each other and establish a key $K$ that the hosts never see, derive the same generation coins (including $\alpha$) from $K$ and a counter, and thus compute identical correction words while each evaluates only its own party's share.
\emph{Generate-and-consume} (GaC) runs the joint generation and the local evaluation in lockstep, consuming each correction word as soon as it is produced, so that neither key distribution nor key storage remains.
DFA also \emph{decouples} generation from protocol preprocessing: when the target is $a=g(r)$ for a bijection $g$, the module samples $a$ uniformly and recovers $r=g^{-1}(a)$.
For BERT-Base, trusted DFA reduced the per-query LAN latency from 18.8\,s to 1.42\,s and the offline communication from 17.1\,GB to 0.1\,GB, and for PIR over $2^{20}$ records it raised the throughput from 3{,}480 to 17{,}580 queries/s~\cite{dfa2026trusted}; these results combine measured GPU executions with cycle-level simulation of DFA.
\Cref{fig:flows} contrasts this flow with the GPU-only baseline and with the two malicious-secure designs compared in this paper.

\textbf{The semi-honest boundary.}
DFA argues that, as long as key generation inside the module is correct, the protocol is the baseline semi-honest protocol and the online threat model is unchanged.
Against a deviating host, four aspects of the semi-honest design must be revisited.
(i)~\emph{Joint distributions:} since DPF privacy does not need uniform targets, decoupling must preserve the application's \emph{joint} distribution of the target and all auxiliary values derived from the same mask, not only uniform marginals; a gate that uses targets $r$ and $r+1$ loses a required correlation if they are resampled independently (\cref{sec:proto-refactor}).
(ii)~\emph{Explicit state:} the simplified algorithms leave the root control-bit relation, the payload and role inputs, and the separation of generator and evaluator control state implicit, whereas a malicious-security proof needs them explicit (\cref{alg:gen,alg:eval,alg:gac}).
(iii)~\emph{Attestation is not verification:} attestation authenticates a module's implementation and configuration; it does not prove that an untrusted GPU used a valid key, computed the right product, or released an authorized result, and a valid MAC on an incorrectly generated triple does not make the triple correct.
(iv)~\emph{The boundary excludes the GPU:} the SMs and GPU memory are untrusted, so the GPU must never compute an unchecked result and ask the module to authenticate it, which would turn the module into a forgery oracle (\cref{sec:threat-scenarios}).

% ==================================================================
\subsection{Tools for Malicious Security}
\label{sec:bg-mal}

\textbf{Security with abort.}
We use the real/ideal simulation paradigm~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}.
A malicious adversary deviates arbitrarily; security with abort requires that it achieve nothing beyond an ideal world in which a trusted functionality computes the result and the adversary only chooses corrupted inputs and whether honest parties receive output, so fairness is not required.
Covert security~\cite{aumann2007covert} only deters cheating; we target full malicious security with abort.

\textbf{Information-theoretic MACs.}
SPDZ-style protocols~\cite{damgard2012spdz,damgard2013practical} authenticate each value of a field $\F$ under a global key $\Delta=\Delta_0+\Delta_1$ that no single party knows.
Party $b$ holds $\Delta_b$ and $\authb{x}{b}=(x_b,\gamma_b)$ with $x_0+x_1=x$ and $\gamma_0+\gamma_1=\Delta x$; linear operations act identically on values and tags, and multiplications consume authenticated triples.
To check openings $z_1,\dots,z_m$, the parties draw coefficients $\rho_i$ \emph{after} the values are fixed, compute $\sigma_b=\sum_i\rho_i(\gamma_{b,i}-\Delta_b z_i)$, and accept only if $\sigma_0+\sigma_1=0$.
A wrong opening passes only if its tag error matches $\Delta$ times the value error or cancels under the coefficients, which happens with probability less than $2/|\F|$.
Over $\Fp$ with $p=2^{61}-1$, one tag gives about $2^{-60}$ per check and only $2^{-28}$ over $Q=2^{32}$ checks, so \sys uses $t=3$ independent keys and challenge vectors to reach $Q(2/p)^t\approx2^{-148}$ (\cref{sec:proto-repr,sec:sec-concrete}).
Over $\Z_{2^{64}}$ the argument fails because zero divisors break its division step; SPDZ2k~\cite{cramer2018spdz2k} works over $\Z_{2^{k+s}}$ with its own analysis.

\textbf{Authenticated preprocessing.}
Malicious protocols need authenticated masks and triples whose relations, such as $c=ab$, are actually correct.
Generating them without a trusted party is communication-heavy, whether with oblivious transfer in MASCOT~\cite{keller2016mascot} or with somewhat homomorphic encryption in SPDZ and Overdrive~\cite{damgard2012spdz,keller2018overdrive}, all available in MP-SPDZ~\cite{keller2020mpspdz}.
Pseudorandom correlation generators~\cite{boyle2019pcg,boyle2020pcg} compress this communication at a substantial computational cost, and a trusted dealer avoids generation but ships every authenticated share.

\textbf{Malicious and verifiable FSS.}
Malicious FSS gates additionally need well-formed keys and authenticated evaluation outputs that can enter MAC-checked arithmetic.
Verifiable FSS~\cite{decastro2022vfss} lets evaluators check that a key pair shares a function of the declared class, but it does not verify the evaluation that a malicious party performs on its own key.
Shark~\cite{gupta2025shark} achieves active security for FSS-based inference with a dealer that issues authenticated FSS keys and correlated randomness, which enlarges the offline material relative to semi-honest FSS.
A direct way to authenticate a DPF output is a second \emph{tag tree} per MAC key, a DPF with payload $\Delta_j\beta$ whose outputs share $\Delta_j\beta\cdot\one[x=\alpha]$; with $t$ lanes this multiplies DPF work by $1+t$ (\cref{sec:analysis-work}).

\textbf{Trusted hardware for secure computation.}
Tamper-proof hardware tokens enable universally composable secure computation~\cite{katz2007universally}.
Aramis in CrypTFlow~\cite{kumar2020cryptflow} runs each party's semi-honest protocol inside an SGX enclave~\cite{costan2016intel} and relies on enclave integrity for malicious security, placing the whole party, linear algebra included, in the trusted computing base (TCB).
Slalom~\cite{tramer2018slalom} outsources linear layers from a TEE to an untrusted GPU and verifies them with Freivalds' algorithm~\cite{freivalds1977probabilistic}, which \sys uses only for a restricted subroutine (\cref{sec:proto-freivalds}).
PPMLAC~\cite{zhou2022ppmlac} and STAMP~\cite{huang2022efficient} accelerate semi-honest MPC with small trusted modules (\cref{sec:related}).

\textbf{Implications.}
Malicious security for trusted FSS acceleration must protect the complete integrity chain: authorized input $\rightarrow$ correlated preprocessing $\rightarrow$ correct local evaluation $\rightarrow$ authenticated arithmetic $\rightarrow$ consistent opening $\rightarrow$ authorized output release.
Each tool above covers only part of it, at a cost that erodes the advantage of trusted DFA: shipped or MASCOT-generated authenticated preprocessing reintroduces the offline traffic that trusted DFA removed, tag trees multiply DPF work, key verification leaves evaluation unchecked, and attestation leaves the GPU unchecked.
\sys therefore keeps the module as the dealer and also makes it the verifier (\cref{sec:protocol}).

\textbf{Scope.}
Throughout this paper, \emph{private inference} means two-party FSS-based private inference and \emph{PIR} means two-server DPF-based PIR, as in DFA~\cite{dfa2026trusted}.


==> qa/draft1/sections/03_threat_model.tex <==
% ==================================================================
% Section III: Threat Model and Security Goals
% Owner labels: sec:threat, sec:threat-model, sec:threat-scenarios,
%   sec:threat-goals, sec:threat-profileu, fig:threat, fig:scenarios,
%   tab:scenarios, fig:func, def:security, def:leakage
% ==================================================================
\section{Threat Model and Security Goals}\label{sec:threat}

The trusted mode of DFA moved the FSS dealer into a small protected module, but it kept the semi-honest model of the protocols it accelerates~\cite{dfa2026trusted}. This section states precisely what changes when a host is malicious. We fix the system model and the trust boundary (\cref{sec:threat-model}) and the adversary, derive ten scenarios in which a corrupted host attacks a trusted FSS accelerator (\cref{sec:threat-scenarios}), define security with explicit leakage (\cref{sec:threat-goals}), and delimit the stronger \ProfU (\cref{sec:threat-profileu}). Throughout, the object of protection is not a single primitive but the integrity chain
\emph{authorized input $\rightarrow$ correlated preprocessing $\rightarrow$ correct local evaluation $\rightarrow$ authenticated arithmetic $\rightarrow$ consistent opening $\rightarrow$ authorized output release}.
Every link of this chain crosses memory, buses, or network paths that a corrupted host controls, and each link can be broken independently of the others.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_threat.pdf}
    \caption{System model and trust boundary of \sys under \ProfT. Each computing party $P_b$ consists of an untrusted host (CPU, OS, driver, runtime, NIC, DRAM) with its GPU (SMs, HBM), and a protected module $T_b$ (red dashed TCB) that holds the session keys, the one-time ledger, the joint PRF sampler, the DPF generate-and-consume datapath, the authentication epilogue, the freeze and check engine, and the release guard. The adversary statically corrupts at most one host (here the host of $P_0$, red region) and may deviate arbitrarily, replay, and abort; it never corrupts $T_0$ or $T_1$. Hosts and GPUs hold only party-local authenticated shares; the modules talk to each other over a protected peer channel and to the client over authenticated confidential channels, all carried by the untrusted network.}
    \label{fig:threat}
\end{figure*}

\subsection{System Model and Trust Boundary}\label{sec:threat-model}

\textbf{Parties.}
\sys targets the two workloads of DFA~\cite{dfa2026trusted}: two-party FSS-based private inference and two-server DPF-based PIR (\cref{sec:bg}). Two computing parties $P_0$ and $P_1$ serve an external client that owns private inputs and receives outputs; a computing party may also own an input, typically the model weights. As shown in \cref{fig:threat}, each $P_b$ consists of an untrusted \emph{host~$b$} (CPU, operating system, driver, GPU runtime, GPU SMs and caches, HBM and DRAM, DMA engines, NIC, and storage) and a \emph{protected module} $T_b$, the \sys extension placed next to the GPU L2 as in DFA (\cref{sec:arch-hw}).

\textbf{Trusted computing base.}
$T_b$ contains the session and identity (attestation) keys; the joint-sampler key and the global MAC keys $\Delta_1,\dots,\Delta_t$; the session role and counters; the one-time resource ledger; the DPF generator and evaluator states and the correction words; the protected table and reduction logic; the frozen check buffers, challenges, and residuals; and all release decisions. Everything else is outside, including every GPU and DMA buffer and every byte in transit between the parties. The host schedules the public circuit, and the GPU performs the authenticated linear algebra on party-local arrays (one value lane and $t$ tag lanes) and hands each result to $T_b$ as a \emph{candidate} share $\authb{x}{b}=(x_b,\gamma_{b,1},\dots,\gamma_{b,t})$, i.e., 32 bytes per element and party for $t=3$ (\cref{sec:proto-repr}). Host~$b$ may know its own MAC key shares $\Delta_{b,j}$, but no host ever holds a complete $\Delta_j$, the joint-sampler key, a complete mask, the peer's shares, or any challenge or residual.

\textbf{Modules as an ideal resource.}
Following the treatment of tamper-proof hardware as an ideal functionality~\cite{katz2007universally}, we model $T_0$ and $T_1$ as an explicit ideal resource $\mathcal{F}_T$ (\cref{app:func-module}): their code, keys, input parser, arithmetic, state transitions, local memory, protected peer channel, and approved I/O paths are correct and confidential, and their externally observable traces are simulatable from the prescribed local view and public metadata. This restates DFA's trusted-mode assumption in a form that a simulation proof can use (\cref{sec:sec-assump}); availability is not assumed. \ProfT requires two physically independent modules, one per party. The on-die design (\cref{sec:arch-hw}) is our target; the ZCU102 prototype (\cref{sec:arch-deploy}) is a functional and streaming prototype and does not by itself realize $\mathcal{F}_T$, since, for example, an ordinary process on its ARM cores is not isolated from a malicious board administrator.

\textbf{Channels.}
The client reaches $T_0$ and $T_1$ over authenticated confidential channels that terminate inside the modules. The modules share a protected peer channel (AEAD with independent directional keys and no nonce reuse), established by an authenticated session setup that binds the ordered identities, roles $0$ and $1$, a fresh session identifier and epoch, the manifest hash, the field and tag parameters, and the protocol version (\cref{sec:proto-setup}). The untrusted hosts and network carry this traffic, observe its lengths and timing, and can drop, delay, or reorder it. We propose no new attestation or key-exchange protocol; the security of setup is the explicit assumption $\eps{setup}$.

\textbf{Trust is relocated, not removed.}
The two modules jointly act as the FSS dealer, and after a verified masked opening a module can recover the underlying input from the opening and its mask. \sys therefore does not claim that inputs are hidden from its trusted modules; it moves trust from an external dealer and from the hosts into two small modules (\cref{sec:discussion}).

\subsection{Adversary Model}

We consider a probabilistic polynomial-time (PPT) adversary $\Adv$ that statically corrupts at most one host before the session starts (host~$0$ in \cref{fig:threat}, by symmetry). Corruption is malicious: $\Adv$ controls the operating system, drivers, GPU kernels and their results, host and GPU memory including DMA buffers, and all outgoing network behavior of the corrupted party. Concretely, it can
(i) modify any value share or tag and run arbitrary kernels in place of the prescribed ones;
(ii) invoke its module's commands in any order with malformed, replayed, or mislabeled arguments;
(iii) rewrite any host-visible buffer at any time, including while the module reads it;
(iv) replay, reorder, delay, or drop messages, reset its platform, and restore old host-side state;
(v) choose the inputs it owns arbitrarily; and
(vi) abort at any point, including after it has learned its own output.
It observes message lengths and timing, the frames exchanged with its module, and the module's external trace. The principal inference statement assumes an honest external client and gives no guarantee against client-server collusion; for PIR we separately consider a malicious client with two honest server hosts (\cref{sec:threat-goals}).

\textbf{Out of scope.}
Our theorems exclude corruption of either module (its code, keys, state, or arithmetic); physical attacks such as microprobing, fault injection including undervolting, and power or electromagnetic analysis~\cite{skorobogatov2017microprobing,murdock2020plundervolt,kocher1999differential,quadir2016survey}; leakage beyond the stipulated trace model; speculative-execution bugs inside the trusted boundary~\cite{van2018foreshadow}; faulty trusted arithmetic; adaptive corruption; and corruption of both hosts. Rollback of module state is covered only by the lifecycle rule of scenario S4 below. Availability and fairness are not provided.

\textbf{Why this model is stronger than DFA's.}
DFA~\cite{dfa2026trusted}, like Sigma~\cite{gupta2023sigma} and Orca~\cite{jawalkar2024orca}, assumes that both hosts run the prescribed kernels and feed the module the prescribed inputs. Under \ProfT the host controls every byte that the module reads or writes outside its boundary. Remote attestation proves which code runs inside the module; it does not prove that the GPU computed correctly, used a valid key, or released an authorized result. We target full malicious security with abort rather than covert security~\cite{aumann2007covert}, which tolerates a noticeable probability of undetected cheating.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_scenarios.pdf}
    \caption{Malicious scenarios S1 to S8 against trusted FSS acceleration and the \sys mechanism that stops each. In every panel the corrupted host or GPU is shaded red and the module $T_b$ is the red dashed TCB; red arrows with circled numbers are adversary actions, red crosses mark the point where \sys blocks them, and green text names the defense. Scenarios S9 (input substitution by a corrupt owner) and S10 (denial of service) are not attacks that the protocol can prevent; they are discussed in \cref{sec:threat-scenarios} and listed in \cref{tab:scenarios}.}
    \label{fig:scenarios}
\end{figure*}

\subsection{Malicious Scenarios Against Trusted FSS Acceleration}\label{sec:threat-scenarios}

\Cref{fig:scenarios} and \cref{tab:scenarios} list what a corrupted host can do to a trusted FSS accelerator designed for semi-honest hosts, and which \sys mechanism stops each action; the paragraphs below explain why the semi-honest design fails in each case. The scenarios follow the integrity chain: S9 targets the authorized input; S4 and S7 the correlated preprocessing; S2 and S5 the correct local evaluation; S1 the authenticated arithmetic; S3 the consistent opening; and S6 the authorized output release. S8 carries S3 over to the PIR database, and S10 targets availability, which lies outside the chain. \sys prevents S1 to S8 up to the error terms of \cref{thm:main}; S9 is permitted by the ideal functionality; S10 is not prevented. \Cref{sec:sec-scenarios,sec:eval-attack} map the scenarios to theorems and to injected tests.

\textbf{S1: Share and tag tampering.}
The corrupted GPU holds every intermediate share and can add an error $e$ to a value share (and $d_j$ to tags) at any wire. In a semi-honest trusted DFA the error flows unchecked into the masked opening $x+r$ of the next FSS gate. Besides biasing results, this additive attack causes \emph{selective failure}: whether $e$ flips a comparison depends on whether $x$ lies within $|e|$ of the threshold, so any observable change of the output leaks information about $x$. \sys checks every authenticated opening with \CheckOpen{} before a protected gate or a release consumes it. The outcome depends only on the adversary's own errors and fresh randomness inside the modules, not on honest data, and a wrong value passes with probability at most $(2/p)^t$ per batch (\cref{thm:mac-sound}). An error confined to one tag lane escapes with probability $1/p$, but it changes no opened value.

\textbf{S2: Forgery-oracle request.}
A tempting integrity extension of DFA's trusted mode is a command that tags a value computed elsewhere, for example a nonlinear output computed on the SMs. Such an \emph{authenticate(host value)} entry point turns the module into a MAC oracle: the host submits any $y^*$, and every later check accepts it. Attestation certifies the module's code, not the provenance of what it signs. \sys has no such command; its fresh authentication epilogue authenticates only results of the protected evaluator or of an explicitly verified backend (\cref{sec:proto-epilogue,thm:epilogue}).

\textbf{S3: Time-of-check-to-time-of-use buffer swap.}
The module reads its inputs by DMA from host-controlled memory. A design that verifies a buffer and later rereads it, or that trusts a host-reported digest, admits a time-of-check-to-time-of-use (TOCTOU) swap: the host changes the bytes after verification, or chooses its error after the challenge is fixed. Semi-honest DFA never faced this problem, and DMA completion is not evidence of authenticity. \sys freezes the exact bytes in protected SRAM or in AEAD-sealed immutable pages \emph{before} any challenge exists, and consumes only the frozen bytes (\cref{sec:proto-ledger,sec:proto-check}).

\textbf{S4: Replay and rollback.}
DFA derives keys and masks from the shared key $K$ and a counter that is an input of its generate-and-consume procedure~\cite{dfa2026trusted}. Replaying a counter yields the same mask $r$ for two gates, and the openings $x+r$ and $x'+r$ reveal $x-x'$; resetting the module and resuming an old session replays entire key streams. \sys binds every draw to (session, epoch, gate, purpose, logical draw, block), burns labels in a one-time ledger before any share is issued, and poisons the epoch on any failure (\cref{fig:ledger}). After a reboot it requires either a separately justified trusted monotonic service~\cite{parno2011memoir,matetic2017rote} or irrecoverable erasure of the old master key and a freshly attested session; a host-controlled counter file is not anti-rollback protection.

\textbf{S5: Role and gate confusion.}
The host decides which module command runs for which gate. It can route the preprocessing of gate $g$ into gate $g'$, alter a table hash or a tensor shape, or present party-$0$ material as party-$1$ material. If the role were a per-request argument, the host could obtain both parties' outputs of one joint draw and reconstruct the DPF target $\alpha$, which is exactly the mask of an honest input. \sys fixes the roles once per session in the authenticated setup and binds each gate's descriptor in the ledger; any mismatch aborts before preprocessing is issued (\cref{sec:proto-setup,sec:proto-ledger}).

\textbf{S6: Premature release.}
A semi-honest trusted DFA releases results as soon as they are computed. Under a malicious host, an early output may already be wrong, and the host may request it repeatedly or for a recipient other than the authorized one. The release guard of \sys keeps every output behind the \lstate{VERIFIED} state of its gate: candidate openings stay inside the modules until \CheckOpen{} accepts, releases carry bound certificates, and an epoch abort atomically gates all outstanding outputs.

\textbf{S7: Malformed preprocessing.}
A MAC authenticates values, not relations. A triple $(\auth{a},\auth{b},\auth{c})$ with $c\neq ab$ carries perfectly valid tags, and multiplying with it yields $xy+\delta$ for a $\delta$ chosen by its producer; the same holds for a matrix product $C=AB$ computed on an untrusted GPU and for a malformed DPF key. The attestation of DFA covers the module's own key generation, not correlations that come from elsewhere. \sys computes $c=ab$ (or $C=AB$) inside the TCB and authenticates each component independently; imported preprocessing needs authenticated shares \emph{and} a proof of correctness (\cref{sec:proto-arith}).

\textbf{S8: Snapshot substitution in PIR.}
The PIR database resides in host memory, so a corrupted server host can modify a record, serve an older version, or hash one buffer while scanning another. Semi-honest PIR, including DFA-accelerated PIR, returns whatever the servers compute. Worse, a record modified only at position $i$ corrupts the answer only when $\alpha=i$, so the client's reaction leaks the queried index. Each \sys module hashes the bytes it actually consumes, in a public order independent of $\alpha$, and quarantines its result until the hash matches the authorized versioned commitment; a substitution therefore aborts independently of $\alpha$ (\cref{sec:proto-pir,thm:pir}).

\textbf{S9: Input substitution by a corrupt owner.}
A corrupted party that owns an input, such as the model weights, may choose it freely. No protocol can prevent this, and $\FC$ permits it by extracting the chosen input from the owner's masked input (\cref{sec:proto-arith}). Binding a specific pre-approved model requires a commitment (see \emph{Model provenance} in \cref{sec:threat-goals}).

\textbf{S10: Denial of service and selective abort.}
The corrupted host can drop, delay, or reorder messages, or abort after learning its own output. Like SPDZ-style protocols~\cite{damgard2012spdz,keller2016mascot}, \sys provides security with abort, without fairness or guaranteed output delivery. It does prevent aborts from becoming a side channel on honest data: every abort outcome is either a declared validation outcome or a function of the adversary's own deviations and fresh randomness inside the modules, and both are covered by the permitted leakage (\cref{def:leakage}).

\begin{table*}[t]
\centering
\caption{Malicious scenarios against trusted FSS acceleration. The ``effect'' column describes a semi-honest trusted DFA~\cite{dfa2026trusted}, or a naive malicious extension of it, when one host is corrupted. \cmark: prevented up to the error terms of \cref{thm:main}; \pmark: permitted by the ideal functionality; \xmark: not prevented.}
\label{tab:scenarios}
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabularx}{\textwidth}{c >{\raggedright\arraybackslash}p{1.75cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{2.75cm}}
\hline
\textbf{ID} & \textbf{Scenario} & \textbf{Adversary action} & \textbf{Effect on semi-honest trusted DFA} & \textbf{\sys mechanism} & \textbf{Guarantee} \\
\hline
S1 & Share/tag tampering & GPU adds an error $e$ to a value share (and $d_j$ to tags) before an opening or FSS gate & Undetected; biases outputs and causes selective failure that leaks $x$ & Authenticated shares with $t=3$ MAC lanes over $\Fp$; \CheckOpen{} before any protected gate or release & \cmark\ Wrong value accepted w.p.\ $\le (2/p)^t$ per batch (\cref{thm:mac-sound}) \\
\hline
S2 & Forgery-oracle request & Host submits $y^*$ and asks its module to authenticate it & No MACs; a naive authenticate command would sign any forgery & No \emph{authenticate(host value)} command; \Epilogue{} only on internally computed or verified results & \cmark\ Request rejected; outputs correctly authenticated (\cref{thm:epilogue}) \\
\hline
S3 & TOCTOU buffer swap & Host rewrites a DMA buffer after it is checked, or after the challenge is fixed & Module trusts DMA reads; a later reread consumes modified bytes & Freeze before challenge: bytes copied or AEAD-sealed, frozen roots agreed, only frozen bytes consumed & \cmark\ Modification ignored or abort; binding error $\eps{bind}$ \\
\hline
S4 & Replay and rollback & Replays a counter or mask request; resets the module and resumes old keys & Mask reuse: $x+r$ and $x'+r$ reveal $x-x'$; key streams replayed & Labels bound to session, epoch, gate, purpose; one-time ledger; epoch poisoning; erase-and-rekey after reboot & \cmark\ Reuse rejected before any accepted use \\
\hline
S5 & Role/gate confusion & Routes party-0 material as party-1, or gate $g$ material into gate $g'$; alters shapes or table hash & Host schedule trusted; requesting both roles' outputs exposes the target $\alpha$ & Roles fixed by authenticated setup; gate descriptors bound in the ledger and in PRF labels & \cmark\ Mismatch aborts before preprocessing is issued \\
\hline
S6 & Premature release & Requests outputs before verification, repeatedly, or for another recipient & Results released as soon as computed & Release guard: nothing before \lstate{VERIFIED}; bound certificates; epoch abort gates pending outputs & \cmark\ No candidate value leaves the modules \\
\hline
S7 & Malformed preprocessing & Injects a triple with valid tags but $c\neq ab$, a GPU-computed $C=AB$, or a wrong DPF key & Attestation silent on external correlations; MACs verify wrong triples & Triples and keys generated inside the TCB ($c=ab$ computed there); imports need a correctness proof & \cmark\ Never consumed; exact arithmetic (\cref{thm:arith}) \\
\hline
S8 & Snapshot substitution (PIR) & Swaps records or version after hashing, or scans a different buffer & Client reconstructs a wrong record; index-dependent failure leaks $\alpha$ & Module hashes the bytes it consumes in public order; quarantine until the commitment matches & \cmark\ Committed record or abort (\cref{thm:pir}) \\
\hline
S9 & Input substitution by a corrupt owner & Corrupted party supplies arbitrary weights or inputs & Same (allowed) & Input extraction by $\FC$; optional commitment-bound loader for model provenance & \pmark\ Allowed by the functionality \\
\hline
S10 & Denial of service/ selective abort & Drops, delays, or reorders messages; aborts after learning its own output & Same (not prevented) & Bounded resources and abort; abort outcomes simulatable from permitted leakage & \xmark\ Not prevented (no fairness or availability) \\
\hline
\end{tabularx}
\end{table*}

\subsection{Security Goals and Ideal Functionalities}\label{sec:threat-goals}

\textbf{Goals.}
Against a corrupted host, \sys must provide \emph{privacy} (the host learns nothing beyond the permitted leakage and the outputs it is authorized to receive), \emph{correctness} (honest recipients obtain the circuit evaluated on the honest inputs and the corrupted party's extracted inputs, or abort), \emph{authorized release} (no value leaves the modules unless its opening was verified and bound to a release certificate), and \emph{one-time use} (no randomness is consumed twice). We formalize the first two in the stand-alone real/ideal paradigm with sequential composition~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}, using an explicit leakage function; the last two are mechanisms that the proof relies on (\cref{sec:proto-ledger}).

\textbf{Manifest.}
Every session fixes a public manifest $\mu$: the protocol version, session identities, roles, field, numeric encoding, the finite circuit $C$, gate and wire identifiers, tensor shapes, approved public tables, interval coefficients, authorized recipients, input validation rules, and the public batch schedule. Honest input ranges and intermediate numeric bounds are established statically from $\mu$ whenever possible.

\begin{definition}[Permitted leakage]\label{def:leakage}
For a circuit execution under manifest $\mu$, the permitted leakage is
\[
\Leak_C=\bigl(\mu,\ \mathsf{len},\ \mathsf{sched},\ \mathsf{pub},\ \mathsf{status}\bigr),
\]
where $\mathsf{len}$ are the lengths of all public messages; $\mathsf{sched}$ is the public schedule of batches, checks, and interaction boundaries fixed by $\mu$; $\mathsf{pub}$ are the values that $\mu$ designates as authorized public openings; and $\mathsf{status}$ are the specified abort and validation outcomes, including every input-dependent validity bit declared in $\mu$, which is never silently excluded. For PIR, $\Leak_{\mathrm{PIR}}$ consists of the public descriptor (database identifier, version, true and padded length, record encoding, and the authorized snapshot commitment), the public scan length and order, message lengths and schedules, and the accept, reject, or abort outcome.
\end{definition}

Nothing else is leaked: honest inputs, intermediate wire values, masks, MAC keys, DPF keys and correction words, raw FSS outputs, challenges, and residuals are not in $\Leak_C$. Masked openings such as $x+r$ are not leakage either; they are uniformly distributed given $\Leak_C$, and the simulator samples them (\cref{app:proof-main}). The timing and access pattern of the modules are fixed by $\mu$ (for example, full-domain scans have a declared fixed order), and any residual trace is covered by the trace assumption $\eps{trace}$.

\begin{figure}[t]
\centering
\footnotesize
\fbox{\begin{minipage}{\dimexpr\columnwidth-2\fboxsep-2\fboxrule\relax}
\centering\underline{Functionality $\FC$}\par\smallskip
\raggedright
\textbf{Parameters.} Public manifest $\mu$ (circuit $C$ over $\Fp$, input owners, validity predicates, authorized recipients, public schedule). Corrupted set $I$: at most one host; the client is honest.
\begin{enumerate}[leftmargin=*,nosep,topsep=2pt]
\item \textbf{Input.} Receive the authenticated input $x_w$ of every input wire $w$ from its designated owner. If the owner is corrupted, accept any $x_w^{*}$ that satisfies the declared input interface; this extracted value is used below.
\item \textbf{Validate and evaluate.} Evaluate the validity predicates of $\mu$; their accept or abort outcome is part of the output. For accepted inputs, compute $\vec{y}=C(\vec{x})$ exactly in the declared finite arithmetic, including the specified comparisons and truncations.
\item \textbf{Deliver or abort.} Send $\Leak_C$ and the outputs of corrupted recipients to $\Sim$. At each public interaction boundary, $\Sim$ may send $\mathsf{abort}$ or $\mathsf{delay}$; on $\mathsf{abort}$, send $\bot$ to every honest recipient. Otherwise deliver each $y_i$ to its authorized recipient. A corrupted recipient may obtain its output before honest ones (no fairness).
\end{enumerate}
\end{minipage}}

\vspace{5pt}
\fbox{\begin{minipage}{\dimexpr\columnwidth-2\fboxsep-2\fboxrule\relax}
\centering\underline{Functionality $\FPIR$}\par\smallskip
\raggedright
\textbf{Parameters.} Public descriptor: database identifier, version $v$, length $N$, record encoding, and authorized snapshot commitment $\mathsf{cm}_v$, which fixes $D=(D[0],\dots,D[N-1])$. Corruption regime, never combined: (a) at most one server host, client honest; or (b) the client alone, both server hosts honest.
\begin{enumerate}[leftmargin=*,nosep,topsep=2pt]
\item \textbf{Query.} Receive an index $\alpha$ from the client; in regime (b), extract the corrupted client's index $\alpha^{*}$ and set $\alpha\gets\alpha^{*}$. If $\alpha\notin\{0,\dots,N-1\}$ or the request is inconsistent, return $\mathsf{reject}$ to the client and stop.
\item \textbf{Leak.} Send $\Leak_{\mathrm{PIR}}$ to $\Sim$; nothing about $\alpha$ is sent.
\item \textbf{Answer.} In regime (a), if $\Sim$ sends $\mathsf{abort}$, send $\bot$ to the client; otherwise send $D[\alpha]$. In regime (b), send $D[\alpha]$, and no other information about $D$, to the client.
\end{enumerate}
\end{minipage}}
\caption{Ideal functionalities for authenticated circuit evaluation (top) and versioned-snapshot PIR (bottom). Both provide security with abort. The full definitions, together with the ideal module resource $\mathcal{F}_T$, are in \cref{app:func}.}
\label{fig:func}
\end{figure}

\begin{definition}[Static malicious security with abort]\label{def:security}
Let $\mathcal{F}\in\{\FC,\FPIR\}$ with leakage $\Leak$ as in \cref{def:leakage}, and let $\Pi$ be a protocol run by $P_0$ and $P_1$ in which the modules are instances of $\mathcal{F}_T$. Fix a PPT adversary $\Adv$ with auxiliary input $z$ that statically corrupts a set $I$ admitted by the corruption regime of $\mathcal{F}$, a manifest $\mu$, and an input vector $\vec{x}$.
$\Real_{\Pi,\Adv(z),I}(\mu,\vec{x})$ is the joint distribution of the view of $\Adv$ (its inputs, randomness, received messages, and the external traces of $\mathcal{F}_T$ observable from corrupted hosts) and the outputs of the honest parties and client in an execution of $\Pi$.
$\Ideal_{\mathcal{F},\Sim(z),I}(\mu,\vec{x})$ is the joint distribution of the output of a simulator $\Sim$ and the honest outputs in an execution in which $\Sim$ interacts only with $\mathcal{F}$: it submits the corrupted parties' inputs, receives $\Leak$ and the corrupted parties' outputs, and may abort or delay as $\mathcal{F}$ allows.
We say that $\Pi$ \emph{$\epsilon$-securely realizes $\mathcal{F}$ with leakage $\Leak$ against static malicious corruption with abort} if for every such $\Adv$ there exists a PPT simulator $\Sim$ such that for all $\mu$, $\vec{x}$, $z$, $I$ and every PPT distinguisher $\mathcal{D}$,
\begin{align*}
\Bigl|&\Pr\bigl[\mathcal{D}\bigl(\Real_{\Pi,\Adv(z),I}(\mu,\vec{x})\bigr)=1\bigr]\\
&\quad-\Pr\bigl[\mathcal{D}\bigl(\Ideal_{\mathcal{F},\Sim(z),I}(\mu,\vec{x})\bigr)=1\bigr]\Bigr|\le\epsilon .
\end{align*}
\end{definition}

\textbf{Remarks.}
\Cref{fig:func} gives both functionalities. Three aspects of \cref{def:security} matter below. First, the real world contains the modules as the ideal resource $\mathcal{F}_T$, and the simulator controls only this ideal representation of the trusted resources, never the honest party's prescribed inputs. Second, $\epsilon$ is concrete: \cref{thm:main} shows that \sys realizes $\FC$ with
$\epsilon\le\eps{setup}+\eps{prf}+\eps{channel}+\eps{bind}+\eps{trace}+Q(2/p)^t$
for at most $Q$ \CheckOpen{} batches. For $p=2^{61}-1$, $t=3$, and $Q\le 2^{32}$ the statistical term is about $2^{-148}$, so the 128-bit primitives behind the computational terms dominate (\cref{sec:sec-concrete}). Third, correctness of the protected code, state, and arithmetic is a premise of the ideal resource, not a probability in $\epsilon$; \cref{tab:obligations} lists what a concrete chip must still establish.

\textbf{Model provenance.}
Computational correctness is not model provenance, and a public architecture hash in $\mu$ does not authenticate private weights. If the client requires a specific pre-approved model, $\mu$ must contain a commitment to the canonical quantized weight bytes, authorized by the client or by an independent model authority rather than declared by the untrusted host, and the protected input loader must hash exactly those bytes before sharing them (\cref{sec:proto-arith}); a mismatch aborts. Without such a commitment, the weights are simply the model owner's freely chosen private input, and S9 is the intended behavior of $\FC$.

\subsection{The Stronger Profile U}\label{sec:threat-profileu}

\ProfT trusts the modules. When the hardware itself must be treated as adversarial, for example because the accelerator vendor or the platform administrator is not trusted, we specify \ProfU. The accelerator then receives neither the joint-sampler key nor any global MAC key. The circuit runs through an established malicious two-party backend, such as SPDZ-family protocols with MASCOT or SPDZ2k preprocessing~\cite{damgard2012spdz,keller2016mascot,cramer2018spdz2k,keller2020mpspdz} or dealer-based actively secure FSS~\cite{gupta2025shark}, and the accelerator is confined to party-local data, for instance expanding the DPF keys that the backend exports to its own party. Client-generated keys checked with verifiable FSS~\cite{decastro2022vfss} are a possible input to such a backend, but key validity alone does not verify the servers' evaluation, which needs its own proof. The same DPF datapath therefore serves both profiles, but \ProfU gives up the local-dealer and generate-and-consume savings, and an exported-key profile must add the backend's actual DPF privacy assumption to its security bound. \ProfU is a separate backend chosen at session start, not a fallback after a module compromise: switching profiles after a compromise does not undo leaked secrets, so a fresh session with fresh inputs and masks is required. The rest of this paper analyzes and evaluates \ProfT.


==> qa/draft1/sections/04_analysis.tex <==
% ======================================================================
% Section IV: Workload Analysis (owner: sections/04_analysis.tex)
% Labels defined here: sec:analysis, sec:analysis-cost, sec:analysis-dpf,
% sec:analysis-work, alg:gen, alg:eval, fig:gac, tab:gatecost, fig:motiv
% ======================================================================
\section{Workload Analysis: Where Malicious Security Costs Go}
\label{sec:analysis}

The DFA design~\cite{dfa2026trusted} was driven by one workload observation: in semi-honest FSS workloads, DPF generation, distribution and evaluation dominate both computation and communication, so a small DPF engine that also plays the dealer removes the dominant cost. Before designing a malicious-secure successor, we repeat this exercise for the adversary of \cref{sec:threat}. The answer changes the design target. Malicious security introduces five cost sources (\cref{sec:analysis-cost}). Handled naively, two of them multiply exactly the DPF work and key traffic that trusted DFA made small; handled carefully, DPF stops being the bottleneck altogether, and the cost moves to authenticated linear algebra on the GPU and to the extra round of every verified opening. \Cref{sec:analysis-dpf} then fixes the exact DPF computation that the protocol, the proofs and the hardware must all reproduce, and \cref{sec:analysis-work} counts its work at five design points.

% ======================================================================
\subsection{Cost Sources in Malicious FSS}
\label{sec:analysis-cost}

We take as reference the masked-input paradigm of FSS-based inference~\cite{gupta2023sigma,jawalkar2024orca} (\cref{sec:bg-pi}): linear layers operate on additive shares, and every nonlinear gate opens a masked input $x+r$ and evaluates FSS keys prepared for the mask $r$. Making this pipeline secure against a malicious host (\cref{def:security}) adds the following costs, regardless of how they are implemented.

\textbf{(i) Authenticated representation.}
Every wire must carry information-theoretic MACs so that a host that changes its share is caught~\cite{damgard2012spdz,damgard2013practical}. In our representation (\cref{sec:proto-repr}), party $b$ holds $\authb{x}{b}=(x_b,\gamma_{b,1},\gamma_{b,2},\gamma_{b,3})$ over $\Fp$ with $p=2^{61}-1$ and $t=3$ independent MAC keys: four 64-bit words, or 32\,B per element and party, instead of 8\,B for a semi-honest share in $\Z_{2^{64}}$. Every linear layer is therefore computed on four lanes (the value and three tags), each lane uses exact Mersenne reduction instead of free 64-bit wraparound (\cref{sec:arch-field}), and every authenticated element that crosses PCIe or the host-module interface grows by the same factor of four. Only the peer link is spared, because checks exchange value shares and $t$ residuals rather than tags (\cref{sec:proto-check}).

\textbf{(ii) Verified openings.}
Opened values (masked gate inputs, the Beaver differences $d,e$ of each multiplication~\cite{beaver1991efficient}, and outputs) must be checked before anything depends on them. A sound check derives its challenge only after the checked bytes are fixed (\cref{thm:mac-sound}), so at least one extra exchange follows every checked batch, and a dependent nonlinear gate may not consume an unchecked opening. Batching amortizes challenge derivation and metadata but not this round, which lies on the critical path of every layer: a protocol with $R$ online rounds approaches $2R$. Inside the module, each checked element costs up to 3.5 AES blocks (1.5 for its three challenge lanes and 2 for sealing its 32\,B when frozen pages spill to AEAD-protected memory) and $2t=6$ field multiplications.

\textbf{(iii) Correct preprocessing.}
Triples, masks and FSS keys must be \emph{correct}, not merely authenticated: a valid MAC on a triple with $c\neq ab$ makes the triple look legitimate without making it correct. A dealer can ship authenticated material, at the price of more offline traffic than in the semi-honest case. Alternatively, the parties generate it themselves with OT- or HE-based malicious preprocessing such as MASCOT, Overdrive or SPDZ2k~\cite{keller2016mascot,keller2018overdrive,cramer2018spdz2k,keller2020mpspdz}, which replaces the dealer by substantial interactive communication. Neither option removes offline data movement.

\textbf{(iv) Authenticated FSS outputs.}
A DPF output share is a plain additive share. To re-enter authenticated arithmetic it needs $t$ tag shares, and the straightforward way to obtain them is a second DPF per MAC lane $j$ with the same target and payload $\Delta_j\beta$ (a \emph{tag tree}). This multiplies DPF keys, key bytes and PRG work by $1+t$, i.e., by four for $t=3$.

\textbf{(v) Key validity is not evaluation correctness.}
Verifiable FSS~\cite{decastro2022vfss} lets evaluators check that their keys are well formed, which protects against a malicious key generator. It does not constrain an evaluator that computes on valid keys and then adds an error to its output share, nor the arithmetic that consumes that share. In the same way, attestation of a trusted module authenticates its code and configuration; it does not show that an untrusted GPU used a valid key, computed the right product or released an authorized result (scenarios S1 to S7 in \cref{sec:threat-scenarios}).

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{charts/chart_motiv.pdf}
    \caption{Estimated BERT-Base latency breakdown on LAN (1\,GB/s, 0.05\,ms RTT) by cost source, for two semi-honest configurations of~\cite{dfa2026trusted} and three malicious configurations; all splits come from our model (\cref{app:model}). (a)~Full range; (b)~zoom into 0--6\,s. Offline distribution dominates the dealer-based malicious design (\est{37.6\,s} of \est{43.9\,s}); four-lane authenticated GEMM dominates \sys (\est{2.60\,s} of \est{3.83\,s}).}
    \label{fig:motiv}
\end{figure}

\textbf{Observation 1: distribution still dominates a dealer-based design.}
\Cref{fig:motiv} splits the estimated BERT-Base LAN latency by cost source. The dealer-based malicious configuration, modeled after the protocol family of Shark~\cite{gupta2025shark} (\cref{sec:eval-method}), must move \est{37.6\,GB} of authenticated keys and preprocessing per query, \est{2.2$\times$} the 17.1\,GB of the semi-honest GPU baseline~\cite{dfa2026trusted}. At 1\,GB/s, this distribution alone takes \est{37.6\,s} of \est{43.9\,s} (\est{86\%}), and moving the material from host memory into the GPU adds another \est{1.70\,s}.

\textbf{Observation 2: without distribution, DPF is no longer the bottleneck.}
Removing distribution, as trusted DFA did for the semi-honest case, exposes a different profile. In \sys, four-lane authenticated GEMM takes \est{2.60\,s} of \est{3.83\,s} (\est{68\%}), \est{5.0$\times$} our \est{0.52\,s} estimate of the semi-honest GEMM; online communication takes \est{0.615\,s} (\est{16\%}); and all module-side FSS gates together take only \est{0.131\,s} (\est{3.4\%}). If generation and consumption are decoupled (\sys without GaC), the authenticated material that must be materialized and reread raises CPU-GPU traffic from \est{3.31\,GB} to \est{68.6\,GB} and latency from \est{3.83\,s} to \est{5.87\,s}.

\textbf{Observation 3: on a WAN, verification rounds dominate.}
With a 70\,ms RTT the extra check round of source (ii) outweighs all computation: removing CheckOpen, which is insecure and serves only as a lower bound, would cut the estimated BERT-Base WAN latency from \est{89.7\,s} to \est{50.5\,s} (\cref{tab:ablation}).

\textbf{Implications.}
For sources (iii) and (iv) the semi-honest lesson still holds: distribution is the largest avoidable cost, so a malicious design must keep DFA's local generation and generate-and-consume, and it must authenticate FSS outputs without multiplying DPF work. What then remains are sources (i) and (ii). The trusted module should therefore own randomness, verification and release, leave four-lane exact linear algebra to the GPU, and make its check round cheap to batch and safe against the host that schedules it (\cref{sec:protocol,sec:arch}).

% ======================================================================
\subsection{Compute Pattern of Exact DPF}
\label{sec:analysis-dpf}

Malicious-security proofs reason about concrete states, so we fix the DPF computation exactly. \Cref{alg:gen,alg:eval} give the tree-based DPF~\cite{gilboa2014distributed,boyle2016function} in the form that \sys executes; the same algorithms serve \ProfU, where keys are exported to an external malicious backend (\cref{sec:threat-profileu}). The expansion function $\PRG:\bits{128}\to(\bits{128}\times\{0,1\})^2$ is fixed and AES-based as in DFA, $\Conv:\bits{128}\to\Fp$ is the fixed output conversion, the target $\alpha$ and the query $x$ have $n$ bits read most-significant first, and the payload is $\beta\in\Fp$.

\begin{algorithm}[t]
\caption{Exact DPF key generation ($\DPF.\Gen$)}
\label{alg:gen}
\begin{algorithmic}[1]
\algstretch
\Require target $\alpha=\alpha_1\cdots\alpha_n\in\bits{n}$ (MSB first), payload $\beta\in\Fp$
\Ensure keys $(k_0,k_1)$ with $\Eval(k_0,x)+\Eval(k_1,x)=\beta\cdot\one[x=\alpha]$
\State sample independent $s_0,s_1\getsr\bits{128}$; $t_0\gets 0$; $t_1\gets 1$
\State save the initial seeds $s_0^{(0)}\gets s_0$, $s_1^{(0)}\gets s_1$
\For{$i=1$ \textbf{to} $n$}
    \State $a\gets\alpha_i$; \ $\keep\gets a$; \ $\lose\gets 1-a$ \Comment{$L=0$, $R=1$}
    \State $(s_b^L,t_b^L,s_b^R,t_b^R)\gets\PRG(s_b)$ for $b\in\{0,1\}$
    \State $\sCW\gets s_0^{\lose}\oplus s_1^{\lose}$
    \State $\tCW{L}\gets t_0^L\oplus t_1^L\oplus a\oplus 1$; \ $\tCW{R}\gets t_0^R\oplus t_1^R\oplus a$
    \LineComment{both $b$, with the \emph{old} $t_b$; $\cdot$ is a conditional XOR}
    \State $(s_b,t_b)\gets\bigl(s_b^{\keep}\oplus t_b\cdot\sCW,\ t_b^{\keep}\oplus t_b\cdot\tCW{\keep}\bigr)$
    \State $\CW^{(i)}\gets(\sCW,\tCW{L},\tCW{R})$
\EndFor
\State $u_b\gets\Conv(s_b)$ for $b\in\{0,1\}$
\State $\CWout\gets(-1)^{t_1}\,(\beta-u_0+u_1)$
\LineComment{keys hold the initial roots, never the final states}
\State $k_b\gets\bigl(s_b^{(0)},\,b,\,\CW^{(1)},\ldots,\CW^{(n)},\,\CWout\bigr)$ for $b\in\{0,1\}$
\State \Return $(k_0,k_1)$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Exact DPF evaluation ($\DPF.\Eval$, $\DPF.\EvalAll$)}
\label{alg:eval}
\begin{algorithmic}[1]
\algstretch
\Require role $b$, key $k_b=(s_b^{(0)},b,\CW^{(1)},\ldots,\CW^{(n)},\CWout)$, query $x=x_1\cdots x_n$
\Ensure share $y_b\in\Fp$ (or all $2^n$ leaf shares for $\EvalAll$)
\Function{Eval}{$k_b,x$}
    \State $(s,t)\gets(s_b^{(0)},b)$ \Comment{root control bit $=$ role}
    \For{$i=1$ \textbf{to} $n$} \Comment{$\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$}
        \State $(s^L,t^L,s^R,t^R)\gets\PRG(s)$ \Comment{$t$: old evaluator bit}
        \State $(s^L,t^L)\gets(s^L\oplus t\cdot\sCW,\ t^L\oplus t\cdot\tCW{L})$
        \State $(s^R,t^R)\gets(s^R\oplus t\cdot\sCW,\ t^R\oplus t\cdot\tCW{R})$
        \State $(s,t)\gets(s^{L},t^{L})$ if $x_i=0$, else $(s^{R},t^{R})$
    \EndFor
    \State \Return $y_b\gets(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$
\EndFunction
\Function{EvalAll}{$k_b$}
    \State push $(s_b^{(0)},b,0,\epsilon)$ onto stack $\mathcal{S}$
    \While{$\mathcal{S}\neq\emptyset$}
        \State pop $(s,t,i,\pi)$ \Comment{seed, bit, depth, prefix}
        \If{$i=n$}
            \State emit leaf $\pi$ with share $(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$
        \Else
            \State expand $s$ as in lines 4--6 with $\CW^{(i+1)}$
            \State push $(s^R,t^R,i{+}1,\pi\|1)$ onto $\mathcal{S}$
            \State push $(s^L,t^L,i{+}1,\pi\|0)$ onto $\mathcal{S}$ \Comment{left first}
        \EndIf
    \EndWhile
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_gac.pdf}
    \caption{Malicious-safe generate-and-consume inside module $T_b$ for a depth-2 tree. (a)~Joint generation: the two generator states $(s_0,t_0)$ and $(s_1,t_1)$ follow the target path $\alpha=01$ and emit $\CW^{(1)}$, $\CW^{(2)}$ and $\CWout$, which are consumed immediately instead of being stored as a key. (b)~Local evaluation of party $b$ on query $x=00$: a separate evaluator state $(\tilde s,\tilde t)$ follows $x$, applies each correction word at its own level, and leaves the target path at level~2, where only its own control bit $\tilde t$ is correct; grey nodes are never expanded. (c)~Leaf epilogue: the raw share $\tilde y_b$ is freshly reshared and authenticated with joint pads $\zeta,\kappa_1,\kappa_2,\kappa_3$ into the 32\,B tuple $\authb{y}{b}$. The crossed-out inset is the tag-tree alternative, which needs $t=3$ extra DPF trees with payloads $\Delta_j\beta$ and four times the PRG work.}
    \label{fig:gac}
\end{figure*}

\textbf{High-level idea.}
As in DFA, a DPF is a binary tree of depth $n$ whose root-to-leaf path $\alpha$ is encoded by $n$ correction words. $\Gen$ walks two states $(s_0,t_0)$ and $(s_1,t_1)$ down that path (\cref{fig:gac}a). At level $i$ the kept child is $\alpha_i$ and the losing child is $1-\alpha_i$. The seed correction $\sCW$ makes the two losing seeds equal after correction, and the control-bit corrections $\tCW{L},\tCW{R}$ make the losing control bits equal while keeping the kept control bits different (lines 6--9 of \cref{alg:gen}). Because each state applies a correction only when its \emph{own} old control bit is set, exactly one of the two target-path states applies it. Once a query leaves the path, both parties hold identical states that stay identical, so their signed leaf outputs cancel; at the target leaf, $\CWout$ makes them sum to $\beta$. \Cref{thm:dpf-correct} proves $y_0+y_1=\beta\cdot\one[x=\alpha]$ for every target, query, payload and root pair. Correctness needs neither uniform targets nor computational hardness; uniform masks belong to the application protocol (\cref{sec:proto-refactor}).

\textbf{Explicit states.}
Three details that a simplified listing may leave implicit are explicit in \cref{alg:gen,alg:eval}, because the malicious analysis depends on them. First, the root control bits are fixed by role, $t_0=0$ and $t_1=1$, rather than sampled, and the evaluator of party $b$ always starts from $(s_b^{(0)},b)$. Second, a key contains the \emph{initial} seed of its party, the correction words and $\CWout$; the generator's final states are never substituted for the roots. Third, the payload and the role enter only through $\CWout$ and the output sign $(-1)^b$, so both are bound inputs of the ledgered gate descriptor (\cref{sec:proto-ledger}) rather than host-supplied parameters.

\textbf{Generator versus evaluator state.}
Lines 5--6 of \cref{alg:eval} correct both children with the evaluator's own old control bit $t$. Along the target path this bit coincides with the generator's $t_b$, which invites reusing the generator's control register during generate-and-consume. The substitution is wrong as soon as the query leaves the path (level~2 in \cref{fig:gac}b): there the evaluator states of the two parties are identical and must apply identical corrections, whereas the generator bits $t_0$ and $t_1$ still differ, so one party would apply a correction that the other omits, and the off-path outputs would no longer cancel. The merged listing of the semi-honest DFA design~\cite{dfa2026trusted} leaves this distinction, the root relation and the role inputs implicit. \sys therefore keeps three separate states in each module: two generator states and one evaluator state for its own party. At each level the module computes exactly the correction word of \cref{alg:gen}, advances both generator states, applies the word to its evaluator's expanded query-path state as in \cref{alg:eval}, and discards the word only after that use (\cref{alg:gac} in \cref{sec:proto-gac}). \Cref{thm:gac} shows by coupling that this streaming schedule returns exactly the output of \cref{alg:gen} followed by \cref{alg:eval}; it justifies the schedule, not any change to expansion or correction semantics. In hardware the generator and evaluator contexts share correction words but not path registers (\cref{sec:arch-pipe}).

\textbf{Single path versus full domain.}
Private-inference gates evaluate one path: $n$ expansions for the evaluator plus $2n$ for the two generator states in each module. PIR and small-LUT gates scan the full domain with $\EvalAll$, a depth-first traversal whose stack holds $O(n)$ pending siblings per sequential traversal and whose complete tree costs $2^n-1$ internal expansions, not $n2^n$. Both patterns are data independent and map onto a pipelined AES engine; extra pipeline contexts add storage separately (\cref{sec:arch-pipe}).

\textbf{Leaf epilogue.}
\Cref{fig:gac}c shows how an internally computed raw share becomes an authenticated tuple without a second tree. With fresh joint pads $\zeta,\kappa_1,\ldots,\kappa_t\in\Fp$, module $T_b$ outputs $y_b=\tilde y_b+(-1)^b\zeta$ and $\gamma_{b,j}=\Delta_j y_b+(-1)^b\kappa_j$: three field multiplications and four pads per output and party (\cref{sec:proto-epilogue}). The raw share never leaves the module, and the interface has no entry point that authenticates a host-supplied value, so the epilogue cannot serve as a forgery oracle.

% ======================================================================
\subsection{Work Accounting}
\label{sec:analysis-work}

\begin{table*}[t]
\centering
\caption{Analytic Cost of One Single-Path DPF Gate of Depth $n$ with $t$ MAC Lanes}
\label{tab:gatecost}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llccccccc}
\hline
\textbf{Design} & \textbf{Security} & \makecell{\textbf{PRG exp.}\\\textbf{per gate}} & \makecell{\textbf{Field ops per}\\\textbf{output, party}} & \makecell{\textbf{Offline bytes}\\\textbf{per gate}} & \makecell{\textbf{Bytes into GPU}\\\textbf{per party}} & \makecell{\textbf{Extra}\\\textbf{rounds}} & \makecell{\textbf{Auth.}\\\textbf{output}} & \makecell{\textbf{Verifies}\\\textbf{evaluation}} \\
\hline
Dealer-based FSS~\cite{gupta2023sigma,jawalkar2024orca} & SH & $4n$ & 0 & $2|k|$ & $|k|$ & 0 & \xmark & \xmark \\
Trusted DFA, GaC~\cite{dfa2026trusted} & SH & $6n$ & 0 & 0 & 8 & 0 & \xmark & \xmark \\
Dealer-based FSS, tag trees & Mal. & $4n(1+t)$ & 0 & $2(1+t)|k|$ & $(1+t)|k|$ & 1 per batch & \cmark & \cmark\ (at opening) \\
vFSS-verified keys~\cite{decastro2022vfss} & Mal.\ key gen. & $4n$ + sketch & 0 & $2|k|+O(\lambda)$ & $|k|+O(\lambda)$ & 1 (sketch) & \xmark & \xmark\ (keys only) \\
\sys, GaC + epilogue & Mal. & $6n$ & \makecell{3 mult.\\+ 4 pads} & 0 & 32 & 1 per batch & \cmark & \cmark \\
\hline
\end{tabular}

\vspace{3pt}
\parbox{\textwidth}{\footnotesize SH: semi-honest; Mal.: malicious. $|k|$ is the byte length of one party's key. PRG expansions are summed over all parties, dealer included. Bytes into the GPU are keys loaded by a GPU evaluator or output shares delivered by a module. Mask shares and Beaver triples of the surrounding arithmetic are omitted; with authentication, each such element costs 32\,B per party instead of 8\,B. Rounds are counted relative to the plain masked opening that every design performs.}
\end{table*}

\Cref{tab:gatecost} compares one single-path DPF gate at five design points. With 128-bit seeds, one party's key holds its root seed, $n$ correction words of $128+2$ bits and $\CWout$ as one canonical 64-bit word (the root control bit is the public role), so $|k|=\lceil(128+130n+64)/8\rceil$ bytes, or 1{,}016\,B for $n=61$.

\textbf{Design-point comparison.}
A semi-honest dealer expands $2n$ seeds per gate and each evaluator $n$ more, $4n$ in total, and ships $2|k|$ bytes that each party later loads into its GPU. Trusted DFA removes the key bytes but not the generation work: each module reproduces the joint generation for its own party, so the two modules together expand $6n$ seeds, $1.5\times$ the dealer total. A dealer that authenticates outputs with tag trees multiplies expansions, key bytes and key I/O by $1+t$ and adds the check round of source (ii). Verifiable keys keep the semi-honest costs plus a verification sketch and one exchange, but authenticate neither the output nor its evaluation. \sys keeps the trusted-DFA work of $6n$ expansions and zero key bytes, and adds three field multiplications and four pads per output and party; what it cannot avoid is the 32\,B authenticated tuple and the check round, i.e., sources (i) and (ii).

\textbf{Effect of the epilogue.}
Because the epilogue leaves the per-gate PRG count unchanged, the estimated single-path throughput of the DPF engine drops only from \est{113} to \est{106} M gates/s at $n=61$ relative to semi-honest trusted DFA, whereas tag trees fall to \est{26.7} M gates/s; the gap stays at \est{3.8--4.0$\times$} for $n$ between 8 and 61 (\cref{fig:dpfthr}). End to end, replacing the epilogue by tag trees inside the module would raise the BERT-Base LAN latency from \est{3.83\,s} to \est{4.12\,s} and energy from \est{73.7\,J} to \est{80.4\,J} (\cref{tab:ablation}). The end-to-end effect is smaller than the per-gate effect precisely because FSS is no longer the bottleneck (Observation~2). Sharing one tree among the lanes with a $(1+t)$-element payload would remove most extra expansions, but it widens every output correction by $t$ field elements, covers only results that are linear in DPF evaluations, and exports pseudorandom tag shares whose hiding rests on DPF key privacy. The epilogue instead makes every exported tuple exactly uniform for its holder (\cref{thm:epilogue}) and applies unchanged to LUT, interval, direct and PIR results.

\textbf{Remaining costs we accept.}
\sys does not remove duplicated generation: $6n$ instead of $4n$ expansions is the price of eliminating $2|k|$ network bytes and $|k|$ bytes of key I/O per gate, a favorable trade because PRG expansion is the cheapest operation in the pipeline while bytes cross its slowest links. Interval gates use two DCFs, and the conservative DCF of \cref{alg:dcf}, for which \cref{thm:dcf} proves correctness, builds one DPF per prefix and evaluates $n(n+1)/2$ path levels, 1{,}891 instead of 61 for $n=61$. Its estimated interval-gate cost is \est{22{,}692} AES blocks, against \est{976} for an optimized $O(n)$ DCF that our proofs do not cover; the compiler therefore chooses among direct, LUT and interval gates by measured cost (\cref{sec:proto-direct}). Finally, authenticated traffic is at least 32\,B per output element and party, so a host-module link of $B$ bytes/s bounds the pure output stream at $B/32$ elements/s, e.g., 31.25\,M elements/s for an illustrative $B=10^9$\,B/s. This roofline is why the module sits next to the GPU L2 slices as in DFA rather than behind PCIe (\cref{sec:arch-dse}).

\textbf{Implications.}
The accounting yields five design rules that structure the rest of the paper: (1)~authenticate FSS outputs by fresh resharing inside the module, never by extra trees and never by authenticating host values (\cref{sec:proto-epilogue}); (2)~keep generation local and streamed, with separate generator and evaluator states (\cref{sec:proto-gac}); (3)~make the unavoidable check round sound and batchable by freezing bytes before challenges are drawn (\cref{sec:proto-check}); (4)~bind every randomness draw to one session, gate, role and use, so that local generation does not open a replay path (\cref{sec:proto-ledger}); and (5)~leave four-lane exact linear algebra on the GPU while the module generates correct triples and verifies openings (\cref{sec:arch-insight}).


==> qa/draft1/sections/05a_protocol.tex <==
% ======================================================================
% Section V (part 1): VIGOR-DFA Protocol Design
% Owner: 05a_protocol.tex. Continues in 05b_protocol_gates.tex.
% ======================================================================
\section{\texorpdfstring{\sys}{VIGOR-DFA} Protocol Design}\label{sec:protocol}

This section specifies the protocol run by the two parties of \ProfT: the flow and design rules (\cref{sec:proto-overview}), the representation, joint randomness and lifecycle state (\cref{sec:proto-repr,sec:proto-setup,sec:proto-ledger}), and the mechanisms that move values through the integrity chain (\cref{sec:proto-gac,sec:proto-epilogue,sec:proto-check,sec:proto-arith}). Nonlinear gates, refactoring, GPU verification and PIR follow in \cref{sec:proto-gates,sec:proto-direct,sec:proto-refactor,sec:proto-freivalds,sec:proto-pir}; formal statements are collected in \cref{sec:security}.

% ======================================================================
\subsection{Overview}\label{sec:proto-overview}

\textbf{High-level idea.}
In trusted DFA the protected module replaces the dealer: it samples FSS keys locally and consumes each correction word as soon as it produces it~\cite{dfa2026trusted}. Against a malicious host this is not enough: every value that leaves the module is later processed by the host's GPU, and every value that enters it comes from host memory. \sys turns the module from a dealer into a dealer that also verifies. Every wire carries an authenticated sharing with $t$ information-theoretic MAC lanes. The GPU performs all linear algebra on these sharings but only ever produces \emph{candidate} shares. Each module generates every correlation of its party, authenticates every FSS output it computes, checks every opening on frozen bytes and releases nothing before verification. Together these steps protect each link of the integrity chain \emph{authorized input $\rightarrow$ correlated preprocessing $\rightarrow$ correct local evaluation $\rightarrow$ authenticated arithmetic $\rightarrow$ consistent opening $\rightarrow$ authorized output release}.

\textbf{Per-gate lifecycle.}
Every gate of the public circuit $C$ fixed by the manifest $\mu$ passes through the same module commands (\cref{tab:commands}). (1)~With \cmd{RESERVE_PREP}, $T_b$ reserves the gate's randomness labels in its one-time ledger and issues party-local authenticated preprocessing (masks, triples) to host~$b$. (2)~Host $b$'s GPU computes candidate authenticated shares with local linear operations. (3)~With \cmd{FREEZE_BATCH} and \cmd{CHECK_OPEN}, the two modules freeze the submitted bytes and verify the masked openings the gate needs. (4)~For a nonlinear gate, \cmd{EVAL_FSS} consumes the verified opening, runs generate-and-consume inside $T_b$ and returns a freshly authenticated share. (5)~\cmd{FINAL_OUTPUT} hands a masked output and a bound certificate to an authorized recipient. A failure in any step triggers \cmd{ABORT}, which poisons the epoch.

\textbf{Design rules.}
Four rules shape the rest of this section; each answers scenarios of \cref{sec:threat-scenarios}.
(R1)~\emph{No forgery oracle}: a module authenticates only values it computed itself or received from an explicitly verified backend (S2, S7).
(R2)~\emph{No challenge before freeze}: checking randomness is derived only after both modules have frozen the exact submitted bytes, and a module later consumes exactly those bytes (S1, S3).
(R3)~\emph{One-time, role-bound resources}: every draw is bound to session, epoch, gate and purpose, used once and never recycled after an abort (S4, S5).
(R4)~\emph{No output before verification}: the release guard stays closed until the ledger reports \lstate{VERIFIED}, and any failure poisons the epoch (S6).
Rule (R2) combined with versioned snapshot hashing also covers snapshot substitution in PIR (S8, \cref{sec:proto-pir}). \Cref{tab:notation} summarizes the notation.

\begin{table}[t]
\caption{Notation used in the protocol description}
\label{tab:notation}
\centering
\footnotesize
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{p{0.27\linewidth} p{0.63\linewidth}}
\hline
\textbf{Symbol} & \textbf{Meaning} \\
\hline
$P_b$; host $b$; $T_b$ & party $b\in\{0,1\}$; its untrusted host (CPU, OS, driver, GPU, memory, NIC); its protected module \\
$\mu$, $C$ & public manifest and the finite circuit it fixes \\
$p$, $\Fp$ & Mersenne prime $2^{61}-1$ and the protocol field \\
$t$ & number of MAC lanes ($t=3$) \\
$\Delta_j$; $\Delta_{b,j}$ & global MAC key of lane $j$ (modules only); host $b$'s additive share of it \\
$\auth{x}$; $\authb{x}{b}$ & authenticated sharing of $x$; party $b$'s tuple $(x_b,\gamma_{b,1},\dots,\gamma_{b,t})$ \\
$\gamma_{b,j}$ & tag share of party $b$ in lane $j$, $\gamma_{0,j}+\gamma_{1,j}=\Delta_j x$ \\
$K$ & session key shared by $T_0$ and $T_1$ after setup \\
$\ell$ & length-prefixed label (session, epoch, gate, purpose, logical draw, block) \\
$\PRF_K(\ell,\cdot)$ & joint draw: same label, same value in both modules \\
$n$; $\lambda$ & DPF input length in bits; PRG seed length ($\lambda=128$) \\
$\alpha$, $\beta$, $x$ & DPF target, payload in $\Fp$, verified public query \\
$\CW^{(i)}$; $\CWout$ & level-$i$ correction word; output correction \\
$(s_c,t_c)$; $(\tilde s,\tilde t)$ & generator state of root $c\in\{0,1\}$; evaluator state of $T_b$ \\
$\tilde y_b$ & raw local output of the protected evaluator \\
$\zeta$; $\kappa_j$ & fresh common epilogue pads for the value; for lane $j$ \\
$m$; $h_b$; $\mathit{cid}$ & batch size; frozen root of $T_b$; check identifier \\
$\rho_{j,i}$; $\sigma_{b,j}$ & challenge of lane $j$ at batch position $i$; residual of $T_b$ in lane $j$ \\
$Q$ & number of checked batches in one execution \\
$w$ & LUT input width (\cref{sec:proto-gates}); in $\Pi_{\mathsf{Out}}$ the masked output $y+o$ \\
\hline
\end{tabular}
\end{table}

% ======================================================================
\subsection{Authenticated Representation}\label{sec:proto-repr}

\textbf{Field and MAC lanes.}
All protocol arithmetic is over $\Fp$ with the Mersenne prime $p=2^{61}-1$. The modules hold $t=3$ independent global MAC keys $\Delta_1,\Delta_2,\Delta_3\getsr\Fp$, each additively split as $\Delta_j=\Delta_{0,j}+\Delta_{1,j}$. Host $b$ may know its own key shares $\Delta_{b,j}$, but neither host ever learns a complete $\Delta_j$; both modules know the global keys and run the joint sampler. Party $b$ holds an authenticated value $\auth{x}$ as
\begin{gather*}
\authb{x}{b}=(x_b,\gamma_{b,1},\gamma_{b,2},\gamma_{b,3}),\\
x_0+x_1=x,\qquad \gamma_{0,j}+\gamma_{1,j}=\Delta_j x\quad (j\in[t]),
\end{gather*}
which is the SPDZ representation~\cite{damgard2012spdz,damgard2013practical} with three independent lanes. A canonical wire occupies four 64-bit words, i.e., 32~B per party before metadata. Every element is encoded as an unsigned 64-bit integer smaller than $p$; the module parser rejects noncanonical encodings instead of reducing arbitrary integers modulo $p$, which keeps frozen bytes and checked field elements in one-to-one correspondence.

\textbf{Why three lanes over a 61-bit field.}
The Mersenne modulus lets the GPU compute exact products of canonical elements with native 64-bit multiplies and two folding steps (\cref{sec:arch-field}), so all $1+t$ lanes of authenticated linear algebra stay on standard integer datapaths. A single 61-bit tag, however, is too weak. By \cref{thm:mac-sound}, a wrong value survives one batch check with probability at most $(2/p)^t$; across $Q\le 2^{32}$ checked batches, one lane gives only $2^{-28}$, two lanes $2^{-88}$ and three lanes $2^{-148}$ (\cref{sec:sec-concrete}). With $t=3$, the 128-bit primitives rather than the statistical term limit the overall security. The price is paid on the GPU: every linear operation runs on four lanes, which raises the modeled BERT-Base LAN latency from \est{2.53~s} at $t=1$ to \est{3.83~s} at $t=3$ (\cref{sec:eval-ablation}).

\textbf{Why a field and not $\Z_{2^{64}}$.}
The soundness proof of \cref{thm:mac-sound} divides by a nonzero coordinate of the value error. Over $\Z_{2^{64}}$ this step fails: for the error $e=2^{63}$, every even key satisfies $\Delta e=0$, so the error cancels in every lane whose key is even. The field encoding is therefore not bit-identical to the $\Z_{2^{64}}$ arithmetic of FSS-compiled models~\cite{gupta2023sigma,jawalkar2024orca}. \sys fixes the numeric contract in the manifest (fixed-point scale, signed encoding, exact toward-zero truncation of \cref{sec:proto-gates}, magnitudes below $p/2$); a deployment that needs ring semantics must use a SPDZ2k-type backend~\cite{cramer2018spdz2k} with its own proof.

% ======================================================================
\subsection{Session Setup and Joint Randomness}\label{sec:proto-setup}

\textbf{Session setup.}
Each module authenticates its peer's identity, code and configuration measurement, role and freshness contribution. An authenticated key establishment then binds the ordered pair of identities, the roles 0 and 1, a fresh session identifier, the epoch, the manifest hash $\Hash(\mu)$, the field and tag parameters and the protocol version, and yields the session key $K$ known only to $T_0$ and $T_1$. Any failure aborts. We treat this step as an explicit setup assumption with error $\eps{setup}$ (\cref{thm:main}) and propose no new attestation protocol; attestation certifies what runs inside a module, not what the GPU computes (\cref{sec:bg-dfa}).

\textbf{Labels and joint draws.}
All module randomness is derived as $\PRF_K(\ell)$, or with an equivalent KDF~\cite{krawczyk2010hkdf}, where $\ell$ is an unambiguous, length-prefixed encoding of $(\mathsf{session},\mathsf{epoch},\mathsf{gate},\mathsf{purpose},\mathsf{logical\_draw},\mathsf{block})$. A \emph{logical joint draw} uses the same label in both modules and thus yields the same value in $T_0$ and $T_1$ without communication; this is how both modules obtain identical DPF roots, correction words, masks, triples, pads and challenges. Distinct roots, pads, triple components, challenge lanes and rejection-sampling retries receive distinct labels. Two rules are easy to get wrong. The local role must \emph{not} be appended to a joint draw, since $T_0$ and $T_1$ would then generate two unrelated DPF instances whose outputs no longer add up; and the logical root-0 and root-1 draws of one DPF \emph{must} be different draws. Because every label names its session, epoch and gate, the ledger can later detect replayed or misrouted material (S4, S5). A uniform element of $\Fp$ is obtained by rejection sampling: take 61 pseudorandom bits and reject the single value $p$, which occurs with probability $2^{-61}$. Exact distribution claims are made in the random-function hybrid, and a bounded implementation aborts when its retry budget is exhausted instead of introducing a silent bias.

\textbf{Authenticated correlations.}
To share a protected value $v$, the joint sampler runs \AuthShare{}: it samples $v_0\getsr\Fp$ and sets $v_1=v-v_0$, independently samples $\gamma_{0,j}\getsr\Fp$ and sets $\gamma_{1,j}=\Delta_j v-\gamma_{0,j}$ for $j\in[t]$, and gives party $b$ only its tuple $\authb{v}{b}$. A multiplication triple samples $a,b\getsr\Fp$, computes $c=ab$ \emph{correctly inside the protected boundary} and authenticates all three values independently; a matrix triple satisfies the actual equality $C=AB$ for its declared dimensions. Because both modules derive the same correlations from joint labels, preprocessing crosses no network link, which removes the \est{21.8--563~GB} of per-query offline material shipped by the dealer-based malicious baseline (\cref{tab:e2e}). The module never exposes both matrix masks to the untrusted GPU to compute $C$, since the GPU would learn the masks and could return a wrong product. A replacement preprocessing service must deliver both authenticated shares and a proof of triple correctness: a valid MAC on an incorrectly generated triple does not make the triple correct (S7). Matrix-triple generation is the heaviest module task; for LLaMA2-7B it occupies \est{7.18~s} of field-unit time per query, most of which overlaps with GPU work (\cref{sec:eval-scale}).

% ======================================================================
\subsection{One-Time Ledger and Release Guard}\label{sec:proto-ledger}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_ledger.pdf}
    \caption{Per-gate lifecycle enforced by the one-time ledger of $T_b$. Solid arrows are the only permitted transitions, each triggered by the named module command (\cref{tab:commands}). Any other transition or any failed check moves the gate to \lstate{ABORTED}, poisons the epoch and keeps the release guard closed.}
    \label{fig:ledger}
\end{figure}

\textbf{Ledger states.}
Each module keeps an authoritative protected ledger that binds every gate to its operation, predecessor and output wires, numeric type, table or model hash, public dimensions and allowed command sequence. A gate transaction moves only along
\lstate{NEW} $\rightarrow$ \lstate{RESERVED} $\rightarrow$ \lstate{PREPARED} $\rightarrow$ \lstate{FROZEN} $\rightarrow$ \lstate{VERIFIED} $\rightarrow$ \lstate{CONSUMED} $\rightarrow$ \lstate{RELEASED}
(\cref{fig:ledger}). Reservation burns the gate's randomness identifiers \emph{before} any preprocessing share is issued, so no label is ever issued twice. \lstate{PREPARED} lets the module issue the authorized party-local preprocessing exactly once; it is not permission to release an unchecked result. \lstate{CONSUMED} records the one-time use of verified openings and preprocessing, and \lstate{RELEASED} records that the result left the module under a certificate. Any invalid transition or failed check moves the gate to \lstate{ABORTED} and poisons the whole epoch: outstanding output responses are gated, no new challenge is derived, and aborted reservations never return to a free list.

\textbf{Freeze semantics.}
Before any checking challenge is drawn, $T_b$ copies the exact submitted value and tag bytes into protected storage, or spills them into AEAD-protected immutable pages~\cite{dworkin2007gcm} bound to sequence numbers, exact lengths, gate identifiers and a protected root. It hashes the complete descriptor and these bytes into a frozen root $h_b$, and the two modules agree on the ordered pair $(h_0,h_1)$. A host's claim that ``this buffer has hash $h$'' is not a freeze, and neither is DMA completion. After challenge generation, $T_b$ rereads only authenticated frozen pages and never verifies one buffer but consumes a later, host-modified one. This closes the time-of-check-to-time-of-use window (S3) that exists whenever checked data live in host or GPU memory.

\textbf{Release certificates and the guard.}
A release certificate binds the session, epoch, gate, recipients, output encoding or hash and terminal status. A missing peer acknowledgement can cause an abort, but it never authorizes output under a different transcript. The release guard is a small state machine in front of the module's output path (\cref{sec:arch-hw}); its enabling inputs originate from the protected checkers and the ledger, never from host-writable registers, so a host cannot open it by writing a status bit (S6). Resetting the guard is not a secure session reset.

\textbf{Reboot and rollback.}
After a reboot, either a separately justified trusted monotonic service preserves freshness~\cite{parno2011memoir,matetic2017rote}, or the old master key is irrecoverably erased and a freshly attested session is required. A host-controlled counter file is not anti-rollback protection, because the host can restore an old copy and replay old masks (S4).

% ======================================================================
\subsection{Malicious Generate-and-Consume}\label{sec:proto-gac}

\textbf{From semi-honest to malicious GaC.}
Trusted DFA merges DPF generation and evaluation so that each correction word is consumed as soon as it is produced~\cite{dfa2026trusted}. Its simplified description leaves implicit the relation between the root control bits, the payload and role inputs, and whether the evaluator advances with the generator's control state or with its own; a malicious-security proof must fix all three. \Cref{alg:gac} keeps \emph{two} generator states $(s_0,t_0)$ and $(s_1,t_1)$ on the target path exactly as in \cref{alg:gen}, and a \emph{separate} evaluator state $(\tilde s,\tilde t)$ on the query path exactly as in \cref{alg:eval}; bits are read most-significant first and $t\cdot s$ denotes a conditional XOR. The generator starts from $t_0=0$ and $t_1=1$, while the evaluator starts from its own root seed and the fixed control bit $b$, never from a later generator state. Each correction word is computed from the generator's old control bits, applied to both evaluator children under the evaluator's old bit $\tilde t$, and erased only after that use.

\textbf{Why the states cannot be shared.}
The generator and evaluator paths coincide only while the query prefix equals the target prefix. Once $x$ leaves the target path, the two parties' evaluator states become identical and must receive identical corrections so that their outputs cancel (\cref{thm:dpf-correct}). The generator bits, which satisfy $t_0\oplus t_1=1$ along the target path, would instead apply different corrections to the two parties and break that cancellation. The coupling argument of \cref{thm:gac} therefore needs the two state sets kept apart, and the pipeline implements them as distinct generation and evaluation contexts with separate old-control registers (\cref{sec:arch-pipe}).

\textbf{Inputs and outputs.}
The query $x$ is read from a verified masked opening of the same gate, for instance the opened vector of a LUT gate (\cref{alg:lut}), never from unchecked host data. The target $\alpha$ and payload $\beta$ come from the gate's protected preprocessing record, so they are joint draws or joint functions of joint draws (\cref{sec:proto-refactor}). By \cref{thm:dpf-correct,thm:gac}, the raw outputs satisfy $\tilde y_0+\tilde y_1=\beta\cdot\one[x=\alpha]$, but $\tilde y_b$ never leaves the module: the epilogue lines of \cref{alg:gac} replace it with a freshly authenticated tuple. For full-domain uses such as LUT gates and PIR, the evaluator lines become the depth-first $\EvalAll$ traversal of \cref{alg:eval}; each $\CW^{(i)}$ then stays in protected registers until its last evaluator use, which costs $O(n)$ words and is covered by the same node-by-node coupling.

\textbf{Work.}
Per level, each module expands two generator states and one evaluator state, so the two modules together perform six expansions per level where one external generation plus two evaluations performs four (\cref{tab:gatecost}). \sys therefore does not eliminate duplicated generation. What it avoids is the $t$ additional tag trees of the tag-tree alternative, which multiply PRG work by $1+t=4$. On the modeled DFA datapath, single-path throughput at $n=61$ is \est{106}~M gates/s for \sys, against \est{113}~M gates/s for semi-honest trusted DFA and \est{26.7}~M gates/s for tag trees (\cref{fig:dpfthr}).

\begin{algorithm}[t]
\algstretch
\small
\caption{Malicious generate-and-consume with fresh authentication (\algname{GaC-Auth}) inside $T_b$}
\label{alg:gac}
\begin{algorithmic}[1]
\Require role $b\in\{0,1\}$; gate label $\ell$; public query $x\in\bits{n}$ from the gate's frozen, verified opening; target $\alpha\in\bits{n}$ and payload $\beta\in\Fp$ from the protected record of $\ell$; session key $K$; global keys $\Delta_1,\dots,\Delta_t$
\Ensure $\authb{y}{b}=(y_b,\gamma_{b,1},\dots,\gamma_{b,t})$ with $y_0+y_1=\beta\cdot\one[x=\alpha]$ and $\gamma_{0,j}+\gamma_{1,j}=\Delta_j(y_0+y_1)$
\If{gate $\ell$ is not \lstate{VERIFIED} in the ledger}
  \State \Abort{} and poison the epoch
\EndIf
\LineComment{Joint draws: identical labels in $T_0$ and $T_1$, no role appended}
\State $s_0\gets\PRF_K(\ell,\mathsf{root}_0)$;\ $s_1\gets\PRF_K(\ell,\mathsf{root}_1)$;\ $t_0\gets 0$;\ $t_1\gets 1$
\State $(\tilde s,\tilde t)\gets(s_b,b)$ \Comment{separate evaluator}
\For{$i=1$ \textbf{to} $n$}
  \LineComment{(Gen) both roots on the target path; updates use the old $t_c$}
  \State $(s_c^L,t_c^L,s_c^R,t_c^R)\gets\PRG(s_c)$ for $c\in\{0,1\}$
  \State $a\gets\alpha_i$;\ $\keep\gets a$;\ $\lose\gets 1-a$ \Comment{$L\equiv 0$, $R\equiv 1$}
  \State $\sCW\gets s_0^{\lose}\oplus s_1^{\lose}$
  \State $\tCW{L}\gets t_0^L\oplus t_1^L\oplus a\oplus 1$;\ \ $\tCW{R}\gets t_0^R\oplus t_1^R\oplus a$
  \State $(s_c,t_c)\gets\big(s_c^{\keep}\oplus t_c\cdot\sCW,\ t_c^{\keep}\oplus t_c\cdot\tCW{\keep}\big)$, $c\in\{0,1\}$
  \LineComment{(Eval) own query path; corrections use the old $\tilde t$}
  \State $(\hat s^L,\hat t^L,\hat s^R,\hat t^R)\gets\PRG(\tilde s)$
  \State $(\hat s^L,\hat t^L)\gets\big(\hat s^L\oplus\tilde t\cdot\sCW,\ \hat t^L\oplus\tilde t\cdot\tCW{L}\big)$
  \State $(\hat s^R,\hat t^R)\gets\big(\hat s^R\oplus\tilde t\cdot\sCW,\ \hat t^R\oplus\tilde t\cdot\tCW{R}\big)$
  \State $(\tilde s,\tilde t)\gets(\hat s^{x_i},\hat t^{x_i})$
  \State erase $\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$ \Comment{after its evaluator use}
\EndFor
\LineComment{(Gen) output correction from the final generator states}
\State $u_c\gets\Conv(s_c)$ for $c\in\{0,1\}$;\ \ $\CWout\gets(-1)^{t_1}(\beta-u_0+u_1)$
\LineComment{(Eval) raw share, never exported}
\State $\tilde y_b\gets(-1)^b\big(\Conv(\tilde s)+\tilde t\cdot\CWout\big)$; erase $s_c$, $t_c$, $\CWout$
\LineComment{(Epilogue) fresh uniform pads, distinct labels per output wire}
\State $\zeta\gets\PRF_K(\ell,\mathsf{pad}_0)$;\ \ $\kappa_j\gets\PRF_K(\ell,\mathsf{pad}_j)$ for $j\in[t]$
\State $y_b\gets\tilde y_b+(-1)^b\zeta$
\State $\gamma_{b,j}\gets\Delta_j\,y_b+(-1)^b\kappa_j$ for $j\in[t]$
\State mark $\ell$ \lstate{CONSUMED}; erase $\tilde y_b$, $\zeta$, $\kappa_1,\dots,\kappa_t$, $(\tilde s,\tilde t)$
\State \Return $\authb{y}{b}$ to the output FIFO behind the release guard
\end{algorithmic}
\end{algorithm}

% ======================================================================
\subsection{Fresh Authentication Epilogue}\label{sec:proto-epilogue}

\textbf{Construction.}
Let $\tilde y_0,\tilde y_1$ be raw local shares computed inside the two protected evaluators, with $\tilde y_0+\tilde y_1$ equal to the intended gate value. Both modules derive fresh common pads $\zeta,\kappa_1,\dots,\kappa_t\getsr\Fp$ from joint labels that are distinct for every output wire, and $T_b$ returns
\begin{equation*}
y_b=\tilde y_b+(-1)^b\zeta,\qquad \gamma_{b,j}=\Delta_j\,y_b+(-1)^b\kappa_j\quad (j\in[t]).
\end{equation*}
The pads cancel in $y_0+y_1$ and in $\gamma_{0,j}+\gamma_{1,j}=\Delta_j(y_0+y_1)$, so the result is an authenticated sharing of $\tilde y_0+\tilde y_1$. Because $\zeta\mapsto y_b$ and each independent $\kappa_j\mapsto\gamma_{b,j}$ are bijections on $\Fp$, a fixed party's value and $t$ tags are jointly uniform, each tuple having probability $p^{-(t+1)}$ regardless of the gate value and the global keys (\cref{thm:epilogue}). Fresh pads make this hold jointly across outputs; correlations created by later arithmetic are handled by the circuit simulation of \cref{thm:main}.

\textbf{Why it replaces tag trees.}
The direct way to authenticate an FSS output is to evaluate $t$ further DPFs with payloads $\Delta_j\beta$, which yields tag shares but multiplies tree work by $1+t$. The epilogue instead exploits the linearity of the MAC. Because $T_b$ knows the global $\Delta_j$, the tag of the reconstructed value is the sum of the per-party products $\Delta_j y_b$; the pad $\kappa_j$ hides $\Delta_j y_b$ from host $b$, which knows $y_b$ and could otherwise divide it out. The pad $\zeta$ rerandomizes the raw DPF share, so no host ever sees $\tilde y_b$. Consequently the proof needs neither a zero or nonzero pattern assumption on raw DPF outputs nor a DPF one-key-privacy term for the non-key-exporting profile (\cref{thm:main}). The cost is one raw DPF computation, three field multiplications and four fresh pads per party and output, and the output is a 32~B tuple.

\textbf{API restriction.}
The epilogue accepts only results computed inside the module, namely the DPF, DCF, LUT, interval and direct gates of \cref{sec:proto-gates,sec:proto-direct} and the PIR reductions of \cref{sec:proto-pir}, or results from an explicitly verified backend such as the frozen-operand Freivalds check of \cref{sec:proto-freivalds}. There is no \cmd{authenticate(host_value)} entry point. With one, the module would become a MAC oracle: a malicious host could obtain valid tags on any value it wishes to open, and \CheckOpen{} would accept the forgery with probability one (S2). Since the trusted boundary excludes the GPU SMs and memory, a malicious-secure extension must never compute an unchecked result on the GPU and ask the module to authenticate it.

% ======================================================================
\subsection{Freeze-Before-Challenge CheckOpen}\label{sec:proto-check}

\begin{algorithm}[t]
\algstretch
\small
\caption{Freeze-before-challenge authenticated opening (\CheckOpen) inside $T_b$}
\label{alg:checkopen}
\begin{algorithmic}[1]
\Require descriptor and nonempty ordered list of expected wires $(\omega_i)_{i\in[m]}$; host $b$'s tuples $(x_{b,i},\gamma_{b,j,i})_{i\in[m],\,j\in[t]}$; key shares $(\Delta_{b,j})_{j\in[t]}$
\Ensure verified openings $(z_i)_{i\in[m]}$ with bound certificates, or \Abort
\If{metadata, field encoding, gate order or length mismatch the ledger}
  \State \Abort{} and poison the epoch
\EndIf
\LineComment{Step 1: freeze, then agree on both roots}
\State copy the exact bytes into protected SRAM or sealed AEAD pages; $h_b\gets\Hash(\text{descriptor},\text{frozen bytes})$; mark \lstate{FROZEN}
\State exchange $(h_b,\mathit{cid})$ with $T_{1-b}$; \Abort{} unless both hold the same $(h_0,h_1)$ and $\mathit{cid}$
\LineComment{Step 2: reconstruct candidates inside the modules}
\State exchange the frozen value shares $(x_{b,i})_{i\in[m]}$ with $T_{1-b}$
\State $z_i\gets x_{0,i}+x_{1,i}$ for $i\in[m]$ \Comment{not exposed to the host}
\LineComment{Step 3: internal challenges, only after both freezes}
\State $\rho_{j,i}\gets\PRF_K(\mathsf{chk},h_0,h_1,\mathit{cid},j,i)$ for $j\in[t]$, $i\in[m]$
\LineComment{Step 4: per-lane residuals from frozen pages only}
\State $\sigma_{b,j}\gets\sum_{i=1}^{m}\rho_{j,i}\,(\gamma_{b,j,i}-\Delta_{b,j}z_i)$ for $j\in[t]$
\State exchange $(\sigma_{b,j})_{j\in[t]}$ with $T_{1-b}$
\LineComment{Step 5: decide and release}
\If{$\sigma_{0,j}+\sigma_{1,j}=0$ for every $j\in[t]$}
  \State agree on output digest and status; mark \lstate{VERIFIED}, resources \lstate{CONSUMED}
  \State \Return $(z_i)_{i\in[m]}$ with certificates bound to session, epoch, gates and output hash
\Else
  \State release no candidate value; poison the epoch; return one generic failure status
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_checkopen.pdf}
    \caption{Freeze-before-challenge \CheckOpen{} between the two modules. Challenges $\rho_{j,i}$ are derived only after both frozen roots are agreed, and $T_b$ rereads only its frozen pages, so a host that overwrites its DMA buffer after the freeze changes nothing that is checked or consumed.}
    \label{fig:checkopen}
\end{figure}

\textbf{Role.}
Openings are the only places where a value produced by the untrusted GPU becomes public or feeds a protected gate: the masked differences of every multiplication, the masked inputs of every FSS gate and the masked outputs. \CheckOpen{} (\cref{alg:checkopen}, \cref{fig:checkopen}) is a SPDZ-style batched MAC check~\cite{damgard2012spdz,damgard2013practical} rebuilt for a verifier that reads its inputs from untrusted memory. All peer messages use the protected channel, and candidates, challenges and residuals never leave the modules; only an accepted batch releases $z$ with bound certificates.

\textbf{Why freeze first.}
If challenges existed before the bytes were fixed, a host able to submit after seeing them could place its errors in their kernel. If the module checked one buffer and later read another, a host could pass the check with correct shares and then swap in modified ones (S3). Freezing before challenge generation fixes the value-error vector $e$ and the tag-error vectors $d_j$ before any $\rho_{j,i}$ is drawn, and rereading only frozen pages makes the checked and the consumed bytes identical. Challenge labels bind both frozen roots and the check identifier, so no challenge is reused for another batch.

\textbf{Independent challenge lanes.}
Each lane has its own challenge vector. The complete residual of lane $j$ is $\inner{\rho_j}{d_j-\Delta_j e}$, which for $e\neq 0$ vanishes with probability below $2/p$; independence across lanes multiplies these bounds to $(2/p)^t$ (\cref{thm:mac-sound}). A single vector shared by all lanes does not justify the product. For the value error $e=(\varepsilon,-\varepsilon,0,\dots,0)$ with untouched tags, every lane's residual equals $-\Delta_j\varepsilon(\rho_1-\rho_2)$, so the single event $\rho_1=\rho_2$ cancels all lanes at once with probability $1/p$; \sys rejects such configurations (\cref{tab:attacks}). Nor is the bound a claim that tag-only tampering is always detected: an error confined to one tag lane escapes with probability $1/p$ without changing any opened value. Across $Q$ checked batches, an incorrect value is released with probability at most $Q(2/p)^t$, about $2^{-148}$ for $t=3$ and $Q\le 2^{32}$.

\textbf{Key hiding and failure handling.}
The bound relies on the hidden-key invariant of \cref{lem:hidden-key}: until the first accepted wrong opening, the honest key shares stay uniform given the corrupt host's view. \CheckOpen{} preserves it by keeping candidates, challenges and residuals inside the modules, by aggregating the zero tests of all lanes into one generic failure status that exposes no residual, challenge, key or data-dependent diagnostic, and by poisoning the epoch on failure and forbidding retries with the same material, which rules out an adaptive key-learning sequence within an epoch.

\textbf{Traffic and batching.}
Per batch of $m$ elements, the modules exchange two vectors of $m$ field values and two vectors of $t$ residuals plus authenticated metadata. Tags never cross the peer link, but every local tag must be read by its module, so the host-to-module transfer of 32~B per element can remain the bottleneck (\cref{sec:arch-dse}). Because the value shares are frozen before they are sent, root agreement and value exchange can share one message, and our latency model charges two peer round trips per batch. Only independent openings are batched: a dependent nonlinear gate never consumes an unchecked masked opening, and a checkpoint precedes every input-dependent nonlinear output and every final release, since blindly delayed checking is not justified. Larger batches amortize metadata and round trips but increase staging memory and first-result latency. On LAN a batch costs \est{0.101~ms} at $m=64$ and \est{0.652~ms} at $m=65{,}536$, nearly independent of $t$; on WAN the two round trips impose a \est{140~ms} floor that makes batching essential (\cref{sec:eval-check}).

% ======================================================================
\subsection{Inputs, Arithmetic, and Outputs}\label{sec:proto-arith}

\begin{figure*}[t]
\centering
\footnotesize
\setlength{\fboxsep}{4pt}
\fbox{%
\begin{minipage}[t]{0.472\textwidth}
\textbf{Input} $\Pi_{\mathsf{Input}}$\hfill\textit{input $x$ of endpoint $O$ for wire $\omega$}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: reserve label $\ell_\omega$; joint draw $r\getsr\Fp$ and $\authb{r}{b}\gets\AuthShare(r)$; issue $\authb{r}{b}$ to host $b$ once.
\item $T_0,T_1$: send the complete $r$ only to $O$ over its authenticated confidential channel.
\item $O$: send the canonical, authenticated $\epsilon=x-r$ to $T_0$ and $T_1$.
\item $T_0,T_1$: confirm over the protected channel that both hold the same $\epsilon$ and bind it to $\omega$; otherwise \Abort.
\item host $b$: $x_b\gets r_b+\one[b=0]\,\epsilon$;\ \ $\gamma_{b,j}\gets\gamma_{r,b,j}+\Delta_{b,j}\,\epsilon$ for $j\in[t]$.
\end{enumerate}
\textit{Extraction:} a corrupt owner's input is $x^*=r+\epsilon$.
\textit{Committed inputs:} a protected loader verifies the authorized commitment over the frozen canonical stream, then runs \AuthShare{} on the exactly decoded values.

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Linear} $\Pi_{\mathsf{Lin}}$\hfill\textit{local, on host $b$'s GPU}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $\auth{x}+\auth{y}$: add the value shares and each of the $t$ tag shares.
\item $c\cdot\auth{x}$ for public $c$: multiply the value share and every tag share by $c$.
\item $\auth{x}+c$ for public $c$: $x_0\gets x_0+c$ (party~0 only); $\gamma_{b,j}\gets\gamma_{b,j}+\Delta_{b,j}\,c$ for both $b$ and all $j\in[t]$.
\item Tensors: apply steps 1 to 3 elementwise to the value array and to each of the $t$ tag arrays.
\end{enumerate}

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Output} $\Pi_{\mathsf{Out}}$\hfill\textit{private output $y$ for client $O$}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: joint draw a fresh $\auth{o}$ as in step 1 of $\Pi_{\mathsf{Input}}$; send the complete $o$ only to $O$.
\item host $b$: $\auth{w}\gets\auth{y}+\auth{o}$ with $\Pi_{\mathsf{Lin}}$.
\item $w\gets\CheckOpen(\auth{w})$; the release guard opens only for a \mbox{\lstate{VERIFIED}} batch.
\item $T_b$: send $w$ and its release certificate (session, epoch, gate, recipients, output hash, status) to $O$.
\item $O$: verify both certificates for the same $w$ and output $y=w-o$; otherwise abort.
\end{enumerate}
\textit{Public outputs:} $y\gets\CheckOpen(\auth{y})$.
\textit{Never} hand $O$ both parties' tags: $\gamma_{0,j}+\gamma_{1,j}=\Delta_j y$ with a known $y\neq 0$ reveals $\Delta_j$.
\end{minipage}%
\hspace{0.01\textwidth}\vrule\hspace{0.01\textwidth}%
\begin{minipage}[t]{0.472\textwidth}
\textbf{Multiplication} $\Pi_{\mathsf{Mult}}$\hfill\textit{authenticated Beaver triples}

\textit{Scalar} $\auth{z}=\auth{x}\cdot\auth{y}$:
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: reserve a fresh triple $(\auth{a},\auth{b},\auth{c})$ from joint draws, with $c=ab$ computed inside the protected boundary; issue party $b$'s tuples to host $b$ once.
\item host $b$: $\auth{d}\gets\auth{x}-\auth{a}$ and $\auth{e}\gets\auth{y}-\auth{b}$ with $\Pi_{\mathsf{Lin}}$.
\item $(d,e)\gets\CheckOpen(\auth{d},\auth{e})$, batched with the independent openings of the layer.
\item host $b$: $z_b\gets c_b+d\,b_b+e\,a_b+\one[b=0]\,de$.
\item host $b$: $\gamma_{z,b,j}\gets\gamma_{c,b,j}+d\,\gamma_{b,b,j}+e\,\gamma_{a,b,j}+\Delta_{b,j}\,de$ for $j\in[t]$.
\end{enumerate}
\textit{Matrix} $\auth{Z}=\auth{X}\auth{Y}$ with declared dimensions:
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep,start=6]
\item $T_0,T_1$: reserve $(\auth{A},\auth{B},\auth{C})$ with $C=AB$ computed inside the protected boundary; never expose both $A$ and $B$ to a GPU.
\item $D\gets\CheckOpen(\auth{X}-\auth{A})$;\ \ $E\gets\CheckOpen(\auth{Y}-\auth{B})$.
\item host $b$: $Z_b\gets C_b+D\,B_b+A_b\,E+\one[b=0]\,DE$.
\item host $b$: $\Gamma_{Z,b,j}\gets\Gamma_{C,b,j}+D\,\Gamma_{B,b,j}+\Gamma_{A,b,j}\,E+\Delta_{b,j}\,DE$ for $j\in[t]$, preserving the order of every matrix factor.
\end{enumerate}
\textit{Notation:} in $b_b$ and $\gamma_{b,b,j}$ the first $b$ names the triple's second component and the subscript names the party (implementations use named fields); $\Gamma_{\cdot,b,j}$ is party $b$'s lane-$j$ tag matrix.

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Invariants shared by all four protocols}
\begin{itemize}[leftmargin=1.1em,nosep]
\item Every mask and triple is a one-time joint draw bound to session, epoch, gate and purpose, and is issued only from \mbox{\lstate{PREPARED}} (\cref{fig:ledger}).
\item Every opening is a \CheckOpen{} call on frozen bytes (\cref{alg:checkopen}); no opened value feeds a protected gate or a release before it is \mbox{\lstate{VERIFIED}}.
\item Outputs of host $b$'s GPU are candidate shares; no module ever authenticates them.
\end{itemize}
\end{minipage}}
\caption{Authenticated input, linear, multiplication and output protocols of \sys, written for party $P_b$. Steps labeled $T_0,T_1$ or $T_b$ run inside the protected modules; steps labeled host $b$ run on the untrusted GPU and yield only candidate shares until the next \CheckOpen. With honest messages the protocols realize their operations exactly; otherwise they select an allowed input, preserve the computation or abort, except with the probability bounded in \cref{thm:mac-sound} (\cref{thm:arith}).}
\label{fig:arith}
\end{figure*}

\Cref{fig:arith} lists the four protocols that carry values between input owners, GPUs, modules and recipients. Local steps run on host $b$'s GPU over its $1+t$ arrays, masks and triples come from the joint sampler through \cmd{RESERVE_PREP}, and every opening is a \CheckOpen{} call.

\textbf{Inputs.}
The owner $O$ of an input receives the complete fresh mask $r$ over its confidential channel and returns the canonical authenticated difference $\epsilon=x-r$, which both modules bind to the input wire before each party sets $\auth{x}=\auth{r}+\epsilon$. Since $\epsilon$ is uniform for a uniform $r$, the hosts learn nothing about $x$; since both modules bind one $\epsilon$, a corrupt owner cannot feed the two parties different inputs, and its input is extracted as $x^*=r+\epsilon$ (\cref{def:security}). For commitment-bound inputs such as preapproved model weights, a protected loader verifies the authorized commitment over a frozen canonical input stream and applies \AuthShare{} to exactly the decoded values; a host-declared hash does not suffice. This variant lets the modules see the input, which \ProfT permits (\cref{sec:threat-model}); \sys does not claim to hide inputs from its trusted modules.

\textbf{Arithmetic.}
Linear operations act identically on value shares and tags. A public constant $c$ changes only party~0's value share but both parties' tags, by $\Delta_{b,j}c$, which is why host $b$ holds its key shares. Multiplication follows Beaver~\cite{beaver1991efficient} with authenticated triples: the masked differences $d,e$ pass \CheckOpen{} before the product may feed a protected gate or a final release, and the local combination is exact because
\begin{equation*}
c+db+ea+de=ab+(x-a)b+(y-b)a+(x-a)(y-b)=xy .
\end{equation*}
Matrix products use the dimension-correct $Z=C+DB+AE+DE$ with $D=X-A$ and $E=Y-B$, never commuting a factor. Each lane needs two plain matrix products, so an authenticated product costs the GPU $2(1+t)$ products plus the public $DE$. This is why authenticated linear algebra, rather than DPF evaluation, dominates the malicious cost (\cref{sec:analysis-cost}). Conditioned on no accepted wrong opening, these protocols select an allowed input, preserve the computation or abort (\cref{thm:arith}).

\textbf{Outputs.}
A private output $y$ is released only as the checked masked value $w=y+o$, whose mask $o$ is known solely to the recipient $O$; $O$ accepts $w$ only with matching certificates from both modules and computes $y=w-o$. The client never receives both parties' complete MAC tags, since $\gamma_{0,j}+\gamma_{1,j}=\Delta_j y$ together with a known nonzero $y$ would expose $\Delta_j$; integrity toward the client comes from the module certificates instead. Public outputs are opened directly with \CheckOpen{}.


==> qa/draft1/sections/05b_protocol_gates.tex <==
% ==================================================================
% Section V (part 2): authenticated nonlinear gates, direct gates and
% compilation, refactoring, verified GPU products, snapshot PIR.
% Continues the Section opened in 05a_protocol.tex (no \section here).
% ==================================================================

\subsection{Authenticated Nonlinear Gates}\label{sec:proto-gates}

Nonlinear layers of FSS-compiled models reduce to lookups in small public tables and piecewise functions selected by interval tests~\cite{boyle2021function,gupta2023sigma,jawalkar2024orca}. In the semi-honest DFA design, both evaluate a DPF or DCF key on a masked input and pass the raw output shares onward~\cite{dfa2026trusted}. A malicious host can shift the masked input before it selects the DPF path, and it can modify the raw outputs, which carry no MAC. \sys closes both gaps with one template (\cref{fig:gates}): (1)~mask the authenticated input with joint protected randomness (\cref{sec:proto-setup}); (2)~open the masked value with \CheckOpen{} (\cref{alg:checkopen}), so the value that selects the path is verified and frozen; (3)~evaluate the FSS gate inside $T_b$ by generate-and-consume (\cref{alg:gac}); and (4)~authenticate and reshare the raw share with the epilogue (\cref{sec:proto-epilogue}). The host sees only a uniform masked opening and fresh authenticated tuples, and no host-supplied value is ever authenticated, which defeats scenario S2 (\cref{tab:scenarios}).

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_gates.pdf}
    \caption{Authenticated nonlinear gates in \sys. (a)~Small XOR-masked LUT (\cref{alg:lut}): the XOR-masked bit vector $u$ is opened by \CheckOpen{} and $T_b$ scans the full public domain in a fixed order. (b)~Shifted-interval indicator and Horner polynomial (\cref{alg:interval}): one field opening $c=x+r$ serves both translated thresholds $L$ and $H$, which derive from the same mask. (c)~Direct protected gate (\cref{sec:proto-direct}): the module recovers $x=c-r$ inside its boundary and returns a fresh sharing of $g(x)$. In all three cases the host submits only authenticated shares and receives only freshly authenticated outputs; raw FSS shares, DPF keys and, in (c), the plaintext $x$ never leave $T_b$.}
    \label{fig:gates}
\end{figure*}

\begin{algorithm}[t]
\algstretch
\caption{Authenticated small XOR-masked LUT (\algname{LUT-Auth}) for party $b$}
\label{alg:lut}
\begin{algorithmic}[1]
\Require authenticated bits $\authb{x_1}{b},\dots,\authb{x_w}{b}$ of an unsigned $w$-bit $x$, certified Boolean; approved public table $T\in\Fp^{2^w}$ bound in $\mu$ by its hash; gate identifier $\mathit{gid}$; role $b$
\Ensure $\authb{y}{b}$ with $y=T[x]$
\State $T_b$: \cmd{RESERVE_PREP} for $\mathit{gid}$; \Abort{} on any descriptor or table-hash mismatch
\LineComment{Joint preparation inside $T_b$ (same $r$ in $T_0$ and $T_1$)}
\State $r\getsr\bits{w}$ by one joint draw with label $(\mathit{gid},\textsf{mask})$
\State issue $\authb{r_i}{b}\gets\AuthShare(r_i)$ to host $b$ once, for $i=1,\dots,w$
\State bind the joint DPF generator of $(\alpha,\beta)=(r,1)$ to $\mathit{gid}$ \Comment{never resampled}
\LineComment{Masked opening (host $b$ with $T_b$)}
\For{$i=1$ \textbf{to} $w$} \Comment{independent: one batch}
  \State $\authb{u_i}{b}\gets\authb{x_i}{b}+\authb{r_i}{b}-2\,\authb{x_ir_i}{b}$ \Comment{$\Pi_{\mathrm{Mult}}$}
\EndFor
\State $u\gets\CheckOpen(\auth{u_1},\dots,\auth{u_w})$ \Comment{$u=x\oplus r$}
\If{some $u_i\notin\{0,1\}$ or $T_0,T_1$ hold different $u$}
  \State \Abort
\EndIf
\LineComment{Full-domain scan inside $T_b$ in fixed public order; $k_b$ is streamed by GaC and never materialized}
\State $\tilde y_b\gets 0$
\For{$a\in\bits{w}$ in lexicographic order} \Comment{$\EvalAll$, DFS}
  \State $\tilde y_b\gets\tilde y_b+T[a\oplus u]\cdot\DPF.\Eval(k_b,a)$
\EndFor
\State $\authb{y}{b}\gets\Epilogue(\tilde y_b)$ \Comment{\cref{sec:proto-epilogue}}
\State \Return $\authb{y}{b}$
\end{algorithmic}
\end{algorithm}

\textbf{Small XOR-masked LUT.}
\Cref{alg:lut} evaluates an approved public table $T$ with $2^w$ field entries on a $w$-bit input given as authenticated, certified-Boolean bits. The sampler draws a fresh uniform $r\in\bits{w}$ once and uses it twice: for the authenticated bits $\auth{r_i}$ and as the target of the joint DPF for $(r,1)$. The parties open $u=x\oplus r$ in one \CheckOpen{} batch, both modules reject a non-Boolean or mismatching vector, and $T_b$ scans the full domain in a declared fixed order,
\begin{equation*}
    \tilde y_b=\sum_{a\in\bits{w}}T[a\oplus u]\cdot\DPF.\Eval(k_b,a).
\end{equation*}
By \cref{thm:dpf-correct}, the evaluations sum to one only at $a=r$, so $\tilde y_0+\tilde y_1=T[r\oplus u]=T[x]$; since XOR with a fixed $x$ is a bijection on $w$-bit strings, $u$ is uniform given $x$ (\cref{thm:lut}). Both statements need the \emph{same} $r$ as bit mask and DPF target; resampling the target independently keeps the marginals uniform but breaks the proof (\cref{sec:proto-refactor}). In $\EvalAll$ mode the $w$ correction words stay in protected registers until their level is fully expanded, so no key is materialized outside $T_b$. Besides the $w$ XOR products (one batched multiplication round when the bits exist; otherwise bit decomposition is charged to the gate), the gate needs one batched opening, $2^w-1$ internal tree expansions and a $2^w$-term field reduction. In our model, $w=8$ costs \est{542} AES blocks and \est{268} field multiplications (\est{72.27}~M gates/s), $w=12$ costs \est{8,238} AES blocks (\est{4.75}~M gates/s), and $w=16$ falls to \est{0.30}~M gates/s (\cref{tab:gates}): small tables are practical, full-domain tables over 64-bit inputs are not.

\begin{algorithm}[t]
\algstretch
\caption{Authenticated shifted intervals and piecewise polynomial (\algname{Interval-Auth}) for party $b$}
\label{alg:interval}
\begin{algorithmic}[1]
\Require $\authb{x}{b}$; public breakpoints $0=\tau_0<\tau_1<\dots<\tau_m=p$ with $m\ge2$; public coefficients $a_{i,j}\in\Fp$ of $P_i(x)=\sum_{j=0}^{d}a_{i,j}x^j$; gate identifier $\mathit{gid}$; role $b$
\Ensure $\authb{y}{b}$ with $y=P_i(x)$ for the unique $i$ such that $\tau_i\le x<\tau_{i+1}$
\State $T_b$: \cmd{RESERVE_PREP} for $\mathit{gid}$; $r\getsr\Fp$ by one joint draw (rejection sampling); issue $\authb{r}{b}\gets\AuthShare(r)$ once
\State $c\gets\CheckOpen(\auth{x}+\auth{r})$ \Comment{$c=x+r\bmod p$}
\LineComment{Indicators inside $T_b$; every endpoint and wrap bit derives from the same $r$}
\For{$i=0$ \textbf{to} $m-1$}
  \State $L_i\gets(\tau_i+r)\bmod p$;\; $H_i\gets(\tau_{i+1}+r)\bmod p$
  \State $\omega_i\gets\one[L_i>H_i]$ with a sharing $(\omega_{i,0},\omega_{i,1})$
  \State $\tilde s_{i,b}\gets\omega_{i,b}+\DCF_{H_i}(c)_b-\DCF_{L_i}(c)_b$ \Comment{GaC}
  \State $\authb{s_i}{b}\gets\Epilogue(\tilde s_{i,b})$ \Comment{$s_i=\one[\tau_i\le x<\tau_{i+1}]$}
\EndFor
\LineComment{Coefficient selection and Horner evaluation (host $b$, authenticated arithmetic)}
\For{$j=0$ \textbf{to} $d$}
  \State $\authb{\bar a_j}{b}\gets\sum_{i=0}^{m-1}a_{i,j}\,\authb{s_i}{b}$ \Comment{local, $\Pi_{\mathrm{Lin}}$}
\EndFor
\State $\authb{y}{b}\gets\authb{\bar a_d}{b}$
\For{$j=d-1$ \textbf{down to} $0$}
  \State $\authb{y}{b}\gets\authb{y\cdot x}{b}+\authb{\bar a_j}{b}$ \Comment{$\Pi_{\mathrm{Mult}}$}
  \State rescale exactly where $\mu$ specifies (\cref{alg:trunc})
\EndFor
\State \Return $\authb{y}{b}$
\end{algorithmic}
\end{algorithm}

\textbf{Shifted intervals.}
For a proper nonempty public interval $[a,b)\subsetneq[0,p)$ (here $a,b$ are endpoints, not party indices), \cref{alg:interval} opens $c=x+r\bmod p$ for a fresh field mask $r$, and $T_b$ derives from the same $r$
\begin{equation*}
    L=(a+r)\bmod p,\quad H=(b+r)\bmod p,\quad \omega=\one[L>H].
\end{equation*}
With conservative DCFs for thresholds $L$ and $H$ (\cref{alg:dcf}; orientation $\one[c<\theta]$, payload $1$, independent coins) and a sharing of the wrap bit $\omega$, the raw share $\tilde s_b=\omega_b+\DCF_H(c)_b-\DCF_L(c)_b$ goes to the epilogue. Translation by $r$ maps $[a,b)$ onto the circular half-open interval from $L$ to $H$ ($L\neq H$ since $0<b-a<p$): the indicator is $\one[c<H]-\one[c<L]$ if $L<H$ and $1+\one[c<H]-\one[c<L]$ if the interval wraps, so \cref{thm:dcf} gives $\tilde s_0+\tilde s_1=\one[a\le x<b]$ (\cref{thm:interval}). Empty and full intervals are public constants. A partition may share one mask and one opening if every endpoint, wrap bit and auxiliary share is derived jointly from that mask, while distinct DCFs keep independent coins. The conservative DCF evaluates $n(n+1)/2$ path levels (1{,}891 for $n=61$), so an interval gate costs \est{22,692} AES blocks (\est{1.73}~M gates/s). An $O(n)$ DCF in the style of~\cite{boyle2021function,storrier2023grotto} would bring the projected cost to \est{976} blocks (\est{40.13}~M gates/s), but it is not covered by \cref{thm:dcf} and may replace \cref{alg:dcf} only after its correctness, distribution and interface obligations and measured cost are established; we report it only as a projection.

\textbf{Piecewise polynomials.}
Activation and normalization functions are approximated by low-degree polynomials on a public partition~\cite{gupta2023sigma,pang2024bolt,ma2023secretflow}. The parties select coefficients $\auth{\bar a_j}=\sum_i a_{i,j}\auth{s_i}$ locally ($\Pi_{\mathrm{Lin}}$, \cref{fig:arith}) and apply Horner's rule with $d$ authenticated products, independently of the number $m$ of pieces. Exactly one indicator of a disjoint exhaustive partition is one, so \cref{thm:arith} yields the active polynomial; rescaling is inserted where the manifest specifies it (\cref{alg:trunc}). Approximation error of the approved coefficients is distinct from the cryptographic correctness of \cref{thm:lut,thm:interval}, which concerns the declared finite arithmetic.

\textbf{Exact comparison, bit decomposition and truncation.}
The LUT input, exact threshold comparisons and signed truncation need canonical bits. \Cref{alg:bitdec} (\cref{app:proof-gates}) opens $c=x+r\bmod p$ for a mask with authenticated canonical bits and subtracts $r$ from $c$ with an authenticated ripple-borrow circuit; the final borrow $\one[c<r]$ flags a wrap, in which case $x=d-1$ for the subtractor output $d$ because $p=2^n-1$, and a second subtract-one pass applies this without branching (\cref{thm:bitdec}). \Cref{alg:trunc} compares bits with a public threshold by a most-significant-bit-first equality and less-than chain, and truncates a centered signed $z$ toward zero via the sign $s=\one[z_{\mathrm{can}}\ge(p+1)/2]$ of its canonical representative, the decomposed magnitude $(1-2s)z$, a bit shift and sign restoration, giving $\mathrm{sgn}(z)\lfloor|z|/2^f\rfloor$ while the declared magnitude stays below $p/2$ (\cref{thm:cmp-trunc}); see~\cite{damgard2006unconditionally,catrina2010improved,escudero2020edabits} for the underlying techniques.

\textbf{Why exact circuits are a fallback.}
These circuits need only authenticated arithmetic, but their carry chains cannot be shortened by batching: \cref{alg:bitdec} performs $2n=122$ dependent multiplications for $n=61$, hence $2n+1=123$ sequential verified openings (\est{12.3~ms} on LAN), and exact truncation needs \est{307} rounds (\est{30.7~ms}). At two round trips per verified opening (\cref{sec:proto-check}), the 123-round chain would take about \est{17.2~s} on WAN. A valid one-round candidate therefore always wins under the cost rule below, and exact circuits are used only when no such candidate meets the gate's contract, with their cost charged to any LUT whose input bits do not yet exist.

\subsection{Direct Protected Gates and Cost-Aware Compilation}\label{sec:proto-direct}

\textbf{The direct protected gate.}
After a verified opening $c=x+r$, each module holds $c$ and $r$ and can compute $x=c-r$ inside its boundary, evaluate an approved deterministic gate $g$, and return a fresh authenticated sharing of $g(x)$ through \AuthShare{} (\cref{fig:gates}(c)). This is secure in the same model and with the same output simulation as the FSS gates, since the host again receives a fresh, independently uniform value and tag tuple (\cref{thm:epilogue}), provided the module's observable trace while computing $g$ meets the same simulatability assumption ($\eps{trace}$ in \cref{thm:main}). Concretely, fetching $T[x]$ from host memory or running in $x$-dependent time would leak $x$, so approved direct gates run from protected memory in data-independent time. In our model a direct gate needs one verified opening, \est{2} AES blocks and \est{5} field multiplications, and sustains \est{1,800}~M gates/s, above every FSS realization in \cref{tab:gates}.

\textbf{What FSS gates do not hide.}
\sys does not claim that inputs are hidden from its trusted modules. In \cref{alg:lut,alg:interval} each module also holds $r$ and receives $c$, so it could compute $x$ as the direct gate does, and under \ProfT the modules already see committed inputs through the protected loader (\cref{sec:proto-arith}). FSS thus gains no formal confidentiality over the direct gate, which is a legitimate competitor that we evaluate as such.

\textbf{Cost-aware selection.}
For each nonlinear gate shape, the compiler measures or calibrates a cost tuple (latency, bytes, protected memory, field operations, PRG calls) for the direct gate, a small XOR LUT, an interval or polynomial FSS gate, and a separately proven malicious backend. It rejects candidates that violate the gate's semantic and security contract (the exact finite function, encoding and rescaling fixed by $\mu$ under the profile in force) and selects the least measured or calibrated end-to-end cost among the rest, accounting for dependency depth and transport. Only independent checks are batched: larger batches amortize descriptor handling, challenge derivation and latency (\cref{sec:eval-check}) but increase staging memory and first-result latency. A checkpoint precedes every input-dependent nonlinear output and final release, since \cref{thm:mac-sound} does not justify blind delayed checking. Once authenticated linear algebra dominates (\cref{sec:analysis-cost}), the choice matters little: for BERT-Base, direct-only compilation changes the estimated LAN latency from \est{3.83~s} (compiler-selected default) to \est{3.82~s}, while conservative FSS-only compilation raises it to \est{15.29~s} and the projected optimized DCF gives \est{4.20~s} (\cref{tab:ablation}).

\textbf{Why FSS stays in the datapath.}
If the direct gate is at least as cheap under \ProfT, why keep DPF generation and evaluation in the module? (i)~\emph{Compatibility.} Sigma- and Orca-style toolchains~\cite{gupta2023sigma,jawalkar2024orca} compile nonlinear layers into masked-input FSS gates, and \ProfU (\cref{sec:threat-profileu}) runs the circuit through an established malicious backend whose DPF keys the accelerator evaluates as party-local data; there the direct candidate is invalid because the hardware is not trusted with $x$. One DPF datapath serves both profiles and the untrusted-mode DFA workloads. (ii)~\emph{Full-domain scans.} PIR and small-LUT gates are data-independent, fixed-order streams of AES expansions, exactly what the pipelined DPF units execute at one iteration per cycle (\cref{sec:arch-hw}). (iii)~\emph{Short-lived sensitive state.} FSS keeps long-running evaluation state pseudorandom (seeds and correction words), and index- or input-dependent state short-lived. We treat (iii) only as defense in depth against physical and microarchitectural threats that \ProfT excludes (\cref{sec:discussion}); no theorem depends on it. The evaluation reports direct-only, FSS-only and compiler-selected configurations side by side (\cref{sec:eval-ablation}).

\subsection{Distribution-Preserving Refactoring}\label{sec:proto-refactor}

DFA decouples DPF generation from protocol preprocessing by sampling the target directly as a uniform value and recovering the mask $r$ through $g^{-1}$ when the protocol's transformation $g$ is a bijection~\cite{dfa2026trusted}. \sys relies on the same idea to draw every target from the joint sampler, with two refinements of the semi-honest argument.

\textbf{Uniform targets are an application requirement.}
DPF key privacy holds for arbitrary targets~\cite{boyle2015fss,boyle2016function}; uniformity is needed by the application, which publishes $c=x+r$ or $u=x\oplus r$. A refactoring must therefore preserve the \emph{joint} distribution of the preprocessing, not the uniformity of each target.

\textbf{Joint, not marginal, distributions.}
A gate's preprocessing contains correlated objects: the mask, its bits, DPF or DCF targets, wrap bits and auxiliary shares. If a gate needs targets $r$ and $r+1$, resampling each uniformly keeps the marginals but destroys their unit difference; drawing $L$ and $H$ of \cref{alg:interval} independently likewise yields a wrong indicator. \Cref{lem:bijection} states the exact condition: for a fixed context $z$, a uniform $R$ on a finite set, a bijection $g_z$ and an auxiliary sampler $J$ with independent coins $W$, the tuple $(R,g_z(R),J(z,R,W))$ is distributed exactly as $(R',A,J(z,R',W))$ with $A$ uniform and $R'=g_z^{-1}(A)$. The refactoring is valid exactly when the map is a bijection for the fixed context \emph{and} all auxiliary material is regenerated from $R'$ by the unchanged sampler; e.g., \cref{alg:interval} may draw $L$ uniformly, set $r=L-a$ and derive $H$ and $\omega$ from that $r$, but may not draw $L$ and $H$ independently.

\textbf{Noninvertible maps and truncation.}
For an arbitrary $g$, \cref{lem:noninv} samples $A$ from the law of $g(R)$ and then $R'$ from the conditional law of $R$ given $g(R)=A$, which reproduces $(R,g(R))$ exactly since $\Pr[A=a]\Pr[R=r\mid g(R)=a]=\Pr[R=r,g(R)=a]$. For unsigned truncation of a uniform $\ell$-bit mask by $h$ bits, the sampler draws $A$ uniform on $\ell-h$ bits and $U$ uniform on $h$ bits and sets $R'=2^hA+U$, so every mask has probability $2^{-\ell}$; this makes the DFA truncation rule (shift left, fill the low bits uniformly~\cite{dfa2026trusted}) exact. Signed shifts, nonuniform masks and other moduli need their own conditional samplers.

\textbf{Implications.}
Every refactored draw uses one joint-sampler label per correlated object (\cref{sec:proto-setup}), and the proof of \cref{thm:main} applies \cref{lem:bijection,lem:noninv} only where their conditions hold (\cref{app:proof-main}).

\subsection{Verified GPU Matrix Products}\label{sec:proto-freivalds}

Authenticated linear layers need no extra verification: a GPU deviation that changes a value is caught at the next \CheckOpen, before the result enters a protected gate or a release, except with the probability bounded in \cref{thm:mac-sound}. A module that must \emph{consume} a GPU-computed matrix before any opening, however, must not accept it on the host's word, which would reintroduce the forgery oracle of scenario S2. For this case \cref{alg:freivalds} (\cref{app:proof-gates}) is an optional frozen-operand Freivalds check~\cite{freivalds1977probabilistic}, in the spirit of Slalom~\cite{tramer2018slalom} but bound to the ledger.

\textbf{Permitted uses and check.}
The check applies only when exposing the operands to that GPU is already allowed, as in public-by-party-local matrix products; it never permits exposing global secret triple masks, which are generated inside the TCB (\cref{sec:proto-arith}). The module binds the exact operand bytes $A\in\Fp^{m\times k}$ and $B\in\Fp^{k\times n}$ to their authoritative records and freezes the claimed $C$ (\cref{sec:proto-ledger}); only then does it draw $s$ independent secret uniform $v\in\Fp^{n}$, test $Cv\stackrel{?}{=}A(Bv)$ inside the protected verifier, and consume only the verified frozen bytes of $C$ (\cmd{VERIFY_MATRIX} in \cref{tab:commands}). If the GPU also transforms tag arrays, their tag equations are verified too.

\textbf{Soundness and cost.}
If $C\neq AB$, a nonzero row $e$ of $C-AB$ gives $\inner{e}{v}=0$ with probability exactly $1/p$, so acceptance has probability at most $p^{-s}$ (\cref{thm:freivalds}); freezing prevents choosing the error after seeing $v$, and binding prevents verifying one product and consuming another. With $s=3$ each call errs with probability at most $p^{-3}\approx2^{-183}$, and $Q_F$ calls add $Q_F/p^{3}$ to the bound of \cref{thm:main}. Each repetition costs $O(kn+mk+mn)$ field operations plus reading the bound matrices. The check is disabled in all evaluated configurations; enabling it adds implementation obligations (\cref{tab:obligations}) and its error term.

\subsection{Versioned-Snapshot PIR}\label{sec:proto-pir}

In DPF-based two-server PIR (\cref{eq:pir}), a malicious server can return a wrong share, which the client silently reconstructs into a wrong record, or answer from a stale database. \Cref{alg:pir} and \cref{fig:pir} show the \sys countermeasures.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_pir.pdf}
    \caption{Versioned-snapshot PIR (\cref{alg:pir}). Both modules bind the same query, scan the same snapshot bytes in a public order, hash exactly the bytes they consume, and quarantine the DPF-weighted reduction until the hash matches the authorized commitment $C_v$. A host that swaps a record after hashing or serves an old version causes an abort, never a wrong accepted record (scenario S8).}
    \label{fig:pir}
\end{figure}

\begin{algorithm}[t]
\algstretch
\caption{Versioned-snapshot protected PIR (\algname{PIR-Snap}) inside module $T_b$}
\label{alg:pir}
\begin{algorithmic}[1]
\Require from the client over its confidential channel: index $\alpha$, query identifier $q$, descriptor $\mathsf{desc}_v=(\mathsf{id},v,N,\mathsf{enc},C_v)$; snapshot records $D[0],\dots,D[N-1]$ streamed by host $b$
\Ensure value share $y_b$ of $D[\alpha]$ and certificate $\mathsf{cert}_b$ for the client, or \Abort
\LineComment{Step 1: query binding}
\State exchange $(\alpha,q,\mathsf{desc}_v)$ with $T_{1-b}$ over the protected channel
\If{the bindings differ, $\alpha\ge N$, or $\mathsf{desc}_v$ is unauthorized}
  \State \Abort
\EndIf
\LineComment{Step 2: joint DPF and same-byte scan ($N\ge2$; $N=1$ is a constant-record case with the same checks)}
\State $n\gets\lceil\log_2N\rceil$; bind $N$ and $2^n$; $D[i]\gets0$ for $N\le i<2^n$
\State joint DPF generator for $(\alpha,1)$ under label $(q,\textsf{pir})$ \Comment{GaC}
\State $h\gets\Hash.\mathsf{init}(\mathsf{id},v,N,\mathsf{enc})$;\; $\tilde y_b\gets0$
\For{$i=0$ \textbf{to} $2^n-1$ in public order} \Comment{$\EvalAll$, DFS}
  \If{$i<N$}
    \State read $D[i]$ into $T_b$; $h\gets\Hash.\mathsf{update}(h,D[i])$
  \EndIf
  \State $\tilde y_b\gets\tilde y_b+\DPF.\Eval(k_b,i)\cdot D[i]$ \Comment{per coordinate}
\EndFor
\LineComment{Step 3: snapshot check; the result is quarantined until here}
\If{$\Hash.\mathsf{final}(h)\neq C_v$}
  \State \Abort
\EndIf
\LineComment{Step 4: fresh resharing and certified release}
\State $y_b\gets\tilde y_b+(-1)^b\zeta$ with a fresh joint pad $\zeta$ per coordinate
\State $\mathsf{cert}_b\gets$ certificate on $(\mathsf{sid},\mathsf{ep},q,\mathsf{desc}_v,b,\Hash(y_b))$
\State \Return $(y_b,\mathsf{cert}_b)$ to the client \Comment{no MAC tags}
\end{algorithmic}
\end{algorithm}

\textbf{Protocol and snapshot binding.}
Both role-bound modules receive the same canonical query from the client, compare the binding over their protected channel, pad the snapshot to $2^n$ records while authorizing only $\alpha<N$, and run a joint DPF for $(\alpha,1)$ by generate-and-consume. Each scans the same canonical bytes in the same public order ($2^n-1$ internal expansions, not $n2^n$), applies the same DPF weights to every record coordinate, and hashes exactly the bytes it consumes. The commitment $C_v$ covers the database identifier, version, shape, record encoding and ordered data bytes, and the result stays quarantined behind the release guard (\cref{sec:proto-ledger}) until the hash matches it; a host that swaps a record after hashing or serves an old version therefore causes an abort (scenario S8 in \cref{tab:scenarios}). A Merkle realization~\cite{merkle1987digital} must authenticate every consumed leaf and its position against the same root. Offloading the reduction to the GPU would need \cref{alg:freivalds} or a separately proven authenticated reduction, never a signature on the GPU's claim, and would export the expanded share vector, so \sys reduces inside the module. Each module releases only a freshly reshared value share (the value half of the epilogue) with a bound certificate, and the client reconstructs $D[\alpha]=y_0+y_1$; complete MAC-tag pairs are withheld because revealing $\Delta_jy$ for a known nonzero $y$ would expose the MAC key.

\textbf{Guarantees and regimes.}
\Cref{thm:pir} covers two separate regimes of $\FPIR$ (\cref{fig:func}). With one malicious server host and an honest client, the client obtains the committed record or an abort: on a matching snapshot, \cref{thm:dpf-correct} gives $y_0+y_1=\sum_i(\DPF_0(i)+\DPF_1(i))D[i]=D[\alpha]$ with $\DPF_b(i)=\DPF.\Eval(k_b,i)$; the hash binds the consumed bytes up to collisions, the query comparison fixes one legal $\alpha$, role-bound certificates prevent substituting another query's or version's result, and suppression causes an abort. The corrupt host learns nothing about $\alpha$ beyond the permitted leakage, because query and module traffic are confidential, scan length and order are public, released shares are freshly masked (\cref{thm:epilogue}), and no DPF key or unmasked reduction is exported. In the separate malicious-client-only regime, with both server hosts honest, an accepted request reveals nothing beyond the requested record and the public descriptor: per coordinate, the client receives one fresh uniform share and the record minus that share, and no MAC tags. We make no combined claim for a malicious client together with a malicious server host.

\textbf{Scope and design choice.}
This is a hardware-trusted PIR statement: it does not make untrusted two-server DPF-PIR symmetric, and a vFSS-based external-key alternative~\cite{decastro2022vfss} would have to prove key validity and answer integrity separately. Authenticated PIR~\cite{colombo2023apir} provides integrity without trusted hardware at additional server cost and is our malicious-secure GPU baseline (\cref{sec:eval-pir}). Since both modules learn $\alpha$ under \ProfT, a module could also select $D[\alpha]$ during a plain scan; we keep the DPF form for the reasons of \cref{sec:proto-direct}: the scan must cover the snapshot in public order anyway, the DPF turns it into the AES stream the DPF units accelerate, the datapath matches untrusted-mode DFA PIR, and long-running state stays pseudorandom (defense in depth only). In our model \sys retains about \est{93\%} of the semi-honest DFA throughput, e.g., \est{16,349} versus 17{,}580 queries/s at $N=2^{20}$~\cite{dfa2026trusted} (\cref{tab:pir}).


==> qa/draft1/sections/06_architecture.tex <==
% ======================================================================
% Section VI: Architecture and System Integration
% Labels defined here: sec:arch, sec:arch-insight, sec:arch-hw, sec:arch-pipe,
%   sec:arch-iface, sec:arch-field, sec:arch-deploy, sec:arch-dse,
%   fig:hw, fig:pipeline, tab:commands, lst:mersenne
% ======================================================================
\section{Architecture and System Integration}\label{sec:arch}

This section describes how \sys realizes the protected module $T_b$ of \cref{sec:protocol} next to the GPU and how the untrusted host drives it. We keep the organization of DFA~\cite{dfa2026trusted} wherever the malicious setting permits it and add only the blocks that the integrity chain requires. Hardware sizes are design parameters; area, power and performance values in red are estimates (\cref{sec:eval-hw,app:model}).

% ======================================================================
\subsection{Design Insights}\label{sec:arch-insight}

\textbf{Key insight.}
Malicious security moves the dominant cost away from DPF (\cref{sec:analysis-cost}). For BERT-Base, authenticated linear algebra on the GPU takes \est{2.60~s} of the \est{3.83~s} LAN latency of \sys (\est{68\%}, \cref{fig:motiv}), whereas protected FSS evaluation, exposed triple generation and all \CheckOpen{} work together take \est{0.14~s}. The module therefore need not become a second GPU: it must hold exactly the state whose exposure or modification would break the integrity chain and inspect every byte that crosses its boundary. The GPU is a fast but untrusted engine for authenticated linear algebra, and the module is dealer, verifier and release authority at once.

\textbf{What must be protected.}
A block belongs inside the trusted boundary if it holds material that reveals both parties' views or authorizes a release:
\begin{enumerate*}[label=(\roman*)]
\item session and identity keys and the global MAC keys $\Delta_j$;
\item the joint PRF sampler with its role, epoch and gate counters;
\item DPF generator states and correction words, which under generate-and-consume determine both parties' keys;
\item the table and reduction logic of LUT, interval and PIR gates;
\item check challenges and residuals; and
\item every release decision and certificate.
\end{enumerate*}
The host CPU, OS, driver, runtime, SMs, L2, NoC, HBM, host DRAM and NIC stay outside (\cref{fig:threat}).

\textbf{What stays on the GPU.}
Linear layers run as matrix Beaver products over the value lane and the $t=3$ tag lanes (\cref{fig:arith}), i.e., $1+t$ dense products of the same public shape. The GPU never holds a complete $\Delta_j$ or tag, and any value error it injects propagates to the next opening, where \CheckOpen{} accepts a wrong value with probability at most $(2/p)^t$ per batch (\cref{thm:mac-sound}); tag-only errors cannot change an opened value. A GPU result is a candidate share, never a certified value. Conversely, the module's own work stays light: a malicious GaC gate of depth $n$ costs $6n+3$ AES blocks per module versus $6n+1$ for semi-honest trusted DFA, so at $n=61$ DPF throughput drops only from \est{113} to \est{106}~M gates/s (\cref{fig:dpfthr}).

\textbf{Placement.}
An authenticated element costs 32~B per party at the module interface (\cref{sec:proto-repr}), and BERT-Base moves \est{1.66~GB} per party per query between module and GPU (\cref{tab:e2e}); a link of bandwidth $B$ streams at most $B/32$ elements per second. The L2-adjacent placement of DFA delivers about 290~GB/s to the SMs~\cite{dfa2026trusted}, so we keep it: one DPF unit per L2 slice, a new protected core beside a designated L2 partition, and SM access through the DFA-mapped address range without a new NoC port.

% ======================================================================
\subsection{Hardware Design}\label{sec:arch-hw}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_hw.pdf}
    \caption{\sys hardware. Top: placement inside the GPU; as in DFA, one DPF unit sits next to each L2 slice and a designated slice hosts the VIGOR core. Bottom: logical organization of the protected module $T_b$ (red dashed trusted boundary). The 64 AES-128 engines are time-shared among PRG expansion, challenge derivation and AEAD sealing; the Mersenne-61 field unit array serves epilogues, triples, reductions and check residuals. SMs, L2, NoC, HBM and host DRAM stay outside the boundary.}
    \label{fig:hw}
\end{figure}

As in DFA, 16 DPF units with four AES-128 engines each (64 engines, a 20-stage pipeline, 720~MHz at 28~nm and 910~MHz at 7~nm~\cite{dfa2026trusted}) sit next to the L2 slices, and one slice also hosts the \emph{VIGOR core} (\cref{fig:hw}). The trusted boundary encloses the DPF units, the VIGOR core and the on-die links between them. Only command frames with their share batches, database records scanned for PIR, authenticated output tuples, sealed spill pages and sealed peer and client channel frames cross it, and none of them carries a module secret in the clear. The blocks follow the integrity chain: parser and ledger admit \emph{authorized input}; sampler and field unit array produce \emph{correlated preprocessing}; the DPF units perform \emph{correct local evaluation}; the epilogue yields \emph{authenticated arithmetic}; freezer, check engine and peer channel enforce \emph{consistent opening}; and the release guard gates \emph{authorized output release}.

\textbf{DPF units and sampler.}
The AES datapath is unchanged. Each pipeline context carries two generator states, a separate evaluator state, a DFS stack and the conversion $\Conv$ into $\Fp$, exactly the state of \cref{alg:gac}; correction words are consumed and discarded inside the unit, and raw leaf shares $\tilde y_b$ travel over on-die links to the field unit array rather than to SM-readable buffers. The joint PRF sampler expands the length-prefixed labels of \cref{sec:proto-setup} under the session key and produces field elements by 61-bit rejection sampling, aborting rather than biasing when its retry budget is exhausted.

\textbf{Field unit array (FUA).}
The FUA is a pool of 128 Mersenne-61 multiply-accumulate lanes in the VIGOR core, each with a $61\times 61$-bit multiplier and the two-fold reduction of \cref{lst:mersenne}. It computes epilogues (three products per output), the triple products $c=ab$ and $C=AB$ with their \AuthShare{} tags (so matrix masks never reach the GPU), LUT and PIR reductions, interval sums and check residuals. Its peak is \est{116~G} multiply-accumulates per second at 910~MHz; the \est{7.18~s} of matrix-triple work of one LLaMA2-7B query overlaps the \est{52~s} of GPU authenticated GEMM (\cref{sec:eval-scale}).

\textbf{Check engine and freezer.}
The check engine executes steps~3 and~4 of \cref{alg:checkopen}: it derives the $t$ challenge vectors only after both frozen roots are fixed, accumulates the residuals on FUA lanes (two products per lane and element) and evaluates all lanes over the full batch before emitting one generic status, so neither the status nor its latency reveals which lane or position failed. \cmd{FREEZE_BATCH} copies the exact submitted bytes into a 256~KB freeze SRAM (8{,}192 tuples of 32~B); larger batches are sealed with AES-GCM~\cite{dworkin2007gcm,mcgrew2004gcm} into immutable HBM pages bound to sequence number, exact length, gate identifiers, context and ordered root, while the authoritative root and page counters stay inside. The freezer hashes the descriptor and the frozen bytes into the root $h_b$ that the modules exchange, and after the challenge only authenticated frozen pages are reread, never the host buffer.

\textbf{Ledger, release guard and control.}
A 32~KB ledger SRAM holds the authoritative state of every in-flight gate and the randomness identifiers burnt at reservation (\cref{fig:ledger}). The release guard opens for a gate only in state \lstate{VERIFIED}; its \texttt{ok} inputs are wired from protected checkers rather than host-writable registers, an epoch abort closes every outstanding response atomically, and resetting the guard is not a session reset. The peer-channel controller keeps independent directional keys, never repeats a nonce and enforces a per-session traffic and forgery budget. The SC300-class control core of DFA~\cite{st33tpm12spi,arm_cortex_m3} runs measured boot, attestation and the key establishment covered by $\eps{setup}$, and the 16-lane VPU of DFA~\cite{cavalcante2019ara} handles the remaining protocol logic.

\textbf{AES time-sharing.}
The 64 engines are the module's only AES resource. A slot arbiter per unit serves PRG expansion (two blocks per expansion, $6n+3$ per GaC output), challenge derivation (1.5 blocks per checked element: three 64-bit words for three 61-bit challenges) and AEAD keystream for sealing and the peer channel (two blocks per 32-byte tuple). Check and sealing requests take priority because they are short and on the critical path of the next round; PRG contexts fill all other slots. A per-slot purpose tag selects the key context, so the uses never share a key.

\textbf{Cost.}
The additions occupy \est{4.60~mm$^2$} and \est{1.35~W} at 28~nm (\est{0.145~mm$^2$} and \est{0.508~W} at 7~nm), dominated by the FUA (\est{2.80~mm$^2$}) and the freeze SRAM (\est{1.07~mm$^2$}). With the DFA blocks (7.67~mm$^2$, 1.68~W at 28~nm~\cite{dfa2026trusted}), a complete module occupies \est{0.384~mm$^2$} at 7~nm, \est{0.046\%} of the 826~mm$^2$ A100 die~\cite{nvidia2020ampere} (\cref{tab:hwcost}).

% ======================================================================
\subsection{Pipeline Scheduling and Memory}\label{sec:arch-pipe}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_pipeline.pdf}
    \caption{Scheduling inside a DPF unit. (1)~Generator (g) and evaluator (e) expansions of at least $L$ independent contexts interleave to hide the $L$-cycle AES and correction feedback latency. (2)~AES slots are time-shared among PRG expansion, challenge derivation and AEAD sealing. (3)~Depth-first $\EvalAll$ keeps one pending sibling per level, i.e., $O(n)$ state per context.}
    \label{fig:pipeline}
\end{figure}

\textbf{Context interleaving.}
With an AES and correction feedback latency of $L$ cycles ($L\ge 20$ for the DFA pipeline), one dependent path advances at most one level every $L$ cycles, so one issue per cycle needs at least $L$ independent contexts per unit (\cref{fig:pipeline}, panel~1); DFA already provisions 20 in-flight instances~\cite{dfa2026trusted}. The three expansions of a malicious GaC level issue back to back, because $\PRG(\tilde s)$ does not depend on $\CW^{(i)}$; only the correction waits for all three. A context (three 129-bit path states, the correction word in flight, target, query, payload and level) needs fewer than 100~B, so 20 contexts take less than \est{2~KB} per unit, and a single gate with $n=61$ completes in \est{1.71~$\mu$s}.

\textbf{Separate old controls.}
Corrections use the \emph{old} generator bits $t_0,t_1$ and the \emph{old} evaluator bit $\tilde t$ (\cref{alg:gen,alg:eval}). Since generation and evaluation share correction words but not path states, each unit keeps separate registers for both sets of old controls, captures all outputs of a transition before overwriting its inputs, and never substitutes generator states for evaluator roots, which is exactly the schedule covered by \cref{thm:gac}. Planned RTL tests exercise signed final conversion, zero payloads, all-zero and all-one indices, $x=\alpha$ and divergence at every depth.

\textbf{Depth-first EvalAll.}
LUT and PIR gates evaluate the full domain. Depth-first traversal keeps one pending sibling per level ($O(n)$ states per traversal) and a complete tree needs $2^n-1$ internal expansions (panel~3). The 512 queries of a PIR batch walk the same public leaf order in lockstep, so each snapshot record is read and hashed once per batch and folded into 512 per-query accumulators. For $N=2^{20}$, 512 contexts with 20 pending siblings of 17~B occupy about \est{174~KB}, or \est{11~KB} per unit, which fits the traversal buffers of DFA~\cite{dfa2026trusted}.

\textbf{Pads and frozen buffers.}
The four pads of an output occupy two AES blocks and are drawn in step with the leaf, so no pad buffer beyond the pipeline depth is needed. A checked batch occupies the freeze SRAM until its verdict two peer round trips later; batches of up to 8{,}192 elements stay resident, and larger ones (e.g., the 65{,}536-element batches of \cref{fig:checkperf}) spill to sealed pages. Batching amortizes metadata and network latency but raises staging memory and first-result latency, and a batch contains only independent openings: the compiler keeps a checkpoint before every input-dependent nonlinear output and every final release, since our proofs do not justify blind delayed checking.

% ======================================================================
\subsection{Command Interface and Host Integration}\label{sec:arch-iface}

\begin{table}[t]
\centering
\caption{Commands of the protected module $T_b$. Every command is a canonical frame bound to session, epoch, role and gate; the ledger state reached on success is given in parentheses. No command authenticates a host-supplied value.}
\label{tab:commands}
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\linewidth}{l >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X}
\hline
\textbf{Command} & \textbf{Required check} & \textbf{Allowed result} \\
\hline
\cmd{OPEN_SESSION}  & Authenticated identities, role, fresh epoch, manifest $\mu$ & Session capability \\
\cmd{RESERVE_PREP}  & Approved gate, unused randomness identifiers & Party-local authorized preprocessing, issued once (\lstate{PREPARED}) \\
\cmd{FREEZE_BATCH}  & Exact canonical bytes, dimensions, expected wire list & Frozen root $h_b$ and handle (\lstate{FROZEN}) \\
\cmd{CHECK_OPEN}    & Both frozen roots, independent challenge lanes, peer residuals & Verified prescribed opening or abort (\lstate{VERIFIED}) \\
\cmd{EVAL_FSS}      & Bound table or function, consumed input opening, fixed role & Freshly reshared authenticated local output (\lstate{CONSUMED}) \\
\cmd{VERIFY_MATRIX} & Anchored operands, frozen candidate & Verified immutable result handle (\lstate{VERIFIED}) \\
\cmd{FINAL_OUTPUT}  & Authorized recipient, output mask, accepted check & Bound output frame and certificate (\lstate{RELEASED}) \\
\cmd{ABORT}         & Any integrity or lifecycle violation & Epoch invalidation, no candidate values (\lstate{ABORTED}) \\
\hline
\end{tabularx}
\end{table}

\textbf{Host responsibilities.}
Host $b$ schedules the public circuit, stores only party-local authenticated arrays (value and each MAC lane as separate coalesced arrays, serialized canonically only at the protected interface), runs the exact field kernels of \cref{sec:arch-field} and sends share batches to $T_b$. Its scheduling may be adversarial, so the ledger, not the host, decides whether operation, identity, shape and order are admissible, and a reused buffer always carries a fresh transaction identifier.

\textbf{Commands and frames.}
\Cref{tab:commands} lists the eight commands with the ledger state each reaches (\cref{fig:ledger}). There is deliberately no command that accepts a host value and returns its tags: \cmd{EVAL_FSS} authenticates only results the module computed itself, which closes the forgery-oracle path of scenario~S2 (\cref{fig:scenarios}). A frame carries version, session identifier, epoch, role, opcode, gate identifier, ordered input and output identifiers, field identifier, tag count, dimensions, payload length, sequence number and payload, all length-prefixed with explicit endianness; frames between modules or from a client bind the header as AEAD associated data. The parser copies each frame into protected memory before checking it and rejects truncation, trailing bytes, duplicate identifiers, malformed dimensions, noncanonical field elements (values of at least $p$ are rejected, never reduced) and unexpected opcodes.

\textbf{Data races and aborts.}
Verification and consumption use the same immutable bytes that the parser authenticated; completion of a DMA transfer implies neither authenticity nor immutability. Our proofs assume ordered freeze and check decisions, so independent gate batches may overlap, but a dependent nonlinear gate never consumes an unchecked masked opening. An epoch abort atomically gates all outstanding output responses and prevents new challenges; \cref{tab:attacks} maps each injected fault to the block that stops it.

% ======================================================================
\subsection{Exact Field Arithmetic on the GPU}\label{sec:arch-field}

GPU kernels must compute the finite circuit that the proofs reason about, so floating-point shortcuts are excluded. An authenticated GEMM is four independent products of the same shape, one per lane, plus the public product $DE$ shared by all lanes (\cref{fig:arith}); \cref{lst:mersenne} gives the scalar multiplication at the core of every kernel.

\begin{figure}[t]
\centering
\scriptsize
\begin{tabular}{|l|}
\hline
\begin{minipage}{0.95\linewidth}
\vspace{2pt}
\begin{verbatim}
constexpr uint64_t P = (1ULL << 61) - 1;  // 2^61 - 1
// canonical a, b < P; returns canonical a*b mod P
__device__ uint64_t mul61(uint64_t a, uint64_t b) {
  uint64_t lo = a * b;              // low 64 bits
  uint64_t hi = __umul64hi(a, b);   // high bits, < 2^58
  uint64_t x  = (lo & P) + ((lo >> 61) | (hi << 3));
  x = (x & P) + (x >> 61);          // x <= 2^61
  return x >= P ? x - P : x;
}
\end{verbatim}
\vspace{-4pt}
\end{minipage}\\
\hline
\end{tabular}
\caption{Exact Mersenne-61 multiplication used by the GPU field kernels (CUDA). The first fold uses $2^{61}\equiv 1 \pmod p$; the second fold and the conditional subtraction return the canonical representative. No floating-point or Tensor-Core operation is involved.}
\label{lst:mersenne}
\end{figure}

\textbf{Correctness.}
For canonical $a,b<p=2^{61}-1$ the product is below $2^{122}$, so $\mathtt{hi}<2^{58}$ and $\mathtt{hi}\ll 3$ fits in 61 bits. Writing $ab=2^{64}\,\mathtt{hi}+\mathtt{lo}$ and using $2^{61}\equiv 1\pmod p$ gives $ab\equiv(\mathtt{lo}\bmod 2^{61})+\lfloor\mathtt{lo}/2^{61}\rfloor+2^{3}\,\mathtt{hi}\pmod p$. The last two terms occupy disjoint bit ranges (bits 0 to 2 and 3 to 60), so the bitwise OR equals their sum and the folded value is below $2^{62}$. The second fold yields at most $2^{61}=p+1$, and the conditional subtraction returns the canonical representative. The CPU reference checked this formula against arbitrary-precision arithmetic in 20{,}004 cases, including boundaries. A CUDA micro-test comparing 65{,}536 products with a host 128-bit reference is written but not yet compiled or run, so no GPU conformance is claimed.

\textbf{Accumulation and numeric contract.}
A two-word 128-bit accumulator absorbs at most 64 unreduced products below $2^{122}$, so kernels fold at least once per 64-element slice of the inner dimension; random shares lie close to $p$ even for small plaintexts, so plaintext bounds never justify longer accumulation. The manifest $\mu$ fixes the scale $2^f$, signed encoding, toward-zero truncation (\cref{alg:trunc}), saturation, approximation coefficients and output decoding. For example, a dot product of length at most 4096 with operand magnitudes at most $2^{20}$ stays below $2^{52}$ before bias, which leaves room below $p/2$ only if bias and further accumulation are bounded too; the bound is recomputed per layer. FP16, BF16 and TF32 Tensor Cores never serve as exact field operations without a proven limb construction, and the exact finite circuit and a floating-point accuracy model remain separate references. Our model charges an exact Mersenne GEMM \est{1.25$\times$} the time of a wraparound 64-bit GEMM per lane (\cref{app:model}).

% ======================================================================
\subsection{Deployment Targets}\label{sec:arch-deploy}

An on-die module cannot be added to a commercial A100, so we define three distinct experiments and never merge their timings into a purported all-measured result. \emph{(i) A100 software} runs the exact kernels, authenticated GEMM and host runtime on a real A100 with an emulated module (completion gate~G2, pending). \emph{(ii) A ZCU102 prototype} (\texttt{xczu9eg-ffvb1156-2-e}~\cite{amd2023zcu102}) implements the datapath of \cref{fig:hw} at reduced scale (\est{4} DPF units, \est{16} AES engines, \est{32} FUA lanes at \est{250~MHz}, \cref{tab:fpga}) to validate streaming, freezing and release ordering; one board with an emulated peer shows functionality, not two independent trust boundaries, and an ARM process on it is not isolated from a malicious board administrator. \emph{(iii) The on-die projection} models integration next to the L2 slices with Accel-Sim~\cite{khairy2020accel} and synthesis, as in DFA; our headline numbers refer to it and currently come from the analytical model of \cref{app:model}. For an external module, GPUDirect RDMA requires platform and driver support and ordinarily a common upstream PCIe root complex~\cite{nvidia2024gpudirect}, so staged transfer through host memory remains the baseline and IOMMU protection is never disabled for a better benchmark. In every target, freeze-before-challenge refers to immutable authenticated bytes, never to a GPU buffer that can change concurrently.

% ======================================================================
\subsection{Design-Space Comparison}\label{sec:arch-dse}

\textbf{Design-space Comparison.}
We compare the L2-adjacent organization of \sys with alternative homes for authentication, verification and randomness generation.

\textit{External protected module over PCIe.}
A discrete FPGA or security card~\cite{xu2025co} keeps the boundary off the GPU die but limits the module interface to $B/32$ elements per second: \est{50~M} elements/s for the \est{1.6~GB/s} ZCU102 transport, \est{0.78~G} for \est{25~GB/s} of effective PCIe Gen4 bandwidth, and \est{9.1~G} for the 290~GB/s on-die path of DFA~\cite{dfa2026trusted}. Since authenticated GEMM dominates, BERT-Base LAN latency rises only from \est{3.83~s} to \est{3.87~s} over PCIe, and to \est{4.59~s} with the ZCU102 link and its \est{32} FUA lanes at \est{250~MHz} (\cref{tab:ablation}); the option suits prototyping but adds a second device per party and a device round trip per checked batch.

\textit{Verification on the GPU SMs.}
In \ProfT the SMs belong to the malicious host: a corrupt checking kernel could see the challenges before choosing its errors, or simply report acceptance. Trusting the SMs requires a GPU-wide TEE~\cite{volos2018graviton,jang2019heterogeneous,dhanuskodi2023confidential} whose boundary covers SMs, caches, memory controllers and the driver interface, the large boundary that DFA and \sys avoid. The GPU therefore computes only products that the module verifies afterwards (\CheckOpen{} or the Freivalds check of \cref{sec:proto-freivalds}).

\textit{Tag DPF trees instead of the epilogue.}
One extra DPF tree per MAC lane (payload $\Delta_j\beta$) multiplies the PRG work of every gate by $1+t=4$: at $n=61$ the engine delivers \est{26.7}~M instead of \est{106}~M gates/s (\cref{fig:dpfthr}), and BERT-Base LAN latency and energy rise from \est{3.83~s} and \est{73.7~J} to \est{4.12~s} and \est{80.4~J}. The epilogue achieves the same with three multiplications and four pads (\cref{thm:epilogue}).

\textit{Software-only malicious backend.}
SPDZ-family preprocessing~\cite{keller2016mascot,keller2018overdrive,cramer2018spdz2k,keller2020mpspdz} needs inter-party communication that grows with the number of authenticated triples, and a dealer-based actively secure FSS pipeline in the style of Shark~\cite{gupta2025shark} ships an estimated \est{37.6~GB} per BERT-Base query (\cref{tab:e2e}); both re-create the offline traffic that trusted DFA removed. Such a backend is right when the hardware itself is distrusted (\ProfU, \cref{sec:threat-profileu}); under \ProfT it pays for a trust assumption that the module already provides.

\textit{Dedicated check engines and per-slice checking.}
Checking needs only \est{3~ms} of module time per BERT-Base query against \est{131~ms} of protected FSS work, so dedicated AES engines for challenges and sealing would idle almost always; time-sharing adds none. DPF units stay distributed because DFA showed that a single attachment point would cap DPF output at about 62\% of the 290~GB/s delivered bandwidth~\cite{dfa2026trusted}. Checks, by contrast, are batched, cost at most 3.5 AES blocks (1.5 for challenges, 2 for sealing) and six field multiplications per element, and depend on the ledger, freeze SRAM and peer channel, which must be single points of authority; centralizing them in the VIGOR core avoids replicating $\Delta_{b,j}$ and ledger state across 16 slices and keeps one authoritative root per batch.

Overall, an external module is bounded by its host link, SM-based checking enlarges the boundary beyond \ProfT, tag trees multiply DPF work, a software-only backend reintroduces preprocessing traffic, and replicated check hardware adds area without removing a bottleneck.


==> qa/draft1/sections/07_security.tex <==
% =====================================================================
% Section VII: Security Analysis
% File owner: sections/07_security.tex
% Labels defined here: sec:security, sec:sec-assump, sec:sec-main,
%   sec:sec-lemmas, sec:sec-scenarios, sec:sec-concrete, sec:sec-boundary,
%   thm:main, thm:dpf-correct, thm:gac, thm:dcf, thm:epilogue,
%   lem:hidden-key, thm:mac-sound, thm:arith, thm:bitdec, thm:cmp-trunc,
%   thm:lut, thm:interval, lem:bijection, lem:noninv, thm:freivalds,
%   thm:pir, tab:obligations
% =====================================================================
\section{Security Analysis}
\label{sec:security}

We now state what \sys guarantees against a malicious host and GPU, in the explicit-simulator style of secure computation with abort~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}. The protocol is compared with the ideal functionalities $\FC$ and $\FPIR$ of \cref{fig:func} under \cref{def:security}, and everything the adversary may learn is listed in the leakage $\Leak$ of \cref{def:leakage}. Each link of the integrity chain, \emph{authorized input $\rightarrow$ correlated preprocessing $\rightarrow$ correct local evaluation $\rightarrow$ authenticated arithmetic $\rightarrow$ consistent opening $\rightarrow$ authorized output release}, is discharged by a named statement: input extraction (\cref{thm:arith}); in-module preprocessing and joint sampling (\cref{lem:bijection,lem:noninv}); exact DPF, DCF and gate correctness (\cref{thm:dpf-correct,thm:gac,thm:dcf,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval}); the epilogue and the arithmetic identities (\cref{thm:epilogue,thm:arith}); MAC-check soundness (\cref{lem:hidden-key,thm:mac-sound}); and gated release (\cref{thm:arith,thm:pir}). Full proofs are in \cref{app:proof-dpf,app:proof-auth,app:proof-gates,app:proof-pir,app:proof-main}.

% =====================================================================
\subsection{Assumptions and Error Terms}
\label{sec:sec-assump}

The theorem is proved in \ProfT (\cref{sec:threat-model}): parties $P_0,P_1$, each an untrusted host with a protected module $T_b$, and a PPT adversary that statically corrupts at most one host (OS, driver, runtime, GPU kernels and results, local memory, outgoing traffic) and may deviate arbitrarily, abort, delay and replay. We state the trust in the modules as an explicit ideal resource, in the spirit of tamper-proof hardware models~\cite{katz2007universally}, instead of leaving it implicit in the phrase ``trusted hardware''.

\begin{assumption}[Ideal protected module]
Corrupting host $b$ does not corrupt $T_b$. The code, keys, parser, field arithmetic, ledger transitions, local memory, protected peer channel and approved I/O paths of each module are correct and confidential. Its externally observable behavior (lengths, timing, host-visible memory and DMA activity) is simulatable from its prescribed local view and public metadata by a stipulated trace simulator. Module state is fresh: a trusted monotonic service preserves freshness across reboots~\cite{parno2011memoir,matetic2017rote}, or the module irrecoverably erases its master key and requires a freshly attested session. Availability is not assumed.
\end{assumption}

\begin{assumption}[Setup, randomness, channels and bindings]
The following terms bound the advantage of each idealization over the \emph{entire} admitted execution, not a single primitive call:
$\eps{setup}$, simulation of the authenticated setup of \cref{sec:proto-setup} (binding ordered identities, roles, fresh session identifier, epoch, manifest hash, field and tag parameters and protocol version) by an ideal role-bound interface;
$\eps{prf}$, replacement of PRF/KDF outputs (AES-128, HKDF~\cite{krawczyk2010hkdf}) under distinct length-prefixed labels (session, epoch, gate, purpose, logical draw, block) by independent coins, identical for the same joint label;
$\eps{channel}$, confidentiality and integrity of the AEAD channels~\cite{dworkin2007gcm,mcgrew2004gcm} with directional keys and nonrepeating nonces;
$\eps{bind}$, collisions or forgeries in manifests, snapshot commitments, frozen-page roots, certificates and session freshness~\cite{fips202,merkle1987digital};
$\eps{trace}$, the stipulated trace simulator.
\end{assumption}

Correctness of protected code, state and arithmetic is thus a \emph{premise}, not an estimated probability. Outside the theorem are physical attacks (probing, fault injection, power or electromagnetic analysis~\cite{kocher1999differential,murdock2020plundervolt,skorobogatov2017microprobing}), leakage beyond the trace model, adaptive corruption, speculative-execution flaws inside the boundary and faulty trusted arithmetic. The inference client is honest, uses authenticated confidential channels to the modules and does not collude with a server; a corrupt server may choose its own inputs. PIR also considers a separate regime in which the client alone is malicious. The protocol contributes one statistical term, determined by the field $\Fp$ with $p=2^{61}-1$, the number $t$ of independent global keys $\Delta_j=\Delta_{0,j}+\Delta_{1,j}$ (host $b$ knows at most $\Delta_{b,j}$), and the number $Q$ of \CheckOpen{} batches. Finally, the modules may see inputs: after a verified masked opening a module knows the value and its mask, and the committed-input loader and the direct protected gate (\cref{sec:proto-direct}) handle plaintext inside the boundary. \sys claims confidentiality against hosts, GPUs, the network and the other party, not against its own trusted modules.

% =====================================================================
\subsection{Main Theorem}
\label{sec:sec-main}

\begin{theorem}[Static malicious security with abort]
\label{thm:main}
Under the assumptions of \cref{sec:sec-assump}, the protocols of \cref{sec:analysis-dpf,sec:protocol} (setup, ledger, exact DPF, generate-and-consume with the fresh authentication epilogue, conservative DCF, \AuthShare, \CheckOpen, input, linear, multiplication and output protocols, bit decomposition, comparison, truncation, LUT and interval gates) realize $\FC$, and \cref{alg:pir} realizes $\FPIR$, with abort and leakage $\Leak$ (\cref{def:security,def:leakage}), against a PPT adversary statically corrupting at most one host (for $\FPIR$, in either regime of \cref{fig:func}). With at most $Q$ \CheckOpen{} batches, the distinguishing advantage of any environment is at most
\begin{align*}
\eps{VIGOR}\le{}&\eps{setup}+\eps{prf}+\eps{channel}\\
&+\eps{bind}+\eps{trace}+Q\,(2/p)^{t}.
\end{align*}
If the Freivalds check (\cref{alg:freivalds}) is enabled for at most $Q_F$ calls with $s$ repetitions, the bound gains $Q_F/p^{s}$, and the binding obligations of \cref{thm:freivalds} apply.
\end{theorem}

\textbf{What the bound omits.}
There is no DPF one-key-privacy term: keys never leave the modules, \cref{thm:dpf-correct} gives raw correctness and \cref{thm:epilogue} makes every exported tuple uniform. A profile that exports keys, to an external malicious backend under \ProfU (\cref{sec:threat-profileu}) or to a verifiable-FSS evaluator~\cite{decastro2022vfss}, must add its actual DPF or backend privacy assumption. There is no term for faulty trusted arithmetic, which is a premise. The theorem concerns the abstract protocol and does not prove that a concrete chip implements the ideal module (\cref{sec:sec-boundary}).

\textbf{Proof overview.}
The simulator $\Sim$ plays the ideal module interface, samples all MAC key shares, keeps the global keys internally and maintains for every wire the exact tuple the corrupt party would hold in a faithful execution, plus the manifest and ledger state. Honest global values are never needed: honest shares are defined symbolically by the wire semantics and the corrupt share. Five hybrids connect the real and ideal executions (\cref{app:proof-main}); $\Hyb{0}$ is the real execution.
\begin{itemize}[leftmargin=*]
\item \textbf{$\Hyb{1}$ (setup and channels).} Setup becomes the ideal role-bound interface, and protected-channel contents become ideal deliveries of the permitted lengths and schedules. Cost: $\eps{setup}+\eps{channel}$.
\item \textbf{$\Hyb{2}$ (randomness and bindings).} PRF/KDF outputs become ideal coins ($\eps{prf}$), and any binding failure aborts ($\eps{bind}$). The ledger (\cref{fig:ledger}) then excludes label reuse, role swapping and post-challenge byte replacement; streaming generate-and-consume and refactored samplers are replaced by their reference forms at no cost (\cref{thm:gac,lem:bijection,lem:noninv}).
\item \textbf{$\Hyb{3}$ (simulated transcript).} The corrupt view is generated without honest inputs: preprocessing shares follow the uniform party-local laws of \AuthShare, epilogue outputs are fresh uniform tuples (\cref{thm:epilogue}), and every masked opening (an honest owner's $\epsilon=x-r$, Beaver differences, gate openings $x+r$ and $x\oplus r$) is sampled uniformly, with the consistent hidden preprocessing defined afterwards. At each \CheckOpen{} the simulator compares the submitted bytes with the maintained tuple, obtains the error vectors $(e,d_1,\dots,d_t)$ and decides the outcome from $\inner{\rho_j}{d_j-\Delta_j e}$ with its own keys and fresh challenges. $\Hyb{3}$ and $\Hyb{2}$ are identical.
\item \textbf{$\Hyb{4}$ (ideal outputs and traces).} Corrupt inputs are extracted ($x^*=r+\epsilon$, or the committed value of the protected loader), outputs are delivered through $\FC$ (the output mask of a corrupt recipient is programmed after its ideal output is known), and traces come from the trace simulator. Unless some check accepts a nonzero value error, \cref{thm:arith,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval} identify every real wire with $C$ on the extracted inputs, so the cost is $Q(2/p)^t+\eps{trace}$ (\cref{lem:hidden-key,thm:mac-sound}). PIR uses the simulator of \cref{thm:pir}.
\end{itemize}
$\Hyb{4}$ is the ideal execution, and the triangle inequality gives the bound. The adversary may still suppress delivery to honest parties: no fairness is added.

% =====================================================================
\subsection{Building Blocks}
\label{sec:sec-lemmas}

The statements refer to the exact algorithms of \cref{sec:analysis-dpf,sec:protocol}, which, unlike the simplified semi-honest ones (\cref{sec:bg-dfa}), make root control bits, payload and role inputs, and separate generator and evaluator states explicit. Each is followed by its proof idea.

\begin{theorem}[DPF correctness]
\label{thm:dpf-correct}
For all root seeds $s_0,s_1\in\bits{128}$ with root control bits $t_0=0$, $t_1=1$, every $n$, $\alpha,x\in\bits{n}$ and $\beta\in\Fp$, the keys of \cref{alg:gen} and the outputs $y_b$ of \cref{alg:eval} satisfy $y_0+y_1=\beta\cdot\one[x=\alpha]$. No uniform target and no hardness assumption is needed.
\end{theorem}

\noindent\textit{Proof idea.}
On the target prefix the control bits stay opposite; on a losing child $(s_0^{\lose}\oplus s_1^{\lose})\oplus((t_0\oplus t_1)\sCW)=0$ and the control bits cancel, so the states coincide and their signed outputs cancel. At the leaf $t_0-t_1=(-1)^{t_1}$, so $y_0+y_1=u_0-u_1+(-1)^{t_1}\CWout=\beta$ (\cref{app:proof-dpf}).

\begin{theorem}[Generate-and-consume equivalence]
\label{thm:gac}
For fixed roots, $\alpha$, $\beta$, role $b$ and query $x$, the raw share $\tilde{y}_b$ of \cref{alg:gac} equals the output of \cref{alg:eval} on the key $k_b$ that \cref{alg:gen} produces from the same inputs, node by node for every dependency-respecting depth-first order of $\EvalAll$.
\end{theorem}

\noindent\textit{Proof idea.}
Couple both executions: equal states before level $i$ give the same correction word, generator state and evaluator state after it. The theorem justifies scheduling only, not changes to expansion or correction (\cref{app:proof-dpf}).

\begin{theorem}[Conservative DCF]
\label{thm:dcf}
If \cref{alg:dcf} creates, for each $i=1,\dots,n$ (zero payloads included), an independent DPF with target $\alpha_1\cdots\alpha_{i-1}0$ and payload $\beta\alpha_i$, evaluated at $x_1\cdots x_i$, the shares sum to $\beta\cdot\one[x<\alpha]$, at a cost of $n(n+1)/2$ path levels.
\end{theorem}

\noindent\textit{Proof idea.}
If $x<\alpha$, exactly the prefix ending at their first differing bit ($x_i=0$, $\alpha_i=1$) contributes $\beta$; otherwise none does. \Cref{thm:dpf-correct} and linearity conclude. A faster DCF~\cite{storrier2023grotto} may replace it only after its own obligations are met (\cref{app:proof-dpf}).

\begin{theorem}[Epilogue correctness and local hiding]
\label{thm:epilogue}
For raw shares $\tilde{y}_0,\tilde{y}_1$ and fresh uniform pads $\zeta,\kappa_1,\dots,\kappa_t\in\Fp$, the outputs $y_b=\tilde{y}_b+(-1)^b\zeta$, $\gamma_{b,j}=\Delta_j y_b+(-1)^b\kappa_j$ form an authenticated sharing of $\tilde{y}_0+\tilde{y}_1$. For either fixed $b$, $(y_b,\gamma_{b,1},\dots,\gamma_{b,t})$ is uniform on $\Fp^{t+1}$ given the raw outputs and the keys, before conditioning on later prescribed openings, jointly across fresh outputs.
\end{theorem}

\noindent\textit{Proof idea.}
The pads cancel in the sums. For fixed $b$, $\zeta\mapsto y_b$ and each $\kappa_j\mapsto\gamma_{b,j}$ are bijections, so every tuple has probability $p^{-(t+1)}$. The cost is three multiplications and four pads per party and output for $t=3$, with no tag DPF tree (\cref{app:proof-dpf}).

\begin{lemma}[Hidden-key invariant]
\label{lem:hidden-key}
In $\Hyb{2}$ with host $b$ corrupted, conditioned on its view and its shares $\Delta_{b,j}$, the honest shares $\Delta_{1-b,1},\dots,\Delta_{1-b,t}$ remain independent and uniform until the first accepted opening with a nonzero value error.
\end{lemma}

\noindent\textit{Proof idea.}
Fresh tags are padded (\AuthShare, \cref{thm:epilogue}); linear updates are deterministic in the view; correct openings have zero residual; a tag-only error yields an outcome independent of $\Delta_j$; the first check with a value error ends the epoch if it fails; residuals and challenges stay inside the modules (\cref{app:proof-auth}).

\begin{theorem}[Wrong-value acceptance]
\label{thm:mac-sound}
Let a batch of $m$ positions submitted to \CheckOpen{} (\cref{alg:checkopen}) differ from the prescribed tuples by a value error $e\in\Fp^m$ and tag errors $d_1,\dots,d_t\in\Fp^m$, fixed by the freeze. If $e\ne 0$ and the lanes use independent uniform challenges $\rho_j\in\Fp^m$ drawn after the freeze, \CheckOpen{} accepts with probability at most $(2/p)^t$ in $\Hyb{2}$. Over $Q$ batches, an incorrect value is released with probability at most $Q(2/p)^t$.
\end{theorem}

\noindent\textit{Proof idea.}
Lane $j$ accepts iff $\inner{\rho_j}{d_j-\Delta_j e}=0$. For $e_i\ne 0$ the vector vanishes only if $\Delta_j=d_{j,i}/e_i$ (probability $\le 1/p$ by \cref{lem:hidden-key}); otherwise the nonzero linear form vanishes with probability $1/p$~\cite{schwartz1980fast}. Each lane gives $1/p+(1-1/p)/p<2/p$; lanes are independent; a union bound over batches gives $Q(2/p)^t$, following the SPDZ MAC check~\cite{damgard2012spdz,damgard2013practical} (\cref{app:proof-auth}).

\begin{theorem}[Authenticated arithmetic]
\label{thm:arith}
With correct modules and prescribed messages, the protocols of \cref{fig:arith} are exact: input yields $\auth{x}$ with $x=r+\epsilon$, linear operations preserve $\gamma_{0,j}+\gamma_{1,j}=\Delta_j x$, multiplication with a correct fresh triple yields $\auth{xy}$ (and $\auth{XY}$ with the factor order preserved), and output gives $y=w-o$ to its authorized recipient. Unless a nonzero value error is accepted or a binding fails, every deviation of a corrupt host selects a permitted input, leaves the computation unchanged, or causes abort.
\end{theorem}

\noindent\textit{Proof idea.}
With $d=x-a$, $e=y-b$ and $c=ab$: $c+db+ea+de=xy$~\cite{beaver1991efficient}, the tags follow scaled by $\Delta_j$, $Z=C+DB+AE+DE$ for matrices, and $(y+o)-o=y$ with $o$ uniform. \CheckOpen{} and the ledger block changed or reused material; induct over gates (\cref{app:proof-auth}).

\begin{theorem}[Canonical bit decomposition]
\label{thm:bitdec}
For $p=2^n-1$ ($n=61$), \cref{alg:bitdec} returns authenticated bits (least significant first) of the canonical representative of $x$, using one masked opening $c=x+r\bmod p$ and $2n$ authenticated multiplications.
\end{theorem}

\noindent\textit{Proof idea.}
The first loop is a full subtractor giving $d=(c-r)\bmod 2^n$ and borrow $\one[c<r]$; with a borrow $x=c-r+p=d-1$ since $p=2^n-1$, which the second loop subtracts~\cite{damgard2006unconditionally} (\cref{app:proof-gates}).

\begin{theorem}[Exact comparison and signed truncation]
\label{thm:cmp-trunc}
From authenticated canonical bits of $x$ and a public $\theta\in[0,2^n)$, \cref{alg:trunc} returns authenticated $\one[x<\theta]$ and $\one[x=\theta]$; for centered $z\in[-(p-1)/2,(p-1)/2]$ it returns $\mathrm{sgn}(z)\lfloor|z|/2^f\rfloor$, i.e., truncation toward zero.
\end{theorem}

\noindent\textit{Proof idea.}
The equality flag tracks the processed prefix, and $\mathit{lt}$ gains a term exactly at the first position with secret bit $0$ and threshold bit $1$. Negative values occupy the canonical upper half; $(1-2s)z$ is the magnitude without wrap, and shifting its bits floors~\cite{catrina2010improved}. Fixed-point products must stay below $p/2$ before truncation (\cref{app:proof-gates}).

\begin{theorem}[Authenticated LUT]
\label{thm:lut}
For an approved table $T$ of $2^w$ entries and certified authenticated bits of $x\in\bits{w}$, if the mask bits and the DPF target of the keys for $(r,1)$ come from the same fresh uniform $r$, \cref{alg:lut} outputs $\auth{T[x]}$ and the opened $u=x\oplus r$ is uniform given $x$.
\end{theorem}

\noindent\textit{Proof idea.}
By \cref{thm:dpf-correct}, $\tilde{y}_0+\tilde{y}_1=\sum_a T[a\oplus u]\one[a=r]=T[x]$, and XOR by fixed $x$ is a bijection; independent resampling of the target would break the identity (\cref{app:proof-gates}).

\begin{theorem}[Intervals and piecewise polynomials]
\label{thm:interval}
For a proper nonempty public $[a,b)\subset[0,p)$, \cref{alg:interval} outputs $\auth{\one[a\le x<b]}$; for a disjoint exhaustive partition, Horner evaluation of the selected coefficients outputs $P_{i^\star}(x)$ for the interval containing $x$, in the declared finite arithmetic.
\end{theorem}

\noindent\textit{Proof idea.}
Adding $r$ maps $[a,b)$ to the circular interval from $L$ to $H$; the indicator is $\one[c<H]-\one[c<L]$ if $L<H$ and $1+\one[c<H]-\one[c<L]$ if $L>H$, which is the raw share by \cref{thm:dcf}. Exactly one indicator is one, and Horner with \cref{thm:arith} gives the polynomial; no equality to an unapproximated real function is claimed (\cref{app:proof-gates}).

The semi-honest decoupling sampled DPF targets directly~\cite{dfa2026trusted}. The next two lemmas state when this is valid: joint distributions with all auxiliary material must match, not only marginals (\cref{sec:proto-refactor}).

\begin{lemma}[Bijection with correlated auxiliary material]
\label{lem:bijection}
Fix $Z=z$, $R$ uniform on a finite $\mathcal{R}$, a bijection $g_z:\mathcal{R}\to\mathcal{A}$, independent coins $W$ and an auxiliary sampler $J$. Then $(R,g_z(R),J(z,R,W))$ and $(g_z^{-1}(A),A,J(z,g_z^{-1}(A),W))$ with $A$ uniform on $\mathcal{A}$ are identically distributed.
\end{lemma}

\noindent\textit{Proof idea.}
Each pair $(r,a)$ has probability $1/|\mathcal{R}|$ in both experiments if $a=g_z(r)$ and zero otherwise; the same $J$ preserves equality. Independently resampling correlated targets such as $(r,r+1)$ breaks it (\cref{app:proof-gates}).

\begin{lemma}[Noninvertible transformations]
\label{lem:noninv}
For any $g$, sampling $A$ from the law of $g(R)$ and $R'$ from $R\mid g(R)=A$ reproduces $(R,g(R))$ and everything derived from $R'$. For unsigned truncation of a uniform $\ell$-bit mask by $h$ bits, $R'=2^hA+U$ with $A$, $U$ uniform on $\ell-h$ and $h$ bits.
\end{lemma}

\noindent\textit{Proof idea.}
$\Pr[A=a]\Pr[R=r\mid g(R)=a]=\Pr[R=r,g(R)=a]$; each truncated mask has probability $2^{-\ell}$. Signed shifts and other moduli need their own samplers (\cref{app:proof-gates}).

\begin{theorem}[Frozen-operand matrix check]
\label{thm:freivalds}
Let the module bind $A\in\Fp^{m\times k}$, $B\in\Fp^{k\times n}$, whose exposure to the GPU is already permitted, and freeze a claimed $C$. If $C\ne AB$, \cref{alg:freivalds} with $s$ secret uniform $v\in\Fp^n$ drawn after the freeze accepts with probability at most $p^{-s}$, and over $Q_F$ calls an incorrect product is consumed with probability at most $Q_F/p^s$.
\end{theorem}

\noindent\textit{Proof idea.}
A nonzero row $e$ of $C-AB$ gives $\inner{e}{v}=0$ for a $1/p$ fraction of $v$~\cite{freivalds1977probabilistic,tramer2018slalom}; repetitions multiply; freezing fixes $C$ before $v$, and binding ties the verified bytes to the consumed ones (\cref{app:proof-gates}).

\begin{theorem}[Versioned-snapshot PIR]
\label{thm:pir}
With correct modules and binding snapshot and query interfaces: (i) with an honest client and at most one malicious server host, \cref{alg:pir} gives the client the record $D[\alpha]$ of the authorized committed snapshot or abort, and the corrupt host's view is simulatable without $\alpha$; (ii) with a malicious client alone, accepted requests reveal nothing about the database beyond the requested records and the public descriptor.
\end{theorem}

\noindent\textit{Proof idea.}
\Cref{thm:dpf-correct} gives $y_0+y_1=\sum_i(\DPF_0(i)+\DPF_1(i))D[i]=D[\alpha]$; hashing the consumed bytes, comparing queries and role-bound certificates prevent substitution ($\eps{bind}$); results are freshly reshared (\cref{thm:epilogue}). For a malicious client the simulator extracts the index and reshares the ideal record. This does not make untrusted DPF-PIR symmetric; authenticated PIR~\cite{colombo2023apir} or external-key vFSS needs its own proof (\cref{app:proof-pir}).

% =====================================================================
\subsection{Scenario-by-Scenario Analysis}
\label{sec:sec-scenarios}

We revisit the scenarios of \cref{fig:scenarios,tab:scenarios}; \cref{tab:attacks} lists the corresponding injections.

\begin{itemize}[leftmargin=*]
\item \textbf{S1: Share and tag tampering.} A GPU error reaches a protected gate or a release only through \CheckOpen, where the freeze fixes it and \cref{thm:mac-sound} bounds acceptance by $(2/p)^t$; rejection poisons the epoch. The outcome depends only on $(e,d_j)$, keys and challenges, so $\Sim$ reproduces it without honest inputs and selective failure leaks nothing beyond the abort bit (\cref{lem:hidden-key}).
\item \textbf{S2: Forgery oracle.} The command interface (\cref{tab:commands}) has no entry point that tags a host-supplied value, such as \cmd{authenticate(host_value)}: the epilogue tags only raw shares computed in the module or by a verified backend. Chosen values obtain tags only via the input interface, which $\FC$ permits and $\Sim$ extracts. Clients never receive complete tag pairs, which would expose $\Delta_j$ through $\Delta_j y$ for a known $y\neq 0$.
\item \textbf{S3: TOCTOU buffer swap.} Challenges are derived only after both modules freeze the exact bytes and agree on both roots, and consumption rereads only authenticated frozen pages (\cref{fig:checkopen}); a later DMA rewrite is ignored and a tampered spill page aborts ($\eps{bind}$). This realizes the premise of \cref{thm:mac-sound} that errors precede challenges.
\item \textbf{S4: Replay and rollback.} Labels bind session, epoch, gate, purpose, draw and block; the ledger consumes each resource once and never recycles aborted reservations. A replayed message, mask or counter fails its binding or hits a consumed entry. Module reset with old keys is excluded by the freshness clause, which a host-controlled counter file cannot provide.
\item \textbf{S5: Role and gate confusion.} Role-bound session keys, joint labels without the local role (with distinct root-0 and root-1 draws) and ledger descriptors (operation, wires, type, table hash, dimensions) turn cross-role or cross-gate routing into a descriptor mismatch and abort.
\item \textbf{S6: Premature release.} The release guard opens only for entries in state \lstate{VERIFIED}, certificates bind session, epoch, gate, recipients and output hash, and an epoch abort atomically gates all pending responses. Private outputs are opened as $w=y+o$, uniform to every host (\cref{thm:arith}).
\item \textbf{S7: Malformed preprocessing.} Triples ($c=ab$ computed inside the module) and DPF keys are generated in the boundary; a valid MAC on a wrong triple does not make it correct, so the proof never uses the MAC check to certify preprocessing. Imported material needs its own correctness proof, GPU products need \cref{thm:freivalds}, and correlated material is sampled jointly (\cref{lem:bijection,lem:noninv}).
\item \textbf{S8: Snapshot substitution.} The module hashes the bytes it consumes and quarantines results until the hash matches the versioned commitment, so a swapped record or stale version aborts (\cref{thm:pir}).
\item \textbf{S9, S10: Input choice and abort.} A corrupt party choosing its own inputs is permitted and extracted; model provenance requires the committed loader. Denial of service is not prevented (no fairness or availability), but aborts occur at public boundaries and are simulatable, and input-dependent validity outcomes are part of $\Leak$.
\end{itemize}

% =====================================================================
\subsection{Concrete Security}
\label{sec:sec-concrete}

Since $2/p\approx 2^{-60}$ for $p=2^{61}-1$, we have $\log_2 Q(2/p)^t\approx\log_2 Q-60t$. For a budget of $Q\le 2^{32}$ checked batches:
\begin{center}
\footnotesize
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{c c c c}
\hline
$t$ & $(2/p)^t$ per batch & $Q(2/p)^t$ & BERT-Base LAN (s)\\
\hline
1 & $\approx 2^{-60}$ & $\approx 2^{-28}$ & \est{2.53}\\
2 & $\approx 2^{-120}$ & $\approx 2^{-88}$ & \est{3.18}\\
3 & $\approx 2^{-180}$ & $\approx 2^{-148}$ & \est{3.83}\\
\hline
\end{tabular}
\end{center}
One lane is inadequate. Since setup, channels, bindings and randomness target 128-bit computational security, $t=3$ is the smallest $t$ whose statistical term falls below $2^{-128}$, after which the primitives, not the MAC, limit the bound. Extra lanes barely change \CheckOpen{} itself (\est{0.648}~ms for $t=1$ versus \est{0.652}~ms for $t=3$ at $m=65{,}536$ on LAN, \cref{fig:checkperf}); their cost is one more authenticated GEMM lane per key (last column, \cref{sec:eval-ablation}).

\textbf{Tag-only errors.}
The bound concerns wrong \emph{values}: an error in a single tag lane escapes with probability $1/p$ without changing the opened value.

\textbf{Independent challenges.}
With one shared vector $\rho$, an adversary submitting $d_j=0$ and any $e\ne 0$ makes every lane residual $-\Delta_j\inner{\rho}{e}$, and all lanes vanish together with probability $1/p$. The product bound then collapses to one lane, so shared challenges are rejected (injection~8, \cref{tab:attacks}).

\textbf{Field, not ring.}
The step $\Delta_j=d_{j,i}/e_i$ needs a field. Over $\Z_{2^{64}}$, $e_i=2^{63}$ gives $\Delta_j e_i\equiv 0$ for every even $\Delta_j$, so one lane accepts with probability at least $1/2$; ring arithmetic needs a SPDZ2k-type backend~\cite{cramer2018spdz2k} with its own proof.

\textbf{Matrix checks.}
With $s=3$, each Freivalds call adds at most $p^{-3}\approx 2^{-183}$, i.e., about $2^{-151}$ for $Q_F\le 2^{32}$. Rejection sampling rejects one value with probability $2^{-61}$ per draw and retries under a fresh label; exhaustion affects only availability.

% =====================================================================
\subsection{Proof Boundary and Implementation Obligations}
\label{sec:sec-boundary}

\Cref{thm:main} concerns the abstract protocol in the protected-module model; \cref{tab:obligations} separates what this paper establishes from what a deployment must still provide. The executed CPU reference (22 unit tests, 0 failures, 0 errors; 21,840 DPF cases, 2,728 generate-and-consume comparisons, 1,364 DCF comparisons, 20,004 Mersenne multiplication checks, 124 signed-truncation cases; \cref{sec:eval-attack}) exercises finite cases and attack examples. It is neither a machine-checked proof nor evidence of 128-bit empirical security, and no forgery rate is inferred from zero observed failures: bounds come from the proofs, tests check conformance.

\begin{table}[t]
\centering
\caption{Proof boundary: what this paper establishes and what a deployment must still provide}
\label{tab:obligations}
\footnotesize
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}p{1.8cm}>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X}
\hline
\textbf{Obligation} & \textbf{Established here} & \textbf{Still required}\\
\hline
DPF/DCF, GaC, field, Boolean, LUT algebra & Explicit algorithms; \cref{thm:dpf-correct,thm:gac,thm:dcf,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval}; CPU reference tests & Constant-time, bit-exact CUDA and RTL refinement\\
\hline
Wrong-value authentication & \Cref{lem:hidden-key,thm:mac-sound}, independent lanes & Correct freeze, entropy, parser and check engine\\
\hline
End-to-end privacy and correctness & \Cref{thm:main} in the protected-module model & Realization of every module and trace assumption\\
\hline
PIR & \Cref{thm:pir} for the specified snapshot and regimes & Secure query channel, same-byte scan, certificates\\
\hline
GPU matrix verification & \Cref{thm:freivalds} & Protected verifier, bound input/result integration\\
\hline
Physical leakage and faults & Not claimed & Threat-specific engineering and evidence\\
\hline
Rollback protection & Required semantics specified (\cref{sec:proto-ledger}) & Monotonic service or erase-and-rekey lifecycle\\
\hline
Machine-checked proof & Not claimed & Future Lean, Coq or EasyCrypt development\\
\hline
\end{tabularx}
\end{table}

\textbf{Relation to the semi-honest design.}
The DFA analysis~\cite{dfa2026trusted} shows that its transformations preserve the security of the baseline FSS protocol. \Cref{thm:main} is a different statement about an explicitly specified protocol that tolerates a malicious host and GPU by placing a larger integrity and lifecycle responsibility inside the boundary. Trust is relocated to the modules, not removed (\cref{sec:discussion}); \ProfU (\cref{sec:threat-profileu}) serves deployments that cannot accept this.


==> qa/draft1/sections/08_evaluation.tex <==
% =====================================================================
% Section VIII: Evaluation
% Numbers: model/numbers.md (red via \est{}), DFA paper (black + cite),
% executed CPU reference tests (black).
% =====================================================================
\section{Evaluation}\label{sec:eval}

We evaluate \sys along the integrity chain of \cref{sec:threat} and organize the section around five questions.
(Q1)~What do the protected mechanisms cost per gate and per verified opening (\cref{sec:eval-micro,sec:eval-check})?
(Q2)~What does malicious security cost end to end, relative to semi-honest trusted DFA and to dealer-based malicious FSS (\cref{sec:eval-e2e})?
(Q3)~Does PIR keep the throughput of DFA once integrity is added (\cref{sec:eval-pir})?
(Q4)~Does the implementation reject the attacks of \cref{sec:threat-scenarios}, and what does the protected datapath cost in silicon (\cref{sec:eval-attack,sec:eval-hw})?
(Q5)~Which design choices matter, and how does the design scale (\cref{sec:eval-ablation,sec:eval-scale})?

% =====================================================================
\subsection{Evaluation Methodology}\label{sec:eval-method}

\textbf{Evidence Status.}
We distinguish three kinds of numbers throughout this section.
Black numbers cited to~\cite{dfa2026trusted} are copied from the semi-honest DFA paper; its end-to-end rows combine measured A100 execution with simulated DFA hardware.
Black numbers without a citation are either analytical (operation counts and security parameters such as $p=2^{61}-1$, $t=3$ and $Q(2/p)^t$) or counts from the executed CPU reference tests described in \cref{sec:eval-attack}.
Red numbers are estimates produced by the analytical performance model of \cref{app:model}; they are placeholders to be replaced by measurements.
The artifact has reached completion gates G0 (specification) and G1 (a functional model that passes its own tests); G2 (bit-exact GPU and RTL conformance), G3 (protected runtime) and G4 (two-party deployment and measured claims) are not yet complete.
Every conclusion drawn from a red number is therefore conditional on the model assumptions listed below, and we name the dominant assumption wherever a conclusion depends on it.

\textbf{Hardware Cost.}
The DFA blocks that \sys reuses (16 DPF units with 64 AES-128 engines, SRAM buffers, a 16-lane Ara VPU~\cite{cavalcante2019ara} and an SC300-class control unit~\cite{st33tpm12spi,arm_cortex_m3}) keep the TSMC 28\,nm synthesis results of~\cite{dfa2026trusted}, which use a pipelined open-source AES-128 core~\cite{opencores_aes128_pipeline}.
For the blocks that \sys adds (\cref{sec:arch-hw}), namely the Mersenne-61 field unit array (FUA), the check engine, the AEAD/GHASH freezer, the ledger with release guard and parser, and the ledger and freeze SRAMs, this revision reports pre-synthesis component estimates at the DFA clock (720\,MHz at 28\,nm, 910\,MHz at 7\,nm); they will be replaced by synthesis in the same 28\,nm flow.
As in DFA, we scale to 7\,nm with DeepScaleTool~\cite{sarangi2021deepscaletool}.
Separately, we size a functional prototype on a ZCU102 board (XCZU9EG, ffvb1156, speed grade $-2$)~\cite{amd2023zcu102} for Vivado implementation; its resource and power figures are pre-implementation estimates and will be reported separately from measured board energy.

\textbf{System-Level Performance.}
The target methodology for headline numbers is that of DFA: the module sits next to the GPU L2 slices, its DPF and FSS work is modeled as a stream consumed by GPU kernels in Accel-Sim~\cite{khairy2020accel}, where DFA delivers about 290\,GB/s~\cite{dfa2026trusted}, and non-FSS work comes from real GPU execution.
We keep three experiments strictly apart (\cref{sec:arch-deploy}): (i)~exact Mersenne-field kernels in software on a real A100, (ii)~the external ZCU102 functional and streaming prototype, and (iii)~the Accel-Sim study of hypothetical on-die integration.
No reported number combines (ii) with (iii).
Until (i) and (iii) are measured, every \sys configuration is derived from a decomposition of the trusted-mode DFA rows into GPU linear algebra, other GPU work, module FSS work, CPU-GPU transfers, online bytes and online rounds; this decomposition reproduces the LAN and WAN latencies of~\cite{dfa2026trusted} within \est{0.1\%}.
The malicious configuration then scales GPU linear algebra by the $(1+t)$ value and tag lanes and by \est{1.25$\times$} for exact 61-bit Mersenne GEMM relative to wraparound $\Z_{2^{64}}$ GEMM (Tensor Cores are not used for field arithmetic, \cref{sec:arch-field}), other GPU work by \est{1.35$\times$}, module FSS work by \est{1.45$\times$}, and online and CPU-GPU bytes by \est{1.3$\times$} for canonical 64-bit field words, residuals and certificates; it doubles the online round count, because each checked batch adds a residual exchange.
Triple generation runs on the FUA (128 multiply-accumulate lanes) and overlaps with GPU work except for an exposed \est{10\%}.
Each checked element costs 3.5 AES blocks (1.5 for challenge derivation and 2 for the AEAD freeze of a 32-byte tuple) and $2t=6$ field multiplications inside the module.
\Cref{app:model} lists all constants.

\textbf{Baselines.}
For private inference we compare five configurations per model.
\emph{GPU (SH)} and \emph{GPU+Trusted DFA (SH)} are the semi-honest rows of~\cite{dfa2026trusted}, which build on Orca~\cite{jawalkar2024orca} for CNNs and Sigma~\cite{gupta2023sigma} for Transformers.
\emph{Dealer-based malicious FSS} represents the actively secure, dealer-based protocol family of Shark~\cite{gupta2025shark}: an external dealer ships authenticated keys and preprocessing, which we model as \est{2.2$\times$} the semi-honest key and preprocessing volume and \est{2.0$\times$} the GPU FSS evaluation work, while charging exactly the same authenticated linear algebra, online bytes and doubled rounds as \sys.
The comparison therefore isolates preprocessing and key handling.
This row is a model of the protocol family and not a measurement of the Shark artifact; we make no performance claim against Shark itself until a matching artifact has been run, and the row will be replaced by that measurement.
\emph{GPU+\sys w/o GaC} generates authenticated material locally but, like the corresponding DFA ablation, spills it to host memory through the AEAD spill path and rereads it.
\emph{GPU+\sys} is the full design.
For PIR we compare GPU-DPF~\cite{lam2023gpu} and GPU+DFA, both semi-honest and taken from~\cite{dfa2026trusted}, a GPU-DPF variant that adds authenticated PIR in the style of Colombo et al.~\cite{colombo2023apir} (modeled at \est{0.45$\times$} the GPU-DPF throughput and \est{350}\,W), and GPU+\sys.

\textbf{Workloads.}
We run ResNet-50~\cite{he2016deep}, BERT-Base~\cite{devlin2019bert}, GPT-Neo~\cite{brown2020language} and LLaMA2-7B~\cite{touvron2023llama}, with 128 input tokens for the Transformer models, as in~\cite{dfa2026trusted}.
LAN is 1\,GB/s with a 0.05\,ms round-trip time (RTT) and WAN is 70\,MB/s with a 70\,ms RTT, following~\cite{gupta2023sigma,jawalkar2024orca,huang2026beyond}.
Malicious configurations use $\Fp$ with $p=2^{61}-1$ and $t=3$ MAC lanes; semi-honest rows use $\Z_{2^{64}}$ as in their sources.
Unless stated otherwise, the compiler selects among direct, LUT and interval gates by modeled cost (\cref{sec:proto-direct}).
PIR databases range from 16K to 4M entries of 128 bits, served in batches of 512 queries.
We do not report inference accuracy in this revision; exact finite-reference agreement and model accuracy will be reported separately once G2 is reached.

\textbf{Measurement Protocol.}
The replacement measurements will use 5 warm-up runs and 30 measured repetitions, report the median and the 95th percentile with bootstrap confidence intervals, keep raw per-run records, and fix random seeds only for public synthetic inputs, since randomness used for security must remain fresh.
We will report cold setup, amortized setup, preprocessing, online arithmetic, nonlinear evaluation, checking, transfers and final release as per-stage service times next to the critical-path wall time, counting both parties and any external preprocessing service.
Network conditions are shaped on dedicated interfaces with Linux traffic control, and achieved throughput and RTT are recorded.
GPU energy is the integral of sampled GPU power, board energy is measured at the rail or the wall, and every energy figure is cross-checked against average power times latency (or throughput times energy per query).
Each deployment uses two independent protected devices; a single ZCU102 with an emulated peer serves functional tests only.
GPUDirect RDMA~\cite{nvidia2024gpudirect} requires platform and driver support and usually a common PCIe root complex, so a staged transfer path remains the baseline, and the IOMMU stays enabled in all runs.

% =====================================================================
\subsection{Microbenchmarks}\label{sec:eval-micro}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_dpfthr.pdf}
\caption{Single-path DPF gate throughput per module (M gates/s, log scale) at 28\,nm, 720\,MHz and 64 AES-128 engines, for input length $n$: semi-honest trusted DFA, \sys (GaC with fresh authentication epilogue), and a malicious variant that runs $t=3$ extra tag trees. Model estimates.}
\label{fig:dpfthr}
\end{figure}

\textbf{DPF Gate Throughput.}
\Cref{fig:dpfthr} reports single-path DPF gate throughput per module.
Under GaC, each module advances two generator states and one evaluator state per level (\cref{alg:gac}), i.e., $3n$ expansions or $6n$ AES blocks per gate, so the two modules together perform $6n$ expansions instead of the $4n$ of one external generation plus two evaluations.
Semi-honest trusted DFA adds one block for output conversion; \sys adds three for output conversion and the four fresh epilogue pads.
\sys thus sustains \est{768}, \est{396}, \est{201} and \est{106}\,M gates/s for $n=8,16,32,61$, which is \est{6--9\%} below trusted DFA (\est{846} down to \est{113}\,M gates/s).
The tag-tree alternative, which evaluates one extra DPF tree with payload $\Delta_j\beta$ per MAC lane, reaches only \est{201} down to \est{26.7}\,M gates/s.
The epilogue is therefore \est{3.8--4.0$\times$} faster, approaching the factor $1+t=4$ by which tag trees multiply DPF work (\cref{tab:gatecost}).
Single-gate latency follows the 20-cycle dependent pipeline per level and equals \est{0.24}, \est{0.46}, \est{0.91} and \est{1.71}\,$\mu$s for the same $n$.
Two caveats apply.
First, both modules still reproduce the joint generation, so \sys removes the $t$ extra trees but not the duplicated generation.
Second, these are DPF gate rates, not inference throughput: a complete gate also includes input masking, a verified opening, authentication and the surrounding arithmetic, which the next paragraph and \cref{sec:eval-e2e} account for.

\begin{table}[t]
\centering
\caption{Authenticated nonlinear gate options per module ($n=61$; 28\,nm, 720\,MHz, 64 AES engines, 128 field lanes). Rounds, AES blocks and field multiplications are analytical counts per gate; throughput and LAN latency are model estimates.}
\label{tab:gates}
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l r r r r r}
\hline
\textbf{Gate} & \makecell{\textbf{Online}\\\textbf{rounds}} & \makecell{\textbf{AES}\\\textbf{blocks}} & \makecell{\textbf{Field}\\\textbf{mults}} & \makecell{\textbf{Thr.}\\\textbf{(M/s)}} & \makecell{\textbf{LAN lat.}\\\textbf{(ms)}} \\
\hline
Direct protected gate & 1 & 2 & 5 & \est{1800} & \est{0.100} \\
LUT, $w=8$ & 1 & 542 & 268 & \est{72.3} & \est{0.100} \\
LUT, $w=12$ & 1 & 8,238 & 4,112 & \est{4.75} & \est{0.100} \\
LUT, $w=16$ & 1 & 131,134 & 65,556 & \est{0.30} & \est{0.104} \\
Interval, conservative DCF & 1 & 22,692 & 8 & \est{1.73} & \est{0.100} \\
Interval, optimized DCF$^{\ast}$ & 1 & \est{976} & 8 & \est{40.1} & \est{0.100} \\
Bit decomposition & 123 & 244 & 122 & n/a & \est{12.3} \\
Exact signed truncation & 307 & n/m & 307 & n/a & \est{30.7} \\
\hline
\end{tabular}

\vspace{2pt}
\raggedright
\footnotesize
One online round is one \CheckOpen, i.e., two inter-module round trips. n/a: round-bound, throughput not meaningful; n/m: not modeled.
$^{\ast}$Projected $O(n)$ DCF; not covered by \cref{thm:dcf}.
\end{table}

\textbf{Nonlinear Gates.}
\Cref{tab:gates} compares the authenticated gate options of \cref{sec:proto-gates}.
All single-opening gates share a LAN latency of about \est{0.1}\,ms, because one \CheckOpen{} costs two inter-module round trips of 0.05\,ms each (\cref{alg:checkopen}); they differ in throughput.
The direct protected gate needs two AES blocks and five field multiplications and sustains \est{1800}\,M gates/s.
The XOR-masked LUT of \cref{alg:lut} scans its full domain, so its work grows as $2^w$: \est{72.3}\,M gates/s at $w=8$, \est{4.75} at $w=12$ and \est{0.30} at $w=16$, which confirms that only small tables are practical.
The interval gate of \cref{alg:interval} with the conservative DCF of \cref{thm:dcf} costs $2\cdot 6\cdot n(n+1)/2 = 22{,}692$ AES blocks at $n=61$ and reaches \est{1.73}\,M gates/s.
An optimized $O(n)$ DCF would reach \est{40.1}\,M gates/s, but it is a projection that our proofs do not cover.
Exact bit decomposition and signed truncation (\cref{alg:bitdec,alg:trunc}) are bound by sequential openings: $2n+1=123$ and $307$ rounds cost \est{12.3} and \est{30.7}\,ms on LAN.
The compiler therefore uses them only as a fallback when no table or interval formulation of the gate exists.

% =====================================================================
\subsection{Cost of Verified Openings}\label{sec:eval-check}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_checkopen.pdf}
\caption{\CheckOpen{} cost versus batch size $m$ (64 to 65,536 elements): (a)~LAN latency for $t=1,2,3$ MAC lanes (the curves overlap); (b)~throughput on LAN and WAN for $t=3$ (log scale). Model estimates.}
\label{fig:checkperf}
\end{figure}

\Cref{fig:checkperf} sweeps the \CheckOpen{} batch size $m$ from 64 to 65,536 elements, and three observations guide the compiler.
First, the number of MAC lanes barely matters for cost.
Challenge derivation takes $t/2$ AES blocks and the residual $2t$ field multiplications per element inside the module, and even at $m=65{,}536$ moving from $t=1$ to $t=3$ raises LAN latency only from \est{0.648} to \est{0.652}\,ms.
The statistical term, in contrast, improves from $2^{-28}$ to $2^{-148}$ at $Q=2^{32}$ (\cref{thm:mac-sound}).
Second, on LAN the check is latency-bound up to a few thousand elements: the two round trips (0.1\,ms) dominate, and latency grows only from \est{0.101} to \est{0.135}\,ms between $m=64$ and $m=4{,}096$.
Beyond that, the 8-byte value share per element on the peer link dominates (\est{0.52}\,ms of the \est{0.652}\,ms at $m=65{,}536$), and throughput saturates near \est{100}\,M elements/s.
Tags never cross the peer link; only frozen value shares and $t$ residuals do.
The protected work (freeze, challenge derivation and residuals) stays below \est{5\%} of the check latency at every batch size.
Third, on WAN the two 70\,ms round trips set a floor of 140\,ms per check, so throughput is only \est{0.44}\,M elements/s even at $m=65{,}536$.
Batching independent openings is therefore essential, and on WAN the round count, rather than bandwidth or module work, is the price of malicious security (\cref{sec:eval-e2e,sec:eval-ablation}).
Larger batches amortize round trips but increase staging memory and first-result latency, so the compiler batches only independent checks and keeps a checkpoint before every input-dependent nonlinear output and every final release; blind delayed checking is not justified by our proofs.

% =====================================================================
\subsection{End-to-End Private Inference}\label{sec:eval-e2e}

\begin{table*}[t]
\centering
\caption{End-to-end private inference per query. SH: semi-honest; Mal: static malicious security with abort. Latency is end to end, including offline distribution where present. Energy is GPU plus module energy summed over both computing parties (and the dealer when present). Module-GPU is the authenticated tuple stream per party on the on-die path; n/a: no module; n/r: not reported in~\cite{dfa2026trusted}. SH rows are copied from~\cite{dfa2026trusted}; red values are model estimates.}
\label{tab:e2e}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l l c r r r r r r}
\hline
\textbf{Model} & \textbf{Method} & \textbf{Security} & \makecell{\textbf{Offline}\\\textbf{comm. (GB)}} & \makecell{\textbf{CPU-GPU}\\\textbf{(GB)}} & \makecell{\textbf{Module-GPU}\\\textbf{(GB/party)}} & \makecell{\textbf{LAN}\\\textbf{latency (s)}} & \makecell{\textbf{WAN}\\\textbf{latency (s)}} & \makecell{\textbf{GPU+module}\\\textbf{energy (J)}} \\
\hline
\multirow{5}{*}{ResNet-50}
 & GPU~\cite{dfa2026trusted} & SH & 9.9 & 10.2 & n/a & 10.9 & 162 & 71.0 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.02 & 0.34 & n/r & 0.73 & 18.0 & 11.9 \\
 & Dealer-based malicious FSS & Mal & \est{21.8} & \est{22.4} & n/a & \est{25.1} & \est{346} & \est{170} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{38.0} & \est{1.22} & \est{2.97} & \est{34.7} & \est{48.6} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{0.44} & \est{1.22} & \est{1.79} & \est{33.6} & \est{43.6} \\
\hline
\multirow{5}{*}{BERT-Base}
 & GPU~\cite{dfa2026trusted} & SH & 17.1 & 19.3 & n/a & 18.8 & 296 & 121 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.1 & 2.55 & n/r & 1.42 & 46.4 & 18.2 \\
 & Dealer-based malicious FSS & Mal & \est{37.6} & \est{42.5} & n/a & \est{43.9} & \est{630} & \est{290} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{68.6} & \est{1.66} & \est{5.87} & \est{91.8} & \est{82.2} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{3.31} & \est{1.66} & \est{3.83} & \est{89.7} & \est{73.7} \\
\hline
\multirow{5}{*}{GPT-Neo}
 & GPU~\cite{dfa2026trusted} & SH & 76.4 & 80.4 & n/a & 83.6 & 1140 & 587 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.24 & 4.27 & n/r & 5.93 & 101 & 114 \\
 & Dealer-based malicious FSS & Mal & \est{168} & \est{177} & n/a & \est{197} & \est{2611} & \est{1409} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{296} & \est{9.92} & \est{28.6} & \est{209} & \est{522} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{5.55} & \est{9.92} & \est{19.5} & \est{200} & \est{477} \\
\hline
\multirow{5}{*}{LLaMA2-7B}
 & GPU~\cite{dfa2026trusted} & SH & 256 & 268 & n/a & 279 & 3695 & 1879 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.81 & 12.8 & n/r & 18.0 & 193 & 303 \\
 & Dealer-based malicious FSS & Mal & \est{563} & \est{590} & n/a & \est{661} & \est{8467} & \est{4510} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{994} & \est{33.3} & \est{93.6} & \est{418} & \est{1483} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{16.6} & \est{33.3} & \est{63.1} & \est{387} & \est{1343} \\
\hline
\end{tabular}
\end{table*}

\Cref{tab:e2e} reports per-query results for the four models.
The semi-honest rows are context, not same-security competitors: they show what the trusted-DFA design achieves before malicious security is added.

\textbf{Comparison with Dealer-Based Malicious FSS.}
The modeled dealer-based baseline pays for malicious security mainly in the offline phase.
Its authenticated keys and preprocessing reach \est{21.8}, \est{37.6}, \est{168} and \est{563}\,GB per query, which the dealer ships over the network and each party then stages through CPU-GPU transfers (\est{22.4} to \est{590}\,GB).
\sys generates the authenticated correlations inside the modules and ships none of them, so offline communication shrinks to session setup (\est{$<$0.001}\,GB).
Across the four models this yields \est{10.1--14.0$\times$} lower LAN latency, \est{7.0--21.9$\times$} lower WAN latency and \est{3.0--3.9$\times$} lower energy than the modeled baseline; for BERT-Base the factors are \est{11.4$\times$}, \est{7.0$\times$} and \est{3.9$\times$}.
The WAN gain is largest for LLaMA2-7B (\est{21.9$\times$}), whose \est{563}\,GB of authenticated material alone would occupy a 70\,MB/s link for more than \est{2.2}\,hours.

\textbf{Cost of Malicious Security.}
Relative to semi-honest trusted DFA, \sys raises LAN latency by \est{2.46--3.51$\times$} and WAN latency by \est{1.86--2.01$\times$}.
It nevertheless remains \est{4.3--6.1$\times$} faster on LAN and \est{3.3--9.5$\times$} faster on WAN than the semi-honest GPU baseline, and it uses \est{1.2--1.6$\times$} less energy, although it tolerates a malicious host.
CPU-GPU traffic grows by only \est{1.3$\times$} over trusted DFA (e.g., \est{3.31} vs.\ 2.55\,GB for BERT-Base), because authenticated tuples move between the module and the GPU over the on-die path (\est{1.22} to \est{33.3}\,GB per party) instead of through host memory.

\textbf{Generate-and-Consume Remains Essential.}
Without GaC, the locally generated authenticated material must be spilled and reread, which inflates CPU-GPU traffic by \est{20.7--86$\times$} (\est{68.6} instead of \est{3.31}\,GB for BERT-Base) and LAN latency by \est{1.47--1.66$\times$}.
The authenticated representation makes materialization costlier than in the semi-honest case, where DFA reports 36.1\,GB of CPU-GPU traffic and a 1.74$\times$ LAN penalty for BERT-Base without GaC~\cite{dfa2026trusted}.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_bert.pdf}
\caption{BERT-Base bottleneck analysis for \sys (model estimates). (a)~Speedup over dealer-based malicious FSS versus network bandwidth, split into the part due to eliminated key and preprocessing distribution and the remainder. (b)~LAN latency versus host-module link bandwidth (1.6, 8, 25 and 290\,GB/s). (c)~Breakdown of the \est{3.83}\,s LAN latency.}
\label{fig:bert}
\end{figure}

\textbf{Bottleneck Analysis.}
\Cref{fig:bert} decomposes the BERT-Base results.
(a)~The advantage over the dealer-based baseline depends on network bandwidth: \est{43.7$\times$} at 0.1\,GB/s, \est{11.4$\times$} at 1\,GB/s and \est{2.9$\times$} at 10\,GB/s.
At 1\,GB/s, \est{9.8$\times$} of the \est{11.4$\times$} comes from eliminated key and preprocessing distribution; at 10\,GB/s the remaining \est{1.7$\times$} from lower key I/O and cheaper FSS evaluation dominates.
Faster networks shrink the advantage but do not remove it, and, as observed for the semi-honest case~\cite{dfa2026trusted,huang2026beyond}, the energy and monetary cost of moving tens of gigabytes per query persists at any bandwidth.
(b)~Moving the module off die costs little for BERT-Base: LAN latency is \est{3.83}\,s on die (290\,GB/s), \est{3.87}\,s over a 25\,GB/s PCIe-class link, \est{3.96}\,s at 8\,GB/s and \est{4.46}\,s at the 1.6\,GB/s of the ZCU102 prototype, because only \est{1.66}\,GB of authenticated tuples per party cross the link.
(c)~With malicious security the dominant cost moves from DPF to authenticated linear algebra.
The four-lane GEMM takes \est{2.60}\,s (\est{68\%}) of the \est{3.83}\,s; online communication takes \est{0.615}\,s (\est{16\%}), other GPU work \est{0.338}\,s, CPU-GPU transfer \est{0.133}\,s and nonlinear gates \est{0.131}\,s, while triple generation, checks and on-die transfers together take \est{0.016}\,s.
Of the \est{2.41}\,s that \sys adds over trusted DFA, \est{86\%} is authenticated GEMM.
The protected module is thus not the bottleneck; the tag lanes on the GPU and the doubled round count are, which motivates the compressed-check direction discussed in \cref{sec:eval-scale}.

% =====================================================================
\subsection{Private Information Retrieval}\label{sec:eval-pir}

\begin{table}[t]
\centering
\caption{PIR throughput and energy per query (128-bit entries, batch 512). SH rows are from~\cite{dfa2026trusted} with energy expressed in mJ; implied power is throughput times energy per query and serves as a unit cross-check. Integrity: the client obtains the committed record or abort against a malicious server. Red values are model estimates.}
\label{tab:pir}
\footnotesize
\setlength{\tabcolsep}{2.8pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l l c r r r}
\hline
\textbf{DB} & \textbf{Method} & \textbf{Integ.} & \makecell{\textbf{Throughput}\\\textbf{(k queries/s)}} & \makecell{\textbf{Energy/}\\\textbf{query (mJ)}} & \makecell{\textbf{Implied}\\\textbf{power (W)}} \\
\hline
\multirow{4}{*}{16K}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & 134 & 2.61 & 350 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & 1,125 & 0.187 & 210 \\
 & GPU-DPF+APIR & \cmark & \est{60.3} & \est{5.80} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \est{1,046} & \est{0.180} & \est{188} \\
\hline
\multirow{4}{*}{1M}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & 3.48 & 100 & 348 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & 17.58 & 11.9 & 209 \\
 & GPU-DPF+APIR & \cmark & \est{1.57} & \est{224} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \est{16.35} & \est{11.5} & \est{188} \\
\hline
\multirow{4}{*}{4M}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & 0.788 & 443 & 349 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & 4.39 & 47.7 & 209 \\
 & GPU-DPF+APIR & \cmark & \est{0.355} & \est{987} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \est{4.08} & \est{46.0} & \est{188} \\
\hline
\end{tabular}
\end{table}

\Cref{tab:pir} reports PIR throughput and energy per query.
We express energy per query in mJ: with this unit, throughput multiplied by energy per query gives a consistent average power for every source row (about 350\,W for GPU-DPF and 210\,W with DFA), which we list as a cross-check column.

\sys retains \est{93\%} of the semi-honest DFA throughput at every database size (\est{1,046}, \est{16.35} and \est{4.08}\,k queries/s for 16K, 1M and 4M entries), while guaranteeing that an honest client receives the committed record or abort even with one malicious server host (\cref{thm:pir}).
The \est{7\%} loss models the work that \cref{alg:pir} adds to the protected path: hashing the snapshot bytes actually consumed, the field-weighted record reduction inside the module, and a fresh resharing with bound certificates per query.
Energy per query is \est{3--4\%} lower than with DFA (\est{0.180} vs.\ 0.187\,mJ at 16K entries), because the record reduction runs inside the protected path instead of on the SMs, which lowers the modeled average power to \est{188}\,W.
This effect rests entirely on the power model and is among the first values we will measure.
Against the authenticated GPU baseline, \sys is \est{10.4--17.4$\times$} faster and \est{19--32$\times$} more energy efficient; against semi-honest GPU-DPF it is \est{4.7--7.8$\times$} faster.

\textbf{Bottleneck Analysis.}
As in DFA, full-domain PIR is bound by DPF expansion in the AES array rather than by memory: DFA expands about 18.4\,G leaves/s~\cite{dfa2026trusted}, and \sys about \est{17.1}\,G leaves/s.
The additional protected work is amortized over a batch.
Each batch of 512 queries scans the snapshot once in public order, so the snapshot hash costs one pass per batch rather than one per query, and every record is weighted by the 512 DPF outputs of the batch in the FUA.
A 128-bit record occupies three $\Fp$ coordinates, all weighted by the same DPF output (\cref{sec:proto-pir}); at 16K entries this requires about \est{51}\,G field multiply-accumulates per second, within the 92\,G/s peak of the 128-lane FUA at 720\,MHz.
Integrity therefore does not move the PIR bottleneck; it consumes part of the slack of the protected datapath.

% =====================================================================
\subsection{Security Validation}\label{sec:eval-attack}

\begin{table*}[t]
\centering
\caption{Attack and fault injections, the mechanism that must stop each one, coverage by the executed CPU reference model (\cmark: executed and passing; planned: no executed evidence yet), and the expected outcome on the RTL and FPGA implementations (red: expected, not yet observed). Scenario ids refer to \cref{tab:scenarios}.}
\label{tab:attacks}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{c >{\raggedright\arraybackslash}p{4.3cm} >{\raggedright\arraybackslash}p{5.0cm} c >{\raggedright\arraybackslash}p{4.9cm}}
\hline
\textbf{\#} & \textbf{Injection} & \textbf{Mechanism} & \makecell{\textbf{Reference}\\\textbf{model}} & \textbf{Expected RTL/FPGA outcome} \\
\hline
1 & Change payload, query, role, gate id, table hash or shape (S5) & Ledger descriptor binding; role- and gate-bound PRF labels (\cref{sec:proto-ledger}) & \cmark & \est{Rejected at frame parse or authenticated computation fails; no preprocessing issued} \\
2 & Flip a control bit, root seed or correction word in a candidate engine &Conformance against the reference DPF (\cref{thm:dpf-correct}); unverified engine output is never authenticated & planned & \est{Reference mismatch flagged; engine output never authenticated or released} \\
3 & Change a GPU value share or tag (S1) & \CheckOpen{} with $t=3$ independent lanes (\cref{thm:mac-sound}) & \cmark & \est{Abort within one \CheckOpen{} (0.10--0.65\,ms on LAN)}; acceptance at most $(2/p)^3$ per batch \\
4 & Triple with valid-looking tags but $c\neq ab$ (S7) & Triples computed inside the TCB; imported material needs a correctness proof & planned & \est{Never consumed; unproven import refused at reservation} \\
5 & Reuse a mask or counter; reset and resume old keys (S4) & One-time ledger, epoch poisoning, erase-and-rekey & \cmark & \est{Rejected before any accepted reuse} \\
6 & Modify a DMA buffer after freezing (S3) & Freeze-before-challenge; consume only frozen pages & \cmark & \est{Frozen authenticated bytes consumed, or abort} \\
7 & Swap only the last column of a GPU matrix product & Frozen-operand Freivalds over all columns, $s=3$ (\cref{thm:freivalds}) & planned & \est{Rejected}, except with probability at most $p^{-3}$ \\
8 & Reuse one challenge vector across MAC lanes & Independent per-lane challenges; configuration check & \cmark\,(toy) & \est{Configuration refused at session setup} \\
9 & Change database bytes or version after hashing (S8) & Same-byte snapshot hash and certificate binding (\cref{thm:pir}) & \cmark & \est{Abort; quarantined result never released} \\
10 & Request output before the verification barrier (S6) & Release guard (\cref{sec:proto-ledger}) & planned & \est{Guard stays closed; no candidate values leave} \\
11 & Overflow or truncate with the wrong signed rule & Exact finite reference; numeric contract (\cref{thm:cmp-trunc}) & \cmark & \est{Mismatch detected; manifest rejected} \\
12 & Delay, drop or reorder packets (S10) & Bounded resources and abort & planned & \est{Abort; no fairness or availability claimed} \\
\hline
\end{tabular}
\end{table*}

\Cref{tab:attacks} lists the twelve attack and fault injections of our test plan, the mechanism that must stop each one, whether the executed CPU reference model already covers it, and the outcome we expect on the RTL and FPGA implementations.
The injections cover the scenarios of \cref{tab:scenarios} except the forgery-oracle scenario S2, which the interface excludes by construction rather than by a runtime check: the command set of \cref{tab:commands} has no entry point that authenticates a host-supplied value, and row~2 checks the related requirement that even the module's own engine output is never authenticated before it conforms to the reference.

\textbf{Executed Functional Validation.}
The functional reference implements the ideal-module model in Python~3.10+ using only the standard library.
In the preparation environment it passes 22 unit tests with 0 failures and 0 errors.
The tests cover 21,840 exhaustive small-domain DPF target, query and payload cases (\cref{thm:dpf-correct}); 2,728 party-local comparisons between streaming GaC and materialized evaluation (\cref{thm:gac}); 1,364 DCF comparisons (\cref{thm:dcf}); 20,004 CPU checks of the GPU Mersenne multiplication formula of \cref{sec:arch-field} against arbitrary-precision arithmetic, including boundary operands; all 31 elements of a toy field with $p=31$ for bit decomposition (\cref{thm:bitdec}); 124 signed-truncation cases (\cref{thm:cmp-trunc}); all 16 inputs of a small LUT (\cref{thm:lut}); selected exhaustive toy intervals (\cref{thm:interval}); a small composed nonlinear and arithmetic pipeline; and PIR snapshot rejection.
Negative tests exercise noncanonical encodings, tag and value mutations, poisoned epochs, role, replay and ordering errors, immutable frozen objects, joint sampling, truncation fibers, and the ring zero-divisor counterexample that motivates the field representation (\cref{app:proof-auth}).

\textbf{Limits of This Evidence.}
The toy field $p=31$ serves finite correctness tests only and provides no cryptographic security.
The reference expands seeds with SHAKE rather than the pinned AES-based PRG, so the equivalence tests must be rerun against the production PRG and output conversion.
The CUDA micro-test (65,536 products against a host 128-bit reference) is written but has not been compiled or run, and the RTL release guard is written but has not been simulated or synthesized; no GPU toolchain, Vivado or RTL simulator was available in that environment.
Rows marked ``planned'' in \cref{tab:attacks} therefore have no executed evidence yet.
Most importantly, these tests check that the implementation conforms to the algorithms; they do not measure a forgery probability.
Observing zero accepted forgeries in any finite campaign cannot support a bound such as $2^{-148}$; that bound comes from \cref{thm:mac-sound} together with the ledger rules, and testing only checks that the implementation realizes the assumptions of the proof.
Power and electromagnetic analysis, probing and fault injection require separate, threat-specific engineering evaluation (\cref{sec:discussion}).

% =====================================================================
\subsection{Hardware Cost}\label{sec:eval-hw}

\begin{table}[t]
\centering
\caption{Hardware cost of one \sys module. DFA blocks are synthesis results from~\cite{dfa2026trusted}; blocks added by \sys are pre-synthesis estimates (red). 7\,nm values are scaled with DeepScaleTool~\cite{sarangi2021deepscaletool}.}
\label{tab:hwcost}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l r r r r}
\hline
\multirow{2}{*}{\textbf{Component}} & \multicolumn{2}{c}{\textbf{28\,nm}} & \multicolumn{2}{c}{\textbf{7\,nm}} \\
\cline{2-5}
 & \textbf{mm$^2$} & \textbf{mW} & \textbf{mm$^2$} & \textbf{mW} \\
\hline
\multicolumn{5}{l}{\textit{DFA blocks reused by \sys~\cite{dfa2026trusted}}} \\
16 DPF units (64 AES-128) & 1.73 & 29 & 0.054 & 11 \\
SRAM buffers & 3.06 & 585 & 0.096 & 219 \\
VPU (16-lane Ara) & 1.97 & 794 & 0.062 & 298 \\
All DFA (incl.\ control unit) & 7.67 & 1,683.5 & 0.239 & 631 \\
\hline
\multicolumn{5}{l}{\textit{Blocks added by \sys}} \\
Field unit array (128 lanes) & \est{2.80} & \est{1,000} & \est{0.088} & \est{375} \\
Check engine & \est{0.18} & \est{45} & \est{0.006} & \est{17} \\
AEAD + GHASH freezer & \est{0.21} & \est{60} & \est{0.007} & \est{23} \\
Ledger, guard, parser & \est{0.09} & \est{12} & \est{0.003} & \est{5} \\
Ledger SRAM (32\,KB) & \est{0.25} & \est{35} & \est{0.008} & \est{13} \\
Freeze SRAM (256\,KB) & \est{1.07} & \est{200} & \est{0.033} & \est{75} \\
\cline{1-5}
\sys additions & \est{4.60} & \est{1,352} & \est{0.145} & \est{508} \\
\hline
\rowcolor{blue!6}All \sys & \est{12.27} & \est{3,036} & \est{0.384} & \est{1,139} \\
\hline
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{Planned ZCU102 functional prototype (XCZU9EG-2FFVB1156~\cite{amd2023zcu102}): configuration and pre-implementation estimates (red).}
\label{tab:fpga}
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l r r r}
\hline
\textbf{Resource} & \textbf{Used} & \textbf{Available} & \textbf{Utilization} \\
\hline
LUT & \est{168K} & 274K & \est{61\%} \\
Flip-flop & \est{201K} & 548K & \est{37\%} \\
BRAM36 & \est{412} & 912 & \est{45\%} \\
DSP & \est{356} & 2,520 & \est{14\%} \\
\hline
\multicolumn{4}{l}{Datapath: 4 DPF units (16 AES-128), 32 field lanes, 250\,MHz} \\
\multicolumn{4}{l}{DPF throughput: \est{1.0}\,G expansions/s; board power: \est{9.8}\,W} \\
\multicolumn{4}{l}{Host link: 1.6\,GB/s, i.e., 50\,M authenticated elements/s} \\
\hline
\end{tabular}
\end{table}

\Cref{tab:hwcost} reports the cost of one module.
\sys adds \est{4.60}\,mm$^2$ and \est{1.35}\,W at 28\,nm to the 7.67\,mm$^2$ and 1.68\,W of DFA~\cite{dfa2026trusted}; at 7\,nm the additions are \est{0.145}\,mm$^2$ and \est{0.508}\,W, and the complete module occupies \est{0.384}\,mm$^2$ and draws \est{1.14}\,W.
This is \est{0.046\%} of the 826\,mm$^2$ A100 die~\cite{nvidia2020ampere}.
The FUA dominates the additions with \est{61\%} of the added area and \est{74\%} of the added power at 7\,nm, followed by the 256\,KB freeze SRAM with \est{23\%} of the added area.
The logic that enforces the security policy (ledger, release guard, parser and check engine) takes only \est{0.009}\,mm$^2$, or \est{6\%} of the additions.
As in DFA, arithmetic and memory dominate the cost, not control.
No AES engines are added: challenge derivation (1.5 blocks per checked element) and AEAD freezing (2 blocks per 32-byte tuple) time-share the 64 engines with PRG expansion.
For BERT-Base, checking occupies the AES array and the FUA for about \est{2.8}\,ms per query, below \est{0.1\%} of its latency.
The freeze SRAM holds 8,192 authenticated 32-byte tuples; larger batches spill as AEAD-sealed immutable pages bound to sequence numbers, lengths, gate ids and a protected root (\cref{sec:proto-ledger}), which costs HBM bandwidth but no additional trusted storage.

\Cref{tab:fpga} sizes the external ZCU102 prototype.
Four DPF units with 16 AES engines and 32 field lanes at 250\,MHz are estimated to use \est{61\%} of the LUTs, \est{37\%} of the flip-flops, \est{45\%} of the BRAM and \est{14\%} of the DSP slices, at \est{9.8}\,W board power and \est{1.0}\,G expansions/s.
The prototype exists to check functional conformance and streaming behavior with two independent boards.
Its 1.6\,GB/s host link (50\,M authenticated elements/s at 32 bytes each) and its smaller FUA make it a pessimistic performance point, which the ablation quantifies (\cref{tab:ablation}).
Moreover, an ordinary ARM process on the board is not automatically isolated from a malicious board administrator, so the prototype is not a \ProfT deployment target.

% =====================================================================
\subsection{Ablation Study}\label{sec:eval-ablation}

\begin{table*}[t]
\centering
\caption{Ablation on BERT-Base (LAN 1\,GB/s, WAN 70\,MB/s). Each row changes one choice of the full design. Rel.\ LAN is LAN latency relative to the full design. Secure: \cmark{} covered by our theorems; \pmark{} projected construction outside our proofs; \xmark{} not secure (statistically inadequate, or no verification). All latency and energy values are model estimates.}
\label{tab:ablation}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l c r r r r >{\raggedright\arraybackslash}p{5.1cm}}
\hline
\textbf{Configuration} & \textbf{Secure} & \makecell{\textbf{LAN}\\\textbf{(s)}} & \makecell{\textbf{Rel.}\\\textbf{LAN}} & \makecell{\textbf{WAN}\\\textbf{(s)}} & \makecell{\textbf{Energy}\\\textbf{(J)}} & \textbf{Note} \\
\hline
\rowcolor{blue!6}Full \sys ($t=3$, compiled gates, batched checks) & \cmark & \est{3.83} & \est{1.00$\times$} & \est{89.7} & \est{73.7} & Reference configuration \\
w/o GaC & \cmark & \est{5.87} & \est{1.53$\times$} & \est{91.8} & \est{82.2} & Authenticated material spilled and reread \\
Tag trees instead of epilogue & \cmark & \est{4.12} & \est{1.08$\times$} & \est{90.0} & \est{80.4} & $(1+t)\times$ DPF work; FSS share is small \\
$t=1$ MAC lane & \xmark & \est{2.53} & \est{0.66$\times$} & \est{88.4} & \est{43.2} & $Q(2/p)^t=2^{-28}$ at $Q=2^{32}$: inadequate \\
$t=2$ MAC lanes & \cmark & \est{3.18} & \est{0.83$\times$} & \est{89.1} & \est{58.4} & $2^{-88}$ at $Q=2^{32}$ \\
FSS-only gates, conservative DCF & \cmark & \est{15.29} & \est{3.99$\times$} & \est{101.2} & \est{342.2} & $O(n^2)$ DCF of \cref{thm:dcf} \\
FSS-only gates, optimized DCF & \pmark & \est{4.20} & \est{1.10$\times$} & \est{90.1} & \est{82.3} & Projected; not covered by \cref{thm:dcf} \\
Direct protected gates only & \cmark & \est{3.82} & \est{1.00$\times$} & \est{89.7} & \est{73.3} & \ProfT only; no FSS compatibility \\
Small check batches ($m=64$) & \cmark & \est{4.24} & \est{1.11$\times$} & \est{90.2} & \est{74.6} & Per-batch overhead not amortized \\
External PCIe module (25\,GB/s) & \cmark & \est{3.87} & \est{1.01$\times$} & \est{89.8} & \est{73.8} & Link roofline $B/32$ elements/s \\
ZCU102 link (1.6\,GB/s, 32 lanes, 250\,MHz) & \cmark & \est{4.59} & \est{1.20$\times$} & \est{90.5} & \est{75.4} & Prototype link and slower triple generation \\
No \CheckOpen{} & \xmark & \est{3.80} & \est{0.99$\times$} & \est{50.5} & \est{73.6} & INSECURE performance lower bound \\
\hline
\end{tabular}
\end{table*}

\Cref{tab:ablation} changes one design choice at a time for BERT-Base.

\textbf{Protocol Mechanisms.}
Disabling GaC costs \est{1.53$\times$} LAN latency, as discussed in \cref{sec:eval-e2e}.
Replacing the epilogue by tag trees costs only \est{8\%} LAN latency end to end (\est{4.12} vs.\ \est{3.83}\,s) and \est{9\%} energy, although it quadruples DPF work (\cref{fig:dpfthr}): in BERT-Base, FSS evaluation is a small part of the malicious latency.
The epilogue matters most when FSS work dominates, for example in LUT-heavy compiled models, where the \est{3.8--4.0$\times$} gate-level gap of \cref{sec:eval-micro} carries over.

\textbf{MAC Lanes.}
With $t=1$ the LAN latency drops to \est{2.53}\,s, but the statistical term $Q(2/p)$ is only $2^{-28}$ at $Q=2^{32}$, which is inadequate; $t=2$ gives $2^{-88}$ at \est{3.18}\,s.
We choose $t=3$, whose $2^{-148}$ is well below the 128-bit computational target of the primitives (\cref{sec:sec-concrete}); each lane costs about \est{0.65}\,s of authenticated GEMM for BERT-Base.

\textbf{Gate Selection.}
Restricting the compiler to FSS gates with the conservative $O(n^2)$ DCF raises LAN latency to \est{15.29}\,s (\est{4.0$\times$}) and energy to \est{342}\,J, because every interval gate then costs 22,692 AES blocks.
A projected optimized DCF would cut this to \est{4.20}\,s, but it lies outside \cref{thm:dcf} and would first need its own correctness, distribution and interface obligations.
The direct protected gate alone is marginally faster than the compiled mix (\est{3.82} vs.\ \est{3.83}\,s), a difference within model resolution.
Under \ProfT the direct gate is therefore a legitimate competitor, and the compiler may select it.
We keep LUT and interval FSS in the compiler because they remain compatible with FSS-compiled models and with \ProfU, where DPF keys are exported to an external malicious backend, and because full-domain scans match the pipelined AES engine (\cref{sec:proto-direct}).

\textbf{Batching and Placement.}
Checking in batches of only $m=64$ adds \est{11\%} LAN latency through unamortized per-batch overhead.
An external module on a 25\,GB/s PCIe link adds \est{1\%}, and the ZCU102 configuration adds \est{20\%}; of the latter, the slower triple generation of 32 lanes at 250\,MHz contributes \est{0.13}\,s beyond the link effect (\est{4.59} vs.\ \est{4.46}\,s).
Finally, removing \CheckOpen, which is insecure and listed only as a performance lower bound, barely changes LAN latency (\est{3.80}\,s) but cuts WAN latency from \est{89.7} to \est{50.5}\,s.
The \est{39}\,s difference is the doubled round count, the dominant WAN cost of malicious security.
Ablations on staged versus local checks and on caching versus recomputing bit decompositions are part of the measurement plan but are not yet modeled.

% =====================================================================
\subsection{Scalability}\label{sec:eval-scale}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_scale.pdf}
\caption{Scalability (model estimates). (a)~LAN latency with $t=1,2,3$ MAC lanes, normalized to semi-honest trusted DFA, annotated with the statistical term $Q(2/p)^t$ at $Q=2^{32}$ ($2^{-28}$, $2^{-88}$, $2^{-148}$). (b)~PIR throughput (queries/s, log scale) for $2^{14}$ to $2^{24}$ entries.}
\label{fig:scale}
\end{figure}

\textbf{MAC Lanes and Model Size.}
\Cref{fig:scale}(a) normalizes LAN latency to semi-honest trusted DFA.
With $t=3$ the overhead grows from \est{2.46$\times$} for ResNet-50 to \est{3.51$\times$} for LLaMA2-7B, because the share of linear algebra grows with model size and each MAC lane replicates it: every additional lane adds about \est{0.65}\,s for BERT-Base and \est{13.0}\,s for LLaMA2-7B.
Authenticated GEMM on the GPU, not the protected module, is the scaling bottleneck.

\textbf{Triple Generation.}
Correct matrix triples must be computed inside the protected boundary (\cref{sec:proto-arith}), so FUA work scales with the model's multiply-accumulate count.
LLaMA2-7B needs about \est{7.18}\,s of FUA time per query at 128 lanes and 910\,MHz, which overlaps with the \est{52.0}\,s of authenticated GEMM and leaves about \est{0.72}\,s exposed.
The 32-lane prototype at 250\,MHz would need about \est{105}\,s for the same triples; this is one more reason why it is a functional prototype rather than a performance target for large models, and why the on-die FUA should scale with the linear-algebra throughput of the host GPU.
If triple generation ever dominates, the alternatives are an imported malicious preprocessing backend with its own proof, or restructuring public-by-secret operations; exposing global secret masks to the GPU is not an option.

\textbf{Host-Module Bandwidth.}
Authenticated traffic is at least 32 bytes per element and party, so a link of bandwidth $B$ bounds the output stream at $B/32$ elements/s: about 9.1\,G elements/s on die at 290\,GB/s, 781\,M elements/s over a 25\,GB/s PCIe link, and 50\,M elements/s over the ZCU102 link.
BERT-Base moves \est{1.66}\,GB per party, well inside the on-die budget, which is why \cref{fig:bert}(b) is nearly flat above 8\,GB/s.

\textbf{PIR.}
\Cref{fig:scale}(b) shows PIR throughput from $2^{14}$ to $2^{24}$ entries.
Like DFA, \sys scales linearly in the number of entries, from \est{1.05}\,M down to \est{1,022} queries/s, whereas GPU-DPF reaches its peak per-entry efficiency near $2^{20}$ entries~\cite{dfa2026trusted,lam2023gpu}.
At $2^{24}$ entries \sys is \est{5.2$\times$} faster than GPU-DPF and \est{11.5$\times$} faster than the authenticated GPU baseline.
Larger records increase the per-entry field reduction linearly while the DPF expansion stays unchanged, so for very large records the FUA, not the AES array, becomes the limit.

\textbf{Beyond Per-Lane Tags.}
Because the tag lanes dominate large models, the most promising direction is to compress MAC checking, for example with rank-1 compressed checks that avoid carrying $t$ full tag arrays through the GPU.
Such schemes are not covered by our proofs and need their own soundness analysis, so we leave them to future work.
Scaling the number of DPF units and FUA lanes is a second, orthogonal knob; DFA found DPF-unit scaling to be nearly linear until on-chip bandwidth, about 7\,TB/s of aggregate L2 read bandwidth on A100~\cite{nvidia2020ampere}, becomes the limit~\cite{dfa2026trusted}.


==> qa/draft1/sections/09_discussion.tex <==
% ==================================================================
% Section IX: Discussion and Limitations
% Owner labels: sec:discussion
% ==================================================================
\section{Discussion and Limitations}
\label{sec:discussion}

\sys claims that, under \ProfT, one maliciously corrupted host, including its GPU, driver and network stack, cannot make an honest party accept a wrong value or release an unauthorized one, except with the probability bounded in \cref{thm:main}. We now state what this claim does not cover and which evidence is still missing.

\textbf{Trust relocation, not removal.}
\sys moves the dealer of dealer-based FSS into two protected modules; it does not remove the dealer assumption. Both modules hold the joint-sampler key and the global MAC keys $\Delta_1,\dots,\Delta_t$ (\cref{sec:proto-setup}), so extracting the secrets of either module voids privacy and integrity for every session whose keys it holds. Attestation authenticates the module's code and configuration; only the MAC, freeze and ledger machinery of \cref{sec:protocol} establishes that the untrusted GPU computed correctly. \Cref{thm:main} is an abstract-protocol statement in the ideal-module model of \cref{sec:threat-model}: it does not prove that a concrete chip realizes that model, and it excludes adaptive corruption, corruption of both hosts, client-server collusion, leakage beyond the stipulated traces, speculative-execution bugs inside the trusted boundary and faulty trusted arithmetic. The boundary also grows relative to DFA~\cite{dfa2026trusted}: the ledger, freezer, check engine, field unit array and release guard add only \est{0.145~mm$^2$} at 7~nm (\cref{tab:hwcost}), but each of them is logic that must be verified (\cref{tab:obligations}).

\textbf{What the modules learn.}
The modules are not blind. After a verified opening $c = x + r$, module $T_b$ knows $c$ and its own mask $r$, hence $x$; the committed-input loader and the direct gate (\cref{sec:proto-direct}) see inputs explicitly, and in PIR both modules receive the client's index (\cref{alg:pir}). This is inherent to generate-and-consume and already holds for trusted DFA~\cite{dfa2026trusted}, so \sys does not claim that inputs are hidden from its modules. FSS gates keep only pseudorandom seeds, control bits and correction words in long-lived state and never materialize $x$ in a single register, whereas a direct gate computes on $x$ itself. We treat this as defense in depth only, because the trace model of \cref{thm:main} makes both options equivalent. Its price is visible in \cref{tab:ablation}: for BERT-Base on LAN, FSS-only execution with the conservative $O(n^2)$ DCF of \cref{thm:dcf} needs \est{15.29~s}, a projected optimized DCF that our proofs do not cover needs \est{4.20~s}, and direct-only execution needs \est{3.82~s}, essentially the cost-aware default (\est{3.83~s}).

\textbf{Where the malicious cost goes.}
Relative to semi-honest trusted DFA (1.42~s for BERT-Base on LAN~\cite{dfa2026trusted}), \sys costs \est{2.70$\times$}, and DPF is no longer the main reason. Authenticated GEMM on the GPU, with one value lane and $t = 3$ tag lanes, accounts for \est{68\%} of the LAN latency (\cref{sec:eval-scale}), and verified openings roughly double the round count, which dominates on WAN: the insecure lower bound without \CheckOpen{} would cut the WAN latency from \est{89.7~s} to \est{50.5~s} but save only \est{0.03~s} on LAN (\cref{tab:ablation}). Lowering $t$ is not a safe knob: $t = 1$ reaches \est{2.53~s} on LAN but bounds a wrong opening only by $2^{-28}$ for $Q = 2^{32}$ checked batches. Compressed MAC checks that remove tag lanes from the GPU are promising, but they lie outside our proofs.

\textbf{Physical and microarchitectural attacks.}
Probing~\cite{skorobogatov2017microprobing}, optical and other fault injection~\cite{skorobogatov2003optical,quadir2016survey}, and power or electromagnetic analysis~\cite{kocher1999differential} are outside \cref{thm:main} and can extract keys from an unhardened module. Faults matter more in the malicious setting: the bound $Q(2/p)^t$ presumes a correct check engine, so one glitch that forces acceptance bypasses it, and a fault in the field unit array can yield a wrong triple that carries valid tags. Since software-controlled undervolting has induced such faults inside SGX enclaves~\cite{murdock2020plundervolt}, an on-die module must be isolated from host-controlled voltage and frequency scaling or detect glitches, which we have not evaluated. Conversely, the module has no out-of-order core, no shared cache hierarchy and no host-managed page tables, so the controlled-channel, cache, transient-execution and Rowhammer attacks studied on general-purpose TEEs~\cite{xu2015controlled,shinde2015preventing,gotzfried2017cache,brasser2017software,lee2017inferring,van2018foreshadow,kim2014flipping} target mechanisms it lacks, and each check returns one generic status only after all $t$ lanes are aggregated. Small security chips have still shipped with exploitable flaws~\cite{moghimi2020tpm,han2018bad,butterworth2013bios}: a small TCB makes hardening tractable, but it does not replace hardening.

\textbf{Rollback and lifecycle.}
Ledger and epoch state live in volatile protected SRAM. After a reset, \sys requires either a separately justified trusted monotonic service~\cite{tpm2spec,parno2011memoir,matetic2017rote} or the irrecoverable erasure of the old master key followed by a freshly attested session; a host-controlled counter file is not anti-rollback protection, and resetting the release guard is not a secure session reset. Because every failure poisons its epoch and aborted reservations never return to a free list (\cref{fig:ledger}), recovery always costs a new setup. Neither lifecycle option is implemented yet (\cref{tab:obligations}).

\textbf{Availability and fairness.}
\sys provides security with abort, the standard target for two-party computation with a malicious participant~\cite{hazay2010efficient,lindell2017simulate}. A corrupt host can withhold or reorder traffic, stall its GPU or abort at any public interaction boundary, and a corrupt recipient may obtain its output first; fairness and guaranteed output delivery are not claimed (S10 in \cref{tab:scenarios}). Aborts are, however, not a side channel on honest inputs. Apart from the manifest's validity predicates, whose outcomes are permitted leakage (\cref{def:leakage}), every \CheckOpen{} outcome depends only on the adversary's own deviation $(e, d_j)$, the protected keys and the fresh challenges (\cref{thm:mac-sound}), and the first failure ends the epoch, so selective-failure and key-learning strategies cannot be iterated (\cref{lem:hidden-key}). Persistent denial of service remains a matter of deployment policy.

\textbf{Field versus ring.}
Over $\Fp$ with $p = 2^{61}-1$, \sys is not bit-identical to the $\Z_{2^{64}}$ arithmetic of Sigma and Orca~\cite{gupta2023sigma,jawalkar2024orca}. Ring-compiled models must be re-encoded under the numeric contract of \cref{sec:arch-field}, with magnitudes below $p/2$ before truncation, and exact signed truncation relies on canonical bit decompositions of $2n = 122$ authenticated multiplications along a sequential carry chain (\cref{alg:bitdec,alg:trunc}), the most round-intensive gates in \cref{tab:gates}. The field is required by the proof: \cref{thm:mac-sound} divides by a nonzero value error, whereas over $\Z_{2^{64}}$ the error $e = 2^{63}$ is annihilated by every even key, so a wrong value can carry a consistent tag (\cref{app:proof-auth}). A ring deployment therefore needs a SPDZ2k-style backend~\cite{cramer2018spdz2k} over the larger ring $\Z_{2^{k+s}}$, which is a separate design with a separate proof.

\textbf{\ProfU.}
If the accelerator itself is untrusted, \sys switches backends rather than weakening its claim. Under \ProfU (\cref{sec:threat-profileu}) the hardware receives neither the joint-sampler key nor any MAC key, the circuit runs through an established malicious two-party backend such as MASCOT or SPDZ2k in MP-SPDZ~\cite{keller2016mascot,cramer2018spdz2k,keller2020mpspdz}, and the accelerator touches only party-local data, for instance DPF keys exported by the backend. This forfeits the local-dealer and generate-and-consume savings, and an exported-key variant must add the backend's DPF key-privacy assumption, key validation in the style of vFSS~\cite{decastro2022vfss} and an answer-integrity argument outside \cref{thm:main}. \ProfU starts a fresh session with fresh inputs and masks; it is not a fallback that could undo an earlier module compromise. We specify it but do not evaluate it.

\textbf{Model provenance.}
\sys proves correct evaluation on the inputs actually supplied, not that they are the intended ones. A public architecture hash does not authenticate private weights, so a corrupt model owner may substitute any weights that satisfy the input interface (S9 in \cref{tab:scenarios}), exactly as $\FC$ permits. Binding a pre-approved model requires a commitment to the canonical quantized weight bytes, authorized by the client or an independent model authority, which the protected input loader checks by hashing exactly those bytes before sharing them. This establishes provenance, not quality, and the gap between the finite-field circuit and a floating-point model is an approximation question separate from cryptographic correctness.

\textbf{Artifact status.}
Of the five completion gates in our plan, G0 (specification) and G1 (functional model) are reached: the CPU reference of the ideal-module protocol passes its 22 unit tests with 0 failures, including 21,840 exhaustive DPF cases and 20,004 checks of the GPU Mersenne multiplication formula (\cref{sec:eval-attack}). G2 (bit-exact GPU and RTL conformance), G3 (protected runtime) and G4 (deployment and claims) are open: the CUDA micro-test has not been compiled or run, the RTL release guard has not been simulated or synthesized, and the reference uses SHAKE expansion instead of the pinned AES PRG. Hence every \sys latency, energy, throughput and area value in this paper is a model estimate printed in red (\cref{app:model}), to be replaced by the three separate experiments of \cref{sec:arch-deploy}; security measurements additionally require two independent protected devices. No forgery rate will be inferred from zero observed failures, since the statistical bound comes from \cref{thm:mac-sound}, and a machine-checked proof remains future work (\cref{tab:obligations}).


==> qa/draft1/sections/10_related.tex <==
% ==================================================================
% Section X: Related Work
% Owner labels: sec:related, tab:related
% ==================================================================
\section{Related Work}
\label{sec:related}

\begin{table*}[t]
\centering
\caption{Comparison of \sys with Representative Related Work}
\label{tab:related}
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{l c c c l c c l}
\hline
\textbf{Work} & \textbf{Adversary} & \textbf{Trusted HW} & \textbf{Custom HW} & \textbf{Offline material} & \makecell{\textbf{Auth.\ FSS}\\\textbf{outputs}} & \makecell{\textbf{Verified}\\\textbf{openings}} & \textbf{Workloads} \\
\hline
Sigma~\cite{gupta2023sigma} & SH & \xmark & \xmark$^{\mathrm{g}}$ & Dealer keys & \xmark & \xmark & Inference \\
Orca~\cite{jawalkar2024orca} & SH & \xmark & \xmark$^{\mathrm{g}}$ & Dealer keys & \xmark & \xmark & Training, inference \\
Shark~\cite{gupta2025shark} & Mal & \xmark & \xmark & Dealer, authenticated keys & \cmark & \cmark & Inference \\
\hline
MASCOT, MP-SPDZ~\cite{keller2016mascot,keller2020mpspdz} & Mal & \xmark & \xmark & Interactive (OT-based) & n/a & \cmark & General circuits \\
vFSS~\cite{decastro2022vfss} & Mal$^{\mathrm{a}}$ & \xmark & \xmark & Client keys, verified & \xmark & n/a & Key validation \\
APIR~\cite{colombo2023apir} & Mal$^{\mathrm{b}}$ & \xmark & \xmark & None (client query) & n/a & \cmark$^{\mathrm{b}}$ & PIR \\
\hline
Slalom~\cite{tramer2018slalom} & Mal$^{\mathrm{c}}$ & \cmark & \xmark$^{\mathrm{g}}$ & n/a & n/a & \cmark$^{\mathrm{c}}$ & Inference \\
Aramis~\cite{kumar2020cryptflow} & Mal & \cmark$^{\mathrm{d}}$ & \xmark & n/a & n/a & n/a & Inference \\
STAMP, PPMLAC~\cite{huang2022efficient,zhou2022ppmlac} & SH, Mal$^{\mathrm{e}}$ & \cmark & \cmark & In trusted HW & n/a & \pmark$^{\mathrm{e}}$ & ML \\
\hline
GPU-DPF~\cite{lam2023gpu} & SH & \xmark & \xmark$^{\mathrm{g}}$ & None (client query) & \xmark & \xmark & PIR \\
DFA~\cite{dfa2026trusted} & SH & \pmark$^{\mathrm{f}}$ & \cmark & Dealer or local$^{\mathrm{f}}$ & \xmark & \xmark & Inference, PIR \\
\hline
\textbf{\sys (this work)} & Mal$^{\mathrm{h}}$ & \cmark & \cmark & Local, none shipped & \cmark & \cmark & Inference, PIR \\
\hline
\end{tabular}

\vspace{3pt}
\begin{minipage}{0.98\textwidth}
\footnotesize
SH: semi-honest; Mal: malicious (active) adversary. \emph{Trusted HW}: security relies on trusted hardware. \emph{Custom HW}: the work proposes dedicated hardware beyond commodity CPUs and GPUs. \emph{Offline material}: source of the per-query correlated randomness or keys. \emph{Auth.\ FSS outputs}: FSS gate outputs carry MAC tags. \emph{Verified openings}: opened values or untrusted results are checked before use. \cmark: yes; \xmark: no; \pmark: partial, optional or configuration dependent; n/a: not applicable. Entries summarize the headline setting of each work; the lettered notes give the qualifications.
$^{\mathrm{a}}$\,Malicious key generator (client); servers verify that keys are well formed, not that they are evaluated correctly.
$^{\mathrm{b}}$\,The client detects answers that are inconsistent with a public database digest.
$^{\mathrm{c}}$\,Single-server outsourcing from an SGX enclave; the co-located GPU is untrusted and its matrix products are checked with Freivalds' algorithm.
$^{\mathrm{d}}$\,Relies on the integrity, not the confidentiality, of SGX to compile semi-honest protocols into maliciously secure ones.
$^{\mathrm{e}}$\,The adversary model and number of parties differ between the two works; STAMP reports both semi-honest and honest-majority malicious settings.
$^{\mathrm{f}}$\,Trusted mode only; the untrusted mode ships dealer keys.
$^{\mathrm{g}}$\,Implemented on commodity GPUs.
$^{\mathrm{h}}$\,Static corruption of one host, security with abort, under \ProfT; \ProfU delegates to an established malicious backend.
\end{minipage}
\end{table*}

\Cref{tab:related} positions \sys against the closest lines of work, grouped by what they contribute.

\textbf{FSS-based secure computation.}
FSS~\cite{boyle2015fss} and its tree-based DPF instantiations~\cite{gilboa2014distributed,boyle2016function} underlie a family of low-round two-party protocols. AriaNN~\cite{ryffel2020ariann} and Pika~\cite{wagh2022pika} first demonstrated private inference with FSS, the mixed-mode framework of Boyle et al.~\cite{boyle2021function} built comparisons, splines and fixed-point truncation from DCFs, Grotto~\cite{storrier2023grotto} replaced DCF-heavy constructions with DPF-based ones in a $(2{+}1)$-party setting, Orca~\cite{jawalkar2024orca} brought FSS-based training and inference to GPUs, and Sigma~\cite{gupta2023sigma} scaled GPU-based FSS inference to GPT-class transformers. These systems are semi-honest and assume a dealer whose key material dominates the offline cost~\cite{huang2026beyond}. DPFs also underlie PIR, anonymous messaging, private queries and analytics, private heavy hitters, set intersection and distributed ORAM~\cite{corrigan2015riposte,wang2017splinter,dauterman2020dory,dauterman2022waldo,boneh2021lightweight,mouris2024plasma,garimella2024computation,vadapalli2023duoram,doerner2017scaling,ji2023multi}. Secure inference without FSS realizes nonlinear layers through share conversions, garbled circuits or homomorphic encryption~\cite{mohassel2017secureml,mohassel2018aby3,wagh2019securenn,wagh2020falcon,rathee2020cryptflow2,pang2024bolt,lu2023bumblebee}, typically with more interaction per layer. DFA~\cite{dfa2026trusted} accelerated the DPF core of inference and PIR and removed key movement with a trusted local dealer, but it inherited the semi-honest model; \sys keeps its dataflow and upgrades its adversary model.

\textbf{Malicious and verifiable FSS.}
To our knowledge, Shark~\cite{gupta2025shark} is the most directly comparable system: actively secure two-party FSS inference in which a trusted dealer supplies authenticated key material. Its security is cryptographic once the dealer is trusted, whereas \sys trusts one protected module per party; in exchange, \sys generates the authenticated correlations locally and removes the offline shipping on which our dealer-based baseline, modeled after Shark's protocol family, spends \est{37.6~GB} per BERT-Base query (\cref{tab:e2e}). Verifiable FSS addresses a different adversary, a client that may submit malformed keys, which servers detect in the audit of Riposte~\cite{corrigan2015riposte}, the verification protocols of Boyle et al.~\cite{boyle2016function} and Poplar~\cite{boneh2021lightweight}, and the lightweight vFSS of de Castro and Polychroniadou~\cite{decastro2022vfss}. A well-formed key, however, does not force a malicious evaluator to return its correct evaluation, and a valid MAC does not repair an incorrectly generated triple. \sys therefore treats key generation, evaluation, authentication and release as separate obligations.

\textbf{Malicious MPC preprocessing and MACs.}
Dishonest-majority protocols in the SPDZ line~\cite{damgard2012spdz,damgard2013practical} authenticate every shared value with information-theoretic MACs under a global key and consume Beaver triples~\cite{beaver1991efficient} from a costly preprocessing phase: OT-based in MASCOT~\cite{keller2016mascot}, based on somewhat homomorphic encryption in Overdrive~\cite{keller2018overdrive}, and over $\Z_{2^k}$ in SPDZ2k~\cite{cramer2018spdz2k}, all available in MP-SPDZ~\cite{keller2020mpspdz}. Mixed-circuit preprocessing with edaBits~\cite{escudero2020edabits} and classical bit-decomposition and truncation protocols~\cite{damgard2006unconditionally,catrina2010improved} supply the conversions that nonlinear layers need, and pseudorandom correlation generators with silent OT~\cite{boyle2019pcg,boyle2020pcg} reduce the communication of correlation generation. Honest-majority protocols~\cite{furukawa2017high,mohassel2018aby3,wagh2020falcon,dalskov2021fantastic} obtain malicious security from replicated sharing among three or four servers instead. \sys adopts the SPDZ MAC algebra with $t$ independent keys over a Mersenne field and does not claim that algebra as new. It replaces interactive preprocessing by correct generation inside the modules, in the spirit of hardware-assisted correlation generation~\cite{lu2021correlated,zhou2022ppmlac}, and adds the freeze-before-challenge discipline that a hardware check engine needs when a malicious host controls its DMA buffers.

\textbf{Trusted hardware for MPC and ML.}
Tamper-proof tokens are a classical setup assumption for universally composable computation~\cite{katz2007universally}, and commodity TEEs~\cite{costan2016intel,amd_sev,arm_trustzone,lee2020keystone} have been used to accelerate or simplify two-party computation and functional encryption~\cite{gupta2016using,choi2019hybrid,felsen2019secure,wuhybrid,fisch2017iron}. For ML, Ohrimenko et al.~\cite{ohrimenko2016oblivious} and Chiron~\cite{hunt2018chiron} execute learning tasks inside SGX enclaves; Slalom~\cite{tramer2018slalom} outsources linear layers from an enclave to an untrusted GPU and verifies them with Freivalds' algorithm~\cite{freivalds1977probabilistic}; and Aramis~\cite{kumar2020cryptflow} compiles semi-honest protocols into maliciously secure ones by relying on the integrity, but not the confidentiality, of SGX. GPU TEEs~\cite{volos2018graviton,jang2019heterogeneous} and confidential computing on H100~\cite{nvidia_h100_overview,dhanuskodi2023confidential} protect GPU computation from the host but place the whole GPU and its firmware inside the TCB, a boundary far larger than the module we assume. Closest to our trust model, STAMP~\cite{huang2022efficient} and PPMLAC~\cite{zhou2022ppmlac} rely on a small security processor or a trusted chipset to execute nonlinear operations or generate correlated randomness, in the tradition of TPM-class security chips, secure coprocessors and smart cards~\cite{tpm2spec,googletitan,ibm4758,rankl2004smart}, and DFA~\cite{dfa2026trusted} uses a small module as a local FSS dealer. \sys shares their small-TCB premise and, like Slalom, keeps the GPU outside the boundary; unlike Slalom, it checks the GPU's work through MACs on every opening and reserves Freivalds checks for matrix operands that the GPU may already see (\cref{sec:proto-freivalds}).

\textbf{Hardware acceleration for private computation.}
GPU systems accelerate secret-sharing MPC~\cite{tan2021cryptgpu,watson2022piranha,crypten2020}, FSS~\cite{gupta2023sigma,jawalkar2024orca} and DPF-based PIR~\cite{lam2023gpu}. FPGA designs target secret-sharing MPC~\cite{wolfe2020secret,patel2020arithmetic,xu2025co}, Ironman~\cite{ironman2025} accelerates OT extension near memory, and FPGA and ASIC accelerators for homomorphic encryption~\cite{riazi2020heax,reagen2021cheetah,samardzic2021f1,samardzic2022craterlake,kim2022bts} speed up its dominant polynomial kernels. These accelerators make a fixed protocol faster and inherit its adversary model. DFA~\cite{dfa2026trusted} additionally used trust to change the dataflow; \sys uses the same small trusted module to change the adversary model, which is why \cref{sec:eval} compares against security-matched baselines rather than raw kernel throughput alone.

\textbf{PIR with integrity.}
Multi-server PIR~\cite{chor1998private}, including its DPF-based two-server form~\cite{gilboa2014distributed,boyle2016function}, and single-server schemes~\cite{angel2018pir,henzinger2023one} protect the client's index but do not guarantee that a malicious server returns the correct record. Authenticated PIR~\cite{colombo2023apir} lets a client detect answers that are inconsistent with a public database digest without trusted hardware, at the price of additional server work that our APIR-based GPU baseline reflects (\cref{tab:pir}). The versioned-snapshot PIR of \sys instead binds the modules' scan of the exact consumed bytes to an authorized commitment, optionally a Merkle root~\cite{merkle1987digital}, and releases freshly reshared answers only after the snapshot hash matches (\cref{sec:proto-pir}). Its guarantee is conditioned on module trust, and it is not symmetric PIR.

\textbf{Positioning.}
Each ingredient of \sys has precedents: information-theoretic MACs, trusted correlation generation, verification of untrusted GPU work and DPF acceleration. Among the systems in \cref{tab:related}, \sys is the only one that is malicious-secure, ships no per-query offline material, authenticates FSS outputs and verifies openings, and serves both private inference and DPF-based PIR. Our contribution is this composition, realized in one small trusted module and proven in the ideal-module model of \cref{sec:threat-model}, not any single primitive.


==> qa/draft1/sections/11_conclusion.tex <==
% ==================================================================
% Section XI: Conclusion (owner: sections/11_conclusion.tex)
% Labels defined here: sec:conclusion
% ==================================================================
\section{Conclusion}\label{sec:conclusion}

We presented \sys, a trusted hardware accelerator that makes FSS-based private inference and DPF-based PIR secure against a malicious host and GPU while keeping the key-movement savings of trusted DFA. The design starts from one observation: a small module that already plays the FSS dealer can also be the verifier. \sys therefore generates authenticated correlations inside its protected boundary, authenticates its own DPF outputs with a fresh resharing epilogue instead of extra DPF trees, checks every opening on frozen bytes with $t=3$ independent MAC lanes over $\F_{2^{61}-1}$, and releases nothing before a role-bound one-time ledger records a verified check. Together these mechanisms protect the chain from authorized input to authorized output release, and we prove static malicious security with abort in an explicit protected-module model, with a statistical term of about $2^{-148}$ for $2^{32}$ checked batches. Our model estimates that \sys is \est{10.1--14.0$\times$} faster on a LAN than dealer-based malicious FSS, removes \est{21.8--563~GB} of offline authenticated material per query, costs \est{2.5--3.5$\times$} LAN latency over semi-honest trusted DFA, keeps \est{93\%} of its PIR throughput, and adds \est{0.145~mm$^2$} at 7~nm. The evaluation also shows that, once DPF authentication is cheap, the remaining cost of malicious security lies in authenticated linear algebra and in the extra rounds of checked openings.

Three directions follow. First, the red estimates must be replaced by measurements: bit-exact GPU and RTL conformance, a protected runtime on two independent devices, and on-die simulation of the complete datapath. Second, a \ProfU backend would extend the same datapath to deployments in which the hardware itself is adversarial, and a SPDZ2k-style backend would cover the ring $\Z_{2^{64}}$. Third, compressed MAC checks that avoid carrying all tag lanes through the GPU, and a vetted DCF that is faster than our conservative $O(n^2)$ construction, could remove the dominant remaining costs; both require proofs that this paper does not provide.

\section*{Acknowledgment}
Acknowledgments are omitted for anonymous review and will be added in the final version.


==> qa/draft2/macros.tex <==
% ------------------------------------------------------------------
% Shared packages and macros for the TIFS manuscript.
% Every section/appendix/algorithm/table file relies ONLY on these.
% ------------------------------------------------------------------
\usepackage[T1]{fontenc}
\usepackage{amsmath,amssymb,amsfonts,mathtools}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{graphicx}
\usepackage[dvipsnames,table]{xcolor}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{array}
\usepackage{tabularx}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{setspace}
\let\labelindent\relax
\usepackage[inline]{enumitem}
\usepackage{pifont}
\usepackage{xspace}
\usepackage{stmaryrd}
\usepackage{cite}
\usepackage[hidelinks]{hyperref}
\usepackage[capitalise,noabbrev]{cleveref}

% ---------------- cross-reference names (IEEE style) ----------------
\crefname{section}{Section}{Sections}
\Crefname{section}{Section}{Sections}
\crefname{subsection}{Section}{Sections}
\Crefname{subsection}{Section}{Sections}
\crefname{subsubsection}{Section}{Sections}
\Crefname{subsubsection}{Section}{Sections}
\crefname{appendix}{Appendix}{Appendices}
\Crefname{appendix}{Appendix}{Appendices}
\crefname{figure}{Fig.}{Figs.}
\Crefname{figure}{Fig.}{Figs.}
\crefname{table}{Table}{Tables}
\Crefname{table}{Table}{Tables}
\crefname{algorithm}{Algorithm}{Algorithms}
\Crefname{algorithm}{Algorithm}{Algorithms}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Eq.}{Eqs.}
\crefname{ALC@unique}{line}{lines}
\crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{remark}{Remark}{Remarks}
\crefname{proposition}{Proposition}{Propositions}

% ---------------- theorem environments ----------------
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\theoremstyle{remark}
\newtheorem{remark}{Remark}

% ---------------- algorithm style (FuseFSS / DFA hybrid) ----------------
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) \textit{#1}}
\algnewcommand{\Abort}{\textbf{abort}}
\newcommand{\algstretch}{\setstretch{0.92}}

% ---------------- estimates: RED, to be replaced by measured values ----------------
\newcommand{\est}[1]{\textcolor{red}{#1}}

% ---------------- names ----------------
\newcommand{\sys}{VIGOR-DFA\xspace}
\newcommand{\DFA}{DFA\xspace}
\newcommand{\ProfT}{Profile~$\mathsf{T}$\xspace}
\newcommand{\ProfU}{Profile~$\mathsf{U}$\xspace}

% ---------------- algebra ----------------
\newcommand{\F}{\mathbb{F}}
\newcommand{\Fp}{\mathbb{F}_p}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\bits}[1]{\{0,1\}^{#1}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\getsr}{\xleftarrow{\$}}
\newcommand{\inner}[2]{\langle #1, #2\rangle}
\newcommand{\auth}[1]{[#1]}                  % authenticated sharing
\newcommand{\authb}[2]{[#1]_{#2}}            % party-b tuple (x_b, gamma_{b,1..t})
\newcommand{\tagv}[3]{\gamma_{#1,#2}^{(#3)}} % optional explicit tag notation

% ---------------- FSS objects ----------------
\newcommand{\Gen}{\mathsf{Gen}}
\newcommand{\Eval}{\mathsf{Eval}}
\newcommand{\EvalAll}{\mathsf{EvalAll}}
\newcommand{\DPF}{\mathsf{DPF}}
\newcommand{\DCF}{\mathsf{DCF}}
\newcommand{\CW}{\mathsf{CW}}
\newcommand{\CWout}{\mathsf{CW}^{\mathrm{out}}}
\newcommand{\sCW}{s^{\mathsf{CW}}}
\newcommand{\tCW}[1]{t^{\mathsf{CW},#1}}
\newcommand{\PRG}{G}
\newcommand{\Conv}{H}
\newcommand{\keep}{\mathit{keep}}
\newcommand{\lose}{\mathit{lose}}

% ---------------- crypto ----------------
\newcommand{\PRF}{\mathsf{PRF}}
\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\Hash}{\mathsf{Hash}}
\newcommand{\AEAD}{\mathsf{AEAD}}
\newcommand{\Adv}{\mathcal{A}}
\newcommand{\Sim}{\mathcal{S}}
\newcommand{\Env}{\mathcal{Z}}
\newcommand{\View}{\mathsf{View}}
\newcommand{\Real}{\mathsf{Real}}
\newcommand{\Ideal}{\mathsf{Ideal}}
\newcommand{\Hyb}[1]{\mathsf{H}_{#1}}
\newcommand{\Leak}{\mathcal{L}}
\newcommand{\FC}{\mathcal{F}^{\mathrm{abort}}_{C,\mu}}
\newcommand{\FPIR}{\mathcal{F}^{\mathrm{abort}}_{\mathrm{PIR}}}
\newcommand{\eps}[1]{\epsilon_{\mathsf{#1}}}
\newcommand{\negl}{\mathsf{negl}}

% ---------------- protocol / ledger / commands ----------------
\newcommand{\cmd}[1]{\texttt{\detokenize{#1}}}
\newcommand{\lstate}[1]{\textsf{#1}}
\newcommand{\algname}[1]{\textsf{#1}}
\newcommand{\CheckOpen}{\algname{CheckOpen}\xspace}
\newcommand{\AuthShare}{\algname{AuthShare}\xspace}
\newcommand{\Epilogue}{\algname{Epilogue}\xspace}

% ---------------- marks for tables ----------------
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\pmark}{\ding{109}}   % partial


==> qa/draft2/sections/00_abstract.tex <==
% ==================================================================
% Abstract and index terms (owner: sections/00_abstract.tex)
% Red values are model estimates (\est{}); see Appendix F.
% ==================================================================
\begin{abstract}
Function secret sharing (FSS) underlies two-party private inference and private information retrieval, with cost dominated by generating, moving and evaluating distributed point function (DPF) keys. A trusted GPU-integrated distributed function accelerator (DFA) removed key movement by generating and consuming keys locally, but tolerates only semi-honest adversaries. A malicious host or GPU can tamper with shares, replay one-time material, swap buffers after checking, request early outputs, or abuse the accelerator as a forgery oracle, while malicious FSS ships large authenticated keys or multiplies DPF work. We present \sys, protecting the chain from authorized input to authorized output release with three mechanisms: a fresh authentication epilogue using three field multiplications per DPF output, \est{3.8--4.0$\times$} faster per gate than per-lane DPF tag trees; a freeze-before-challenge check of every opening with $t=3$ independent MAC lanes over $\F_{2^{61}-1}$; and a role-bound one-time resource ledger with a release guard, in a protected datapath beside the GPU L2 cache. We prove stand-alone static malicious security with abort in a protected-module model, with statistical error $Q(2/p)^t\approx 2^{-148}$ for $Q\le 2^{32}$ checked batches. Our DFA-calibrated model estimates that, against dealer-based malicious FSS modeled after the protocol family of Shark, \sys removes \est{21.8--563~GB} of per-query offline authenticated material and, mainly by generating it in-module, lowers LAN latency by \est{10.1--14.0$\times$} (\est{1.5--1.8$\times$} excluding offline distribution) and energy by \est{3.0--3.9$\times$}. Malicious security costs \est{2.5--3.5$\times$} LAN latency over semi-honest DFA and \est{0.145~mm$^2$} at 7~nm. We executed a specification and a functional CPU reference model; GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet.
\end{abstract}

\begin{IEEEkeywords}
Distributed point function, function secret sharing, hardware accelerator, malicious security, private information retrieval, secure inference, trusted hardware.
\end{IEEEkeywords}


==> qa/draft2/sections/01_introduction.tex <==
% ==================================================================
% Section I: Introduction (owner: sections/01_introduction.tex)
% Labels defined here: sec:intro
% Red (\est{}): model outputs, assumed parameters. Black: cited DFA
% values, design constants, analytical counts, executed tests.
% ==================================================================
\section{Introduction}\label{sec:intro}

\IEEEPARstart{P}{rivacy}-preserving computation is moving into deployments where data are both valuable and regulated: hospitals running diagnostic models on records they may not export, cloud providers serving proprietary models to clients who will not reveal their queries, and lookup services whose queries disclose a user's interests. Secure two-party computation (2PC) for private machine-learning (ML) inference~\cite{yao1986generate,goldreich2019play,mohassel2017secureml,rathee2020cryptflow2} and private information retrieval (PIR)~\cite{chor1998private,angel2018pir} address these settings with cryptographic rather than contractual guarantees. Function secret sharing (FSS)~\cite{boyle2015fss,boyle2016function} has become one of the most effective building blocks for both. In FSS-based private inference, the parties open a masked input $x+r$ and evaluate one-time keys for the gate function shifted by the mask, so that a nonlinear layer often costs a single online round~\cite{boyle2021function,gupta2023sigma,jawalkar2024orca}. In two-server PIR, the client splits a point function into two short keys and each server evaluates its key over the entire database~\cite{gilboa2014distributed,wang2017splinter,lam2023gpu}.

The price of this online efficiency is paid in distributed point function (DPF) work. Every comparison, lookup table and interval test in an FSS-compiled model is built from DPFs or from the distributed comparison functions (DCFs) derived from them~\cite{boyle2021function,storrier2023grotto,gupta2023sigma}, and each key is used once. A dealer must therefore generate, ship and store fresh keys for every nonlinear element of every query: 17.1~GB of offline material for a single BERT-Base inference~\cite{dfa2026trusted}, a cost that cannot always be hidden behind the online phase~\cite{huang2026beyond}. PIR, conversely, is dominated by full-domain DPF evaluation, which is AES-bound even on a modern GPU~\cite{lam2023gpu}. The distributed function accelerator (DFA)~\cite{dfa2026trusted} attacked both costs with a small DPF engine integrated next to the GPU L2 cache. In its trusted mode, a protected module in each server attests to its peer, establishes a shared key and plays the dealer locally: it generates its own party's key share on demand and consumes each correction word as soon as it is produced (\emph{generate-and-consume}, GaC), so keys are never distributed, stored or reread. For BERT-Base, trusted DFA reduces LAN latency from 18.8~s to 1.42~s and offline communication from 17.1~GB to 0.1~GB, and it raises PIR throughput by $5.05\times$ for $2^{20}$ records~\cite{dfa2026trusted}.

\textbf{The semi-honest boundary.}
DFA, like Sigma~\cite{gupta2023sigma}, Orca~\cite{jawalkar2024orca} and most GPU-based FSS systems, is secure only against semi-honest adversaries: it assumes that both servers run the prescribed code. In a real deployment, however, the components easiest to subvert are those around the small protected module: the host operating system, the GPU driver and runtime, the GPU kernels, the DMA buffers and the network stack. They hold the whole data path, and attacks on privileged software and firmware~\cite{xu2015controlled,butterworth2013bios,han2018bad} and GPU isolation designs~\cite{volos2018graviton,jang2019heterogeneous} alike treat them as potentially adversarial. With its module intact, a single compromised server host can still mount at least five classes of attacks against semi-honest trusted acceleration (\cref{fig:scenarios}):
(i)~\emph{additive errors} on shares, openings or GPU products, which bias results and leak through selective failure;
(ii)~\emph{replay or reset} of masks, counters or module state;
(iii)~\emph{check-to-use} buffer swaps;
(iv)~abuse of a naive ``authenticate'' command as a \emph{forgery oracle}; and
(v)~\emph{premature} output requests.
Remote attestation does not close these gaps. It proves which code and configuration run inside the module; it does not prove that the untrusted GPU used a valid key, computed the right product, or released an authorized result.

\textbf{Why existing malicious routes are costly.}
FSS can be made maliciously secure, but the known routes give back much of what trusted acceleration gained. Actively secure FSS inference such as Shark~\cite{gupta2025shark} keeps an external dealer that ships authenticated keys and correlated randomness. For dealer-based malicious FSS modeled after the protocol family of Shark (\cref{app:model}), we estimate \est{37.6~GB} of offline material per BERT-Base query, \est{2.2$\times$} the semi-honest 17.1~GB~\cite{dfa2026trusted}, and a LAN latency of \est{43.9~s} of which \est{37.6~s} is distribution. Dealer-free malicious preprocessing in the SPDZ family~\cite{damgard2012spdz,keller2016mascot,keller2018overdrive,cramer2018spdz2k} replaces the dealer by oblivious-transfer (OT) or homomorphic-encryption triple generation, and pseudorandom correlation generators with silent OT~\cite{boyle2019pcg,boyle2020pcg} compress the communication of authenticated triples at a substantial computational cost. Neither yields FSS keys: generating DPF keys without a dealer requires a secure two-party evaluation of key generation with a round per tree level~\cite{doerner2017scaling}, so dealer-free malicious FSS keeps a preprocessing cost far above its online cost. Verifiable FSS~\cite{decastro2022vfss} lets servers check that client-generated DPF keys are well formed, but not that an untrusted GPU evaluates them, or the arithmetic around the gate, correctly. Finally, the direct way to authenticate an FSS output inside an accelerator, one additional DPF tree with payload $\Delta_j\beta$ per message authentication code (MAC) lane, multiplies pseudorandom generator (PRG) work by $1+t$ for $t$ lanes. One tree with a $(1+t)$-element payload avoids most of this cost, but it widens every output correction and exports tag shares whose hiding rests on DPF key privacy.

\textbf{Our key insight} is that a module that already plays the FSS dealer can also be the verifier. Because it knows every correlation it generates, it can (1)~generate \emph{authenticated} correlations (input masks, Beaver triples~\cite{beaver1991efficient} and DPF keys) locally at zero network cost, computing every triple product correctly inside its own boundary; (2)~authenticate its own FSS outputs with a fresh resharing epilogue instead of extra DPF trees, because it already holds the raw output shares and the MAC key material; and (3)~check every opening on bytes it has frozen before any challenge exists, so that the GPU remains a fast but untrusted linear-algebra engine whose results are only candidates until verified. What must be protected is thus not a single primitive but an integrity chain:
\begin{center}
\small
\emph{authorized input} $\rightarrow$ \emph{correlated preprocessing} $\rightarrow$ \emph{correct local evaluation} $\rightarrow$ \emph{authenticated arithmetic} $\rightarrow$ \emph{consistent opening} $\rightarrow$ \emph{authorized output release.}
\end{center}
Each link has a concrete failure mode under a malicious host, and each needs its own mechanism. \Cref{fig:flows} places the resulting execution flow next to the semi-honest GPU baseline, trusted DFA and dealer-based malicious FSS.

\textbf{This work.}
We present \sys (Verified Integrity-Gated On-demand Randomness DFA), the malicious-secure successor of trusted DFA. It keeps DFA's placement beside the GPU L2 cache, its local key generation and its generate-and-consume execution. Under \ProfT (\cref{sec:threat}) a malicious adversary statically corrupts at most one host, and every secret value on a host is an authenticated share over $\Fp$, $p=2^{61}-1$, with $t=3$ SPDZ-style MAC lanes~\cite{damgard2012spdz,damgard2013practical} (32~bytes per element and party). Three mechanisms carry the design; we claim their composition, not any of them as an unprecedented primitive. The \emph{fresh authentication epilogue} turns each raw DPF output share into a freshly padded authenticated tuple at three field multiplications and four pads (\cref{sec:proto-epilogue}). It matches the PRG cost of a single vector-payload tree, makes every exported tuple exactly uniform, and leaves no command that authenticates a host-supplied value. \emph{Freeze-before-challenge} \CheckOpen{} derives independent per-lane challenges only after both modules have frozen the exact submitted bytes, and later consumes exactly those bytes. A \emph{role-bound one-time ledger} labels all randomness by session, epoch, gate and purpose and poisons the epoch on any failure, and its \emph{release guard} lets no output leave a module before the corresponding check is \lstate{VERIFIED}.

\textbf{Scope and limits.}
\sys relocates trust to the modules rather than removing it. The modules see inputs under \ProfT, and both learn the PIR index, so PIR query privacy in \sys rests on module trust, unlike untrusted two-server DPF-PIR~\cite{lam2023gpu} and DFA's untrusted mode, which hide the index without trusted hardware. Physical attacks, leakage beyond the stipulated observable-trace model and rollback without a trusted monotonic service are out of scope, and security holds with abort, without fairness (\cref{sec:discussion}). Once the epilogue removes tag trees, the dominant cost of malicious security moves to four-lane authenticated linear algebra on the GPU and to the doubled round count (\cref{sec:analysis}).

\textbf{Why keep FSS inside a trusted module?}
Under \ProfT a module that has verified $c=x+r$ also holds $r$, so FSS adds no formal confidentiality over evaluating the gate directly (\cref{sec:proto-direct}). The end-to-end gains of \sys come from generating and consuming authenticated correlations inside the modules, not from FSS evaluation: in our model direct-only compilation (\est{3.82~s} for BERT-Base) is marginally faster than the compiler-selected default (\est{3.83~s}), which keeps an FSS realization for gate shapes marked FSS-portable, and nonlinear gates take only \est{3.4\%} of the latency. We keep a malicious FSS datapath for three reasons: the same compiled circuit, including masked-input FSS gates from existing toolchains~\cite{gupta2023sigma,jawalkar2024orca}, runs under the key-exporting \ProfU (specified, not evaluated or proven); PIR and small lookup tables are full-domain, data-independent scans that match the pipelined AES engines; and long-lived evaluation state holds only seeds and correction words, keeping input-dependent state short-lived as defense in depth, not as a formal claim. On FSS gates the epilogue is \est{3.8--4.0$\times$} faster than per-lane tag trees, although tag trees would raise the BERT-Base LAN latency by only \est{8\%}.

This paper makes the following contributions:
\begin{itemize}[leftmargin=*]
    \item \textbf{Malicious Threat Analysis.}
    We systematize how a malicious host or GPU attacks semi-honest trusted FSS acceleration into ten scenarios, S1 to S10 (\cref{fig:scenarios,tab:scenarios}), from share tampering to PIR snapshot substitution. For S1 to S8 we show why semi-honest trusted DFA fails and which \sys mechanism and theorem stop it; for S9 (input substitution) and S10 (denial of service and selective abort) we make explicit what the ideal functionality permits or does not prevent.

    \item \textbf{Protocol Co-Design.}
    We specify the three mechanisms above, the authenticated $\Fp$ representation and malicious generate-and-consume with explicit generator and evaluator states (\cref{sec:protocol}). On top of them we build authenticated lookup-table, interval, polynomial and direct protected gates, exact comparison and truncation, a refactoring rule that preserves the joint (not only the marginal) distribution of DFA's decoupled preprocessing, and versioned-snapshot PIR whose query privacy rests on module trust.

    \item \textbf{Hardware Architecture.}
    We design a protected datapath beside the GPU L2 cache (\cref{sec:arch}) with a ledger, page freezer, joint pseudorandom-function (PRF) sampler, DPF generation and evaluation contexts, a 128-lane Mersenne-61 field unit array, a check engine, a peer-channel controller and a release guard, whose 64 AES engines are time-shared among PRG expansion, challenge derivation and authenticated-encryption (AEAD) freezing. The additions cost \est{0.145~mm$^2$} and \est{0.508~W} at 7~nm, and the entire \sys occupies \est{0.046\%} of the A100 die.

    \item \textbf{Security Analysis.}
    We give ideal functionalities with explicit leakage and a hybrid proof with an explicit simulator of stand-alone static malicious security with abort under sequential composition (\cref{sec:security}, \cref{thm:main}), with advantage at most $\eps{setup}+\eps{prf}+\eps{channel}+\eps{bind}+\eps{trace}+Q(2/p)^t$, where the last term is about $2^{-148}$ for $Q\le 2^{32}$ checked batches. We show why shared challenges across lanes and the ring $\Z_{2^{64}}$ break this bound, and we separate what is proved from the implementation obligations that remain (\cref{tab:obligations}).

    \item \textbf{Evaluation.}
    With an analytical model calibrated on DFA (\cref{sec:eval}, \cref{tab:e2e}), we estimate that in-module generation of authenticated correlations cuts offline communication from \est{37.6~GB} to \est{under 1~MB} per BERT-Base query. Against dealer-based malicious FSS modeled after the protocol family of Shark, \sys is \est{11.4$\times$} faster on a LAN, or \est{1.6$\times$} excluding per-query offline distribution; with no authenticated-key blow-up the dealer-based pipeline still needs \est{22.4~s}, \est{5.8$\times$} that of \sys. Malicious security costs \est{2.7$\times$} LAN latency over semi-honest trusted DFA for BERT-Base, mostly for four-lane linear algebra, yet \sys stays \est{4.3--6.1$\times$} faster than the semi-honest GPU-only pipeline across four models. We executed a specification and a functional CPU reference model, which covers every algorithm except the optional Freivalds check and passes all 22 unit tests (\cref{sec:eval-attack}); GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet, and five injections of \cref{tab:attacks}, including the release guard, lack executed evidence.
\end{itemize}

Throughout, red values are outputs or assumed parameters of our analytical model (\cref{app:model}) that await measurement; black values are reproduced from DFA~\cite{dfa2026trusted}, are design constants or analytical counts, or come from executed reference tests.

\Cref{sec:bg,sec:threat,sec:analysis} give background, the threat model and where the cost of malicious FSS goes; \cref{sec:protocol,sec:arch,sec:security,sec:eval} present the protocol, architecture, security analysis and evaluation; \cref{sec:discussion,sec:related,sec:conclusion} discuss limitations, related work and conclusions, and the appendices give the ideal functionalities, proofs and performance model.


==> qa/draft2/sections/02_background.tex <==
% ==================================================================
% Section II: Background
% Owner labels: sec:bg, sec:bg-fss, sec:bg-pi, sec:bg-pir, sec:bg-dfa,
%               sec:bg-mal, fig:flows, eq:dpf, eq:pir
% ==================================================================
\section{Background}
\label{sec:bg}

This section reviews the primitives that \sys builds on and the semi-honest DFA design~\cite{dfa2026trusted} that it extends.
We write $P_0,P_1$ for the two computing parties, $b\in\{0,1\}$ for a party index, $\lambda$ for the seed length of the pseudorandom generator (PRG), and $\one[\cdot]$ for the indicator of a predicate.

% ==================================================================
\subsection{Function Secret Sharing, DPF, and DCF}
\label{sec:bg-fss}

\textbf{Function secret sharing.}
A two-party function secret sharing (FSS) scheme~\cite{boyle2015fss,boyle2016function} for a function class $\mathcal{F}$ with output group $\mathbb{G}$ consists of $\Gen(1^\lambda,\hat f)$, which maps a description of $f\in\mathcal{F}$ to a key pair $(k_0,k_1)$, and $\Eval(k_b,x)$, which returns party $b$'s share $y_b\in\mathbb{G}$.
Correctness requires $\Eval(k_0,x)+\Eval(k_1,x)=f(x)$ for every $x$; security requires that each key alone be simulatable from public information (domain, output group, function class), so that a single key hides $f$.

\textbf{Distributed point function.}
A distributed point function (DPF)~\cite{gilboa2014distributed,boyle2015fss,boyle2016function} shares the point function $f_{\alpha,\beta}$ with target $\alpha\in\bits{n}$ and payload $\beta\in\mathbb{G}$:
\begin{equation}\label{eq:dpf}
\Eval(k_0,x)+\Eval(k_1,x)=\beta\cdot\one[x=\alpha]\quad\text{for all } x\in\bits{n}.
\end{equation}
In this paper $\mathbb{G}=\Fp$ with $p=2^{61}-1$ (\cref{sec:proto-repr}), inputs are read most-significant bit first, and we use the tree-based construction of Boyle et al.~\cite{boyle2016function}.
Each node of a depth-$n$ binary tree carries a state $(s,t)$ of a $\lambda$-bit seed and a control bit; a fixed PRG $\PRG:\bits{\lambda}\rightarrow(\bits{\lambda}\times\bits{})^2$ expands a seed into the states of its two children, and $\Conv:\bits{\lambda}\rightarrow\Fp$ converts a leaf seed into a field element.
Generation walks the target path from two independent root seeds with control bits $t_0=0$ and $t_1=1$; each level's correction word $\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$ makes both parties' states identical on the child leaving the path and keeps them pseudorandom with opposite control bits on the child staying on it, and an output correction $\CWout$ makes the signed outputs $y_b=(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$ sum to $\beta$ at $x=\alpha$ and cancel elsewhere.
Party $b$'s key holds its root seed, its fixed control bit $t_b^{(0)}=b$, the $n$ correction words and $\CWout$, i.e., $O(\lambda n)$ bits; \cref{alg:gen,alg:eval} in \cref{sec:analysis-dpf} give the exact algorithms.

\textbf{Evaluation patterns and cost.}
Generation expands $2n$ states and a single-path $\Eval(k_b,x)$ expands $n$; a full-domain $\EvalAll(k_b)$ expands $2^n-1$ internal nodes, keeping only $O(n)$ pending siblings in a depth-first traversal.
The PRG dominates all patterns; DFA, GPU-DPF~\cite{lam2023gpu} and \sys instantiate it with AES-128.
Two properties matter later.
Keys are \emph{one-time}: each encodes one mask or query index, and reusing a mask reveals the difference of the two inputs it hides.
DPF key privacy holds for \emph{arbitrary} $(\alpha,\beta)$~\cite{boyle2016function}, so uniform targets come from the application's masking (\cref{sec:bg-pi}), whose joint distribution any refactoring of generation must preserve (\cref{sec:proto-refactor}).

\textbf{Distributed comparison function.}
A distributed comparison function (DCF) shares $f^{<}_{\alpha,\beta}(x)=\beta\cdot\one[x<\alpha]$.
We use this ``$<$'' orientation throughout; DFA~\cite{dfa2026trusted} uses ``$>$'', and we convert explicitly at interfaces via $\beta\cdot\one[x>\alpha]=\beta-f^{<}_{\alpha+1,\beta}(x)$, treating the threshold $2^n$ as a public constant.
Optimized DCFs evaluate with $O(n)$ PRG expansions~\cite{boyle2021function}, and DCFs can be assembled from DPFs~\cite{storrier2023grotto}.
\sys uses the conservative $O(n^2)$ DCF of \cref{alg:dcf}, which sums $n$ prefix DPFs and whose correctness \cref{thm:dcf} proves (\cref{app:proof-dpf}).

% ==================================================================
\subsection{FSS-Based Private Inference}
\label{sec:bg-pi}

\textbf{Two-party secure inference.}
Private inference runs a neural network with private input, and possibly private weights, as a secure two-party computation~\cite{yao1986generate,goldreich2019play,mohassel2017secureml,rathee2020cryptflow2,crypten2020,tan2021cryptgpu,watson2022piranha}.
With additive shares $x=x_0+x_1$, linear operations are local, and a multiplication consumes a Beaver triple $(a,b,c=ab)$~\cite{beaver1991efficient}: the parties open $d=x-a$ and $e=y-b$ and locally compute shares of $xy=c+db+ea+de$.
Nonlinear layers (ReLU, GeLU, Softmax, LayerNorm) dominate the cost; earlier systems use multi-round Boolean conversions for them~\cite{demmler2015aby,mohassel2018aby3,wagh2019securenn,wagh2020falcon}.

\textbf{Masked-input FSS gates.}
FSS-based systems~\cite{boyle2019preprocessing,boyle2021function,ryffel2020ariann,wagh2022pika,gupta2023sigma,jawalkar2024orca} evaluate each nonlinear gate $g$ in the masked-input paradigm.
Offline, a dealer samples a fresh uniform mask $r$, shares it, and generates FSS keys for the offset function $g_r(c)=g(c-r)$, often with an output mask.
Online, the parties open $c=x+r$, which is uniform and independent of $x$, and the outputs $\Eval(k_b,c)$ are shares of $g(x)$.
Comparisons and ReLU use DCFs; splines for GeLU, exponentials and inverse square roots use DCF-based interval selection plus low-degree polynomials; and small lookup tables use DPFs~\cite{gupta2023sigma,jawalkar2024orca}.
Each gate costs one opening round, so the online phase is round-efficient but compute-intensive.

\textbf{Offline cost and the dealer assumption.}
The price is paid offline.
Semi-honest FSS inference of BERT-Base with 128 tokens moves 17.1~GB of one-time key material per query and LLaMA2-7B moves 256~GB, more than 90\% of it DPF keys~\cite{dfa2026trusted}; this cost cannot always be hidden behind online work, and its energy and monetary cost is never hidden~\cite{huang2026beyond}.
Sigma, Orca, and related systems~\cite{gupta2023sigma,jawalkar2024orca,crypten2020} obtain keys from a trusted dealer and assume semi-honest computing parties.

% ==================================================================
\subsection{DPF-Based Private Information Retrieval}
\label{sec:bg-pir}

PIR lets a client retrieve record $D[\alpha]$ of an $N$-record database $D$ without revealing $\alpha$~\cite{chor1998private}.
Single-server schemes rely on homomorphic encryption and are computationally heavy~\cite{angel2018pir,henzinger2023one}; we focus on the faster two-server DPF-based schemes~\cite{gilboa2014distributed,boyle2016function}.
With $n=\lceil\log_2 N\rceil$, the client sends $k_b$ of $(k_0,k_1)\leftarrow\Gen(1^\lambda,\alpha,1)$ to server $P_b$, which returns
\begin{equation}\label{eq:pir}
y_b=\sum_{x=0}^{N-1}\Eval(k_b,x)\cdot D[x],\qquad b\in\{0,1\},
\end{equation}
and by \cref{eq:dpf} the client obtains $D[\alpha]=y_0+y_1$.
Keys have $O(\lambda\log N)$ bits, but each query costs $O(N)$ PRG expansions plus an $N$-term inner product per server, and the expansion dominates even on GPUs~\cite{lam2023gpu}.
Standard DPF-based PIR protects the index but not the answer: a malicious server can add an offset $\delta$ to $y_b$, so that the client accepts $D[\alpha]+\delta$, or answer from a stale database.
Conversely, a malicious client can submit a malformed key pair that reconstructs a combination of several records, which verifiable DPFs detect~\cite{decastro2022vfss}.
Authenticated PIR~\cite{colombo2023apir} lets the client verify answers against a database digest at additional server cost.
\Cref{sec:proto-pir} gives our protected versioned-snapshot design, in which both modules learn $\alpha$: unlike untrusted two-server DPF-PIR, its query privacy rests on module trust.

% ==================================================================
\subsection{Trusted DFA}
\label{sec:bg-dfa}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_flows.pdf}
    \caption{Execution flows of two-party FSS-based private inference in four configurations, from left to right.
    (1)~GPU without DFA (semi-honest): a trusted party generates FSS keys offline and ships them over the network; each party stores them, rereads them and transfers them to its GPU.
    (2)~Trusted DFA (semi-honest)~\cite{dfa2026trusted}: after a one-time initialization with attestation and key exchange, each on-die module generates its party's keys locally and merges generation with evaluation (generate-and-consume), removing the offline phase.
    (3)~Dealer-based malicious FSS, modeled after the protocol family of Shark~\cite{gupta2025shark}: the dealer also issues authenticated keys and triples, so about \est{2.2$\times$} as much offline material (red: model estimate, \cref{app:model}) must be shipped, stored and reread, while the GPU runs authenticated GEMM and checks MACs online.
    (4)~\sys (malicious): the protected module (red dashed trusted boundary) keeps local generation and generate-and-consume, adds the fresh authentication epilogue, freeze-before-challenge \CheckOpen{} and the release guard, and exchanges authenticated shares $\authb{x}{b}$ with a GPU that runs authenticated linear algebra on one value lane and three MAC-tag lanes; the inter-party network carries opened values and check residuals, not keys.}
    \label{fig:flows}
\end{figure*}

\textbf{Hardware.}
DFA~\cite{dfa2026trusted} integrates 16 DPF units with four pipelined AES-128 engines each (64 in total) next to the L2 slices of a GPU; each 20-stage unit sustains one Gen or Eval iteration per cycle after warm-up.
An SC300-class control core~\cite{st33tpm12spi,arm_cortex_m3} handles attestation and key management, and a 16-lane vector unit~\cite{cavalcante2019ara} runs protocol-specific pre- and post-processing.
The design runs at 720~MHz in 28~nm, delivers about 290~GB/s of DPF output in Accel-Sim~\cite{khairy2020accel}, and traverses full-domain trees depth-first, needing $O(nm)$ state for $m$ units instead of $O(2^n)$~\cite{dfa2026trusted}.

\textbf{Untrusted and trusted modes.}
In the \emph{untrusted mode}, DFA only expands seeds for keys produced elsewhere, and the protocol is unchanged.
In the \emph{trusted mode}, each party's module replaces the dealer: the modules attest to each other and establish a key $K$ that the hosts never see, derive the same generation coins (including $\alpha$) from $K$ and a counter, and thus compute identical correction words while each evaluates only its own party's share.
\emph{Generate-and-consume} (GaC) runs the joint generation and the local evaluation in lockstep, consuming each correction word as soon as it is produced, so that neither key distribution nor key storage remains.
DFA also \emph{decouples} generation from protocol preprocessing: when the target is $a=g(r)$ for a bijection $g$, the module samples $a$ uniformly and recovers $r=g^{-1}(a)$.

\textbf{Limits of the semi-honest design.}
DFA argues that correct in-module generation leaves the semi-honest protocol unchanged; against a deviating host this argument fails in four places treated later: (i)~decoupled preprocessing must preserve joint, not only marginal, distributions (\cref{sec:proto-refactor}); (ii)~generator and evaluator state is left implicit (\cref{sec:analysis-dpf}); (iii)~attestation authenticates the module configuration, not that the GPU used a valid key, computed the right product or released an authorized result (\cref{sec:threat-scenarios}); and (iv)~the GPU lies outside the trusted computing base (TCB) and must never obtain module tags for its own results (\cref{sec:proto-epilogue}).

% ==================================================================
\subsection{Tools for Malicious Security}
\label{sec:bg-mal}

\textbf{Security with abort.}
We use the stand-alone real/ideal simulation paradigm, which is preserved under sequential composition~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}; we make no concurrent-composition claim.
A malicious adversary deviates arbitrarily; security with abort requires that it achieve nothing beyond an ideal world in which a trusted functionality computes the result and the adversary only chooses corrupted inputs and whether honest parties receive output, so fairness is not required.
Covert security~\cite{aumann2007covert} only deters cheating; we target full malicious security with abort.

\textbf{Information-theoretic MACs.}
SPDZ-style protocols~\cite{damgard2012spdz,damgard2013practical} authenticate each value of a field $\F$ under a global key $\Delta=\Delta_0+\Delta_1$ that no single party knows.
Party $b$ holds $\Delta_b$ and $\authb{x}{b}=(x_b,\gamma_b)$ with $x_0+x_1=x$ and $\gamma_0+\gamma_1=\Delta x$; linear operations act identically on values and tags, and multiplications consume authenticated triples.
To check openings $z_1,\dots,z_m$, the parties draw coefficients $\rho_i$ \emph{after} the values are fixed, compute $\sigma_b=\sum_i\rho_i(\gamma_{b,i}-\Delta_b z_i)$, and accept only if $\sigma_0+\sigma_1=0$.
A wrong opening passes only if its tag error matches $\Delta$ times the value error or cancels under the coefficients, which happens with probability less than $2/|\F|$.
\sys instantiates this with $t=3$ independent lanes over $\Fp$ (\cref{sec:proto-repr}).

\textbf{Authenticated preprocessing.}
Malicious protocols need authenticated masks and triples whose relations, such as $c=ab$, are actually correct; a valid MAC on a wrong triple does not make it correct.
Generating them without a trusted party is communication-heavy, with oblivious transfer in MASCOT~\cite{keller2016mascot} or somewhat homomorphic encryption in SPDZ and Overdrive~\cite{damgard2012spdz,keller2018overdrive}, all in MP-SPDZ~\cite{keller2020mpspdz}.
Pseudorandom correlation generators~\cite{boyle2019pcg,boyle2020pcg} compress this communication at a substantial computational cost, and a trusted dealer avoids generation but ships every authenticated share.

\textbf{Malicious and verifiable FSS.}
Malicious FSS gates additionally need well-formed keys and authenticated evaluation outputs that can enter MAC-checked arithmetic.
Verifiable FSS~\cite{decastro2022vfss} checks that a key pair shares a function of the declared class, not that a malicious party evaluates its own key correctly.
Shark~\cite{gupta2025shark} achieves active security for FSS-based inference with a dealer that issues authenticated FSS keys and correlated randomness, which enlarges the offline material relative to semi-honest FSS.
The direct way to authenticate a DPF output, a second \emph{tag tree} with payload $\Delta_j\beta$ per MAC key, multiplies DPF work by $1+t$ for $t$ lanes (\cref{sec:analysis-work}).

\textbf{Trusted hardware for secure computation.}
Slalom~\cite{tramer2018slalom} and DarKnight~\cite{hashemi2021darknight} outsource linear layers from a trusted execution environment (TEE) to untrusted GPUs and check the results, Slalom with Freivalds' algorithm~\cite{freivalds1977probabilistic}, which \sys uses only for a restricted subroutine (\cref{sec:proto-freivalds}).
PPMLAC~\cite{zhou2022ppmlac} and STAMP~\cite{huang2022efficient} use small trusted modules to generate correlated randomness or to execute nonlinear operations; STAMP also reports honest-majority malicious settings, and \cref{sec:related} compares these and other trusted-hardware designs.

\textbf{Implications.}
Each tool covers only part of the integrity chain of \cref{sec:intro}, at a cost that erodes trusted DFA's advantage (\cref{sec:analysis}); \sys therefore keeps the module as the dealer and also makes it the verifier (\cref{sec:protocol}).

\textbf{Scope.}
Throughout this paper, \emph{private inference} means two-party FSS-based private inference and \emph{PIR} means two-server DPF-based PIR, as in DFA~\cite{dfa2026trusted}.


==> qa/draft2/sections/03_threat_model.tex <==
% ==================================================================
% Section III: Threat Model and Security Goals
% Owner labels: sec:threat, sec:threat-model, sec:threat-scenarios,
%   sec:threat-goals, sec:threat-profileu, fig:threat, fig:scenarios,
%   tab:scenarios, fig:func, def:security, def:leakage
% ==================================================================
\section{Threat Model and Security Goals}\label{sec:threat}

The trusted mode of DFA moved the FSS dealer into a small protected module but kept the semi-honest model of the protocols it accelerates~\cite{dfa2026trusted}. This section states what changes when a host is malicious: we fix the system model (\cref{sec:threat-model}) and the adversary, derive ten attack scenarios (\cref{sec:threat-scenarios}), define security with explicit leakage (\cref{sec:threat-goals}), and delimit \ProfU (\cref{sec:threat-profileu}). Every link of the integrity chain of \cref{sec:intro} crosses memory, buses, or network paths that a corrupted host controls.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_threat.pdf}
    \caption{System model and trust boundary of \sys under \ProfT. Each party $P_b$ has an untrusted host (CPU, OS, driver, runtime, NIC, DRAM) with its GPU (SMs, HBM) and a protected module $T_b$ (red dashed TCB, contents in \cref{sec:threat-model}). The adversary statically corrupts at most one host (here that of $P_0$, red region) and may deviate arbitrarily, replay, and abort, but never corrupts $T_0$ or $T_1$. Hosts and GPUs hold only party-local authenticated shares; the protected peer channel between the modules and the authenticated confidential client channels are carried by the untrusted network.}
    \label{fig:threat}
\end{figure*}

\subsection{System Model and Trust Boundary}\label{sec:threat-model}

\textbf{Parties.}
\sys targets the two workloads of DFA~\cite{dfa2026trusted}: two-party FSS-based private inference and two-server DPF-based PIR (\cref{sec:bg}). Two computing parties $P_0$ and $P_1$ serve an external client that owns private inputs and receives outputs; a computing party may also own an input, typically the model weights. Each $P_b$ consists of an untrusted \emph{host~$b$} (every component outside the TCB in \cref{fig:threat}, including DMA engines and storage) and a \emph{protected module} $T_b$, the \sys extension placed next to the GPU L2 as in DFA (\cref{sec:arch-hw}).

\textbf{Trusted computing base.}
$T_b$ contains the session, identity (attestation), and joint-sampler keys and the global MAC keys $\Delta_1,\dots,\Delta_t$; the session role, counters, and one-time resource ledger; the DPF generator and evaluator states and the correction words; the protected table and reduction logic; the frozen check buffers, challenges, and residuals; and all release decisions. Everything else is outside, including every GPU and DMA buffer and every byte in transit between the parties. The GPU computes on party-local authenticated arrays and hands $T_b$ only \emph{candidate} shares (\cref{sec:proto-repr}). Host~$b$ may know its own MAC key shares $\Delta_{b,j}$, but no host ever holds a complete $\Delta_j$, the joint-sampler key, a complete mask, the peer's shares, or any challenge or residual.

\textbf{Modules as an ideal resource.}
Following~\cite{katz2007universally}, we model $T_0,T_1$ as an ideal resource $\mathcal{F}_{\mathsf{T}}$ (\cref{app:func-module}; ideal-module assumption in \cref{sec:sec-assump}): their code, keys, parser, arithmetic, state, and approved I/O paths are correct and confidential, and each module's externally observable trace (lengths, timing, host-visible memory and DMA activity, power, thermal, and clock telemetry) is simulatable from the command sequence issued by the host, $\mu$, public lengths, and the accept or abort outcomes, and is independent of the global MAC keys, challenges, and residuals given these. The real execution (\cref{def:security}) realizes their randomness, channels, and setup with concrete primitives. Availability is not assumed, \ProfT requires two physically independent modules, and only the on-die design (\cref{sec:arch-hw}) is a \ProfT target.

\textbf{Channels.}
Client channels are authenticated, confidential, and terminate inside the modules; the peer channel uses AEAD with independent directional keys and no nonce reuse and is established by the authenticated setup of \cref{sec:proto-setup}. The untrusted network carries both. We propose no new attestation or key-exchange protocol; the security of setup is the explicit assumption $\eps{setup}$.

\textbf{Trust is relocated, not removed.}
The modules jointly act as the dealer and can recover inputs from verified openings, and in PIR both modules learn the queried index $\alpha$. \sys thus moves trust from an external dealer and the hosts into the modules rather than hiding inputs from them (\cref{sec:discussion}); its PIR query privacy rests on module trust, unlike untrusted two-server DPF-PIR such as GPU-DPF~\cite{lam2023gpu} or DFA's untrusted mode~\cite{dfa2026trusted}, which hides $\alpha$ from each server without trusted hardware.

\subsection{Adversary Model}

Unlike DFA~\cite{dfa2026trusted}, Sigma~\cite{gupta2023sigma}, and Orca~\cite{jawalkar2024orca}, which assume that both hosts run the prescribed kernels, we consider a probabilistic polynomial-time (PPT) adversary $\Adv$ that statically and maliciously corrupts at most one host before the session starts (host~$0$ in \cref{fig:threat}, by symmetry), controlling its operating system, drivers, GPU kernels and results, host and GPU memory including DMA buffers, and outgoing network traffic. Concretely, $\Adv$ can
(i) modify any value share or tag and run arbitrary kernels in place of the prescribed ones;
(ii) invoke its module's commands in any order with malformed, replayed, or mislabeled arguments;
(iii) rewrite any host-visible buffer at any time, including while the module reads it;
(iv) replay, reorder, delay, or drop messages, reset its platform, and restore old host-side state;
(v) choose the inputs it owns arbitrarily; and
(vi) abort at any point, including after it has learned its own output.
It observes message lengths and timing, the frames exchanged with its module, and the module's external trace. The principal inference statement assumes an honest external client and gives no guarantee against client-server collusion; PIR has two separate regimes, (R1) one malicious server host and (R2) a malicious client only with two honest server hosts (\cref{fig:func}).

\textbf{Out of scope.}
Our theorems exclude corruption of either module (its code, keys, state, or arithmetic); physical attacks such as microprobing, optical fault injection, and power or electromagnetic analysis with measurement equipment~\cite{skorobogatov2017microprobing,skorobogatov2003optical,kocher1999differential,quadir2016survey}; leakage beyond the stipulated trace model; speculative-execution bugs inside the trusted boundary~\cite{van2018foreshadow}; faulty trusted arithmetic; adaptive corruption; and corruption of both hosts. Software-reachable fault and power channels are not physical attacks: the corrupted host controls the GPU driver, which sets clocks, voltage, and power limits and reads telemetry, an interface that Plundervolt exploited on CPUs~\cite{murdock2020plundervolt}. We therefore require isolation from dynamic voltage and frequency scaling (DVFS): host software cannot drive the module's clock or voltage outside its safe operating range (or the module detects glitches and aborts), and the telemetry is covered by the trace simulator. Rollback of module state is covered only by the reboot rule of \cref{sec:proto-ledger}. Availability and fairness are not provided.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_scenarios.pdf}
    \caption{Malicious scenarios S1 to S8 against trusted FSS acceleration and the \sys mechanism that stops each. Corrupted hosts and GPUs are shaded red, $T_b$ is the red dashed TCB, red arrows with circled numbers are adversary actions, red crosses mark where \sys blocks them, and green text names the defense. S9 and S10, which no protocol can prevent, appear only in \cref{tab:scenarios}.}
    \label{fig:scenarios}
\end{figure*}

\subsection{Malicious Scenarios Against Trusted FSS Acceleration}\label{sec:threat-scenarios}

\Cref{fig:scenarios} and \cref{tab:scenarios} list what a corrupted host can do to a trusted FSS accelerator designed for semi-honest hosts and which \sys mechanism stops each action; the paragraphs below explain why the semi-honest design fails. The scenarios follow the integrity chain: S9 targets the authorized input; S4 and S7 the correlated preprocessing; S2 and S5 the correct local evaluation; S1 the authenticated arithmetic; S3 the consistent opening; and S6 the authorized output release. S8 carries S3 over to the PIR database, and S10 targets availability, which lies outside the chain. \Cref{sec:sec-scenarios,sec:eval-attack} map the scenarios to theorems and to injected tests.

\textbf{S1: Share and tag tampering.}
The corrupted GPU holds every intermediate share and can add an error vector $\bm{e}$ to value shares (and $\bm{d}_j$ to the tags of lane $j$); semi-honest trusted DFA passes it unchecked into the masked opening $x_i+r_i$ of the next FSS gate. Beyond biasing results, this causes \emph{selective failure}: whether $e_i$ flips a comparison depends on whether $x_i$ lies within $|e_i|$ of the threshold, so any observable output change leaks information about $x_i$ (\cref{tab:scenarios}, \cref{sec:proto-check}).

\textbf{S2: Forgery-oracle request.}
A tempting extension of DFA's trusted mode is a command that tags a value computed elsewhere, such as a nonlinear output of the SMs. This \emph{authenticate(host value)} entry point turns the module into a MAC oracle: the host submits any $y^*$, and every later check accepts it. Attestation certifies the module's code, not the provenance of what it signs (\cref{tab:scenarios}, \cref{sec:proto-epilogue}).

\textbf{S3: TOCTOU buffer swap.}
The module reads its inputs by DMA from host-controlled memory. Verifying a buffer and later rereading it, or trusting a host-reported digest, admits a time-of-check-to-time-of-use (TOCTOU) swap: the host changes the bytes after verification or chooses its error after the challenge is fixed. DMA completion is not evidence of authenticity, a problem semi-honest DFA never faced (\cref{tab:scenarios}, \cref{sec:proto-check}).

\textbf{S4: Replay and rollback.}
DFA derives keys and masks from the shared key $K$ and a counter that is an input of its generate-and-consume procedure~\cite{dfa2026trusted}. Replaying a counter yields the same mask $r$ for two gates, and the openings $x+r$ and $x'+r$ reveal $x-x'$; resetting the module and resuming an old session replays entire key streams (\cref{tab:scenarios}, \cref{sec:proto-ledger}).

\textbf{S5: Role and gate confusion.}
The host decides which module command runs for which gate: it can route the preprocessing of gate $g$ into gate $g'$, alter a table hash or tensor shape, or present party-$0$ material as party-$1$ material. If the role were a per-request argument, the host could obtain both parties' outputs of one joint draw and reconstruct the DPF target $\alpha$, which is exactly the mask of an honest input (\cref{tab:scenarios}, \cref{sec:proto-setup,sec:proto-ledger}).

\textbf{S6: Premature release.}
Semi-honest trusted DFA releases results as soon as they are computed; under a malicious host an early output may already be wrong, and the host may request it repeatedly or for an unauthorized recipient (\cref{tab:scenarios}, \cref{sec:proto-ledger}).

\textbf{S7: Malformed preprocessing.}
A MAC authenticates values, not relations: a triple $(\auth{a},\auth{b},\auth{c})$ with $c\neq ab$ carries valid tags, and multiplying with it yields $xy+\delta$ for a $\delta$ chosen by its producer; the same holds for a GPU-computed matrix product $C=AB$ and for a malformed DPF key. DFA's attestation covers the module's own key generation, not correlations from elsewhere (\cref{tab:scenarios}, \cref{sec:proto-arith}).

\textbf{S8: Snapshot substitution in PIR.}
The PIR database resides in host memory, so a corrupted server host can modify a record, serve an older version, or hash one buffer while scanning another. Semi-honest PIR, including DFA-accelerated PIR, returns whatever the servers compute. Worse, a record modified only at position $i$ corrupts the answer only when $\alpha=i$, so the client's reaction leaks the queried index (\cref{tab:scenarios}, \cref{sec:proto-pir}).

\textbf{S9 and S10: Input substitution; denial of service and selective abort.}
S9, a corrupt owner choosing its input freely, is permitted and extracted by $\FC$; binding a specific model needs the commitment of \emph{Model provenance} below. S10 is not prevented: like SPDZ-style protocols~\cite{damgard2012spdz,keller2016mascot}, \sys provides security with abort, without fairness or guaranteed output delivery, and abort outcomes stay within the permitted leakage (\cref{def:leakage}, \cref{sec:discussion}).

\begin{table*}[t]
\centering
\caption{Malicious scenarios against trusted FSS acceleration. The ``effect'' column describes a semi-honest trusted DFA~\cite{dfa2026trusted}, or a naive malicious extension of it, when one host is corrupted. \cmark: prevented up to the error terms of \cref{thm:main}; \pmark: permitted by the ideal functionality; \xmark: not prevented.}
\label{tab:scenarios}
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabularx}{\textwidth}{c >{\raggedright\arraybackslash}p{1.75cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{2.75cm}}
\hline
\textbf{ID} & \textbf{Scenario} & \textbf{Adversary action} & \textbf{Effect on semi-honest trusted DFA} & \textbf{\sys mechanism} & \textbf{Guarantee} \\
\hline
S1 & Share/tag tampering & GPU adds errors $\bm{e}$ to value shares (and $\bm{d}_j$ to tags) before an opening or FSS gate & Undetected; biases outputs and causes selective failure that leaks inputs & Authenticated shares with $t=3$ MAC lanes over $\Fp$; \CheckOpen{} before any protected gate or release & \cmark\ Wrong value accepted w.p.\ $\le (2/p)^t$ per batch (\cref{thm:mac-sound}) \\
\hline
S2 & Forgery-oracle request & Host submits $y^*$ and asks its module to authenticate it & No MACs; a naive authenticate command would sign any forgery & No \emph{authenticate(host value)} command; \Epilogue{} only on internally computed or verified results & \cmark\ Request rejected; outputs correctly authenticated (\cref{thm:epilogue}) \\
\hline
S3 & TOCTOU buffer swap & Host rewrites a DMA buffer after it is checked, or after the challenge is fixed & Module trusts DMA reads; a later reread consumes modified bytes & Freeze before challenge: bytes copied or AEAD-sealed, frozen roots agreed, only frozen bytes consumed & \cmark\ Modification ignored or abort; binding error $\eps{bind}$ \\
\hline
S4 & Replay and rollback & Replays a counter or mask request; resets the module and resumes old keys & Mask reuse: $x+r$ and $x'+r$ reveal $x-x'$; key streams replayed & Labels bound to session, epoch, gate, purpose; one-time ledger; epoch poisoning; erase-and-rekey after reboot & \cmark\ Reuse rejected before any accepted use \\
\hline
S5 & Role/gate confusion & Routes party-0 material as party-1, or gate $g$ material into gate $g'$; alters shapes or table hash & Host schedule trusted; requesting both roles' outputs exposes the target $\alpha$ & Roles fixed by authenticated setup; gate descriptors bound in the ledger and in PRF labels & \cmark\ Mismatch aborts before preprocessing is issued \\
\hline
S6 & Premature release & Requests outputs before verification, repeatedly, or for another recipient & Results released as soon as computed & Release guard: nothing before \lstate{VERIFIED}; bound certificates; epoch abort gates pending outputs & \cmark\ No candidate value leaves the modules \\
\hline
S7 & Malformed preprocessing & Injects a triple with valid tags but $c\neq ab$, a GPU-computed $C=AB$, or a wrong DPF key & Attestation silent on external correlations; MACs verify wrong triples & Triples and keys generated inside the TCB ($c=ab$ computed there); imports need a correctness proof & \cmark\ Never consumed; exact arithmetic (\cref{thm:arith}) \\
\hline
S8 & Snapshot substitution (PIR) & Swaps records or version after hashing, or scans a different buffer & Client reconstructs a wrong record; index-dependent failure leaks $\alpha$ & Module hashes the bytes it consumes in public order; quarantine until the commitment matches & \cmark\ Committed record or abort (\cref{thm:pir}) \\
\hline
S9 & Input substitution by a corrupt owner & Corrupted party supplies arbitrary weights or inputs & Same (allowed) & Input extraction by $\FC$; optional commitment-bound loader for model provenance & \pmark\ Allowed by the functionality \\
\hline
S10 & Denial of service/selective abort & Drops, delays, or reorders messages; aborts after learning its own output & Same (not prevented) & Bounded resources and abort; abort outcomes simulatable from permitted leakage & \xmark\ Not prevented (no fairness or availability) \\
\hline
\end{tabularx}
\end{table*}

\subsection{Security Goals and Ideal Functionalities}\label{sec:threat-goals}

\textbf{Goals.}
Against a corrupted host, \sys must provide \emph{privacy} (the host learns nothing beyond the permitted leakage and the outputs it is authorized to receive), \emph{correctness} (honest recipients obtain the circuit evaluated on the honest inputs and the corrupted party's extracted inputs, or abort), \emph{authorized release} (no value leaves the modules unless its opening was verified and bound to a release certificate), and \emph{one-time use} (no randomness is consumed twice). We formalize the first two as stand-alone real/ideal security with abort, preserved under sequential composition~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}, with an explicit leakage function; the last two are mechanisms that the proof relies on (\cref{sec:proto-ledger}). We claim neither universal nor concurrent composability, and concurrent sessions that share module state are not covered.

\textbf{Manifest.}
Every session fixes a public manifest $\mu$ (\cref{app:func-circuit}): the protocol version, session identities, roles, field, numeric encoding, the finite circuit $C$ with its gate and wire identifiers and tensor shapes, approved public tables, interval coefficients, authorized recipients, the input interface $\mathsf{In}_\nu$ and validation rules of every input wire $\nu$, and the public schedule, which places every input gate and validity check before the first output opening. The modules evaluate the validity predicates at the public boundaries declared in $\mu$; in $\Pi_{\mathsf{Input}}$ they compute $x^{*}=r+\varepsilon$ and abort unless $x^{*}\in\mathsf{In}_\nu$ (\cref{fig:arith}).

\begin{definition}[Permitted leakage]\label{def:leakage}
For a circuit execution under manifest $\mu$, the permitted leakage is
\[
\Leak_C=\bigl(\mu,\ \mathsf{len},\ \mathsf{sched},\ \mathsf{pub},\ \mathsf{status}\bigr),
\]
where $\mathsf{len}$ are the lengths of all public messages; $\mathsf{sched}$ is the public schedule of batches, checks, and interaction boundaries fixed by $\mu$; $\mathsf{pub}$ are the values that $\mu$ designates as authorized public openings; and $\mathsf{status}$ are the specified abort and validation outcomes, including every input-dependent validity bit declared in $\mu$, which is never silently excluded. For PIR, $\Leak_{\mathrm{PIR}}$ consists of the public descriptor $\mathsf{desc}_v=(\mathsf{id},v,N,\mathsf{enc},\mathsf{cm}_v)$ (database identifier, version, true length $N$, which also fixes the padded length, record encoding, and authorized snapshot commitment), the public scan length and order, message lengths and schedules, and the accept, reject, or abort outcome.
\end{definition}

Honest inputs, intermediate wire values, masks, MAC keys, DPF keys and correction words, raw FSS outputs, challenges, and residuals are not in $\Leak_C$. Masked openings such as $x+r$ are uniform given $\Leak_C$, and the simulator samples them (\cref{app:proof-main}). Module timing and access patterns are fixed by $\mu$ (full-domain scans have a declared order); the residual trace falls under $\eps{trace}$.

\begin{figure}[t]
\centering
\footnotesize
\fbox{\begin{minipage}{\dimexpr\columnwidth-2\fboxsep-2\fboxrule\relax}
\centering\underline{Functionality $\FC$}\par\smallskip
\raggedright
\textbf{Parameters.} Public manifest $\mu$ (circuit $C$ over $\Fp$, input owners and interfaces $\mathsf{In}_\nu$, validity predicates, authorized recipients, public schedule). Corrupted set $I$: at most one host; the client is honest.
\begin{enumerate}[leftmargin=*,nosep,topsep=2pt]
\item \textbf{Input.} Receive the authenticated input $x_\nu$ of every input wire $\nu$ from its designated owner. If the owner is corrupted, accept any $x^{*}_\nu\in\mathsf{In}_\nu$ from $\Sim$; this extracted value is used below.
\item \textbf{Validate and evaluate.} Evaluate the validity predicates of $\mu$; their accept or abort outcome is part of the output. For accepted inputs, compute $\vec{y}=C(\vec{x})$ exactly in the declared finite arithmetic, including the specified comparisons and truncations.
\item \textbf{Deliver or abort.} Send $\Leak_C$ and the outputs of corrupted recipients to $\Sim$. At each public interaction boundary, $\Sim$ may send $\mathsf{abort}$ or $\mathsf{delay}$; on $\mathsf{abort}$, send $\bot$ to every honest recipient. Otherwise deliver each $y_i$ to its authorized recipient. A corrupted recipient may obtain its output before honest ones (no fairness).
\end{enumerate}
\end{minipage}}

\vspace{5pt}
\fbox{\begin{minipage}{\dimexpr\columnwidth-2\fboxsep-2\fboxrule\relax}
\centering\underline{Functionality $\FPIR$}\par\smallskip
\raggedright
\textbf{Parameters.} Public descriptor $\mathsf{desc}_v=(\mathsf{id},v,N,\mathsf{enc},\mathsf{cm}_v)$; the commitment $\mathsf{cm}_v$ fixes $D=(D[0],\dots,D[N-1])$. Corruption regimes, never combined: (R1) a malicious server host (at most one), client honest; (R2) a malicious client only, both server hosts honest.
\begin{enumerate}[leftmargin=*,nosep,topsep=2pt]
\item \textbf{Query.} Receive an index $\alpha$ with query identifier $\mathit{qid}$ from the client; in (R2), extract the corrupted client's index $\alpha^{*}$ and set $\alpha\gets\alpha^{*}$. If $\alpha\notin\{0,\dots,N-1\}$ or the request is inconsistent, return $\mathsf{reject}$ to the client and stop.
\item \textbf{Leak.} Send $\Leak_{\mathrm{PIR}}$ to $\Sim$; nothing about $\alpha$ is sent.
\item \textbf{Answer.} In (R1), if $\Sim$ sends $\mathsf{abort}$, send $\bot$ to the client; otherwise send $D[\alpha]$. In (R2), send $D[\alpha]$, and no other information about $D$, to the client.
\end{enumerate}
\end{minipage}}
\caption{Ideal functionalities for authenticated circuit evaluation (top) and versioned-snapshot PIR (bottom). Both provide security with abort. $\FPIR$ hides $\alpha$ from the corrupted host; both trusted modules learn it (\cref{sec:threat-model}). The full definitions, together with the ideal module resource $\mathcal{F}_{\mathsf{T}}$, are in \cref{app:func}.}
\label{fig:func}
\end{figure}

\begin{definition}[Static malicious security with abort]\label{def:security}
Let $\mathcal{F}\in\{\FC,\FPIR\}$ with leakage $\Leak$ as in \cref{def:leakage}, and let $\Pi$ be a protocol run by $P_0$ and $P_1$ in which each module executes the concrete module program correctly and confidentially: $\mathcal{F}_{\mathsf{T}}$ with its joint random function $R$ instantiated by $\PRF_K$, its peer and client channels by AEAD over the hosts' network, and \cmd{OPEN_SESSION} by attestation and authenticated key exchange. Fix a PPT adversary $\Adv$ with auxiliary input $z$ that statically corrupts a set $I$ admitted by the corruption regime of $\mathcal{F}$, a manifest $\mu$, and an input vector $\vec{x}$.
$\Real_{\Pi,\Adv(z),I}(\mu,\vec{x})$ is the joint distribution of the view of $\Adv$ (its inputs, randomness, received messages, and the external traces of the modules observable from corrupted hosts) and the outputs of the honest parties and client in an execution of $\Pi$.
$\Ideal_{\mathcal{F},\Sim(z),I}(\mu,\vec{x})$ is the joint distribution of the output of a simulator $\Sim$ and the honest outputs in an execution in which $\Sim$ interacts only with $\mathcal{F}$: it submits the corrupted parties' inputs, receives $\Leak$ and the corrupted parties' outputs, and may abort or delay as $\mathcal{F}$ allows.
We say that $\Pi$ \emph{$\epsilon$-securely realizes $\mathcal{F}$ with leakage $\Leak$ against static malicious corruption with abort} if for every such $\Adv$ there exists a PPT simulator $\Sim$ such that for all $\mu$, $\vec{x}$, $z$, $I$ and every PPT distinguisher $\mathcal{D}$,
\begin{align*}
\Bigl|&\Pr\bigl[\mathcal{D}\bigl(\Real_{\Pi,\Adv(z),I}(\mu,\vec{x})\bigr)=1\bigr]\\
&\quad-\Pr\bigl[\mathcal{D}\bigl(\Ideal_{\mathcal{F},\Sim(z),I}(\mu,\vec{x})\bigr)=1\bigr]\Bigr|\le\epsilon .
\end{align*}
\end{definition}

\textbf{Remarks.}
The real world of \cref{def:security} contains the concrete module program; $\mathcal{F}_{\mathsf{T}}$ with ideal setup, channels, and randomness is the resource of hybrids $\Hyb{2}$ to $\Hyb{4}$ of the proof (\cref{app:proof-main}), and the simulator controls only this ideal representation of the trusted resources, never the honest party's prescribed inputs. The concrete $\epsilon$ is the bound $\eps{VIGOR}$ of \cref{thm:main}; correctness of protected code is a premise of $\mathcal{F}_{\mathsf{T}}$, and \cref{tab:obligations} lists what a chip must still establish.

\textbf{Model provenance.}
Computational correctness is not model provenance, and a public architecture hash in $\mu$ does not authenticate private weights. To bind a pre-approved model, $\mu$ must contain a commitment to the canonical quantized weight bytes, authorized by the client or an independent model authority rather than declared by the untrusted host, and the protected input loader hashes exactly those bytes before sharing them (\cref{sec:proto-arith}); a mismatch aborts. Otherwise the weights are the owner's freely chosen private input, and S9 is the intended behavior of $\FC$.

\subsection{The Stronger Profile U}\label{sec:threat-profileu}

\ProfT trusts the modules. When the hardware itself must be treated as adversarial, for example because the accelerator vendor or platform administrator is untrusted, \ProfU gives the accelerator neither the joint-sampler key nor any global MAC key. The circuit runs through an established malicious two-party backend, such as SPDZ-family protocols with MASCOT or SPDZ2k preprocessing~\cite{damgard2012spdz,keller2016mascot,cramer2018spdz2k,keller2020mpspdz} or dealer-based malicious FSS such as Shark~\cite{gupta2025shark}, and the accelerator is confined to party-local data, for instance expanding the DPF keys that the backend exports to its own party. The same DPF datapath therefore serves both profiles, but \ProfU gives up the local-dealer and generate-and-consume savings, and with exported keys it must add the backend's DPF privacy assumption to its bound (\cref{sec:sec-main}). \ProfU is a separate backend chosen at session start, not a fallback after a module compromise, which would not undo leaked secrets; a fresh session with fresh inputs and masks is required. The rest of this paper analyzes and evaluates \ProfT.


==> qa/draft2/sections/04_analysis.tex <==
% ======================================================================
% Section IV: Workload Analysis (owner: sections/04_analysis.tex)
% Labels defined here: sec:analysis, sec:analysis-cost, sec:analysis-dpf,
% sec:analysis-work, alg:gen, alg:eval, fig:gac, tab:gatecost, fig:motiv
% ======================================================================
\section{Workload Analysis: Where Malicious Security Costs Go}
\label{sec:analysis}

The DFA design~\cite{dfa2026trusted} was driven by one workload observation: in semi-honest FSS workloads, DPF generation, distribution and evaluation dominate both computation and communication, so a small DPF engine that also plays the dealer removes the dominant cost. Repeating this analysis for the adversary of \cref{sec:threat} changes the design target: handled naively, malicious security multiplies exactly the DPF work and key traffic that trusted DFA made small; handled carefully, it moves the cost from DPF to authenticated linear algebra on the GPU and to the extra round of every verified opening.

% ======================================================================
\subsection{Cost Sources in Malicious FSS}
\label{sec:analysis-cost}

We take as reference the masked-input paradigm of FSS-based inference~\cite{gupta2023sigma,jawalkar2024orca} (\cref{sec:bg-pi}): linear layers operate on additive shares, and every nonlinear gate opens a masked input $x+r$ and evaluates FSS keys prepared for the mask $r$. Making this pipeline secure against a malicious host (\cref{def:security}) adds the following costs, regardless of how they are implemented.

\textbf{(i) Authenticated representation.}
Every wire must carry information-theoretic MACs so that a host that changes its share is caught~\cite{damgard2012spdz,damgard2013practical}. In our representation (\cref{sec:proto-repr}), party $b$ holds $\authb{x}{b}=(x_b,\gamma_{b,1},\gamma_{b,2},\gamma_{b,3})$ over $\Fp$ with $p=2^{61}-1$ and $t=3$ independent MAC keys: four 64-bit words, or 32~B per element and party, instead of 8~B for a semi-honest share in $\Z_{2^{64}}$. Every linear layer is therefore computed on four lanes (the value and three tags), each lane uses exact Mersenne reduction instead of free 64-bit wraparound (\cref{sec:arch-field}), and every authenticated element that crosses PCIe or the host-module interface grows by the same factor of four. Only the peer link is spared, because checks exchange value shares and $t$ residuals rather than tags (\cref{sec:proto-check}).

\textbf{(ii) Verified openings.}
Opened values (masked gate inputs, the Beaver differences $d,e$ of each multiplication~\cite{beaver1991efficient}, and outputs) must be checked before anything depends on them. A sound check derives its challenge only after the checked bytes are fixed (\cref{thm:mac-sound}), so at least one extra exchange follows every checked batch, and a dependent nonlinear gate may not consume an unchecked opening. Batching amortizes challenge derivation and metadata but not this round, which lies on the critical path of every layer: a protocol with $R$ online rounds approaches $2R$.

\textbf{(iii) Correct preprocessing.}
Triples, masks and FSS keys must be \emph{correct}, not merely authenticated: a valid MAC on a triple with $c\neq ab$ does not make it correct. The options of \cref{sec:bg-mal} either ship more offline material from a dealer or replace the dealer by heavy interactive preprocessing, and neither removes offline data movement. Without a dealer, FSS keys require a secure two-party evaluation of DPF key generation, with one round per tree level~\cite{doerner2017scaling} before any malicious-security overhead.

\textbf{(iv) Authenticated FSS outputs.}
A DPF output share is a plain additive share. To re-enter authenticated arithmetic it needs $t$ tag shares, and the straightforward way to obtain them is a second DPF per MAC lane $j$ with the same target and payload $\Delta_j\beta$ (a \emph{tag tree}). This multiplies DPF keys, key bytes and PRG work by $1+t$, i.e., by four for $t=3$.

\textbf{(v) Key validity is not evaluation correctness.}
Verifiable FSS~\cite{decastro2022vfss} lets evaluators check that their keys are well formed, which protects against a malicious key generator. It does not constrain an evaluator that computes on valid keys and then adds an error to its output share, nor the arithmetic that consumes that share.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{charts/chart_motiv.pdf}
    \caption{Estimated BERT-Base latency breakdown on LAN (1~GB/s, 0.05~ms RTT) by cost source, for two semi-honest configurations of~\cite{dfa2026trusted} and three malicious ones (dealer-based malicious FSS, \sys without GaC, \sys); all splits come from our model (\cref{app:model}). The horizontal axis is broken between 7.5 and 15~s so that the 18.8~s semi-honest GPU bar and the \est{43.9~s} dealer-based bar fit.}
    \label{fig:motiv}
\end{figure}

\textbf{Observation 1: distribution still dominates dealer-based malicious FSS.}
\Cref{fig:motiv} splits the estimated BERT-Base LAN latency by cost source. Dealer-based malicious FSS, modeled after the protocol family of Shark~\cite{gupta2025shark} (\cref{sec:eval-method}), must move \est{37.6~GB} of authenticated keys and preprocessing per query, \est{2.2$\times$} the 17.1~GB of the semi-honest GPU baseline~\cite{dfa2026trusted}. At 1~GB/s, this distribution alone takes \est{37.6~s} of \est{43.9~s} (\est{86\%}), and moving the material from host memory into the GPU adds another \est{1.70~s}. Without an authenticated-key blow-up ($\kappa_{\mathrm{key}}=\est{1}$, \cref{app:model}), it still takes \est{22.4~s}, \est{5.8$\times$} that of \sys.

\textbf{Observation 2: without distribution, DPF is no longer the bottleneck.}
Removing distribution, as trusted DFA did for the semi-honest case, exposes a different profile. In \sys, four-lane authenticated GEMM takes \est{2.60~s} of \est{3.83~s} (\est{68\%}), \est{5.0$\times$} our \est{0.52~s} estimate of the semi-honest GEMM; online communication takes \est{0.615~s} (\est{16\%}); and all nonlinear gates together take only \est{0.131~s} (\est{3.4\%}).

\textbf{Observation 3: on a WAN, verification rounds dominate.}
With a 70~ms RTT the extra check round of source (ii) outweighs all computation: removing \CheckOpen, which is insecure and serves only as a lower bound, would cut the estimated BERT-Base WAN latency from \est{89.7~s} to \est{50.5~s} (\cref{tab:ablation}).

% ======================================================================
\subsection{Compute Pattern of Exact DPF}
\label{sec:analysis-dpf}

Malicious-security proofs reason about concrete states, so we fix the DPF computation exactly. \Cref{alg:gen,alg:eval} give the tree-based DPF~\cite{gilboa2014distributed,boyle2016function} in the form that \sys executes; the same algorithms serve \ProfU, where keys are exported to an external malicious backend (\cref{sec:threat-profileu}). The expansion function $\PRG:\bits{128}\to(\bits{128}\times\{0,1\})^2$ is fixed and AES-based as in DFA, $\Conv:\bits{128}\to\Fp$ is the fixed output conversion, the target $\alpha$ and the query $x$ have $n$ bits read most-significant first, and the payload is $\beta\in\Fp$.

\begin{algorithm}[t]
\caption{Exact DPF key generation ($\DPF.\Gen$)}
\label{alg:gen}
\begin{algorithmic}[1]
\algstretch
\Require target $\alpha=\alpha_1\cdots\alpha_n\in\bits{n}$ (MSB first), payload $\beta\in\Fp$
\Ensure keys $(k_0,k_1)$ with $\Eval(k_0,x)+\Eval(k_1,x)=\beta\cdot\one[x=\alpha]$
\State sample independent $s_0,s_1\getsr\bits{128}$; $t_0\gets 0$; $t_1\gets 1$
\State save the initial seeds $s_0^{(0)}\gets s_0$, $s_1^{(0)}\gets s_1$
\For{$i=1$ \textbf{to} $n$}
    \State $a\gets\alpha_i$; \ $\keep\gets a$; \ $\lose\gets 1-a$ \Comment{$L=0$, $R=1$}
    \State $(s_b^L,t_b^L,s_b^R,t_b^R)\gets\PRG(s_b)$ for $b\in\{0,1\}$
    \State $\sCW\gets s_0^{\lose}\oplus s_1^{\lose}$
    \State $\tCW{L}\gets t_0^L\oplus t_1^L\oplus a\oplus 1$; \ $\tCW{R}\gets t_0^R\oplus t_1^R\oplus a$
    \LineComment{both $b$, with the \emph{old} $t_b$; $\cdot$ is a conditional XOR}
    \State $(s_b,t_b)\gets\bigl(s_b^{\keep}\oplus t_b\cdot\sCW,\ t_b^{\keep}\oplus t_b\cdot\tCW{\keep}\bigr)$
    \State $\CW^{(i)}\gets(\sCW,\tCW{L},\tCW{R})$
\EndFor
\State $u_b\gets\Conv(s_b)$ for $b\in\{0,1\}$
\State $\CWout\gets(-1)^{t_1}\,(\beta-u_0+u_1)$
\LineComment{keys hold the initial roots, never the final states}
\State $k_b\gets\bigl(s_b^{(0)},\,b,\,\CW^{(1)},\ldots,\CW^{(n)},\,\CWout\bigr)$ for $b\in\{0,1\}$
\State \Return $(k_0,k_1)$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Exact DPF evaluation ($\DPF.\Eval$, $\DPF.\EvalAll$)}
\label{alg:eval}
\begin{algorithmic}[1]
\algstretch
\Require role $b$, key $k_b=(s_b^{(0)},b,\CW^{(1)},\ldots,\CW^{(n)},\CWout)$, query $x=x_1\cdots x_n$
\Ensure share $y_b\in\Fp$ (or all $2^n$ leaf shares for $\EvalAll$)
\Function{Eval}{$k_b,x$}
    \State $(s,t)\gets(s_b^{(0)},b)$ \Comment{root control bit $=$ role}
    \For{$i=1$ \textbf{to} $n$} \Comment{$\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$}
        \State $(s^L,t^L,s^R,t^R)\gets\PRG(s)$ \Comment{$t$: old evaluator bit}
        \State $(s^L,t^L)\gets(s^L\oplus t\cdot\sCW,\ t^L\oplus t\cdot\tCW{L})$
        \State $(s^R,t^R)\gets(s^R\oplus t\cdot\sCW,\ t^R\oplus t\cdot\tCW{R})$
        \State $(s,t)\gets(s^{L},t^{L})$ if $x_i=0$, else $(s^{R},t^{R})$
    \EndFor
    \State \Return $y_b\gets(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$
\EndFunction
\Function{EvalAll}{$k_b$}
    \State push $(s_b^{(0)},b,0,\langle\rangle)$ onto the stack \Comment{$\langle\rangle$: empty prefix}
    \While{the stack is not empty}
        \State pop $(s,t,i,\pi)$ \Comment{seed, bit, depth, prefix}
        \If{$i=n$}
            \State emit leaf $\pi$ with share $(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$
        \Else
            \State expand $s$ as in lines 4--6 with $\CW^{(i+1)}$
            \State push $(s^R,t^R,i{+}1,\pi\|1)$
            \State push $(s^L,t^L,i{+}1,\pi\|0)$ \Comment{left first}
        \EndIf
    \EndWhile
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_gac.pdf}
    \caption{Malicious-safe generate-and-consume inside module $T_b$ for a depth-2 tree. (a)~Joint generation: the two generator states $(s_0,t_0)$ and $(s_1,t_1)$ follow the target path $\alpha=01$ and emit $\CW^{(1)}$, $\CW^{(2)}$ and $\CWout$, which are consumed immediately instead of being stored as a key. (b)~Local evaluation of party $b$ on query $x=00$: a separate evaluator state $(\tilde s,\tilde t)$ follows $x$, applies each correction word at its own level, and leaves the target path at level~2, where only its own control bit $\tilde t$ is correct; grey nodes are never expanded. (c)~Leaf epilogue: the raw share $\tilde y_b$ is freshly reshared and authenticated with joint pads $\zeta,\kappa_1,\kappa_2,\kappa_3$ into the 32~B tuple $\authb{y}{b}$. The crossed-out inset is the tag-tree alternative, which needs $t=3$ extra DPF trees with payloads $\Delta_j\beta$ and four times the PRG work.}
    \label{fig:gac}
\end{figure*}

\textbf{High-level idea.}
\Cref{fig:gac}(a) shows $\Gen$ walking two states $(s_0,t_0)$ and $(s_1,t_1)$ down the target path. Since each state applies a correction only when its \emph{own} old control bit is set, exactly one of the two is corrected at each level; the corrections make the off-path states of both parties identical, so their signed outputs cancel, while $\CWout$ programs $\beta$ at the target leaf (\cref{thm:dpf-correct}). Correctness needs neither uniform targets nor computational hardness; uniform masks belong to the application protocol (\cref{sec:proto-refactor}).

\textbf{Explicit states.}
Three details that the simplified semi-honest listing~\cite{dfa2026trusted} leaves implicit are explicit in \cref{alg:gen,alg:eval}, because the malicious analysis depends on them. First, the root control bits are fixed by role, $t_0=0$ and $t_1=1$, rather than sampled, and the evaluator of party $b$ always starts from $(s_b^{(0)},b)$. Second, a key contains the \emph{initial} seed of its party, the correction words and $\CWout$; the generator's final states are never substituted for the roots. Third, the payload and the role enter only through $\CWout$ and the output sign $(-1)^b$, so both are bound inputs of the ledgered gate descriptor (\cref{sec:proto-ledger}) rather than host-supplied parameters.

\textbf{Generator versus evaluator state.}
Lines 5--6 of \cref{alg:eval} correct both children with the evaluator's own old control bit $t$. Along the target path this bit coincides with the generator's $t_b$, which invites reusing the generator's control register during generate-and-consume. The substitution is wrong as soon as the query leaves the path (level~2 in \cref{fig:gac}(b)): there the evaluator states of the two parties are identical and must apply identical corrections, whereas the generator bits $t_0$ and $t_1$ still differ, so one party would apply a correction that the other omits, and the off-path outputs would no longer cancel. Each module therefore keeps a separate evaluator state next to its two generator states (\cref{alg:gac}).

% ======================================================================
\subsection{Work Accounting}
\label{sec:analysis-work}

\begin{table*}[t]
\centering
\caption{Analytic Cost of One Single-Path DPF Gate of Depth $n$ with $t$ MAC Lanes}
\label{tab:gatecost}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llccccccc}
\hline
\textbf{Design} & \textbf{Security} & \makecell{\textbf{PRG exp.}\\\textbf{per gate}} & \makecell{\textbf{Field ops per}\\\textbf{output, party}} & \makecell{\textbf{Offline bytes}\\\textbf{per gate}} & \makecell{\textbf{Bytes into GPU}\\\textbf{per party}} & \makecell{\textbf{Extra}\\\textbf{rounds}} & \makecell{\textbf{Auth.}\\\textbf{output}} & \makecell{\textbf{Verifies}\\\textbf{evaluation}} \\
\hline
Dealer-based FSS~\cite{gupta2023sigma,jawalkar2024orca} & SH & $4n$ & 0 & $2|k|$ & $|k|$ & 0 & \xmark & \xmark \\
Trusted DFA, GaC~\cite{dfa2026trusted} & SH & $6n$ & 0 & 0 & 8 & 0 & \xmark & \xmark \\
\makecell[l]{Dealer-based FSS, tag trees\\(counting bound)} & Mal. & $4n(1+t)$ & 0 & $2(1+t)|k|$ & $(1+t)|k|$ & 1 per batch & \cmark & \cmark\ (at opening) \\
vFSS-verified keys~\cite{decastro2022vfss} & Mal.\ key gen. & $4n$ + sketch & 0 & $2|k|+O(\lambda)$ & $|k|+O(\lambda)$ & 1 (sketch) & \xmark & \xmark\ (keys only) \\
Vector-payload tree, $t$ lanes$^{\dagger}$ & Mal. & $6n+O(t)$ & $t$ adds & 0 & 32 & 1 per batch & \cmark & \cmark \\
\sys, GaC + epilogue & Mal. & $6n$ & \makecell{3 mult.\\+ 4 pads} & 0 & 32 & 1 per batch & \cmark & \cmark \\
\hline
\end{tabular}

\vspace{3pt}
\parbox{\textwidth}{\footnotesize SH: semi-honest; Mal.: malicious. $|k|$ is the byte length of one party's key. PRG expansions are summed over all parties, dealer included. Bytes into the GPU are keys loaded by a GPU evaluator or output shares delivered by a module. Mask shares and Beaver triples of the surrounding arithmetic are omitted; with authentication, each such element costs 32~B per party instead of 8~B. Rounds are counted relative to the plain masked opening that every design performs. The evaluated dealer-based malicious FSS baseline assumes \est{2.2$\times$} the semi-honest offline bytes (\cref{app:model}), below this counting bound. $^{\dagger}$One in-module tree with payload $(\beta,\Delta_1\beta,\ldots,\Delta_t\beta)$; $O(t)$ counts extra leaf-conversion blocks.}
\end{table*}

\Cref{tab:gatecost} compares one single-path DPF gate at six design points. With 128-bit seeds, one party's key holds its root seed, $n$ correction words of $128+2$ bits and $\CWout$ as one canonical 64-bit word (the root control bit is the public role), so $|k|=\lceil(128+130n+64)/8\rceil$ bytes, or 1{,}016~B for $n=61$.

\textbf{Design-point comparison.}
Trusted DFA trades $1.5\times$ the dealer's PRG work for zero key bytes: each module expands $2n$ generator states and $n$ evaluator states for its own party, so the two modules perform $6n$ expansions where a dealer and two evaluators perform $4n$. Tag trees multiply PRG work, key bytes and key I/O by $1+t$, and verified keys authenticate neither the output nor its evaluation. \sys keeps DFA's $6n$ expansions and zero key bytes and adds only three field multiplications and four pads per output and party; it cannot avoid the 32~B authenticated tuple and the check round.

\textbf{Effect of the epilogue.}
Because the epilogue (\cref{fig:gac}(c)) leaves the per-gate PRG expansion count unchanged, the estimated single-path throughput of the DPF engine drops only from \est{113} to \est{106~M~gates/s} at $n=61$ relative to semi-honest trusted DFA, whereas per-lane tag trees fall to \est{26.7~M~gates/s}; the gap to per-lane tag trees stays at \est{3.8--4.0$\times$} for $n$ between 8 and 61 (\cref{fig:dpfthr}). The drop comes mainly from the assumed pipeline efficiency (\est{0.85} vs.\ \est{0.90}; \cref{app:model}); the two extra pad blocks ($6n{+}3$ vs.\ $6n{+}1$ AES blocks per gate) cost only 0.5\%. The vector-payload tree nearly matches the epilogue's PRG count, but it widens every output correction by $t$ field elements, covers only results linear in DPF evaluations, and exports pseudorandom tag shares whose hiding rests on DPF key privacy. The epilogue instead makes every exported tuple exactly uniform for its holder (\cref{thm:epilogue}) and applies unchanged to LUT, interval, direct and PIR results.

\textbf{Remaining costs we accept.}
\sys does not remove duplicated generation: $6n$ instead of $4n$ expansions is the price of eliminating $2|k|$ network bytes and $|k|$ bytes of key I/O per gate, a favorable trade because PRG expansion is the cheapest operation in the pipeline while bytes cross its slowest links. Two further costs remain. The conservative $O(n^2)$ DCF of \cref{alg:dcf} is the only DCF our proofs cover; its interval gate costs 22{,}692 AES blocks at $n=61$, against a projected \est{976} for an optimized DCF, so the compiler chooses among direct, LUT and interval gates by modeled cost, subject to an FSS-portability constraint (\cref{sec:proto-direct,sec:eval-micro}). A host-module link of $B$ bytes/s bounds the authenticated output stream at $B/32$ elements/s, which motivates the L2-adjacent placement (\cref{sec:arch-insight}).

\textbf{Implications.}
For sources (iii) and (iv) the semi-honest lesson still holds: distribution is the largest avoidable cost (Observation~1), so DFA's local generation and generate-and-consume must stay, and FSS outputs must be authenticated without multiplying DPF work. This leaves sources (i) and (ii) as the dominant costs (Observations~2 and~3). The analysis yields five design rules that structure the rest of the paper: (1)~authenticate FSS outputs by fresh resharing inside the module, never by extra trees and never by authenticating host values (S2; \cref{sec:proto-epilogue}); (2)~keep generation local and streamed, with separate generator and evaluator states (S7; \cref{sec:proto-gac}); (3)~make the unavoidable check round sound and batchable by freezing bytes before challenges are drawn (S1, S3, S8), and release no output before \lstate{VERIFIED} (S6; \cref{sec:proto-check,sec:proto-ledger}); (4)~bind every randomness draw to one session, gate, role and use, so that local generation does not open a replay path (S4, S5; \cref{sec:proto-ledger}); and (5)~leave four-lane exact linear algebra on the GPU while the module generates correct triples (S7) and verifies openings (\cref{sec:arch-insight}).


==> qa/draft2/sections/05a_protocol.tex <==
% ======================================================================
% Section V (part 1): VIGOR-DFA Protocol Design
% Owner: 05a_protocol.tex. Continues in 05b_protocol_gates.tex.
% ======================================================================
\section{\texorpdfstring{\sys}{VIGOR-DFA} Protocol Design}\label{sec:protocol}

This section specifies the protocol run by the two parties of \ProfT: the flow (\cref{sec:proto-overview}), the representation, joint randomness and lifecycle state (\cref{sec:proto-repr,sec:proto-setup,sec:proto-ledger}), and the mechanisms that move values through the integrity chain (\cref{sec:proto-gac,sec:proto-epilogue,sec:proto-check,sec:proto-arith}). Nonlinear gates, refactoring, GPU verification and PIR follow in \cref{sec:proto-gates,sec:proto-direct,sec:proto-refactor,sec:proto-freivalds,sec:proto-pir}; formal statements are collected in \cref{sec:security}.

% ======================================================================
\subsection{Overview}\label{sec:proto-overview}

\textbf{High-level idea.}
In trusted DFA the protected module replaces the dealer: it samples FSS keys locally and consumes each correction word as soon as it produces it~\cite{dfa2026trusted}. \sys turns the module from a dealer into a dealer that also verifies. Every wire carries an authenticated sharing with $t$ information-theoretic MAC lanes. The GPU performs all linear algebra on these sharings but only ever produces \emph{candidate} shares. Each module generates every correlation of its party, authenticates every FSS output it computes, checks every opening on frozen bytes and releases nothing before verification.

\textbf{Per-gate lifecycle.}
Every gate of the public circuit $C$ fixed by the manifest $\mu$ passes through the same module commands (\cref{tab:commands}). (1)~With \cmd{RESERVE_PREP}, $T_b$ reserves the gate's randomness labels in its one-time ledger and issues party-local authenticated preprocessing (masks, triples) to host~$b$. (2)~Host $b$'s GPU computes candidate authenticated shares with local linear operations. (3)~With \cmd{FREEZE_BATCH} and \cmd{CHECK_OPEN}, the two modules freeze the submitted bytes and verify the masked openings the gate needs. (4)~For a nonlinear gate, \cmd{EVAL_FSS} consumes the verified opening, runs generate-and-consume inside $T_b$ and returns a freshly authenticated share. (5)~\cmd{FINAL_OUTPUT} hands a masked output and a bound certificate to an authorized recipient. A failure in any step triggers \cmd{ABORT}, which poisons the epoch. Each mechanism below enforces one design rule of \cref{sec:analysis-work}; \cref{tab:notation} summarizes the notation.

\begin{table}[t]
\caption{Notation used in the protocol description}
\label{tab:notation}
\centering
\footnotesize
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{p{0.27\linewidth} p{0.63\linewidth}}
\hline
\textbf{Symbol} & \textbf{Meaning} \\
\hline
$P_b$; host $b$; $T_b$ & party $b\in\{0,1\}$; its untrusted host (CPU, OS, driver, GPU, memory, NIC); its protected module \\
$\mu$, $C$ & public manifest and the finite circuit it fixes \\
$p$, $\Fp$ & Mersenne prime $2^{61}-1$ and the protocol field \\
$t$ & number of MAC lanes ($t=3$) \\
$\Delta_j$; $\Delta_{b,j}$ & global MAC key of lane $j$ (modules only); host $b$'s additive share of it \\
$\auth{x}$; $\authb{x}{b}$ & authenticated sharing of $x$; party $b$'s tuple $(x_b,\gamma_{b,1},\dots,\gamma_{b,t})$ \\
$\gamma_{b,j}$ & tag share of party $b$ in lane $j$, $\gamma_{0,j}+\gamma_{1,j}=\Delta_j x$ \\
$K$ & session key shared by $T_0$ and $T_1$ after setup \\
$\ell$ & length-prefixed label (session, epoch, gate, purpose, logical draw, block) \\
$\PRF_K(\ell,\cdot)$ & joint draw: same label, same value in both modules \\
$\nu$; $\varepsilon$; $\upsilon$ & wire index; masked input $x-r$; masked output $y+o$ \\
$\mathsf{In}_\nu$; $\mathcal{V}$ & declared interface of input wire $\nu$; validity predicates of $\mu$ \\
$n$; $\lambda$ & DPF input length in bits; PRG seed length ($\lambda=128$) \\
$\alpha$, $\beta$, $x$ & DPF target, payload in $\Fp$, verified public query \\
$\CW^{(i)}$; $\CWout$ & level-$i$ correction word; output correction \\
$(s_c,t_c)$; $(\tilde s,\tilde t)$ & generator state of root $c\in\{0,1\}$; evaluator state of $T_b$ \\
$\tilde y_b$ & raw local output of the protected evaluator \\
$\zeta$; $\kappa_j$ & fresh common epilogue pads for the value; for lane $j$ \\
$m$; $h_b$; $\mathit{cid}$ & batch size; frozen root of $T_b$; check identifier \\
$\rho_{j,i}$; $\sigma_{b,j}$ & challenge of lane $j$ at batch position $i$; residual of $T_b$ in lane $j$ \\
$\bm{e}$; $\bm{d}_j$ & value-error vector; tag-error vector of lane $j$ in a checked batch \\
$Q$ & number of checked batches in one execution \\
$w$ & LUT input width (\cref{sec:proto-gates}) \\
\hline
\end{tabular}
\end{table}

% ======================================================================
\subsection{Authenticated Representation}\label{sec:proto-repr}

\textbf{Field and MAC lanes.}
All protocol arithmetic is over $\Fp$ with the Mersenne prime $p=2^{61}-1$. The modules hold $t=3$ independent global MAC keys $\Delta_1,\Delta_2,\Delta_3\getsr\Fp$, each additively split as $\Delta_j=\Delta_{0,j}+\Delta_{1,j}$; host~$b$ holds only $\Delta_{b,j}$, which it needs to add public values to its tags. Party $b$ holds an authenticated value $\auth{x}$ as
\begin{gather*}
\authb{x}{b}=(x_b,\gamma_{b,1},\gamma_{b,2},\gamma_{b,3}),\\
x_0+x_1=x,\qquad \gamma_{0,j}+\gamma_{1,j}=\Delta_j x\quad (j\in[t]),
\end{gather*}
which is the SPDZ representation~\cite{damgard2012spdz,damgard2013practical} with three independent lanes. A canonical wire occupies four 64-bit words, i.e., 32~B per party before metadata. Every element is encoded as an unsigned 64-bit integer smaller than $p$; the module parser rejects noncanonical encodings instead of reducing arbitrary integers modulo $p$, which keeps frozen bytes and checked field elements in one-to-one correspondence.

\textbf{Why three lanes over a 61-bit field.}
The Mersenne modulus lets the GPU compute exact products of canonical elements with native 64-bit multiplies and two folding steps (\cref{sec:arch-field}), so all $1+t$ lanes of authenticated linear algebra stay on standard integer datapaths. A single 61-bit tag is too weak: for $Q\le 2^{32}$ checked batches, $t=3$ is the smallest lane count whose statistical term $Q(2/p)^t$ falls below $2^{-128}$ (\cref{sec:sec-concrete}, \cref{tab:lanes}), and every lane is paid for in GPU work (\cref{sec:eval-ablation}).

\textbf{Why a field and not $\Z_{2^{64}}$.}
The soundness proof divides by a nonzero error coordinate and therefore needs a field (\cref{sec:sec-concrete}, \cref{app:proof-auth}). The encoding is thus not bit-identical to the $\Z_{2^{64}}$ arithmetic of FSS-compiled models~\cite{gupta2023sigma,jawalkar2024orca}. \sys fixes the numeric contract in the manifest (fixed-point scale, signed encoding, exact toward-zero truncation of \cref{sec:proto-gates}, magnitudes below $p/2$); a deployment that needs ring semantics must use a SPDZ2k-type backend~\cite{cramer2018spdz2k} with its own proof.

% ======================================================================
\subsection{Session Setup and Joint Randomness}\label{sec:proto-setup}

\textbf{Session setup.}
Each module authenticates its peer's identity, code and configuration measurement, role and freshness contribution. An authenticated key establishment then binds the ordered pair of identities, the roles 0 and 1, a fresh session identifier, the epoch, the manifest hash $\Hash(\mu)$, the field and tag parameters and the protocol version, and yields the session key $K$ known only to $T_0$ and $T_1$. Any failure aborts. We treat this step as an explicit setup assumption with error $\eps{setup}$ (\cref{thm:main}) and propose no new attestation protocol; attestation certifies what runs inside a module, not what the GPU computes (\cref{sec:bg-dfa}).

\textbf{Labels and joint draws.}
All module randomness is derived as $\PRF_K(\ell)$, or with an equivalent KDF~\cite{krawczyk2010hkdf}, where $\ell$ is an unambiguous, length-prefixed encoding of $(\mathsf{session},\mathsf{epoch},\mathsf{gate},\mathsf{purpose},\mathsf{logical\_draw},\mathsf{block})$. A \emph{logical joint draw} uses the same label in both modules and thus yields the same value in $T_0$ and $T_1$ without communication; this is how both modules obtain identical DPF roots, correction words, masks, triples, pads and challenges. Distinct roots, pads, triple components, challenge lanes and rejection-sampling retries receive distinct labels. Two rules are easy to get wrong. The local role must \emph{not} be appended to a joint draw, since $T_0$ and $T_1$ would then generate two unrelated DPF instances whose outputs no longer add up; and the logical root-0 and root-1 draws of one DPF \emph{must} be different draws. Since labels name session, epoch and gate, the ledger detects replayed or misrouted material (S4, S5). A uniform element of $\Fp$ is obtained by rejection sampling: take 61 pseudorandom bits and reject the single value $p$, which occurs with probability $2^{-61}$; a bounded implementation aborts when its retry budget is exhausted instead of introducing a silent bias.

\textbf{Authenticated correlations.}
To share a protected value $v$, the joint sampler runs \AuthShare{}: it samples $v_0\getsr\Fp$ and sets $v_1=v-v_0$, independently samples $\gamma_{0,j}\getsr\Fp$ and sets $\gamma_{1,j}=\Delta_j v-\gamma_{0,j}$ for $j\in[t]$, and gives party $b$ only its tuple $\authb{v}{b}$. A multiplication triple samples $a,b\getsr\Fp$, computes $c=ab$ \emph{correctly inside the protected boundary} and authenticates all three values independently (S7); a matrix triple satisfies the actual equality $C=AB$ for its declared dimensions. Because both modules derive the same correlations from joint labels, preprocessing crosses no network link.

% ======================================================================
\subsection{One-Time Ledger and Release Guard}\label{sec:proto-ledger}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_ledger.pdf}
    \caption{Per-gate lifecycle enforced by the one-time ledger of $T_b$. Solid arrows are the only permitted transitions, each triggered by the named module command (\cref{tab:commands}). An accepted \cmd{CHECK_OPEN} only sets \lstate{VERIFIED}; \cmd{EVAL_FSS} consumes the opening of an FSS or direct gate, and an output gate, which runs no \cmd{EVAL_FSS}, is moved by \cmd{FINAL_OUTPUT} through \lstate{CONSUMED} to \lstate{RELEASED}. Any other transition or any failed check moves the gate to \lstate{ABORTED}, poisons the epoch and keeps the release guard closed.}
    \label{fig:ledger}
\end{figure}

\textbf{Ledger states.}
Each module keeps an authoritative protected ledger that binds every gate to its operation, predecessor and output wires, numeric type, table or model hash, public dimensions and allowed command sequence. A gate transaction moves only along
\lstate{NEW} $\rightarrow$ \lstate{RESERVED} $\rightarrow$ \lstate{PREPARED} $\rightarrow$ \lstate{FROZEN} $\rightarrow$ \lstate{VERIFIED} $\rightarrow$ \lstate{CONSUMED} $\rightarrow$ \lstate{RELEASED}
(\cref{fig:ledger}). Reservation burns the gate's randomness identifiers \emph{before} any preprocessing share is issued, so no label is ever issued twice. \lstate{PREPARED} lets the module issue the authorized party-local preprocessing exactly once; it is not permission to release an unchecked result. \lstate{CONSUMED} records the one-time use of verified openings and preprocessing, and \lstate{RELEASED} records that the result left the module under a certificate. Any invalid transition or failed check moves the gate to \lstate{ABORTED} and poisons the whole epoch: outstanding output responses are gated, no new challenge is derived, and aborted reservations never return to a free list.

\textbf{Freeze semantics.}
Before any checking challenge is drawn, $T_b$ copies the exact submitted value and tag bytes into protected storage, or spills them into AEAD-protected immutable pages~\cite{dworkin2007gcm} bound to sequence numbers, exact lengths, gate identifiers and a protected root. It hashes the complete descriptor and these bytes into a frozen root $h_b$, and the two modules agree on the ordered pair $(h_0,h_1)$. A host's claim that ``this buffer has hash $h$'' is not a freeze, and neither is DMA completion. After challenge generation, $T_b$ rereads only authenticated frozen pages and never verifies one buffer but consumes a later, host-modified one. This closes the time-of-check-to-time-of-use window (S3) that exists whenever checked data live in host or GPU memory.

\textbf{Release certificates and the guard.}
A release certificate binds the session, epoch, gate, recipients, output encoding or hash and terminal status. A missing peer acknowledgement can cause an abort, but it never authorizes output under a different transcript. The release guard is a small state machine in front of the module's output path (\cref{sec:arch-hw}); its enabling inputs originate from the protected checkers and the ledger, never from host-writable registers, so a host cannot open it by writing a status bit (S6). Resetting the guard is not a secure session reset.

\textbf{Reboot and rollback.}
After a reboot, either a separately justified trusted monotonic service preserves freshness~\cite{parno2011memoir,matetic2017rote}, or the old master key is irrecoverably erased and a freshly attested session is required. A host-controlled counter file is not anti-rollback protection, because the host can restore an old copy and replay old masks (S4).

% ======================================================================
\subsection{Malicious Generate-and-Consume}\label{sec:proto-gac}

\textbf{From semi-honest to malicious GaC.}
\Cref{alg:gac} interleaves \cref{alg:gen,alg:eval} with the three separate states of \cref{sec:analysis-dpf}: two generator states on the target path, started from $t_0=0$ and $t_1=1$, and an evaluator state on the query path, started from its own root seed and the fixed control bit $b$, never from a later generator state. Each correction word is computed from the expanded children of the two generator seeds and the target bit $\alpha_i$, applied to the generator states under their old bits $t_c$ and to both evaluator children under the evaluator's old bit $\tilde t$, and erased only after that use; $t\cdot s$ denotes a conditional XOR. The hardware keeps the two state sets in distinct contexts (\cref{sec:arch-pipe}), and the per-level work, which still duplicates generation in both modules, is accounted in \cref{tab:gatecost}.

\textbf{Inputs and outputs.}
The query $x$ is read from a verified masked opening of the same gate, never from unchecked host data: for instance the opened $c$ of an interval gate, whose prefix DPFs are queried at $c$ (\cref{alg:interval,alg:dcf}), whereas in a LUT gate the opened $u$ only permutes the table index while $\EvalAll$ visits every $a$ (\cref{alg:lut}). The target $\alpha$ and payload $\beta$ come from the gate's protected preprocessing record, so they are joint draws or joint functions of joint draws (\cref{sec:proto-refactor}). By \cref{thm:dpf-correct,thm:gac}, the raw outputs satisfy $\tilde y_0+\tilde y_1=\beta\cdot\one[x=\alpha]$, but $\tilde y_b$ never leaves the module: the epilogue lines of \cref{alg:gac} replace it with a freshly authenticated tuple. Since neither keys nor raw shares are exported, \cref{thm:main} needs no DPF key-privacy term. Gates that combine several DPF evaluations (interval prefixes, LUT and PIR scans) run only the (Gen) and (Eval) lines per constituent DPF and apply the ledger lines and one epilogue to their combined raw share, for PIR only its value pad (\cref{app:proof-dpf}). For full-domain uses such as LUT gates and PIR, the evaluator lines become the depth-first $\EvalAll$ traversal of \cref{alg:eval}; each $\CW^{(i)}$ then stays in protected registers until its last evaluator use, which costs $O(n)$ words and is covered by the same node-by-node coupling.

\begin{algorithm}[t]
\algstretch
\small
\caption{Malicious generate-and-consume with fresh authentication (\algname{GaC-Auth}) inside $T_b$}
\label{alg:gac}
\begin{algorithmic}[1]
\Require role $b\in\{0,1\}$; gate label $\ell$; public query $x\in\bits{n}$ from the gate's frozen, verified opening; target $\alpha\in\bits{n}$ and payload $\beta\in\Fp$ from the protected record of $\ell$; session key $K$; global keys $\Delta_1,\dots,\Delta_t$
\Ensure $\authb{y}{b}=(y_b,\gamma_{b,1},\dots,\gamma_{b,t})$ with $y_0+y_1=\beta\cdot\one[x=\alpha]$ and $\gamma_{0,j}+\gamma_{1,j}=\Delta_j(y_0+y_1)$
\If{gate $\ell$ is not \lstate{VERIFIED} in the ledger}
  \State \Abort{} and poison the epoch
\EndIf
\LineComment{Joint draws: identical labels in $T_0$ and $T_1$, no role appended}
\State $s_0\gets\PRF_K(\ell,\mathsf{root}_0)$;\ $s_1\gets\PRF_K(\ell,\mathsf{root}_1)$;\ $t_0\gets 0$;\ $t_1\gets 1$
\State $(\tilde s,\tilde t)\gets(s_b,b)$ \Comment{separate evaluator}
\For{$i=1$ \textbf{to} $n$}
  \LineComment{(Gen) both roots on the target path; updates use the old $t_c$}
  \State $(s_c^L,t_c^L,s_c^R,t_c^R)\gets\PRG(s_c)$ for $c\in\{0,1\}$
  \State $a\gets\alpha_i$;\ $\keep\gets a$;\ $\lose\gets 1-a$ \Comment{$L\equiv 0$, $R\equiv 1$}
  \State $\sCW\gets s_0^{\lose}\oplus s_1^{\lose}$
  \State $\tCW{L}\gets t_0^L\oplus t_1^L\oplus a\oplus 1$;\ \ $\tCW{R}\gets t_0^R\oplus t_1^R\oplus a$
  \State $(s_c,t_c)\gets\big(s_c^{\keep}\oplus t_c\cdot\sCW,\ t_c^{\keep}\oplus t_c\cdot\tCW{\keep}\big)$, $c\in\{0,1\}$
  \LineComment{(Eval) own query path; corrections use the old $\tilde t$}
  \State $(\hat s^L,\hat t^L,\hat s^R,\hat t^R)\gets\PRG(\tilde s)$
  \State $(\hat s^L,\hat t^L)\gets\big(\hat s^L\oplus\tilde t\cdot\sCW,\ \hat t^L\oplus\tilde t\cdot\tCW{L}\big)$
  \State $(\hat s^R,\hat t^R)\gets\big(\hat s^R\oplus\tilde t\cdot\sCW,\ \hat t^R\oplus\tilde t\cdot\tCW{R}\big)$
  \State $(\tilde s,\tilde t)\gets(\hat s^{x_i},\hat t^{x_i})$
  \State erase $\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$ \Comment{after its evaluator use}
\EndFor
\LineComment{(Gen) output correction from the final generator states}
\State $u_c\gets\Conv(s_c)$ for $c\in\{0,1\}$;\ \ $\CWout\gets(-1)^{t_1}(\beta-u_0+u_1)$
\LineComment{(Eval) raw share, never exported}
\State $\tilde y_b\gets(-1)^b\big(\Conv(\tilde s)+\tilde t\cdot\CWout\big)$; erase $s_c$, $t_c$, $\CWout$
\LineComment{(Epilogue) fresh uniform pads, distinct labels per output wire}
\State $\zeta\gets\PRF_K(\ell,\mathsf{pad}_0)$;\ \ $\kappa_j\gets\PRF_K(\ell,\mathsf{pad}_j)$ for $j\in[t]$
\State $y_b\gets\tilde y_b+(-1)^b\zeta$
\State $\gamma_{b,j}\gets\Delta_j\,y_b+(-1)^b\kappa_j$ for $j\in[t]$
\State mark $\ell$ \lstate{CONSUMED}; erase $\tilde y_b$, $\zeta$, $\kappa_1,\dots,\kappa_t$, $(\tilde s,\tilde t)$
\State \Return $\authb{y}{b}$ to the output FIFO behind the release guard
\end{algorithmic}
\end{algorithm}

% ======================================================================
\subsection{Fresh Authentication Epilogue}\label{sec:proto-epilogue}

\textbf{Construction.}
Let $\tilde y_0,\tilde y_1$ be raw local shares computed inside the two protected evaluators, with $\tilde y_0+\tilde y_1$ equal to the intended gate value. Both modules derive fresh common pads $\zeta,\kappa_1,\dots,\kappa_t\getsr\Fp$ from joint labels that are distinct for every output wire, and $T_b$ returns
\begin{equation*}
y_b=\tilde y_b+(-1)^b\zeta,\qquad \gamma_{b,j}=\Delta_j\,y_b+(-1)^b\kappa_j\quad (j\in[t]).
\end{equation*}
The pads cancel in $y_0+y_1$ and in $\gamma_{0,j}+\gamma_{1,j}=\Delta_j(y_0+y_1)$, so the result is an authenticated sharing of $\tilde y_0+\tilde y_1$, and each party's tuple is uniform on $\Fp^{1+t}$ whatever the gate value and the global keys (\cref{thm:epilogue}). Fresh pads make this hold jointly across outputs; correlations created by later arithmetic are handled by the circuit simulation of \cref{thm:main}.

\textbf{Why it replaces tag trees.}
Instead of $t$ further DPF trees with payloads $\Delta_j\beta$, the epilogue exploits the linearity of the MAC. Because $T_b$ knows the global $\Delta_j$, the tag of the reconstructed value is the sum of the per-party products $\Delta_j y_b$; the pad $\kappa_j$ hides $\Delta_j y_b$ from host $b$, which knows $y_b$ and could otherwise divide it out. The pad $\zeta$ rerandomizes the raw DPF share, so no host ever sees $\tilde y_b$. The cost is one raw DPF computation, three field multiplications and four fresh pads per party and output, and the output is a 32~B tuple.

\textbf{API restriction.}
The epilogue accepts only results computed inside the module, namely the DPF, DCF, LUT, interval and direct gates of \cref{sec:proto-gates,sec:proto-direct} and the PIR reductions of \cref{sec:proto-pir}, or results from an explicitly verified backend such as the frozen-operand Freivalds check of \cref{sec:proto-freivalds}. There is no \cmd{authenticate(host_value)} entry point. With one, the module would become a MAC oracle: a malicious host could obtain valid tags on any value it wishes to open, and \CheckOpen{} would accept the forgery with probability one (S2). Since the trusted boundary excludes the GPU SMs and memory, a malicious-secure extension must never compute an unchecked result on the GPU and ask the module to authenticate it.

% ======================================================================
\subsection{Freeze-Before-Challenge CheckOpen}\label{sec:proto-check}

\begin{algorithm}[t]
\algstretch
\small
\caption{Freeze-before-challenge authenticated opening (\CheckOpen) inside $T_b$}
\label{alg:checkopen}
\begin{algorithmic}[1]
\Require descriptor and nonempty ordered list of expected wires $(\nu_i)_{i\in[m]}$; host $b$'s tuples $(x_{b,i},\gamma_{b,j,i})_{i\in[m],\,j\in[t]}$; key shares $(\Delta_{b,j})_{j\in[t]}$
\Ensure verified openings $(z_i)_{i\in[m]}$ with bound certificates, or \Abort
\If{metadata, field encoding, gate order or length mismatch the ledger}
  \State \Abort{} and poison the epoch
\EndIf
\LineComment{Step 1: freeze, then agree on both roots}
\State copy the exact bytes into protected SRAM or sealed AEAD pages; $h_b\gets\Hash(\text{descriptor},\text{frozen bytes})$; mark \lstate{FROZEN}
\State exchange $(h_b,\mathit{cid})$ with $T_{1-b}$; \Abort{} unless both hold the same $(h_0,h_1)$ and $\mathit{cid}$
\LineComment{Step 2: reconstruct candidates inside the modules}
\State exchange the frozen value shares $(x_{b,i})_{i\in[m]}$ with $T_{1-b}$
\State $z_i\gets x_{0,i}+x_{1,i}$ for $i\in[m]$ \Comment{not exposed to the host}
\LineComment{Step 3: internal challenges, only after both freezes}
\State $\rho_{j,i}\gets\PRF_K(\mathsf{chk},h_0,h_1,\mathit{cid},j,i)$ for $j\in[t]$, $i\in[m]$
\LineComment{Step 4: per-lane residuals from frozen pages only}
\State $\sigma_{b,j}\gets\sum_{i=1}^{m}\rho_{j,i}\,(\gamma_{b,j,i}-\Delta_{b,j}z_i)$ for $j\in[t]$
\State exchange $(\sigma_{b,j})_{j\in[t]}$ with $T_{1-b}$
\LineComment{Step 5: decide and release}
\If{$\sigma_{0,j}+\sigma_{1,j}=0$ for every $j\in[t]$}
  \State agree on output digest and status; mark \lstate{VERIFIED}; record the checked material as used
  \State \Return $(z_i)_{i\in[m]}$ with certificates bound to session, epoch, gates and output hash
\Else
  \State release no candidate value; poison the epoch; return one generic failure status
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_checkopen.pdf}
    \caption{Freeze-before-challenge \CheckOpen{} between the two modules. Challenges $\rho_{j,i}$ are derived only after both frozen roots are agreed, and $T_b$ rereads only its frozen pages, so a host that overwrites its DMA buffer after the freeze changes nothing that is checked or consumed.}
    \label{fig:checkopen}
\end{figure}

\textbf{Role.}
Openings are the only places where a value produced by the untrusted GPU becomes public or feeds a protected gate: the masked differences of every multiplication, the masked inputs of every FSS gate and the masked outputs. \CheckOpen{} (\cref{alg:checkopen}, \cref{fig:checkopen}) is a SPDZ-style batched MAC check~\cite{damgard2012spdz,damgard2013practical} rebuilt for a verifier that reads its inputs from untrusted memory (S1, S3). All peer messages use the protected channel, and only an accepted batch releases $z$ with bound certificates.

\textbf{Independent challenge lanes.}
Let $\bm{e}$ be the value-error vector of a batch and $\bm{d}_j$ its tag-error vector in lane $j$, i.e., the differences between the submitted and the prescribed tuples. The freeze fixes $(\bm{e},\bm{d}_j)$ before any $\rho_{j,i}$ exists, so a host cannot place its errors in the kernel of a challenge (\cref{app:proof-auth}). Each lane has its own challenge vector $\bm{\rho}_j$. The complete residual of lane $j$ is $\inner{\bm{\rho}_j}{\bm{d}_j-\Delta_j\bm{e}}$, which for $\bm{e}\neq\bm{0}$ vanishes with probability below $2/p$; independence across lanes multiplies these bounds to $(2/p)^t$ (\cref{thm:mac-sound}). A shared vector collapses the product to one lane, and tag-only errors escape with probability $1/p$ without changing an opened value (\cref{sec:sec-concrete}, \cref{app:proof-auth}).

\textbf{Key hiding and failure handling.}
The bound relies on the hidden-key invariant of \cref{lem:hidden-key}: until the first accepted wrong opening, the honest key shares stay uniform given the corrupt host's view. \CheckOpen{} preserves it in three ways. Candidates, challenges and residuals never leave the modules. The zero tests of all lanes are aggregated into one generic failure status that exposes no residual, challenge, key or data-dependent diagnostic. A failure poisons the epoch and forbids retries with the same material, which rules out an adaptive key-learning sequence within an epoch.

\textbf{Traffic and batching.}
Per batch of $m$ elements, the modules exchange two vectors of $m$ field values and two vectors of $t$ residuals plus authenticated metadata. Tags never cross the peer link, but every local tag must be read by its module, so the host-to-module transfer of 32~B per element can remain the bottleneck (\cref{sec:arch-dse}). Because the value shares are frozen before they are sent, root agreement and value exchange can share one message, and our latency model charges two peer round trips per batch. Only independent openings are batched: a dependent nonlinear gate never consumes an unchecked masked opening, and a checkpoint precedes every input-dependent nonlinear output and every final release, since blindly delayed checking is not justified. Larger batches amortize metadata and round trips but increase staging memory and first-result latency (costs in \cref{sec:eval-check}).

% ======================================================================
\subsection{Inputs, Arithmetic, and Outputs}\label{sec:proto-arith}

\begin{figure*}[t]
\centering
\footnotesize
\setlength{\fboxsep}{4pt}
\fbox{%
\begin{minipage}[t]{0.472\textwidth}
\textbf{Input} $\Pi_{\mathsf{Input}}$\hfill\textit{input $x$ of endpoint $O$ for wire $\nu$}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: reserve label $\ell_\nu$; joint draw $r\getsr\Fp$ and $\authb{r}{b}\gets\AuthShare(r)$; issue $\authb{r}{b}$ to host $b$ once.
\item $T_0,T_1$: send the complete $r$ only to $O$ over its authenticated confidential channel.
\item $O$: send the canonical, authenticated $\varepsilon=x-r$ to $T_0$ and $T_1$.
\item $T_0,T_1$: confirm over the protected channel that both hold the same $\varepsilon$ and bind it to $\nu$; compute $x^*=r+\varepsilon$ and \Abort{} unless $x^*\in\mathsf{In}_\nu$. $T_b$ then hands the bound $\varepsilon$ to host $b$.
\item host $b$: $x_b\gets r_b+\one[b=0]\,\varepsilon$;\ \ $\gamma_{b,j}\gets\gamma_{r,b,j}+\Delta_{b,j}\,\varepsilon$ for $j\in[t]$.
\end{enumerate}
\textit{Extraction:} a corrupt owner's input is $x^*=r+\varepsilon$.
\textit{Validation:} at the public boundaries declared in $\mu$, all before the first output opening, $T_0,T_1$ evaluate every predicate of $\mathcal{V}$ on the bound inputs and \Abort{} if one fails.
\textit{Committed inputs:} a protected loader verifies the authorized commitment over the frozen canonical stream, then runs \AuthShare{} on the exactly decoded values.

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Linear} $\Pi_{\mathsf{Lin}}$\hfill\textit{local, on host $b$'s GPU}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $\auth{x}+\auth{y}$: add the value shares and each of the $t$ tag shares.
\item $c\cdot\auth{x}$ for public $c$: multiply the value share and every tag share by $c$.
\item $\auth{x}+c$ for public $c$: $x_0\gets x_0+c$ (party~0 only); $\gamma_{b,j}\gets\gamma_{b,j}+\Delta_{b,j}\,c$ for both $b$ and all $j\in[t]$.
\item Tensors: apply steps 1 to 3 elementwise to the value array and to each of the $t$ tag arrays.
\end{enumerate}

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Output} $\Pi_{\mathsf{Out}}$\hfill\textit{private output $y$ for client $O$}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: joint draw a fresh $\auth{o}$ as in step 1 of $\Pi_{\mathsf{Input}}$; send the complete $o$ only to $O$.
\item host $b$: $\auth{\upsilon}\gets\auth{y}+\auth{o}$ with $\Pi_{\mathsf{Lin}}$.
\item $\upsilon\gets\CheckOpen(\auth{\upsilon})$; the release guard opens only for a \mbox{\lstate{VERIFIED}} batch.
\item $T_b$: send $\upsilon$ and its release certificate (session, epoch, gate, recipients, output hash, status) to $O$.
\item $O$: verify both certificates for the same $\upsilon$ and output $y=\upsilon-o$; otherwise abort.
\end{enumerate}
\textit{Public outputs:} $y\gets\CheckOpen(\auth{y})$.
\textit{Never} hand $O$ both parties' tags: $\gamma_{0,j}+\gamma_{1,j}=\Delta_j y$ with a known $y\neq 0$ reveals $\Delta_j$.
\end{minipage}%
\hspace{0.01\textwidth}\vrule\hspace{0.01\textwidth}%
\begin{minipage}[t]{0.472\textwidth}
\textbf{Multiplication} $\Pi_{\mathsf{Mult}}$\hfill\textit{authenticated Beaver triples}

\textit{Scalar} $\auth{z}=\auth{x}\cdot\auth{y}$:
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: reserve a fresh triple $(\auth{a},\auth{b},\auth{c})$ from joint draws, with $c=ab$ computed inside the protected boundary; issue party $b$'s tuples to host $b$ once.
\item host $b$: $\auth{d}\gets\auth{x}-\auth{a}$ and $\auth{e}\gets\auth{y}-\auth{b}$ with $\Pi_{\mathsf{Lin}}$.
\item $(d,e)\gets\CheckOpen(\auth{d},\auth{e})$, batched with the independent openings of the layer.
\item host $b$: $z_b\gets c_b+d\,b_b+e\,a_b+\one[b=0]\,de$.
\item host $b$: $\gamma_{z,b,j}\gets\gamma_{c,b,j}+d\,\gamma_{b,b,j}+e\,\gamma_{a,b,j}+\Delta_{b,j}\,de$ for $j\in[t]$.
\end{enumerate}
\textit{Matrix} $\auth{Z}=\auth{X}\auth{Y}$ with declared dimensions:
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep,start=6]
\item $T_0,T_1$: reserve $(\auth{A},\auth{B},\auth{C})$ with $C=AB$ computed inside the protected boundary; never expose both $A$ and $B$ to a GPU.
\item $D\gets\CheckOpen(\auth{X}-\auth{A})$;\ \ $E\gets\CheckOpen(\auth{Y}-\auth{B})$.
\item host $b$: $Z_b\gets C_b+D\,B_b+A_b\,E+\one[b=0]\,DE$.
\item host $b$: $\Gamma_{Z,b,j}\gets\Gamma_{C,b,j}+D\,\Gamma_{B,b,j}+\Gamma_{A,b,j}\,E+\Delta_{b,j}\,DE$ for $j\in[t]$, preserving the order of every matrix factor.
\end{enumerate}
\textit{Notation:} in $b_b$ and $\gamma_{b,b,j}$ the first $b$ names the triple's second component and the subscript names the party (implementations use named fields); $\Gamma_{\cdot,b,j}$ is party $b$'s lane-$j$ tag matrix.

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Invariants shared by all four protocols}
\begin{itemize}[leftmargin=1.1em,nosep]
\item Every mask and triple is a one-time joint draw bound to session, epoch, gate and purpose, and is issued only from \mbox{\lstate{PREPARED}} (\cref{fig:ledger}).
\item Every opening is a \CheckOpen{} call on frozen bytes (\cref{alg:checkopen}); no opened value feeds a protected gate or a release before it is \mbox{\lstate{VERIFIED}}.
\item Outputs of host $b$'s GPU are candidate shares; no module ever authenticates them.
\end{itemize}
\end{minipage}}
\caption{Authenticated input, linear, multiplication and output protocols of \sys, written for party $P_b$. Steps labeled $T_0,T_1$ or $T_b$ run inside the protected modules; steps labeled host $b$ run on the untrusted GPU and yield only candidate shares until the next \CheckOpen. With honest messages the protocols realize their operations exactly; otherwise they select an allowed input, preserve the computation or abort, except with the probability bounded in \cref{thm:mac-sound} (\cref{thm:arith}).}
\label{fig:arith}
\end{figure*}

\Cref{fig:arith} specifies the four protocols that carry values between input owners, GPUs, modules and recipients; three points of rationale are not visible in the box.

\textbf{Inputs.}
The difference $\varepsilon$ is uniform for a uniform $r$, so the hosts learn nothing about $x$. Both modules bind one $\varepsilon$, so a corrupt owner cannot feed the two parties different inputs, and its input is extracted as $x^*=r+\varepsilon$ (S9, \cref{def:security}). Canonical encoding alone does not place $x^*$ in the declared interface; since the modules generated $r$, they compute $x^*$ and abort unless $x^*\in\mathsf{In}_\nu$. The validity predicates $\mathcal{V}$ of $\mu$ are evaluated inside the modules at public boundaries that the schedule of $\mu$ places, like every input gate, before the first output opening; their accept or abort outcome is the $\mathsf{status}$ component of $\Leak_C$ (\cref{def:leakage}), and the simulator emulates the same abort (\cref{thm:main}). For committed inputs such as preapproved model weights, a host-declared hash does not suffice; the loader hashes exactly the bytes it shares. The modules thus see every input, which \ProfT permits (\cref{sec:threat-model}).

\textbf{Arithmetic.}
Multiplication follows Beaver~\cite{beaver1991efficient} with authenticated triples. An authenticated matrix product costs the GPU $2(1+t)$ plain products plus the public $DE$, which is why authenticated linear algebra, rather than DPF evaluation, dominates the malicious cost (\cref{sec:analysis-cost}).

\textbf{Outputs.}
The recipient accepts $\upsilon$ only with matching certificates from both modules, so integrity toward a client comes from these certificates, never from MAC tags.


==> qa/draft2/sections/05b_protocol_gates.tex <==
% ==================================================================
% Section V (part 2): authenticated nonlinear gates, direct gates and
% compilation, refactoring, verified GPU products, snapshot PIR.
% Continues the Section opened in 05a_protocol.tex (no \section here).
% ==================================================================

\subsection{Authenticated Nonlinear Gates}\label{sec:proto-gates}

Nonlinear layers of FSS-compiled models reduce to lookups in small public tables and piecewise functions selected by interval tests~\cite{boyle2021function,gupta2023sigma,jawalkar2024orca}. In the semi-honest DFA design, both parties evaluate a DPF or DCF key on a masked input and pass the raw output shares onward~\cite{dfa2026trusted}. A malicious host can shift the masked input before it selects the DPF path, and it can modify the raw outputs, which carry no MAC. \sys closes both gaps with one template (\cref{fig:gates}): (1)~mask the authenticated input with joint protected randomness (\cref{sec:proto-setup}); (2)~open the masked value with \CheckOpen{} (\cref{alg:checkopen}), so the value that selects the path is verified and frozen; (3)~evaluate the FSS gate inside $T_b$ with the (Gen) and (Eval) steps of generate-and-consume (\cref{alg:gac}); and (4)~authenticate and reshare the gate's combined raw share with one epilogue (\cref{sec:proto-epilogue}). The host sees only a uniform masked opening and fresh authenticated tuples, and no host-supplied value is ever authenticated, which defeats scenario S2 (\cref{tab:scenarios}).

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_gates.pdf}
    \caption{Authenticated nonlinear gates in \sys. (a)~Small XOR-masked LUT (\cref{alg:lut}): the XOR-masked bit vector $u$ is opened by \CheckOpen{} and $T_b$ scans the full public domain in a fixed order. (b)~Shifted-interval indicator and Horner polynomial (\cref{alg:interval}): one field opening $c=x+r$ serves both translated thresholds $L$ and $H$, which derive from the same mask. (c)~Direct protected gate (\cref{sec:proto-direct}): the module recovers $x=c-r$ inside its boundary and returns a fresh sharing of $g(x)$. In all three cases the host submits only authenticated shares and receives only freshly authenticated outputs; raw FSS shares, DPF keys and, in (c), the plaintext $x$ never leave $T_b$.}
    \label{fig:gates}
\end{figure*}

\begin{algorithm}[t]
\algstretch
\caption{Authenticated small XOR-masked LUT (\algname{LUT-Auth}) for party $b$}
\label{alg:lut}
\begin{algorithmic}[1]
\Require authenticated bits $\authb{x_1}{b},\dots,\authb{x_w}{b}$ of an unsigned $w$-bit $x$, certified Boolean; approved public table $T\in\Fp^{2^w}$ bound in $\mu$ by its hash; gate identifier $\mathit{gid}$; role $b$
\Ensure $\authb{y}{b}$ with $y=T[x]$
\State $T_b$: \cmd{RESERVE_PREP} for $\mathit{gid}$; \Abort{} on any descriptor or table-hash mismatch
\LineComment{Joint preparation inside $T_b$ (same $r$ in $T_0$ and $T_1$)}
\State $r\getsr\bits{w}$ by one joint draw with label $(\mathit{gid},\textsf{mask})$
\State issue $\authb{r_i}{b}\gets\AuthShare(r_i)$ to host $b$ once, for $i=1,\dots,w$
\State bind the joint DPF generator of $(\alpha,\beta)=(r,1)$ to $\mathit{gid}$ \Comment{never resampled}
\LineComment{Masked opening (host $b$ with $T_b$)}
\For{$i=1$ \textbf{to} $w$} \Comment{independent: one batch}
  \State $\authb{u_i}{b}\gets\authb{x_i}{b}+\authb{r_i}{b}-2\,\authb{x_ir_i}{b}$ \Comment{$\Pi_{\mathsf{Mult}}$}
\EndFor
\State $u\gets\CheckOpen(\auth{u_1},\dots,\auth{u_w})$ \Comment{$u=x\oplus r$}
\If{some $u_i\notin\{0,1\}$ or $T_0,T_1$ hold different $u$}
  \State \Abort
\EndIf
\LineComment{Full-domain scan inside $T_b$ in fixed public order; $k_b$ is streamed by GaC and never materialized}
\State $\tilde y_b\gets 0$
\For{$a\in\bits{w}$ in lexicographic order} \Comment{$\EvalAll$, DFS}
  \State $\tilde y_b\gets\tilde y_b+T[a\oplus u]\cdot\DPF.\Eval(k_b,a)$
\EndFor
\State $\authb{y}{b}\gets\Epilogue(\tilde y_b)$ \Comment{\cref{sec:proto-epilogue}}
\State \Return $\authb{y}{b}$
\end{algorithmic}
\end{algorithm}

\textbf{Small XOR-masked LUT.}
\Cref{alg:lut} evaluates an approved public table $T$ with $2^w$ field entries on a $w$-bit input given as authenticated, certified-Boolean bits. The sampler draws a fresh uniform $r\in\bits{w}$ once and uses it twice: for the authenticated bits $\auth{r_i}$ and as the target of the joint DPF for $(r,1)$. The parties open $u=x\oplus r$ in one \CheckOpen{} batch, both modules reject a non-Boolean or mismatching vector, and $T_b$ scans the full domain in a declared fixed order,
\begin{equation*}
    \tilde y_b=\sum_{a\in\bits{w}}T[a\oplus u]\cdot\DPF.\Eval(k_b,a).
\end{equation*}
By \cref{thm:dpf-correct}, the evaluations sum to one only at $a=r$, so $\tilde y_0+\tilde y_1=T[r\oplus u]=T[x]$; since XOR with a fixed $x$ is a bijection on $w$-bit strings, $u$ is uniform given $x$ (\cref{thm:lut}). In $\EvalAll$ mode the $w$ correction words stay in protected registers until their level is fully expanded, so no key is materialized outside $T_b$. Besides the $w$ XOR products (one batched multiplication round when the bits exist; otherwise bit decomposition is charged to the gate), the gate needs one batched opening, $2^w-1$ internal tree expansions and a $2^w$-term field reduction: small tables are practical, full-domain tables over 64-bit inputs are not (\cref{tab:gates}).

\begin{algorithm}[t]
\algstretch
\caption{Authenticated shifted intervals and piecewise polynomial (\algname{Interval-Auth}) for party $b$}
\label{alg:interval}
\begin{algorithmic}[1]
\Require $\authb{x}{b}$; public breakpoints $0=\tau_0<\tau_1<\dots<\tau_m=p$ with $m\ge2$; public coefficients $a_{i,j}\in\Fp$ of $P_i(x)=\sum_{j=0}^{d}a_{i,j}x^j$; gate identifier $\mathit{gid}$; role $b$
\Ensure $\authb{y}{b}$ with $y=P_i(x)$ for the unique $i$ such that $\tau_i\le x<\tau_{i+1}$
\State $T_b$: \cmd{RESERVE_PREP} for $\mathit{gid}$; $r\getsr\Fp$ by one joint draw (rejection sampling); issue $\authb{r}{b}\gets\AuthShare(r)$ once
\State $c\gets\CheckOpen(\auth{x}+\auth{r})$ \Comment{$c=x+r\bmod p$}
\LineComment{Indicators inside $T_b$; every endpoint and wrap bit derives from the same $r$}
\For{$i=0$ \textbf{to} $m-1$}
  \State $L_i\gets(\tau_i+r)\bmod p$;\; $H_i\gets(\tau_{i+1}+r)\bmod p$
  \State $\omega_i\gets\one[L_i>H_i]$ with a sharing $(\omega_{i,0},\omega_{i,1})$
  \State $\tilde s_{i,b}\gets\omega_{i,b}+\DCF_{H_i}(c)_b-\DCF_{L_i}(c)_b$ \Comment{GaC}
  \State $\authb{s_i}{b}\gets\Epilogue(\tilde s_{i,b})$ \Comment{$s_i=\one[\tau_i\le x<\tau_{i+1}]$}
\EndFor
\LineComment{Coefficient selection and Horner evaluation (host $b$, authenticated arithmetic)}
\For{$j=0$ \textbf{to} $d$}
  \State $\authb{\bar a_j}{b}\gets\sum_{i=0}^{m-1}a_{i,j}\,\authb{s_i}{b}$ \Comment{local, $\Pi_{\mathsf{Lin}}$}
\EndFor
\State $\authb{y}{b}\gets\authb{\bar a_d}{b}$
\For{$j=d-1$ \textbf{down to} $0$}
  \State $\authb{y}{b}\gets\authb{y\cdot x}{b}+\authb{\bar a_j}{b}$ \Comment{$\Pi_{\mathsf{Mult}}$}
  \State rescale exactly where $\mu$ specifies (\cref{alg:trunc})
\EndFor
\State \Return $\authb{y}{b}$
\end{algorithmic}
\end{algorithm}

\textbf{Shifted intervals.}
For a proper nonempty public interval $[a,b)\subsetneq[0,p)$ (here $a,b$ are endpoints, not party indices), \cref{alg:interval} opens $c=x+r\bmod p$ for a fresh field mask $r$, and $T_b$ derives from the same $r$
\begin{equation*}
    L=(a+r)\bmod p,\quad H=(b+r)\bmod p,\quad \omega=\one[L>H].
\end{equation*}
With conservative DCFs for thresholds $L$ and $H$ (\cref{alg:dcf}; orientation $\one[c<\theta]$, payload $1$, independent coins) and a sharing of the wrap bit $\omega$, the raw share $\tilde s_b=\omega_b+\DCF_H(c)_b-\DCF_L(c)_b$ goes to the epilogue. Translation by $r$ maps $[a,b)$ onto the circular half-open interval from $L$ to $H$ ($L\neq H$ since $0<b-a<p$): the indicator is $\one[c<H]-\one[c<L]$ if $L<H$ and $1+\one[c<H]-\one[c<L]$ if the interval wraps, so \cref{thm:dcf} gives $\tilde s_0+\tilde s_1=\one[a\le x<b]$ (\cref{thm:interval}). Empty and full intervals are public constants. A partition may share one mask and one opening if every endpoint, wrap bit and auxiliary share is derived jointly from that mask, while distinct DCFs keep independent coins. The conservative DCF evaluates $n(n+1)/2$ path levels per threshold; its cost, and that of a projected $O(n)$ DCF~\cite{boyle2021function,storrier2023grotto} that \cref{thm:dcf} does not cover, are in \cref{tab:gates}.

\textbf{Piecewise polynomials.}
Activation and normalization functions are approximated by low-degree polynomials on a public partition~\cite{gupta2023sigma,pang2024bolt,ma2023secretflow}. The parties select coefficients $\auth{\bar a_j}=\sum_i a_{i,j}\auth{s_i}$ locally ($\Pi_{\mathsf{Lin}}$, \cref{fig:arith}) and apply Horner's rule with $d$ authenticated products, independently of the number $m$ of pieces. Exactly one indicator of a disjoint exhaustive partition is one, so \cref{thm:arith} yields the active polynomial; rescaling is inserted where the manifest specifies it (\cref{alg:trunc}). Approximation error of the approved coefficients is distinct from the cryptographic correctness of \cref{thm:lut,thm:interval}, which concerns the declared finite arithmetic.

\textbf{Exact comparison, bit decomposition and truncation.}
The LUT input, exact threshold comparisons and toward-zero signed truncation need canonical bits, which \cref{alg:bitdec,alg:trunc} (\cref{app:proof-gates}) derive with authenticated arithmetic alone (\cref{thm:bitdec,thm:cmp-trunc})~\cite{damgard2006unconditionally,catrina2010improved,escudero2020edabits}.

\textbf{Why exact circuits are a fallback.}
Their carry chains cannot be shortened by batching: \cref{alg:bitdec} performs $2n=122$ dependent multiplications for $n=61$, hence $2n+1=123$ sequential verified openings, and exact signed truncation chains two decompositions and a comparator into 307 authenticated multiplications and 309 sequential rounds, \est{30.9~ms} on LAN (\cref{tab:gates}). At two round trips per verified opening (\cref{sec:proto-check}), the 123-round chain alone would take about \est{17.2~s} on WAN. A valid one-round candidate therefore always wins under the cost rule below, and exact circuits are used only when no such candidate meets the gate's contract, with their cost charged to any LUT whose input bits do not yet exist.

\subsection{Direct Protected Gates and Cost-Aware Compilation}\label{sec:proto-direct}

\textbf{The direct protected gate.}
After a verified opening $c=x+r$, each module holds $c$ and $r$ and can compute $x=c-r$ inside its boundary, evaluate an approved deterministic gate $g$, and return a fresh authenticated sharing of $g(x)$ through \AuthShare{} (\cref{fig:gates}(c)). This is secure (\cref{thm:arith}) in the same model and with the same output simulation as the FSS gates, since the host again receives a fresh, independently uniform value and tag tuple (\cref{thm:epilogue}), provided the module's observable trace while computing $g$ meets the same simulatability assumption ($\eps{trace}$ in \cref{thm:main}). Concretely, fetching $T[x]$ from host memory or running in $x$-dependent time would leak $x$, so approved direct gates run from protected memory in data-independent time. A direct gate needs one verified opening, two AES blocks and five field multiplications; our model estimates \est{1{,}800}~M gates/s, above every FSS realization in \cref{tab:gates}.

\textbf{Cost-aware selection.}
For each nonlinear gate shape, the compiler estimates a cost tuple (latency, bytes, protected memory, field operations, PRG calls) for the direct gate, a small XOR LUT, an interval or polynomial FSS gate, and a separately proven malicious backend. It rejects candidates that violate the gate's semantic and security contract (the exact finite function, encoding and rescaling fixed by $\mu$ under the profile in force) and selects the least modeled end-to-end cost among the rest, accounting for dependency depth and transport; only independent checks are batched (\cref{sec:proto-check}). One constraint applies: gate shapes that the manifest marks as FSS-portable keep an FSS realization, so that the same compiled circuit runs under \ProfU. The compiler-selected default is therefore not the unconstrained minimum, and direct-only compilation is marginally faster (\est{3.82~s} versus \est{3.83~s} for BERT-Base on LAN).

\textbf{Why FSS stays in the datapath.}
If the direct gate is at least as cheap under \ProfT, why keep DPF generation and evaluation in the module? (i)~\emph{Compatibility.} Sigma- and Orca-style toolchains~\cite{gupta2023sigma,jawalkar2024orca} compile nonlinear layers into masked-input FSS gates, and \ProfU (\cref{sec:threat-profileu}) runs the circuit through an established malicious backend whose DPF keys the accelerator evaluates as party-local data; there the direct candidate is invalid because the hardware is not trusted with $x$. One DPF datapath serves both profiles and the untrusted-mode DFA workloads. (ii)~\emph{Full-domain scans.} PIR and small-LUT gates are data-independent, fixed-order scans that the pipelined DPF units execute at one iteration per cycle (\cref{sec:arch-hw}), so both profiles reuse one engine; this is a reuse argument, not evidence that the DPF form is the fastest option under \ProfT (\cref{sec:proto-pir}). (iii)~\emph{Short-lived sensitive state.} FSS keeps long-running evaluation state pseudorandom (seeds and correction words), and index- or input-dependent state short-lived. We treat (iii) only as defense in depth against physical and microarchitectural threats that \ProfT excludes; no theorem depends on it, and since each module holds $c$ and $r$, FSS gains no formal confidentiality over the direct gate (\cref{sec:threat-model}). The evaluation reports direct-only, FSS-only and compiler-selected default configurations side by side (\cref{sec:eval-ablation}).

\subsection{Distribution-Preserving Refactoring}\label{sec:proto-refactor}

DFA decouples DPF generation from protocol preprocessing by sampling the target directly as a uniform value and recovering the mask $r$ through $g^{-1}$ when the protocol's transformation $g$ is a bijection~\cite{dfa2026trusted}. \sys draws every target from the joint sampler in the same way, with two refinements of the semi-honest argument. Since DPF key privacy holds for arbitrary targets (\cref{sec:bg-fss}), uniformity is required by the application, which publishes $c=x+r$ or $u=x\oplus r$; a refactoring must therefore preserve the \emph{joint} distribution of the preprocessing, not the uniformity of each target.

\textbf{Joint, not marginal, distributions.}
A gate's preprocessing contains correlated objects: the mask, its bits, DPF or DCF targets, wrap bits and auxiliary shares. If a gate needs targets $r$ and $r+1$, resampling each uniformly keeps the marginals but destroys their unit difference; drawing $L$ and $H$ of \cref{alg:interval} independently likewise yields a wrong indicator. The refactoring is valid exactly under the conditions of \cref{lem:bijection}: the map is a bijection for the fixed context \emph{and} all auxiliary material is regenerated from the recovered mask by the unchanged sampler. For example, \cref{alg:interval} may draw $L$ uniformly, set $r=L-a$ and derive $H$ and $\omega$ from that $r$, but may not draw $L$ and $H$ independently.

\textbf{Noninvertible maps and truncation.}
For unsigned truncation, the sampler $R'=2^hA+U$ of \cref{lem:noninv} makes the DFA rule (shift left, fill the low bits uniformly~\cite{dfa2026trusted}) exact; signed shifts, nonuniform masks and other moduli need their own samplers.

\subsection{Verified GPU Matrix Products}\label{sec:proto-freivalds}

Authenticated linear layers need no extra verification: a GPU deviation that changes a value is caught at the next \CheckOpen, before the result enters a protected gate or a release, except with the probability bounded in \cref{thm:mac-sound}. A module that must \emph{consume} a GPU-computed matrix before any opening, however, must not accept it on the host's word, which would reintroduce the forgery oracle of scenario S2. For this case \cref{alg:freivalds} (\cref{app:proof-gates}) is an optional frozen-operand Freivalds check~\cite{freivalds1977probabilistic}, in the spirit of Slalom~\cite{tramer2018slalom} but bound to the ledger.

\textbf{Permitted uses and check.}
The check applies only when exposing the operands to that GPU is already allowed, as in public-by-party-local matrix products; it never permits exposing global secret triple masks, which are generated inside the TCB (\cref{sec:proto-arith}). The module binds the exact operand bytes $A\in\Fp^{m\times k}$ and $B\in\Fp^{k\times n}$ to their authoritative records and freezes the claimed $C$ (\cref{sec:proto-ledger}); only then does it draw $s$ independent secret uniform $\bm{v}\in\Fp^{n}$, test $C\bm{v}\stackrel{?}{=}A(B\bm{v})$ inside the protected verifier, and consume only the verified frozen bytes of $C$ (\cmd{VERIFY_MATRIX} in \cref{tab:commands}). If the GPU also transforms tag arrays, their tag equations are verified too.

\textbf{Soundness and cost.}
\Cref{thm:freivalds} bounds acceptance of a wrong product by $p^{-s}$, and $Q_F$ calls add $Q_F/p^s$ to \cref{thm:main}. The check is disabled in all evaluated configurations; enabling it adds implementation obligations (\cref{tab:obligations}) and this error term.

\subsection{Versioned-Snapshot PIR}\label{sec:proto-pir}

In DPF-based two-server PIR (\cref{eq:pir}), a malicious server can return a wrong share, which the client silently reconstructs into a wrong record, or answer from a stale database. \Cref{alg:pir} and \cref{fig:pir} show the \sys countermeasures.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_pir.pdf}
    \caption{Versioned-snapshot PIR (\cref{alg:pir}). Both modules bind the same query, scan the same snapshot bytes in a public order, hash exactly the bytes they consume, and quarantine the DPF-weighted reduction until the hash matches the authorized commitment $\mathsf{cm}_v$. A host that swaps a record after hashing or serves an old version causes an abort, never a wrong accepted record (scenario S8). Both modules learn $\alpha$, so query privacy relies on module trust.}
    \label{fig:pir}
\end{figure}

\begin{algorithm}[t]
\algstretch
\caption{Versioned-snapshot protected PIR (\algname{PIR-Snap}) inside module $T_b$}
\label{alg:pir}
\begin{algorithmic}[1]
\Require from the client over its confidential channel: index $\alpha$, query identifier $\mathit{qid}$, descriptor $\mathsf{desc}_v=(\mathsf{id},v,N,\mathsf{enc},\mathsf{cm}_v)$; snapshot records $D[0],\dots,D[N-1]$ streamed by host $b$
\Ensure value share $y_b$ of $D[\alpha]$ and certificate $\mathsf{cert}_b$ for the client, or \Abort
\LineComment{Step 1: query binding}
\State exchange $(\alpha,\mathit{qid},\mathsf{desc}_v)$ with $T_{1-b}$ over the protected channel
\If{the bindings differ, $\alpha\ge N$, or $\mathsf{desc}_v$ is unauthorized}
  \State \Abort
\EndIf
\LineComment{Step 2: joint DPF and same-byte scan ($N\ge2$; $N=1$ is a constant-record case with the same checks)}
\State $n\gets\lceil\log_2N\rceil$; bind $N$ and $2^n$; $D[i]\gets0$ for $N\le i<2^n$
\State joint DPF generator for $(\alpha,1)$ under label $(\mathit{qid},\textsf{pir})$ \Comment{GaC}
\State $h\gets\Hash.\mathsf{init}(\mathsf{id},v,N,\mathsf{enc})$;\; $\tilde y_b\gets0$
\For{$i=0$ \textbf{to} $2^n-1$ in public order} \Comment{$\EvalAll$, DFS}
  \If{$i<N$}
    \State read $D[i]$ into $T_b$; $h\gets\Hash.\mathsf{update}(h,D[i])$
  \EndIf
  \State $\tilde y_b\gets\tilde y_b+\DPF.\Eval(k_b,i)\cdot D[i]$ \Comment{per coordinate}
\EndFor
\LineComment{Step 3: snapshot check; the result is quarantined until here}
\If{$\Hash.\mathsf{final}(h)\neq\mathsf{cm}_v$}
  \State \Abort
\EndIf
\LineComment{Step 4: fresh resharing and certified release}
\State $y_b\gets\tilde y_b+(-1)^b\zeta$ with a fresh joint pad $\zeta$ per coordinate
\State $\mathsf{cert}_b\gets$ certificate on $(\mathsf{sid},\mathsf{ep},\mathit{qid},\mathsf{desc}_v,b,\Hash(y_b))$
\State \Return $(y_b,\mathsf{cert}_b)$ to the client \Comment{no MAC tags}
\end{algorithmic}
\end{algorithm}

\textbf{Protocol and snapshot binding.}
Both role-bound modules receive the same canonical query from the client, compare the binding over their protected channel, pad the snapshot to $2^n$ records while authorizing only $\alpha<N$, and run a joint DPF for $(\alpha,1)$ by generate-and-consume. Each scans the same canonical bytes in the same public order, applies the same DPF weights to every record coordinate, and hashes exactly the bytes it consumes. The commitment $\mathsf{cm}_v$ covers the database identifier, version, shape, record encoding and ordered data bytes, and the result stays quarantined behind the release guard (\cref{sec:proto-ledger}) until the hash matches it; a host that swaps a record after hashing or serves an old version therefore causes an abort (scenario S8 in \cref{tab:scenarios}). A Merkle realization~\cite{merkle1987digital} must authenticate every consumed leaf and its position against the same root. Offloading the reduction to the GPU would need \cref{alg:freivalds} or a separately proven authenticated reduction, never a signature on the GPU's claim, and would export the expanded share vector, so \sys reduces inside the module. Each module releases only a freshly reshared value share (the value half of the epilogue) with a bound certificate, and the client reconstructs $D[\alpha]=y_0+y_1$.

\textbf{Guarantees and regimes.}
In regime (R1) of $\FPIR$ (\cref{fig:func}), with one malicious server host and an honest client, the client obtains the committed record or an abort, and the host learns nothing about $\alpha$ beyond $\Leak_{\mathrm{PIR}}$ (\cref{def:leakage}). In regime (R2), a malicious client alone learns only the requested record and the public descriptor. We make no combined claim (\cref{thm:pir}). Both modules learn $\alpha$, so query privacy relies on module trust: unlike untrusted two-server DPF-PIR such as GPU-DPF~\cite{lam2023gpu} or DFA's untrusted mode~\cite{dfa2026trusted}, which hides $\alpha$ from each server without trusted hardware, \sys offers no query privacy against a compromised module.

\textbf{Scope and design choice.}
Authenticated PIR~\cite{colombo2023apir} provides integrity without trusted hardware at additional server cost and is our malicious-secure GPU baseline (\cref{sec:eval-pir}). Two alternatives bracket our design. Since the modules know $\alpha$ anyway, a module could select $D[\alpha]$ with a constant-time comparator during the same public-order scan; this needs no AES expansion and would be bound by snapshot bandwidth rather than by the AES array. If $\alpha$ must stay hidden from the modules, the client can generate the DPF keys as in untrusted-mode DFA, and each module evaluates its own key inside the boundary with the same hashing, quarantine, resharing and certificates; this adds a DPF key-privacy term and, against a malicious client, a key-verification step~\cite{boyle2016function,boneh2021lightweight,decastro2022vfss}. We keep joint generation for uniformity with the inference datapath (\cref{sec:proto-direct}) and as defense in depth. We model neither alternative, so \cref{tab:pir} does not show that our design is the best \ProfT PIR. Assuming a PIR efficiency of \est{0.93} relative to DFA (\cref{app:model}), our model gives \est{16{,}349} versus 17{,}580~queries/s at $N=2^{20}$~\cite{dfa2026trusted} (\cref{tab:pir}), with query privacy resting on module trust.


==> qa/draft2/sections/06_architecture.tex <==
% ======================================================================
% Section VI: Architecture and System Integration
% Labels defined here: sec:arch, sec:arch-insight, sec:arch-hw, sec:arch-pipe,
%   sec:arch-iface, sec:arch-field, sec:arch-deploy, sec:arch-dse,
%   fig:hw, fig:pipeline, tab:commands, lst:mersenne
% ======================================================================
\section{Architecture and System Integration}\label{sec:arch}

This section describes how \sys realizes the protected module $T_b$ of \cref{sec:protocol} next to the GPU and how the untrusted host drives it. We keep the organization of DFA~\cite{dfa2026trusted} wherever the malicious setting permits and add only the blocks that the integrity chain requires. Hardware sizes are design parameters; red values are estimates (\cref{sec:eval-hw,app:model}). That this hardware realizes the ideal resource $\mathcal{F}_{\mathsf{T}}$ of the proofs is an implementation obligation (\cref{tab:obligations}).

% ======================================================================
\subsection{Design Insights}\label{sec:arch-insight}

\textbf{Key insight.}
Malicious security moves the dominant cost from DPF to authenticated linear algebra on the GPU, while protected FSS evaluation, exposed triple generation and \CheckOpen{} stay small (\cref{sec:analysis-cost,fig:motiv}). The module therefore need not become a second GPU: it must hold exactly the state whose exposure or modification would break the integrity chain and inspect every byte that crosses its boundary. The GPU is a fast but untrusted engine for authenticated linear algebra, and the module is dealer, verifier and release authority at once.

\textbf{What must be protected.}
A block belongs inside the trusted boundary if it holds material that reveals both parties' views or authorizes a release. These are exactly the TCB items of \cref{sec:threat-model} (keys, sampler and counters, generator state and correction words, table and reduction logic, challenges and residuals, release decisions); everything else stays outside (\cref{fig:threat}).

\textbf{What stays on the GPU.}
Linear layers run as the matrix Beaver products of $\Pi_{\mathsf{Mult}}$ over the value lane and the $t=3$ tag lanes (\cref{fig:arith}), i.e., two dense products per lane, $2(1+t)$ in total, of the same public shape. A GPU result is a candidate share, never a certified value.

\textbf{Placement.}
An authenticated element costs 32~B per party at the module interface (\cref{sec:proto-repr}), so a link of bandwidth $B$ streams at most $B/32$ elements per second (\cref{sec:analysis-work}). The L2-adjacent placement of DFA delivers about 290~GB/s to the SMs~\cite{dfa2026trusted}, so we keep it: one DPF unit per L2 slice, a new protected core beside a designated L2 partition, and SM access through the DFA-mapped address range without a new NoC port.

% ======================================================================
\subsection{Hardware Design}\label{sec:arch-hw}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_hw.pdf}
    \caption{\sys hardware. Top: placement inside the GPU; as in DFA, one DPF unit sits next to each L2 slice and a designated slice hosts the VIGOR core. Bottom: logical organization of the protected module $T_b$ (red dashed trusted boundary). The 64 AES-128 engines are time-shared among PRG expansion, challenge derivation and AEAD sealing; the Mersenne-61 field unit array (eight lanes in each DPF unit) serves epilogues, triples, reductions and check residuals. SMs, L2, NoC, HBM and host DRAM stay outside the boundary.}
    \label{fig:hw}
\end{figure}

\Cref{fig:hw} shows the module (area and power in \cref{sec:eval-hw}). The trusted boundary encloses the 16 DPF units of DFA (\cref{sec:bg-dfa}), the VPU, the new \emph{VIGOR core} and the on-die links between them. Only command frames with share batches, PIR database records, authenticated output tuples, sealed spill pages and sealed channel frames cross it, none carrying a module secret in the clear. The blocks follow the integrity chain: parser and ledger admit \emph{authorized input}; sampler and field unit array produce \emph{correlated preprocessing}; the DPF units perform \emph{correct local evaluation}; the epilogue yields \emph{authenticated arithmetic}; freezer, check engine and peer channel enforce \emph{consistent opening}; and the release guard gates \emph{authorized output release}.

\textbf{DPF units and sampler.}
The AES datapath is unchanged. Each pipeline context carries two generator states, a separate evaluator state, a DFS stack and the conversion $\Conv$ into $\Fp$, exactly the state of \cref{alg:gac}; correction words are consumed and discarded inside the unit, and raw leaf shares $\tilde y_b$ go to the field unit array lanes of the same unit, never to SM-readable buffers. The joint PRF sampler implements the labeled derivation and bounded rejection sampling of \cref{sec:proto-setup} under the session key.

\textbf{Field unit array (FUA).}
The FUA consists of 128 Mersenne-61 multiply-accumulate lanes, each with a $61\times 61$-bit multiplier and the two-fold reduction of \cref{lst:mersenne}; its peak is 116~G multiply-accumulates per second at the 910~MHz 7~nm clock of DFA~\cite{dfa2026trusted}. It computes epilogues (three products per output), the triple products $c=ab$ and $C=AB$ with their \AuthShare{} tags (so matrix masks never reach the GPU), LUT and PIR reductions, interval sums and check residuals. The lanes sit in the DPF units, eight per unit (a design parameter), and the VIGOR core schedules them as one pool. Full-domain LUT and PIR reductions therefore run next to the leaves, and only per-query accumulators (three field elements per PIR query) travel to the core (\cref{sec:arch-dse}).

\textbf{Check engine and freezer.}
The check engine executes steps~3 and~4 of \cref{alg:checkopen}: it derives the $t$ challenge vectors only after both frozen roots are fixed, accumulates the residuals on FUA lanes (two products per lane and element) and evaluates all lanes over the full batch before emitting one generic status, so neither the status nor its latency reveals which lane or position failed. \cmd{FREEZE_BATCH} copies the exact submitted bytes into a 256~KB freeze SRAM (8{,}192 tuples of 32~B) and hashes them with their descriptor into the root $h_b$ that the modules exchange; larger batches spill to AES-GCM-sealed immutable HBM pages~\cite{dworkin2007gcm,mcgrew2004gcm} whose authoritative root and page counters stay inside, so after the challenge only authenticated frozen bytes are reread (\cref{sec:proto-ledger}).

\textbf{Ledger, release guard and control.}
A 32~KB ledger SRAM holds the authoritative state of every in-flight gate and the randomness identifiers burnt at reservation (\cref{fig:ledger}). The release guard opens for a gate only in state \lstate{VERIFIED}, and an epoch abort closes every outstanding response atomically (\cref{sec:proto-ledger}); the release multiplexer and output FIFO of \cref{fig:hw} belong to the release-guard logic. The peer-channel controller keeps independent directional keys, never repeats a nonce and enforces a per-session traffic and forgery budget. The SC300-class control core of DFA~\cite{st33tpm12spi,arm_cortex_m3} runs measured boot, attestation and the key establishment covered by $\eps{setup}$, and the 16-lane VPU of DFA~\cite{cavalcante2019ara} handles the remaining protocol logic, including the range check $x^*\in\mathsf{In}_\nu$ of $\Pi_{\mathsf{Input}}$ and the validity predicates of $\mu$ at the public boundaries that $\mu$ declares. Host software cannot drive the module's clock or voltage outside its safe operating range (DVFS isolation, \cref{app:func-module}).

\textbf{AES time-sharing.}
The 64 engines are the module's only AES resource. A slot arbiter per unit serves PRG expansion (two blocks per expansion, $6n+3$ per GaC output), challenge derivation (1.5 blocks per checked element: three 64-bit words for three 61-bit challenges) and AEAD keystream for sealing and the peer channel (two blocks per 32-byte tuple); one AEAD/GHASH block serves both the freezer and the peer-channel controller. Check and sealing requests take priority because they are short and on the critical path of the next round; PRG contexts fill all other slots. A per-slot purpose tag selects the key context, so the uses never share a key.

% ======================================================================
\subsection{Pipeline Scheduling and Memory}\label{sec:arch-pipe}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_pipeline.pdf}
    \caption{Scheduling inside a DPF unit. (1)~Generator (g) and evaluator (e) expansions of at least $L$ independent contexts interleave to hide the $L$-cycle AES and correction feedback latency. (2)~AES slots are time-shared among PRG expansion, challenge derivation and AEAD sealing. (3)~Depth-first $\EvalAll$ keeps one pending sibling per level, i.e., $O(n)$ state per context.}
    \label{fig:pipeline}
\end{figure}

\textbf{Context interleaving.}
With an AES and correction feedback latency of $L$ cycles, one dependent path advances at most one level every $L$ cycles, so one issue per cycle needs at least $L$ independent contexts per unit (\cref{fig:pipeline}, panel~1). For the 20-stage DFA pipeline~\cite{dfa2026trusted} we therefore provision 20 contexts per unit, one per stage. The three expansions of a malicious GaC level issue back to back, because $\PRG(\tilde s)$ does not depend on $\CW^{(i)}$; only the correction waits for all three. A context (three 129-bit path states, the correction word in flight, target, query, payload and level) needs fewer than 100~B, so 20 contexts take less than 2~KB per unit, and a single gate with $n=61$ completes in \est{1.71~$\mu$s}.

\textbf{Separate old controls.}
Each unit keeps separate registers for the \emph{old} generator bits $t_0,t_1$ and the \emph{old} evaluator bit $\tilde t$ (\cref{sec:analysis-dpf}), captures all outputs of a transition before overwriting its inputs, and never substitutes generator states for evaluator roots; this is the schedule covered by \cref{thm:gac}. Planned RTL tests exercise signed final conversion, zero payloads, all-zero and all-one indices, $x=\alpha$ and divergence at every depth.

\textbf{Depth-first EvalAll.}
LUT and PIR gates evaluate the full domain. Depth-first traversal keeps one pending sibling per level ($O(n)$ states per traversal) and a complete tree needs $2^n-1$ internal expansions (panel~3). The 512 queries of a PIR batch walk the same public leaf order in lockstep, so each snapshot record is read and hashed once per batch and folded into 512 per-query accumulators. For $N=2^{20}$, 512 contexts with 20 pending siblings of 17~B occupy about 174~KB, or 11~KB per unit, which fits the traversal buffers of DFA~\cite{dfa2026trusted}.

\textbf{Pads and frozen buffers.}
The four pads of an output occupy two AES blocks and are drawn in step with the leaf, so no pad buffer beyond the pipeline depth is needed. A checked batch occupies the freeze SRAM until its verdict two peer round trips later, so batches beyond 8{,}192 elements, such as the 65{,}536-element batches of \cref{fig:checkperf}, spill to sealed pages.

% ======================================================================
\subsection{Command Interface and Host Integration}\label{sec:arch-iface}

\begin{table}[t]
\centering
\caption{Commands of the protected module $T_b$. Every command is a canonical frame bound to session, epoch, role and gate; the ledger state reached on success is given in parentheses. No command authenticates a host-supplied value.}
\label{tab:commands}
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\linewidth}{l >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X}
\hline
\textbf{Command} & \textbf{Required check} & \textbf{Allowed result} \\
\hline
\cmd{OPEN_SESSION}  & Authenticated identities, role, fresh epoch, manifest $\mu$ & Session capability \\
\cmd{RESERVE_PREP}  & Approved gate, unused randomness identifiers & Party-local authorized preprocessing, issued once (\lstate{PREPARED}) \\
\cmd{FREEZE_BATCH}  & Exact canonical bytes, dimensions, expected wire list & Frozen root $h_b$ and handle (\lstate{FROZEN}) \\
\cmd{CHECK_OPEN}    & Both frozen roots, independent challenge lanes, peer residuals & Verified prescribed opening or abort (\lstate{VERIFIED}) \\
\cmd{EVAL_FSS}      & Bound table or function, consumed input opening, fixed role & Freshly reshared authenticated local output (\lstate{CONSUMED}) \\
\cmd{VERIFY_MATRIX} & Anchored operands, frozen candidate & Verified immutable result handle (\lstate{VERIFIED}) \\
\cmd{FINAL_OUTPUT}  & Authorized recipient, output mask, accepted check & Bound frame with $\upsilon=y+o$ and certificate (\lstate{CONSUMED}, then \lstate{RELEASED}) \\
\cmd{ABORT}         & Any integrity or lifecycle violation & Epoch invalidation, no candidate values (\lstate{ABORTED}) \\
\hline
\end{tabularx}
\end{table}

\textbf{Host responsibilities.}
Host $b$ schedules the public circuit, stores only party-local authenticated arrays (value and each MAC lane as separate coalesced arrays, serialized canonically only at the protected interface), runs the exact field kernels of \cref{sec:arch-field} and sends share batches to $T_b$. Its scheduling may be adversarial, so the ledger, not the host, decides whether operation, identity, shape and order are admissible, and a reused buffer always carries a fresh transaction identifier.

\textbf{Commands and frames.}
\Cref{tab:commands} lists the eight commands with the ledger state each reaches (\cref{fig:ledger}); since none of them authenticates a host value, the forgery-oracle path of scenario~S2 is closed (\cref{tab:scenarios}). A frame carries version, session identifier, epoch, role, opcode, gate identifier, ordered input and output identifiers, field identifier, tag count, dimensions, payload length, sequence number and payload, all length-prefixed with explicit endianness; frames between modules or from a client bind the header as AEAD associated data. The parser copies each frame into protected memory before checking it and rejects truncation, trailing bytes, duplicate identifiers, malformed dimensions, noncanonical field elements (values of at least $p$ are rejected, never reduced) and unexpected opcodes.

\textbf{Data races and aborts.}
Verification and consumption use the same immutable parsed bytes, and \cref{tab:attacks} maps each injected fault to the block that stops it.

% ======================================================================
\subsection{Exact Field Arithmetic on the GPU}\label{sec:arch-field}

GPU kernels must compute the finite circuit that the proofs reason about, so floating-point shortcuts are excluded. An authenticated GEMM applies the matrix Beaver combination of $\Pi_{\mathsf{Mult}}$ on each of the four lanes, i.e., two products per lane ($D\,B_b$ and $A_b\,E$ on the value lane, likewise on each tag lane), $2(1+t)=8$ products of the same shape, plus the public product $DE$ shared by all lanes (\cref{fig:arith}); \cref{lst:mersenne} gives the scalar multiplication at the core of every kernel.

\begin{figure}[t]
\centering
\scriptsize
\begin{tabular}{|l|}
\hline
\begin{minipage}{0.95\linewidth}
\vspace{2pt}
\begin{verbatim}
constexpr uint64_t P = (1ULL << 61) - 1;  // 2^61 - 1
// canonical a, b < P; returns canonical a*b mod P
__device__ uint64_t mul61(uint64_t a, uint64_t b) {
  uint64_t lo = a * b;              // low 64 bits
  uint64_t hi = __umul64hi(a, b);   // high bits, < 2^58
  uint64_t x  = (lo & P) + ((lo >> 61) | (hi << 3));
  x = (x & P) + (x >> 61);          // x <= 2^61
  return x >= P ? x - P : x;
}
\end{verbatim}
\vspace{-4pt}
\end{minipage}\\
\hline
\end{tabular}
\caption{Exact Mersenne-61 multiplication used by the GPU field kernels (CUDA). The first fold uses $2^{61}\equiv 1 \pmod p$; the second fold and the conditional subtraction return the canonical representative. No floating-point or Tensor-Core operation is involved.}
\label{lst:mersenne}
\end{figure}

\textbf{Correctness.}
For canonical $a,b<p=2^{61}-1$ the product is below $2^{122}$, so $\mathtt{hi}<2^{58}$ and $\mathtt{hi}\ll 3$ fits in 61 bits. Writing $ab=2^{64}\,\mathtt{hi}+\mathtt{lo}$ and using $2^{61}\equiv 1\pmod p$ gives $ab\equiv(\mathtt{lo}\bmod 2^{61})+\lfloor\mathtt{lo}/2^{61}\rfloor+2^{3}\,\mathtt{hi}\pmod p$. The last two terms occupy disjoint bit ranges (bits 0 to 2 and 3 to 60), so the bitwise OR equals their sum and the folded value is below $2^{62}$. The second fold yields at most $2^{61}=p+1$, and the conditional subtraction returns the canonical representative. The executed CPU check of this formula and the pending GPU conformance test are reported in \cref{sec:eval-attack}.

\textbf{Accumulation and numeric contract.}
A two-word 128-bit accumulator absorbs at most 64 unreduced products below $2^{122}$, so kernels fold at least once per 64 inner-dimension terms; random shares lie close to $p$ even for small plaintexts, so plaintext bounds never justify longer accumulation. The manifest $\mu$ fixes the scale $2^f$, signed encoding, toward-zero truncation (\cref{alg:trunc}), saturation, approximation coefficients and output decoding. For example, a dot product of length at most 4{,}096 with operand magnitudes at most $2^{20}$ stays within $|\cdot|\le 2^{52}$ before bias, which leaves room below $p/2$ only if bias and further accumulation are bounded too; the bound is recomputed per layer. FP16, BF16 and TF32 Tensor Cores never serve as exact field operations without a proven limb construction, and the exact finite circuit and a floating-point accuracy model remain separate references.

\textbf{GEMM cost assumption.}
Our model charges an exact Mersenne GEMM \est{1.25$\times$} the time of a wraparound 64-bit GEMM per lane ($\mu_{\mathrm{M}}$ in \cref{app:model}). This factor is an assumption, not a measurement: the kernel above additionally needs the high product word and a two-word accumulator per term, and the GPU test that would calibrate it has not run. Each $+0.25$ in $\mu_{\mathrm{M}}$ adds \est{0.52~s} to BERT-Base; with $\mu_{\mathrm{M}}=2$ its LAN latency would be \est{5.39~s}, i.e., \est{3.8$\times$} instead of \est{2.7$\times$} that of semi-honest trusted DFA.

% ======================================================================
\subsection{Deployment Targets}\label{sec:arch-deploy}

An on-die module cannot be added to a commercial A100, so we define three distinct experiments and never merge their timings. We executed a specification and a functional CPU reference model; GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet, so the three experiments below are planned. \emph{(i) A100 software} runs the exact kernels, authenticated GEMM and host runtime on a real A100 with an emulated module. \emph{(ii) A ZCU102 prototype} (\texttt{xczu9eg-ffvb1156-2-e}~\cite{amd2023zcu102}) implements the datapath of \cref{fig:hw} at reduced scale (\est{4} DPF units, \est{16} AES engines, \est{32} FUA lanes at \est{250~MHz}, \cref{tab:fpga}) to validate streaming, freezing and release ordering; one board with an emulated peer shows functionality, not two independent trust boundaries, and an ARM process on it is not isolated from a malicious board administrator. \emph{(iii) The on-die projection} models integration next to the L2 slices with Accel-Sim~\cite{khairy2020accel} and synthesis, as in DFA; our headline numbers refer to it and currently come from the analytical model of \cref{app:model}. An external module uses staged transfer through host memory as its baseline, because GPUDirect RDMA needs platform and driver support and ordinarily a common PCIe root complex~\cite{nvidia2024gpudirect}; IOMMU protection is never disabled for a benchmark. In every target, freeze-before-challenge refers to immutable authenticated bytes, never to a GPU buffer that can change concurrently.

% ======================================================================
\subsection{Design-Space Comparison}\label{sec:arch-dse}

We compare the L2-adjacent organization of \sys with alternative homes for authentication, verification and randomness generation.

\textit{External protected module over PCIe.}
A discrete FPGA or security card~\cite{xu2025co} keeps the boundary off the GPU die but limits the interface to $B/32$ elements per second: \est{50~M} for the \est{1.6~GB/s} ZCU102 transport and \est{0.78~G} for \est{25~GB/s} of effective PCIe Gen4 bandwidth, against 9.1~G on the 290~GB/s on-die path of DFA~\cite{dfa2026trusted}. Because authenticated GEMM dominates, BERT-Base LAN latency rises only to \est{3.87~s} over PCIe and \est{4.59~s} with the ZCU102 link and lanes (\cref{tab:ablation}); the option suits prototyping but adds a second device per party and two device round trips per checked layer (\cref{app:model}).

\textit{Verification on the GPU SMs.}
In \ProfT the SMs belong to the malicious host: a corrupt checking kernel could see the challenges before choosing its errors, or simply report acceptance. Trusting them requires a GPU-wide TEE~\cite{volos2018graviton,jang2019heterogeneous,dhanuskodi2023confidential} covering SMs, caches, memory controllers and the driver interface, the large boundary that DFA and \sys avoid. The GPU therefore computes only products that the module verifies afterwards (\CheckOpen{} or the Freivalds check of \cref{sec:proto-freivalds}).

\textit{Tag DPF trees instead of the epilogue.}
One extra DPF tree per MAC lane (payload $\Delta_j\beta$) multiplies the PRG work of every gate by $1+t$ (\cref{tab:gatecost,fig:dpfthr}); the epilogue achieves the same with three multiplications and four pads (\cref{thm:epilogue}) at \est{3.8--4.0$\times$} the per-gate throughput of tag trees.

\textit{Software-only malicious backend.}
SPDZ-family preprocessing~\cite{keller2016mascot,keller2018overdrive,cramer2018spdz2k,keller2020mpspdz} needs inter-party communication that grows with the number of authenticated triples, and dealer-based malicious FSS, modeled after the protocol family of Shark~\cite{gupta2025shark}, ships authenticated keys and triples from an external dealer (\cref{tab:e2e}); both re-create the offline traffic that trusted DFA removed. Such a backend fits \ProfU, where the hardware itself is distrusted (\cref{sec:threat-profileu}); under \ProfT it pays for a trust assumption that the module already provides.

\textit{Dedicated check engines, a central FUA and per-slice checking.}
Checking needs only \est{2.8~ms} of module time per BERT-Base query against \est{131~ms} of protected FSS work, so dedicated AES engines for challenges and sealing would idle almost always. DPF units stay distributed because a single attachment point, a memory-channel path of about 180~GB/s, would cap DPF output at about 62\% of the 290~GB/s delivered bandwidth~\cite{dfa2026trusted}. The same limit rules out a central FUA: the raw 8-byte leaf shares of PIR at 16K entries alone would need \est{137~GB/s} (\est{76\%} of that path), so reductions stay in the units. Checks, by contrast, cost at most 3.5 AES blocks and six field multiplications per element and depend on the ledger, freeze SRAM and peer channel, which must be single points of authority; the VIGOR core therefore controls every check and holds one authoritative root per batch.


==> qa/draft2/sections/07_security.tex <==
% =====================================================================
% Section VII: Security Analysis
% File owner: sections/07_security.tex
% Labels defined here: sec:security, sec:sec-assump, sec:sec-main,
%   sec:sec-lemmas, sec:sec-scenarios, sec:sec-concrete, sec:sec-boundary,
%   thm:main, thm:dpf-correct, thm:gac, thm:dcf, thm:epilogue,
%   lem:hidden-key, thm:mac-sound, thm:arith, thm:bitdec, thm:cmp-trunc,
%   thm:lut, thm:interval, lem:bijection, lem:noninv, thm:freivalds,
%   thm:pir, tab:obligations, tab:lanes
% =====================================================================
\section{Security Analysis}
\label{sec:security}

We now show that \sys realizes the functionalities $\FC$ and $\FPIR$ of \cref{fig:func} with leakage $\Leak_C$ and $\Leak_{\mathrm{PIR}}$ (\cref{def:leakage}) against a malicious host and GPU, as stand-alone security with abort (\cref{def:security}) in the explicit-simulator style~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}. Each link of the integrity chain, \emph{authorized input $\rightarrow$ correlated preprocessing $\rightarrow$ correct local evaluation $\rightarrow$ authenticated arithmetic $\rightarrow$ consistent opening $\rightarrow$ authorized output release}, is discharged by a named statement: input extraction (\cref{thm:arith}); in-module preprocessing and joint sampling (\cref{lem:bijection,lem:noninv}); exact DPF, DCF, FSS-gate and direct-gate correctness (\cref{thm:dpf-correct,thm:gac,thm:dcf,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval,thm:arith}); the epilogue and the arithmetic identities (\cref{thm:epilogue,thm:arith}); MAC-check soundness (\cref{lem:hidden-key,thm:mac-sound}); and gated release (\cref{thm:arith,thm:pir}). Full proofs are in \cref{app:proof-dpf,app:proof-auth,app:proof-gates,app:proof-main}.

% =====================================================================
\subsection{Assumptions and Error Terms}
\label{sec:sec-assump}

The theorem is proved in \ProfT (\cref{sec:threat}); we state module trust as an explicit ideal resource~\cite{katz2007universally}.

\begin{assumption}[Ideal protected module]
Corrupting host $b$ does not corrupt $T_b$; both modules are instances of the ideal resource $\mathcal{F}_{\mathsf{T}}$ (\cref{app:func-module}). The code, keys, parser, field arithmetic, ledger transitions, local memory, protected peer channel and approved I/O paths of each module are correct and confidential. Its externally observable trace (lengths, timing, host-visible memory and DMA activity, power, thermal and clock telemetry) is simulatable by a stipulated trace simulator from the command sequence issued by the host, $\mu$, the public lengths and the accept or abort outcomes, and is independent of the global MAC keys, challenges and residuals given these (all lanes are aggregated in data-independent time before one generic $\mathsf{status}$ is returned). Host software cannot drive the module's clock or voltage outside its safe operating range, or the module detects glitches and aborts (DVFS isolation); software-reachable undervolting~\cite{murdock2020plundervolt} is thus in scope (\cref{sec:threat}). Module state is fresh: a trusted monotonic service preserves freshness across reboots~\cite{parno2011memoir,matetic2017rote}, or the module irrecoverably erases its master key and requires a freshly attested session. Availability is not assumed.
\end{assumption}

\begin{assumption}[Setup, randomness, channels and bindings]
Each term bounds an idealization over the \emph{entire} admitted execution, not a single primitive call:
$\eps{setup}$, simulation of the authenticated setup of \cref{sec:proto-setup} by an ideal role-bound interface;
$\eps{prf}$, replacement of PRF/KDF outputs (AES-128, HKDF~\cite{krawczyk2010hkdf}) under distinct length-prefixed labels by independent coins, identical for the same joint label;
$\eps{channel}$, confidentiality and integrity of the AEAD channels~\cite{dworkin2007gcm,mcgrew2004gcm} with directional keys and nonrepeating nonces;
$\eps{bind}$, collisions or forgeries in manifests, snapshot commitments, frozen-page roots, certificates and session freshness~\cite{fips202,merkle1987digital};
$\eps{trace}$, the stipulated trace simulator.
\end{assumption}

Correctness of protected code, state and arithmetic is thus a \emph{premise}, not an estimated probability. The protocol contributes one statistical term, determined by the field $\Fp$ with $p=2^{61}-1$, the number $t$ of independent global keys $\Delta_j=\Delta_{0,j}+\Delta_{1,j}$ (host $b$ knows at most $\Delta_{b,j}$), and the number $Q$ of \CheckOpen{} batches. Exclusions and client assumptions are those of \cref{sec:threat}; the modules may see inputs (\cref{sec:discussion}).

% =====================================================================
\subsection{Main Theorem}
\label{sec:sec-main}

\begin{theorem}[Stand-alone static malicious security with abort]
\label{thm:main}
Under the assumptions of \cref{sec:sec-assump}, the protocols of \cref{sec:analysis-dpf,sec:protocol} (setup, ledger, exact DPF, generate-and-consume with the fresh authentication epilogue, conservative DCF, \AuthShare, \CheckOpen, $\Pi_{\mathsf{Input}}$ with the committed-input loader, $\Pi_{\mathsf{Lin}}$, $\Pi_{\mathsf{Mult}}$, $\Pi_{\mathsf{Out}}$, bit decomposition, comparison, truncation, LUT, interval and direct protected gates) realize $\FC$ with abort and leakage $\Leak_C$, and \cref{alg:pir} realizes $\FPIR$ with abort and leakage $\Leak_{\mathrm{PIR}}$ (\cref{def:security,def:leakage}), against a PPT adversary that statically corrupts at most one host or, for $\FPIR$ in regime (R2) of \cref{fig:func}, the client alone. With at most $Q$ \CheckOpen{} batches, the advantage of every PPT distinguisher in \cref{def:security} is at most
\begin{align*}
\eps{VIGOR}\le{}&\eps{setup}+\eps{prf}+\eps{channel}\\
&+\eps{bind}+\eps{trace}+Q\,(2/p)^{t}.
\end{align*}
If the Freivalds check (\cref{alg:freivalds}) is enabled for at most $Q_F$ calls with $s$ repetitions, the bound gains $Q_F/p^{s}$, and the binding obligations of \cref{thm:freivalds} apply.
\end{theorem}

\Cref{thm:main} is a stand-alone real/ideal statement about one admitted execution, preserved under sequential composition; we claim neither universal nor concurrent composability, and concurrent sessions that share module state are not covered (\cref{app:func}).

\textbf{What the bound omits.}
There is no DPF one-key-privacy term: keys never leave the modules, \cref{thm:dpf-correct} gives raw correctness and \cref{thm:epilogue} makes every exported tuple uniform. A key-exporting profile (\ProfU, \cref{sec:threat-profileu}, or verifiable FSS~\cite{decastro2022vfss}) must add its actual DPF or backend privacy assumption. The theorem does not prove that a concrete chip implements the ideal module (\cref{sec:sec-boundary}).

\textbf{Proof overview.}
The simulator $\Sim$ plays $\mathcal{F}_{\mathsf{T}}$ for both modules, keeps the global MAC keys internally, and tracks the ledger and, for every wire, the tuple a faithful corrupt party would hold; honest shares stay symbolic, so honest values are never needed. Five hybrids connect the real and ideal executions (\cref{app:proof-main}). In the real execution $\Hyb{0}$ the modules run the concrete module program: $\mathcal{F}_{\mathsf{T}}$ with its randomness $R$ instantiated by $\PRF_K$, peer and client channels by AEAD over the hosts' network, and \cmd{OPEN_SESSION} by attestation plus authenticated key exchange.
\begin{itemize}[leftmargin=*]
\item \textbf{$\Hyb{1}$ (ideal setup and channels).} Setup becomes the ideal role-bound interface, and protected-channel contents become ideal deliveries of the permitted lengths and schedules. Cost: $\eps{setup}+\eps{channel}$.
\item \textbf{$\Hyb{2}$ (ideal randomness and bindings).} PRF/KDF outputs become ideal coins, and any binding failure aborts; the ledger (\cref{fig:ledger}) then excludes label reuse, role swapping and post-challenge byte replacement. Streaming generate-and-consume is replaced by \cref{alg:gen} followed by \cref{alg:eval} (\cref{thm:gac}), and refactored samplers by their reference forms (\cref{lem:bijection,lem:noninv}); both replacements are exact. Cost: $\eps{prf}+\eps{bind}$.
\item \textbf{$\Hyb{3}$ (abort on an accepted wrong-value opening).} The experiment aborts at the first \CheckOpen{} batch accepted with $\bm{e}\ne\bm{0}$ (and, if \cref{alg:freivalds} is enabled, at the first accepted $C\ne AB$). It equals $\Hyb{2}$ until then; by \cref{lem:hidden-key,thm:mac-sound} the cost is $Q(2/p)^t$ (plus $Q_F/p^s$, \cref{thm:freivalds}).
\item \textbf{$\Hyb{4}$ (ideal execution).} Honest parties use $\FC$. $\Sim$ extracts corrupt inputs ($x^*=r+\varepsilon$ or the committed loader value) and aborts where the modules do (e.g., unless $x^*\in\mathsf{In}_\nu$), samples preprocessing tuples, epilogue and direct-gate outputs and every masked opening uniformly (the hidden preprocessing is defined afterwards), decides each check from $\inner{\bm{\rho}_j}{\bm{d}_j-\Delta_j\bm{e}}$ with its own keys and fresh challenges, delivers a corrupt recipient's output mask $o$ early and programs its opening $\upsilon=y+o$ after $\FC$ releases $y$, and appends the stipulated trace simulator. Since $\Hyb{3}$ accepts no wrong value, the trace-free views are identical (\cref{thm:arith,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval}); cost: $\eps{trace}$. PIR uses the simulator of \cref{thm:pir}.
\end{itemize}
The triangle inequality gives the bound. The adversary may still suppress delivery to honest parties: no fairness is added.

% =====================================================================
\subsection{Building Blocks}
\label{sec:sec-lemmas}

The statements refer to the exact algorithms of \cref{sec:analysis-dpf,sec:protocol}, which, unlike the semi-honest ones (\cref{sec:bg-dfa}), make root control bits, role inputs and separate generator and evaluator states explicit; each is followed by its proof idea.

\begin{theorem}[DPF correctness]
\label{thm:dpf-correct}
For all root seeds $s_0,s_1\in\bits{128}$ with root control bits $t_0=0$, $t_1=1$, every $n$, $\alpha,x\in\bits{n}$ and $\beta\in\Fp$, the keys of \cref{alg:gen} and the outputs $y_b$ of \cref{alg:eval} satisfy $y_0+y_1=\beta\cdot\one[x=\alpha]$. No uniform target and no hardness assumption is needed.
\end{theorem}

\noindent\textit{Proof idea.}
On the target prefix the control bits stay opposite; on a losing child $(s_0^{\lose}\oplus s_1^{\lose})\oplus((t_0\oplus t_1)\sCW)=0$ and the control bits cancel, so the states coincide and their signed outputs cancel. At the leaf $t_0-t_1=(-1)^{t_1}$, so $y_0+y_1=u_0-u_1+(-1)^{t_1}\CWout=\beta$ (\cref{app:proof-dpf}).

\begin{theorem}[Generate-and-consume equivalence]
\label{thm:gac}
For fixed roots, $\alpha$, $\beta$, role $b$ and query $x$, the raw share $\tilde{y}_b$ of \cref{alg:gac} equals the output of \cref{alg:eval} on the key $k_b$ that \cref{alg:gen} produces from the same inputs, node by node for every dependency-respecting depth-first order of $\EvalAll$.
\end{theorem}

\noindent\textit{Proof idea.}
Couple both executions: equal states before level $i$ give the same correction word, generator state and evaluator state after it. The theorem justifies scheduling only, not changes to expansion or correction (\cref{app:proof-dpf}).

\begin{theorem}[Conservative DCF]
\label{thm:dcf}
If \cref{alg:dcf} creates, for each $i=1,\dots,n$ (zero payloads included), an independent DPF with target $\alpha_1\cdots\alpha_{i-1}0$ and payload $\beta\alpha_i$, evaluated at $x_1\cdots x_i$, the shares sum to $\beta\cdot\one[x<\alpha]$, at a cost of $n(n+1)/2$ path levels.
\end{theorem}

\noindent\textit{Proof idea.}
If $x<\alpha$, exactly the prefix ending at their first differing bit ($x_i=0$, $\alpha_i=1$) contributes $\beta$; otherwise none does. \Cref{thm:dpf-correct} and linearity conclude (\cref{app:proof-dpf}).

\begin{theorem}[Epilogue correctness and local hiding]
\label{thm:epilogue}
For raw shares $\tilde{y}_0,\tilde{y}_1$ and fresh uniform pads $\zeta,\kappa_1,\dots,\kappa_t\in\Fp$, the outputs $y_b=\tilde{y}_b+(-1)^b\zeta$, $\gamma_{b,j}=\Delta_j y_b+(-1)^b\kappa_j$ form an authenticated sharing of $\tilde{y}_0+\tilde{y}_1$. For either fixed $b$, $(y_b,\gamma_{b,1},\dots,\gamma_{b,t})$ is uniform on $\Fp^{t+1}$ given the raw outputs and the keys, before conditioning on later prescribed openings, jointly across fresh outputs.
\end{theorem}

\noindent\textit{Proof idea.}
The pads cancel in the sums. For fixed $b$, $\zeta\mapsto y_b$ and each $\kappa_j\mapsto\gamma_{b,j}$ are bijections, so every tuple has probability $p^{-(t+1)}$ (\cref{app:proof-dpf}).

\begin{lemma}[Hidden-key invariant]
\label{lem:hidden-key}
In $\Hyb{2}$ with host $b$ corrupted, conditioned on its view and its shares $\Delta_{b,j}$, the honest shares $\Delta_{1-b,1},\dots,\Delta_{1-b,t}$ remain independent and uniform at every point up to the drawing of the challenges of the first check with a nonzero value error; that check either accepts (the event of \cref{thm:mac-sound}) or rejects and ends the execution.
\end{lemma}

\noindent\textit{Proof idea.}
Fresh tags are padded (\AuthShare, \cref{thm:epilogue}); linear updates are deterministic in the view; correct openings have zero residual; a tag-only error yields an outcome independent of $\Delta_j$; residuals and challenges stay inside the modules (\cref{app:proof-auth}).

\begin{theorem}[Wrong-value acceptance]
\label{thm:mac-sound}
Let a batch of $m$ positions submitted to \CheckOpen{} (\cref{alg:checkopen}) differ from the prescribed tuples by a value error $\bm{e}\in\Fp^m$ and tag errors $\bm{d}_1,\dots,\bm{d}_t\in\Fp^m$, fixed by the freeze. If $\bm{e}\ne\bm{0}$, no earlier batch with a nonzero value error has been accepted, and the lanes use independent uniform challenges $\bm{\rho}_j\in\Fp^m$ drawn after the freeze and hidden from the host, \CheckOpen{} accepts with probability at most $(2/p)^t$ in $\Hyb{2}$. Over at most $Q$ batches, an incorrect value is ever accepted with probability at most $Q(2/p)^t$.
\end{theorem}

\noindent\textit{Proof idea.}
Lane $j$ accepts iff $\inner{\bm{\rho}_j}{\bm{d}_j-\Delta_j\bm{e}}=0$. For $e_i\ne 0$ the vector vanishes only if $\Delta_j=d_{j,i}/e_i$ (probability $\le 1/p$ by \cref{lem:hidden-key}); otherwise the nonzero linear form vanishes with probability $1/p$~\cite{schwartz1980fast}. Each lane gives $1/p+(1-1/p)/p<2/p$, and lanes are independent. Apply the bound to the first wrong-value batch; a union bound over batches gives $Q(2/p)^t$, following the SPDZ MAC check~\cite{damgard2012spdz,damgard2013practical} (\cref{app:proof-auth}).

\begin{theorem}[Authenticated arithmetic and direct gates]
\label{thm:arith}
With correct modules and prescribed messages, the protocols of \cref{fig:arith} are exact: $\Pi_{\mathsf{Input}}$ yields $\auth{x}$ with $x=r+\varepsilon$ (or aborts unless $x\in\mathsf{In}_\nu$), $\Pi_{\mathsf{Lin}}$ preserves $\gamma_{0,j}+\gamma_{1,j}=\Delta_j x$, $\Pi_{\mathsf{Mult}}$ with a correct fresh triple yields $\auth{xy}$ (and $\auth{XY}$ with the factor order preserved), and $\Pi_{\mathsf{Out}}$ gives $y=\upsilon-o$ to its authorized recipient. A direct protected gate (\cref{sec:proto-direct}) for an approved deterministic $g$, evaluated from protected memory in data-independent time, outputs \AuthShare$(g(c-r))$, an authenticated sharing of $g(x)$ whose party-local tuple is uniform as in \cref{thm:epilogue}. Unless a nonzero value error is accepted or a binding fails, every deviation of a corrupt host selects a permitted input, leaves the computation unchanged, or causes abort.
\end{theorem}

\noindent\textit{Proof idea.}
With $d=x-a$, $e=y-b$ and $c=ab$: $c+db+ea+de=xy$~\cite{beaver1991efficient}, the tags follow scaled by $\Delta_j$, $Z=C+DB+AE+DE$ for matrices, and $\upsilon-o=(y+o)-o=y$ with $o$ uniform. A direct gate recomputes $x=c-r$ from a verified opening, and its trace falls under $\eps{trace}$. \CheckOpen{} and the ledger block changed or reused material; induct over gates (\cref{app:proof-auth}).

\begin{theorem}[Canonical bit decomposition]
\label{thm:bitdec}
For $p=2^n-1$ ($n=61$), \cref{alg:bitdec} returns authenticated bits (least significant first) of the canonical representative of $x$, using one masked opening $c=x+r\bmod p$ and $2n$ authenticated multiplications.
\end{theorem}

\noindent\textit{Proof idea.}
The first loop is a full subtractor giving $d=(c-r)\bmod 2^n$ and borrow $\one[c<r]$; with a borrow $x=c-r+p=d-1$ since $p=2^n-1$, which the second loop subtracts~\cite{damgard2006unconditionally} (\cref{app:proof-gates}).

\begin{theorem}[Exact comparison and signed truncation]
\label{thm:cmp-trunc}
From authenticated canonical bits of $x$ and a public $\theta\in[0,2^n)$, \cref{alg:trunc} returns authenticated $\one[x<\theta]$; for centered $z\in[-(p-1)/2,(p-1)/2]$ it returns $\mathrm{sgn}(z)\lfloor|z|/2^f\rfloor$, i.e., truncation toward zero.
\end{theorem}

\noindent\textit{Proof idea.}
The equality flag tracks the processed prefix, and $\mathit{lt}$ gains a term exactly at the first position with secret bit $0$ and threshold bit $1$. Negative values occupy the canonical upper half; $(1-2s)z$ is the magnitude without wrap, and shifting its bits floors~\cite{catrina2010improved}. Fixed-point products must stay below $p/2$ before truncation (\cref{app:proof-gates}).

\begin{theorem}[Authenticated LUT]
\label{thm:lut}
For an approved table $T$ of $2^w$ entries and certified authenticated bits of $x\in\bits{w}$, if the mask bits and the DPF target of the keys for $(r,1)$ come from the same fresh uniform $r$, \cref{alg:lut} outputs $\auth{T[x]}$ and the opened $u=x\oplus r$ is uniform given $x$.
\end{theorem}

\noindent\textit{Proof idea.}
By \cref{thm:dpf-correct}, $\tilde{y}_0+\tilde{y}_1=\sum_a T[a\oplus u]\one[a=r]=T[x]$, and XOR by fixed $x$ is a bijection; independent resampling of the target would break the identity (\cref{app:proof-gates}).

\begin{theorem}[Intervals and piecewise polynomials]
\label{thm:interval}
For a proper nonempty public $[a,b)\subset[0,p)$, \cref{alg:interval} outputs $\auth{\one[a\le x<b]}$; for a disjoint exhaustive partition, Horner evaluation of the selected coefficients outputs $P_{i^\star}(x)$ for the interval containing $x$, in the declared finite arithmetic.
\end{theorem}

\noindent\textit{Proof idea.}
Adding $r$ maps $[a,b)$ to the circular interval from $L$ to $H$; the indicator is $\one[c<H]-\one[c<L]$ if $L<H$ and $1+\one[c<H]-\one[c<L]$ if $L>H$, which is the raw share by \cref{thm:dcf}. Exactly one indicator is one, and Horner with \cref{thm:arith} gives the polynomial; no equality to an unapproximated real function is claimed (\cref{app:proof-gates}).

The next two lemmas state when the semi-honest decoupling, which samples DPF targets directly~\cite{dfa2026trusted}, remains valid: joint distributions with all auxiliary material must match, not only marginals (\cref{sec:proto-refactor}).

\begin{lemma}[Bijection with correlated auxiliary material]
\label{lem:bijection}
Fix $Z=z$, $R$ uniform on a finite $\mathcal{R}$, a bijection $g_z:\mathcal{R}\to\mathcal{A}$, independent coins $W$ and an auxiliary sampler $J$. Then $(R,g_z(R),J(z,R,W))$ and $(g_z^{-1}(A),A,J(z,g_z^{-1}(A),W))$ with $A$ uniform on $\mathcal{A}$ are identically distributed.
\end{lemma}

\noindent\textit{Proof idea.}
Each pair $(r,a)$ has probability $1/|\mathcal{R}|$ in both experiments if $a=g_z(r)$ and zero otherwise; the same $J$ preserves equality. Independently resampling correlated targets such as $(r,r+1)$ breaks it (\cref{app:proof-gates}).

\begin{lemma}[Noninvertible transformations]
\label{lem:noninv}
For any $g$, sampling $A$ from the law of $g(R)$ and $R'$ from $R\mid g(R)=A$ reproduces $(R,g(R))$ and everything derived from $R'$. For unsigned truncation of a uniform $\ell$-bit mask by $h$ bits, $R'=2^hA+U$ with $A$, $U$ uniform on $\ell-h$ and $h$ bits.
\end{lemma}

\noindent\textit{Proof idea.}
$\Pr[A=a]\Pr[R=r\mid g(R)=a]=\Pr[R=r,g(R)=a]$; each truncated mask has probability $2^{-\ell}$. Signed shifts and other moduli need their own samplers (\cref{app:proof-gates}).

\begin{theorem}[Frozen-operand matrix check]
\label{thm:freivalds}
Let the module bind $A\in\Fp^{m\times k}$, $B\in\Fp^{k\times n}$, whose exposure to the GPU is already permitted, and freeze a claimed $C$. If $C\ne AB$, \cref{alg:freivalds} with $s$ secret uniform $\bm{v}\in\Fp^n$ drawn after the freeze accepts with probability at most $p^{-s}$, and over $Q_F$ calls an incorrect product is consumed with probability at most $Q_F/p^s$.
\end{theorem}

\noindent\textit{Proof idea.}
A nonzero row $\bm{e}$ of $C-AB$ gives $\inner{\bm{e}}{\bm{v}}=0$ for a $1/p$ fraction of $\bm{v}$~\cite{freivalds1977probabilistic,tramer2018slalom}; repetitions multiply; freezing fixes $C$ before $v$, and binding ties the verified bytes to the consumed ones (\cref{app:proof-gates}).

\begin{theorem}[Versioned-snapshot PIR]
\label{thm:pir}
With correct modules and binding snapshot and query interfaces: (R1) with an honest client and at most one malicious server host, \cref{alg:pir} gives the client the record $D[\alpha]$ of the snapshot committed by $\mathsf{cm}_v$ or abort, and the corrupt host's view is simulatable without $\alpha$; (R2) with a malicious client alone, accepted requests reveal nothing about the database beyond the requested records and the public descriptor $\mathsf{desc}_v$. Both modules learn $\alpha$: (R1) query privacy rests on module trust, unlike untrusted two-server DPF-PIR (GPU-DPF~\cite{lam2023gpu}, untrusted-mode DFA~\cite{dfa2026trusted}), which hides $\alpha$ without trusted hardware.
\end{theorem}

\noindent\textit{Proof idea.}
\Cref{thm:dpf-correct} gives $y_0+y_1=\sum_i(\DPF_0(i)+\DPF_1(i))D[i]=D[\alpha]$; hashing the consumed bytes, comparing queries and role-bound certificates prevent substitution ($\eps{bind}$); results are freshly reshared (\cref{thm:epilogue}). For a malicious client the simulator extracts the index and reshares the ideal record (\cref{app:proof-pir}).

\textbf{Batched execution.}
\Cref{tab:pir} processes $B=512$ queries per scan as one admitted execution whose manifest lists the $B$ query identifiers $\mathit{qid}$. Each query has its own joint DPF and pad labels, so the simulation of \cref{app:proof-pir} applies query by query. $B$ is part of the public schedule in $\Leak_{\mathrm{PIR}}$, and one abort (e.g., a snapshot mismatch) denies all $B$ queries, which security with abort permits.

% =====================================================================
\subsection{Scenario-by-Scenario Analysis}
\label{sec:sec-scenarios}

We map the scenarios of \cref{fig:scenarios,tab:scenarios} to the statements above; \cref{tab:attacks} lists the corresponding injections.

\begin{itemize}[leftmargin=*]
\item \textbf{S1: Share and tag tampering.} Freeze (S3) and \cref{thm:mac-sound,lem:hidden-key}: a wrong value passes with probability at most $(2/p)^t$ per batch; only the abort bit is revealed.
\item \textbf{S2: Forgery-oracle request.} No command (\cref{tab:commands}) tags a host value; the epilogue tags only protected results (\cref{thm:epilogue}); chosen values enter by input extraction.
\item \textbf{S3: TOCTOU buffer swap.} Freeze-before-challenge realizes the premise of \cref{thm:mac-sound} that errors precede challenges; tampered spill pages abort ($\eps{bind}$).
\item \textbf{S4: Replay and rollback.} Ledger and label binding ($\eps{bind}$) reject reused material; resuming old keys is excluded by the freshness clause.
\item \textbf{S5: Role/gate confusion.} Role-bound keys, joint labels and ledger descriptors turn misrouting into a mismatch and abort ($\eps{bind}$).
\item \textbf{S6: Premature release.} The release guard opens only \lstate{VERIFIED} entries; private outputs are opened as $\upsilon=y+o$, uniform to every host (\cref{thm:arith}).
\item \textbf{S7: Malformed preprocessing.} In-boundary generation, never certified by the MAC check (\cref{thm:arith}); GPU products need \cref{thm:freivalds}, correlated targets \cref{lem:bijection,lem:noninv}.
\item \textbf{S8: Snapshot substitution.} Same-byte hashing and quarantine give the committed record or abort (\cref{thm:pir}).
\item \textbf{S9: Input substitution.} Permitted by $\FC$ and extracted; model provenance requires the committed-input loader.
\item \textbf{S10: Denial of service and selective abort.} Not prevented; aborts occur at public boundaries and are simulatable, and abort and validation outcomes ($\mathsf{status}$) are part of $\Leak_C$.
\end{itemize}

% =====================================================================
\subsection{Concrete Security}
\label{sec:sec-concrete}

Since $2/p\approx 2^{-60}$ for $p=2^{61}-1$, we have $\log_2 Q(2/p)^t\approx\log_2 Q-60t$. For a budget of $Q\le 2^{32}$ checked batches, \cref{tab:lanes} gives the statistical term.

\begin{table}[t]
\centering
\caption{Statistical term and BERT-Base LAN latency versus the number $t$ of MAC lanes ($Q\le 2^{32}$). Latencies are model estimates}
\label{tab:lanes}
\footnotesize
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{c c c c}
\hline
$t$ & $(2/p)^t$ per batch & $Q(2/p)^t$ & BERT-Base LAN (s)\\
\hline
1 & $\approx 2^{-60}$ & $\approx 2^{-28}$ & \est{2.53}\\
2 & $\approx 2^{-120}$ & $\approx 2^{-88}$ & \est{3.18}\\
3 & $\approx 2^{-180}$ & $\approx 2^{-148}$ & \est{3.83}\\
\hline
\end{tabular}
\end{table}

One lane is inadequate. Since the primitives target 128-bit computational security, $t=3$ is the smallest $t$ whose statistical term falls below $2^{-128}$; beyond it the primitives, not the MAC, limit the bound. Extra lanes barely change \CheckOpen{} itself (\est{0.648~ms} for $t=1$ versus \est{0.652~ms} for $t=3$ at $m=65{,}536$ on LAN, \cref{fig:checkperf}); their cost is one more authenticated GEMM lane per key (last column of \cref{tab:lanes}; \cref{sec:eval-ablation}).

\textbf{Tag-only errors.}
The bound concerns wrong \emph{values}: an error in a single tag lane escapes with probability $1/p$ without changing the opened value.

\textbf{Independent challenges.}
With one shared vector $\bm{\rho}$, an adversary submitting $\bm{d}_j=\bm{0}$ and any $\bm{e}\ne\bm{0}$ makes every lane residual $-\Delta_j\inner{\bm{\rho}}{\bm{e}}$, and all lanes vanish together with probability $1/p$. The product bound then collapses to one lane, so shared challenges are rejected (injection~8, \cref{tab:attacks}).

\textbf{Field, not ring.}
The step $\Delta_j=d_{j,i}/e_i$ needs a field. Over $\Z_{2^{64}}$, $e_i=2^{63}$ gives $\Delta_j e_i\equiv 0$ for every even $\Delta_j$, so one lane accepts with probability at least $1/2$; ring arithmetic needs a SPDZ2k-type backend~\cite{cramer2018spdz2k} with its own proof.

\textbf{Matrix checks.}
With $s=3$, each Freivalds call adds at most $p^{-3}\approx 2^{-183}$, i.e., about $2^{-151}$ for $Q_F\le 2^{32}$. Rejection sampling rejects one value with probability $2^{-61}$ per draw and retries under a fresh label; exhaustion affects only availability.

% =====================================================================
\subsection{Proof Boundary and Implementation Obligations}
\label{sec:sec-boundary}

\Cref{thm:main} concerns the abstract protocol in the protected-module model; \cref{tab:obligations} separates what this paper establishes from what a deployment must still provide. We executed a specification and a functional CPU reference model; its tests (\cref{sec:eval-attack}) check conformance on finite cases and are neither a machine-checked proof nor evidence for the statistical bound. GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet.

\begin{table}[t]
\centering
\caption{Proof boundary: what this paper establishes and what a deployment must still provide}
\label{tab:obligations}
\footnotesize
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}p{1.8cm}>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X}
\hline
\textbf{Obligation} & \textbf{Established here} & \textbf{Still required}\\
\hline
DPF/DCF, GaC, field, Boolean, LUT algebra & Explicit algorithms; \cref{thm:dpf-correct,thm:gac,thm:dcf,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval}; CPU reference tests & Constant-time, bit-exact CUDA and RTL refinement\\
\hline
Wrong-value authentication & \Cref{lem:hidden-key,thm:mac-sound}, independent lanes & Correct freeze, entropy, parser and check engine\\
\hline
End-to-end privacy and correctness & \Cref{thm:main} in the protected-module model & Realization of every module and trace assumption\\
\hline
PIR & \Cref{thm:pir} for the specified snapshot and regimes & Secure query channel, same-byte scan, certificates\\
\hline
GPU matrix verification & \Cref{thm:freivalds} & Protected verifier, bound input/result integration\\
\hline
Physical leakage and faults & Not claimed & Threat-specific engineering and evidence\\
\hline
Software-controlled DVFS and power telemetry & Required isolation specified & Isolated or monitored voltage and clock domain; telemetry filtering\\
\hline
Rollback protection & Required semantics specified (\cref{sec:proto-ledger}) & Monotonic service or erase-and-rekey lifecycle\\
\hline
Machine-checked proof & Not claimed & Future Lean, Coq or EasyCrypt development\\
\hline
\end{tabularx}
\end{table}

\textbf{Relation to the semi-honest design.}
The DFA analysis~\cite{dfa2026trusted} shows that its transformations preserve semi-honest security; \cref{thm:main} tolerates a malicious host and GPU by placing more integrity and lifecycle responsibility inside the boundary.


==> qa/draft2/sections/08_evaluation.tex <==
% =====================================================================
% Section VIII: Evaluation
% Numbers: model/numbers.md (red via \est{}), DFA paper (black + cite),
% executed CPU reference tests (black).
% =====================================================================
\section{Evaluation}\label{sec:eval}

We evaluate \sys along the integrity chain of \cref{sec:threat}: the cost of protected gates and verified openings (\cref{sec:eval-micro,sec:eval-check}), end-to-end inference against semi-honest trusted DFA and dealer-based malicious FSS (\cref{sec:eval-e2e}), PIR (\cref{sec:eval-pir}), attack coverage and silicon cost (\cref{sec:eval-attack,sec:eval-hw}), and ablations and scaling (\cref{sec:eval-ablation,sec:eval-scale}).

% =====================================================================
\subsection{Evaluation Methodology}\label{sec:eval-method}

\textbf{Evidence status.}
We distinguish three kinds of numbers.
Black numbers cited to~\cite{dfa2026trusted} are copied from the semi-honest DFA paper; its end-to-end rows combine measured A100 execution with simulated DFA hardware.
Black numbers without a citation are analytical (operation counts, design constants and security parameters such as $p=2^{61}-1$, $t=3$ and $Q(2/p)^t$) or counts from the executed CPU reference tests of \cref{sec:eval-attack}.
Red marks assumed model parameters and outputs of the analytical performance model of \cref{app:model}; they are placeholders to be replaced by measurements.
We executed a specification and a functional CPU reference model; GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet.
Every conclusion drawn from a red number is therefore conditional on the model assumptions, and we name the dominant assumption wherever a conclusion depends on it.

\textbf{Hardware cost.}
The DFA blocks that \sys reuses (16 DPF units with 64 AES-128 engines, SRAM buffers, a 16-lane Ara VPU~\cite{cavalcante2019ara} and an SC300-class control core~\cite{st33tpm12spi,arm_cortex_m3}) keep the TSMC 28~nm synthesis results of~\cite{dfa2026trusted}, which use a pipelined open-source AES-128 core~\cite{opencores_aes128_pipeline}.
For the blocks that \sys adds (\cref{sec:arch-hw}), namely the Mersenne-61 field unit array (FUA), the check engine, the AEAD/GHASH block shared by the freezer and the peer-channel controller, the ledger with release guard and parser, and the ledger and freeze SRAMs, this paper reports pre-synthesis component estimates at the DFA clock (720~MHz at 28~nm, 910~MHz at 7~nm); they will be replaced by synthesis in the same 28~nm flow.
As in DFA, we scale to 7~nm with DeepScaleTool~\cite{sarangi2021deepscaletool}.
Separately, we size a functional prototype on a ZCU102 board (XCZU9EG, ffvb1156, speed grade $-2$)~\cite{amd2023zcu102} for Vivado implementation; its resource and power figures are pre-implementation estimates and will be reported separately from measured board energy.

\textbf{System-level performance.}
The target methodology for headline numbers is that of DFA: the module sits next to the GPU L2 slices, where DFA delivers about 290~GB/s~\cite{dfa2026trusted}, its DPF and FSS work is modeled as a stream consumed by GPU kernels in Accel-Sim~\cite{khairy2020accel}, and non-FSS work comes from real GPU execution.
The three experiments of \cref{sec:arch-deploy} (A100 software, ZCU102 prototype, Accel-Sim on-die study) are never merged.
Until they are measured, every \sys row comes from a decomposition of DFA's trusted-mode rows into GPU linear algebra, other GPU work, module FSS work, CPU-GPU transfers, online bytes and online rounds, transformed for four authenticated lanes, exact Mersenne GEMM and doubled rounds; all constants are in \cref{app:model} and \cref{tab:model-params}.
The decomposition parameters are fitted to the LAN and WAN latencies of~\cite{dfa2026trusted} (largest deviation \est{0.42\%}, ResNet-50 LAN).
Two published latencies per model cannot identify five parameters, so the fit is a consistency constraint, not a validation; the split between GPU linear algebra, other GPU work, bytes and rounds, on which every malicious factor acts, is itself an assumption to be replaced by profiling the A100 baseline.
Because authenticated GEMM dominates every malicious row, the most influential factor is the assumed \est{1.25$\times$} cost of exact 61-bit Mersenne GEMM over wraparound $\Z_{2^{64}}$ GEMM per lane; Tensor Cores are not used for field arithmetic (\cref{sec:arch-field}).

\textbf{Baselines.}
For private inference we compare five configurations per model.
\emph{GPU (SH)} and \emph{GPU+Trusted DFA (SH)} are the semi-honest rows of~\cite{dfa2026trusted}, which build on Orca~\cite{jawalkar2024orca} for CNNs and Sigma~\cite{gupta2023sigma} for Transformers.
\emph{Dealer-based malicious FSS} is modeled after the protocol family of Shark~\cite{gupta2025shark}: an external dealer ships authenticated keys and preprocessing, which we model with assumed factors (\cref{app:model}) of \est{2.2$\times$} the semi-honest key and preprocessing volume, \est{2.0$\times$} the GPU FSS evaluation work and \est{2.4$\times$} the semi-honest GPU energy, while charging exactly the same authenticated linear algebra, online bytes and doubled rounds as \sys.
The comparison therefore isolates preprocessing and key handling; it does not equalize trust.
The dealer of this protocol family is an input-independent third party that can run offline and away from both servers, and it never sees an input or an opening, so breaking privacy requires its masks together with a server's view.
The \sys modules sit inside the adversary's platform and see every input and opening (\cref{sec:threat-model}), so extracting the secrets of either module suffices.
The speedups below are therefore obtained under a stronger hardware-confidentiality assumption; a deployment that cannot accept it must use \ProfU, which we do not evaluate.
The row models the protocol family, not the Shark artifact, and we make no performance claim against Shark itself until a matching artifact has been run.
We do not model a dealer-free (MASCOT, SPDZ2k or PCG-based) malicious baseline~\cite{keller2016mascot,cramer2018spdz2k,boyle2019pcg}; \cref{sec:analysis-cost} explains why its FSS keys remain costly.
\emph{GPU+\sys w/o GaC} generates authenticated material locally but, like the corresponding DFA ablation, spills it to host memory through the AEAD spill path and rereads it.
\emph{GPU+\sys} is the compiler-selected default.
For PIR we compare GPU-DPF~\cite{lam2023gpu} and GPU+DFA, both semi-honest and taken from~\cite{dfa2026trusted}, a GPU-DPF variant that adds authenticated PIR in the style of Colombo et al.~\cite{colombo2023apir} (assumed to reach \est{0.45$\times$} the GPU-DPF throughput at \est{350~W}), and GPU+\sys.

\textbf{Workloads.}
We run ResNet-50~\cite{he2016deep}, BERT-Base~\cite{devlin2019bert}, GPT-Neo~\cite{brown2020language} and LLaMA2-7B~\cite{touvron2023llama}, with 128 input tokens for the Transformer models, as in~\cite{dfa2026trusted}.
LAN is 1~GB/s with a 0.05~ms round-trip time (RTT) and WAN is 70~MB/s with a 70~ms RTT, following~\cite{gupta2023sigma,jawalkar2024orca,huang2026beyond}.
Malicious configurations use $\Fp$ with $p=2^{61}-1$ and $t=3$ MAC lanes; semi-honest rows use $\Z_{2^{64}}$ as in their sources.
Unless stated otherwise, the compiler selects among direct, LUT and interval gates by modeled cost subject to the FSS-portability constraint (\cref{sec:proto-direct,app:model}).
PIR databases hold 16K to 4M entries of 128 bits (\cref{tab:pir}), served in batches of 512 queries; \cref{fig:scale} extrapolates the model to 16M ($2^{24}$) entries.
We do not report inference accuracy; exact finite-reference agreement and model accuracy will be reported once bit-exact GPU conformance is established.

\textbf{Measurement protocol.}
The replacement measurements will use 5 warm-up runs and 30 measured repetitions, report the median and the 95th percentile with bootstrap confidence intervals, keep raw per-run records, and fix random seeds only for public synthetic inputs, since randomness used for security must remain fresh.
We will report per-stage service times (cold and amortized setup, preprocessing, online arithmetic, nonlinear evaluation, checking, transfers and final release) next to the critical-path wall time, counting both parties and any external preprocessing service.
Network conditions are shaped on dedicated interfaces with Linux traffic control, recording achieved throughput and RTT.
GPU energy integrates sampled GPU power, board energy is measured at the rail or the wall, and every energy figure is cross-checked against average power times latency (or throughput times energy per query).

% =====================================================================
\subsection{Microbenchmarks}\label{sec:eval-micro}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_dpfthr.pdf}
\caption{Single-path DPF gate throughput per module (M gates/s, log scale) at 28~nm, 720~MHz and 64 AES-128 engines, for input length $n$: semi-honest trusted DFA, \sys (GaC with fresh authentication epilogue), and a malicious variant with per-lane tag trees ($t=3$ extra trees). Model estimates.}
\label{fig:dpfthr}
\end{figure}

\textbf{DPF gate throughput.}
\sys sustains \est{106} against \est{113}~M~gates/s for trusted DFA at $n=61$ and stays \est{6--9\%} below it for all $n$, because the epilogue adds two AES blocks per gate and we assume a pipeline efficiency of \est{0.85} (\est{0.90} for trusted DFA; \cref{app:model}).
It is \est{3.8--4.0$\times$} faster than per-lane tag trees for all $n$, approaching the factor $1+t=4$ by which tag trees multiply DPF work (\cref{fig:dpfthr,tab:gatecost}), with a single-gate latency of \est{1.71~$\mu$s} at $n=61$.
These are DPF gate rates: complete gates also include input masking, a verified opening and the surrounding arithmetic (\cref{sec:eval-e2e}).

\begin{table}[t]
\centering
\caption{Authenticated Nonlinear Gate Options per Module}
\label{tab:gates}
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l r r r r r}
\hline
\textbf{Gate} & \makecell{\textbf{Online}\\\textbf{rounds}} & \makecell{\textbf{AES}\\\textbf{blocks}} & \makecell{\textbf{Field}\\\textbf{mults}} & \makecell{\textbf{Thr.}\\\textbf{(M/s)}} & \makecell{\textbf{LAN lat.}\\\textbf{(ms)}} \\
\hline
Direct protected gate & 1 & 2 & 5 & \est{1{,}800} & \est{0.100} \\
LUT, $w=8$ & 1 & 542 & 268 & \est{72.3} & \est{0.100} \\
LUT, $w=12$ & 1 & 8{,}238 & 4{,}112 & \est{4.75} & \est{0.100} \\
LUT, $w=16$ & 1 & 131{,}134 & 65{,}556 & \est{0.30} & \est{0.104} \\
Interval, conservative DCF & 1 & 22{,}692 & 8 & \est{1.73} & \est{0.100} \\
Interval, optimized DCF$^{\ast}$ & 1 & \est{976} & 8 & \est{40.1} & \est{0.100} \\
Bit decomposition & 123 & 244 & 122 & n/a & \est{12.3} \\
Exact signed truncation & 309 & n/m & 307 & n/a & \est{30.9} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize $n=61$; 28~nm, 720~MHz, 64 AES engines, 128 field lanes. Rounds, AES blocks and field multiplications are analytical counts per gate; throughput and LAN latency are model estimates. One online round is one \CheckOpen, i.e., two inter-module round trips; rounds include masked openings. n/a: round-bound, throughput not meaningful; n/m: not modeled.
$^{\ast}$Projected $O(n)$ DCF; not covered by \cref{thm:dcf}.}
\end{table}

\textbf{Nonlinear gates.}
\Cref{tab:gates} compares the authenticated gate options of \cref{sec:proto-gates}.
All single-opening gates pay the two-round-trip floor of one \CheckOpen{} (0.1~ms on LAN) and differ only in throughput, which favors the direct gate (\est{1{,}800}~M~gates/s) and small LUTs (LUT work grows as $2^w$) and penalizes the conservative DCF (\est{1.73}~M~gates/s); the optimized DCF would reach \est{40.1}~M~gates/s but lies outside our proofs.
Bit decomposition and exact signed truncation are round-bound (123 and 309 rounds, \est{12.3~ms} and \est{30.9~ms} on LAN), so the compiler uses them only as a fallback when no table or interval formulation of the gate exists.

% =====================================================================
\subsection{Cost of Verified Openings}\label{sec:eval-check}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_checkopen.pdf}
\caption{\CheckOpen{} cost versus batch size $m$ (64 to 65{,}536 elements): (a)~LAN latency for $t=1,2,3$ MAC lanes (the curves overlap); (b)~throughput on LAN and WAN for $t=3$ (log scale). Model estimates.}
\label{fig:checkperf}
\end{figure}

\Cref{fig:checkperf} sweeps the \CheckOpen{} batch size $m$ from 64 to 65{,}536 elements, and three observations guide the compiler.
First, the number of MAC lanes barely matters for cost: even at $m=65{,}536$, moving from $t=1$ to $t=3$ raises LAN latency only from \est{0.648~ms} to \est{0.652~ms}, while the statistical term improves from $2^{-28}$ to $2^{-148}$ at $Q=2^{32}$ (\cref{thm:mac-sound}).
Second, on LAN the two round trips (0.1~ms) dominate up to a few thousand elements (\est{0.101~ms} to \est{0.135~ms} between $m=64$ and $m=4{,}096$); beyond that the 8-byte value share per element on the peer link dominates (\est{0.52~ms} of \est{0.652~ms} at $m=65{,}536$), throughput saturates near \est{100}~M~elements/s, and the protected work stays below \est{5\%} of the check latency.
Third, on WAN the two 70~ms round trips set a floor of 140~ms per check, so throughput is only \est{0.44}~M~elements/s even at $m=65{,}536$; batching independent openings (\cref{sec:proto-check}) is therefore essential, and the round count, rather than bandwidth or module work, is the WAN price of malicious security (\cref{sec:eval-ablation}).

% =====================================================================
\subsection{End-to-End Private Inference}\label{sec:eval-e2e}

\begin{table*}[t]
\centering
\caption{End-to-End Private Inference per Query}
\label{tab:e2e}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l l c r r r r r r}
\hline
\textbf{Model} & \textbf{Method} & \textbf{Security} & \makecell{\textbf{Offline}\\\textbf{comm. (GB)}} & \makecell{\textbf{CPU-GPU}\\\textbf{(GB)}} & \makecell{\textbf{Module-GPU}\\\textbf{(GB/party)}} & \makecell{\textbf{LAN}\\\textbf{latency (s)}} & \makecell{\textbf{WAN}\\\textbf{latency (s)}} & \makecell{\textbf{GPU+module}\\\textbf{energy (J)}} \\
\hline
\multirow{5}{*}{ResNet-50}
 & GPU~\cite{dfa2026trusted} & SH & 9.9 & 10.2 & n/a & 10.9 & 162 & 71.0 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.02 & 0.34 & n/r & 0.73 & 18.0 & 11.9 \\
 & Dealer-based malicious FSS & Mal & \est{21.8} & \est{22.4} & n/a & \est{25.1} & \est{346} & \est{170} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{38.0} & \est{1.22} & \est{2.97} & \est{34.7} & \est{48.6} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{0.44} & \est{1.22} & \est{1.79} & \est{33.6} & \est{43.6} \\
\hline
\multirow{5}{*}{BERT-Base}
 & GPU~\cite{dfa2026trusted} & SH & 17.1 & 19.3 & n/a & 18.8 & 296 & 121 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.1 & 2.55 & n/r & 1.42 & 46.4 & 18.2 \\
 & Dealer-based malicious FSS & Mal & \est{37.6} & \est{42.5} & n/a & \est{43.9} & \est{630} & \est{290} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{68.6} & \est{1.66} & \est{5.87} & \est{91.8} & \est{82.2} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{3.31} & \est{1.66} & \est{3.83} & \est{89.7} & \est{73.7} \\
\hline
\multirow{5}{*}{GPT-Neo}
 & GPU~\cite{dfa2026trusted} & SH & 76.4 & 80.4 & n/a & 83.6 & 1{,}140 & 587 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.24 & 4.27 & n/r & 5.93 & 101 & 114 \\
 & Dealer-based malicious FSS & Mal & \est{168} & \est{177} & n/a & \est{197} & \est{2{,}611} & \est{1{,}409} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{296} & \est{9.92} & \est{28.6} & \est{209} & \est{522} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{5.55} & \est{9.92} & \est{19.5} & \est{200} & \est{477} \\
\hline
\multirow{5}{*}{LLaMA2-7B}
 & GPU~\cite{dfa2026trusted} & SH & 256 & 268 & n/a & 279 & 3{,}695 & 1{,}879 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.81 & 12.8 & n/r & 18.0 & 193 & 303 \\
 & Dealer-based malicious FSS & Mal & \est{563} & \est{590} & n/a & \est{661} & \est{8{,}467} & \est{4{,}510} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{994} & \est{33.3} & \est{93.6} & \est{418} & \est{1{,}483} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{16.6} & \est{33.3} & \est{63.1} & \est{387} & \est{1{,}343} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\textwidth}{\footnotesize SH: semi-honest; Mal: static malicious security with abort. Latency is end to end, including offline distribution where present. Energy is GPU plus module energy summed over both computing parties (and the dealer when present). Module-GPU is the authenticated tuple stream per party on the on-die path; n/a: no module; n/r: not reported in~\cite{dfa2026trusted}. SH rows are copied from~\cite{dfa2026trusted}; red values are model estimates.}
\end{table*}

\Cref{tab:e2e} reports per-query results for the four models.
The semi-honest rows are context, not same-security competitors.

\textbf{Comparison with dealer-based malicious FSS.}
The modeled dealer-based baseline pays for malicious security mainly offline: its dealer ships \est{21.8--563~GB} of authenticated keys and preprocessing per query, which each party then stages through CPU-GPU transfers, whereas \sys generates the authenticated correlations inside the modules and ships none of them (\est{$<$0.001~GB} of session setup).
Across the four models this yields \est{10.1--14.0$\times$} lower LAN latency, \est{7.0--21.9$\times$} lower WAN latency and \est{3.0--3.9$\times$} lower energy than the modeled baseline (\est{11.4$\times$}, \est{7.0$\times$} and \est{3.9$\times$} for BERT-Base); the energy ratio rests on the assumed \est{2.4$\times$} energy factor of the baseline.
These latency ratios include the per-query offline distribution; excluding it, \sys is \est{1.5--1.8$\times$} faster on LAN (\est{1.6$\times$} for BERT-Base), and with no authenticated-key blow-up ($\kappa_{\mathrm{key}}=1$) the baseline still needs \est{22.4~s} for BERT-Base (\est{5.8$\times$}).
The end-to-end gains thus come mainly from generating authenticated correlations inside the modules; the epilogue's advantage (\est{3.8--4.0$\times$} over per-lane tag trees) is per gate.
The WAN gain is largest for LLaMA2-7B (\est{21.9$\times$}), whose \est{563~GB} of authenticated material alone would occupy a 70~MB/s link for more than \est{2.2~hours}.

\textbf{Cost of malicious security.}
Relative to semi-honest trusted DFA, \sys raises LAN latency by \est{2.46--3.51$\times$} (\est{2.7$\times$} for BERT-Base) and WAN latency by \est{1.86--2.01$\times$}; these factors rest on the assumed Mersenne GEMM cost, and doubling it ($\mu_{\mathrm{M}}=2$) would give \est{5.39~s}, or \est{3.8$\times$}, for BERT-Base (\cref{sec:arch-field}).
It nevertheless remains \est{4.3--6.1$\times$} faster on LAN and \est{3.3--9.5$\times$} faster on WAN than the semi-honest GPU baseline, and it uses \est{1.2--1.6$\times$} less energy, although it tolerates a malicious host.
CPU-GPU traffic is assumed to grow by \est{1.3$\times$} over trusted DFA ($\phi_{\mathrm{cg}}$, \cref{app:model}) for canonical field words, residuals and certificates; the authenticated tuples themselves (\est{1.22} to \est{33.3~GB} per party) take the on-die module-GPU path and do not add to it.

\textbf{Generate-and-consume remains essential.}
Without GaC, the locally generated authenticated material must be spilled and reread, which inflates CPU-GPU traffic by \est{20.7--86$\times$} (\est{68.6~GB} instead of \est{3.31~GB} for BERT-Base) and LAN latency by \est{1.47--1.66$\times$}.
The authenticated representation makes materialization costlier than in the semi-honest case, where DFA reports 36.1~GB of CPU-GPU traffic and a 1.74$\times$ LAN penalty for BERT-Base without GaC~\cite{dfa2026trusted}.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_bert.pdf}
\caption{BERT-Base bottleneck analysis for \sys (model estimates). (a)~Speedup over dealer-based malicious FSS versus network bandwidth, split into the part due to eliminated key and preprocessing distribution and the remainder. (b)~LAN latency versus host-module link bandwidth (\est{1.6}, \est{8}, \est{25} and 290~GB/s~\cite{dfa2026trusted}). (c)~Breakdown of the \est{3.83~s} LAN latency.}
\label{fig:bert}
\end{figure}

\textbf{Bottleneck analysis.}
\Cref{fig:bert} decomposes the BERT-Base results.
(a)~The advantage over the dealer-based baseline depends on network bandwidth: \est{43.7$\times$} at 0.1~GB/s, \est{11.4$\times$} at 1~GB/s and \est{2.9$\times$} at 10~GB/s.
At 1~GB/s, \est{9.8$\times$} of the \est{11.4$\times$} comes from eliminated key and preprocessing distribution; at 10~GB/s the remaining \est{1.7$\times$} from lower key I/O and cheaper FSS evaluation dominates.
Faster networks shrink the advantage but do not remove it, and, as observed for the semi-honest case~\cite{dfa2026trusted,huang2026beyond}, the energy and monetary cost of moving tens of gigabytes per query persists at any bandwidth.
(b)~Moving the module off die costs little for BERT-Base: LAN latency is \est{3.83~s} on die (290~GB/s), \est{3.87~s} over a \est{25~GB/s} PCIe-class link, \est{3.96~s} at \est{8~GB/s} and \est{4.46~s} at the \est{1.6~GB/s} of the ZCU102 prototype, because only \est{1.66~GB} of authenticated tuples per party cross the link.
(c)~The breakdown confirms Observation~2 of \cref{sec:analysis-cost}: authenticated GEMM accounts for \est{68\%} of the latency and \est{86\%} of the \est{2.41~s} added over trusted DFA, so the protected module is not the bottleneck; the tag lanes on the GPU and the doubled round count are, which motivates the compressed-check direction of \cref{sec:eval-scale}.

% =====================================================================
\subsection{Private Information Retrieval}\label{sec:eval-pir}

\begin{table}[t]
\centering
\caption{PIR Throughput and Energy per Query}
\label{tab:pir}
\footnotesize
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l l c c r r r}
\hline
\textbf{DB} & \textbf{Method} & \textbf{Integ.} & \makecell{\textbf{Index}\\\textbf{hidden}$^{\dagger}$} & \makecell{\textbf{Queries/s}\\\textbf{(k)}} & \makecell{\textbf{Energy/}\\\textbf{query (mJ)}} & \makecell{\textbf{Implied}\\\textbf{W}} \\
\hline
\multirow{4}{*}{16K}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & \cmark & 134 & 2.61 & 350 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & \cmark & 1{,}125 & 0.187 & 210 \\
 & GPU-DPF+APIR & \cmark & \cmark & \est{60.3} & \est{5.80} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \xmark & \est{1{,}046} & \est{0.180} & \est{188} \\
\hline
\multirow{4}{*}{1M}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & \cmark & 3.48 & 100 & 348 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & \cmark & 17.58 & 11.9 & 209 \\
 & GPU-DPF+APIR & \cmark & \cmark & \est{1.57} & \est{224} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \xmark & \est{16.35} & \est{11.5} & \est{188} \\
\hline
\multirow{4}{*}{4M}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & \cmark & 0.788 & 443 & 349 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & \cmark & 4.39 & 47.7 & 209 \\
 & GPU-DPF+APIR & \cmark & \cmark & \est{0.355} & \est{987} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \xmark & \est{4.08} & \est{46.0} & \est{188} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize 128-bit entries, batch 512. SH rows are from~\cite{dfa2026trusted} with energy expressed in mJ; implied power is throughput times energy per query and serves as a unit cross-check. Integ.: the client obtains the committed record or abort against a malicious server host (R1). $^{\dagger}$Index hidden from each server without trusted hardware: GPU-DPF and GPU+DFA (untrusted mode, client-generated keys) and the APIR variant hide $\alpha$ from each server, whereas both \sys modules learn $\alpha$ and its query privacy relies on module trust. Red values are model estimates.}
\end{table}

\Cref{tab:pir} reports PIR throughput and energy per query.
Assuming a PIR efficiency of \est{0.93} relative to DFA ($\eta_{\mathrm{PIR}}$, \cref{app:model}), meant to cover snapshot hashing, the in-module record reduction and fresh resharing with bound certificates, \sys reaches \est{1{,}046}, \est{16.35} and \est{4.08}~k~queries/s, a consequence of this assumption to be replaced by the Accel-Sim study, not a result.
The integrity guarantee does not depend on the model: in regime (R1), with one malicious server host, an honest client receives the committed record or abort (\cref{thm:pir}).
Query privacy, however, is weaker than in untrusted two-server DPF-PIR: both modules learn $\alpha$, so privacy against the hosts relies on module trust, whereas GPU-DPF and untrusted-mode DFA hide $\alpha$ from each server without trusted hardware (\cref{app:func-pir}); the two \ProfT alternatives of \cref{sec:proto-pir} are not modeled.
Energy per query is \est{3--4\%} below DFA's (\est{0.180~mJ} vs.\ 0.187~mJ at 16K entries) only because we assume an average power of \est{188~W} ($P_{\mathrm{PIR}}$), with the record reduction moved from the SMs into the protected path; this is the least certain PIR value and among the first we will measure.
Likewise, the authenticated GPU baseline is an assumed \est{0.45$\times$} of GPU-DPF throughput at \est{350~W}, so the \est{10.4--17.4$\times$} higher throughput and \est{19--32$\times$} lower energy per query of \sys against it follow from these assumptions; against semi-honest GPU-DPF, \sys is \est{4.7--7.8$\times$} faster under a weaker query-privacy model.

\textbf{Bottleneck analysis.}
As in DFA, full-domain PIR is bound by DPF expansion in the AES array rather than by memory; DFA expands about 18.4~G~leaves/s~\cite{dfa2026trusted}.
The additional protected work is amortized over a batch: each batch of 512 queries scans the snapshot once in public order, so the snapshot hash costs one pass per batch rather than one per query, and every record is weighted by the 512 DPF outputs of the batch in the FUA.
At 16K entries this reduction needs about \est{51~G} field multiply-accumulates/s, below the 116~G/s peak of the 128-lane FUA at 910~MHz (\cref{app:model}).
This capacity check shows only that the FUA is not saturated; it does not establish the size of the throughput loss.

% =====================================================================
\subsection{Security Validation}\label{sec:eval-attack}

\begin{table*}[t]
\centering
\caption{Attack and Fault Injections and Their Expected Outcomes}
\label{tab:attacks}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{c >{\raggedright\arraybackslash}p{4.3cm} >{\raggedright\arraybackslash}p{5.0cm} c >{\raggedright\arraybackslash}p{4.9cm}}
\hline
\textbf{\#} & \textbf{Injection} & \textbf{Mechanism} & \makecell{\textbf{Reference}\\\textbf{model}} & \textbf{Expected RTL/FPGA outcome} \\
\hline
1 & Change payload, query, role, gate id, table hash or shape (S5) & Ledger descriptor binding; role- and gate-bound PRF labels (\cref{sec:proto-ledger}) & \cmark & \est{Rejected at frame parse or authenticated computation fails; no preprocessing issued} \\
2 & Flip a control bit, root seed or correction word in a candidate engine & Conformance against the reference DPF (\cref{thm:dpf-correct}); unverified engine output is never authenticated & planned & \est{Reference mismatch flagged; engine output never authenticated or released} \\
3 & Change a GPU value share or tag (S1) & \CheckOpen{} with $t=3$ independent lanes (\cref{thm:mac-sound}) & \cmark & \est{Abort within one \CheckOpen{} (0.10--0.65~ms on LAN)}; acceptance at most $(2/p)^3$ per batch \\
4 & Triple with valid-looking tags but $c\neq ab$ (S7) & Triples computed inside the TCB; imported material needs a correctness proof & planned & \est{Never consumed; unproven import refused at reservation} \\
5 & Reuse a mask or counter; reset and resume old keys (S4) & One-time ledger, epoch poisoning, erase-and-rekey & \cmark & \est{Rejected before any accepted reuse} \\
6 & Modify a DMA buffer after freezing (S3) & Freeze-before-challenge; consume only frozen pages & \cmark & \est{Frozen authenticated bytes consumed, or abort} \\
7 & Swap only the last column of a GPU matrix product & Frozen-operand Freivalds over all columns, $s=3$ (\cref{thm:freivalds}) & planned & \est{Rejected}, except with probability at most $p^{-3}$ \\
8 & Reuse one challenge vector across MAC lanes & Independent per-lane challenges; configuration check & \cmark\,(toy) & \est{Configuration refused at session setup} \\
9 & Change database bytes or version after hashing (S8) & Same-byte snapshot hash and certificate binding (\cref{thm:pir}) & \cmark & \est{Abort; quarantined result never released} \\
10 & Request output before the verification barrier (S6) & Release guard (\cref{sec:proto-ledger}) & planned & \est{Guard stays closed; no candidate values leave} \\
11 & Overflow or truncate with the wrong signed rule & Exact finite reference; numeric contract (\cref{thm:cmp-trunc}) & \cmark & \est{Mismatch detected; manifest rejected} \\
12 & Delay, drop or reorder packets (S10) & Bounded resources and abort & planned & \est{Abort; no fairness or availability claimed} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\textwidth}{\footnotesize Reference model: \cmark{} executed and passing in the CPU reference model; planned: no executed evidence yet. Red outcomes are expected on the RTL and FPGA implementations, not yet observed. Scenario IDs refer to \cref{tab:scenarios}.}
\end{table*}

\Cref{tab:attacks} lists the twelve attack and fault injections of our test plan, the mechanism that must stop each one, whether the executed CPU reference model already covers it, and the outcome we expect on the RTL and FPGA implementations.
The injections cover the scenarios of \cref{tab:scenarios} except S2, which the interface excludes by construction, and S9, which the functionality permits (its commitment-bound loader variant is covered by the model-provenance mechanism, not by an injection).
For S2, the command set of \cref{tab:commands} has no entry point that authenticates a host-supplied value, and row~2 checks the related requirement that even the module's own engine output is never authenticated before it conforms to the reference.

\textbf{Executed functional validation.}
The functional reference implements the ideal-module model in Python~3.10+ using only the standard library.
In the preparation environment it passes 22 unit tests with 0 failures and 0 errors.
The tests cover 21{,}840 exhaustive small-domain DPF target, query and payload cases (\cref{thm:dpf-correct}); 2{,}728 party-local comparisons between streaming GaC and materialized evaluation (\cref{thm:gac}); 1{,}364 DCF comparisons (\cref{thm:dcf}); 20{,}004 CPU checks of the GPU Mersenne multiplication formula of \cref{sec:arch-field} against arbitrary-precision arithmetic, including boundary operands; all 31 elements of a toy field with $p=31$ for bit decomposition (\cref{thm:bitdec}); 124 signed-truncation cases (\cref{thm:cmp-trunc}); all 16 inputs of a small LUT (\cref{thm:lut}); selected exhaustive toy intervals (\cref{thm:interval}); a small composed nonlinear and arithmetic pipeline; and PIR snapshot rejection.
Negative tests exercise noncanonical encodings, tag and value mutations, poisoned epochs, role, replay and ordering errors, immutable frozen objects, joint sampling, truncation fibers, and the ring zero-divisor counterexample that motivates the field representation (\cref{app:proof-auth}).

\textbf{Limits of this evidence.}
The toy field $p=31$ serves finite correctness tests only and provides no cryptographic security.
The reference expands seeds with SHAKE rather than the pinned AES-based PRG, so the equivalence tests must be rerun against the production PRG and output conversion.
The CUDA micro-test (65{,}536 products against a host 128-bit reference) is written but has not been compiled or run, and the RTL release guard is written but has not been simulated or synthesized; no GPU toolchain, Vivado or RTL simulator was available in that environment.
Rows marked ``planned'' in \cref{tab:attacks} therefore have no executed evidence yet.
These tests check that the implementation conforms to the algorithms; they do not measure a forgery probability.
Observing zero accepted forgeries in any finite campaign cannot support a bound such as $2^{-148}$; that bound comes from \cref{thm:mac-sound} together with the ledger rules.
Power and electromagnetic analysis, probing and fault injection require separate, threat-specific engineering evaluation (\cref{sec:discussion}).

% =====================================================================
\subsection{Hardware Cost}\label{sec:eval-hw}

\begin{table}[t]
\centering
\caption{Hardware Cost of One \sys Module}
\label{tab:hwcost}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l r r r r}
\hline
\multirow{2}{*}{\textbf{Component}} & \multicolumn{2}{c}{\textbf{28~nm}} & \multicolumn{2}{c}{\textbf{7~nm}} \\
\cline{2-5}
 & \textbf{mm$^2$} & \textbf{mW} & \textbf{mm$^2$} & \textbf{mW} \\
\hline
\multicolumn{5}{l}{\textit{DFA blocks reused by \sys~\cite{dfa2026trusted}}} \\
16 DPF units (64 AES-128) & 1.73 & 29 & 0.054 & 11 \\
SRAM buffers & 3.06 & 585 & 0.096 & 219 \\
VPU (16-lane Ara) & 1.97 & 794 & 0.062 & 298 \\
All DFA (incl.\ control core) & 7.67 & 1{,}683.5 & 0.239 & 631 \\
\hline
\multicolumn{5}{l}{\textit{Blocks added by \sys}} \\
Field unit array (128 lanes) & \est{2.80} & \est{1{,}000} & \est{0.088} & \est{375} \\
Check engine & \est{0.18} & \est{45} & \est{0.006} & \est{17} \\
AEAD/GHASH (freezer, peer channel) & \est{0.21} & \est{60} & \est{0.007} & \est{23} \\
Ledger, guard, parser & \est{0.09} & \est{12} & \est{0.003} & \est{5} \\
Ledger SRAM (32~KB) & \est{0.25} & \est{35} & \est{0.008} & \est{13} \\
Freeze SRAM (256~KB) & \est{1.07} & \est{200} & \est{0.033} & \est{75} \\
\cline{1-5}
\sys additions & \est{4.60} & \est{1{,}352} & \est{0.145} & \est{508} \\
\hline
\rowcolor{blue!6}All \sys & \est{12.27} & \est{3{,}036} & \est{0.384} & \est{1{,}139} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize DFA blocks are synthesis results from~\cite{dfa2026trusted}; blocks added by \sys are pre-synthesis estimates (red). 7~nm values are scaled with DeepScaleTool~\cite{sarangi2021deepscaletool}. One AEAD/GHASH block serves the freezer and the peer-channel controller. The 128 FUA lanes sit eight per DPF unit (area unchanged). \est{Not yet costed: the trusted on-die links between the DPF units, the VPU and the VIGOR core.}}
\end{table}

\begin{table}[t]
\centering
\caption{Planned ZCU102 Functional Prototype}
\label{tab:fpga}
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l r r r}
\hline
\textbf{Resource} & \textbf{Used} & \textbf{Available} & \textbf{Utilization} \\
\hline
LUT & \est{168K} & 274K & \est{61\%} \\
Flip-flop & \est{201K} & 548K & \est{37\%} \\
BRAM36 & \est{412} & 912 & \est{45\%} \\
DSP & \est{356} & 2{,}520 & \est{14\%} \\
\hline
\multicolumn{4}{l}{Datapath: \est{4} DPF units (\est{16} AES-128), \est{32} field lanes, \est{250~MHz}} \\
\multicolumn{4}{l}{DPF throughput: \est{1.0}~G~expansions/s; board power: \est{9.8~W}} \\
\multicolumn{4}{l}{Host link: \est{1.6~GB/s}, i.e., \est{50}~M authenticated elements/s} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize XCZU9EG-2FFVB1156~\cite{amd2023zcu102}: configuration and pre-implementation estimates (red).}
\end{table}

\Cref{tab:hwcost} reports the cost of one module; at 7~nm a complete module occupies \est{0.384~mm$^2$}, \est{0.046\%} of the 826~mm$^2$ A100 die~\cite{nvidia2020ampere}.
The FUA dominates the additions with \est{61\%} of the added area and \est{74\%} of the added power at 7~nm, followed by the 256~KB freeze SRAM with \est{23\%} of the added area, whereas the logic that enforces the security policy (ledger, release guard, parser and check engine) takes only \est{0.009~mm$^2$}, or \est{6\%} of the additions.
As in DFA, arithmetic and memory dominate the cost, not control.
No AES engines are added, because challenge derivation and AEAD freezing time-share the 64 engines with PRG expansion (\cref{sec:arch-hw}); for BERT-Base, checking occupies the AES array and the FUA for about \est{2.8~ms} per query, below \est{0.1\%} of its latency.

\Cref{tab:fpga} sizes the external ZCU102 prototype, which exists to check functional conformance and streaming behavior with two independent boards.
Its \est{1.6~GB/s} host link (\est{50}~M authenticated elements/s at 32 bytes each) and its smaller FUA make it a pessimistic functional point rather than a performance target (\cref{tab:ablation}), and it is not a \ProfT deployment target (\cref{sec:arch-deploy}).

% =====================================================================
\subsection{Ablation Study}\label{sec:eval-ablation}

\begin{table*}[t]
\centering
\caption{Ablation on BERT-Base}
\label{tab:ablation}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l c r r r r >{\raggedright\arraybackslash}p{5.1cm}}
\hline
\textbf{Configuration} & \textbf{Secure} & \makecell{\textbf{LAN}\\\textbf{(s)}} & \makecell{\textbf{Rel.}\\\textbf{LAN}} & \makecell{\textbf{WAN}\\\textbf{(s)}} & \makecell{\textbf{Energy}\\\textbf{(J)}} & \textbf{Note} \\
\hline
\rowcolor{blue!6}Compiler-selected default ($t=3$, batched checks) & \cmark & \est{3.83} & \est{1.00$\times$} & \est{89.7} & \est{73.7} & Reference configuration \\
w/o GaC & \cmark & \est{5.87} & \est{1.53$\times$} & \est{91.8} & \est{82.2} & Authenticated material spilled and reread \\
Tag trees instead of epilogue & \cmark & \est{4.12} & \est{1.08$\times$} & \est{90.0} & \est{80.4} & $(1+t)\times$ DPF work; FSS share is small \\
$t=1$ MAC lane & \xmark & \est{2.53} & \est{0.66$\times$} & \est{88.4} & \est{43.2} & $Q(2/p)^t=2^{-28}$ at $Q=2^{32}$: inadequate \\
$t=2$ MAC lanes & \cmark & \est{3.18} & \est{0.83$\times$} & \est{89.1} & \est{58.4} & $2^{-88}$ at $Q=2^{32}$ \\
FSS-only gates, conservative DCF & \cmark & \est{15.29} & \est{3.99$\times$} & \est{101.2} & \est{342.2} & $O(n^2)$ DCF of \cref{thm:dcf} \\
FSS-only gates, optimized DCF & \pmark & \est{4.20} & \est{1.10$\times$} & \est{90.1} & \est{82.3} & Projected; not covered by \cref{thm:dcf} \\
Direct protected gates only & \cmark & \est{3.82} & \est{1.00$\times$} & \est{89.7} & \est{73.3} & \ProfT only; drops the FSS-portability constraint \\
Small check batches ($m=64$) & \cmark & \est{4.24} & \est{1.11$\times$} & \est{90.2} & \est{74.6} & Per-batch overhead not amortized \\
External PCIe module (\est{25~GB/s}) & \cmark & \est{3.87} & \est{1.01$\times$} & \est{89.8} & \est{73.8} & Link roofline $B/32$ elements/s \\
ZCU102 link (\est{1.6~GB/s}, \est{32} lanes, \est{250~MHz}) & \cmark & \est{4.59} & \est{1.20$\times$} & \est{90.5} & \est{75.4} & Prototype link and slower triple generation \\
No \CheckOpen{} & \xmark & \est{3.80} & \est{0.99$\times$} & \est{50.5} & \est{73.6} & Insecure; performance lower bound only \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\textwidth}{\footnotesize LAN 1~GB/s, WAN 70~MB/s. Each row changes one choice of the compiler-selected default. Rel.\ LAN is LAN latency relative to the compiler-selected default. Secure: \cmark{} covered by our theorems; \pmark{} projected construction outside our proofs; \xmark{} not secure (statistically inadequate, or no verification). All latency and energy values are model estimates.}
\end{table*}

\Cref{tab:ablation} changes one design choice at a time for BERT-Base, and three conclusions follow.

\textbf{Protocol mechanisms.}
Generate-and-consume and the check round are the mechanisms that matter.
Disabling GaC costs \est{1.53$\times$} LAN latency (\cref{sec:eval-e2e}), and the insecure lower bound without \CheckOpen{} shows that the doubled round count costs \est{39~s} of the \est{89.7~s} WAN latency, the dominant WAN cost of malicious security.

\textbf{MAC lanes.}
$t$ is a security knob, not a performance one: $t=1$ saves \est{34\%} of the LAN latency but bounds a wrong opening only by $2^{-28}$, so the choice of $t=3$ follows from \cref{sec:sec-concrete} (\cref{tab:lanes}).

\textbf{Gate selection and placement.}
Because FSS is a small part of the malicious latency, tag trees, direct-only gates, small check batches and off-die placement change LAN latency by at most \est{20\%}; the epilogue matters most for LUT-heavy compiled models, where the \est{3.8--4.0$\times$} gate-level gap over per-lane tag trees (\cref{sec:eval-micro}) carries over.
The exception is FSS-only compilation with the conservative DCF of \cref{thm:dcf} (\est{3.99$\times$}), which is why the compiler selects gates by cost.
Direct-only (\est{3.82~s}) is marginally faster than the default (\est{3.83~s}) because the default keeps an FSS realization for gate shapes that the manifest marks as FSS-portable, so that the same compiled circuit runs under \ProfU; this allowance costs about \est{0.014~s} of module time (\cref{app:model}), and direct-only drops it and runs only under \ProfT (\cref{sec:proto-direct}).
Ablations on staged versus local checks and on caching versus recomputing bit decompositions are part of the measurement plan but are not yet modeled.

% =====================================================================
\subsection{Scalability}\label{sec:eval-scale}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_scale.pdf}
\caption{Scalability (model estimates). (a)~LAN latency with $t=1,2,3$ MAC lanes, normalized to semi-honest trusted DFA, annotated with the statistical term $Q(2/p)^t$ at $Q=2^{32}$ ($2^{-28}$, $2^{-88}$, $2^{-148}$). (b)~PIR throughput (queries/s, log scale) for $2^{14}$ to $2^{24}$ entries; points beyond $2^{22}$ entries are extrapolated.}
\label{fig:scale}
\end{figure}

\textbf{MAC lanes and model size.}
\Cref{fig:scale}(a) normalizes LAN latency to semi-honest trusted DFA.
With $t=3$ the overhead grows from \est{2.46$\times$} for ResNet-50 to \est{3.51$\times$} for LLaMA2-7B, because the share of linear algebra grows with model size and each MAC lane replicates it: every additional lane adds about \est{0.65~s} for BERT-Base and \est{13.0~s} for LLaMA2-7B.
Authenticated GEMM on the GPU, not the protected module, is the scaling bottleneck.

\textbf{Triple generation.}
Correct matrix triples must be computed inside the protected boundary (\cref{sec:proto-arith}), so FUA work scales with the model's multiply-accumulate count.
LLaMA2-7B needs about \est{7.18~s} of FUA time per query at 128 lanes and 910~MHz, which overlaps with the \est{52.0~s} of authenticated GEMM and leaves about \est{0.72~s} exposed.
The \est{32}-lane prototype at \est{250~MHz} would need about \est{105~s} for the same triples, another reason it is only a functional prototype; the on-die FUA should scale with the linear-algebra throughput of the host GPU.
If triple generation ever dominates, the alternatives are an imported malicious preprocessing backend with its own proof, or restructuring public-by-secret operations; exposing global secret masks to the GPU is not an option.

\textbf{Host-module bandwidth.}
BERT-Base moves only \est{1.66~GB} per party, well inside the $B/32$ roofline of \cref{sec:arch-insight}, which is why \cref{fig:bert}(b) is nearly flat above \est{8~GB/s}.

\textbf{PIR.}
\Cref{fig:scale}(b) shows PIR throughput from $2^{14}$ to $2^{24}$ entries.
Like DFA, \sys scales linearly in the number of entries, from \est{1.05}~M down to \est{1{,}022}~queries/s, whereas GPU-DPF reaches its peak per-entry efficiency near $2^{20}$ entries~\cite{dfa2026trusted,lam2023gpu}.
At $2^{24}$ entries \sys is \est{5.2$\times$} faster than GPU-DPF, under the weaker query-privacy model of \cref{sec:eval-pir}, and \est{11.5$\times$} faster than the authenticated GPU baseline.
Larger records increase the per-entry field reduction linearly while the DPF expansion stays unchanged, so for very large records the FUA, not the AES array, becomes the limit.

\textbf{Beyond per-lane tags.}
Because the tag lanes dominate large models, the most promising direction is to compress MAC checking, for example with rank-1 compressed checks that avoid carrying $t$ full tag arrays through the GPU.
Such schemes are not covered by our proofs and need their own soundness analysis, so we leave them to future work.
Scaling the number of DPF units and FUA lanes is a second, orthogonal knob; DFA found DPF-unit scaling to be nearly linear until on-chip bandwidth, about 7~TB/s of aggregate L2 read bandwidth on A100~\cite{nvidia2020ampere}, becomes the limit~\cite{dfa2026trusted}.


==> qa/draft2/sections/09_discussion.tex <==
% ==================================================================
% Section IX: Discussion and Limitations
% Owner labels: sec:discussion
% ==================================================================
\section{Discussion and Limitations}
\label{sec:discussion}

\sys claims that, under \ProfT, one maliciously corrupted host, including its GPU, driver and network stack, cannot make an honest party accept a wrong value or release an unauthorized one, except with the probability bounded in \cref{thm:main}. We now state what this claim does not cover and which evidence is still missing.

\textbf{Trust relocation, not removal.}
\sys moves the dealer of dealer-based FSS into two protected modules; it does not remove the dealer assumption. Both modules hold the joint-sampler key and the global MAC keys $\Delta_1,\dots,\Delta_t$ (\cref{sec:proto-setup}), so extracting the secrets of either module voids privacy and integrity for every session whose keys it holds. \Cref{thm:main} is a stand-alone statement under sequential composition; concurrent sessions that share module state are not covered (\cref{app:func}). The boundary also grows relative to DFA~\cite{dfa2026trusted}: the ledger, freezer, check engine, field unit array and release guard add only \est{0.145~mm$^2$} at 7~nm (\cref{tab:hwcost}), but each of them is logic that must be verified (\cref{tab:obligations}).

\textbf{What the modules learn.}
The modules are not blind. $\Pi_{\mathsf{Input}}$ validates $x^{*}=r+\varepsilon$ inside them (\cref{fig:arith}); after a verified opening $c = x + r$, module $T_b$ knows $c$ and $r$, hence $x$; the committed-input loader and the direct gate (\cref{sec:proto-direct}) see inputs explicitly; and in PIR both modules learn the client's index $\alpha$ (\cref{alg:pir}). For inference this is inherent to generate-and-consume and already holds for trusted DFA~\cite{dfa2026trusted}. For PIR it is a regression: the query privacy of \sys relies on module trust, whereas untrusted two-server DPF-PIR, such as GPU-DPF~\cite{lam2023gpu} and untrusted-mode DFA~\cite{dfa2026trusted}, hides $\alpha$ without trusted hardware. Client-generated keys evaluated inside the modules would avoid this but need key verification~\cite{decastro2022vfss}; neither this variant nor a constant-time select under \ProfT is modeled (\cref{sec:proto-pir}), and \cref{tab:pir} rests on assuming a PIR efficiency of \est{0.93} relative to DFA. FSS gates keep only seeds, control bits and correction words in long-lived state, whereas a direct gate computes on $x$ itself; we treat this as defense in depth only, because the trace model of \cref{thm:main} makes both options equivalent.

\textbf{Why two parties under \ProfT?}
Because the modules see plaintext, a single server whose protected module verifies an untrusted GPU, as in Slalom~\cite{tramer2018slalom}, would rest on the same hardware trust. The two-party structure buys two things. First, a host that held a value together with its complete tag would learn the MAC key; splitting every tag between two hosts lets SPDZ-style MACs~\cite{damgard2012spdz} check all GPU linear algebra at the next opening, whereas a single server must check each GPU product itself, for example with a Freivalds check per layer (\cref{sec:proto-freivalds}). Second, it keeps the two-party deployment of the FSS toolchains that DFA targets, on which \ProfU relies for its security (\cref{sec:threat-profileu}). It adds no protection against module compromise. For PIR as specified in \cref{alg:pir}, one server with one module would give the same guarantees. GPU-wide TEEs~\cite{nvidia_h100_overview,dhanuskodi2023confidential} avoid the four-lane GEMM cost but place the whole GPU and its firmware in the TCB.

\textbf{Physical and microarchitectural attacks.}
Probing~\cite{skorobogatov2017microprobing}, optical and other fault injection~\cite{skorobogatov2003optical,quadir2016survey}, and power or electromagnetic analysis~\cite{kocher1999differential} are outside \cref{thm:main} and can extract keys from an unhardened module. Faults matter more in the malicious setting: the bound $Q(2/p)^t$ presumes a correct check engine, so one glitch that forces acceptance bypasses it, and a fault in the field unit array can yield a wrong triple that carries valid tags. Software-controlled undervolting, which has induced such faults in SGX enclaves~\cite{murdock2020plundervolt}, is not physical: \cref{thm:main} assumes DVFS isolation (host software cannot drive the module's clock or voltage outside its safe operating range) and simulatable telemetry (\cref{sec:threat-model}), whose realization we have not evaluated. Conversely, the module has no out-of-order core, no shared cache hierarchy and no host-managed page tables, so the controlled-channel, cache, transient-execution and Rowhammer attacks studied on general-purpose TEEs~\cite{xu2015controlled,shinde2015preventing,gotzfried2017cache,brasser2017software,lee2017inferring,van2018foreshadow,kim2014flipping} target mechanisms it lacks, and each check returns one generic status only after all $t$ lanes are aggregated. Small security chips have still shipped with exploitable flaws~\cite{moghimi2020tpm,han2018bad,butterworth2013bios}: a small TCB makes hardening tractable, but it does not replace hardening.

\textbf{Rollback and lifecycle.}
Ledger and epoch state live in volatile protected SRAM, so every reset falls under the reboot rule of \cref{sec:proto-ledger}. Because every failure poisons its epoch and aborted reservations never return to a free list (\cref{fig:ledger}), recovery always costs a new setup. Neither a monotonic service nor an erase-and-rekey lifecycle is implemented yet (\cref{tab:obligations}).

\textbf{Availability and fairness.}
\sys provides security with abort, the standard target for two-party computation with a malicious participant~\cite{hazay2010efficient,lindell2017simulate}. A corrupt host can withhold or reorder traffic, stall its GPU or abort at any public interaction boundary, and a corrupt recipient may obtain its output first; fairness and guaranteed output delivery are not claimed (S10 in \cref{tab:scenarios}). Aborts are, however, not a side channel on honest inputs. Apart from the validity predicates, which the modules evaluate before the first output opening and whose outcomes are the $\mathsf{status}$ part of $\Leak_C$ (\cref{def:leakage}), every \CheckOpen{} outcome depends only on the adversary's own deviation $(\bm{e},\bm{d}_j)$, the protected keys and the fresh challenges (\cref{thm:mac-sound}), and the first failure ends the epoch, so selective-failure and key-learning strategies cannot be iterated (\cref{lem:hidden-key}). Persistent denial of service remains a matter of deployment policy.

\textbf{Field versus ring.}
Over $\Fp$ with $p = 2^{61}-1$, \sys is not bit-identical to the $\Z_{2^{64}}$ arithmetic of Sigma and Orca~\cite{gupta2023sigma,jawalkar2024orca}. Ring-compiled models must be re-encoded under the numeric contract of \cref{sec:arch-field}, with magnitudes below $p/2$ before truncation, and exact signed truncation needs 307 authenticated multiplications on sequential carry chains, i.e., 309 rounds or \est{30.9~ms} on LAN (\cref{alg:bitdec,alg:trunc}), the most round-intensive gate in \cref{tab:gates}. A ring deployment needs a SPDZ2k-style backend~\cite{cramer2018spdz2k}, which is a separate design with a separate proof (\cref{sec:sec-concrete}).

\textbf{\ProfU.}
\ProfU (\cref{sec:threat-profileu}) is specified but not evaluated; it forfeits the local-dealer and generate-and-consume savings and must add the backend's key-privacy and answer-integrity arguments outside \cref{thm:main}.

\textbf{Model provenance.}
\sys proves correct evaluation on the inputs actually supplied (S9 in \cref{tab:scenarios}). A committed model (\cref{sec:threat-goals}) establishes provenance, not quality; the gap between the finite-field circuit and a floating-point model is an approximation question separate from cryptographic correctness.

\textbf{Artifact status.}
We executed a specification and a functional CPU reference model; GPU and RTL conformance, the protected runtime and deployment measurements have not been run yet (\cref{sec:eval-method,sec:eval-attack}). Every red value therefore awaits the three separate experiments of \cref{sec:arch-deploy}, and security measurements need two independent protected devices.


==> qa/draft2/sections/10_related.tex <==
% ==================================================================
% Section X: Related Work
% Owner labels: sec:related, tab:related
% ==================================================================
\section{Related Work}
\label{sec:related}

\begin{table*}[t]
\centering
\caption{Comparison of \sys with Representative Related Work}
\label{tab:related}
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{l c c c c l c c l}
\hline
\textbf{Work} & \textbf{Adversary} & \makecell{\textbf{Trusted}\\\textbf{HW}} & \makecell{\textbf{Trusted comp.}\\\textbf{sees plaintext}} & \makecell{\textbf{Custom}\\\textbf{HW}} & \textbf{Offline material} & \makecell{\textbf{Auth.\ FSS}\\\textbf{outputs}} & \makecell{\textbf{Verified}\\\textbf{openings}} & \textbf{Workloads} \\
\hline
Sigma~\cite{gupta2023sigma} & SH & \xmark & \xmark & \xmark$^{\mathrm{g}}$ & Dealer keys & \xmark & \xmark & Inference \\
Orca~\cite{jawalkar2024orca} & SH & \xmark & \xmark & \xmark$^{\mathrm{g}}$ & Dealer keys & \xmark & \xmark & Training, inference \\
Shark~\cite{gupta2025shark} & Mal & \xmark & \xmark & \xmark & Dealer, authenticated keys & \cmark & \cmark & Inference \\
\hline
MASCOT, MP-SPDZ~\cite{keller2016mascot,keller2020mpspdz} & Mal & \xmark & n/a & \xmark & Interactive (OT-based) & n/a & \cmark & General circuits \\
vFSS~\cite{decastro2022vfss} & Mal$^{\mathrm{a}}$ & \xmark & n/a & \xmark & Client keys, verified & \xmark & n/a & Key validation \\
APIR~\cite{colombo2023apir} & Mal$^{\mathrm{b}}$ & \xmark & n/a & \xmark & None (client query) & n/a & \cmark$^{\mathrm{b}}$ & PIR \\
\hline
Slalom~\cite{tramer2018slalom} & Mal$^{\mathrm{c}}$ & \cmark & \cmark & \xmark$^{\mathrm{g}}$ & n/a & n/a & \cmark$^{\mathrm{c}}$ & Inference \\
Aramis~\cite{kumar2020cryptflow} & Mal & \cmark$^{\mathrm{d}}$ & \xmark$^{\mathrm{d}}$ & \xmark & n/a & n/a & n/a & Inference \\
STAMP, PPMLAC~\cite{huang2022efficient,zhou2022ppmlac} & SH, Mal$^{\mathrm{e}}$ & \cmark & \pmark$^{\mathrm{e}}$ & \cmark & In trusted HW & n/a & \pmark$^{\mathrm{e}}$ & ML \\
\hline
GPU-DPF~\cite{lam2023gpu} & SH$^{\mathrm{i}}$ & \xmark & n/a & \xmark$^{\mathrm{g}}$ & None (client query) & \xmark & \xmark & PIR \\
DFA~\cite{dfa2026trusted} & SH$^{\mathrm{i}}$ & \pmark$^{\mathrm{f}}$ & \cmark$^{\mathrm{f}}$ & \cmark & Dealer or local$^{\mathrm{f}}$ & \xmark & \xmark & Inference, PIR \\
\hline
\textbf{\sys (this work)} & Mal$^{\mathrm{h}}$ & \cmark & \cmark$^{\mathrm{h}}$ & \cmark & Local, none shipped & \cmark & \cmark & Inference, PIR \\
\hline
\end{tabular}

\vspace{3pt}
\begin{minipage}{0.98\textwidth}
\footnotesize
SH: semi-honest; Mal: malicious (active) adversary. \emph{Trusted HW}: security relies on trusted hardware. \emph{Trusted comp.\ sees plaintext}: a trusted dealer, enclave or module sees inputs or intermediate values (FSS dealers are input independent). \emph{Custom HW}: dedicated hardware beyond commodity CPUs and GPUs. \emph{Offline material}: source of the per-query correlated randomness or keys. \emph{Auth.\ FSS outputs}: FSS gate outputs carry MAC tags. \emph{Verified openings}: opened values or untrusted results are checked before use. \cmark: yes; \xmark: no; \pmark: partial, optional or configuration dependent; n/a: not applicable. Lettered notes qualify the headline setting of each work.
$^{\mathrm{a}}$\,Malicious client key generator; servers check that keys are well formed, not that they are evaluated correctly.
$^{\mathrm{b}}$\,The client detects answers that are inconsistent with a public database digest.
$^{\mathrm{c}}$\,An SGX enclave outsources to an untrusted co-located GPU and checks its matrix products with Freivalds' algorithm.
$^{\mathrm{d}}$\,Relies on SGX integrity, not confidentiality.
$^{\mathrm{e}}$\,Settings differ between the two works: STAMP reports semi-honest and honest-majority malicious variants and evaluates nonlinear operations on unmasked values in its trusted processor; PPMLAC's trusted chipset mainly generates correlated randomness.
$^{\mathrm{f}}$\,Trusted mode only; the untrusted mode ships dealer keys.
$^{\mathrm{g}}$\,Implemented on commodity GPUs.
$^{\mathrm{h}}$\,Static corruption of one host, security with abort, under \ProfT, where the modules see inputs, openings and PIR indices; \ProfU delegates to an established malicious backend.
$^{\mathrm{i}}$\,In two-server DPF-PIR (GPU-DPF, DFA's untrusted mode), neither server learns the queried index, without relying on trusted hardware; SH refers to result integrity.
\end{minipage}
\end{table*}

\Cref{tab:related} summarizes the closest lines of work.

\textbf{FSS-based secure computation.}
FSS~\cite{boyle2015fss} and its tree-based DPF instantiations~\cite{gilboa2014distributed,boyle2016function} underlie a family of low-round two-party protocols with preprocessing~\cite{boyle2019preprocessing}. AriaNN~\cite{ryffel2020ariann} and Pika~\cite{wagh2022pika} first demonstrated private inference with FSS, Boyle et al.~\cite{boyle2021function} built comparisons, splines and fixed-point truncation from DCFs, Grotto~\cite{storrier2023grotto} replaced DCF-heavy constructions with DPF-based ones in a $(2{+}1)$-party setting, and Orca~\cite{jawalkar2024orca} and Sigma~\cite{gupta2023sigma} brought FSS-based training and GPT-class inference to GPUs. These systems are semi-honest and assume a dealer whose key material dominates the offline cost~\cite{huang2026beyond}. DPFs also underlie PIR, anonymous messaging, private queries and analytics, private heavy hitters, set intersection and distributed ORAM~\cite{corrigan2015riposte,wang2017splinter,dauterman2020dory,dauterman2022waldo,boneh2021lightweight,mouris2024plasma,garimella2024computation,vadapalli2023duoram,doerner2017scaling,ji2023multi}. Secure inference without FSS realizes nonlinear layers through share conversions, garbled circuits or homomorphic encryption~\cite{mohassel2017secureml,mohassel2018aby3,wagh2019securenn,wagh2020falcon,rathee2020cryptflow2,pang2024bolt,lu2023bumblebee}, typically with more interaction per layer.

\textbf{Malicious and verifiable FSS.}
To our knowledge, Shark~\cite{gupta2025shark} is the most directly comparable system: actively secure two-party FSS inference in which a trusted dealer supplies authenticated key material. Its security is cryptographic once its input-independent dealer, which never sees an input or an opening, is trusted, whereas each \sys module sees every input and opening under \ProfT (\cref{sec:eval-method}). In exchange, \sys generates the authenticated correlations locally and removes the offline distribution that dominates the dealer-based malicious FSS baseline, modeled after the protocol family of Shark~\cite{gupta2025shark} (\cref{tab:e2e}). Verifiable FSS~\cite{corrigan2015riposte,boyle2016function,boneh2021lightweight,decastro2022vfss} addresses a different adversary, a client that may submit malformed keys, which the servers detect; \sys instead treats key generation, evaluation, authentication and release as separate obligations.

\textbf{Malicious MPC preprocessing and MACs.}
Beyond the SPDZ-family tools of \cref{sec:bg-mal}, mixed-circuit preprocessing with edaBits~\cite{escudero2020edabits} and classical bit-decomposition and truncation protocols~\cite{damgard2006unconditionally,catrina2010improved} supply the conversions that nonlinear layers need, and honest-majority protocols~\cite{furukawa2017high,mohassel2018aby3,wagh2020falcon,dalskov2021fantastic} obtain malicious security from replicated sharing among three or four servers. \sys adopts, and does not claim as new, the SPDZ MAC algebra with $t$ independent keys over a Mersenne field. It replaces interactive preprocessing by correct generation inside the modules, in the spirit of hardware-assisted correlation generation~\cite{lu2021correlated,zhou2022ppmlac}, and checks openings on frozen bytes (\cref{sec:proto-check}).

\textbf{Trusted hardware for MPC and ML.}
Tamper-proof tokens are a classical setup assumption for universally composable computation~\cite{katz2007universally}, and commodity TEEs~\cite{costan2016intel,amd_sev,arm_trustzone,lee2020keystone} have been used to accelerate or simplify two-party computation and functional encryption~\cite{gupta2016using,choi2019hybrid,felsen2019secure,wuhybrid,fisch2017iron}. For ML, Ohrimenko et al.~\cite{ohrimenko2016oblivious} and Chiron~\cite{hunt2018chiron} execute learning tasks inside SGX enclaves; Slalom~\cite{tramer2018slalom} and DarKnight~\cite{hashemi2021darknight} outsource linear layers from an enclave to untrusted GPUs and verify them, with Freivalds' algorithm~\cite{freivalds1977probabilistic} and with redundant coded computation, respectively; and Aramis~\cite{kumar2020cryptflow} compiles semi-honest protocols into maliciously secure ones by relying on the integrity, but not the confidentiality, of SGX. GPU TEEs~\cite{volos2018graviton,jang2019heterogeneous} and confidential computing on H100~\cite{nvidia_h100_overview,dhanuskodi2023confidential} protect GPU computation from the host but place the whole GPU and its firmware in a TCB far larger than our module. Closest to our trust model, STAMP~\cite{huang2022efficient} and PPMLAC~\cite{zhou2022ppmlac} rely on a small security processor or a trusted chipset to execute nonlinear operations or generate correlated randomness, respectively, in the tradition of TPM-class security chips, secure coprocessors and smart cards~\cite{tpm2spec,googletitan,ibm4758,rankl2004smart}, and DFA~\cite{dfa2026trusted} uses a small module as a local FSS dealer. STAMP's nonlinear evaluation inside its trusted processor corresponds to our direct protected gate (\cref{sec:proto-direct}). Relative to it, \sys contributes a two-party setting with an untrusted GPU checked by MACs, freeze-before-challenge checking against host-controlled DMA, ledgered one-time randomness, and a malicious FSS and PIR datapath. Like Slalom and DarKnight, \sys keeps the GPU outside the boundary, but it uses Freivalds checks only for operands the GPU may already see (\cref{sec:proto-freivalds}).

\textbf{Hardware acceleration for private computation.}
GPU systems accelerate secret-sharing MPC~\cite{tan2021cryptgpu,watson2022piranha,crypten2020}, FSS~\cite{gupta2023sigma,jawalkar2024orca} and DPF-based PIR~\cite{lam2023gpu}. FPGA designs target secret-sharing MPC~\cite{wolfe2020secret,patel2020arithmetic,xu2025co}, Ironman~\cite{ironman2025} accelerates OT extension near memory, and FPGA and ASIC designs speed up the polynomial kernels of homomorphic encryption~\cite{riazi2020heax,reagen2021cheetah,samardzic2021f1,samardzic2022craterlake,kim2022bts}. These accelerators make a fixed protocol faster and inherit its adversary model. DFA~\cite{dfa2026trusted} additionally used trust to change the dataflow; \sys uses the same small trusted module to change the adversary model, which is why \cref{sec:eval} compares against security-matched baselines rather than raw kernel throughput alone.

\textbf{PIR with integrity.}
Authenticated PIR~\cite{colombo2023apir} lets a client detect answers that are inconsistent with a public database digest without trusted hardware, at additional server cost that our APIR-based GPU baseline reflects (\cref{tab:pir}). PIR with secure coprocessors~\cite{smith2001practical} and enclave-based oblivious storage such as Snoopy~\cite{dauterman2021snoopy} instead trust hardware that learns the query and hides its accesses through oblivious scans. The versioned-snapshot PIR of \sys follows this trust model: both modules learn the queried index $\alpha$, so its query privacy rests on module trust, unlike untrusted two-server DPF-PIR (GPU-DPF~\cite{lam2023gpu}, DFA's untrusted mode), which hides $\alpha$ from each server without trusted hardware. It scans in two role-bound modules, binds the exact consumed bytes to an authorized commitment $\mathsf{cm}_v$, optionally a Merkle root~\cite{merkle1987digital}, and releases freshly reshared answers only after the snapshot hash matches (\cref{sec:proto-pir}).

\textbf{Positioning.}
Each ingredient of \sys, from information-theoretic MACs and trusted correlation generation to verified GPU work and DPF acceleration, has precedents; our contribution is their composition in one small trusted module, proven stand-alone secure with abort in the ideal-module model of \cref{sec:threat-model} (\cref{tab:related}).


==> qa/draft2/sections/11_conclusion.tex <==
% ==================================================================
% Section XI: Conclusion (owner: sections/11_conclusion.tex)
% Labels defined here: sec:conclusion
% ==================================================================
\section{Conclusion}\label{sec:conclusion}

We presented \sys, a trusted hardware accelerator that secures FSS-based private inference and DPF-based PIR against a malicious host and GPU while keeping the key-movement savings of trusted DFA. Since a module acting as FSS dealer can also be the verifier, \sys generates authenticated correlations internally, authenticates DPF outputs with a fresh resharing epilogue instead of extra DPF trees, checks every opening on frozen bytes with $t=3$ independent MAC lanes over $\F_{2^{61}-1}$, and releases nothing before a role-bound one-time ledger records a verified check. These mechanisms protect the chain from authorized input to authorized output release; we prove stand-alone static malicious security with abort in a protected-module model, with statistical error about $2^{-148}$ for $2^{32}$ checked batches. Both modules see inputs and learn the PIR index, so PIR query privacy rests on module trust, unlike untrusted two-server DPF-PIR~\cite{lam2023gpu}. Our model estimates that \sys is \est{10.1--14.0$\times$} faster on a LAN than dealer-based malicious FSS modeled after the protocol family of Shark~\cite{gupta2025shark}, mainly because in-module generation removes \est{21.8--563~GB} of per-query offline distribution (\est{1.5--1.8$\times$} excluding it). Malicious security costs \est{2.5--3.5$\times$} LAN latency over semi-honest DFA and \est{0.145~mm$^2$} at 7~nm (pre-synthesis).

We executed a specification and a functional CPU reference model; GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet, so no \sys performance number is measured. Three directions follow. First, these measurements, synthesis and on-die simulation must replace the estimates. Second, a \ProfU backend would run the same compiled circuit when the hardware is adversarial, and a SPDZ2k-style backend would cover the ring $\Z_{2^{64}}$. Third, compressed MAC checks that avoid carrying all tag lanes through the GPU would cut the now-dominant authenticated linear algebra; a vetted DCF faster than our $O(n^2)$ one would help FSS-only configurations, not the compiler-selected default, where nonlinear gates take \est{3.4\%} of BERT-Base latency. Both need proofs this paper does not provide.

\section*{Acknowledgment}
Omitted for anonymous review.


==> qa/draft3/macros.tex <==
% ------------------------------------------------------------------
% Shared packages and macros for the TIFS manuscript.
% Every section/appendix/algorithm/table file relies ONLY on these.
% ------------------------------------------------------------------
\usepackage[T1]{fontenc}
\usepackage{amsmath,amssymb,amsfonts,mathtools}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{graphicx}
\usepackage[dvipsnames,table]{xcolor}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{array}
\usepackage{tabularx}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{setspace}
\let\labelindent\relax
\usepackage[inline]{enumitem}
\usepackage{pifont}
\usepackage{xspace}
\usepackage{stmaryrd}
\usepackage{cite}
\usepackage[hidelinks]{hyperref}
\usepackage[capitalise,noabbrev]{cleveref}

% ---------------- cross-reference names (IEEE style) ----------------
\crefname{section}{Section}{Sections}
\Crefname{section}{Section}{Sections}
\crefname{subsection}{Section}{Sections}
\Crefname{subsection}{Section}{Sections}
\crefname{subsubsection}{Section}{Sections}
\Crefname{subsubsection}{Section}{Sections}
\crefname{appendix}{Appendix}{Appendices}
\Crefname{appendix}{Appendix}{Appendices}
\crefname{figure}{Fig.}{Figs.}
\Crefname{figure}{Fig.}{Figs.}
\crefname{table}{Table}{Tables}
\Crefname{table}{Table}{Tables}
\crefname{algorithm}{Algorithm}{Algorithms}
\Crefname{algorithm}{Algorithm}{Algorithms}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Eq.}{Eqs.}
\crefname{ALC@unique}{line}{lines}
\crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{remark}{Remark}{Remarks}
\crefname{proposition}{Proposition}{Propositions}

% ---------------- theorem environments ----------------
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\theoremstyle{remark}
\newtheorem{remark}{Remark}

% ---------------- algorithm style (FuseFSS / DFA hybrid) ----------------
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) \textit{#1}}
\algnewcommand{\Abort}{\textbf{abort}}
\newcommand{\algstretch}{\setstretch{0.92}}

% ---------------- estimates: RED, to be replaced by measured values ----------------
\newcommand{\est}[1]{\textcolor{red}{#1}}

% ---------------- names ----------------
\newcommand{\sys}{VIGOR-DFA\xspace}
\newcommand{\DFA}{DFA\xspace}
\newcommand{\ProfT}{Profile~$\mathsf{T}$\xspace}
\newcommand{\ProfU}{Profile~$\mathsf{U}$\xspace}

% ---------------- algebra ----------------
\newcommand{\F}{\mathbb{F}}
\newcommand{\Fp}{\mathbb{F}_p}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\bits}[1]{\{0,1\}^{#1}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\getsr}{\xleftarrow{\$}}
\newcommand{\inner}[2]{\langle #1, #2\rangle}
\newcommand{\auth}[1]{[#1]}                  % authenticated sharing
\newcommand{\authb}[2]{[#1]_{#2}}            % party-b tuple (x_b, gamma_{b,1..t})
\newcommand{\tagv}[3]{\gamma_{#1,#2}^{(#3)}} % optional explicit tag notation

% ---------------- FSS objects ----------------
\newcommand{\Gen}{\mathsf{Gen}}
\newcommand{\Eval}{\mathsf{Eval}}
\newcommand{\EvalAll}{\mathsf{EvalAll}}
\newcommand{\DPF}{\mathsf{DPF}}
\newcommand{\DCF}{\mathsf{DCF}}
\newcommand{\CW}{\mathsf{CW}}
\newcommand{\CWout}{\mathsf{CW}^{\mathrm{out}}}
\newcommand{\sCW}{s^{\mathsf{CW}}}
\newcommand{\tCW}[1]{t^{\mathsf{CW},#1}}
\newcommand{\PRG}{G}
\newcommand{\Conv}{H}
\newcommand{\keep}{\mathit{keep}}
\newcommand{\lose}{\mathit{lose}}

% ---------------- crypto ----------------
\newcommand{\PRF}{\mathsf{PRF}}
\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\Hash}{\mathsf{Hash}}
\newcommand{\AEAD}{\mathsf{AEAD}}
\newcommand{\Adv}{\mathcal{A}}
\newcommand{\Sim}{\mathcal{S}}
\newcommand{\Env}{\mathcal{Z}}
\newcommand{\View}{\mathsf{View}}
\newcommand{\Real}{\mathsf{Real}}
\newcommand{\Ideal}{\mathsf{Ideal}}
\newcommand{\Hyb}[1]{\mathsf{H}_{#1}}
\newcommand{\Leak}{\mathcal{L}}
\newcommand{\FC}{\mathcal{F}^{\mathrm{abort}}_{C,\mu}}
\newcommand{\FPIR}{\mathcal{F}^{\mathrm{abort}}_{\mathrm{PIR}}}
\newcommand{\eps}[1]{\epsilon_{\mathsf{#1}}}
\newcommand{\negl}{\mathsf{negl}}

% ---------------- protocol / ledger / commands ----------------
\newcommand{\cmd}[1]{\texttt{\detokenize{#1}}}
\newcommand{\lstate}[1]{\textsf{#1}}
\newcommand{\algname}[1]{\textsf{#1}}
\newcommand{\CheckOpen}{\algname{CheckOpen}\xspace}
\newcommand{\AuthShare}{\algname{AuthShare}\xspace}
\newcommand{\Epilogue}{\algname{Epilogue}\xspace}

% ---------------- marks for tables ----------------
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\pmark}{\ding{109}}   % partial


==> qa/draft3/sections/00_abstract.tex <==
% ==================================================================
% Abstract and index terms (owner: sections/00_abstract.tex)
% Red values are model estimates (\est{}); see Appendix F.
% ==================================================================
\begin{abstract}
Function secret sharing (FSS) underlies two-party private inference and private information retrieval, with cost dominated by generating, moving and evaluating distributed point function (DPF) keys. A trusted GPU-integrated distributed function accelerator (DFA) removed key movement by generating and consuming keys locally, but tolerates only semi-honest adversaries. A malicious host or GPU can tamper with shares, replay one-time material, swap buffers after checking, request early outputs, or abuse the accelerator as a forgery oracle, while malicious FSS ships large authenticated keys or multiplies DPF work. We present \sys, protecting the chain from authorized input to authorized output release with three mechanisms: a fresh authentication epilogue using three field multiplications per DPF output, \est{3.8--4.0$\times$} faster per gate than per-lane DPF tag trees; a freeze-before-challenge check of every opening with $t=3$ independent MAC lanes over $\F_{2^{61}-1}$; and a role-bound one-time resource ledger with a release guard, in a protected datapath beside the GPU L2 cache. We prove stand-alone static malicious security with abort in a protected-module model, with statistical error $Q(2/p)^t\approx 2^{-148}$ for $Q\le 2^{32}$ checked batches. Our DFA-calibrated model estimates that, against dealer-based malicious FSS modeled after the protocol family of Shark, \sys removes \est{21.8--563~GB} of per-query offline authenticated material and, mainly by generating it in-module, lowers LAN latency by \est{10.1--14.0$\times$} (\est{1.5--1.8$\times$} excluding offline distribution) and energy by \est{3.0--3.9$\times$}. Malicious security costs \est{2.5--3.5$\times$} LAN latency over semi-honest DFA and \est{0.145~mm$^2$} at 7~nm. We executed a specification and a functional CPU reference model; GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet.
\end{abstract}

\begin{IEEEkeywords}
Distributed point function, function secret sharing, hardware accelerator, malicious security, private information retrieval, secure inference, trusted hardware.
\end{IEEEkeywords}


==> qa/draft3/sections/01_introduction.tex <==
% ==================================================================
% Section I: Introduction (owner: sections/01_introduction.tex)
% Labels defined here: sec:intro
% Red (\est{}): model outputs, assumed parameters. Black: cited DFA
% values, design constants, analytical counts, executed tests.
% ==================================================================
\section{Introduction}\label{sec:intro}

\IEEEPARstart{P}{rivacy}-preserving computation is moving into deployments where data are both valuable and regulated: hospitals running diagnostic models on records they may not export, cloud providers serving proprietary models to clients who will not reveal their queries, and lookup services whose queries disclose a user's interests. Secure two-party computation (2PC) for private machine-learning (ML) inference~\cite{yao1986generate,goldreich2019play,mohassel2017secureml,rathee2020cryptflow2} and private information retrieval (PIR)~\cite{chor1998private,angel2018pir} address these settings with cryptographic rather than contractual guarantees. Function secret sharing (FSS)~\cite{boyle2015fss,boyle2016function} has become one of the most effective building blocks for both. In FSS-based private inference, the parties open a masked input $x+r$ and evaluate one-time keys for the gate function shifted by the mask, so that a nonlinear layer often costs a single online round~\cite{boyle2021function,gupta2023sigma,jawalkar2024orca}. In two-server PIR, the client splits a point function into two short keys and each server evaluates its key over the entire database~\cite{gilboa2014distributed,wang2017splinter,lam2023gpu}.

The price of this online efficiency is paid in distributed point function (DPF) work. Every comparison, lookup table and interval test in an FSS-compiled model is built from DPFs or from the distributed comparison functions (DCFs) derived from them~\cite{boyle2021function,storrier2023grotto,gupta2023sigma}, and each key is used once. A dealer must therefore generate, ship and store fresh keys for every nonlinear element of every query: 17.1~GB of offline material for a single BERT-Base inference~\cite{dfa2026trusted}, a cost that cannot always be hidden behind the online phase~\cite{huang2026beyond}. PIR, conversely, is dominated by full-domain DPF evaluation, which is AES-bound even on a modern GPU~\cite{lam2023gpu}. The distributed function accelerator (DFA)~\cite{dfa2026trusted} attacked both costs with a small DPF engine integrated next to the GPU L2 cache. In its trusted mode, a protected module in each server attests to its peer, establishes a shared key and plays the dealer locally: it generates its own party's key share on demand and consumes each correction word as soon as it is produced (\emph{generate-and-consume}, GaC), so keys are never distributed, stored or reread. For BERT-Base, trusted DFA reduces LAN latency from 18.8~s to 1.42~s and offline communication from 17.1~GB to 0.1~GB; for PIR, DFA in its untrusted mode (client-generated keys) raises throughput by $5.05\times$ for $2^{20}$ records~\cite{dfa2026trusted}.

\textbf{The semi-honest boundary.}
DFA, like Sigma~\cite{gupta2023sigma}, Orca~\cite{jawalkar2024orca} and most GPU-based FSS systems, is secure only against semi-honest adversaries: it assumes that both servers run the prescribed code. In a real deployment, however, the components easiest to subvert are those around the small protected module: the host operating system, the GPU driver and runtime, the GPU kernels, the direct memory access (DMA) buffers and the network stack. They hold the whole data path, and attacks on privileged software and firmware~\cite{xu2015controlled,butterworth2013bios,han2018bad} and GPU isolation designs~\cite{volos2018graviton,jang2019heterogeneous} alike treat them as potentially adversarial. With its module intact, a single compromised server host can still mount at least five classes of attacks against semi-honest trusted acceleration (\cref{fig:scenarios}):
(i)~\emph{additive errors} on shares, openings or GPU products, which bias results and leak through selective failure;
(ii)~\emph{replay or reset} of masks, counters or module state;
(iii)~\emph{check-to-use} buffer swaps;
(iv)~abuse of a naive ``authenticate'' command as a \emph{forgery oracle}; and
(v)~\emph{premature} output requests.
Remote attestation does not close these gaps. It proves which code and configuration run inside the module; it does not prove that the untrusted GPU used a valid key, computed the right product, or released an authorized result.

\textbf{Why existing malicious routes are costly.}
FSS can be made maliciously secure, but the known routes give back much of what trusted acceleration gained. Actively secure FSS inference such as Shark~\cite{gupta2025shark} keeps an external dealer that ships authenticated keys and correlated randomness. For dealer-based malicious FSS modeled after the protocol family of Shark (\cref{app:model}), we estimate \est{37.6~GB} of offline material per BERT-Base query, \est{2.2$\times$} the semi-honest 17.1~GB~\cite{dfa2026trusted}, and a LAN latency of \est{43.9~s} of which \est{37.6~s} is distribution. Dealer-free malicious preprocessing in the SPDZ family~\cite{damgard2012spdz,keller2016mascot,keller2018overdrive,cramer2018spdz2k} replaces the dealer by oblivious-transfer (OT) or homomorphic-encryption triple generation, and pseudorandom correlation generators (PCGs) with silent OT~\cite{boyle2019pcg,boyle2020pcg} compress the communication of authenticated triples at a substantial computational cost. Neither yields FSS keys: generating DPF keys without a dealer requires a secure two-party evaluation of key generation with a round per tree level~\cite{doerner2017scaling}, so dealer-free malicious FSS keeps a preprocessing cost far above its online cost. Verifiable FSS (vFSS)~\cite{decastro2022vfss} lets servers check that client-generated DPF keys are well formed, but not that an untrusted GPU evaluates them, or the arithmetic around the gate, correctly. Finally, the direct way to authenticate an FSS output inside an accelerator, one additional DPF tree with payload $\Delta_j\beta$ per message authentication code (MAC) lane, multiplies pseudorandom generator (PRG) work by $1+t$ for $t$ lanes. One tree with a $(1+t)$-element payload avoids most of this cost, but it widens every output correction and exports tag shares whose hiding rests on DPF key privacy.

\textbf{Our key insight} is that a module that already plays the FSS dealer can also be the verifier. Because it knows every correlation it generates, it can (1)~generate \emph{authenticated} correlations (input masks, Beaver triples~\cite{beaver1991efficient} and DPF keys) locally at zero network cost, computing every triple product correctly inside its own boundary; (2)~authenticate its own FSS outputs with a fresh resharing epilogue instead of extra DPF trees, because it already holds the raw output shares and the MAC key material; and (3)~check every opening on bytes it has frozen before any challenge exists, so that the GPU remains a fast but untrusted linear-algebra engine whose results are only candidates until verified. What must be protected is thus not a single primitive but an integrity chain:
\begin{center}
\small
\emph{authorized input} $\rightarrow$ \emph{correlated preprocessing} $\rightarrow$ \emph{correct local evaluation} $\rightarrow$ \emph{authenticated arithmetic} $\rightarrow$ \emph{consistent opening} $\rightarrow$ \emph{authorized output release.}
\end{center}
Each link has a concrete failure mode under a malicious host, and each needs its own mechanism. \Cref{fig:flows} places the resulting execution flow next to the semi-honest GPU baseline, trusted DFA and dealer-based malicious FSS.

\textbf{This work.}
We present \sys (Verified Integrity-Gated On-demand Randomness DFA), the malicious-secure successor of trusted DFA. It keeps DFA's placement beside the GPU L2 cache, its local key generation and its generate-and-consume execution. Under \ProfT (\cref{sec:threat}) a malicious adversary statically corrupts at most one host, and every secret value on a host is an authenticated share over $\Fp$, $p=2^{61}-1$, with $t=3$ SPDZ-style MAC lanes~\cite{damgard2012spdz,damgard2013practical} (32~bytes per element and party). Three mechanisms carry the design; we claim their composition, not any of them as an unprecedented primitive. The \emph{fresh authentication epilogue} turns each raw DPF output share into a freshly padded authenticated tuple at three field multiplications and four pads (\cref{sec:proto-epilogue}). It matches the PRG cost of a single vector-payload tree, makes every exported tuple exactly uniform, and leaves no command that authenticates a host-supplied value. \emph{Freeze-before-challenge} \CheckOpen{} derives independent per-lane challenges only after both modules have frozen the exact submitted bytes, and later consumes exactly those bytes. A \emph{role-bound one-time ledger} labels all randomness by session, epoch, gate and purpose and poisons the epoch on any failure, and its \emph{release guard} lets no output leave a module before the corresponding check is \lstate{VERIFIED}.

\textbf{Scope and limits.}
\sys relocates trust to the modules rather than removing it. The modules see inputs under \ProfT, and both learn the PIR index, so PIR query privacy in \sys rests on module trust, unlike untrusted two-server DPF-PIR~\cite{lam2023gpu} and DFA's untrusted mode, which hide the index without trusted hardware. Physical attacks, leakage beyond the stipulated observable-trace model and rollback without a trusted monotonic service are out of scope, and security holds with abort, without fairness (\cref{sec:discussion}). Once the epilogue removes tag trees, the dominant cost of malicious security moves to four-lane authenticated linear algebra on the GPU and to the doubled round count (\cref{sec:analysis}).

\textbf{Why keep FSS inside a trusted module?}
Under \ProfT a module that has verified $c=x+r$ also holds $r$, so FSS adds no formal confidentiality over evaluating the gate directly (\cref{sec:proto-direct}). The end-to-end gains of \sys come from generating and consuming authenticated correlations inside the modules, not from FSS evaluation: in our model direct-only compilation (\est{3.82~s} for BERT-Base) is marginally faster than the compiler-selected default (\est{3.83~s}), which keeps an FSS realization for gate shapes marked FSS-portable, and nonlinear gates take only \est{3.4\%} of the latency. We keep a malicious FSS datapath for three reasons: the same compiled circuit, including masked-input FSS gates from existing toolchains~\cite{gupta2023sigma,jawalkar2024orca}, runs under the key-exporting \ProfU (specified, not evaluated or proven); PIR and small lookup tables are full-domain, data-independent scans that match the pipelined AES engines; and long-lived evaluation state holds only seeds and correction words, keeping input-dependent state short-lived as defense in depth, not as a formal claim. On FSS gates the epilogue is \est{3.8--4.0$\times$} faster than per-lane tag trees, although tag trees would raise the BERT-Base LAN latency by only \est{8\%}.

This paper makes the following contributions:
\begin{itemize}[leftmargin=*]
    \item \textbf{Malicious Threat Analysis.}
    We systematize how a malicious host or GPU attacks semi-honest trusted FSS acceleration into ten scenarios, S1 to S10 (\cref{fig:scenarios,tab:scenarios}), from share tampering to PIR snapshot substitution. For S1 to S8 we show why semi-honest trusted DFA fails and which \sys mechanism and theorem stop it; for S9 (input substitution) and S10 (denial of service and selective abort) we make explicit what the ideal functionality permits or does not prevent.

    \item \textbf{Protocol Co-Design.}
    We specify the three mechanisms above, the authenticated $\Fp$ representation and malicious generate-and-consume with explicit generator and evaluator states (\cref{sec:protocol}). On top of them we build authenticated lookup-table, interval, polynomial and direct protected gates, exact comparison and truncation, a refactoring rule that preserves the joint (not only the marginal) distribution of DFA's decoupled preprocessing, and versioned-snapshot PIR whose query privacy rests on module trust.

    \item \textbf{Hardware Architecture.}
    We design a protected datapath beside the GPU L2 cache (\cref{sec:arch}) with a ledger, page freezer, joint pseudorandom-function (PRF) sampler, DPF generation and evaluation contexts, a 128-lane Mersenne-61 field unit array, a check engine, a peer-channel controller and a release guard, whose 64 AES engines are time-shared among PRG expansion, challenge derivation and authenticated-encryption (AEAD) freezing. The additions cost \est{0.145~mm$^2$} and \est{0.508~W} at 7~nm, and the entire \sys occupies \est{0.046\%} of the A100 die.

    \item \textbf{Security Analysis.}
    We give ideal functionalities with explicit leakage and a hybrid proof with an explicit simulator of stand-alone static malicious security with abort under sequential composition (\cref{sec:security}, \cref{thm:main}), with advantage at most $\eps{setup}+\eps{prf}+\eps{channel}+\eps{bind}+\eps{trace}+Q(2/p)^t$, where the last term is about $2^{-148}$ for $Q\le 2^{32}$ checked batches. We show why shared challenges across lanes and the ring $\Z_{2^{64}}$ break this bound, and we separate what is proved from the implementation obligations that remain (\cref{tab:obligations}).

    \item \textbf{Evaluation.}
    With an analytical model calibrated on DFA (\cref{sec:eval}, \cref{tab:e2e}), we estimate that in-module generation of authenticated correlations cuts offline communication from \est{37.6~GB} to \est{under 1~MB} per BERT-Base query. Against dealer-based malicious FSS modeled after the protocol family of Shark, \sys is \est{11.4$\times$} faster on a LAN, or \est{1.6$\times$} excluding per-query offline distribution; with no authenticated-key blow-up the dealer-based pipeline still needs \est{22.4~s}, \est{5.8$\times$} that of \sys. Malicious security costs \est{2.7$\times$} LAN latency over semi-honest trusted DFA for BERT-Base, mostly for four-lane linear algebra, yet \sys stays \est{4.3--6.1$\times$} faster than the semi-honest GPU-only pipeline across four models. We executed a specification and a functional CPU reference model, which covers every algorithm except the optional Freivalds check and passes all 22 unit tests (\cref{sec:eval-attack}); GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet, and six injections of \cref{tab:attacks}, including the release guard, lack executed evidence.
\end{itemize}

Throughout, red values are outputs or assumed parameters of our analytical model (\cref{app:model}) that await measurement; black values are reproduced from DFA~\cite{dfa2026trusted}, are design constants or analytical counts, or come from executed reference tests.

\Cref{sec:bg,sec:threat,sec:analysis} give background, the threat model and where the cost of malicious FSS goes; \cref{sec:protocol,sec:arch,sec:security,sec:eval} present the protocol, architecture, security analysis and evaluation; \cref{sec:discussion,sec:related,sec:conclusion} discuss limitations, related work and conclusions, and the appendices give the ideal functionalities, proofs and performance model.


==> qa/draft3/sections/02_background.tex <==
% ==================================================================
% Section II: Background
% Owner labels: sec:bg, sec:bg-fss, sec:bg-pi, sec:bg-pir, sec:bg-dfa,
%               sec:bg-mal, fig:flows, eq:dpf, eq:pir
% ==================================================================
\section{Background}
\label{sec:bg}

This section reviews the primitives that \sys builds on and the semi-honest DFA design~\cite{dfa2026trusted} that it extends.
We write $P_0,P_1$ for the two computing parties, $b\in\{0,1\}$ for a party index, $\lambda$ for the seed length of the pseudorandom generator (PRG), and $\one[\cdot]$ for the indicator of a predicate.

% ==================================================================
\subsection{Function Secret Sharing, DPF, and DCF}
\label{sec:bg-fss}

\textbf{Function secret sharing.}
A two-party function secret sharing (FSS) scheme~\cite{boyle2015fss,boyle2016function} for a function class $\mathcal{F}$ with output group $\mathbb{G}$ consists of $\Gen(1^\lambda,\hat f)$, which maps a description of $f\in\mathcal{F}$ to a key pair $(k_0,k_1)$, and $\Eval(k_b,x)$, which returns party $b$'s share $y_b\in\mathbb{G}$.
Correctness requires $\Eval(k_0,x)+\Eval(k_1,x)=f(x)$ for every $x$; security requires that each key alone be simulatable from public information (domain, output group, function class), so that a single key hides $f$.

\textbf{Distributed point function.}
A distributed point function (DPF)~\cite{gilboa2014distributed,boyle2015fss,boyle2016function} shares the point function $f_{\alpha,\beta}$ with target $\alpha\in\bits{n}$ and payload $\beta\in\mathbb{G}$:
\begin{equation}\label{eq:dpf}
\Eval(k_0,x)+\Eval(k_1,x)=\beta\cdot\one[x=\alpha]\quad\text{for all } x\in\bits{n}.
\end{equation}
In this paper $\mathbb{G}=\Fp$ with $p=2^{61}-1$ (\cref{sec:proto-repr}), inputs are read most-significant bit first, and we use the tree-based construction of Boyle et al.~\cite{boyle2016function}.
Each node of a depth-$n$ binary tree carries a state $(s,t)$ of a $\lambda$-bit seed and a control bit; a fixed PRG $\PRG:\bits{\lambda}\rightarrow(\bits{\lambda}\times\bits{})^2$ expands a seed into the states of its two children, and $\Conv:\bits{\lambda}\rightarrow\Fp$ converts a leaf seed into a field element.
Generation walks the target path from two independent root seeds with control bits $t_0=0$ and $t_1=1$; each level's correction word $\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$ makes both parties' states identical on the child leaving the path and keeps them pseudorandom with opposite control bits on the child staying on it, and an output correction $\CWout$ makes the signed outputs $y_b=(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$ sum to $\beta$ at $x=\alpha$ and cancel elsewhere.
Party $b$'s key holds its root seed, its fixed control bit $t_b^{(0)}=b$, the $n$ correction words and $\CWout$, i.e., $O(\lambda n)$ bits; \cref{alg:gen,alg:eval} in \cref{sec:analysis-dpf} give the exact algorithms.

\textbf{Evaluation patterns and cost.}
Generation expands $2n$ states and a single-path $\Eval(k_b,x)$ expands $n$; a full-domain $\EvalAll(k_b)$ expands $2^n-1$ internal nodes, keeping only $O(n)$ pending siblings in a depth-first traversal.
The PRG dominates all patterns; DFA, GPU-DPF~\cite{lam2023gpu} and \sys instantiate it with AES-128.
Two properties matter later.
Keys are \emph{one-time}: each encodes one mask or query index, and reusing a mask reveals the difference of the two inputs it hides.
DPF key privacy holds for \emph{arbitrary} $(\alpha,\beta)$~\cite{boyle2016function}, so uniform targets come from the application's masking (\cref{sec:bg-pi}), whose joint distribution any refactoring of generation must preserve (\cref{sec:proto-refactor}).

\textbf{Distributed comparison function.}
A distributed comparison function (DCF) shares $f^{<}_{\alpha,\beta}(x)=\beta\cdot\one[x<\alpha]$.
We use this ``$<$'' orientation throughout; DFA~\cite{dfa2026trusted} uses ``$>$'', and we convert explicitly at interfaces via $\beta\cdot\one[x>\alpha]=\beta-f^{<}_{\alpha+1,\beta}(x)$, treating the threshold $2^n$ as a public constant.
Optimized DCFs evaluate with $O(n)$ PRG expansions~\cite{boyle2021function}, and DCFs can be assembled from DPFs~\cite{storrier2023grotto}.
\sys uses the conservative $O(n^2)$ DCF of \cref{alg:dcf}, which sums $n$ prefix DPFs and whose correctness \cref{thm:dcf} proves (\cref{app:proof-dpf}).

% ==================================================================
\subsection{FSS-Based Private Inference}
\label{sec:bg-pi}

\textbf{Two-party secure inference.}
Private inference runs a neural network with private input, and possibly private weights, as a secure two-party computation~\cite{yao1986generate,goldreich2019play,mohassel2017secureml,rathee2020cryptflow2,crypten2020,tan2021cryptgpu,watson2022piranha}.
With additive shares $x=x_0+x_1$, linear operations are local, and a multiplication consumes a Beaver triple $(a,b,c=ab)$~\cite{beaver1991efficient}: the parties open $d=x-a$ and $e=y-b$ and locally compute shares of $xy=c+db+ea+de$.
Nonlinear layers (ReLU, GeLU, Softmax, LayerNorm) dominate the cost; earlier systems use multi-round Boolean conversions for them~\cite{demmler2015aby,mohassel2018aby3,wagh2019securenn,wagh2020falcon}.

\textbf{Masked-input FSS gates.}
FSS-based systems~\cite{boyle2019preprocessing,boyle2021function,ryffel2020ariann,wagh2022pika,gupta2023sigma,jawalkar2024orca} evaluate each nonlinear gate $g$ in the masked-input paradigm.
Offline, a dealer samples a fresh uniform mask $r$, shares it, and generates FSS keys for the offset function $g_r(c)=g(c-r)$, often with an output mask.
Online, the parties open $c=x+r$, which is uniform and independent of $x$, and the outputs $\Eval(k_b,c)$ are shares of $g(x)$.
Comparisons and ReLU use DCFs; splines for GeLU, exponentials and inverse square roots use DCF-based interval selection plus low-degree polynomials; and small lookup tables (LUTs) use DPFs~\cite{gupta2023sigma,jawalkar2024orca}.
Each gate costs one opening round, so the online phase is round-efficient but compute-intensive.

\textbf{Offline cost and the dealer assumption.}
The price is paid offline.
Semi-honest FSS inference of BERT-Base with 128 tokens moves 17.1~GB of one-time key material per query and LLaMA2-7B moves 256~GB, more than 90\% of it DPF keys~\cite{dfa2026trusted}; this cost cannot always be hidden behind online work, and its energy and monetary cost is never hidden~\cite{huang2026beyond}.
Sigma, Orca, and related systems~\cite{gupta2023sigma,jawalkar2024orca,crypten2020} obtain keys from a trusted dealer and assume semi-honest computing parties.

% ==================================================================
\subsection{DPF-Based Private Information Retrieval}
\label{sec:bg-pir}

PIR lets a client retrieve record $D[\alpha]$ of an $N$-record database $D$ without revealing $\alpha$~\cite{chor1998private}.
Single-server schemes rely on homomorphic encryption and are computationally heavy~\cite{angel2018pir,henzinger2023one}; we focus on the faster two-server DPF-based schemes~\cite{gilboa2014distributed,boyle2016function}.
With $n=\lceil\log_2 N\rceil$, the client sends $k_b$ of $(k_0,k_1)\leftarrow\Gen(1^\lambda,\alpha,1)$ to server $P_b$, which returns
\begin{equation}\label{eq:pir}
y_b=\sum_{x=0}^{N-1}\Eval(k_b,x)\cdot D[x],\qquad b\in\{0,1\},
\end{equation}
and by \cref{eq:dpf} the client obtains $D[\alpha]=y_0+y_1$.
Keys have $O(\lambda\log N)$ bits, but each query costs $O(N)$ PRG expansions plus an $N$-term inner product per server, and the expansion dominates even on GPUs~\cite{lam2023gpu}.
Standard DPF-based PIR protects the index but not the answer: a malicious server can add an offset $\delta$ to $y_b$, so that the client accepts $D[\alpha]+\delta$, or answer from a stale database.
Conversely, a malicious client can submit a malformed key pair that reconstructs a combination of several records, which verifiable DPFs detect~\cite{decastro2022vfss}.
Authenticated PIR (APIR)~\cite{colombo2023apir} lets the client verify answers against a database digest at additional server cost.
\Cref{sec:proto-pir} gives our protected versioned-snapshot design, in which both modules learn $\alpha$: unlike untrusted two-server DPF-PIR, its query privacy rests on module trust.

% ==================================================================
\subsection{Trusted DFA}
\label{sec:bg-dfa}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_flows.pdf}
    \caption{Execution flows of two-party FSS-based private inference in four configurations, from left to right.
    (1)~GPU without DFA (semi-honest): a trusted party generates FSS keys offline and ships them over the network; each party stores them, rereads them and transfers them to its GPU.
    (2)~Trusted DFA (semi-honest)~\cite{dfa2026trusted}: after a one-time initialization with attestation and key exchange, each on-die module generates its party's keys locally and merges generation with evaluation (generate-and-consume), removing the offline phase.
    (3)~Dealer-based malicious FSS, modeled after the protocol family of Shark~\cite{gupta2025shark}: the dealer also issues authenticated keys and triples, so about \est{2.2$\times$} as much offline material (red: model estimate, \cref{app:model}) must be shipped, stored and reread, while the GPU runs authenticated general matrix multiplication (GEMM) and checks MACs online.
    (4)~\sys (malicious): the protected module (red dashed trusted boundary) keeps local generation and generate-and-consume, adds the fresh authentication epilogue, freeze-before-challenge \CheckOpen{} and the release guard, and exchanges authenticated shares $\authb{x}{b}$ with a GPU that runs authenticated linear algebra on one value lane and three MAC-tag lanes; the inter-party network carries opened values and check residuals, not keys.}
    \label{fig:flows}
\end{figure*}

\textbf{Hardware.}
DFA~\cite{dfa2026trusted} integrates 16 DPF units with four pipelined AES-128 engines each (64 in total) next to the L2 slices of a GPU; each 20-stage unit sustains one Gen or Eval iteration per cycle after warm-up.
An SC300-class control core~\cite{st33tpm12spi,arm_cortex_m3} handles attestation and key management, and a 16-lane vector unit~\cite{cavalcante2019ara} runs protocol-specific pre- and post-processing.
The design runs at 720~MHz in 28~nm, delivers about 290~GB/s of DPF output in Accel-Sim~\cite{khairy2020accel}, and traverses full-domain trees depth-first, needing $O(nm)$ state for $m$ units instead of $O(2^n)$~\cite{dfa2026trusted}.

\textbf{Untrusted and trusted modes.}
In the \emph{untrusted mode}, DFA only expands seeds for keys produced elsewhere, and the protocol is unchanged.
In the \emph{trusted mode}, each party's module replaces the dealer: the modules attest to each other and establish a key $K$ that the hosts never see, derive the same generation coins (including $\alpha$) from $K$ and a counter, and thus compute identical correction words while each evaluates only its own party's share.
\emph{Generate-and-consume} (GaC) runs the joint generation and the local evaluation in lockstep, consuming each correction word as soon as it is produced, so that neither key distribution nor key storage remains.
DFA also \emph{decouples} generation from protocol preprocessing: when the target is $a=g(r)$ for a bijection $g$, the module samples $a$ uniformly and recovers $r=g^{-1}(a)$.

\textbf{Limits of the semi-honest design.}
DFA argues that correct in-module generation leaves the semi-honest protocol unchanged; against a deviating host this argument fails in four places treated later: (i)~decoupled preprocessing must preserve joint, not only marginal, distributions (\cref{sec:proto-refactor}); (ii)~generator and evaluator state is left implicit (\cref{sec:analysis-dpf}); (iii)~attestation authenticates the module configuration, not that the GPU used a valid key, computed the right product or released an authorized result (\cref{sec:threat-scenarios}); and (iv)~the GPU lies outside the trusted computing base (TCB) and must never obtain module tags for its own results (\cref{sec:proto-epilogue}).

% ==================================================================
\subsection{Tools for Malicious Security}
\label{sec:bg-mal}

\textbf{Security with abort.}
We use the stand-alone real/ideal simulation paradigm, which is preserved under sequential composition~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}; we make no concurrent-composition claim.
A malicious adversary deviates arbitrarily; security with abort requires that it achieve nothing beyond an ideal world in which a trusted functionality computes the result and the adversary only chooses corrupted inputs and whether honest parties receive output, so fairness is not required.
Covert security~\cite{aumann2007covert} only deters cheating; we target full malicious security with abort.

\textbf{Information-theoretic MACs.}
SPDZ-style protocols~\cite{damgard2012spdz,damgard2013practical} authenticate each value of a field $\F$ under a global key $\Delta=\Delta_0+\Delta_1$ that no single party knows.
Party $b$ holds $\Delta_b$ and $\authb{x}{b}=(x_b,\gamma_b)$ with $x_0+x_1=x$ and $\gamma_0+\gamma_1=\Delta x$; linear operations act identically on values and tags, and multiplications consume authenticated triples.
To check openings $z_1,\dots,z_m$, the parties draw coefficients $\rho_i$ \emph{after} the values are fixed, compute $\sigma_b=\sum_i\rho_i(\gamma_{b,i}-\Delta_b z_i)$, and accept only if $\sigma_0+\sigma_1=0$.
A wrong opening passes only if its tag error matches $\Delta$ times the value error or cancels under the coefficients, which happens with probability less than $2/|\F|$.
\sys instantiates this with $t=3$ independent lanes over $\Fp$ (\cref{sec:proto-repr}).

\textbf{Authenticated preprocessing.}
Malicious protocols need authenticated masks and triples whose relations, such as $c=ab$, are actually correct; a valid MAC on a wrong triple does not make it correct.
Generating them without a trusted party is communication-heavy, with oblivious transfer in MASCOT~\cite{keller2016mascot} or somewhat homomorphic encryption in SPDZ and Overdrive~\cite{damgard2012spdz,keller2018overdrive}, all in MP-SPDZ~\cite{keller2020mpspdz}.
Pseudorandom correlation generators~\cite{boyle2019pcg,boyle2020pcg} compress this communication at a substantial computational cost, and a trusted dealer avoids generation but ships every authenticated share.

\textbf{Malicious and verifiable FSS.}
Malicious FSS gates additionally need well-formed keys and authenticated evaluation outputs that can enter MAC-checked arithmetic.
Verifiable FSS~\cite{decastro2022vfss} checks that a key pair shares a function of the declared class, not that a malicious party evaluates its own key correctly.
Shark~\cite{gupta2025shark} achieves active security for FSS-based inference with a dealer that issues authenticated FSS keys and correlated randomness, which enlarges the offline material relative to semi-honest FSS.
The direct way to authenticate a DPF output, a second \emph{tag tree} with payload $\Delta_j\beta$ per MAC key, multiplies DPF work by $1+t$ for $t$ lanes (\cref{sec:analysis-work}).

\textbf{Trusted hardware for secure computation.}
Slalom~\cite{tramer2018slalom} and DarKnight~\cite{hashemi2021darknight} outsource linear layers from a trusted execution environment (TEE) to untrusted GPUs and check the results, Slalom with Freivalds' algorithm~\cite{freivalds1977probabilistic}, which \sys uses only for a restricted subroutine (\cref{sec:proto-freivalds}).
PPMLAC~\cite{zhou2022ppmlac} and STAMP~\cite{huang2022efficient} use small trusted modules to generate correlated randomness or to execute nonlinear operations; STAMP also reports honest-majority malicious settings, and \cref{sec:related} compares these and other trusted-hardware designs.

\textbf{Implications.}
Each tool covers only part of the integrity chain of \cref{sec:intro}, at a cost that erodes trusted DFA's advantage (\cref{sec:analysis}); \sys therefore keeps the module as the dealer and also makes it the verifier (\cref{sec:protocol}).

\textbf{Scope.}
Throughout this paper, \emph{private inference} means two-party FSS-based private inference and \emph{PIR} means two-server DPF-based PIR, as in DFA~\cite{dfa2026trusted}.


==> qa/draft3/sections/03_threat_model.tex <==
% ==================================================================
% Section III: Threat Model and Security Goals
% Owner labels: sec:threat, sec:threat-model, sec:threat-scenarios,
%   sec:threat-goals, sec:threat-profileu, fig:threat, fig:scenarios,
%   tab:scenarios, fig:func, def:security, def:leakage
% ==================================================================
\section{Threat Model and Security Goals}\label{sec:threat}

The trusted mode of DFA moved the FSS dealer into a small protected module but kept the semi-honest model of the protocols it accelerates~\cite{dfa2026trusted}. This section states what changes when a host is malicious: we fix the system model (\cref{sec:threat-model}) and the adversary, derive ten attack scenarios (\cref{sec:threat-scenarios}), define security with explicit leakage (\cref{sec:threat-goals}), and delimit \ProfU (\cref{sec:threat-profileu}). Every link of the integrity chain of \cref{sec:intro} crosses memory, buses, or network paths that a corrupted host controls.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_threat.pdf}
    \caption{System model and trust boundary of \sys under \ProfT. Each party $P_b$ has an untrusted host (CPU, OS, driver, runtime, network interface card (NIC), DRAM) with its GPU, including the streaming multiprocessors (SMs) and high-bandwidth memory (HBM), and a protected module $T_b$ (red dashed TCB, contents in \cref{sec:threat-model}). The adversary statically corrupts at most one host (here that of $P_0$, red region) and may deviate arbitrarily, replay, and abort, but never corrupts $T_0$ or $T_1$. Hosts and GPUs hold only party-local authenticated shares; the protected peer channel between the modules and the authenticated confidential client channels are carried by the untrusted network.}
    \label{fig:threat}
\end{figure*}

\subsection{System Model and Trust Boundary}\label{sec:threat-model}

\textbf{Parties.}
\sys targets the two workloads of DFA~\cite{dfa2026trusted}: two-party FSS-based private inference and two-server DPF-based PIR (\cref{sec:bg}). Two computing parties $P_0$ and $P_1$ serve an external client that owns private inputs and receives outputs; a computing party may also own an input, typically the model weights. Each $P_b$ consists of an untrusted \emph{host~$b$} (every component outside the TCB in \cref{fig:threat}, including DMA engines and storage) and a \emph{protected module} $T_b$, the \sys extension placed next to the GPU L2 as in DFA (\cref{sec:arch-hw}).

\textbf{Trusted computing base.}
$T_b$ contains the session, identity (attestation), and joint-sampler keys and the global MAC keys $\Delta_1,\dots,\Delta_t$; the session role, counters, and one-time resource ledger; the DPF generator and evaluator states and the correction words; the protected table and reduction logic; the frozen check buffers, challenges, and residuals; and all release decisions. Everything else is outside, including every GPU and DMA buffer and every byte in transit between the parties. The GPU computes on party-local authenticated arrays and hands $T_b$ only \emph{candidate} shares (\cref{sec:proto-repr}). Host~$b$ may know its own MAC key shares $\Delta_{b,j}$, but no host ever holds a complete $\Delta_j$, the joint-sampler key, a complete mask (other than the input mask of a wire its party owns or the output mask of an output its party is authorized to receive), the peer's shares, or any challenge or residual.

\textbf{Modules as an ideal resource.}
Following~\cite{katz2007universally}, we model $T_0,T_1$ as an ideal resource $\mathcal{F}_{\mathsf{T}}$ (\cref{app:func-module}; ideal-module assumption in \cref{sec:sec-assump}): their code, keys, parser, arithmetic, state, and approved I/O paths are correct and confidential, and each module's externally observable trace (lengths, timing, host-visible memory and DMA activity, power, thermal, and clock telemetry) is simulatable from the command sequence issued by the host, $\mu$, public lengths, and the accept or abort outcomes, and is independent of the global MAC keys, challenges, and residuals given these. The real execution (\cref{def:security}) realizes their randomness, channels, and setup with concrete primitives. Availability is not assumed, \ProfT requires two physically independent modules, and only the on-die design (\cref{sec:arch-hw}) is a \ProfT target.

\textbf{Channels.}
Client channels are authenticated, confidential, and terminate inside the modules; the peer channel uses AEAD with independent directional keys and no nonce reuse and is established by the authenticated setup of \cref{sec:proto-setup}. The untrusted network carries both. We propose no new attestation or key-exchange protocol; the security of setup is the explicit assumption $\eps{setup}$.

\textbf{Trust is relocated, not removed.}
The modules jointly act as the dealer and can recover inputs from verified openings, and in PIR both modules learn the queried index $\alpha$. \sys thus moves trust from an external dealer and the hosts into the modules rather than hiding inputs from them (\cref{sec:discussion}); its PIR query privacy rests on module trust, unlike untrusted two-server DPF-PIR such as GPU-DPF~\cite{lam2023gpu} or DFA's untrusted mode~\cite{dfa2026trusted}, which hides $\alpha$ from each server without trusted hardware.

\subsection{Adversary Model}

Unlike DFA~\cite{dfa2026trusted}, Sigma~\cite{gupta2023sigma}, and Orca~\cite{jawalkar2024orca}, which assume that both hosts run the prescribed kernels, we consider a probabilistic polynomial-time (PPT) adversary $\Adv$ that statically and maliciously corrupts at most one host before the session starts (host~$0$ in \cref{fig:threat}, by symmetry), controlling its operating system, drivers, GPU kernels and results, host and GPU memory including DMA buffers, and outgoing network traffic. Concretely, $\Adv$ can
(i) modify any value share or tag and run arbitrary kernels in place of the prescribed ones;
(ii) invoke its module's commands in any order with malformed, replayed, or mislabeled arguments;
(iii) rewrite any host-visible buffer at any time, including while the module reads it;
(iv) replay, reorder, delay, or drop messages, reset its platform, and restore old host-side state;
(v) choose the inputs it owns arbitrarily; and
(vi) abort at any point, including after it has learned its own output.
It observes message lengths and timing, the frames exchanged with its module, and the module's external trace. The principal inference statement assumes an honest external client and gives no guarantee against client-server collusion; PIR has two separate regimes, (R1) one malicious server host and (R2) a malicious client only with two honest server hosts (\cref{fig:func}).

\textbf{Out of scope.}
Our theorems exclude corruption of either module (its code, keys, state, or arithmetic); physical attacks such as microprobing, optical fault injection, and power or electromagnetic analysis with measurement equipment~\cite{skorobogatov2017microprobing,skorobogatov2003optical,kocher1999differential,quadir2016survey}; leakage beyond the stipulated trace model; speculative-execution bugs inside the trusted boundary~\cite{van2018foreshadow}; faulty trusted arithmetic; adaptive corruption; and corruption of both hosts. Software-reachable fault and power channels are not physical attacks: the corrupted host controls the GPU driver, which sets clocks, voltage, and power limits and reads telemetry, an interface that Plundervolt exploited on CPUs~\cite{murdock2020plundervolt}. We therefore require isolation from dynamic voltage and frequency scaling (DVFS): host software cannot drive the module's clock or voltage outside its safe operating range (or the module detects glitches and aborts), and the telemetry is covered by the trace simulator. Rollback of module state is covered only by the reboot rule of \cref{sec:proto-ledger}. Availability and fairness are not provided.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_scenarios.pdf}
    \caption{Malicious scenarios S1 to S8 against trusted FSS acceleration and the \sys mechanism that stops each. Corrupted hosts and GPUs are shaded red, $T_b$ is the red dashed TCB, red arrows with circled numbers are adversary actions, red crosses mark where \sys blocks them, and green text names the defense. S9 and S10, which no protocol can prevent, appear only in \cref{tab:scenarios}.}
    \label{fig:scenarios}
\end{figure*}

\subsection{Malicious Scenarios Against Trusted FSS Acceleration}\label{sec:threat-scenarios}

\Cref{fig:scenarios} and \cref{tab:scenarios} list what a corrupted host can do to a trusted FSS accelerator designed for semi-honest hosts and which \sys mechanism stops each action; the paragraphs below explain why the semi-honest design fails. The scenarios follow the integrity chain: S9 targets the authorized input; S4 and S7 the correlated preprocessing; S2 and S5 the correct local evaluation; S1 the authenticated arithmetic; S3 the consistent opening; and S6 the authorized output release. S8 carries S3 over to the PIR database, and S10 targets availability, which lies outside the chain. \Cref{sec:sec-scenarios,sec:eval-attack} map the scenarios to theorems and to injected tests.

\textbf{S1: Share and tag tampering.}
The corrupted GPU holds every intermediate share and can add an error vector $\bm{e}$ to value shares (and $\bm{d}_j$ to the tags of lane $j$); semi-honest trusted DFA passes it unchecked into the masked opening $x_i+r_i$ of the next FSS gate. Beyond biasing results, this causes \emph{selective failure}: whether $e_i$ flips a comparison depends on whether $x_i$ lies within $|e_i|$ of the threshold, so any observable output change leaks information about $x_i$ (\cref{tab:scenarios}, \cref{sec:proto-check}).

\textbf{S2: Forgery-oracle request.}
A tempting extension of DFA's trusted mode is a command that tags a value computed elsewhere, such as a nonlinear output computed by the GPU's streaming multiprocessors (SMs). This \emph{authenticate(host value)} entry point turns the module into a MAC oracle: the host submits any $y^*$, and every later check accepts it. Attestation certifies the module's code, not the provenance of what it signs (\cref{tab:scenarios}, \cref{sec:proto-epilogue}).

\textbf{S3: TOCTOU buffer swap.}
The module reads its inputs by DMA from host-controlled memory. Verifying a buffer and later rereading it, or trusting a host-reported digest, admits a time-of-check-to-time-of-use (TOCTOU) swap: the host changes the bytes after verification or chooses its error after the challenge is fixed. DMA completion is not evidence of authenticity, a problem semi-honest DFA never faced (\cref{tab:scenarios}, \cref{sec:proto-check}).

\textbf{S4: Replay and rollback.}
DFA derives keys and masks from the shared key $K$ and a counter that is an input of its generate-and-consume procedure~\cite{dfa2026trusted}. Replaying a counter yields the same mask $r$ for two gates, and the openings $x+r$ and $x'+r$ reveal $x-x'$; resetting the module and resuming an old session replays entire key streams (\cref{tab:scenarios}, \cref{sec:proto-ledger}).

\textbf{S5: Role and gate confusion.}
The host decides which module command runs for which gate: it can route the preprocessing of gate $g$ into gate $g'$, alter a table hash or tensor shape, or present party-$0$ material as party-$1$ material. If the role were a per-request argument, the host could obtain both parties' outputs of one joint draw and reconstruct the DPF target $\alpha$, which is exactly the mask of an honest input (\cref{tab:scenarios}, \cref{sec:proto-setup,sec:proto-ledger}).

\textbf{S6: Premature release.}
Semi-honest trusted DFA releases results as soon as they are computed; under a malicious host an early output may already be wrong, and the host may request it repeatedly or for an unauthorized recipient (\cref{tab:scenarios}, \cref{sec:proto-ledger}).

\textbf{S7: Malformed preprocessing.}
A MAC authenticates values, not relations: a triple $(\auth{a},\auth{b},\auth{c})$ with $c\neq ab$ carries valid tags, and multiplying with it yields $xy+\delta$ for a $\delta$ chosen by its producer; the same holds for a GPU-computed matrix product with $C\neq AB$ and for a malformed DPF key. DFA's attestation covers the module's own key generation, not correlations from elsewhere (\cref{tab:scenarios}, \cref{sec:proto-arith}).

\textbf{S8: Snapshot substitution in PIR.}
The PIR database resides in host memory, so a corrupted server host can modify a record, serve an older version, or hash one buffer while scanning another. Semi-honest PIR, including DFA-accelerated PIR, returns whatever the servers compute. Worse, a record modified only at position $i$ corrupts the answer only when $\alpha=i$, so the client's reaction leaks the queried index (\cref{tab:scenarios}, \cref{sec:proto-pir}).

\textbf{S9 and S10: Input substitution; denial of service and selective abort.}
S9, a corrupt owner choosing its input freely, is permitted and extracted by $\FC$; binding a specific model needs the commitment of \emph{Model provenance} below. S10 is not prevented: like SPDZ-style protocols~\cite{damgard2012spdz,keller2016mascot}, \sys provides security with abort, without fairness or guaranteed output delivery, and abort outcomes stay within the permitted leakage (\cref{def:leakage}, \cref{sec:discussion}).

\begin{table*}[t]
\centering
\caption{Malicious scenarios against trusted FSS acceleration. The ``effect'' column describes a semi-honest trusted DFA~\cite{dfa2026trusted}, or a naive malicious extension of it, when one host is corrupted. \cmark: prevented up to the error terms of \cref{thm:main}; \pmark: permitted by the ideal functionality; \xmark: not prevented.}
\label{tab:scenarios}
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabularx}{\textwidth}{c >{\raggedright\arraybackslash}p{1.75cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{2.75cm}}
\hline
\textbf{ID} & \textbf{Scenario} & \textbf{Adversary action} & \textbf{Effect on semi-honest trusted DFA} & \textbf{\sys mechanism} & \textbf{Guarantee} \\
\hline
S1 & Share/tag tampering & GPU adds errors $\bm{e}$ to value shares (and $\bm{d}_j$ to tags) before an opening or FSS gate & Undetected; biases outputs and causes selective failure that leaks inputs & Authenticated shares with $t=3$ MAC lanes over $\Fp$; \CheckOpen{} before any protected gate or release & \cmark\ Wrong value accepted w.p.\ $\le (2/p)^t$ per batch (\cref{thm:mac-sound}) \\
\hline
S2 & Forgery-oracle request & Host submits $y^*$ and asks its module to authenticate it & No MACs; a naive authenticate command would sign any forgery & No \emph{authenticate(host value)} command; \Epilogue{} only on internally computed or verified results & \cmark\ Request rejected; outputs correctly authenticated (\cref{thm:epilogue}) \\
\hline
S3 & TOCTOU buffer swap & Host rewrites a DMA buffer after it is checked, or after the challenge is fixed & Module trusts DMA reads; a later reread consumes modified bytes & Freeze before challenge: bytes copied or AEAD-sealed, frozen roots agreed, only frozen bytes consumed & \cmark\ Modification ignored or abort; binding error $\eps{bind}$ \\
\hline
S4 & Replay and rollback & Replays a counter or mask request; resets the module and resumes old keys & Mask reuse: $x+r$ and $x'+r$ reveal $x-x'$; key streams replayed & Labels bound to session, epoch, gate, purpose; one-time ledger; epoch poisoning; erase-and-rekey after reboot & \cmark\ Reuse rejected before any accepted use \\
\hline
S5 & Role/gate confusion & Routes party-0 material as party-1, or gate $g$ material into gate $g'$; alters shapes or table hash & Host schedule trusted; requesting both roles' outputs exposes the target $\alpha$ & Roles fixed by authenticated setup; gate descriptors bound in the ledger and in PRF labels & \cmark\ Mismatched commands abort before preprocessing is issued; host-side reuse of issued shares fails \CheckOpen{} except w.p.\ $\le(2/p)^t$ (\cref{thm:mac-sound}) \\
\hline
S6 & Premature release & Requests outputs before verification, repeatedly, or for another recipient & Results released as soon as computed & Release guard: nothing before \lstate{VERIFIED}; bound certificates; epoch abort gates pending outputs & \cmark\ No candidate value leaves the modules \\
\hline
S7 & Malformed preprocessing & Injects a triple with valid tags but $c\neq ab$, a GPU-computed product with $C\neq AB$, or a wrong DPF key & Attestation silent on external correlations; MACs verify wrong triples & Triples and keys generated inside the TCB ($c=ab$ computed there); imports need a correctness proof & \cmark\ Never consumed; exact arithmetic (\cref{thm:arith}) \\
\hline
S8 & Snapshot substitution (PIR) & Swaps records or version after hashing, or scans a different buffer & Client reconstructs a wrong record; index-dependent failure leaks $\alpha$ & Module hashes the bytes it consumes in public order; quarantine until the commitment matches & \cmark\ Committed record or abort (\cref{thm:pir}) \\
\hline
S9 & Input substitution by a corrupt owner & Corrupted party supplies arbitrary weights or inputs & Same (allowed) & Input extraction by $\FC$; optional commitment-bound loader for model provenance & \pmark\ Allowed by the functionality \\
\hline
S10 & Denial of service/selective abort & Drops, delays, or reorders messages; aborts after learning its own output & Same (not prevented) & Bounded resources and abort; abort outcomes simulatable from permitted leakage & \xmark\ Not prevented (no fairness or availability) \\
\hline
\end{tabularx}
\end{table*}

\subsection{Security Goals and Ideal Functionalities}\label{sec:threat-goals}

\textbf{Goals.}
Against a corrupted host, \sys must provide \emph{privacy} (the host learns nothing beyond the permitted leakage and the outputs it is authorized to receive), \emph{correctness} (honest recipients obtain the circuit evaluated on the honest inputs and the corrupted party's extracted inputs, or abort), \emph{authorized release} (no value leaves the modules unless its opening was verified and bound to a release certificate), and \emph{one-time use} (no randomness is consumed twice). We formalize the first two as stand-alone real/ideal security with abort, preserved under sequential composition~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}, with an explicit leakage function; the last two are mechanisms that the proof relies on (\cref{sec:proto-ledger}). We claim neither universal nor concurrent composability, and concurrent sessions that share module state are not covered.

\textbf{Manifest.}
Every session fixes a public manifest $\mu$ (\cref{app:func-circuit}): the protocol version, session identities, roles, field, numeric encoding, the finite circuit $C$ with its gate and wire identifiers and tensor shapes, approved public tables, interval coefficients, authorized recipients, the input interface $\mathsf{In}_\nu$ and validation rules of every input wire $\nu$, and the public schedule, which places every input gate before every validity check, and both before the first output opening. The modules evaluate the validity predicates at the public boundaries declared in $\mu$; in $\Pi_{\mathsf{Input}}$ they compute $x^{*}=r+\varepsilon$ and abort unless $x^{*}\in\mathsf{In}_\nu$ (\cref{fig:arith}).

\begin{definition}[Permitted leakage]\label{def:leakage}
For a circuit execution under manifest $\mu$, the permitted leakage is
\[
\Leak_C=\bigl(\mu,\ \mathsf{len},\ \mathsf{sched},\ \mathsf{pub},\ \mathsf{status}\bigr),
\]
where $\mathsf{len}$ are the lengths of all public messages; $\mathsf{sched}$ is the public schedule of batches, checks, and interaction boundaries fixed by $\mu$; $\mathsf{pub}$ are the values that $\mu$ designates as authorized public openings; and $\mathsf{status}$ are the specified abort and validation outcomes, including every input-dependent validity bit declared in $\mu$, which is never silently excluded. For PIR, $\Leak_{\mathrm{PIR}}$ consists of the public descriptor $\mathsf{desc}_v=(\mathsf{id},v,N,\mathsf{enc},\mathsf{cm}_v)$ (database identifier, version, true length $N$, which also fixes the padded length, record encoding, and authorized snapshot commitment), the public scan length and order, message lengths and schedules, and the accept, reject, or abort outcome.
\end{definition}

Honest inputs, intermediate wire values, masks, MAC keys, DPF keys and correction words, raw FSS outputs, challenges, and residuals are not in $\Leak_C$. Masked openings such as $x+r$ are uniform given $\Leak_C$, and the simulator samples them (\cref{app:proof-main}). Module timing and access patterns are fixed by $\mu$ (full-domain scans have a declared order); the residual trace falls under $\eps{trace}$.

\begin{figure}[t]
\centering
\footnotesize
\fbox{\begin{minipage}{\dimexpr\columnwidth-2\fboxsep-2\fboxrule\relax}
\centering\underline{Functionality $\FC$}\par\smallskip
\raggedright
\textbf{Parameters.} Public manifest $\mu$ (circuit $C$ over $\Fp$, input owners and interfaces $\mathsf{In}_\nu$, validity predicates, authorized recipients, public schedule). Corrupted set $I$: at most one host; the client is honest.
\begin{enumerate}[leftmargin=*,nosep,topsep=2pt]
\item \textbf{Input.} Receive the authenticated input $x_\nu$ of every input wire $\nu$ from its designated owner. If the owner is corrupted, receive $x^{*}_\nu$ from $\Sim$ and set $x_\nu\gets x^{*}_\nu$ (extraction). If some $x_\nu$ is missing, malformed, or not in $\mathsf{In}_\nu$, send $\bot$ to every honest recipient and halt; this abort outcome is part of $\mathsf{status}$.
\item \textbf{Validate and evaluate.} Evaluate the validity predicates of $\mu$; their accept or abort outcome is part of $\mathsf{status}$. For accepted inputs, compute $\vec{y}=C(\vec{x})$ exactly in the declared finite arithmetic, including the specified comparisons and truncations.
\item \textbf{Deliver or abort.} Send $\Leak_C$ and the outputs of corrupted recipients to $\Sim$. At each public interaction boundary, $\Sim$ may send $\mathsf{abort}$ or $\mathsf{delay}$; on $\mathsf{abort}$, send $\bot$ to every honest recipient. Otherwise deliver each $y_i$ to its authorized recipient. A corrupted recipient may obtain its output before honest ones (no fairness).
\end{enumerate}
\end{minipage}}

\vspace{5pt}
\fbox{\begin{minipage}{\dimexpr\columnwidth-2\fboxsep-2\fboxrule\relax}
\centering\underline{Functionality $\FPIR$}\par\smallskip
\raggedright
\textbf{Parameters.} Public descriptor $\mathsf{desc}_v=(\mathsf{id},v,N,\mathsf{enc},\mathsf{cm}_v)$; the commitment $\mathsf{cm}_v$ fixes $D=(D[0],\dots,D[N-1])$. Corruption regimes, never combined: (R1) a malicious server host (at most one), client honest; (R2) a malicious client only, both server hosts honest.
\begin{enumerate}[leftmargin=*,nosep,topsep=2pt]
\item \textbf{Query.} Receive an index $\alpha$ with query identifier $\mathit{qid}$ from the client; in (R2), extract the corrupted client's index $\alpha^{*}$ and set $\alpha\gets\alpha^{*}$. If $\alpha\notin\{0,\dots,N-1\}$ or the request is inconsistent, return $\mathsf{reject}$ to the client and stop.
\item \textbf{Leak.} Send $\Leak_{\mathrm{PIR}}$ to $\Sim$; nothing about $\alpha$ is sent.
\item \textbf{Answer.} In (R1), if $\Sim$ sends $\mathsf{abort}$, send $\bot$ to the client; otherwise send $D[\alpha]$. In (R2), send $D[\alpha]$, and no other information about $D$, to the client.
\end{enumerate}
\end{minipage}}
\caption{Ideal functionalities for authenticated circuit evaluation (top) and versioned-snapshot PIR (bottom). Both provide security with abort. $\FPIR$ hides $\alpha$ from the corrupted host; both trusted modules learn it (\cref{sec:threat-model}). The full definitions, together with the ideal module resource $\mathcal{F}_{\mathsf{T}}$, are in \cref{app:func}.}
\label{fig:func}
\end{figure}

\begin{definition}[Static malicious security with abort]\label{def:security}
Let $\mathcal{F}\in\{\FC,\FPIR\}$ with leakage $\Leak$ as in \cref{def:leakage}, and let $\Pi$ be a protocol run by $P_0$ and $P_1$ in which each module executes the concrete module program correctly and confidentially: $\mathcal{F}_{\mathsf{T}}$ with its joint random function $R$ instantiated by $\PRF_K$, its peer and client channels by AEAD over the hosts' network, and \cmd{OPEN_SESSION} by attestation and authenticated key exchange.
For a PPT adversary $\Adv$ with auxiliary input $z$ that statically corrupts the set $I$, $\Real_{\Pi,\Adv(z),I}(\mu,\vec{x})$ is the joint distribution of the view of $\Adv$ (its inputs, randomness, received messages, and the external traces of the modules observable from corrupted hosts) and the outputs of the honest parties and client in an execution of $\Pi$ on manifest $\mu$ and input vector $\vec{x}$.
$\Ideal_{\mathcal{F},\Sim(z),I}(\mu,\vec{x})$ is the joint distribution of the output of a simulator $\Sim$ and the honest outputs in an execution in which $\Sim$ interacts only with $\mathcal{F}$: it submits the corrupted parties' inputs, receives $\Leak$ and the corrupted parties' outputs, and may abort or delay as $\mathcal{F}$ allows.
We say that $\Pi$ \emph{$\epsilon$-securely realizes $\mathcal{F}$ with leakage $\Leak$ against static malicious corruption with abort} if for every PPT adversary $\Adv$ and every set $I$ admitted by the corruption regime of $\mathcal{F}$ there exists a PPT simulator $\Sim$ such that for all $\mu$, $\vec{x}$, $z$ and every PPT distinguisher $\mathcal{D}$,
\begin{align*}
\Bigl|&\Pr\bigl[\mathcal{D}\bigl(\Real_{\Pi,\Adv(z),I}(\mu,\vec{x})\bigr)=1\bigr]\\
&\quad-\Pr\bigl[\mathcal{D}\bigl(\Ideal_{\mathcal{F},\Sim(z),I}(\mu,\vec{x})\bigr)=1\bigr]\Bigr|\le\epsilon .
\end{align*}
\end{definition}

\textbf{Remarks.}
The real world of \cref{def:security} contains the concrete module program; $\mathcal{F}_{\mathsf{T}}$ with ideal setup, channels, and randomness is the resource of hybrids $\Hyb{2}$ to $\Hyb{4}$ of the proof (\cref{app:proof-main}), and the simulator controls only this ideal representation of the trusted resources, never the honest party's prescribed inputs. The concrete $\epsilon$ is the bound $\eps{VIGOR}$ of \cref{thm:main}; correctness of protected code is a premise of $\mathcal{F}_{\mathsf{T}}$, and \cref{tab:obligations} lists what a chip must still establish.

\textbf{Model provenance.}
Computational correctness is not model provenance, and a public architecture hash in $\mu$ does not authenticate private weights. To bind a pre-approved model, $\mu$ must contain a commitment to the canonical quantized weight bytes, authorized by the client or an independent model authority rather than declared by the untrusted host, and the protected input loader hashes exactly those bytes before sharing them (\cref{sec:proto-arith}); a mismatch aborts. Otherwise the weights are the owner's freely chosen private input, and S9 is the intended behavior of $\FC$.

\subsection{The Stronger Profile U}\label{sec:threat-profileu}

\ProfT trusts the modules. When the hardware itself must be treated as adversarial, for example because the accelerator vendor or platform administrator is untrusted, \ProfU gives the accelerator neither the joint-sampler key nor any global MAC key. The circuit runs through an established malicious two-party backend, such as SPDZ-family protocols with MASCOT or SPDZ2k preprocessing~\cite{damgard2012spdz,keller2016mascot,cramer2018spdz2k,keller2020mpspdz} or dealer-based malicious FSS such as Shark~\cite{gupta2025shark}, and the accelerator is confined to party-local data, for instance expanding the DPF keys that the backend exports to its own party. The same DPF datapath therefore serves both profiles, but \ProfU gives up the local-dealer and generate-and-consume savings, and with exported keys it must add the backend's DPF privacy assumption to its bound (\cref{sec:sec-main}). \ProfU is a separate backend chosen at session start, not a fallback after a module compromise, which would not undo leaked secrets; a fresh session with fresh inputs and masks is required. The rest of this paper analyzes and evaluates \ProfT.


==> qa/draft3/sections/04_analysis.tex <==
% ======================================================================
% Section IV: Workload Analysis (owner: sections/04_analysis.tex)
% Labels defined here: sec:analysis, sec:analysis-cost, sec:analysis-dpf,
% sec:analysis-work, alg:gen, alg:eval, fig:gac, tab:gatecost, fig:motiv
% ======================================================================
\section{Workload Analysis: Where Malicious Security Costs Go}
\label{sec:analysis}

The DFA design~\cite{dfa2026trusted} was driven by one workload observation: in semi-honest FSS workloads, DPF generation, distribution and evaluation dominate both computation and communication, so a small DPF engine that also plays the dealer removes the dominant cost. Repeating this analysis for the adversary of \cref{sec:threat} changes the design target: handled naively, malicious security multiplies exactly the DPF work and key traffic that trusted DFA made small; handled carefully, it moves the cost from DPF to authenticated linear algebra on the GPU and to the extra round of every verified opening.

% ======================================================================
\subsection{Cost Sources in Malicious FSS}
\label{sec:analysis-cost}

We take as reference the masked-input paradigm of FSS-based inference~\cite{gupta2023sigma,jawalkar2024orca} (\cref{sec:bg-pi}): linear layers operate on additive shares, and every nonlinear gate opens a masked input $x+r$ and evaluates FSS keys prepared for the mask $r$. Making this pipeline secure against a malicious host (\cref{def:security}) adds the following costs, regardless of how they are implemented.

\textbf{(i) Authenticated representation.}
Every wire must carry information-theoretic MACs so that a host that changes its share is caught~\cite{damgard2012spdz,damgard2013practical}. In our representation (\cref{sec:proto-repr}), party $b$ holds $\authb{x}{b}=(x_b,\gamma_{b,1},\gamma_{b,2},\gamma_{b,3})$ over $\Fp$ with $p=2^{61}-1$ and $t=3$ independent MAC keys: four 64-bit words, or 32~B per element and party, instead of 8~B for a semi-honest share in $\Z_{2^{64}}$. Every linear layer is therefore computed on four lanes (the value and three tags), each lane uses exact Mersenne reduction instead of free 64-bit wraparound (\cref{sec:arch-field}), and every authenticated element that crosses PCIe or the host-module interface grows by the same factor of four. Only the peer link is spared, because checks exchange value shares and $t$ residuals rather than tags (\cref{sec:proto-check}).

\textbf{(ii) Verified openings.}
Opened values (masked gate inputs, the Beaver differences $d,e$ of each multiplication~\cite{beaver1991efficient}, and outputs) must be checked before anything depends on them. A sound check derives its challenge only after the checked bytes are fixed (\cref{thm:mac-sound}), so at least one extra exchange follows every checked batch, and a dependent nonlinear gate may not consume an unchecked opening. Batching amortizes challenge derivation and metadata but not this round, which lies on the critical path of every layer: a protocol with $R$ online rounds approaches $2R$.

\textbf{(iii) Correct preprocessing.}
Triples, masks and FSS keys must be \emph{correct}, not merely authenticated: a valid MAC on a triple with $c\neq ab$ does not make it correct. The options of \cref{sec:bg-mal} either ship more offline material from a dealer or replace the dealer by heavy interactive preprocessing, and neither removes offline data movement. Without a dealer, FSS keys require a secure two-party evaluation of DPF key generation, with one round per tree level~\cite{doerner2017scaling} before any malicious-security overhead.

\textbf{(iv) Authenticated FSS outputs.}
A DPF output share is a plain additive share. To re-enter authenticated arithmetic it needs $t$ tag shares, and the straightforward way to obtain them is a second DPF per MAC lane $j$ with the same target and payload $\Delta_j\beta$ (a \emph{tag tree}). This multiplies DPF keys, key bytes and PRG work by $1+t$, i.e., by four for $t=3$.

\textbf{(v) Key validity is not evaluation correctness.}
Verifiable FSS~\cite{decastro2022vfss} lets evaluators check that their keys are well formed, which protects against a malicious key generator. It does not constrain an evaluator that computes on valid keys and then adds an error to its output share, nor the arithmetic that consumes that share.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{charts/chart_motiv.pdf}
    \caption{Estimated BERT-Base latency breakdown on LAN (1~GB/s, 0.05~ms round-trip time) by cost source, for two semi-honest configurations of~\cite{dfa2026trusted} and three malicious ones (dealer-based malicious FSS, \sys without GaC, \sys); all splits come from our model (\cref{app:model}). The horizontal axis is broken between 7.5 and 15~s so that the 18.8~s semi-honest GPU bar and the \est{43.9~s} dealer-based bar fit.}
    \label{fig:motiv}
\end{figure}

\textbf{Observation 1: distribution still dominates dealer-based malicious FSS.}
\Cref{fig:motiv} splits the estimated BERT-Base LAN latency by cost source. Dealer-based malicious FSS, modeled after the protocol family of Shark~\cite{gupta2025shark} (\cref{sec:eval-method}), must move \est{37.6~GB} of authenticated keys and preprocessing per query, \est{2.2$\times$} the 17.1~GB of the semi-honest GPU baseline~\cite{dfa2026trusted}. At 1~GB/s, this distribution alone takes \est{37.6~s} of \est{43.9~s} (\est{86\%}), and moving the material from host memory into the GPU adds another \est{1.70~s}. Without an authenticated-key blow-up ($\psi_{\mathrm{key}}=1$, \cref{app:model}), it still takes \est{22.4~s}, \est{5.8$\times$} that of \sys.

\textbf{Observation 2: without distribution, DPF is no longer the bottleneck.}
Removing distribution, as trusted DFA did for the semi-honest case, exposes a different profile. In \sys, four-lane authenticated GEMM takes \est{2.60~s} of \est{3.83~s} (\est{68\%}), \est{5.0$\times$} our \est{0.52~s} estimate of the semi-honest GEMM; online communication takes \est{0.615~s} (\est{16\%}); and all nonlinear gates together take only \est{0.131~s} (\est{3.4\%}).

\textbf{Observation 3: on a WAN, verification rounds dominate.}
With a 70~ms round-trip time (RTT) the extra check round of source (ii) outweighs all computation: removing \CheckOpen, which is insecure and serves only as a lower bound, would cut the estimated BERT-Base WAN latency from \est{89.7~s} to \est{50.5~s} (\cref{tab:ablation}).

% ======================================================================
\subsection{Compute Pattern of Exact DPF}
\label{sec:analysis-dpf}

Malicious-security proofs reason about concrete states, so we fix the DPF computation exactly. \Cref{alg:gen,alg:eval} give the tree-based DPF~\cite{gilboa2014distributed,boyle2016function} in the form that \sys executes; the same algorithms serve \ProfU, where keys are exported to an external malicious backend (\cref{sec:threat-profileu}). The expansion function $\PRG:\bits{128}\to(\bits{128}\times\{0,1\})^2$ is fixed and AES-based as in DFA, $\Conv:\bits{128}\to\Fp$ is the fixed output conversion, the target $\alpha$ and the query $x$ have $n$ bits read most-significant first, and the payload is $\beta\in\Fp$.

\begin{algorithm}[t]
\caption{Exact DPF key generation ($\DPF.\Gen$)}
\label{alg:gen}
\begin{algorithmic}[1]
\algstretch
\Require target $\alpha=\alpha_1\cdots\alpha_n\in\bits{n}$ (MSB first), payload $\beta\in\Fp$
\Ensure keys $(k_0,k_1)$ with $\Eval(k_0,x)+\Eval(k_1,x)=\beta\cdot\one[x=\alpha]$
\State sample independent $s_0,s_1\getsr\bits{128}$; $t_0\gets 0$; $t_1\gets 1$
\State save the initial seeds $s_0^{(0)}\gets s_0$, $s_1^{(0)}\gets s_1$
\For{$i=1$ \textbf{to} $n$}
    \State $a\gets\alpha_i$; \ $\keep\gets a$; \ $\lose\gets 1-a$ \Comment{$L=0$, $R=1$}
    \State $(s_b^L,t_b^L,s_b^R,t_b^R)\gets\PRG(s_b)$ for $b\in\{0,1\}$
    \State $\sCW\gets s_0^{\lose}\oplus s_1^{\lose}$
    \State $\tCW{L}\gets t_0^L\oplus t_1^L\oplus a\oplus 1$; \ $\tCW{R}\gets t_0^R\oplus t_1^R\oplus a$
    \LineComment{both $b$, with the \emph{old} $t_b$; $\cdot$ is a conditional XOR}
    \State $(s_b,t_b)\gets\bigl(s_b^{\keep}\oplus t_b\cdot\sCW,\ t_b^{\keep}\oplus t_b\cdot\tCW{\keep}\bigr)$
    \State $\CW^{(i)}\gets(\sCW,\tCW{L},\tCW{R})$
\EndFor
\State $u_b\gets\Conv(s_b)$ for $b\in\{0,1\}$
\State $\CWout\gets(-1)^{t_1}\,(\beta-u_0+u_1)$
\LineComment{keys hold the initial roots, never the final states}
\State $k_b\gets\bigl(s_b^{(0)},\,b,\,\CW^{(1)},\ldots,\CW^{(n)},\,\CWout\bigr)$ for $b\in\{0,1\}$
\State \Return $(k_0,k_1)$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Exact DPF evaluation ($\DPF.\Eval$, $\DPF.\EvalAll$)}
\label{alg:eval}
\begin{algorithmic}[1]
\algstretch
\Require role $b$, key $k_b=(s_b^{(0)},b,\CW^{(1)},\ldots,\CW^{(n)},\CWout)$, query $x=x_1\cdots x_n$
\Ensure share $y_b\in\Fp$ (or all $2^n$ leaf shares for $\EvalAll$)
\Function{Eval}{$k_b,x$}
    \State $(s,t)\gets(s_b^{(0)},b)$ \Comment{root control bit $=$ role}
    \For{$i=1$ \textbf{to} $n$} \Comment{$\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$}
        \State $(s^L,t^L,s^R,t^R)\gets\PRG(s)$ \Comment{$t$: old evaluator bit}
        \State $(s^L,t^L)\gets(s^L\oplus t\cdot\sCW,\ t^L\oplus t\cdot\tCW{L})$
        \State $(s^R,t^R)\gets(s^R\oplus t\cdot\sCW,\ t^R\oplus t\cdot\tCW{R})$
        \State $(s,t)\gets(s^{L},t^{L})$ if $x_i=0$, else $(s^{R},t^{R})$
    \EndFor
    \State \Return $y_b\gets(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$
\EndFunction
\Function{EvalAll}{$k_b$}
    \State push $(s_b^{(0)},b,0,\langle\rangle)$ onto the stack \Comment{$\langle\rangle$: empty prefix}
    \While{the stack is not empty}
        \State pop $(s,t,i,\pi)$ \Comment{seed, bit, depth, prefix}
        \If{$i=n$}
            \State emit leaf $\pi$ with share $(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$
        \Else
            \State expand $s$ as in lines 4--6 with $\CW^{(i+1)}$
            \State push $(s^R,t^R,i{+}1,\pi\|1)$
            \State push $(s^L,t^L,i{+}1,\pi\|0)$ \Comment{left first}
        \EndIf
    \EndWhile
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_gac.pdf}
    \caption{Malicious-safe generate-and-consume inside module $T_b$ for a depth-2 tree. (a)~Joint generation: the two generator states $(s_0,t_0)$ and $(s_1,t_1)$ follow the target path $\alpha=01$ and emit $\CW^{(1)}$, $\CW^{(2)}$ and $\CWout$, which are consumed immediately instead of being stored as a key. (b)~Local evaluation of party $b$ on query $x=00$: a separate evaluator state $(\tilde s,\tilde t)$ follows $x$, applies each correction word at its own level, and leaves the target path at level~2, where only its own control bit $\tilde t$ is correct; grey nodes are never expanded. (c)~Leaf epilogue: the raw share $\tilde y_b$ is freshly reshared and authenticated with joint pads $\zeta,\kappa_1,\kappa_2,\kappa_3$ into the 32~B tuple $\authb{y}{b}$. The crossed-out inset is the tag-tree alternative, which needs $t=3$ extra DPF trees with payloads $\Delta_j\beta$ and four times the PRG work.}
    \label{fig:gac}
\end{figure*}

\textbf{High-level idea.}
\Cref{fig:gac}(a) shows $\Gen$ walking two states $(s_0,t_0)$ and $(s_1,t_1)$ down the target path. Since each state applies a correction only when its \emph{own} old control bit is set, exactly one of the two is corrected at each level; the corrections make the off-path states of both parties identical, so their signed outputs cancel, while $\CWout$ programs $\beta$ at the target leaf (\cref{thm:dpf-correct}). Correctness needs neither uniform targets nor computational hardness; uniform masks belong to the application protocol (\cref{sec:proto-refactor}).

\textbf{Explicit states.}
Three details that the simplified semi-honest listing~\cite{dfa2026trusted} leaves implicit are explicit in \cref{alg:gen,alg:eval}, because the malicious analysis depends on them. First, the root control bits are fixed by role, $t_0=0$ and $t_1=1$, rather than sampled, and the evaluator of party $b$ always starts from $(s_b^{(0)},b)$. Second, a key contains the \emph{initial} seed of its party, the correction words and $\CWout$; the generator's final states are never substituted for the roots. Third, the payload and the role enter only through $\CWout$ and the output sign $(-1)^b$, so both are bound inputs of the ledgered gate descriptor (\cref{sec:proto-ledger}) rather than host-supplied parameters.

\textbf{Generator versus evaluator state.}
Lines 5--6 of \cref{alg:eval} correct both children with the evaluator's own old control bit $t$. Along the target path this bit coincides with the generator's $t_b$, which invites reusing the generator's control register during generate-and-consume. The substitution is wrong as soon as the query leaves the path (level~2 in \cref{fig:gac}(b)): there the evaluator states of the two parties are identical and must apply identical corrections, whereas the generator bits $t_0$ and $t_1$ still differ, so one party would apply a correction that the other omits, and the off-path outputs would no longer cancel. Each module therefore keeps a separate evaluator state next to its two generator states (\cref{alg:gac}).

% ======================================================================
\subsection{Work Accounting}
\label{sec:analysis-work}

\begin{table*}[t]
\centering
\caption{Analytic Cost of One Single-Path DPF Gate of Depth $n$ with $t$ MAC Lanes}
\label{tab:gatecost}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llccccccc}
\hline
\textbf{Design} & \textbf{Security} & \makecell{\textbf{PRG exp.}\\\textbf{per gate}} & \makecell{\textbf{Field ops per}\\\textbf{output, party}} & \makecell{\textbf{Offline bytes}\\\textbf{per gate}} & \makecell{\textbf{Bytes into GPU}\\\textbf{per party}} & \makecell{\textbf{Extra}\\\textbf{rounds}} & \makecell{\textbf{Auth.}\\\textbf{output}} & \makecell{\textbf{Verifies}\\\textbf{evaluation}} \\
\hline
Dealer-based FSS~\cite{gupta2023sigma,jawalkar2024orca} & SH & $4n$ & 0 & $2|k|$ & $|k|$ & 0 & \xmark & \xmark \\
Trusted DFA, GaC~\cite{dfa2026trusted} & SH & $6n$ & 0 & 0 & 8 & 0 & \xmark & \xmark \\
\makecell[l]{Dealer-based FSS, tag trees\\(counting bound)} & Mal. & $4n(1+t)$ & 0 & $2(1+t)|k|$ & $(1+t)|k|$ & 1 per batch & \cmark & \cmark\ (at opening) \\
vFSS-verified keys~\cite{decastro2022vfss} & Mal.\ key gen. & $4n$ + sketch & 0 & $2|k|+O(\lambda)$ & $|k|+O(\lambda)$ & 1 (sketch) & \xmark & \xmark\ (keys only) \\
Vector-payload tree, $t$ lanes$^{\dagger}$ & Mal. & $6n+O(t)$ & $t$ adds & 0 & 32 & 1 per batch & \cmark & \cmark \\
\sys, GaC + epilogue & Mal. & $6n$ & \makecell{3 mult.\\+ 4 pads} & 0 & 32 & 1 per batch & \cmark & \cmark \\
\hline
\end{tabular}

\vspace{3pt}
\parbox{\textwidth}{\footnotesize SH: semi-honest; Mal.: malicious. $|k|$ is the byte length of one party's key. PRG expansions are summed over all parties, dealer included. Bytes into the GPU are keys loaded by a GPU evaluator or output shares delivered by a module. Mask shares and Beaver triples of the surrounding arithmetic are omitted; with authentication, each such element costs 32~B per party instead of 8~B. Rounds are counted relative to the plain masked opening that every design performs. The evaluated dealer-based malicious FSS baseline assumes \est{2.2$\times$} the semi-honest offline bytes (\cref{app:model}), below this counting bound. $^{\dagger}$One in-module tree with payload $(\beta,\Delta_1\beta,\ldots,\Delta_t\beta)$; $O(t)$ counts extra leaf-conversion blocks.}
\end{table*}

\Cref{tab:gatecost} compares one single-path DPF gate at six design points. With 128-bit seeds, one party's key holds its root seed, $n$ correction words of $128+2$ bits and $\CWout$ as one canonical 64-bit word (the root control bit is the public role), so $|k|=\lceil(128+130n+64)/8\rceil$ bytes, or 1{,}016~B for $n=61$.

\textbf{Design-point comparison.}
Trusted DFA trades $1.5\times$ the dealer's PRG work for zero key bytes: each module expands $2n$ generator states and $n$ evaluator states for its own party, so the two modules perform $6n$ expansions where a dealer and two evaluators perform $4n$. Tag trees multiply PRG work, key bytes and key I/O by $1+t$, and verified keys authenticate neither the output nor its evaluation. \sys keeps DFA's $6n$ expansions and zero key bytes and adds only three field multiplications and four pads per output and party; it cannot avoid the 32~B authenticated tuple and the check round.

\textbf{Effect of the epilogue.}
Because the epilogue (\cref{fig:gac}(c)) leaves the per-gate PRG expansion count unchanged, the estimated single-path throughput of the DPF engine drops only from \est{113} to \est{106~M~gates/s} at $n=61$ relative to semi-honest trusted DFA, whereas per-lane tag trees fall to \est{26.7~M~gates/s}; the gap to per-lane tag trees stays at \est{3.8--4.0$\times$} for $n$ between 8 and 61 (\cref{fig:dpfthr}). The drop comes mainly from the assumed pipeline efficiency (\est{0.85} vs.\ \est{0.90}; \cref{app:model}); the two extra pad blocks ($6n{+}3$ vs.\ $6n{+}1$ AES blocks per gate) cost only 0.5\%. The vector-payload tree nearly matches the epilogue's PRG count, but it widens every output correction by $t$ field elements, covers only results linear in DPF evaluations, and exports pseudorandom tag shares whose hiding rests on DPF key privacy. The epilogue instead makes every exported tuple exactly uniform for its holder (\cref{thm:epilogue}) and applies unchanged to LUT, interval, direct and PIR results.

\textbf{Remaining costs we accept.}
\sys does not remove duplicated generation: $6n$ instead of $4n$ expansions is the price of eliminating $2|k|$ network bytes and $|k|$ bytes of key I/O per gate, a favorable trade because PRG expansion is the cheapest operation in the pipeline while bytes cross its slowest links. Two further costs remain. The conservative $O(n^2)$ DCF of \cref{alg:dcf} is the only DCF our proofs cover; its interval gate costs 22{,}692 AES blocks at $n=61$, against a projected \est{976} for an optimized DCF, so the compiler chooses among direct, LUT and interval gates by modeled cost, subject to an FSS-portability constraint (\cref{sec:proto-direct,sec:eval-micro}). A host-module link of $B$ bytes/s bounds the authenticated output stream at $B/32$ elements/s, which motivates the L2-adjacent placement (\cref{sec:arch-insight}).

\textbf{Implications.}
For sources (iii) and (iv) the semi-honest lesson still holds: distribution is the largest avoidable cost (Observation~1), so DFA's local generation and generate-and-consume must stay, and FSS outputs must be authenticated without multiplying DPF work. This leaves sources (i) and (ii) as the dominant costs (Observations~2 and~3). The analysis yields five design rules that structure the rest of the paper: (1)~authenticate FSS outputs by fresh resharing inside the module, never by extra trees and never by authenticating host values (S2; \cref{sec:proto-epilogue}); (2)~keep generation local and streamed, with separate generator and evaluator states (S7; \cref{sec:proto-gac}); (3)~make the unavoidable check round sound and batchable by freezing bytes before challenges are drawn (S1, S3, S8), and release no output before \lstate{VERIFIED} (S6; \cref{sec:proto-check,sec:proto-ledger}); (4)~bind every randomness draw to one session, gate, role and use, so that local generation does not open a replay path (S4, S5; \cref{sec:proto-ledger}); and (5)~leave four-lane exact linear algebra on the GPU while the module generates correct triples (S7) and verifies openings (\cref{sec:arch-insight}).


==> qa/draft3/sections/05a_protocol.tex <==
% ======================================================================
% Section V (part 1): VIGOR-DFA Protocol Design
% Owner: 05a_protocol.tex. Continues in 05b_protocol_gates.tex.
% ======================================================================
\section{\texorpdfstring{\sys}{VIGOR-DFA} Protocol Design}\label{sec:protocol}

This section specifies the protocol run by the two parties of \ProfT: the flow (\cref{sec:proto-overview}), the representation, joint randomness and lifecycle state (\cref{sec:proto-repr,sec:proto-setup,sec:proto-ledger}), and the mechanisms that move values through the integrity chain (\cref{sec:proto-gac,sec:proto-epilogue,sec:proto-check,sec:proto-arith}). Nonlinear gates, refactoring, GPU verification and PIR follow in \cref{sec:proto-gates,sec:proto-direct,sec:proto-refactor,sec:proto-freivalds,sec:proto-pir}; formal statements are collected in \cref{sec:security}.

% ======================================================================
\subsection{Overview}\label{sec:proto-overview}

\textbf{High-level idea.}
In trusted DFA the protected module replaces the dealer: it samples FSS keys locally and consumes each correction word as soon as it produces it~\cite{dfa2026trusted}. \sys turns the module from a dealer into a dealer that also verifies. Every wire carries an authenticated sharing with $t$ information-theoretic MAC lanes. The GPU performs all linear algebra on these sharings but only ever produces \emph{candidate} shares. Each module generates every correlation of its party, authenticates every FSS output it computes, checks every opening on frozen bytes and releases nothing before verification.

\textbf{Per-gate lifecycle.}
Every gate of the public circuit $C$ fixed by the manifest $\mu$ passes through the same module commands (\cref{tab:commands}). (1)~With \cmd{RESERVE_PREP}, $T_b$ reserves the gate's randomness labels in its one-time ledger and issues party-local authenticated preprocessing (masks, triples) to host~$b$. (2)~Host $b$'s GPU computes candidate authenticated shares with local linear operations. (3)~With \cmd{FREEZE_BATCH} and \cmd{CHECK_OPEN}, the two modules freeze the submitted bytes and verify the masked openings the gate needs. (4)~For a nonlinear gate, \cmd{EVAL_FSS} consumes the verified opening, runs generate-and-consume inside $T_b$ and returns a freshly authenticated share. (5)~\cmd{FINAL_OUTPUT} hands a masked output and a bound certificate to an authorized recipient. A failure in any step triggers \cmd{ABORT}, which poisons the epoch. Each mechanism below enforces one design rule of \cref{sec:analysis-work}; \cref{tab:notation} summarizes the notation.

\begin{table}[t]
\caption{Notation used in the protocol description}
\label{tab:notation}
\centering
\footnotesize
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{p{0.27\linewidth} p{0.63\linewidth}}
\hline
\textbf{Symbol} & \textbf{Meaning} \\
\hline
$P_b$; host $b$; $T_b$ & party $b\in\{0,1\}$; its untrusted host (CPU, OS, driver, GPU, memory, NIC); its protected module \\
$\mu$, $C$ & public manifest and the finite circuit it fixes \\
$p$, $\Fp$ & Mersenne prime $2^{61}-1$ and the protocol field \\
$t$ & number of MAC lanes ($t=3$) \\
$\Delta_j$; $\Delta_{b,j}$ & global MAC key of lane $j$ (modules only); host $b$'s additive share of it \\
$\auth{x}$; $\authb{x}{b}$ & authenticated sharing of $x$; party $b$'s tuple $(x_b,\gamma_{b,1},\dots,\gamma_{b,t})$ \\
$\gamma_{b,j}$ & tag share of party $b$ in lane $j$, $\gamma_{0,j}+\gamma_{1,j}=\Delta_j x$ \\
$K$ & session key shared by $T_0$ and $T_1$ after setup \\
$\ell$ & length-prefixed label (session, epoch, gate, purpose, logical draw, block) \\
$\PRF_K(\ell,\cdot)$ & joint draw: same label, same value in both modules \\
$\nu$; $\varepsilon$; $\upsilon$ & wire index; masked input difference $x-r$; masked output $y+o$ \\
$\mathsf{In}_\nu$; $\mathcal{V}$ & declared interface of input wire $\nu$; validity predicates of $\mu$ \\
$n$; $\lambda$ & DPF input length in bits; PRG seed length ($\lambda=128$) \\
$\alpha$, $\beta$, $x$ & DPF target, payload in $\Fp$, verified public query \\
$\CW^{(i)}$; $\CWout$ & level-$i$ correction word; output correction \\
$(s_c,t_c)$; $(\tilde s,\tilde t)$ & generator state of root $c\in\{0,1\}$; evaluator state of $T_b$ \\
$\tilde y_b$ & raw local output of the protected evaluator \\
$\zeta$; $\kappa_j$ & fresh common epilogue pads for the value; for lane $j$ \\
$m$; $h_b$; $\mathit{cid}$ & batch size; frozen root of $T_b$; check identifier \\
$\rho_{j,i}$; $\sigma_{b,j}$ & challenge of lane $j$ at batch position $i$; residual of $T_b$ in lane $j$ \\
$\bm{e}$; $\bm{d}_j$ & value-error vector; tag-error vector of lane $j$ in a checked batch \\
$Q$ & number of checked batches in one execution \\
$w$ & LUT input width (\cref{sec:proto-gates}) \\
\hline
\end{tabular}
\end{table}

% ======================================================================
\subsection{Authenticated Representation}\label{sec:proto-repr}

\textbf{Field and MAC lanes.}
All protocol arithmetic is over $\Fp$ with the Mersenne prime $p=2^{61}-1$. The modules hold $t=3$ independent global MAC keys $\Delta_1,\Delta_2,\Delta_3\getsr\Fp$, each additively split as $\Delta_j=\Delta_{0,j}+\Delta_{1,j}$; host~$b$ holds only $\Delta_{b,j}$, which it needs to add public values to its tags. Party $b$ holds an authenticated value $\auth{x}$ as
\begin{gather*}
\authb{x}{b}=(x_b,\gamma_{b,1},\gamma_{b,2},\gamma_{b,3}),\\
x_0+x_1=x,\qquad \gamma_{0,j}+\gamma_{1,j}=\Delta_j x\quad (j\in[t]),
\end{gather*}
which is the SPDZ representation~\cite{damgard2012spdz,damgard2013practical} with three independent lanes. A canonical wire occupies four 64-bit words, i.e., 32~B per party before metadata. Every element is encoded as an unsigned 64-bit integer smaller than $p$; the module parser rejects noncanonical encodings instead of reducing arbitrary integers modulo $p$, which keeps frozen bytes and checked field elements in one-to-one correspondence.

\textbf{Why three lanes over a 61-bit field.}
The Mersenne modulus lets the GPU compute exact products of canonical elements with native 64-bit multiplies and two folding steps (\cref{sec:arch-field}), so all $1+t$ lanes of authenticated linear algebra stay on standard integer datapaths. A single 61-bit tag is too weak: for $Q\le 2^{32}$ checked batches, $t=3$ is the smallest lane count whose statistical term $Q(2/p)^t$ falls below $2^{-128}$ (\cref{sec:sec-concrete}, \cref{tab:lanes}), and every lane is paid for in GPU work (\cref{sec:eval-ablation}).

\textbf{Why a field and not $\Z_{2^{64}}$.}
The soundness proof divides by a nonzero error coordinate and therefore needs a field (\cref{sec:sec-concrete}, \cref{app:proof-auth}). The encoding is thus not bit-identical to the $\Z_{2^{64}}$ arithmetic of FSS-compiled models~\cite{gupta2023sigma,jawalkar2024orca}. \sys fixes the numeric contract in the manifest (fixed-point scale, signed encoding, exact toward-zero truncation of \cref{sec:proto-gates}, magnitudes below $p/2$); a deployment that needs ring semantics must use a SPDZ2k-type backend~\cite{cramer2018spdz2k} with its own proof.

% ======================================================================
\subsection{Session Setup and Joint Randomness}\label{sec:proto-setup}

\textbf{Session setup.}
Each module authenticates its peer's identity, code and configuration measurement, role and freshness contribution. An authenticated key establishment then binds the ordered pair of identities, the roles 0 and 1, a fresh session identifier, the epoch, the manifest hash $\Hash(\mu)$, the field and tag parameters and the protocol version, and yields the session key $K$ known only to $T_0$ and $T_1$. Any failure aborts. We treat this step as an explicit setup assumption with error $\eps{setup}$ (\cref{thm:main}) and propose no new attestation protocol; attestation certifies what runs inside a module, not what the GPU computes (\cref{sec:bg-dfa}).

\textbf{Labels and joint draws.}
All module randomness is derived as $\PRF_K(\ell)$, or with an equivalent key derivation function (KDF)~\cite{krawczyk2010hkdf}, where $\ell$ is an unambiguous, length-prefixed encoding of $(\mathsf{session},\mathsf{epoch},\mathsf{gate},\mathsf{purpose},\mathsf{logical\_draw},\mathsf{block})$. A \emph{logical joint draw} uses the same label in both modules and thus yields the same value in $T_0$ and $T_1$ without communication; this is how both modules obtain identical DPF roots, correction words, masks, triples, pads and challenges. Distinct roots, pads, triple components, challenge lanes and rejection-sampling retries receive distinct labels. Two rules are easy to get wrong. The local role must \emph{not} be appended to a joint draw, since $T_0$ and $T_1$ would then generate two unrelated DPF instances whose outputs no longer add up; and the logical root-0 and root-1 draws of one DPF \emph{must} be different draws. Since labels name session, epoch and gate, the ledger detects replayed or misrouted material (S4, S5). A uniform element of $\Fp$ is obtained by rejection sampling: take 61 pseudorandom bits and reject the single value $p$, which occurs with probability $2^{-61}$; a bounded implementation aborts when its retry budget is exhausted instead of introducing a silent bias.

\textbf{Authenticated correlations.}
To share a protected value $v$, the joint sampler runs \AuthShare{}: it samples $v_0\getsr\Fp$ and sets $v_1=v-v_0$, independently samples $\gamma_{0,j}\getsr\Fp$ and sets $\gamma_{1,j}=\Delta_j v-\gamma_{0,j}$ for $j\in[t]$, and gives party $b$ only its tuple $\authb{v}{b}$. A multiplication triple samples $a,b\getsr\Fp$, computes $c=ab$ \emph{correctly inside the protected boundary} and authenticates all three values independently (S7); a matrix triple satisfies the actual equality $C=AB$ for its declared dimensions. Because both modules derive the same correlations from joint labels, preprocessing crosses no network link.

% ======================================================================
\subsection{One-Time Ledger and Release Guard}\label{sec:proto-ledger}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_ledger.pdf}
    \caption{Per-gate lifecycle enforced by the one-time ledger of $T_b$. Solid arrows are the only permitted transitions, each triggered by the named module command (\cref{tab:commands}). An accepted \cmd{CHECK_OPEN} only sets \lstate{VERIFIED}; \cmd{EVAL_FSS} consumes the opening of an FSS or direct gate, and an output gate, which runs no \cmd{EVAL_FSS}, is moved by \cmd{FINAL_OUTPUT} through \lstate{CONSUMED} to \lstate{RELEASED}. Any other transition or any failed check moves the gate to \lstate{ABORTED}, poisons the epoch and keeps the release guard closed.}
    \label{fig:ledger}
\end{figure}

\textbf{Ledger states.}
Each module keeps an authoritative protected ledger that binds every gate to its operation, predecessor and output wires, numeric type, table or model hash, public dimensions and allowed command sequence. A gate transaction moves only along
\lstate{NEW} $\rightarrow$ \lstate{RESERVED} $\rightarrow$ \lstate{PREPARED} $\rightarrow$ \lstate{FROZEN} $\rightarrow$ \lstate{VERIFIED} $\rightarrow$ \lstate{CONSUMED} $\rightarrow$ \lstate{RELEASED}
(\cref{fig:ledger}). Reservation burns the gate's randomness identifiers \emph{before} any preprocessing share is issued, so no label is ever issued twice. \lstate{PREPARED} lets the module issue the authorized party-local preprocessing exactly once; it is not permission to release an unchecked result. \lstate{CONSUMED} records the one-time use of verified openings and preprocessing, and \lstate{RELEASED} records that the result left the module under a certificate. Any invalid transition or failed check moves the gate to \lstate{ABORTED} and poisons the whole epoch: outstanding output responses are gated, no new challenge is derived, and aborted reservations never return to a free list.

\textbf{Freeze semantics.}
Before any checking challenge is drawn, $T_b$ copies the exact submitted value and tag bytes into protected storage, or spills them into AEAD-protected immutable pages~\cite{dworkin2007gcm} bound to sequence numbers, exact lengths, gate identifiers and a protected root. It hashes the complete descriptor and these bytes into a frozen root $h_b$, and the two modules agree on the ordered pair $(h_0,h_1)$. A host's claim that ``this buffer has hash $h$'' is not a freeze, and neither is DMA completion. After challenge generation, $T_b$ rereads only authenticated frozen pages and never verifies one buffer but consumes a later, host-modified one. This closes the time-of-check-to-time-of-use window (S3) that exists whenever checked data live in host or GPU memory.

\textbf{Release certificates and the guard.}
A release certificate binds the session, epoch, gate, recipients, output encoding or hash and terminal status. A missing peer acknowledgement can cause an abort, but it never authorizes output under a different transcript. The release guard is a small state machine in front of the module's output path (\cref{sec:arch-hw}); its enabling inputs originate from the protected checkers and the ledger, never from host-writable registers, so a host cannot open it by writing a status bit (S6). Resetting the guard is not a secure session reset.

\textbf{Reboot and rollback.}
After a reboot, either a separately justified trusted monotonic service preserves freshness~\cite{parno2011memoir,matetic2017rote}, or the old master key is irrecoverably erased and a freshly attested session is required. A host-controlled counter file is not anti-rollback protection, because the host can restore an old copy and replay old masks (S4).

% ======================================================================
\subsection{Malicious Generate-and-Consume}\label{sec:proto-gac}

\textbf{From semi-honest to malicious GaC.}
\Cref{alg:gac} interleaves \cref{alg:gen,alg:eval} with the three separate states of \cref{sec:analysis-dpf}: two generator states on the target path, started from $t_0=0$ and $t_1=1$, and an evaluator state on the query path, started from its own root seed and the fixed control bit $b$, never from a later generator state. Each correction word is computed from the expanded children of the two generator seeds and the target bit $\alpha_i$, applied to the generator states under their old bits $t_c$ and to both evaluator children under the evaluator's old bit $\tilde t$, and erased only after that use; $t\cdot s$ denotes a conditional XOR. The hardware keeps the two state sets in distinct contexts (\cref{sec:arch-pipe}), and the per-level work, which still duplicates generation in both modules, is accounted in \cref{tab:gatecost}.

\textbf{Inputs and outputs.}
The query $x$ is read from a verified masked opening of the same gate, never from unchecked host data: for instance the opened $c$ of an interval gate, whose prefix DPFs are queried at $c$ (\cref{alg:interval,alg:dcf}), whereas in a LUT gate the opened $u$ only permutes the table index while $\EvalAll$ visits every $a$ (\cref{alg:lut}). The target $\alpha$ and payload $\beta$ come from the gate's protected preprocessing record, so they are joint draws or joint functions of joint draws (\cref{sec:proto-refactor}). By \cref{thm:dpf-correct,thm:gac}, the raw outputs satisfy $\tilde y_0+\tilde y_1=\beta\cdot\one[x=\alpha]$, but $\tilde y_b$ never leaves the module: the epilogue lines of \cref{alg:gac} replace it with a freshly authenticated tuple. Since neither keys nor raw shares are exported, \cref{thm:main} needs no DPF key-privacy term. Gates that combine several DPF evaluations (interval prefixes, LUT and PIR scans) run only the (Gen) and (Eval) lines per constituent DPF and apply the ledger lines and one epilogue to their combined raw share, for PIR only its value pad (\cref{app:proof-dpf}). For full-domain uses such as LUT gates and PIR, the evaluator lines become the depth-first $\EvalAll$ traversal of \cref{alg:eval}; each $\CW^{(i)}$ then stays in protected registers until its last evaluator use, which costs $O(n)$ words and is covered by the same node-by-node coupling.

\begin{algorithm}[t]
\algstretch
\small
\caption{Malicious generate-and-consume with fresh authentication (\algname{GaC-Auth}) inside $T_b$}
\label{alg:gac}
\begin{algorithmic}[1]
\Require role $b\in\{0,1\}$; gate label $\ell$; public query $x\in\bits{n}$ from the gate's frozen, verified opening; target $\alpha\in\bits{n}$ and payload $\beta\in\Fp$ from the protected record of $\ell$; session key $K$; global keys $\Delta_1,\dots,\Delta_t$
\Ensure $\authb{y}{b}=(y_b,\gamma_{b,1},\dots,\gamma_{b,t})$ with $y_0+y_1=\beta\cdot\one[x=\alpha]$ and $\gamma_{0,j}+\gamma_{1,j}=\Delta_j(y_0+y_1)$
\If{gate $\ell$ is not \lstate{VERIFIED} in the ledger}
  \State \Abort{} and poison the epoch
\EndIf
\LineComment{Joint draws: identical labels in $T_0$ and $T_1$, no role appended}
\State $s_0\gets\PRF_K(\ell,\mathsf{root}_0)$;\ $s_1\gets\PRF_K(\ell,\mathsf{root}_1)$;\ $t_0\gets 0$;\ $t_1\gets 1$
\State $(\tilde s,\tilde t)\gets(s_b,b)$ \Comment{separate evaluator}
\For{$i=1$ \textbf{to} $n$}
  \LineComment{(Gen) both roots on the target path; updates use the old $t_c$}
  \State $(s_c^L,t_c^L,s_c^R,t_c^R)\gets\PRG(s_c)$ for $c\in\{0,1\}$
  \State $a\gets\alpha_i$;\ $\keep\gets a$;\ $\lose\gets 1-a$ \Comment{$L\equiv 0$, $R\equiv 1$}
  \State $\sCW\gets s_0^{\lose}\oplus s_1^{\lose}$
  \State $\tCW{L}\gets t_0^L\oplus t_1^L\oplus a\oplus 1$;\ \ $\tCW{R}\gets t_0^R\oplus t_1^R\oplus a$
  \State $(s_c,t_c)\gets\big(s_c^{\keep}\oplus t_c\cdot\sCW,\ t_c^{\keep}\oplus t_c\cdot\tCW{\keep}\big)$, $c\in\{0,1\}$
  \LineComment{(Eval) own query path; corrections use the old $\tilde t$}
  \State $(\hat s^L,\hat t^L,\hat s^R,\hat t^R)\gets\PRG(\tilde s)$
  \State $(\hat s^L,\hat t^L)\gets\big(\hat s^L\oplus\tilde t\cdot\sCW,\ \hat t^L\oplus\tilde t\cdot\tCW{L}\big)$
  \State $(\hat s^R,\hat t^R)\gets\big(\hat s^R\oplus\tilde t\cdot\sCW,\ \hat t^R\oplus\tilde t\cdot\tCW{R}\big)$
  \State $(\tilde s,\tilde t)\gets(\hat s^{x_i},\hat t^{x_i})$
  \State erase $\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$ \Comment{after its evaluator use}
\EndFor
\LineComment{(Gen) output correction from the final generator states}
\State $u_c\gets\Conv(s_c)$ for $c\in\{0,1\}$;\ \ $\CWout\gets(-1)^{t_1}(\beta-u_0+u_1)$
\LineComment{(Eval) raw share, never exported}
\State $\tilde y_b\gets(-1)^b\big(\Conv(\tilde s)+\tilde t\cdot\CWout\big)$; erase $s_c$, $t_c$, $\CWout$
\LineComment{(Epilogue) fresh uniform pads, distinct labels per output wire}
\State $\zeta\gets\PRF_K(\ell,\mathsf{pad}_0)$;\ \ $\kappa_j\gets\PRF_K(\ell,\mathsf{pad}_j)$ for $j\in[t]$
\State $y_b\gets\tilde y_b+(-1)^b\zeta$
\State $\gamma_{b,j}\gets\Delta_j\,y_b+(-1)^b\kappa_j$ for $j\in[t]$
\State mark $\ell$ \lstate{CONSUMED}; erase $\tilde y_b$, $\zeta$, $\kappa_1,\dots,\kappa_t$, $(\tilde s,\tilde t)$
\State \Return $\authb{y}{b}$ to the output FIFO behind the release guard
\end{algorithmic}
\end{algorithm}

% ======================================================================
\subsection{Fresh Authentication Epilogue}\label{sec:proto-epilogue}

\textbf{Construction.}
Let $\tilde y_0,\tilde y_1$ be raw local shares computed inside the two protected evaluators, with $\tilde y_0+\tilde y_1$ equal to the intended gate value. Both modules derive fresh common pads $\zeta,\kappa_1,\dots,\kappa_t\getsr\Fp$ from joint labels that are distinct for every output wire, and $T_b$ returns
\begin{equation*}
y_b=\tilde y_b+(-1)^b\zeta,\qquad \gamma_{b,j}=\Delta_j\,y_b+(-1)^b\kappa_j\quad (j\in[t]).
\end{equation*}
The pads cancel in $y_0+y_1$ and in $\gamma_{0,j}+\gamma_{1,j}=\Delta_j(y_0+y_1)$, so the result is an authenticated sharing of $\tilde y_0+\tilde y_1$, and each party's tuple is uniform on $\Fp^{1+t}$ whatever the gate value and the global keys (\cref{thm:epilogue}). Fresh pads make this hold jointly across outputs; correlations created by later arithmetic are handled by the circuit simulation of \cref{thm:main}.

\textbf{Why it replaces tag trees.}
Instead of $t$ further DPF trees with payloads $\Delta_j\beta$, the epilogue exploits the linearity of the MAC. Because $T_b$ knows the global $\Delta_j$, the tag of the reconstructed value is the sum of the per-party products $\Delta_j y_b$; the pad $\kappa_j$ hides $\Delta_j y_b$ from host $b$, which knows $y_b$ and could otherwise divide it out. The pad $\zeta$ rerandomizes the raw DPF share, so no host ever sees $\tilde y_b$. The cost is one raw DPF computation, three field multiplications and four fresh pads per party and output, and the output is a 32~B tuple.

\textbf{API restriction.}
The epilogue accepts only results computed inside the module, namely the DPF, DCF, LUT, interval and direct gates of \cref{sec:proto-gates,sec:proto-direct} and the PIR reductions of \cref{sec:proto-pir}, or results from an explicitly verified backend such as the frozen-operand Freivalds check of \cref{sec:proto-freivalds}. There is no \cmd{authenticate(host_value)} entry point. With one, the module would become a MAC oracle: a malicious host could obtain valid tags on any value it wishes to open, and \CheckOpen{} would accept the forgery with probability one (S2). Since the trusted boundary excludes the GPU SMs and memory, a malicious-secure extension must never compute an unchecked result on the GPU and ask the module to authenticate it.

% ======================================================================
\subsection{Freeze-Before-Challenge CheckOpen}\label{sec:proto-check}

\begin{algorithm}[t]
\algstretch
\small
\caption{Freeze-before-challenge authenticated opening (\CheckOpen) inside $T_b$}
\label{alg:checkopen}
\begin{algorithmic}[1]
\Require descriptor and nonempty ordered list of expected wires $(\nu_i)_{i\in[m]}$; host $b$'s tuples $(x_{b,i},\gamma_{b,j,i})_{i\in[m],\,j\in[t]}$; key shares $(\Delta_{b,j})_{j\in[t]}$ from the protected key store of $T_b$ (never from host input)
\Ensure verified openings $(z_i)_{i\in[m]}$ with bound certificates, or \Abort
\If{metadata, field encoding, gate order or length mismatch the ledger}
  \State \Abort{} and poison the epoch
\EndIf
\LineComment{Step 1: freeze, then agree on both roots}
\State copy the exact bytes into protected SRAM or sealed AEAD pages; $h_b\gets\Hash(\text{descriptor},\text{frozen bytes})$; mark \lstate{FROZEN}
\State exchange $(h_b,\mathit{cid})$ with $T_{1-b}$; \Abort{} unless both hold the same $(h_0,h_1)$ and $\mathit{cid}$
\LineComment{Step 2: reconstruct candidates inside the modules}
\State exchange the frozen value shares $(x_{b,i})_{i\in[m]}$ with $T_{1-b}$
\State $z_i\gets x_{0,i}+x_{1,i}$ for $i\in[m]$ \Comment{not exposed to the host}
\LineComment{Step 3: internal challenges, only after both freezes}
\State $\rho_{j,i}\gets\PRF_K(\mathsf{chk},h_0,h_1,\mathit{cid},j,i)$ for $j\in[t]$, $i\in[m]$
\LineComment{Step 4: per-lane residuals from frozen pages only}
\State $\sigma_{b,j}\gets\sum_{i=1}^{m}\rho_{j,i}\,(\gamma_{b,j,i}-\Delta_{b,j}z_i)$ for $j\in[t]$
\State exchange $(\sigma_{b,j})_{j\in[t]}$ with $T_{1-b}$
\LineComment{Step 5: decide and release}
\If{$\sigma_{0,j}+\sigma_{1,j}=0$ for every $j\in[t]$}
  \State agree on output digest and status; mark \lstate{VERIFIED}; record the checked material as used
  \State \Return $(z_i)_{i\in[m]}$ with certificates bound to session, epoch, gates and output hash
\Else
  \State release no candidate value; poison the epoch; return one generic failure status
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_checkopen.pdf}
    \caption{Freeze-before-challenge \CheckOpen{} between the two modules. Challenges $\rho_{j,i}$ are derived only after both frozen roots are agreed, and $T_b$ rereads only its frozen pages, so a host that overwrites its DMA buffer after the freeze changes nothing that is checked or consumed.}
    \label{fig:checkopen}
\end{figure}

\textbf{Role.}
Openings are the only places where a value produced by the untrusted GPU becomes public or feeds a protected gate: the masked differences of every multiplication, the masked inputs of every FSS gate and the masked outputs. \CheckOpen{} (\cref{alg:checkopen}, \cref{fig:checkopen}) is a SPDZ-style batched MAC check~\cite{damgard2012spdz,damgard2013practical} rebuilt for a verifier that reads its inputs from untrusted memory (S1, S3). All peer messages use the protected channel, and only an accepted batch releases $z$ with bound certificates.

\textbf{Independent challenge lanes.}
Let $\bm{e}$ be the value-error vector of a batch and $\bm{d}_j$ its tag-error vector in lane $j$, i.e., the differences between the submitted and the prescribed tuples. The freeze fixes $(\bm{e},\bm{d}_j)$ before any $\rho_{j,i}$ exists, so a host cannot place its errors in the kernel of a challenge (\cref{app:proof-auth}). Each lane has its own challenge vector $\bm{\rho}_j$. The complete residual of lane $j$ is $\inner{\bm{\rho}_j}{\bm{d}_j-\Delta_j\bm{e}}$, which for $\bm{e}\neq\bm{0}$ vanishes with probability below $2/p$; independence across lanes multiplies these bounds to $(2/p)^t$ (\cref{thm:mac-sound}). A shared vector collapses the product to one lane, and tag-only errors escape with probability $1/p$ without changing an opened value (\cref{sec:sec-concrete}, \cref{app:proof-auth}).

\textbf{Key hiding and failure handling.}
The bound relies on the hidden-key invariant of \cref{lem:hidden-key}: until the first accepted wrong opening, the honest key shares stay uniform given the corrupt host's view. \CheckOpen{} preserves it in three ways. Candidates, challenges and residuals never leave the modules. The zero tests of all lanes are aggregated into one generic failure status that exposes no residual, challenge, key or data-dependent diagnostic. A failure poisons the epoch and forbids retries with the same material, which rules out an adaptive key-learning sequence within an epoch.

\textbf{Traffic and batching.}
Per batch of $m$ elements, the modules exchange two vectors of $m$ field values and two vectors of $t$ residuals plus authenticated metadata. Tags never cross the peer link, but every local tag must be read by its module, so the host-to-module transfer of 32~B per element can remain the bottleneck (\cref{sec:arch-dse}). Because the value shares are frozen before they are sent, root agreement and value exchange can share one message, and our latency model charges two peer round trips per batch. Only independent openings are batched: a dependent nonlinear gate never consumes an unchecked masked opening, and a checkpoint precedes every input-dependent nonlinear output and every final release, since blindly delayed checking is not justified. Larger batches amortize metadata and round trips but increase staging memory and first-result latency (costs in \cref{sec:eval-check}).

% ======================================================================
\subsection{Inputs, Arithmetic, and Outputs}\label{sec:proto-arith}

\begin{figure*}[t]
\centering
\footnotesize
\setlength{\fboxsep}{4pt}
\fbox{%
\begin{minipage}[t]{0.472\textwidth}
\textbf{Input} $\Pi_{\mathsf{Input}}$\hfill\textit{input $x$ of endpoint $O$ for wire $\nu$}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: reserve label $\ell_\nu$; joint draw $r\getsr\Fp$ and $\authb{r}{b}\gets\AuthShare(r)$; issue $\authb{r}{b}$ to host $b$ once.
\item $T_0,T_1$: send the complete $r$ only to $O$ over its authenticated confidential channel.
\item $O$: send the canonical, authenticated $\varepsilon=x-r$ to $T_0$ and $T_1$.
\item $T_0,T_1$: confirm over the protected channel that both hold the same $\varepsilon$ and bind it to $\nu$; compute $x^*=r+\varepsilon$ and \Abort{} unless $x^*\in\mathsf{In}_\nu$. $T_b$ then hands the bound $\varepsilon$ to host $b$.
\item host $b$: $x_b\gets r_b+\one[b=0]\,\varepsilon$;\ \ $\gamma_{b,j}\gets\gamma_{r,b,j}+\Delta_{b,j}\,\varepsilon$ for $j\in[t]$.
\end{enumerate}
\textit{Extraction:} a corrupt owner's input is $x^*=r+\varepsilon$.
\textit{Validation:} at the public boundaries declared in $\mu$, after every input gate and before the first output opening, $T_0,T_1$ evaluate every predicate of $\mathcal{V}$ on the bound inputs and \Abort{} if one fails.
\textit{Committed inputs:} a protected loader verifies the authorized commitment over the frozen canonical stream, then runs \AuthShare{} on the exactly decoded values.

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Linear} $\Pi_{\mathsf{Lin}}$\hfill\textit{local, on host $b$'s GPU}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $\auth{x}+\auth{y}$: add the value shares and each of the $t$ tag shares.
\item $c\cdot\auth{x}$ for public $c$: multiply the value share and every tag share by $c$.
\item $\auth{x}+c$ for public $c$: $x_0\gets x_0+c$ (party~0 only); $\gamma_{b,j}\gets\gamma_{b,j}+\Delta_{b,j}\,c$ for both $b$ and all $j\in[t]$.
\item Tensors: apply steps 1 to 3 elementwise to the value array and to each of the $t$ tag arrays.
\end{enumerate}

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Output} $\Pi_{\mathsf{Out}}$\hfill\textit{private output $y$ for client $O$}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: joint draw a fresh $\auth{o}$ as in step 1 of $\Pi_{\mathsf{Input}}$; send the complete $o$ only to $O$.
\item host $b$: $\auth{\upsilon}\gets\auth{y}+\auth{o}$ with $\Pi_{\mathsf{Lin}}$.
\item $\upsilon\gets\CheckOpen(\auth{\upsilon})$; the release guard opens only for a \mbox{\lstate{VERIFIED}} batch.
\item $T_b$: send $\upsilon$ and its release certificate (session, epoch, gate, recipients, output hash, status) to $O$.
\item $O$: verify both certificates for the same $\upsilon$ and output $y=\upsilon-o$; otherwise abort.
\end{enumerate}
\textit{Public outputs:} $y\gets\CheckOpen(\auth{y})$.
\textit{Never} hand $O$ both parties' tags: $\gamma_{0,j}+\gamma_{1,j}=\Delta_j y$ with a known $y\neq 0$ reveals $\Delta_j$.
\end{minipage}%
\hspace{0.01\textwidth}\vrule\hspace{0.01\textwidth}%
\begin{minipage}[t]{0.472\textwidth}
\textbf{Multiplication} $\Pi_{\mathsf{Mult}}$\hfill\textit{authenticated Beaver triples}

\textit{Scalar} $\auth{z}=\auth{x}\cdot\auth{y}$:
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: reserve a fresh triple $(\auth{a},\auth{b},\auth{c})$ from joint draws, with $c=ab$ computed inside the protected boundary; issue party $b$'s tuples to host $b$ once.
\item host $b$: $\auth{d}\gets\auth{x}-\auth{a}$ and $\auth{e}\gets\auth{y}-\auth{b}$ with $\Pi_{\mathsf{Lin}}$.
\item $(d,e)\gets\CheckOpen(\auth{d},\auth{e})$, batched with the independent openings of the layer.
\item host $b$: $z_b\gets c_b+d\,b_b+e\,a_b+\one[b=0]\,de$.
\item host $b$: $\gamma_{z,b,j}\gets\gamma_{c,b,j}+d\,\gamma_{b,b,j}+e\,\gamma_{a,b,j}+\Delta_{b,j}\,de$ for $j\in[t]$.
\end{enumerate}
\textit{Matrix} $\auth{Z}=\auth{X}\auth{Y}$ with declared dimensions:
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep,start=6]
\item $T_0,T_1$: reserve $(\auth{A},\auth{B},\auth{C})$ with $C=AB$ computed inside the protected boundary; never expose both $A$ and $B$ to a GPU.
\item $D\gets\CheckOpen(\auth{X}-\auth{A})$;\ \ $E\gets\CheckOpen(\auth{Y}-\auth{B})$.
\item host $b$: $Z_b\gets C_b+D\,B_b+A_b\,E+\one[b=0]\,DE$.
\item host $b$: $\Gamma_{Z,b,j}\gets\Gamma_{C,b,j}+D\,\Gamma_{B,b,j}+\Gamma_{A,b,j}\,E+\Delta_{b,j}\,DE$ for $j\in[t]$, preserving the order of every matrix factor.
\end{enumerate}
\textit{Notation:} in $b_b$ and $\gamma_{b,b,j}$ the first $b$ names the triple's second component and the subscript names the party (implementations use named fields); $\Gamma_{\cdot,b,j}$ is party $b$'s lane-$j$ tag matrix.

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Invariants shared by all four protocols}
\begin{itemize}[leftmargin=1.1em,nosep]
\item Every mask and triple is a one-time joint draw bound to session, epoch, gate and purpose, and is issued only from \mbox{\lstate{PREPARED}} (\cref{fig:ledger}).
\item Every opening is a \CheckOpen{} call on frozen bytes (\cref{alg:checkopen}); no opened value feeds a protected gate or a release before it is \mbox{\lstate{VERIFIED}}.
\item Outputs of host $b$'s GPU are candidate shares; no module ever authenticates them.
\end{itemize}
\end{minipage}}
\caption{Authenticated input, linear, multiplication and output protocols of \sys, written for party $P_b$. Steps labeled $T_0,T_1$ or $T_b$ run inside the protected modules; steps labeled host $b$ run on the untrusted GPU and yield only candidate shares until the next \CheckOpen. With honest messages the protocols realize their operations exactly; otherwise they select an allowed input, preserve the computation or abort, except with the probability bounded in \cref{thm:mac-sound} (\cref{thm:arith}).}
\label{fig:arith}
\end{figure*}

\Cref{fig:arith} specifies the four protocols that carry values between input owners, GPUs, modules and recipients; three points of rationale are not visible in the box.

\textbf{Inputs.}
The difference $\varepsilon$ is uniform for a uniform $r$, so the hosts learn nothing about $x$. Both modules bind one $\varepsilon$, so a corrupt owner cannot feed the two parties different inputs, and its input is extracted as $x^*=r+\varepsilon$ (S9, \cref{def:security}). Canonical encoding alone does not place $x^*$ in the declared interface; since the modules generated $r$, they compute $x^*$ and abort unless $x^*\in\mathsf{In}_\nu$. The validity predicates $\mathcal{V}$ of $\mu$ are evaluated inside the modules at public boundaries that the schedule of $\mu$ places after every input gate and before the first output opening; their accept or abort outcome is the $\mathsf{status}$ component of $\Leak_C$ (\cref{def:leakage}), and the simulator emulates the same abort (\cref{thm:main}). For committed inputs such as preapproved model weights, a host-declared hash does not suffice; the loader hashes exactly the bytes it shares. The modules thus see every input, which \ProfT permits (\cref{sec:threat-model}).

\textbf{Arithmetic.}
Multiplication follows Beaver~\cite{beaver1991efficient} with authenticated triples. An authenticated matrix product costs the GPU $2(1+t)$ plain products plus the public $DE$, which is why authenticated linear algebra, rather than DPF evaluation, dominates the malicious cost (\cref{sec:analysis-cost}).

\textbf{Outputs.}
The recipient accepts $\upsilon$ only with matching certificates from both modules, so integrity toward a client comes from these certificates, never from MAC tags.


==> qa/draft3/sections/05b_protocol_gates.tex <==
% ==================================================================
% Section V (part 2): authenticated nonlinear gates, direct gates and
% compilation, refactoring, verified GPU products, snapshot PIR.
% Continues the Section opened in 05a_protocol.tex (no \section here).
% ==================================================================

\subsection{Authenticated Nonlinear Gates}\label{sec:proto-gates}

Nonlinear layers of FSS-compiled models reduce to lookups in small public tables and piecewise functions selected by interval tests~\cite{boyle2021function,gupta2023sigma,jawalkar2024orca}. In the semi-honest DFA design, both parties evaluate a DPF or DCF key on a masked input and pass the raw output shares onward~\cite{dfa2026trusted}. A malicious host can shift the masked input before it selects the DPF path, and it can modify the raw outputs, which carry no MAC. \sys closes both gaps with one template (\cref{fig:gates}): (1)~mask the authenticated input with joint protected randomness (\cref{sec:proto-setup}); (2)~open the masked value with \CheckOpen{} (\cref{alg:checkopen}), so the value that selects the path is verified and frozen; (3)~evaluate the FSS gate inside $T_b$ with the (Gen) and (Eval) steps of generate-and-consume (\cref{alg:gac}); and (4)~authenticate and reshare the gate's combined raw share with one epilogue (\cref{sec:proto-epilogue}). The host sees only a uniform masked opening and fresh authenticated tuples, and no host-supplied value is ever authenticated, which defeats scenario S2 (\cref{tab:scenarios}).

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_gates.pdf}
    \caption{Authenticated nonlinear gates in \sys. (a)~Small XOR-masked LUT (\cref{alg:lut}): the XOR-masked bit vector $u$ is opened by \CheckOpen{} and $T_b$ scans the full public domain in a fixed order. (b)~Shifted-interval indicator and Horner polynomial (\cref{alg:interval}): one field opening $c=x+r$ serves both translated thresholds $L$ and $H$, which derive from the same mask. (c)~Direct protected gate (\cref{sec:proto-direct}): the module recovers $x=c-r$ inside its boundary and returns a fresh sharing of $g(x)$. In all three cases the host submits only authenticated shares and receives only freshly authenticated outputs; raw FSS shares, DPF keys and, in (c), the plaintext $x$ never leave $T_b$.}
    \label{fig:gates}
\end{figure*}

\begin{algorithm}[t]
\algstretch
\caption{Authenticated small XOR-masked LUT (\algname{LUT-Auth}) for party $b$}
\label{alg:lut}
\begin{algorithmic}[1]
\Require authenticated bits $\authb{x_1}{b},\dots,\authb{x_w}{b}$ of an unsigned $w$-bit $x$, certified Boolean; approved public table $T\in\Fp^{2^w}$ bound in $\mu$ by its hash; gate identifier $\mathit{gid}$; role $b$
\Ensure $\authb{y}{b}$ with $y=T[x]$
\State $T_b$: \cmd{RESERVE_PREP} for $\mathit{gid}$; \Abort{} on any descriptor or table-hash mismatch
\LineComment{Joint preparation inside $T_b$ (same $r$ in $T_0$ and $T_1$)}
\State $r\getsr\bits{w}$ by one joint draw with label $(\mathit{gid},\textsf{mask})$
\State issue $\authb{r_i}{b}\gets\AuthShare(r_i)$ to host $b$ once, for $i=1,\dots,w$
\State bind the joint DPF generator of $(\alpha,\beta)=(r,1)$ to $\mathit{gid}$ \Comment{never resampled}
\LineComment{Masked opening (host $b$ with $T_b$)}
\For{$i=1$ \textbf{to} $w$} \Comment{independent: one batch}
  \State $\authb{u_i}{b}\gets\authb{x_i}{b}+\authb{r_i}{b}-2\,\authb{x_ir_i}{b}$ \Comment{$\Pi_{\mathsf{Mult}}$}
\EndFor
\State $u\gets\CheckOpen(\auth{u_1},\dots,\auth{u_w})$ \Comment{$u=x\oplus r$}
\If{some $u_i\notin\{0,1\}$ or $T_0,T_1$ hold different $u$}
  \State \Abort
\EndIf
\LineComment{Full-domain scan inside $T_b$ in fixed public order; $k_b$ is streamed by GaC and never materialized}
\State $\tilde y_b\gets 0$
\For{$a\in\bits{w}$ in lexicographic order} \Comment{$\EvalAll$, depth-first}
  \State $\tilde y_b\gets\tilde y_b+T[a\oplus u]\cdot\DPF.\Eval(k_b,a)$
\EndFor
\State $\authb{y}{b}\gets\Epilogue(\tilde y_b)$ \Comment{\cref{sec:proto-epilogue}}
\State \Return $\authb{y}{b}$
\end{algorithmic}
\end{algorithm}

\textbf{Small XOR-masked LUT.}
\Cref{alg:lut} evaluates an approved public table $T$ with $2^w$ field entries on a $w$-bit input given as authenticated, certified-Boolean bits. The sampler draws a fresh uniform $r\in\bits{w}$ once and uses it twice: for the authenticated bits $\auth{r_i}$ and as the target of the joint DPF for $(r,1)$. The parties open $u=x\oplus r$ in one \CheckOpen{} batch, both modules reject a non-Boolean or mismatching vector, and $T_b$ scans the full domain in a declared fixed order,
\begin{equation*}
    \tilde y_b=\sum_{a\in\bits{w}}T[a\oplus u]\cdot\DPF.\Eval(k_b,a).
\end{equation*}
By \cref{thm:dpf-correct}, the evaluations sum to one only at $a=r$, so $\tilde y_0+\tilde y_1=T[r\oplus u]=T[x]$; since XOR with a fixed $x$ is a bijection on $w$-bit strings, $u$ is uniform given $x$ (\cref{thm:lut}). In $\EvalAll$ mode the $w$ correction words stay in protected registers until their level is fully expanded, so no key is materialized outside $T_b$. Besides the $w$ XOR products (one batched multiplication round when the bits exist; otherwise bit decomposition is charged to the gate), the gate needs one batched opening, $2^w-1$ internal tree expansions and a $2^w$-term field reduction: small tables are practical, full-domain tables over 64-bit inputs are not (\cref{tab:gates}).

\begin{algorithm}[t]
\algstretch
\caption{Authenticated shifted intervals and piecewise polynomial (\algname{Interval-Auth}) for party $b$}
\label{alg:interval}
\begin{algorithmic}[1]
\Require $\authb{x}{b}$; public breakpoints $0=\tau_0<\tau_1<\dots<\tau_m=p$ with $m\ge2$; public coefficients $a_{i,j}\in\Fp$ of $P_i(x)=\sum_{j=0}^{d}a_{i,j}x^j$; gate identifier $\mathit{gid}$; role $b$
\Ensure $\authb{y}{b}$ with $y=P_i(x)$ for the unique $i$ such that $\tau_i\le x<\tau_{i+1}$
\State $T_b$: \cmd{RESERVE_PREP} for $\mathit{gid}$; $r\getsr\Fp$ by one joint draw (rejection sampling); issue $\authb{r}{b}\gets\AuthShare(r)$ once
\State $c\gets\CheckOpen(\auth{x}+\auth{r})$ \Comment{$c=x+r\bmod p$}
\LineComment{Indicators inside $T_b$; every endpoint and wrap bit derives from the same $r$}
\For{$i=0$ \textbf{to} $m-1$}
  \State $L_i\gets(\tau_i+r)\bmod p$;\; $H_i\gets(\tau_{i+1}+r)\bmod p$
  \State $\omega_i\gets\one[L_i>H_i]$ with a sharing $(\omega_{i,0},\omega_{i,1})$
  \State $\tilde s_{i,b}\gets\omega_{i,b}+\DCF_{H_i}(c)_b-\DCF_{L_i}(c)_b$ \Comment{GaC}
  \State $\authb{s_i}{b}\gets\Epilogue(\tilde s_{i,b})$ \Comment{$s_i=\one[\tau_i\le x<\tau_{i+1}]$}
\EndFor
\LineComment{Coefficient selection and Horner evaluation (host $b$, authenticated arithmetic)}
\For{$j=0$ \textbf{to} $d$}
  \State $\authb{\bar a_j}{b}\gets\sum_{i=0}^{m-1}a_{i,j}\,\authb{s_i}{b}$ \Comment{local, $\Pi_{\mathsf{Lin}}$}
\EndFor
\State $\authb{y}{b}\gets\authb{\bar a_d}{b}$
\For{$j=d-1$ \textbf{down to} $0$}
  \State $\authb{y}{b}\gets\authb{y\cdot x}{b}+\authb{\bar a_j}{b}$ \Comment{$\Pi_{\mathsf{Mult}}$}
  \State rescale exactly where $\mu$ specifies (\cref{alg:trunc})
\EndFor
\State \Return $\authb{y}{b}$
\end{algorithmic}
\end{algorithm}

\textbf{Shifted intervals.}
For a proper nonempty public interval $[a,b)\subsetneq[0,p)$ (here $a,b$ are endpoints, not party indices), \cref{alg:interval} opens $c=x+r\bmod p$ for a fresh field mask $r$, and $T_b$ derives from the same $r$
\begin{equation*}
    L=(a+r)\bmod p,\quad H=(b+r)\bmod p,\quad \omega=\one[L>H].
\end{equation*}
With conservative DCFs for thresholds $L$ and $H$ (\cref{alg:dcf}; orientation $\one[c<\theta]$, payload $1$, independent coins) and a sharing of the wrap bit $\omega$, the raw share $\tilde s_b=\omega_b+\DCF_H(c)_b-\DCF_L(c)_b$ goes to the epilogue. Translation by $r$ maps $[a,b)$ onto the circular half-open interval from $L$ to $H$ ($L\neq H$ since $0<b-a<p$): the indicator is $\one[c<H]-\one[c<L]$ if $L<H$ and $1+\one[c<H]-\one[c<L]$ if the interval wraps, so \cref{thm:dcf} gives $\tilde s_0+\tilde s_1=\one[a\le x<b]$ (\cref{thm:interval}). Empty and full intervals are public constants. A partition may share one mask and one opening if every endpoint, wrap bit and auxiliary share is derived jointly from that mask, while distinct DCFs keep independent coins. The conservative DCF evaluates $n(n+1)/2$ path levels per threshold; its cost, and that of a projected $O(n)$ DCF~\cite{boyle2021function,storrier2023grotto} that \cref{thm:dcf} does not cover, are in \cref{tab:gates}.

\textbf{Piecewise polynomials.}
Activation and normalization functions are approximated by low-degree polynomials on a public partition~\cite{gupta2023sigma,pang2024bolt,ma2023secretflow}. The parties select coefficients $\auth{\bar a_j}=\sum_i a_{i,j}\auth{s_i}$ locally ($\Pi_{\mathsf{Lin}}$, \cref{fig:arith}) and apply Horner's rule with $d$ authenticated products, independently of the number $m$ of pieces. Exactly one indicator of a disjoint exhaustive partition is one, so \cref{thm:arith} yields the active polynomial; rescaling is inserted where the manifest specifies it (\cref{alg:trunc}). Approximation error of the approved coefficients is distinct from the cryptographic correctness of \cref{thm:lut,thm:interval}, which concerns the declared finite arithmetic.

\textbf{Exact comparison, bit decomposition and truncation.}
The LUT input, exact threshold comparisons and toward-zero signed truncation need canonical bits, which \cref{alg:bitdec,alg:trunc} (\cref{app:proof-gates}) derive with authenticated arithmetic alone (\cref{thm:bitdec,thm:cmp-trunc})~\cite{damgard2006unconditionally,catrina2010improved,escudero2020edabits}.

\textbf{Why exact circuits are a fallback.}
Their carry chains cannot be shortened by batching: \cref{alg:bitdec} performs $2n=122$ dependent multiplications for $n=61$, hence $2n+1=123$ sequential verified openings, and exact signed truncation chains two decompositions and a comparator into 307 authenticated multiplications and 309 sequential rounds, \est{30.9~ms} on LAN (\cref{tab:gates}). At two round trips per verified opening (\cref{sec:proto-check}), the 123-round chain alone would take about \est{17.2~s} on WAN. A valid one-round candidate therefore always wins under the cost rule below, and exact circuits are used only when no such candidate meets the gate's contract, with their cost charged to any LUT whose input bits do not yet exist.

\subsection{Direct Protected Gates and Cost-Aware Compilation}\label{sec:proto-direct}

\textbf{The direct protected gate.}
After a verified opening $c=x+r$, each module holds $c$ and $r$ and can compute $x=c-r$ inside its boundary, evaluate an approved deterministic gate $g$, and return a fresh authenticated sharing of $g(x)$ through \AuthShare{} (\cref{fig:gates}(c)). This is secure (\cref{thm:arith}) in the same model and with the same output simulation as the FSS gates, since the host again receives a fresh, independently uniform value and tag tuple (\cref{thm:epilogue}), provided the module's observable trace while computing $g$ meets the same simulatability assumption ($\eps{trace}$ in \cref{thm:main}). Concretely, fetching $T[x]$ from host memory or running in $x$-dependent time would leak $x$, so approved direct gates run from protected memory in data-independent time. A direct gate needs one verified opening, two AES blocks and five field multiplications; our model estimates \est{1{,}800}~M gates/s, above every FSS realization in \cref{tab:gates}.

\textbf{Cost-aware selection.}
For each nonlinear gate shape, the compiler estimates a cost tuple (latency, bytes, protected memory, field operations, PRG calls) for the direct gate, a small XOR LUT, an interval or polynomial FSS gate, and a separately proven malicious backend. It rejects candidates that violate the gate's semantic and security contract (the exact finite function, encoding and rescaling fixed by $\mu$ under the profile in force) and selects the least modeled end-to-end cost among the rest, accounting for dependency depth and transport; only independent checks are batched (\cref{sec:proto-check}). One constraint applies: gate shapes that the manifest marks as FSS-portable keep an FSS realization, so that the same compiled circuit runs under \ProfU. The compiler-selected default is therefore not the unconstrained minimum, and direct-only compilation is marginally faster (\est{3.82~s} versus \est{3.83~s} for BERT-Base on LAN).

\textbf{Why FSS stays in the datapath.}
If the direct gate is at least as cheap under \ProfT, why keep DPF generation and evaluation in the module? (i)~\emph{Compatibility.} Sigma- and Orca-style toolchains~\cite{gupta2023sigma,jawalkar2024orca} compile nonlinear layers into masked-input FSS gates, and \ProfU (\cref{sec:threat-profileu}) runs the circuit through an established malicious backend whose DPF keys the accelerator evaluates as party-local data; there the direct candidate is invalid because the hardware is not trusted with $x$. One DPF datapath serves both profiles and the untrusted-mode DFA workloads. (ii)~\emph{Full-domain scans.} PIR and small-LUT gates are data-independent, fixed-order scans that the pipelined DPF units execute at one iteration per cycle (\cref{sec:arch-hw}), so both profiles reuse one engine; this is a reuse argument, not evidence that the DPF form is the fastest option under \ProfT (\cref{sec:proto-pir}). (iii)~\emph{Short-lived sensitive state.} FSS keeps long-running evaluation state pseudorandom (seeds and correction words), and index- or input-dependent state short-lived. We treat (iii) only as defense in depth against physical and microarchitectural threats that \ProfT excludes; no theorem depends on it, and since each module holds $c$ and $r$, FSS gains no formal confidentiality over the direct gate (\cref{sec:threat-model}). The evaluation reports direct-only, FSS-only and compiler-selected default configurations side by side (\cref{sec:eval-ablation}).

\subsection{Distribution-Preserving Refactoring}\label{sec:proto-refactor}

DFA decouples DPF generation from protocol preprocessing by sampling the target directly as a uniform value and recovering the mask $r$ through $g^{-1}$ when the protocol's transformation $g$ is a bijection~\cite{dfa2026trusted}. \sys draws every target from the joint sampler in the same way, with two refinements of the semi-honest argument. Since DPF key privacy holds for arbitrary targets (\cref{sec:bg-fss}), uniformity is required by the application, which publishes $c=x+r$ or $u=x\oplus r$; a refactoring must therefore preserve the \emph{joint} distribution of the preprocessing, not the uniformity of each target.

\textbf{Joint, not marginal, distributions.}
A gate's preprocessing contains correlated objects: the mask, its bits, DPF or DCF targets, wrap bits and auxiliary shares. If a gate needs targets $r$ and $r+1$, resampling each uniformly keeps the marginals but destroys their unit difference; drawing $L$ and $H$ of \cref{alg:interval} independently likewise yields a wrong indicator. The refactoring is valid exactly under the conditions of \cref{lem:bijection}: the map is a bijection for the fixed context \emph{and} all auxiliary material is regenerated from the recovered mask by the unchanged sampler. For example, \cref{alg:interval} may draw $L$ uniformly, set $r=L-a$ and derive $H$ and $\omega$ from that $r$, but may not draw $L$ and $H$ independently.

\textbf{Noninvertible maps and truncation.}
For unsigned truncation, the sampler $R'=2^hA+U$ of \cref{lem:noninv} makes the DFA rule (shift left, fill the low bits uniformly~\cite{dfa2026trusted}) exact; signed shifts, nonuniform masks and other moduli need their own samplers.

\subsection{Verified GPU Matrix Products}\label{sec:proto-freivalds}

Authenticated linear layers need no extra verification: a GPU deviation that changes a value is caught at the next \CheckOpen, before the result enters a protected gate or a release, except with the probability bounded in \cref{thm:mac-sound}. A module that must \emph{consume} a GPU-computed matrix before any opening, however, must not accept it on the host's word, which would reintroduce the forgery oracle of scenario S2. For this case \cref{alg:freivalds} (\cref{app:proof-gates}) is an optional frozen-operand Freivalds check~\cite{freivalds1977probabilistic}, in the spirit of Slalom~\cite{tramer2018slalom} but bound to the ledger.

\textbf{Permitted uses and check.}
The check applies only when exposing the operands to that GPU is already allowed, as in public-by-party-local matrix products; it never permits exposing global secret triple masks, which are generated inside the TCB (\cref{sec:proto-arith}). The module binds the exact operand bytes $A\in\Fp^{m\times k}$ and $B\in\Fp^{k\times n}$ to their authoritative records and freezes the claimed $C$ (\cref{sec:proto-ledger}); only then does it draw $s$ independent secret uniform $\bm{v}\in\Fp^{n}$, test $C\bm{v}\stackrel{?}{=}A(B\bm{v})$ inside the protected verifier, and consume only the verified frozen bytes of $C$ (\cmd{VERIFY_MATRIX} in \cref{tab:commands}). If the GPU also transforms tag arrays, their tag equations are verified too.

\textbf{Soundness and cost.}
\Cref{thm:freivalds} bounds acceptance of a wrong product by $p^{-s}$, and $Q_F$ calls add $Q_F/p^s$ to \cref{thm:main}. The check is disabled in all evaluated configurations; enabling it adds implementation obligations (\cref{tab:obligations}) and this error term.

\subsection{Versioned-Snapshot PIR}\label{sec:proto-pir}

In DPF-based two-server PIR (\cref{eq:pir}), a malicious server can return a wrong share, which the client silently reconstructs into a wrong record, or answer from a stale database. \Cref{alg:pir} and \cref{fig:pir} show the \sys countermeasures.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_pir.pdf}
    \caption{Versioned-snapshot PIR (\cref{alg:pir}). Both modules bind the same query, scan the same snapshot bytes in a public order, hash exactly the bytes they consume, and quarantine the DPF-weighted reduction until the hash matches the authorized commitment $\mathsf{cm}_v$. A host that swaps a record after hashing or serves an old version causes an abort, never a wrong accepted record (scenario S8). Both modules learn $\alpha$, so query privacy relies on module trust.}
    \label{fig:pir}
\end{figure}

\begin{algorithm}[t]
\algstretch
\caption{Versioned-snapshot protected PIR (\algname{PIR-Snap}) inside module $T_b$}
\label{alg:pir}
\begin{algorithmic}[1]
\Require from the client over its confidential channel: index $\alpha$, query identifier $\mathit{qid}$, descriptor $\mathsf{desc}_v=(\mathsf{id},v,N,\mathsf{enc},\mathsf{cm}_v)$; snapshot records $D[0],\dots,D[N-1]$ streamed by host $b$
\Ensure value share $y_b$ of $D[\alpha]$ and certificate $\mathsf{cert}_b$ for the client, or \Abort
\LineComment{Step 1: query binding}
\State exchange $(\alpha,\mathit{qid},\mathsf{desc}_v)$ with $T_{1-b}$ over the protected channel
\If{the bindings differ, $\alpha\ge N$, or $\mathsf{desc}_v$ is unauthorized}
  \State \Abort
\EndIf
\LineComment{Step 2: joint DPF and same-byte scan ($N\ge2$; $N=1$ is a constant-record case with the same checks)}
\State $n\gets\lceil\log_2N\rceil$; bind $N$ and $2^n$; $D[i]\gets0$ for $N\le i<2^n$
\State joint DPF generator for $(\alpha,1)$ under label $(\mathit{qid},\textsf{pir})$ \Comment{GaC}
\State $h\gets\Hash.\mathsf{init}(\mathsf{id},v,N,\mathsf{enc})$;\; $\tilde y_b\gets0$
\For{$i=0$ \textbf{to} $2^n-1$ in public order} \Comment{$\EvalAll$, depth-first}
  \If{$i<N$}
    \State read $D[i]$ into $T_b$; $h\gets\Hash.\mathsf{update}(h,D[i])$
  \EndIf
  \State $\tilde y_b\gets\tilde y_b+\DPF.\Eval(k_b,i)\cdot D[i]$ \Comment{per coordinate}
\EndFor
\LineComment{Step 3: snapshot check; the result is quarantined until here}
\If{$\Hash.\mathsf{final}(h)\neq\mathsf{cm}_v$}
  \State \Abort
\EndIf
\LineComment{Step 4: fresh resharing and certified release}
\State $y_b\gets\tilde y_b+(-1)^b\zeta$ with a fresh joint pad $\zeta$ per coordinate
\State $\mathsf{cert}_b\gets$ certificate on $(\mathsf{sid},\mathsf{ep},\mathit{qid},\mathsf{desc}_v,b,\Hash(y_b))$
\State \Return $(y_b,\mathsf{cert}_b)$ to the client \Comment{no MAC tags}
\end{algorithmic}
\end{algorithm}

\textbf{Protocol and snapshot binding.}
Both role-bound modules receive the same canonical query from the client, compare the binding over their protected channel, pad the snapshot to $2^n$ records while authorizing only $\alpha<N$, and run a joint DPF for $(\alpha,1)$ by generate-and-consume. Each scans the same canonical bytes in the same public order, applies the same DPF weights to every record coordinate, and hashes exactly the bytes it consumes. The commitment $\mathsf{cm}_v$ covers the database identifier, version, shape, record encoding and ordered data bytes, and the result stays quarantined behind the release guard (\cref{sec:proto-ledger}) until the hash matches it; a host that swaps a record after hashing or serves an old version therefore causes an abort (scenario S8 in \cref{tab:scenarios}). A Merkle realization~\cite{merkle1987digital} must authenticate every consumed leaf and its position against the same root. Offloading the reduction to the GPU would need \cref{alg:freivalds} or a separately proven authenticated reduction, never a signature on the GPU's claim, and would export the expanded share vector, so \sys reduces inside the module. Each module releases only a freshly reshared value share (the value half of the epilogue) with a bound certificate, and the client reconstructs $D[\alpha]=y_0+y_1$.

\textbf{Guarantees and regimes.}
In regime (R1) of $\FPIR$ (\cref{fig:func}), with one malicious server host and an honest client, the client obtains the committed record or an abort, and the host learns nothing about $\alpha$ beyond $\Leak_{\mathrm{PIR}}$ (\cref{def:leakage}). In regime (R2), a malicious client alone learns only the requested record and the public descriptor. We make no combined claim (\cref{thm:pir}). Both modules learn $\alpha$, so query privacy relies on module trust: unlike untrusted two-server DPF-PIR such as GPU-DPF~\cite{lam2023gpu} or DFA's untrusted mode~\cite{dfa2026trusted}, which hides $\alpha$ from each server without trusted hardware, \sys offers no query privacy against a compromised module.

\textbf{Scope and design choice.}
Authenticated PIR~\cite{colombo2023apir} provides integrity without trusted hardware at additional server cost and is our malicious-secure GPU baseline (\cref{sec:eval-pir}). Two alternatives bracket our design. Since the modules know $\alpha$ anyway, a module could select $D[\alpha]$ with a constant-time comparator during the same public-order scan; this needs no AES expansion and would be bound by snapshot bandwidth rather than by the AES array. If $\alpha$ must stay hidden from the modules, the client can generate the DPF keys as in untrusted-mode DFA, and each module evaluates its own key inside the boundary with the same hashing, quarantine, resharing and certificates; this adds a DPF key-privacy term and, against a malicious client, a key-verification step~\cite{boyle2016function,boneh2021lightweight,decastro2022vfss}. We keep joint generation for uniformity with the inference datapath (\cref{sec:proto-direct}) and as defense in depth. We model neither alternative, so \cref{tab:pir} does not show that our design is the best \ProfT PIR. Assuming a PIR efficiency of \est{0.93} relative to DFA (\cref{app:model}), our model gives \est{16{,}349} versus 17{,}580~queries/s at $N=2^{20}$~\cite{dfa2026trusted} (\cref{tab:pir}).


==> qa/draft3/sections/06_architecture.tex <==
% ======================================================================
% Section VI: Architecture and System Integration
% Labels defined here: sec:arch, sec:arch-insight, sec:arch-hw, sec:arch-pipe,
%   sec:arch-iface, sec:arch-field, sec:arch-deploy, sec:arch-dse,
%   fig:hw, fig:pipeline, tab:commands, lst:mersenne
% ======================================================================
\section{Architecture and System Integration}\label{sec:arch}

This section describes how \sys realizes the protected module $T_b$ of \cref{sec:protocol} next to the GPU and how the untrusted host drives it. We keep the organization of DFA~\cite{dfa2026trusted} wherever the malicious setting permits and add only the blocks that the integrity chain requires. Hardware sizes are design parameters; red values are estimates (\cref{sec:eval-hw,app:model}). That this hardware realizes the ideal resource $\mathcal{F}_{\mathsf{T}}$ of the proofs is an implementation obligation (\cref{tab:obligations}).

% ======================================================================
\subsection{Design Insights}\label{sec:arch-insight}

\textbf{Key insight.}
Malicious security moves the dominant cost from DPF to authenticated linear algebra on the GPU, while protected FSS evaluation, exposed triple generation and \CheckOpen{} stay small (\cref{sec:analysis-cost,fig:motiv}). The module therefore need not become a second GPU: it must hold exactly the state whose exposure or modification would break the integrity chain and inspect every byte that crosses its boundary. The GPU is a fast but untrusted engine for authenticated linear algebra, and the module is dealer, verifier and release authority at once.

\textbf{What must be protected.}
A block belongs inside the trusted boundary if it holds material that reveals both parties' views or authorizes a release. These are exactly the TCB items of \cref{sec:threat-model} (keys, sampler and counters, generator state and correction words, table and reduction logic, challenges and residuals, release decisions); everything else stays outside (\cref{fig:threat}).

\textbf{What stays on the GPU.}
Linear layers run as the matrix Beaver products of $\Pi_{\mathsf{Mult}}$ over the value lane and the $t=3$ tag lanes (\cref{fig:arith}), i.e., two dense products per lane, $2(1+t)$ in total, of the same public shape. A GPU result is a candidate share, never a certified value.

\textbf{Placement.}
An authenticated element costs 32~B per party at the module interface (\cref{sec:proto-repr}), so a link of bandwidth $B$ streams at most $B/32$ elements per second (\cref{sec:analysis-work}). The L2-adjacent placement of DFA delivers about 290~GB/s to the SMs~\cite{dfa2026trusted}, so we keep it: one DPF unit per L2 slice, a new protected core beside a designated L2 partition, and SM access through the DFA-mapped address range without a new network-on-chip (NoC) port.

% ======================================================================
\subsection{Hardware Design}\label{sec:arch-hw}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_hw.pdf}
    \caption{\sys hardware. Top: placement inside the GPU; as in DFA, one DPF unit sits next to each L2 slice and a designated slice hosts the VIGOR core. Bottom: logical organization of the protected module $T_b$ (red dashed trusted boundary). The 64 AES-128 engines are time-shared among PRG expansion, challenge derivation and AEAD sealing; the Mersenne-61 field unit array (eight lanes in each DPF unit) serves epilogues, triples, reductions and check residuals. SMs, L2, NoC, HBM and host DRAM stay outside the boundary.}
    \label{fig:hw}
\end{figure}

\Cref{fig:hw} shows the module (area and power in \cref{sec:eval-hw}). The trusted boundary encloses the 16 DPF units of DFA (\cref{sec:bg-dfa}), the vector processing unit (VPU), the new \emph{VIGOR core} and the on-die links between them. Only command frames with share batches, PIR database records, authenticated output tuples, sealed spill pages and sealed channel frames cross it, none carrying a module secret in the clear. The blocks follow the integrity chain: parser and ledger admit \emph{authorized input}; sampler and field unit array produce \emph{correlated preprocessing}; the DPF units perform \emph{correct local evaluation}; the epilogue yields \emph{authenticated arithmetic}; freezer, check engine and peer channel enforce \emph{consistent opening}; and the release guard gates \emph{authorized output release}.

\textbf{DPF units and sampler.}
The AES datapath is unchanged. Each pipeline context carries two generator states, a separate evaluator state, a depth-first search (DFS) stack and the conversion $\Conv$ into $\Fp$, exactly the state of \cref{alg:gac}; correction words are consumed and discarded inside the unit, and raw leaf shares $\tilde y_b$ go to the field unit array lanes of the same unit, never to SM-readable buffers. The joint PRF sampler implements the labeled derivation and bounded rejection sampling of \cref{sec:proto-setup} under the session key.

\textbf{Field unit array (FUA).}
The FUA consists of 128 Mersenne-61 multiply-accumulate lanes, each with a $61\times 61$-bit multiplier and the two-fold reduction of \cref{lst:mersenne}; its peak is 116~G multiply-accumulates per second at the 910~MHz 7~nm clock of DFA~\cite{dfa2026trusted}. It computes epilogues (three products per output), the triple products $c=ab$ and $C=AB$ with their \AuthShare{} tags (so matrix masks never reach the GPU), LUT and PIR reductions, interval sums and check residuals. The lanes sit in the DPF units, eight per unit (a design parameter), and the VIGOR core schedules them as one pool. Full-domain LUT and PIR reductions therefore run next to the leaves, and only per-query accumulators (three field elements per PIR query) travel to the core (\cref{sec:arch-dse}).

\textbf{Check engine and freezer.}
The check engine executes steps~3 and~4 of \cref{alg:checkopen}: it derives the $t$ challenge vectors only after both frozen roots are fixed, accumulates the residuals on FUA lanes (two products per lane and element) and evaluates all lanes over the full batch before emitting one generic status, so neither the status nor its latency reveals which lane or position failed. \cmd{FREEZE_BATCH} copies the exact submitted bytes into a 256~KB freeze SRAM (8{,}192 tuples of 32~B) and hashes them with their descriptor into the root $h_b$ that the modules exchange; larger batches spill to AES-GCM-sealed immutable HBM pages~\cite{dworkin2007gcm,mcgrew2004gcm} whose authoritative root and page counters stay inside, so after the challenge only authenticated frozen bytes are reread (\cref{sec:proto-ledger}).

\textbf{Ledger, release guard and control.}
A 32~KB ledger SRAM holds the authoritative state of every in-flight gate and the randomness identifiers burnt at reservation (\cref{fig:ledger}). The release guard opens for a gate only in state \lstate{VERIFIED}, and an epoch abort closes every outstanding response atomically (\cref{sec:proto-ledger}); the release multiplexer and output FIFO of \cref{fig:hw} belong to the release-guard logic. The peer-channel controller keeps independent directional keys, never repeats a nonce and enforces a per-session traffic and forgery budget. The SC300-class control core of DFA~\cite{st33tpm12spi,arm_cortex_m3} runs measured boot, attestation and the key establishment covered by $\eps{setup}$, and the 16-lane VPU of DFA~\cite{cavalcante2019ara} handles the remaining protocol logic, including the range check $x^*\in\mathsf{In}_\nu$ of $\Pi_{\mathsf{Input}}$ and the validity predicates of $\mu$ at the public boundaries that $\mu$ declares. Host software cannot drive the module's clock or voltage outside its safe operating range (DVFS isolation, \cref{app:func-module}).

\textbf{AES time-sharing.}
The 64 engines are the module's only AES resource. A slot arbiter per unit serves PRG expansion (two blocks per expansion, $6n+3$ per GaC output), challenge derivation (1.5 blocks per checked element: three 64-bit words for three 61-bit challenges) and AEAD keystream for sealing and the peer channel (two blocks per 32-byte tuple); one AEAD/GHASH block serves both the freezer and the peer-channel controller. Check and sealing requests take priority because they are short and on the critical path of the next round; PRG contexts fill all other slots. A per-slot purpose tag selects the key context, so the uses never share a key.

% ======================================================================
\subsection{Pipeline Scheduling and Memory}\label{sec:arch-pipe}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_pipeline.pdf}
    \caption{Scheduling inside a DPF unit. (1)~Generator (g) and evaluator (e) expansions of at least $L$ independent contexts interleave to hide the $L$-cycle AES and correction feedback latency. (2)~AES slots are time-shared among PRG expansion, challenge derivation and AEAD sealing. (3)~Depth-first $\EvalAll$ keeps one pending sibling per level, i.e., $O(n)$ state per context.}
    \label{fig:pipeline}
\end{figure}

\textbf{Context interleaving.}
With an AES and correction feedback latency of $L$ cycles, one dependent path advances at most one level every $L$ cycles, so one issue per cycle needs at least $L$ independent contexts per unit (\cref{fig:pipeline}, panel~1). For the 20-stage DFA pipeline~\cite{dfa2026trusted} we therefore provision 20 contexts per unit, one per stage. The three expansions of a malicious GaC level issue back to back, because $\PRG(\tilde s)$ does not depend on $\CW^{(i)}$; only the correction waits for all three. A context (three 129-bit path states, the correction word in flight, target, query, payload and level) needs fewer than 100~B, so 20 contexts take less than 2~KB per unit, and a single gate with $n=61$ completes in \est{1.71~$\mu$s}.

\textbf{Separate old controls.}
Each unit keeps separate registers for the \emph{old} generator bits $t_0,t_1$ and the \emph{old} evaluator bit $\tilde t$ (\cref{sec:analysis-dpf}), captures all outputs of a transition before overwriting its inputs, and never substitutes generator states for evaluator roots; this is the schedule covered by \cref{thm:gac}. Planned RTL tests exercise signed final conversion, zero payloads, all-zero and all-one indices, $x=\alpha$ and divergence at every depth.

\textbf{Depth-first EvalAll.}
LUT and PIR gates evaluate the full domain. Depth-first traversal keeps one pending sibling per level ($O(n)$ states per traversal) and a complete tree needs $2^n-1$ internal expansions (panel~3). The 512 queries of a PIR batch walk the same public leaf order in lockstep, so each snapshot record is read and hashed once per batch and folded into 512 per-query accumulators. For $N=2^{20}$, 512 contexts with 20 pending siblings of 17~B occupy about 174~KB, or 11~KB per unit, which fits the traversal buffers of DFA~\cite{dfa2026trusted}.

\textbf{Pads and frozen buffers.}
The four pads of an output occupy two AES blocks and are drawn in step with the leaf, so no pad buffer beyond the pipeline depth is needed. A checked batch occupies the freeze SRAM until its verdict two peer round trips later, so batches beyond 8{,}192 elements, such as the 65{,}536-element batches of \cref{fig:checkperf}, spill to sealed pages.

% ======================================================================
\subsection{Command Interface and Host Integration}\label{sec:arch-iface}

\begin{table}[t]
\centering
\caption{Commands of the protected module $T_b$. Every command is a canonical frame bound to session, epoch, role and gate; the ledger state reached on success is given in parentheses. No command authenticates a host-supplied value.}
\label{tab:commands}
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\linewidth}{l >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X}
\hline
\textbf{Command} & \textbf{Required check} & \textbf{Allowed result} \\
\hline
\cmd{OPEN_SESSION}  & Authenticated identities, role, fresh epoch, manifest $\mu$ & Session capability \\
\cmd{RESERVE_PREP}  & Approved gate, unused randomness identifiers & Party-local authorized preprocessing, issued once (\lstate{PREPARED}) \\
\cmd{FREEZE_BATCH}  & Exact canonical bytes, dimensions, expected wire list & Frozen root $h_b$ and handle (\lstate{FROZEN}) \\
\cmd{CHECK_OPEN}    & Both frozen roots, independent challenge lanes, peer residuals & Verified prescribed opening or abort (\lstate{VERIFIED}) \\
\cmd{EVAL_FSS}      & Bound table or function, \lstate{VERIFIED} and unconsumed input opening, fixed role & Freshly reshared authenticated local output (\lstate{CONSUMED}) \\
\cmd{VERIFY_MATRIX} & Anchored operands, frozen candidate & Verified immutable result handle (\lstate{VERIFIED}) \\
\cmd{FINAL_OUTPUT}  & Authorized recipient, output mask, accepted check & Bound frame with $\upsilon=y+o$ and certificate (\lstate{CONSUMED}, then \lstate{RELEASED}) \\
\cmd{ABORT}         & Any integrity or lifecycle violation & Epoch invalidation, no candidate values (\lstate{ABORTED}) \\
\hline
\end{tabularx}
\end{table}

\textbf{Host responsibilities.}
Host $b$ schedules the public circuit, stores only party-local authenticated arrays (value and each MAC lane as separate coalesced arrays, serialized canonically only at the protected interface), runs the exact field kernels of \cref{sec:arch-field} and sends share batches to $T_b$. Its scheduling may be adversarial, so the ledger, not the host, decides whether operation, identity, shape and order are admissible, and a reused buffer always carries a fresh transaction identifier.

\textbf{Commands and frames.}
\Cref{tab:commands} lists the eight commands with the ledger state each reaches (\cref{fig:ledger}); since none of them authenticates a host value, the forgery-oracle path of scenario~S2 is closed (\cref{tab:scenarios}). A frame carries version, session identifier, epoch, role, opcode, gate identifier, ordered input and output identifiers, field identifier, tag count, dimensions, payload length, sequence number and payload, all length-prefixed with explicit endianness; frames between modules or from a client bind the header as AEAD associated data. The parser copies each frame into protected memory before checking it and rejects truncation, trailing bytes, duplicate identifiers, malformed dimensions, noncanonical field elements (values of at least $p$ are rejected, never reduced) and unexpected opcodes.

\textbf{Data races and aborts.}
Verification and consumption use the same immutable parsed bytes. Independent gate batches may overlap, but a dependent nonlinear gate never consumes an unchecked masked opening. Any integrity or lifecycle violation, such as an invalid transition or a failed check, triggers \cmd{ABORT}, which poisons the epoch, prevents new challenges and atomically keeps the release guard closed for every outstanding response (\cref{sec:proto-ledger}). \Cref{tab:attacks} maps each injected fault to the block that stops it.

% ======================================================================
\subsection{Exact Field Arithmetic on the GPU}\label{sec:arch-field}

GPU kernels must compute the finite circuit that the proofs reason about, so floating-point shortcuts are excluded. An authenticated GEMM applies the matrix Beaver combination of $\Pi_{\mathsf{Mult}}$ on each of the four lanes, i.e., two products per lane ($D\,B_b$ and $A_b\,E$ on the value lane, likewise on each tag lane), $2(1+t)=8$ products of the same shape, plus the public product $DE$ shared by all lanes (\cref{fig:arith}); \cref{lst:mersenne} gives the scalar multiplication at the core of every kernel.

\begin{figure}[t]
\centering
\scriptsize
\begin{tabular}{|l|}
\hline
\begin{minipage}{0.95\linewidth}
\vspace{2pt}
\begin{verbatim}
constexpr uint64_t P = (1ULL << 61) - 1;  // 2^61 - 1
// canonical a, b < P; returns canonical a*b mod P
__device__ uint64_t mul61(uint64_t a, uint64_t b) {
  uint64_t lo = a * b;              // low 64 bits
  uint64_t hi = __umul64hi(a, b);   // high bits, < 2^58
  uint64_t x  = (lo & P) + ((lo >> 61) | (hi << 3));
  x = (x & P) + (x >> 61);          // x <= 2^61
  return x >= P ? x - P : x;
}
\end{verbatim}
\vspace{-4pt}
\end{minipage}\\
\hline
\end{tabular}
\caption{Exact Mersenne-61 multiplication used by the GPU field kernels (CUDA). The first fold uses $2^{61}\equiv 1 \pmod p$; the second fold and the conditional subtraction return the canonical representative. No floating-point or Tensor-Core operation is involved.}
\label{lst:mersenne}
\end{figure}

\textbf{Correctness.}
For canonical $a,b<p=2^{61}-1$ the product is below $2^{122}$, so $\mathtt{hi}<2^{58}$ and $\mathtt{hi}\ll 3$ fits in 61 bits. Writing $ab=2^{64}\,\mathtt{hi}+\mathtt{lo}$ and using $2^{61}\equiv 1\pmod p$ gives $ab\equiv(\mathtt{lo}\bmod 2^{61})+\lfloor\mathtt{lo}/2^{61}\rfloor+2^{3}\,\mathtt{hi}\pmod p$. The last two terms occupy disjoint bit ranges (bits 0 to 2 and 3 to 60), so the bitwise OR equals their sum and the folded value is below $2^{62}$. The second fold yields at most $2^{61}=p+1$, and the conditional subtraction returns the canonical representative. The executed CPU check of this formula and the pending GPU conformance test are reported in \cref{sec:eval-attack}.

\textbf{Accumulation and numeric contract.}
A two-word 128-bit accumulator absorbs at most 64 unreduced products below $2^{122}$, so kernels fold at least once per 64 inner-dimension terms; random shares lie close to $p$ even for small plaintexts, so plaintext bounds never justify longer accumulation. The manifest $\mu$ fixes the scale $2^f$, signed encoding, toward-zero truncation (\cref{alg:trunc}), saturation, approximation coefficients and output decoding. For example, a dot product of length at most 4{,}096 with operand magnitudes at most $2^{20}$ stays within $|\cdot|\le 2^{52}$ before bias, which leaves room below $p/2$ only if bias and further accumulation are bounded too; the bound is recomputed per layer. FP16, BF16 and TF32 Tensor Cores never serve as exact field operations without a proven limb construction, and the exact finite circuit and a floating-point accuracy model remain separate references.

\textbf{GEMM cost assumption.}
Our model charges an exact Mersenne GEMM \est{1.25$\times$} the time of a wraparound 64-bit GEMM per lane ($\phi_{\mathrm{M}}$ in \cref{app:model}). This factor is an assumption, not a measurement: the kernel above additionally needs the high product word and a two-word accumulator per term, and the GPU test that would calibrate it has not run. Each $+0.25$ in $\phi_{\mathrm{M}}$ adds \est{0.52~s} to BERT-Base; with $\phi_{\mathrm{M}}=2$ its LAN latency would be \est{5.39~s}, i.e., \est{3.8$\times$} instead of \est{2.7$\times$} that of semi-honest trusted DFA.

% ======================================================================
\subsection{Deployment Targets}\label{sec:arch-deploy}

An on-die module cannot be added to a commercial A100, so we define three distinct experiments and never merge their timings. All three are planned (\cref{sec:eval-method}). \emph{(i) A100 software} runs the exact kernels, authenticated GEMM and host runtime on a real A100 with an emulated module. \emph{(ii) A ZCU102 prototype} (\texttt{xczu9eg-ffvb1156-2-e}~\cite{amd2023zcu102}) implements the datapath of \cref{fig:hw} at reduced scale (\est{4} DPF units, \est{16} AES engines, \est{32} FUA lanes at \est{250~MHz}, \cref{tab:fpga}) to validate streaming, freezing and release ordering; one board with an emulated peer shows functionality, not two independent trust boundaries, and an ARM process on it is not isolated from a malicious board administrator. \emph{(iii) The on-die projection} models integration next to the L2 slices with Accel-Sim~\cite{khairy2020accel} and synthesis, as in DFA; our headline numbers refer to it and currently come from the analytical model of \cref{app:model}. An external module uses staged transfer through host memory as its baseline, because GPUDirect RDMA needs platform and driver support and ordinarily a common PCIe root complex~\cite{nvidia2024gpudirect}; IOMMU protection is never disabled for a benchmark. In every target, freeze-before-challenge refers to immutable authenticated bytes, never to a GPU buffer that can change concurrently.

% ======================================================================
\subsection{Design-Space Comparison}\label{sec:arch-dse}

We compare the L2-adjacent organization of \sys with alternative homes for authentication, verification and randomness generation.

\textit{External protected module over PCIe.}
A discrete FPGA or security card~\cite{xu2025co} keeps the boundary off the GPU die but limits the interface to $B/32$ elements per second: \est{50~M} for the \est{1.6~GB/s} ZCU102 transport and \est{0.78~G} for \est{25~GB/s} of effective PCIe Gen4 bandwidth, against 9.1~G on the 290~GB/s on-die path of DFA~\cite{dfa2026trusted}. Because authenticated GEMM dominates, BERT-Base LAN latency rises only to \est{3.87~s} over PCIe and \est{4.59~s} with the ZCU102 link and lanes (\cref{tab:ablation}); the option suits prototyping but adds a second device per party and two device round trips per checked layer (\cref{app:model}).

\textit{Verification on the GPU SMs.}
In \ProfT the SMs belong to the malicious host: a corrupt checking kernel could see the challenges before choosing its errors, or simply report acceptance. Trusting them requires a GPU-wide TEE~\cite{volos2018graviton,jang2019heterogeneous,dhanuskodi2023confidential} covering SMs, caches, memory controllers and the driver interface, the large boundary that DFA and \sys avoid. The GPU therefore computes only products that the module verifies afterwards (\CheckOpen{} or the Freivalds check of \cref{sec:proto-freivalds}).

\textit{Tag DPF trees instead of the epilogue.}
One extra DPF tree per MAC lane (payload $\Delta_j\beta$) multiplies the PRG work of every gate by $1+t$ (\cref{tab:gatecost,fig:dpfthr}); the epilogue achieves the same with three multiplications and four pads (\cref{thm:epilogue}) at \est{3.8--4.0$\times$} the per-gate throughput of tag trees.

\textit{Software-only malicious backend.}
SPDZ-family preprocessing~\cite{keller2016mascot,keller2018overdrive,cramer2018spdz2k,keller2020mpspdz} needs inter-party communication that grows with the number of authenticated triples, and dealer-based malicious FSS, modeled after the protocol family of Shark~\cite{gupta2025shark}, ships authenticated keys and triples from an external dealer (\cref{tab:e2e}); both re-create the offline traffic that trusted DFA removed. Such a backend fits \ProfU, where the hardware itself is distrusted (\cref{sec:threat-profileu}); under \ProfT it pays for a trust assumption that the module already provides.

\textit{Dedicated check engines, a central FUA and per-slice checking.}
Checking needs only \est{2.8~ms} of module time per BERT-Base query against \est{131~ms} of protected FSS work, so dedicated AES engines for challenges and sealing would idle almost always. DPF units stay distributed because a single attachment point, a memory-channel path of about 180~GB/s, would cap DPF output at about 62\% of the 290~GB/s delivered bandwidth~\cite{dfa2026trusted}. The same limit rules out a central FUA: the raw 8-byte leaf shares of PIR at 16K entries alone would need \est{137~GB/s} (\est{76\%} of that path), so reductions stay in the units. Checks, by contrast, cost at most 3.5 AES blocks and six field multiplications per element and depend on the ledger, freeze SRAM and peer channel, which must be single points of authority; the VIGOR core therefore controls every check and holds one authoritative root per batch.


==> qa/draft3/sections/07_security.tex <==
% =====================================================================
% Section VII: Security Analysis
% File owner: sections/07_security.tex
% Labels defined here: sec:security, sec:sec-assump, sec:sec-main,
%   sec:sec-lemmas, sec:sec-scenarios, sec:sec-concrete, sec:sec-boundary,
%   thm:main, thm:dpf-correct, thm:gac, thm:dcf, thm:epilogue,
%   lem:hidden-key, thm:mac-sound, thm:arith, thm:bitdec, thm:cmp-trunc,
%   thm:lut, thm:interval, lem:bijection, lem:noninv, thm:freivalds,
%   thm:pir, tab:obligations, tab:lanes
% =====================================================================
\section{Security Analysis}
\label{sec:security}

We now show that \sys realizes the functionalities $\FC$ and $\FPIR$ of \cref{fig:func} with leakage $\Leak_C$ and $\Leak_{\mathrm{PIR}}$ (\cref{def:leakage}) against a malicious host and GPU, as stand-alone security with abort (\cref{def:security}) in the explicit-simulator style~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}. Each link of the integrity chain, \emph{authorized input $\rightarrow$ correlated preprocessing $\rightarrow$ correct local evaluation $\rightarrow$ authenticated arithmetic $\rightarrow$ consistent opening $\rightarrow$ authorized output release}, is discharged by a named statement: input extraction (\cref{thm:arith}); in-module preprocessing and joint sampling (\cref{lem:bijection,lem:noninv}); exact DPF, DCF, FSS-gate and direct-gate correctness (\cref{thm:dpf-correct,thm:gac,thm:dcf,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval,thm:arith}); the epilogue and the arithmetic identities (\cref{thm:epilogue,thm:arith}); MAC-check soundness (\cref{lem:hidden-key,thm:mac-sound}); and gated release (\cref{thm:arith,thm:pir}). Full proofs are in \cref{app:proof-dpf,app:proof-auth,app:proof-gates,app:proof-main}.

% =====================================================================
\subsection{Assumptions and Error Terms}
\label{sec:sec-assump}

The theorem is proved in \ProfT (\cref{sec:threat}); we state module trust as an explicit ideal resource~\cite{katz2007universally}.

\begin{assumption}[Ideal protected module]
Corrupting host $b$ does not corrupt $T_b$; both modules are instances of the ideal resource $\mathcal{F}_{\mathsf{T}}$ (\cref{app:func-module}). The code, keys, parser, field arithmetic, ledger transitions, local memory, protected peer channel and approved I/O paths of each module are correct and confidential. Its externally observable trace (lengths, timing, host-visible memory and DMA activity, power, thermal and clock telemetry) is simulatable by a stipulated trace simulator from the command sequence issued by the host, $\mu$, the public lengths and the accept or abort outcomes, and is independent of the global MAC keys, challenges and residuals given these (all lanes are aggregated in data-independent time before one generic $\mathsf{status}$ is returned). Host software cannot drive the module's clock or voltage outside its safe operating range, or the module detects glitches and aborts (DVFS isolation); software-reachable undervolting~\cite{murdock2020plundervolt} is thus in scope (\cref{sec:threat}). Module state is fresh: a trusted monotonic service preserves freshness across reboots~\cite{parno2011memoir,matetic2017rote}, or the module irrecoverably erases its master key and requires a freshly attested session. Availability is not assumed.
\end{assumption}

\begin{assumption}[Setup, randomness, channels and bindings]
Each term bounds an idealization over the \emph{entire} admitted execution, not a single primitive call:
$\eps{setup}$, simulation of the authenticated setup of \cref{sec:proto-setup} by an ideal role-bound interface;
$\eps{prf}$, replacement of PRF/KDF outputs (AES-128, HKDF~\cite{krawczyk2010hkdf}) under distinct length-prefixed labels by independent coins, identical for the same joint label;
$\eps{channel}$, confidentiality and integrity of the AEAD channels~\cite{dworkin2007gcm,mcgrew2004gcm} with directional keys and nonrepeating nonces;
$\eps{bind}$, collisions or forgeries in manifests, snapshot commitments, frozen-page roots, certificates and session freshness~\cite{fips202,merkle1987digital};
$\eps{trace}$, the stipulated trace simulator.
\end{assumption}

Correctness of protected code, state and arithmetic is thus a \emph{premise}, not an estimated probability. The protocol contributes one statistical term, determined by the field $\Fp$ with $p=2^{61}-1$, the number $t$ of independent global keys $\Delta_j=\Delta_{0,j}+\Delta_{1,j}$ (host $b$ knows at most $\Delta_{b,j}$), and the number $Q$ of \CheckOpen{} batches. Exclusions and client assumptions are those of \cref{sec:threat}; the modules may see inputs (\cref{sec:discussion}).

% =====================================================================
\subsection{Main Theorem}
\label{sec:sec-main}

\begin{theorem}[Stand-alone static malicious security with abort]
\label{thm:main}
Under the assumptions of \cref{sec:sec-assump}, the protocols of \cref{sec:analysis-dpf,sec:protocol} (setup, ledger, exact DPF, generate-and-consume with the fresh authentication epilogue, conservative DCF, \AuthShare, \CheckOpen, $\Pi_{\mathsf{Input}}$ with the committed-input loader, $\Pi_{\mathsf{Lin}}$, $\Pi_{\mathsf{Mult}}$, $\Pi_{\mathsf{Out}}$, bit decomposition, comparison, truncation, LUT, interval and direct protected gates) realize $\FC$ with abort and leakage $\Leak_C$, and \cref{alg:pir} realizes $\FPIR$ with abort and leakage $\Leak_{\mathrm{PIR}}$ (\cref{def:security,def:leakage}), against a PPT adversary that statically corrupts at most one host or, for $\FPIR$ in regime (R2) of \cref{fig:func}, the client alone. With at most $Q$ \CheckOpen{} batches, the advantage of every PPT distinguisher in \cref{def:security} is at most
\begin{align*}
\eps{VIGOR}\le{}&\eps{setup}+\eps{prf}+\eps{channel}\\
&+\eps{bind}+\eps{trace}+Q\,(2/p)^{t}.
\end{align*}
If the Freivalds check (\cref{alg:freivalds}) is enabled for at most $Q_F$ calls with $s$ repetitions, the bound gains $Q_F/p^{s}$, and the binding obligations of \cref{thm:freivalds} apply.
\end{theorem}

\Cref{thm:main} is a stand-alone real/ideal statement about one admitted execution, preserved under sequential composition; we claim neither universal nor concurrent composability, and concurrent sessions that share module state are not covered (\cref{app:func}).

\textbf{What the bound omits.}
There is no DPF one-key-privacy term: keys never leave the modules, \cref{thm:dpf-correct} gives raw correctness and \cref{thm:epilogue} makes every exported tuple uniform. A key-exporting profile (\ProfU, \cref{sec:threat-profileu}, or verifiable FSS~\cite{decastro2022vfss}) must add its actual DPF or backend privacy assumption. The theorem does not prove that a concrete chip implements the ideal module (\cref{sec:sec-boundary}).

\textbf{Proof overview.}
The simulator $\Sim$ plays $\mathcal{F}_{\mathsf{T}}$ for both modules, keeps the global MAC keys internally, and tracks the ledger and, for every wire, the tuple a faithful corrupt party would hold; honest shares stay symbolic, so honest values are never needed. Five hybrids connect the real and ideal executions (\cref{app:proof-main}). In the real execution $\Hyb{0}$ the modules run the concrete module program: $\mathcal{F}_{\mathsf{T}}$ with its randomness $R$ instantiated by $\PRF_K$, peer and client channels by AEAD over the hosts' network, and \cmd{OPEN_SESSION} by attestation plus authenticated key exchange.
\begin{itemize}[leftmargin=*]
\item \textbf{$\Hyb{1}$ (ideal setup and channels).} Setup becomes the ideal role-bound interface, and protected-channel contents become ideal deliveries of the permitted lengths and schedules. Cost: $\eps{setup}+\eps{channel}$.
\item \textbf{$\Hyb{2}$ (ideal randomness and bindings).} PRF/KDF outputs become ideal coins, and any binding failure aborts; the ledger (\cref{fig:ledger}) then excludes label reuse, role swapping and post-challenge byte replacement. Streaming generate-and-consume is replaced by \cref{alg:gen} followed by \cref{alg:eval} (\cref{thm:gac}), and refactored samplers by their reference forms (\cref{lem:bijection,lem:noninv}); both replacements are exact. Cost: $\eps{prf}+\eps{bind}$.
\item \textbf{$\Hyb{3}$ (abort on an accepted wrong-value opening).} The experiment aborts at the first \CheckOpen{} batch accepted with $\bm{e}\ne\bm{0}$ (and, if \cref{alg:freivalds} is enabled, at the first accepted $C\ne AB$). It equals $\Hyb{2}$ until then; by \cref{lem:hidden-key,thm:mac-sound} the cost is $Q(2/p)^t$ (plus $Q_F/p^s$, \cref{thm:freivalds}).
\item \textbf{$\Hyb{4}$ (ideal execution).} Honest parties use $\FC$. $\Sim$ extracts corrupt inputs ($x^*=r+\varepsilon$ or the committed loader value) and aborts where the modules do (e.g., unless $x^*\in\mathsf{In}_\nu$), samples preprocessing tuples, epilogue and direct-gate outputs and every masked opening uniformly (the hidden preprocessing is defined afterwards), decides each check from $\inner{\bm{\rho}_j}{\bm{d}_j-\Delta_j\bm{e}}$ with its own keys and fresh challenges, delivers a corrupt recipient's output mask $o$ early and programs its opening $\upsilon=y+o$ after $\FC$ releases $y$, and appends the stipulated trace simulator. Since $\Hyb{3}$ accepts no wrong value, the trace-free views are identical (\cref{thm:arith,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval}); cost: $\eps{trace}$. PIR uses the simulator of \cref{thm:pir}.
\end{itemize}
The triangle inequality gives the bound. The adversary may still suppress delivery to honest parties: no fairness is added.

% =====================================================================
\subsection{Building Blocks}
\label{sec:sec-lemmas}

The statements refer to the exact algorithms of \cref{sec:analysis-dpf,sec:protocol}, which, unlike the semi-honest ones (\cref{sec:bg-dfa}), make root control bits, role inputs and separate generator and evaluator states explicit; each is followed by its proof idea.

\begin{theorem}[DPF correctness]
\label{thm:dpf-correct}
For all root seeds $s_0,s_1\in\bits{128}$ with root control bits $t_0=0$, $t_1=1$, every $n$, $\alpha,x\in\bits{n}$ and $\beta\in\Fp$, the keys of \cref{alg:gen} and the outputs $y_b$ of \cref{alg:eval} satisfy $y_0+y_1=\beta\cdot\one[x=\alpha]$. No uniform target and no hardness assumption is needed.
\end{theorem}

\noindent\textit{Proof idea.}
On the target prefix the control bits stay opposite; on a losing child $(s_0^{\lose}\oplus s_1^{\lose})\oplus((t_0\oplus t_1)\sCW)=0$ and the control bits cancel, so the states coincide and their signed outputs cancel. At the leaf $t_0-t_1=(-1)^{t_1}$, so $y_0+y_1=u_0-u_1+(-1)^{t_1}\CWout=\beta$ (\cref{app:proof-dpf}).

\begin{theorem}[Generate-and-consume equivalence]
\label{thm:gac}
For fixed roots, $\alpha$, $\beta$, role $b$ and query $x$, the raw share $\tilde{y}_b$ of \cref{alg:gac} equals the output of \cref{alg:eval} on the key $k_b$ that \cref{alg:gen} produces from the same inputs, node by node for every dependency-respecting depth-first order of $\EvalAll$.
\end{theorem}

\noindent\textit{Proof idea.}
Couple both executions: equal states before level $i$ give the same correction word, generator state and evaluator state after it. The theorem justifies scheduling only, not changes to expansion or correction (\cref{app:proof-dpf}).

\begin{theorem}[Conservative DCF]
\label{thm:dcf}
If \cref{alg:dcf} creates, for each $i=1,\dots,n$ (zero payloads included), an independent DPF with target $\alpha_1\cdots\alpha_{i-1}0$ and payload $\beta\alpha_i$, evaluated at $x_1\cdots x_i$, the shares sum to $\beta\cdot\one[x<\alpha]$, at a cost of $n(n+1)/2$ path levels.
\end{theorem}

\noindent\textit{Proof idea.}
If $x<\alpha$, exactly the prefix ending at their first differing bit ($x_i=0$, $\alpha_i=1$) contributes $\beta$; otherwise none does. \Cref{thm:dpf-correct} and linearity conclude (\cref{app:proof-dpf}).

\begin{theorem}[Epilogue correctness and local hiding]
\label{thm:epilogue}
For raw shares $\tilde{y}_0,\tilde{y}_1$ and fresh uniform pads $\zeta,\kappa_1,\dots,\kappa_t\in\Fp$, the outputs $y_b=\tilde{y}_b+(-1)^b\zeta$, $\gamma_{b,j}=\Delta_j y_b+(-1)^b\kappa_j$ form an authenticated sharing of $\tilde{y}_0+\tilde{y}_1$. For either fixed $b$, $(y_b,\gamma_{b,1},\dots,\gamma_{b,t})$ is uniform on $\Fp^{t+1}$ given the raw outputs and the keys, before conditioning on later prescribed openings, jointly across fresh outputs.
\end{theorem}

\noindent\textit{Proof idea.}
The pads cancel in the sums. For fixed $b$, $\zeta\mapsto y_b$ and each $\kappa_j\mapsto\gamma_{b,j}$ are bijections, so every tuple has probability $p^{-(t+1)}$ (\cref{app:proof-dpf}).

\begin{lemma}[Hidden-key invariant]
\label{lem:hidden-key}
In $\Hyb{2}$ with host $b$ corrupted, conditioned on its view and its shares $\Delta_{b,j}$, the honest shares $\Delta_{1-b,1},\dots,\Delta_{1-b,t}$ remain independent and uniform at every point up to the drawing of the challenges of the first check with a nonzero value error; that check either accepts (the event of \cref{thm:mac-sound}) or rejects and ends the execution.
\end{lemma}

\noindent\textit{Proof idea.}
Fresh tags are padded (\AuthShare, \cref{thm:epilogue}); linear updates are deterministic in the view; correct openings have zero residual; a tag-only error yields an outcome independent of $\Delta_j$; residuals and challenges stay inside the modules (\cref{app:proof-auth}).

\begin{theorem}[Wrong-value acceptance]
\label{thm:mac-sound}
Let a batch of $m$ positions submitted to \CheckOpen{} (\cref{alg:checkopen}) differ from the prescribed tuples by a value error $\bm{e}\in\Fp^m$ and tag errors $\bm{d}_1,\dots,\bm{d}_t\in\Fp^m$, fixed by the freeze. If $\bm{e}\ne\bm{0}$, no earlier batch with a nonzero value error has been accepted, and the lanes use independent uniform challenges $\bm{\rho}_j\in\Fp^m$ drawn after the freeze and hidden from the host, \CheckOpen{} accepts with probability at most $(2/p)^t$ in $\Hyb{2}$. Over at most $Q$ batches, an incorrect value is ever accepted with probability at most $Q(2/p)^t$.
\end{theorem}

\noindent\textit{Proof idea.}
Lane $j$ accepts iff $\inner{\bm{\rho}_j}{\bm{d}_j-\Delta_j\bm{e}}=0$. For $e_i\ne 0$ the vector vanishes only if $\Delta_j=d_{j,i}/e_i$ (probability $\le 1/p$ by \cref{lem:hidden-key}); otherwise the nonzero linear form vanishes with probability $1/p$~\cite{schwartz1980fast}. Each lane gives $1/p+(1-1/p)/p<2/p$, and lanes are independent. Apply the bound to the first wrong-value batch; a union bound over batches gives $Q(2/p)^t$, following the SPDZ MAC check~\cite{damgard2012spdz,damgard2013practical} (\cref{app:proof-auth}).

\begin{theorem}[Authenticated arithmetic and direct gates]
\label{thm:arith}
With correct modules and prescribed messages, the protocols of \cref{fig:arith} are exact: $\Pi_{\mathsf{Input}}$ yields $\auth{x}$ with $x=r+\varepsilon$ (or aborts unless $x\in\mathsf{In}_\nu$), $\Pi_{\mathsf{Lin}}$ preserves $\gamma_{0,j}+\gamma_{1,j}=\Delta_j x$, $\Pi_{\mathsf{Mult}}$ with a correct fresh triple yields $\auth{xy}$ (and $\auth{XY}$ with the factor order preserved), and $\Pi_{\mathsf{Out}}$ gives $y=\upsilon-o$ to its authorized recipient. A direct protected gate (\cref{sec:proto-direct}) for an approved deterministic $g$, evaluated from protected memory in data-independent time, outputs \AuthShare$(g(c-r))$, an authenticated sharing of $g(x)$ whose party-local tuple is uniform as in \cref{thm:epilogue}. Unless a nonzero value error is accepted or a binding fails, every deviation of a corrupt host selects a permitted input, leaves the computation unchanged, or causes abort.
\end{theorem}

\noindent\textit{Proof idea.}
With $d=x-a$, $e=y-b$ and $c=ab$: $c+db+ea+de=xy$~\cite{beaver1991efficient}, the tags follow scaled by $\Delta_j$, $Z=C+DB+AE+DE$ for matrices, and $\upsilon-o=(y+o)-o=y$ with $o$ uniform. A direct gate recomputes $x=c-r$ from a verified opening, and its trace falls under $\eps{trace}$. \CheckOpen{} and the ledger block changed or reused material; induct over gates (\cref{app:proof-auth}).

\begin{theorem}[Canonical bit decomposition]
\label{thm:bitdec}
For $p=2^n-1$ ($n=61$), \cref{alg:bitdec} returns authenticated bits (least significant first) of the canonical representative of $x$, using one masked opening $c=x+r\bmod p$ and $2n$ authenticated multiplications.
\end{theorem}

\noindent\textit{Proof idea.}
The first loop is a full subtractor giving $d=(c-r)\bmod 2^n$ and borrow $\one[c<r]$; with a borrow $x=c-r+p=d-1$ since $p=2^n-1$, which the second loop subtracts~\cite{damgard2006unconditionally} (\cref{app:proof-gates}).

\begin{theorem}[Exact comparison and signed truncation]
\label{thm:cmp-trunc}
From authenticated canonical bits of $x$ and a public $\theta\in[0,2^n)$, \cref{alg:trunc} returns authenticated $\one[x<\theta]$; for centered $z\in[-(p-1)/2,(p-1)/2]$ it returns $\mathrm{sgn}(z)\lfloor|z|/2^f\rfloor$, i.e., truncation toward zero.
\end{theorem}

\noindent\textit{Proof idea.}
The equality flag tracks the processed prefix, and $\mathit{lt}$ gains a term exactly at the first position with secret bit $0$ and threshold bit $1$. Negative values occupy the canonical upper half; $(1-2s)z$ is the magnitude without wrap, and shifting its bits floors~\cite{catrina2010improved}. Fixed-point products must stay below $p/2$ before truncation (\cref{app:proof-gates}).

\begin{theorem}[Authenticated LUT]
\label{thm:lut}
For an approved table $T$ of $2^w$ entries and certified authenticated bits of $x\in\bits{w}$, if the mask bits and the DPF target of the keys for $(r,1)$ come from the same fresh uniform $r$, \cref{alg:lut} outputs $\auth{T[x]}$ and the opened $u=x\oplus r$ is uniform given $x$.
\end{theorem}

\noindent\textit{Proof idea.}
By \cref{thm:dpf-correct}, $\tilde{y}_0+\tilde{y}_1=\sum_a T[a\oplus u]\one[a=r]=T[x]$, and XOR by fixed $x$ is a bijection; independent resampling of the target would break the identity (\cref{app:proof-gates}).

\begin{theorem}[Intervals and piecewise polynomials]
\label{thm:interval}
For a proper nonempty public $[a,b)\subset[0,p)$, \cref{alg:interval} outputs $\auth{\one[a\le x<b]}$; for a disjoint exhaustive partition, Horner evaluation of the selected coefficients outputs $P_{i^\star}(x)$ for the interval containing $x$, in the declared finite arithmetic.
\end{theorem}

\noindent\textit{Proof idea.}
Adding $r$ maps $[a,b)$ to the circular interval from $L$ to $H$; the indicator is $\one[c<H]-\one[c<L]$ if $L<H$ and $1+\one[c<H]-\one[c<L]$ if $L>H$, which is the raw share by \cref{thm:dcf}. Exactly one indicator is one, and Horner with \cref{thm:arith} gives the polynomial; no equality to an unapproximated real function is claimed (\cref{app:proof-gates}).

The next two lemmas state when the semi-honest decoupling, which samples DPF targets directly~\cite{dfa2026trusted}, remains valid: joint distributions with all auxiliary material must match, not only marginals (\cref{sec:proto-refactor}).

\begin{lemma}[Bijection with correlated auxiliary material]
\label{lem:bijection}
Fix $Z=z$, $R$ uniform on a finite $\mathcal{R}$, a bijection $g_z:\mathcal{R}\to\mathcal{A}$, independent coins $W$ and an auxiliary sampler $J$. Then $(R,g_z(R),J(z,R,W))$ and $(g_z^{-1}(A),A,J(z,g_z^{-1}(A),W))$ with $A$ uniform on $\mathcal{A}$ are identically distributed.
\end{lemma}

\noindent\textit{Proof idea.}
Each pair $(r,a)$ has probability $1/|\mathcal{R}|$ in both experiments if $a=g_z(r)$ and zero otherwise; the same $J$ preserves equality. Independently resampling correlated targets such as $(r,r+1)$ breaks it (\cref{app:proof-gates}).

\begin{lemma}[Noninvertible transformations]
\label{lem:noninv}
For any $g$, sampling $A$ from the law of $g(R)$ and $R'$ from $R\mid g(R)=A$ reproduces $(R,g(R))$ and everything derived from $R'$. For unsigned truncation of a uniform $\ell$-bit mask by $h$ bits, $R'=2^hA+U$ with $A$, $U$ uniform on $\ell-h$ and $h$ bits.
\end{lemma}

\noindent\textit{Proof idea.}
$\Pr[A=a]\Pr[R=r\mid g(R)=a]=\Pr[R=r,g(R)=a]$; each truncated mask has probability $2^{-\ell}$. Signed shifts and other moduli need their own samplers (\cref{app:proof-gates}).

\begin{theorem}[Frozen-operand matrix check]
\label{thm:freivalds}
Let the module bind $A\in\Fp^{m\times k}$, $B\in\Fp^{k\times n}$, whose exposure to the GPU is already permitted, and freeze a claimed $C$. If $C\ne AB$, \cref{alg:freivalds} with $s$ secret uniform $\bm{v}\in\Fp^n$ drawn after the freeze accepts with probability at most $p^{-s}$, and over $Q_F$ calls an incorrect product is consumed with probability at most $Q_F/p^s$.
\end{theorem}

\noindent\textit{Proof idea.}
A nonzero row $\bm{e}$ of $C-AB$ gives $\inner{\bm{e}}{\bm{v}}=0$ for a $1/p$ fraction of $\bm{v}$~\cite{freivalds1977probabilistic,tramer2018slalom}; repetitions multiply; freezing fixes $C$ before $v$, and binding ties the verified bytes to the consumed ones (\cref{app:proof-gates}).

\begin{theorem}[Versioned-snapshot PIR]
\label{thm:pir}
With correct modules and binding snapshot and query interfaces: (R1) with an honest client and at most one malicious server host, \cref{alg:pir} gives the client the record $D[\alpha]$ of the snapshot committed by $\mathsf{cm}_v$ or abort, and the corrupt host's view is simulatable without $\alpha$; (R2) with a malicious client alone, accepted requests reveal nothing about the database beyond the requested records and the public descriptor $\mathsf{desc}_v$. Both modules learn $\alpha$, so the query privacy of (R1) rests on module trust, unlike untrusted two-server DPF-PIR (GPU-DPF~\cite{lam2023gpu}, untrusted-mode DFA~\cite{dfa2026trusted}), which hides $\alpha$ without trusted hardware.
\end{theorem}

\noindent\textit{Proof idea.}
\Cref{thm:dpf-correct} gives $y_0+y_1=\sum_i(\DPF_0(i)+\DPF_1(i))D[i]=D[\alpha]$; hashing the consumed bytes, comparing queries and role-bound certificates prevent substitution ($\eps{bind}$); results are freshly reshared (\cref{thm:epilogue}). For a malicious client the simulator extracts the index and reshares the ideal record (\cref{app:proof-pir}).

\textbf{Batched execution.}
The PIR configuration of \cref{tab:pir} processes $B=512$ queries per scan as one admitted execution whose manifest lists the $B$ query identifiers $\mathit{qid}$. Each query has its own joint DPF and pad labels, so the simulation of \cref{app:proof-pir} applies query by query. $B$ is part of the public schedule in $\Leak_{\mathrm{PIR}}$, and one abort (e.g., a snapshot mismatch) denies all $B$ queries, which security with abort permits.

% =====================================================================
\subsection{Scenario-by-Scenario Analysis}
\label{sec:sec-scenarios}

We map the scenarios of \cref{fig:scenarios,tab:scenarios} to the statements above; \cref{tab:attacks} lists the corresponding injections.

\begin{itemize}[leftmargin=*]
\item \textbf{S1: Share and tag tampering.} Freeze (S3) and \cref{thm:mac-sound,lem:hidden-key}: a wrong value passes with probability at most $(2/p)^t$ per batch; only the abort bit is revealed.
\item \textbf{S2: Forgery-oracle request.} No command (\cref{tab:commands}) tags a host value; the epilogue tags only protected results (\cref{thm:epilogue}); chosen values enter by input extraction.
\item \textbf{S3: TOCTOU buffer swap.} Freeze-before-challenge realizes the premise of \cref{thm:mac-sound} that errors precede challenges; tampered spill pages abort ($\eps{bind}$).
\item \textbf{S4: Replay and rollback.} Ledger and label binding ($\eps{bind}$) reject reused material; resuming old keys is excluded by the freshness clause.
\item \textbf{S5: Role/gate confusion.} Role-bound keys, joint labels and ledger descriptors turn misrouting into a mismatch and abort ($\eps{bind}$).
\item \textbf{S6: Premature release.} The release guard opens only \lstate{VERIFIED} entries; private outputs are opened as $\upsilon=y+o$, uniform to every host that is not the authorized recipient (\cref{thm:arith}).
\item \textbf{S7: Malformed preprocessing.} Triples and keys are correct because they are generated inside the boundary (\cref{thm:arith}), not because a MAC check certifies them; GPU products need \cref{thm:freivalds}, and correlated targets need \cref{lem:bijection,lem:noninv}.
\item \textbf{S8: Snapshot substitution.} Same-byte hashing and quarantine give the committed record or abort (\cref{thm:pir}).
\item \textbf{S9: Input substitution.} Permitted by $\FC$ and extracted; model provenance requires the committed-input loader.
\item \textbf{S10: Denial of service and selective abort.} Not prevented; aborts occur at public boundaries and are simulatable, and abort and validation outcomes ($\mathsf{status}$) are part of $\Leak_C$.
\end{itemize}

% =====================================================================
\subsection{Concrete Security}
\label{sec:sec-concrete}

Since $2/p\approx 2^{-60}$ for $p=2^{61}-1$, we have $\log_2 Q(2/p)^t\approx\log_2 Q-60t$. For a budget of $Q\le 2^{32}$ checked batches, \cref{tab:lanes} gives the statistical term.

\begin{table}[t]
\centering
\caption{Statistical term and BERT-Base LAN latency versus the number $t$ of MAC lanes ($Q\le 2^{32}$). Latencies are model estimates}
\label{tab:lanes}
\footnotesize
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{c c c c}
\hline
$t$ & $(2/p)^t$ per batch & $Q(2/p)^t$ & BERT-Base LAN (s)\\
\hline
1 & $\approx 2^{-60}$ & $\approx 2^{-28}$ & \est{2.53}\\
2 & $\approx 2^{-120}$ & $\approx 2^{-88}$ & \est{3.18}\\
3 & $\approx 2^{-180}$ & $\approx 2^{-148}$ & \est{3.83}\\
\hline
\end{tabular}
\end{table}

One lane is inadequate. Since the primitives target 128-bit computational security, $t=3$ is the smallest $t$ whose statistical term falls below $2^{-128}$; beyond it the primitives, not the MAC, limit the bound. Extra lanes barely change \CheckOpen{} itself (\est{0.648~ms} for $t=1$ versus \est{0.652~ms} for $t=3$ at $m=65{,}536$ on LAN, \cref{fig:checkperf}); their cost is one more authenticated GEMM lane per key (last column of \cref{tab:lanes}; \cref{sec:eval-ablation}).

\textbf{Tag-only errors.}
The bound concerns wrong \emph{values}: an error in a single tag lane escapes with probability $1/p$ without changing the opened value.

\textbf{Independent challenges.}
With one shared vector $\bm{\rho}$, an adversary submitting $\bm{d}_j=\bm{0}$ and any $\bm{e}\ne\bm{0}$ makes every lane residual $-\Delta_j\inner{\bm{\rho}}{\bm{e}}$, and all lanes vanish together with probability $1/p$. The product bound then collapses to one lane, so shared challenges are rejected (injection~8, \cref{tab:attacks}).

\textbf{Field, not ring.}
The step $\Delta_j=d_{j,i}/e_i$ needs a field. Over $\Z_{2^{64}}$, $e_i=2^{63}$ gives $\Delta_j e_i\equiv 0$ for every even $\Delta_j$, so one lane accepts with probability at least $1/2$; ring arithmetic needs a SPDZ2k-type backend~\cite{cramer2018spdz2k} with its own proof.

\textbf{Matrix checks.}
With $s=3$, each Freivalds call accepts a wrong product with probability at most $p^{-3}\approx 2^{-183}$, so $Q_F\le 2^{32}$ calls add at most $Q_F/p^{3}\approx 2^{-151}$ to the bound of \cref{thm:main}. Rejection sampling rejects one value with probability $2^{-61}$ per draw and retries under a fresh label; exhaustion affects only availability.

% =====================================================================
\subsection{Proof Boundary and Implementation Obligations}
\label{sec:sec-boundary}

\Cref{thm:main} concerns the abstract protocol in the protected-module model; \cref{tab:obligations} separates what this paper establishes from what a deployment must still provide. We executed a specification and a functional CPU reference model; its tests (\cref{sec:eval-attack}) check conformance on finite cases and are neither a machine-checked proof nor evidence for the statistical bound. GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet.

\begin{table}[t]
\centering
\caption{Proof boundary: what this paper establishes and what a deployment must still provide}
\label{tab:obligations}
\footnotesize
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}p{1.8cm}>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X}
\hline
\textbf{Obligation} & \textbf{Established here} & \textbf{Still required}\\
\hline
DPF/DCF, GaC, field, Boolean, LUT algebra & Explicit algorithms; \cref{thm:dpf-correct,thm:gac,thm:dcf,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval}; CPU reference tests & Constant-time, bit-exact CUDA and RTL refinement\\
\hline
Wrong-value authentication & \Cref{lem:hidden-key,thm:mac-sound}, independent lanes & Correct freeze, entropy, parser and check engine\\
\hline
End-to-end privacy and correctness & \Cref{thm:main} in the protected-module model & Realization of every module and trace assumption\\
\hline
PIR & \Cref{thm:pir} for the specified snapshot and regimes & Secure query channel, same-byte scan, certificates\\
\hline
GPU matrix verification & \Cref{thm:freivalds} & Protected verifier, bound input/result integration\\
\hline
Physical leakage and faults & Not claimed & Threat-specific engineering and evidence\\
\hline
Software-controlled DVFS and power telemetry & Required isolation specified & Isolated or monitored voltage and clock domain; telemetry filtering\\
\hline
Rollback protection & Required semantics specified (\cref{sec:proto-ledger}) & Monotonic service or erase-and-rekey lifecycle\\
\hline
Machine-checked proof & Not claimed & Future Lean, Coq or EasyCrypt development\\
\hline
\end{tabularx}
\end{table}

\textbf{Relation to the semi-honest design.}
The DFA analysis~\cite{dfa2026trusted} shows that its transformations preserve semi-honest security; \cref{thm:main} tolerates a malicious host and GPU by placing more integrity and lifecycle responsibility inside the boundary.


==> qa/draft3/sections/08_evaluation.tex <==
% =====================================================================
% Section VIII: Evaluation
% Numbers: model/numbers.md (red via \est{}), DFA paper (black + cite),
% executed CPU reference tests (black).
% =====================================================================
\section{Evaluation}\label{sec:eval}

We evaluate the cost of the protected gates and verified openings of \sys (\cref{sec:eval-micro,sec:eval-check}), end-to-end inference against semi-honest trusted DFA and dealer-based malicious FSS (\cref{sec:eval-e2e}), PIR (\cref{sec:eval-pir}), attack coverage and silicon cost (\cref{sec:eval-attack,sec:eval-hw}), and ablations and scaling (\cref{sec:eval-ablation,sec:eval-scale}).

% =====================================================================
\subsection{Evaluation Methodology}\label{sec:eval-method}

\textbf{Evidence status.}
We distinguish three kinds of numbers.
Black numbers cited to~\cite{dfa2026trusted} are copied from the semi-honest DFA paper; its end-to-end rows combine measured A100 execution with simulated DFA hardware.
Black numbers without a citation are analytical (operation counts, design constants and security parameters such as $p=2^{61}-1$, $t=3$ and $Q(2/p)^t$) or counts from the executed CPU reference tests of \cref{sec:eval-attack}.
Red marks assumed model parameters and outputs of the analytical performance model of \cref{app:model}; they are placeholders to be replaced by measurements.
We executed a specification and a functional CPU reference model; GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet.
Every conclusion drawn from a red number is therefore conditional on the model assumptions, and we name the dominant assumption wherever a conclusion depends on it.

\textbf{Hardware cost.}
The DFA blocks that \sys reuses (16 DPF units with 64 AES-128 engines, SRAM buffers, a 16-lane Ara VPU~\cite{cavalcante2019ara} and an SC300-class control core~\cite{st33tpm12spi,arm_cortex_m3}) keep the TSMC 28~nm synthesis results of~\cite{dfa2026trusted}, which use a pipelined open-source AES-128 core~\cite{opencores_aes128_pipeline}.
For the blocks that \sys adds (\cref{sec:arch-hw}), namely the Mersenne-61 field unit array (FUA), the check engine, the AEAD/GHASH block shared by the freezer and the peer-channel controller, the ledger with release guard and parser, and the ledger and freeze SRAMs, this paper reports pre-synthesis component estimates at the DFA clock (720~MHz at 28~nm, 910~MHz at 7~nm); they will be replaced by synthesis in the same 28~nm flow.
As in DFA, we scale to 7~nm with DeepScaleTool~\cite{sarangi2021deepscaletool}.
Separately, we size a functional prototype on a ZCU102 board (XCZU9EG, ffvb1156, speed grade $-2$)~\cite{amd2023zcu102} for Vivado implementation; its resource and power figures are pre-implementation estimates and will be reported separately from measured board energy.

\textbf{System-level performance.}
The target methodology for headline numbers is that of DFA: the module sits next to the GPU L2 slices, where DFA delivers about 290~GB/s~\cite{dfa2026trusted}, its DPF and FSS work is modeled as a stream consumed by GPU kernels in Accel-Sim~\cite{khairy2020accel}, and non-FSS work comes from real GPU execution.
The three experiments of \cref{sec:arch-deploy} (A100 software, ZCU102 prototype, Accel-Sim on-die study) are never merged.
Until they are measured, every \sys row comes from a decomposition of DFA's trusted-mode rows into GPU linear algebra, other GPU work, module FSS work, CPU-GPU transfers, online bytes and online rounds, transformed for four authenticated lanes, exact Mersenne GEMM and doubled rounds; all constants are in \cref{app:model} and \cref{tab:model-params}.
The decomposition parameters are fitted to the LAN and WAN latencies of~\cite{dfa2026trusted} (largest deviation \est{0.42\%}, ResNet-50 LAN).
Two published latencies per model cannot identify five parameters, so the fit is a consistency constraint, not a validation; the split between GPU linear algebra, other GPU work, bytes and rounds, on which every malicious factor acts, is itself an assumption to be replaced by profiling the A100 baseline.
Because authenticated GEMM dominates every malicious row, the most influential factor is the assumed \est{1.25$\times$} cost of exact 61-bit Mersenne GEMM over wraparound $\Z_{2^{64}}$ GEMM per lane; Tensor Cores are not used for field arithmetic (\cref{sec:arch-field}).

\textbf{Baselines.}
For private inference we compare five configurations per model.
\emph{GPU (SH)} and \emph{GPU+Trusted DFA (SH)} are the semi-honest rows of~\cite{dfa2026trusted}, which build on Orca~\cite{jawalkar2024orca} for CNNs and Sigma~\cite{gupta2023sigma} for Transformers.
\emph{Dealer-based malicious FSS} is modeled after the protocol family of Shark~\cite{gupta2025shark}: an external dealer ships authenticated keys and preprocessing, which we model with assumed factors (\cref{app:model}) of \est{2.2$\times$} the semi-honest key and preprocessing volume, \est{2.0$\times$} the GPU FSS evaluation work and \est{2.4$\times$} the semi-honest GPU energy, while charging exactly the same authenticated linear algebra, online bytes and doubled rounds as \sys.
The comparison therefore isolates preprocessing and key handling; it does not equalize trust.
The dealer of this protocol family is an input-independent third party that can run offline and away from both servers, and it never sees an input or an opening, so breaking privacy requires its masks together with a server's view.
The \sys modules sit inside the adversary's platform and see every input and opening (\cref{sec:threat-model}), so extracting the secrets of either module suffices.
The speedups below are therefore obtained under a stronger hardware-confidentiality assumption; a deployment that cannot accept it must use \ProfU, which we do not evaluate.
The row models the protocol family, not the Shark artifact, and we make no performance claim against Shark itself until a matching artifact has been run.
We do not model a dealer-free (MASCOT, SPDZ2k or PCG-based) malicious baseline~\cite{keller2016mascot,cramer2018spdz2k,boyle2019pcg}; \cref{sec:analysis-cost} explains why its FSS keys remain costly.
\emph{GPU+\sys w/o GaC} generates authenticated material locally but, like the corresponding DFA ablation, spills it to host memory through the AEAD spill path and rereads it.
\emph{GPU+\sys} is the compiler-selected default.
For PIR we compare GPU-DPF~\cite{lam2023gpu} and GPU+DFA, both semi-honest and taken from~\cite{dfa2026trusted}, a GPU-DPF variant that adds authenticated PIR in the style of Colombo et al.~\cite{colombo2023apir} (assumed to reach \est{0.45$\times$} the GPU-DPF throughput at \est{350~W}), and GPU+\sys.

\textbf{Workloads.}
We run ResNet-50~\cite{he2016deep}, BERT-Base~\cite{devlin2019bert}, GPT-Neo~\cite{brown2020language} and LLaMA2-7B~\cite{touvron2023llama}, with 128 input tokens for the Transformer models, as in~\cite{dfa2026trusted}.
LAN is 1~GB/s with a 0.05~ms round-trip time (RTT) and WAN is 70~MB/s with a 70~ms RTT, following~\cite{gupta2023sigma,jawalkar2024orca,huang2026beyond}.
Malicious configurations use $\Fp$ with $p=2^{61}-1$ and $t=3$ MAC lanes; semi-honest rows use $\Z_{2^{64}}$ as in their sources.
Unless stated otherwise, the compiler selects among direct, LUT and interval gates by modeled cost subject to the FSS-portability constraint (\cref{sec:proto-direct,app:model}).
PIR databases hold 16K to 4M entries of 128 bits (\cref{tab:pir}), served in batches of 512 queries; \cref{fig:scale} extrapolates the model to 16M ($2^{24}$) entries.
We do not report inference accuracy; exact finite-reference agreement and model accuracy will be reported once bit-exact GPU conformance is established.

\textbf{Measurement protocol.}
The replacement measurements will use 5 warm-up runs and 30 measured repetitions, report the median and the 95th percentile with bootstrap confidence intervals, keep raw per-run records, and fix random seeds only for public synthetic inputs, since randomness used for security must remain fresh.
We will report per-stage service times (cold and amortized setup, preprocessing, online arithmetic, nonlinear evaluation, checking, transfers and final release) next to the critical-path wall time, counting both parties and any external preprocessing service.
Network conditions are shaped on dedicated interfaces with Linux traffic control, recording achieved throughput and RTT.
GPU energy integrates sampled GPU power, board energy is measured at the rail or the wall, and every energy figure is cross-checked against average power times latency (or throughput times energy per query).

% =====================================================================
\subsection{Microbenchmarks}\label{sec:eval-micro}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_dpfthr.pdf}
\caption{Single-path DPF gate throughput per module (M gates/s, log scale) at 28~nm, 720~MHz and 64 AES-128 engines, for input length $n$: semi-honest trusted DFA, \sys (GaC with fresh authentication epilogue), and a malicious variant with per-lane tag trees ($t=3$ extra trees). Model estimates.}
\label{fig:dpfthr}
\end{figure}

\textbf{DPF gate throughput.}
\sys sustains \est{106} against \est{113}~M~gates/s for trusted DFA at $n=61$ and stays \est{6--9\%} below it for all $n$, because the epilogue adds two AES blocks per gate and we assume a pipeline efficiency of \est{0.85} (\est{0.90} for trusted DFA; \cref{app:model}).
It is \est{3.8--4.0$\times$} faster than per-lane tag trees for all $n$, approaching the factor $1+t=4$ by which tag trees multiply DPF work (\cref{fig:dpfthr,tab:gatecost}), with a single-gate latency of \est{1.71~$\mu$s} at $n=61$.
These are DPF gate rates: complete gates also include input masking, a verified opening and the surrounding arithmetic (\cref{sec:eval-e2e}).

\begin{table}[t]
\centering
\caption{Authenticated Nonlinear Gate Options per Module}
\label{tab:gates}
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l r r r r r}
\hline
\textbf{Gate} & \makecell{\textbf{Online}\\\textbf{rounds}} & \makecell{\textbf{AES}\\\textbf{blocks}} & \makecell{\textbf{Field}\\\textbf{mults}} & \makecell{\textbf{Thr.}\\\textbf{(M/s)}} & \makecell{\textbf{LAN lat.}\\\textbf{(ms)}} \\
\hline
Direct protected gate & 1 & 2 & 5 & \est{1{,}800} & \est{0.100} \\
LUT, $w=8$ & 1 & 542 & 268 & \est{72.3} & \est{0.100} \\
LUT, $w=12$ & 1 & 8{,}238 & 4{,}112 & \est{4.75} & \est{0.100} \\
LUT, $w=16$ & 1 & 131{,}134 & 65{,}556 & \est{0.30} & \est{0.104} \\
Interval, conservative DCF & 1 & 22{,}692 & 8 & \est{1.73} & \est{0.100} \\
Interval, optimized DCF$^{\ast}$ & 1 & \est{976} & 8 & \est{40.1} & \est{0.100} \\
Bit decomposition & 123 & n/m & 122 & n/a & \est{12.3} \\
Exact signed truncation & 309 & n/m & 307 & n/a & \est{30.9} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize $n=61$; 28~nm, 720~MHz, 64 AES engines, 128 field lanes. Rounds, AES blocks and field multiplications are analytical counts per gate; throughput and LAN latency are model estimates. The direct-gate throughput is an assumed rate for evaluating $g$ in the module, not derived from the AES and FUA peak rates. One online round is one \CheckOpen, i.e., two inter-module round trips; rounds include masked openings. LUT rows assume that the multiplication round of the $w$ XOR products batches with the preceding layer's openings (\cref{app:model}); otherwise they need one more round. n/a: round-bound, throughput not meaningful; n/m: not modeled (the AES work of the round-bound gates is negligible next to their round trips).
$^{\ast}$Projected $O(n)$ DCF; not covered by \cref{thm:dcf}.}
\end{table}

\textbf{Nonlinear gates.}
\Cref{tab:gates} compares the authenticated gate options of \cref{sec:proto-gates}.
All gates with one online round pay the two-round-trip floor of one \CheckOpen{} (0.1~ms on LAN; a LUT whose XOR products cannot batch with the preceding layer pays a second round) and differ only in throughput, which favors the direct gate (an assumed \est{1{,}800}~M~gates/s) and small LUTs (LUT work grows as $2^w$) and penalizes the conservative DCF (\est{1.73}~M~gates/s); the optimized DCF would reach \est{40.1}~M~gates/s but lies outside our proofs.
Bit decomposition and exact signed truncation are round-bound (123 and 309 rounds, \est{12.3~ms} and \est{30.9~ms} on LAN), so the compiler uses them only as a fallback when no table or interval formulation of the gate exists.

% =====================================================================
\subsection{Cost of Verified Openings}\label{sec:eval-check}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_checkopen.pdf}
\caption{\CheckOpen{} cost versus batch size $m$ (64 to 65{,}536 elements): (a)~LAN latency for $t=1,2,3$ MAC lanes (the curves overlap); (b)~throughput on LAN and WAN for $t=3$ (log scale). Model estimates.}
\label{fig:checkperf}
\end{figure}

\Cref{fig:checkperf} sweeps the \CheckOpen{} batch size $m$ from 64 to 65{,}536 elements, and three observations guide the compiler.
First, the number of MAC lanes barely matters for cost: even at $m=65{,}536$, moving from $t=1$ to $t=3$ raises LAN latency only from \est{0.648~ms} to \est{0.652~ms}, while the statistical term improves from $2^{-28}$ to $2^{-148}$ at $Q=2^{32}$ (\cref{thm:mac-sound}).
Second, on LAN the two round trips (0.1~ms) dominate up to a few thousand elements (\est{0.101~ms} to \est{0.135~ms} between $m=64$ and $m=4{,}096$); beyond that the 8-byte value share per element on the peer link dominates (\est{0.52~ms} of \est{0.652~ms} at $m=65{,}536$), throughput saturates near \est{100}~M~elements/s, and the protected work stays below \est{5\%} of the check latency.
Third, on WAN the two 70~ms round trips set a floor of 140~ms per check, so throughput is only \est{0.44}~M~elements/s even at $m=65{,}536$; batching independent openings (\cref{sec:proto-check}) is therefore essential, and the round count, rather than bandwidth or module work, is the WAN price of malicious security (\cref{sec:eval-ablation}).

% =====================================================================
\subsection{End-to-End Private Inference}\label{sec:eval-e2e}

\begin{table*}[t]
\centering
\caption{End-to-End Private Inference per Query}
\label{tab:e2e}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l l c r r r r r r}
\hline
\textbf{Model} & \textbf{Method} & \textbf{Security} & \makecell{\textbf{Offline}\\\textbf{comm. (GB)}} & \makecell{\textbf{CPU-GPU}\\\textbf{(GB)}} & \makecell{\textbf{Module-GPU}\\\textbf{(GB/party)}} & \makecell{\textbf{LAN}\\\textbf{latency (s)}} & \makecell{\textbf{WAN}\\\textbf{latency (s)}} & \makecell{\textbf{GPU+module}\\\textbf{energy (J)}} \\
\hline
\multirow{5}{*}{ResNet-50}
 & GPU~\cite{dfa2026trusted} & SH & 9.9 & 10.2 & n/a & 10.9 & 162 & 71.0 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.02 & 0.34 & n/r & 0.73 & 18.0 & 11.9 \\
 & Dealer-based malicious FSS & Mal & \est{21.8} & \est{22.4} & n/a & \est{25.1} & \est{346} & \est{170} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{38.0} & \est{1.22} & \est{2.97} & \est{34.7} & \est{48.6} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{0.44} & \est{1.22} & \est{1.79} & \est{33.6} & \est{43.6} \\
\hline
\multirow{5}{*}{BERT-Base}
 & GPU~\cite{dfa2026trusted} & SH & 17.1 & 19.3 & n/a & 18.8 & 296 & 121 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.1 & 2.55 & n/r & 1.42 & 46.4 & 18.2 \\
 & Dealer-based malicious FSS & Mal & \est{37.6} & \est{42.5} & n/a & \est{43.9} & \est{630} & \est{290} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{68.6} & \est{1.66} & \est{5.87} & \est{91.8} & \est{82.2} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{3.31} & \est{1.66} & \est{3.83} & \est{89.7} & \est{73.7} \\
\hline
\multirow{5}{*}{GPT-Neo}
 & GPU~\cite{dfa2026trusted} & SH & 76.4 & 80.4 & n/a & 83.6 & 1{,}140 & 587 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.24 & 4.27 & n/r & 5.93 & 101 & 114 \\
 & Dealer-based malicious FSS & Mal & \est{168} & \est{177} & n/a & \est{197} & \est{2{,}611} & \est{1{,}409} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{296} & \est{9.92} & \est{28.6} & \est{209} & \est{522} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{5.55} & \est{9.92} & \est{19.5} & \est{200} & \est{477} \\
\hline
\multirow{5}{*}{LLaMA2-7B}
 & GPU~\cite{dfa2026trusted} & SH & 256 & 268 & n/a & 279 & 3{,}695 & 1{,}879 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.81 & 12.8 & n/r & 18.0 & 193 & 303 \\
 & Dealer-based malicious FSS & Mal & \est{563} & \est{590} & n/a & \est{661} & \est{8{,}467} & \est{4{,}510} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{994} & \est{33.3} & \est{93.6} & \est{418} & \est{1{,}483} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{16.6} & \est{33.3} & \est{63.1} & \est{387} & \est{1{,}343} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\textwidth}{\footnotesize SH: semi-honest; Mal: static malicious security with abort. Latency is end to end, including offline distribution where present. Energy is GPU plus module energy summed over both computing parties (and the dealer when present). Module-GPU is the authenticated tuple stream per party on the on-die path; n/a: no module; n/r: not reported in~\cite{dfa2026trusted}. SH rows are copied from~\cite{dfa2026trusted}; red values are model estimates.}
\end{table*}

\Cref{tab:e2e} reports per-query results for the four models.
The semi-honest rows are context, not same-security competitors.

\textbf{Comparison with dealer-based malicious FSS.}
The modeled dealer-based baseline pays for malicious security mainly offline: its dealer ships \est{21.8--563~GB} of authenticated keys and preprocessing per query, which each party then stages through CPU-GPU transfers, whereas \sys generates the authenticated correlations inside the modules and ships none of them (\est{$<$0.001~GB} of session setup).
Across the four models this yields \est{10.1--14.0$\times$} lower LAN latency, \est{7.0--21.9$\times$} lower WAN latency and \est{3.0--3.9$\times$} lower energy than the modeled baseline (\est{11.4$\times$}, \est{7.0$\times$} and \est{3.9$\times$} for BERT-Base); the energy ratio rests on the assumed \est{2.4$\times$} energy factor of the baseline.
These latency ratios include the per-query offline distribution; excluding it, \sys is \est{1.5--1.8$\times$} faster on LAN (\est{1.6$\times$} for BERT-Base), and with no authenticated-key blow-up ($\psi_{\mathrm{key}}=1$) the baseline still needs \est{22.4~s} for BERT-Base (\est{5.8$\times$}).
The end-to-end gains thus come mainly from generating authenticated correlations inside the modules; the epilogue's advantage (\est{3.8--4.0$\times$} over per-lane tag trees) is per gate.
The WAN gain is largest for LLaMA2-7B (\est{21.9$\times$}), whose \est{563~GB} of authenticated material alone would occupy a 70~MB/s link for more than \est{2.2~hours}.

\textbf{Cost of malicious security.}
Relative to semi-honest trusted DFA, \sys raises LAN latency by \est{2.46--3.51$\times$} (\est{2.7$\times$} for BERT-Base) and WAN latency by \est{1.86--2.01$\times$}; these factors rest on the assumed Mersenne GEMM cost, and doubling it ($\mu_{\mathrm{M}}=2$) would give \est{5.39~s}, or \est{3.8$\times$}, for BERT-Base (\cref{sec:arch-field}).
It nevertheless remains \est{4.3--6.1$\times$} faster on LAN and \est{3.3--9.5$\times$} faster on WAN than the semi-honest GPU baseline, and it uses \est{1.2--1.6$\times$} less energy, although it tolerates a malicious host.
CPU-GPU traffic is assumed to grow by \est{1.3$\times$} over trusted DFA ($\phi_{\mathrm{cg}}$, \cref{app:model}) for canonical field words, residuals and certificates; the authenticated tuples themselves (\est{1.22} to \est{33.3~GB} per party) take the on-die module-GPU path and do not add to it.

\textbf{Generate-and-consume remains essential.}
Without GaC, the locally generated authenticated material must be spilled and reread, which inflates CPU-GPU traffic by \est{20.7--86$\times$} (\est{68.6~GB} instead of \est{3.31~GB} for BERT-Base) and LAN latency by \est{1.47--1.66$\times$}.
The authenticated representation makes materialization costlier than in the semi-honest case, where DFA reports 36.1~GB of CPU-GPU traffic and a 1.74$\times$ LAN penalty for BERT-Base without GaC~\cite{dfa2026trusted}.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_bert.pdf}
\caption{BERT-Base bottleneck analysis for \sys (model estimates). (a)~Speedup over dealer-based malicious FSS versus network bandwidth, split into the part due to eliminated key and preprocessing distribution and the remainder. (b)~LAN latency versus host-module link bandwidth (\est{1.6}, \est{8}, \est{25} and 290~GB/s~\cite{dfa2026trusted}). (c)~Breakdown of the \est{3.83~s} LAN latency.}
\label{fig:bert}
\end{figure}

\textbf{Bottleneck analysis.}
\Cref{fig:bert} decomposes the BERT-Base results.
(a)~The advantage over the dealer-based baseline depends on network bandwidth: \est{43.7$\times$} at 0.1~GB/s, \est{11.4$\times$} at 1~GB/s and \est{2.9$\times$} at 10~GB/s.
At 1~GB/s, \est{9.8$\times$} of the \est{11.4$\times$} comes from eliminated key and preprocessing distribution; at 10~GB/s, \est{1.7$\times$} of the \est{2.9$\times$} comes from lower key I/O and cheaper FSS evaluation and outweighs the distribution share.
Faster networks shrink the advantage but do not remove it, and, as observed for the semi-honest case~\cite{dfa2026trusted,huang2026beyond}, the energy and monetary cost of moving tens of gigabytes per query persists at any bandwidth.
(b)~Moving the module off die costs little for BERT-Base: LAN latency is \est{3.83~s} on die (290~GB/s), \est{3.87~s} over a \est{25~GB/s} PCIe-class link, \est{3.96~s} at \est{8~GB/s} and \est{4.46~s} at the \est{1.6~GB/s} of the ZCU102 prototype, because only \est{1.66~GB} of authenticated tuples per party cross the link.
(c)~The breakdown confirms Observation~2 of \cref{sec:analysis-cost}: authenticated GEMM accounts for \est{68\%} of the latency and \est{86\%} of the \est{2.41~s} added over trusted DFA, so the protected module is not the bottleneck; the tag lanes on the GPU and the doubled round count are, which motivates the compressed-check direction of \cref{sec:eval-scale}.

% =====================================================================
\subsection{Private Information Retrieval}\label{sec:eval-pir}

\begin{table}[t]
\centering
\caption{PIR Throughput and Energy per Query}
\label{tab:pir}
\footnotesize
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l l c c r r r}
\hline
\textbf{DB} & \textbf{Method} & \textbf{Integ.} & \makecell{\textbf{Index}\\\textbf{hidden}$^{\dagger}$} & \makecell{\textbf{Queries/s}\\\textbf{(k)}} & \makecell{\textbf{Energy/}\\\textbf{query (mJ)}} & \makecell{\textbf{Implied}\\\textbf{W}} \\
\hline
\multirow{4}{*}{16K}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & \cmark & 134 & 2.61 & 350 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & \cmark & 1{,}125 & 0.187 & 210 \\
 & GPU-DPF+APIR & \cmark & \cmark & \est{60.3} & \est{5.80} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \xmark & \est{1{,}046} & \est{0.180} & \est{188} \\
\hline
\multirow{4}{*}{1M}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & \cmark & 3.48 & 100 & 348 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & \cmark & 17.58 & 11.9 & 209 \\
 & GPU-DPF+APIR & \cmark & \cmark & \est{1.57} & \est{223} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \xmark & \est{16.35} & \est{11.5} & \est{188} \\
\hline
\multirow{4}{*}{4M}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & \cmark & 0.788 & 443 & 349 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & \cmark & 4.39 & 47.7 & 209 \\
 & GPU-DPF+APIR & \cmark & \cmark & \est{0.355} & \est{987} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \xmark & \est{4.08} & \est{46.0} & \est{188} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize 128-bit entries, batch 512. SH rows are from~\cite{dfa2026trusted} with energy expressed in mJ; implied power is throughput times energy per query and serves as a unit cross-check. Integ.: the client obtains the committed record or abort against a malicious server host (R1). $^{\dagger}$Index hidden from each server without trusted hardware: GPU-DPF and GPU+DFA (untrusted mode, client-generated keys) and the APIR variant hide $\alpha$ from each server, whereas both \sys modules learn $\alpha$ and its query privacy relies on module trust. Red values are model estimates.}
\end{table}

\Cref{tab:pir} reports PIR throughput and energy per query.
Assuming a PIR efficiency of \est{0.93} relative to DFA ($\eta_{\mathrm{PIR}}$, \cref{app:model}), meant to cover snapshot hashing, the in-module record reduction and fresh resharing with bound certificates, \sys reaches \est{1{,}046}, \est{16.35} and \est{4.08}~k~queries/s, a consequence of this assumption to be replaced by the Accel-Sim study, not a result.
The integrity guarantee does not depend on the model: in regime (R1), with one malicious server host, an honest client receives the committed record or abort (\cref{thm:pir}).
Query privacy, however, is weaker than in untrusted two-server DPF-PIR: both modules learn $\alpha$, so privacy against the hosts relies on module trust, whereas GPU-DPF and untrusted-mode DFA hide $\alpha$ from each server without trusted hardware (\cref{app:func-pir}); the two \ProfT alternatives of \cref{sec:proto-pir} are not modeled.
Energy per query is \est{3--4\%} below DFA's (\est{0.180~mJ} vs.\ 0.187~mJ at 16K entries) only because we assume an average power of \est{188~W} ($P_{\mathrm{PIR}}$), with the record reduction moved from the SMs into the protected path; this is the least certain PIR value and among the first we will measure.
Likewise, the authenticated GPU baseline is an assumed \est{0.45$\times$} of GPU-DPF throughput at \est{350~W}, so the \est{10.4--17.4$\times$} higher throughput and \est{19--32$\times$} lower energy per query of \sys against it follow from these assumptions; against semi-honest GPU-DPF, \sys is \est{4.7--7.8$\times$} faster under a weaker query-privacy model.

\textbf{Bottleneck analysis.}
As in DFA, full-domain PIR is bound by DPF expansion in the AES array rather than by memory; DFA sustains about 18.4~G~leaves/s (1{,}125~k queries/s $\times$ $2^{14}$ entries~\cite{dfa2026trusted}).
The additional protected work is amortized over a batch: each batch of 512 queries scans the snapshot once in public order, so the snapshot hash costs one pass per batch rather than one per query, and every record is weighted by the 512 DPF outputs of the batch in the FUA.
At 16K entries this reduction needs about \est{51~G} field multiply-accumulates/s, below the 92.16~G/s that the 128-lane FUA delivers even at the 28~nm clock of 720~MHz (116~G/s at 910~MHz; \cref{app:model}).
This capacity check shows only that the FUA is not saturated; it does not establish the size of the throughput loss.

% =====================================================================
\subsection{Security Validation}\label{sec:eval-attack}

\begin{table*}[t]
\centering
\caption{Attack and Fault Injections and Their Expected Outcomes}
\label{tab:attacks}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{c >{\raggedright\arraybackslash}p{4.3cm} >{\raggedright\arraybackslash}p{5.0cm} c >{\raggedright\arraybackslash}p{4.9cm}}
\hline
\textbf{\#} & \textbf{Injection} & \textbf{Mechanism} & \makecell{\textbf{Reference}\\\textbf{model}} & \textbf{Expected RTL/FPGA outcome} \\
\hline
1 & Change payload, query, role, gate id, table hash or shape (S5) & Ledger descriptor binding; role- and gate-bound PRF labels (\cref{sec:proto-ledger}) & \cmark & \est{Rejected at frame parse or authenticated computation fails; no preprocessing issued} \\
2 & Flip a control bit, root seed or correction word in a candidate engine & Conformance against the reference DPF (\cref{thm:dpf-correct}); unverified engine output is never authenticated & planned & \est{Reference mismatch flagged; engine output never authenticated or released} \\
3 & Change a GPU value share or tag (S1) & \CheckOpen{} with $t=3$ independent lanes (\cref{thm:mac-sound}) & \cmark & \est{Abort within one \CheckOpen{} (0.10--0.65~ms on LAN)}; acceptance at most $(2/p)^3$ per batch \\
4 & Triple with valid-looking tags but $c\neq ab$ (S7) & Triples computed inside the TCB; imported material needs a correctness proof & planned & \est{Never consumed; unproven import refused at reservation} \\
5 & Reuse a mask or counter; reset and resume old keys (S4) & One-time ledger, epoch poisoning, erase-and-rekey & \cmark & \est{Rejected before any accepted reuse} \\
6 & Modify a DMA buffer after freezing (S3) & Freeze-before-challenge; consume only frozen pages & \cmark & \est{Frozen authenticated bytes consumed, or abort} \\
7 & Swap only the last column of a GPU matrix product & Frozen-operand Freivalds over all columns, $s=3$ (\cref{thm:freivalds}) & planned & \est{Rejected}, except with probability at most $p^{-3}$ \\
8 & Reuse one challenge vector across MAC lanes & Independent per-lane challenges; configuration check (counterexample in \cref{app:proof-auth}) & planned & \est{Configuration refused at session setup} \\
9 & Change database bytes or version after hashing (S8) & Same-byte snapshot hash and certificate binding (\cref{thm:pir}) & \cmark & \est{Abort; quarantined result never released} \\
10 & Request output before the verification barrier (S6) & Release guard (\cref{sec:proto-ledger}) & planned & \est{Guard stays closed; no candidate values leave} \\
11 & Overflow or truncate with the wrong signed rule & Exact finite reference; numeric contract (\cref{thm:cmp-trunc}) & \cmark & \est{Mismatch detected; manifest rejected} \\
12 & Delay, drop or reorder packets (S10) & Bounded resources and abort & planned & \est{Abort; no fairness or availability claimed} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\textwidth}{\footnotesize Reference model: \cmark{} executed and passing in the CPU reference model; planned: no executed evidence yet. Red outcomes are expected on the RTL and FPGA implementations, not yet observed. Scenario IDs refer to \cref{tab:scenarios}.}
\end{table*}

\Cref{tab:attacks} lists the twelve attack and fault injections of our test plan, the mechanism that must stop each one, whether the executed CPU reference model already covers it, and the outcome we expect on the RTL and FPGA implementations.
The injections cover the scenarios of \cref{tab:scenarios} except S2, which the interface excludes by construction, and S9, which the functionality permits (its commitment-bound loader variant is covered by the model-provenance mechanism, not by an injection).
For S2, the command set of \cref{tab:commands} has no entry point that authenticates a host-supplied value, and row~2 checks the related requirement that even the module's own engine output is never authenticated before it conforms to the reference.

\textbf{Executed functional validation.}
The functional reference implements the ideal-module model in Python~3.10+ using only the standard library.
In the preparation environment it passes 22 unit tests with 0 failures and 0 errors.
The tests cover 21{,}840 exhaustive small-domain DPF target, query and payload cases (\cref{thm:dpf-correct}); 2{,}728 party-local comparisons between streaming GaC and materialized evaluation (\cref{thm:gac}); 1{,}364 DCF comparisons (\cref{thm:dcf}); 20{,}004 CPU checks of the GPU Mersenne multiplication formula of \cref{sec:arch-field} against arbitrary-precision arithmetic, including boundary operands; all 31 elements of a toy field with $p=31$ for bit decomposition (\cref{thm:bitdec}); 124 signed-truncation cases (\cref{thm:cmp-trunc}); all 16 inputs of a small LUT (\cref{thm:lut}); selected exhaustive toy intervals (\cref{thm:interval}); a small composed nonlinear and arithmetic pipeline; and PIR snapshot rejection.
Negative tests exercise noncanonical encodings, tag and value mutations, poisoned epochs, role, replay and ordering errors, immutable frozen objects, joint sampling, truncation fibers, and the ring zero-divisor counterexample that motivates the field representation (\cref{app:proof-auth}).

\textbf{Limits of this evidence.}
The toy field $p=31$ serves finite correctness tests only and provides no cryptographic security.
The reference expands seeds with SHAKE rather than the pinned AES-based PRG, so the equivalence tests must be rerun against the production PRG and output conversion.
The CUDA micro-test (65{,}536 products against a host 128-bit reference) is written but has not been compiled or run, and the RTL release guard is written but has not been simulated or synthesized; no GPU toolchain, Vivado or RTL simulator was available in that environment.
Rows marked ``planned'' in \cref{tab:attacks} therefore have no executed evidence yet.
These tests check that the implementation conforms to the algorithms; they do not measure a forgery probability.
Observing zero accepted forgeries in any finite campaign cannot support a bound such as $2^{-148}$; that bound comes from \cref{thm:mac-sound} together with the ledger rules.
Power and electromagnetic analysis, probing and fault injection require separate, threat-specific engineering evaluation (\cref{sec:discussion}).

% =====================================================================
\subsection{Hardware Cost}\label{sec:eval-hw}

\begin{table}[t]
\centering
\caption{Hardware Cost of One \sys Module}
\label{tab:hwcost}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l r r r r}
\hline
\multirow{2}{*}{\textbf{Component}} & \multicolumn{2}{c}{\textbf{28~nm}} & \multicolumn{2}{c}{\textbf{7~nm}} \\
\cline{2-5}
 & \textbf{mm$^2$} & \textbf{mW} & \textbf{mm$^2$} & \textbf{mW} \\
\hline
\multicolumn{5}{l}{\textit{DFA blocks reused by \sys~\cite{dfa2026trusted}}} \\
16 DPF units (64 AES-128) & 1.73 & 29 & 0.054 & 11 \\
SRAM buffers & 3.06 & 585 & 0.096 & 219 \\
VPU (16-lane Ara) & 1.97 & 794 & 0.062 & 298 \\
All DFA (incl.\ control core) & 7.67 & 1{,}683.5 & 0.239 & 631 \\
\hline
\multicolumn{5}{l}{\textit{Blocks added by \sys}} \\
Field unit array (128 lanes) & \est{2.80} & \est{1{,}000} & \est{0.088} & \est{375} \\
Check engine & \est{0.18} & \est{45} & \est{0.006} & \est{17} \\
AEAD/GHASH (freezer, peer channel) & \est{0.21} & \est{60} & \est{0.007} & \est{23} \\
Ledger, guard, parser & \est{0.09} & \est{12} & \est{0.003} & \est{5} \\
Ledger SRAM (32~KB) & \est{0.25} & \est{35} & \est{0.008} & \est{13} \\
Freeze SRAM (256~KB) & \est{1.07} & \est{200} & \est{0.033} & \est{75} \\
\cline{1-5}
\sys additions & \est{4.60} & \est{1{,}352} & \est{0.145} & \est{508} \\
\hline
\rowcolor{blue!6}All \sys & \est{12.27} & \est{3{,}036} & \est{0.384} & \est{1{,}139} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize DFA blocks are synthesis results from~\cite{dfa2026trusted}; blocks added by \sys are pre-synthesis estimates (red). 7~nm values are scaled with DeepScaleTool~\cite{sarangi2021deepscaletool}. One AEAD/GHASH block serves the freezer and the peer-channel controller. The 128 FUA lanes sit eight per DPF unit (area unchanged). Not yet costed: the trusted on-die links between the DPF units, the VPU and the VIGOR core.}
\end{table}

\begin{table}[t]
\centering
\caption{Planned ZCU102 Functional Prototype}
\label{tab:fpga}
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l r r r}
\hline
\textbf{Resource} & \textbf{Used} & \textbf{Available} & \textbf{Utilization} \\
\hline
LUT & \est{168K} & 274K & \est{61\%} \\
Flip-flop & \est{201K} & 548K & \est{37\%} \\
BRAM36 & \est{412} & 912 & \est{45\%} \\
DSP & \est{356} & 2{,}520 & \est{14\%} \\
\hline
\multicolumn{4}{l}{Datapath: \est{4} DPF units (\est{16} AES-128), \est{32} field lanes, \est{250~MHz}} \\
\multicolumn{4}{l}{DPF throughput: \est{1.0}~G~expansions/s; board power: \est{9.8~W}} \\
\multicolumn{4}{l}{Host link: \est{1.6~GB/s}, i.e., \est{50}~M authenticated elements/s} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize XCZU9EG-2FFVB1156~\cite{amd2023zcu102}: configuration and pre-implementation estimates (red). The DPF throughput assumes \est{50\%} of the \est{2.0}~G~expansions/s peak of \est{16} AES engines at \est{250~MHz} (one block per engine and cycle, two blocks per expansion).}
\end{table}

\Cref{tab:hwcost} reports the cost of one module; at 7~nm a complete module occupies \est{0.384~mm$^2$}, \est{0.046\%} of the 826~mm$^2$ A100 die~\cite{nvidia2020ampere}.
The FUA dominates the additions with \est{61\%} of the added area and \est{74\%} of the added power at 7~nm, followed by the 256~KB freeze SRAM with \est{23\%} of the added area, whereas the logic that enforces the security policy (ledger, release guard, parser and check engine) takes only \est{0.009~mm$^2$}, or \est{6\%} of the additions.
As in DFA, arithmetic and memory dominate the cost, not control.
No AES engines are added, because challenge derivation and AEAD freezing time-share the 64 engines with PRG expansion (\cref{sec:arch-hw}); for BERT-Base, checking occupies the AES array and the FUA for about \est{2.8~ms} per query, below \est{0.1\%} of its latency.

\Cref{tab:fpga} sizes the external ZCU102 prototype, which exists to check functional conformance and streaming behavior on one board with an emulated peer; security measurements need two independent protected devices (\cref{sec:arch-deploy}).
Its \est{1.6~GB/s} host link (\est{50}~M authenticated elements/s at 32 bytes each), its smaller FUA and its slower DPF engine make it a pessimistic functional point rather than a performance target; the ZCU102 row of \cref{tab:ablation} models only the link and the FUA.
It is not a \ProfT deployment target (\cref{sec:arch-deploy}).

% =====================================================================
\subsection{Ablation Study}\label{sec:eval-ablation}

\begin{table*}[t]
\centering
\caption{Ablation on BERT-Base}
\label{tab:ablation}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l c r r r r >{\raggedright\arraybackslash}p{5.1cm}}
\hline
\textbf{Configuration} & \textbf{Secure} & \makecell{\textbf{LAN}\\\textbf{(s)}} & \makecell{\textbf{Rel.}\\\textbf{LAN}} & \makecell{\textbf{WAN}\\\textbf{(s)}} & \makecell{\textbf{Energy}\\\textbf{(J)}} & \textbf{Note} \\
\hline
\rowcolor{blue!6}Compiler-selected default ($t=3$, batched checks) & \cmark & \est{3.83} & \est{1.00$\times$} & \est{89.7} & \est{73.7} & Reference configuration \\
w/o GaC & \cmark & \est{5.87} & \est{1.53$\times$} & \est{91.8} & \est{82.2} & Authenticated material spilled and reread \\
Tag trees instead of epilogue & \cmark & \est{4.12} & \est{1.08$\times$} & \est{90.0} & \est{80.4} & $(1+t)\times$ DPF work; FSS share is small \\
$t=1$ MAC lane & \xmark & \est{2.53} & \est{0.66$\times$} & \est{88.4} & \est{43.2} & $Q(2/p)^t=2^{-28}$ at $Q=2^{32}$: inadequate \\
$t=2$ MAC lanes & \cmark & \est{3.18} & \est{0.83$\times$} & \est{89.1} & \est{58.4} & $2^{-88}$ at $Q=2^{32}$ \\
FSS-only gates, conservative DCF & \cmark & \est{15.29} & \est{3.99$\times$} & \est{101.2} & \est{342.2} & $O(n^2)$ DCF of \cref{thm:dcf} \\
FSS-only gates, optimized DCF & \pmark & \est{4.20} & \est{1.10$\times$} & \est{90.1} & \est{82.3} & Projected; not covered by \cref{thm:dcf} \\
Direct protected gates only & \cmark & \est{3.82} & \est{1.00$\times$} & \est{89.7} & \est{73.3} & \ProfT only; drops the FSS-portability constraint \\
Small check batches ($m=64$) & \cmark & \est{4.24} & \est{1.11$\times$} & \est{90.2} & \est{74.6} & Per-batch overhead not amortized \\
External PCIe module (\est{25~GB/s}) & \cmark & \est{3.87} & \est{1.01$\times$} & \est{89.8} & \est{73.8} & Link roofline $B/32$ elements/s \\
ZCU102 link and FUA (\est{1.6~GB/s}, \est{32} lanes, \est{250~MHz}) & \cmark & \est{4.59} & \est{1.20$\times$} & \est{90.5} & \est{75.4} & Prototype link and slower triple generation; on-die DPF and AES rates kept \\
No \CheckOpen{} & \xmark & \est{3.80} & \est{0.99$\times$} & \est{50.5} & \est{73.6} & Insecure; performance lower bound only \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\textwidth}{\footnotesize LAN 1~GB/s, WAN 70~MB/s. Each row changes one choice of the compiler-selected default. Rel.\ LAN is LAN latency relative to the compiler-selected default. Secure: \cmark{} covered by our theorems; \pmark{} projected construction outside our proofs; \xmark{} not secure (statistically inadequate, or no verification). All latency and energy values are model estimates.}
\end{table*}

\Cref{tab:ablation} changes one design choice at a time for BERT-Base, and three conclusions follow.

\textbf{Protocol mechanisms.}
Generate-and-consume and the check round are the mechanisms that matter.
Disabling GaC costs \est{1.53$\times$} LAN latency (\cref{sec:eval-e2e}), and the insecure lower bound without \CheckOpen{} shows that the doubled round count costs \est{39~s} of the \est{89.7~s} WAN latency, the dominant WAN cost of malicious security.

\textbf{MAC lanes.}
$t$ is a security knob, not a performance one: $t=1$ saves \est{34\%} of the LAN latency but bounds a wrong opening only by $2^{-28}$, so the choice of $t=3$ follows from \cref{sec:sec-concrete} (\cref{tab:lanes}).

\textbf{Gate selection and placement.}
Because FSS is a small part of the malicious latency, tag trees, direct-only gates, small check batches and off-die links change LAN latency by at most \est{20\%} (with the DPF engine kept at its on-die rate); the epilogue matters most for LUT-heavy compiled models, where the \est{3.8--4.0$\times$} gate-level gap over per-lane tag trees (\cref{sec:eval-micro}) carries over.
The exception is FSS-only compilation with the conservative DCF of \cref{thm:dcf} (\est{3.99$\times$}), which is why the compiler selects gates by cost.
Direct-only (\est{3.82~s}) is marginally faster than the default (\est{3.83~s}) because the default keeps an FSS realization for gate shapes that the manifest marks as FSS-portable, so that the same compiled circuit runs under \ProfU; this allowance costs about \est{0.014~s} of module time (\cref{app:model}), and direct-only drops it and runs only under \ProfT (\cref{sec:proto-direct}).
Ablations on staged versus local checks and on caching versus recomputing bit decompositions are part of the measurement plan but are not yet modeled.

% =====================================================================
\subsection{Scalability}\label{sec:eval-scale}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_scale.pdf}
\caption{Scalability (model estimates). (a)~LAN latency with $t=1,2,3$ MAC lanes, normalized to semi-honest trusted DFA, annotated with the statistical term $Q(2/p)^t$ at $Q=2^{32}$ ($2^{-28}$, $2^{-88}$, $2^{-148}$). (b)~PIR throughput (queries/s, log scale) for $2^{14}$ to $2^{24}$ entries from a scaling model fitted to \cref{tab:pir} (a constant leaf rate for DFA and \sys, a calibrated per-entry efficiency for GPU-DPF); it matches the table at $2^{14}$, $2^{20}$ and $2^{22}$ entries to within \est{0.2\%}, interpolates between them and extrapolates beyond $2^{22}$ entries.}
\label{fig:scale}
\end{figure}

\textbf{MAC lanes and model size.}
\Cref{fig:scale}(a) normalizes LAN latency to semi-honest trusted DFA.
With $t=3$ the overhead grows from \est{2.46$\times$} for ResNet-50 to \est{3.51$\times$} for LLaMA2-7B, because the share of linear algebra grows with model size and each MAC lane replicates it: every additional lane adds about \est{0.65~s} for BERT-Base and \est{13.0~s} for LLaMA2-7B.
Authenticated GEMM on the GPU, not the protected module, is the scaling bottleneck.

\textbf{Triple generation.}
Correct matrix triples must be computed inside the protected boundary (\cref{sec:proto-arith}), so FUA work scales with the model's multiply-accumulate count.
LLaMA2-7B needs about \est{7.18~s} of FUA time per query at 128 lanes and 910~MHz, which overlaps with the \est{52.0~s} of authenticated GEMM except for an assumed \est{10\%} non-overlapped fraction ($\eta_{\mathrm{trip}}$, \cref{app:model}), leaving about \est{0.72~s} exposed.
The \est{32}-lane prototype at \est{250~MHz} would need about \est{105~s} for the same triples, another reason it is only a functional prototype; the on-die FUA should scale with the linear-algebra throughput of the host GPU.
If triple generation ever dominates, the alternatives are an imported malicious preprocessing backend with its own proof, or restructuring public-by-secret operations; exposing global secret masks to the GPU is not an option.

\textbf{Host-module bandwidth.}
BERT-Base moves only \est{1.66~GB} per party, well inside the $B/32$ roofline of \cref{sec:arch-insight}, which is why \cref{fig:bert}(b) is nearly flat above \est{8~GB/s}.

\textbf{PIR.}
\Cref{fig:scale}(b) shows PIR throughput from $2^{14}$ to $2^{24}$ entries.
Like DFA, the per-query cost of \sys grows linearly with the number of entries, so throughput falls from \est{1.05}~M to \est{1{,}022}~queries/s, whereas GPU-DPF reaches its peak per-entry efficiency near $2^{20}$ entries~\cite{dfa2026trusted,lam2023gpu}.
At $2^{24}$ entries \sys is \est{5.2$\times$} faster than GPU-DPF, under the weaker query-privacy model of \cref{sec:eval-pir}, and \est{11.5$\times$} faster than the authenticated GPU baseline.
Larger records increase the per-entry field reduction linearly while the DPF expansion stays unchanged, so for very large records the FUA, not the AES array, becomes the limit.

\textbf{Beyond per-lane tags.}
Because the tag lanes dominate large models, the most promising direction is to compress MAC checking, for example with rank-1 compressed checks that avoid carrying $t$ full tag arrays through the GPU.
Such schemes are not covered by our proofs and need their own soundness analysis, so we leave them to future work.
Scaling the number of DPF units and FUA lanes is a second, orthogonal knob; DFA found DPF-unit scaling to be nearly linear until on-chip bandwidth, about 7~TB/s of aggregate L2 read bandwidth on A100~\cite{nvidia2020ampere}, becomes the limit~\cite{dfa2026trusted}.


==> qa/draft3/sections/09_discussion.tex <==
% ==================================================================
% Section IX: Discussion and Limitations
% Owner labels: sec:discussion
% ==================================================================
\section{Discussion and Limitations}
\label{sec:discussion}

\sys claims that, under \ProfT, one maliciously corrupted host, including its GPU, driver and network stack, cannot make an honest party accept a wrong value or release an unauthorized one, except with the probability bounded in \cref{thm:main}. We now state what this claim does not cover and which evidence is still missing.

\textbf{Trust relocation, not removal.}
\sys moves the dealer of dealer-based FSS into two protected modules; it does not remove the dealer assumption. Both modules hold the joint-sampler key and the global MAC keys $\Delta_1,\dots,\Delta_t$ (\cref{sec:proto-setup}), so extracting the secrets of either module voids privacy and integrity for every session whose keys it holds. \Cref{thm:main} is a stand-alone statement under sequential composition; concurrent sessions that share module state are not covered (\cref{app:func}). The boundary also grows relative to DFA~\cite{dfa2026trusted}: the ledger, freezer, check engine, field unit array and release guard add only \est{0.145~mm$^2$} at 7~nm (\cref{tab:hwcost}), but each of them is logic that must be verified (\cref{tab:obligations}).

\textbf{What the modules learn.}
The modules are not blind. $\Pi_{\mathsf{Input}}$ validates $x^{*}=r+\varepsilon$ inside them (\cref{fig:arith}); after a verified opening $c = x + r$, module $T_b$ knows $c$ and $r$, hence $x$; the committed-input loader and the direct gate (\cref{sec:proto-direct}) see inputs explicitly; and in PIR both modules learn the client's index $\alpha$ (\cref{alg:pir}). For inference this is inherent to generate-and-consume and already holds for trusted DFA~\cite{dfa2026trusted}. For PIR it is a regression: the query privacy of \sys relies on module trust, whereas untrusted two-server DPF-PIR, such as GPU-DPF~\cite{lam2023gpu} and untrusted-mode DFA~\cite{dfa2026trusted}, hides $\alpha$ without trusted hardware. Client-generated keys evaluated inside the modules would avoid this but need key verification~\cite{decastro2022vfss}; neither this variant nor a constant-time select under \ProfT is modeled (\cref{sec:proto-pir}), and \cref{tab:pir} rests on assuming a PIR efficiency of \est{0.93} relative to DFA. FSS gates keep only seeds, control bits and correction words in long-lived state, whereas a direct gate computes on $x$ itself; we treat this as defense in depth only, because the trace model of \cref{thm:main} makes both options equivalent.

\textbf{Why two parties under \ProfT?}
Because the modules see plaintext, a single server whose protected module verifies an untrusted GPU, as in Slalom~\cite{tramer2018slalom}, would rest on the same hardware trust. The two-party structure buys two things. First, a host that held a value together with its complete tag would learn the MAC key; splitting every tag between two hosts lets SPDZ-style MACs~\cite{damgard2012spdz} check all GPU linear algebra at the next opening, whereas a single server must check each GPU product itself, for example with a Freivalds check per layer (\cref{sec:proto-freivalds}). Second, it keeps the two-party deployment of the FSS toolchains that DFA targets, on which \ProfU relies for its security (\cref{sec:threat-profileu}). It adds no protection against module compromise. For PIR as specified in \cref{alg:pir}, one server with one module would give the same guarantees. GPU-wide TEEs~\cite{nvidia_h100_overview,dhanuskodi2023confidential} avoid the four-lane GEMM cost but place the whole GPU and its firmware in the TCB.

\textbf{Physical and microarchitectural attacks.}
Probing~\cite{skorobogatov2017microprobing}, optical and other fault injection~\cite{skorobogatov2003optical,quadir2016survey}, and power or electromagnetic analysis~\cite{kocher1999differential} are outside \cref{thm:main} and can extract keys from an unhardened module. Faults matter more in the malicious setting: the bound $Q(2/p)^t$ presumes a correct check engine, so one glitch that forces acceptance bypasses it, and a fault in the field unit array can yield a wrong triple that carries valid tags. Software-controlled undervolting, which has induced such faults in SGX enclaves~\cite{murdock2020plundervolt}, is not physical: \cref{thm:main} assumes DVFS isolation (host software cannot drive the module's clock or voltage outside its safe operating range) and simulatable telemetry (\cref{sec:sec-assump}), whose realization we have not evaluated. Conversely, the module has no out-of-order core, no shared cache hierarchy and no host-managed page tables, so the controlled-channel, cache, transient-execution and Rowhammer attacks studied on general-purpose TEEs~\cite{xu2015controlled,shinde2015preventing,gotzfried2017cache,brasser2017software,lee2017inferring,van2018foreshadow,kim2014flipping} target mechanisms it lacks, and each check returns one generic status only after all $t$ lanes are aggregated. Small security chips have still shipped with exploitable flaws~\cite{moghimi2020tpm,han2018bad,butterworth2013bios}: a small TCB makes hardening tractable, but it does not replace hardening.

\textbf{Rollback and lifecycle.}
Ledger and epoch state live in volatile protected SRAM, so every reset falls under the reboot rule of \cref{sec:proto-ledger}. Because every failure poisons its epoch and aborted reservations never return to a free list (\cref{fig:ledger}), recovery always costs a new setup. Neither a monotonic service nor an erase-and-rekey lifecycle is implemented yet (\cref{tab:obligations}).

\textbf{Availability and fairness.}
\sys provides security with abort, the standard target for two-party computation with a malicious participant~\cite{hazay2010efficient,lindell2017simulate}. A corrupt host can withhold or reorder traffic, stall its GPU or abort at any public interaction boundary, and a corrupt recipient may obtain its output first; fairness and guaranteed output delivery are not claimed (S10 in \cref{tab:scenarios}). Aborts are, however, not a side channel on honest inputs. Apart from the validity predicates, which the modules evaluate before the first output opening and whose outcomes are the $\mathsf{status}$ part of $\Leak_C$ (\cref{def:leakage}), every \CheckOpen{} outcome depends only on the adversary's own deviation $(\bm{e},\bm{d}_j)$, the protected keys and the fresh challenges (\cref{thm:mac-sound}), and the first failure ends the epoch, so selective-failure and key-learning strategies cannot be iterated (\cref{lem:hidden-key}). Persistent denial of service remains a matter of deployment policy.

\textbf{Field versus ring.}
Over $\Fp$ with $p = 2^{61}-1$, \sys is not bit-identical to the $\Z_{2^{64}}$ arithmetic of Sigma and Orca~\cite{gupta2023sigma,jawalkar2024orca}. Ring-compiled models must be re-encoded under the numeric contract of \cref{sec:arch-field}, with magnitudes below $p/2$ before truncation, and exact signed truncation needs 307 authenticated multiplications on sequential carry chains, i.e., 309 rounds or \est{30.9~ms} on LAN (\cref{alg:bitdec,alg:trunc}), the most round-intensive gate in \cref{tab:gates}. A ring deployment needs a SPDZ2k-style backend~\cite{cramer2018spdz2k}, which is a separate design with a separate proof (\cref{sec:sec-concrete}).

\textbf{\ProfU.}
\ProfU (\cref{sec:threat-profileu}) is specified but not evaluated; it forfeits the local-dealer and generate-and-consume savings and must add the backend's key-privacy and answer-integrity arguments outside \cref{thm:main}.

\textbf{Model provenance.}
\sys proves correct evaluation on the inputs actually supplied (S9 in \cref{tab:scenarios}). A committed model (\cref{sec:threat-goals}) establishes provenance, not quality; the gap between the finite-field circuit and a floating-point model is an approximation question separate from cryptographic correctness.

\textbf{Artifact status.}
We executed a specification and a functional CPU reference model; GPU and RTL conformance, the protected runtime and deployment measurements have not been run yet (\cref{sec:eval-method,sec:eval-attack}). Every red value therefore awaits the three separate experiments of \cref{sec:arch-deploy}, and security measurements need two independent protected devices.


==> qa/draft3/sections/10_related.tex <==
% ==================================================================
% Section X: Related Work
% Owner labels: sec:related, tab:related
% ==================================================================
\section{Related Work}
\label{sec:related}

\begin{table*}[t]
\centering
\caption{Comparison of \sys with Representative Related Work}
\label{tab:related}
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{l c c c c l c c l}
\hline
\textbf{Work} & \textbf{Adversary} & \makecell{\textbf{Trusted}\\\textbf{HW}} & \makecell{\textbf{Trusted comp.}\\\textbf{sees plaintext}} & \makecell{\textbf{Custom}\\\textbf{HW}} & \textbf{Offline material} & \makecell{\textbf{Auth.\ FSS}\\\textbf{outputs}} & \makecell{\textbf{Verified}\\\textbf{openings}} & \textbf{Workloads} \\
\hline
Sigma~\cite{gupta2023sigma} & SH & \xmark & \xmark & \xmark$^{\mathrm{g}}$ & Dealer keys & \xmark & \xmark & Inference \\
Orca~\cite{jawalkar2024orca} & SH & \xmark & \xmark & \xmark$^{\mathrm{g}}$ & Dealer keys & \xmark & \xmark & Training, inference \\
Shark~\cite{gupta2025shark} & Mal & \xmark & \xmark & \xmark & Dealer, authenticated keys & \cmark & \cmark & Inference \\
\hline
MASCOT, MP-SPDZ~\cite{keller2016mascot,keller2020mpspdz} & Mal & \xmark & n/a & \xmark & Interactive (OT-based) & n/a & \cmark & General circuits \\
vFSS~\cite{decastro2022vfss} & Mal$^{\mathrm{a}}$ & \xmark & n/a & \xmark & Client keys, verified & \xmark & n/a & Key validation \\
APIR~\cite{colombo2023apir} & Mal$^{\mathrm{b}}$ & \xmark & n/a & \xmark & None (client query) & n/a & \cmark$^{\mathrm{b}}$ & PIR \\
\hline
Slalom~\cite{tramer2018slalom} & Mal$^{\mathrm{c}}$ & \cmark & \cmark & \xmark$^{\mathrm{g}}$ & n/a & n/a & \cmark$^{\mathrm{c}}$ & Inference \\
Aramis~\cite{kumar2020cryptflow} & Mal & \cmark$^{\mathrm{d}}$ & \xmark$^{\mathrm{d}}$ & \xmark & n/a & n/a & n/a & Inference \\
STAMP, PPMLAC~\cite{huang2022efficient,zhou2022ppmlac} & SH, Mal$^{\mathrm{e}}$ & \cmark & \pmark$^{\mathrm{e}}$ & \cmark & In trusted HW & n/a & \pmark$^{\mathrm{e}}$ & ML \\
\hline
GPU-DPF~\cite{lam2023gpu} & SH$^{\mathrm{i}}$ & \xmark & n/a & \xmark$^{\mathrm{g}}$ & None (client query) & \xmark & \xmark & PIR \\
DFA~\cite{dfa2026trusted} & SH$^{\mathrm{i}}$ & \pmark$^{\mathrm{f}}$ & \cmark$^{\mathrm{f}}$ & \cmark & Dealer or local$^{\mathrm{f}}$ & \xmark & \xmark & Inference, PIR \\
\hline
\textbf{\sys (this work)} & Mal$^{\mathrm{h}}$ & \cmark & \cmark$^{\mathrm{h}}$ & \cmark & Local, none shipped & \cmark & \cmark & Inference, PIR \\
\hline
\end{tabular}

\vspace{3pt}
\begin{minipage}{0.98\textwidth}
\footnotesize
SH: semi-honest; Mal: malicious (active) adversary. \emph{Trusted HW}: security relies on trusted hardware. \emph{Trusted comp.\ sees plaintext}: a trusted dealer, enclave or module sees inputs or intermediate values (FSS dealers are input independent). \emph{Custom HW}: dedicated hardware beyond commodity CPUs and GPUs. \emph{Offline material}: source of the per-query correlated randomness or keys. \emph{Auth.\ FSS outputs}: FSS gate outputs carry MAC tags. \emph{Verified openings}: opened values or untrusted results are checked before use. \cmark: yes; \xmark: no; \pmark: partial, optional or configuration dependent; n/a: not applicable. Lettered notes qualify the headline setting of each work.
$^{\mathrm{a}}$\,Malicious client key generator; servers check that keys are well formed, not that they are evaluated correctly.
$^{\mathrm{b}}$\,The client detects answers that are inconsistent with a public database digest.
$^{\mathrm{c}}$\,An SGX enclave outsources to an untrusted co-located GPU and checks its matrix products with Freivalds' algorithm.
$^{\mathrm{d}}$\,Relies on SGX integrity, not confidentiality.
$^{\mathrm{e}}$\,Settings differ between the two works: STAMP reports semi-honest and honest-majority malicious variants and evaluates nonlinear operations on unmasked values in its trusted processor; PPMLAC's trusted chipset mainly generates correlated randomness.
$^{\mathrm{f}}$\,Trusted mode only; the untrusted mode ships dealer keys.
$^{\mathrm{g}}$\,Implemented on commodity GPUs.
$^{\mathrm{h}}$\,Static corruption of one host, security with abort, under \ProfT, where the modules see inputs, openings and PIR indices; \ProfU delegates to an established malicious backend.
$^{\mathrm{i}}$\,In two-server DPF-PIR (GPU-DPF, DFA's untrusted mode), neither server learns the queried index, without relying on trusted hardware; SH refers to result integrity.
\end{minipage}
\end{table*}

\Cref{tab:related} summarizes the closest lines of work.

\textbf{FSS-based secure computation.}
FSS~\cite{boyle2015fss} and its tree-based DPF instantiations~\cite{gilboa2014distributed,boyle2016function} underlie a family of low-round two-party protocols with preprocessing~\cite{boyle2019preprocessing}. AriaNN~\cite{ryffel2020ariann} and Pika~\cite{wagh2022pika} first demonstrated private inference with FSS, Boyle et al.~\cite{boyle2021function} built comparisons, splines and fixed-point truncation from DCFs, Grotto~\cite{storrier2023grotto} replaced DCF-heavy constructions with DPF-based ones in a $(2{+}1)$-party setting, and Orca~\cite{jawalkar2024orca} and Sigma~\cite{gupta2023sigma} brought FSS-based training and GPT-class inference to GPUs. These systems are semi-honest and assume a dealer whose key material dominates the offline cost~\cite{huang2026beyond}. DPFs also underlie PIR, anonymous messaging, private queries and analytics, private heavy hitters, set intersection and distributed ORAM~\cite{corrigan2015riposte,wang2017splinter,dauterman2020dory,dauterman2022waldo,boneh2021lightweight,mouris2024plasma,garimella2024computation,vadapalli2023duoram,doerner2017scaling,ji2023multi}. Secure inference without FSS realizes nonlinear layers through share conversions, garbled circuits or homomorphic encryption~\cite{mohassel2017secureml,mohassel2018aby3,wagh2019securenn,wagh2020falcon,rathee2020cryptflow2,pang2024bolt,lu2023bumblebee}, typically with more interaction per layer.

\textbf{Malicious and verifiable FSS.}
To our knowledge, Shark~\cite{gupta2025shark} is the most directly comparable system: actively secure two-party FSS inference in which a trusted dealer supplies authenticated key material. Its security is cryptographic once its input-independent dealer, which never sees an input or an opening, is trusted, whereas each \sys module sees every input and opening under \ProfT (\cref{sec:eval-method}). In exchange, \sys generates the authenticated correlations locally and removes the offline distribution that dominates the dealer-based malicious FSS baseline, modeled after the protocol family of Shark~\cite{gupta2025shark} (\cref{tab:e2e}). Verifiable FSS~\cite{corrigan2015riposte,boyle2016function,boneh2021lightweight,decastro2022vfss} addresses a different adversary, a client that may submit malformed keys, which the servers detect; \sys instead treats key generation, evaluation, authentication and release as separate obligations.

\textbf{Malicious MPC preprocessing and MACs.}
Beyond the SPDZ-family tools of \cref{sec:bg-mal}, mixed-circuit preprocessing with edaBits~\cite{escudero2020edabits} and classical bit-decomposition and truncation protocols~\cite{damgard2006unconditionally,catrina2010improved} supply the conversions that nonlinear layers need, and honest-majority protocols~\cite{furukawa2017high,mohassel2018aby3,wagh2020falcon,dalskov2021fantastic} obtain malicious security from replicated sharing among three or four servers. \sys adopts, and does not claim as new, the SPDZ MAC algebra with $t$ independent keys over a Mersenne field. It replaces interactive preprocessing by correct generation inside the modules, in the spirit of hardware-assisted correlation generation~\cite{lu2021correlated,zhou2022ppmlac}, and checks openings on frozen bytes (\cref{sec:proto-check}).

\textbf{Trusted hardware for MPC and ML.}
Tamper-proof tokens are a classical setup assumption for universally composable computation~\cite{katz2007universally}, and commodity TEEs~\cite{costan2016intel,amd_sev,arm_trustzone,lee2020keystone} have been used to accelerate or simplify two-party computation and functional encryption~\cite{gupta2016using,choi2019hybrid,felsen2019secure,wuhybrid,fisch2017iron}. For ML, Ohrimenko et al.~\cite{ohrimenko2016oblivious} and Chiron~\cite{hunt2018chiron} execute learning tasks inside SGX enclaves; Slalom~\cite{tramer2018slalom} and DarKnight~\cite{hashemi2021darknight} outsource linear layers from an enclave to untrusted GPUs and verify them, with Freivalds' algorithm~\cite{freivalds1977probabilistic} and with redundant coded computation, respectively; and Aramis~\cite{kumar2020cryptflow} compiles semi-honest protocols into maliciously secure ones by relying on the integrity, but not the confidentiality, of SGX. GPU TEEs~\cite{volos2018graviton,jang2019heterogeneous} and confidential computing on H100~\cite{nvidia_h100_overview,dhanuskodi2023confidential} protect GPU computation from the host but place the whole GPU and its firmware in a TCB far larger than our module. Closest to our trust model, STAMP~\cite{huang2022efficient} and PPMLAC~\cite{zhou2022ppmlac} rely on a small security processor or a trusted chipset to execute nonlinear operations or generate correlated randomness, respectively, in the tradition of TPM-class security chips, secure coprocessors and smart cards~\cite{tpm2spec,googletitan,ibm4758,rankl2004smart}, and DFA~\cite{dfa2026trusted} uses a small module as a local FSS dealer. STAMP's nonlinear evaluation inside its trusted processor corresponds to our direct protected gate (\cref{sec:proto-direct}). Relative to it, \sys contributes a two-party setting with an untrusted GPU checked by MACs, freeze-before-challenge checking against host-controlled DMA, ledgered one-time randomness, and a malicious FSS and PIR datapath. Like Slalom and DarKnight, \sys keeps the GPU outside the boundary, but it uses Freivalds checks only for operands the GPU may already see (\cref{sec:proto-freivalds}).

\textbf{Hardware acceleration for private computation.}
GPU systems accelerate secret-sharing MPC~\cite{tan2021cryptgpu,watson2022piranha,crypten2020}, FSS~\cite{gupta2023sigma,jawalkar2024orca} and DPF-based PIR~\cite{lam2023gpu}. FPGA designs target secret-sharing MPC~\cite{wolfe2020secret,patel2020arithmetic,xu2025co}, Ironman~\cite{ironman2025} accelerates OT extension near memory, and FPGA and ASIC designs speed up the polynomial kernels of homomorphic encryption~\cite{riazi2020heax,reagen2021cheetah,samardzic2021f1,samardzic2022craterlake,kim2022bts}. These accelerators make a fixed protocol faster and inherit its adversary model. DFA~\cite{dfa2026trusted} additionally used trust to change the dataflow; \sys uses the same small trusted module to change the adversary model, which is why \cref{sec:eval} compares against security-matched baselines rather than raw kernel throughput alone.

\textbf{PIR with integrity.}
Authenticated PIR~\cite{colombo2023apir} lets a client detect answers that are inconsistent with a public database digest without trusted hardware, at additional server cost that our APIR-based GPU baseline reflects (\cref{tab:pir}). PIR with secure coprocessors~\cite{smith2001practical} and enclave-based oblivious storage such as Snoopy~\cite{dauterman2021snoopy} instead trust hardware that learns the query and hides its accesses through oblivious scans. The versioned-snapshot PIR of \sys follows this trust model: both modules learn the queried index $\alpha$, so its query privacy rests on module trust, unlike untrusted two-server DPF-PIR (GPU-DPF~\cite{lam2023gpu}, DFA's untrusted mode), which hides $\alpha$ from each server without trusted hardware. It scans in two role-bound modules, binds the exact consumed bytes to an authorized commitment $\mathsf{cm}_v$, optionally a Merkle root~\cite{merkle1987digital}, and releases freshly reshared answers only after the snapshot hash matches (\cref{sec:proto-pir}).

\textbf{Positioning.}
Each ingredient of \sys, from information-theoretic MACs and trusted correlation generation to verified GPU work and DPF acceleration, has precedents; our contribution is their composition in one small trusted module, proven stand-alone secure with abort in the ideal-module model of \cref{sec:threat-model} (\cref{tab:related}).


==> qa/draft3/sections/11_conclusion.tex <==
% ==================================================================
% Section XI: Conclusion (owner: sections/11_conclusion.tex)
% Labels defined here: sec:conclusion
% ==================================================================
\section{Conclusion}\label{sec:conclusion}

We presented \sys, a trusted hardware accelerator that secures FSS-based private inference and DPF-based PIR against a malicious host and GPU while keeping the key-movement savings of trusted DFA. Since a module acting as FSS dealer can also be the verifier, \sys generates authenticated correlations internally, authenticates DPF outputs with a fresh resharing epilogue instead of extra DPF trees, checks every opening on frozen bytes with $t=3$ independent MAC lanes over $\F_{2^{61}-1}$, and releases nothing before a role-bound one-time ledger records a verified check. These mechanisms protect the chain from authorized input to authorized output release; we prove stand-alone static malicious security with abort in a protected-module model, with statistical error about $2^{-148}$ for $2^{32}$ checked batches. Both modules see inputs and learn the PIR index, so PIR query privacy rests on module trust, unlike untrusted two-server DPF-PIR~\cite{lam2023gpu}. Our model estimates that \sys is \est{10.1--14.0$\times$} faster on a LAN than dealer-based malicious FSS modeled after the protocol family of Shark~\cite{gupta2025shark}, mainly because in-module generation removes \est{21.8--563~GB} of per-query offline distribution (\est{1.5--1.8$\times$} excluding it). Malicious security costs \est{2.5--3.5$\times$} LAN latency over semi-honest DFA and \est{0.145~mm$^2$} at 7~nm (pre-synthesis).

We executed a specification and a functional CPU reference model; GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet, so no \sys performance number is measured. Three directions follow. First, these measurements, synthesis and on-die simulation must replace the estimates. Second, a \ProfU backend would run the same compiled circuit when the hardware is adversarial, and a SPDZ2k-style backend would cover the ring $\Z_{2^{64}}$. Third, compressed MAC checks that avoid carrying all tag lanes through the GPU would cut the now-dominant authenticated linear algebra; a vetted DCF faster than our $O(n^2)$ one would help FSS-only configurations, not the compiler-selected default, where nonlinear gates take \est{3.4\%} of BERT-Base latency. Both need proofs this paper does not provide.

\section*{Acknowledgment}
Omitted for anonymous review.


==> qa/draft4/macros.tex <==
% ------------------------------------------------------------------
% Shared packages and macros for the TIFS manuscript.
% Every section/appendix/algorithm/table file relies ONLY on these.
% ------------------------------------------------------------------
\usepackage[T1]{fontenc}
\usepackage{amsmath,amssymb,amsfonts,mathtools}
\usepackage{amsthm}
\usepackage{bm}
\usepackage{graphicx}
\usepackage[dvipsnames,table]{xcolor}
\usepackage{multirow}
\usepackage{makecell}
\usepackage{array}
\usepackage{tabularx}
\usepackage{algorithm}
\usepackage[noend]{algpseudocode}
\usepackage{setspace}
\let\labelindent\relax
\usepackage[inline]{enumitem}
\usepackage{pifont}
\usepackage{xspace}
\usepackage{stmaryrd}
\usepackage{cite}
\usepackage[hidelinks]{hyperref}
\usepackage[capitalise,noabbrev]{cleveref}

% ---------------- cross-reference names (IEEE style) ----------------
\crefname{section}{Section}{Sections}
\Crefname{section}{Section}{Sections}
\crefname{subsection}{Section}{Sections}
\Crefname{subsection}{Section}{Sections}
\crefname{subsubsection}{Section}{Sections}
\Crefname{subsubsection}{Section}{Sections}
\crefname{appendix}{Appendix}{Appendices}
\Crefname{appendix}{Appendix}{Appendices}
\crefname{figure}{Fig.}{Figs.}
\Crefname{figure}{Fig.}{Figs.}
\crefname{table}{Table}{Tables}
\Crefname{table}{Table}{Tables}
\crefname{algorithm}{Algorithm}{Algorithms}
\Crefname{algorithm}{Algorithm}{Algorithms}
\crefname{equation}{Eq.}{Eqs.}
\Crefname{equation}{Eq.}{Eqs.}
\crefname{ALC@unique}{line}{lines}
\crefname{theorem}{Theorem}{Theorems}
\crefname{lemma}{Lemma}{Lemmas}
\crefname{corollary}{Corollary}{Corollaries}
\crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Assumption}{Assumptions}
\crefname{remark}{Remark}{Remarks}
\crefname{proposition}{Proposition}{Propositions}

% ---------------- theorem environments ----------------
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{proposition}{Proposition}
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\theoremstyle{remark}
\newtheorem{remark}{Remark}

% ---------------- algorithm style (FuseFSS / DFA hybrid) ----------------
\algrenewcommand\algorithmicrequire{\textbf{Input:}}
\algrenewcommand\algorithmicensure{\textbf{Output:}}
\algnewcommand{\LineComment}[1]{\State \(\triangleright\) \textit{#1}}
\algnewcommand{\Abort}{\textbf{abort}}
\newcommand{\algstretch}{\setstretch{0.92}}

% ---------------- estimates: RED, to be replaced by measured values ----------------
\newcommand{\est}[1]{\textcolor{red}{#1}}

% ---------------- names ----------------
\newcommand{\sys}{VIGOR-DFA\xspace}
\newcommand{\DFA}{DFA\xspace}
\newcommand{\ProfT}{Profile~$\mathsf{T}$\xspace}
\newcommand{\ProfU}{Profile~$\mathsf{U}$\xspace}

% ---------------- algebra ----------------
\newcommand{\F}{\mathbb{F}}
\newcommand{\Fp}{\mathbb{F}_p}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\bits}[1]{\{0,1\}^{#1}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\getsr}{\xleftarrow{\$}}
\newcommand{\inner}[2]{\langle #1, #2\rangle}
\newcommand{\auth}[1]{[#1]}                  % authenticated sharing
\newcommand{\authb}[2]{[#1]_{#2}}            % party-b tuple (x_b, gamma_{b,1..t})
\newcommand{\tagv}[3]{\gamma_{#1,#2}^{(#3)}} % optional explicit tag notation

% ---------------- FSS objects ----------------
\newcommand{\Gen}{\mathsf{Gen}}
\newcommand{\Eval}{\mathsf{Eval}}
\newcommand{\EvalAll}{\mathsf{EvalAll}}
\newcommand{\DPF}{\mathsf{DPF}}
\newcommand{\DCF}{\mathsf{DCF}}
\newcommand{\CW}{\mathsf{CW}}
\newcommand{\CWout}{\mathsf{CW}^{\mathrm{out}}}
\newcommand{\sCW}{s^{\mathsf{CW}}}
\newcommand{\tCW}[1]{t^{\mathsf{CW},#1}}
\newcommand{\PRG}{G}
\newcommand{\Conv}{H}
\newcommand{\keep}{\mathit{keep}}
\newcommand{\lose}{\mathit{lose}}

% ---------------- crypto ----------------
\newcommand{\PRF}{\mathsf{PRF}}
\newcommand{\KDF}{\mathsf{KDF}}
\newcommand{\Hash}{\mathsf{Hash}}
\newcommand{\AEAD}{\mathsf{AEAD}}
\newcommand{\Adv}{\mathcal{A}}
\newcommand{\Sim}{\mathcal{S}}
\newcommand{\Env}{\mathcal{Z}}
\newcommand{\View}{\mathsf{View}}
\newcommand{\Real}{\mathsf{Real}}
\newcommand{\Ideal}{\mathsf{Ideal}}
\newcommand{\Hyb}[1]{\mathsf{H}_{#1}}
\newcommand{\Leak}{\mathcal{L}}
\newcommand{\FC}{\mathcal{F}^{\mathrm{abort}}_{C,\mu}}
\newcommand{\FPIR}{\mathcal{F}^{\mathrm{abort}}_{\mathrm{PIR}}}
\newcommand{\eps}[1]{\epsilon_{\mathsf{#1}}}
\newcommand{\negl}{\mathsf{negl}}

% ---------------- protocol / ledger / commands ----------------
\newcommand{\cmd}[1]{\texttt{\detokenize{#1}}}
\newcommand{\lstate}[1]{\textsf{#1}}
\newcommand{\algname}[1]{\textsf{#1}}
\newcommand{\CheckOpen}{\algname{CheckOpen}\xspace}
\newcommand{\AuthShare}{\algname{AuthShare}\xspace}
\newcommand{\Epilogue}{\algname{Epilogue}\xspace}

% ---------------- marks for tables ----------------
\newcommand{\cmark}{\ding{51}}
\newcommand{\xmark}{\ding{55}}
\newcommand{\pmark}{\ding{109}}   % partial


==> qa/draft4/sections/00_abstract.tex <==
% ==================================================================
% Abstract and index terms (owner: sections/00_abstract.tex)
% Red values are model estimates (\est{}); see Appendix F.
% ==================================================================
\begin{abstract}
Function secret sharing (FSS) underlies two-party private inference and private information retrieval, with cost dominated by generating, moving and evaluating distributed point function (DPF) keys. A trusted GPU-integrated distributed function accelerator (DFA) removed key movement by generating and consuming keys locally, but tolerates only semi-honest adversaries. A malicious host or GPU can tamper with shares, replay one-time material, swap buffers after checking, request early outputs, or abuse the accelerator as a forgery oracle, while malicious FSS ships large authenticated keys or multiplies DPF work. We present \sys, protecting the chain from authorized input to authorized output release with three mechanisms: a fresh authentication epilogue using three field multiplications per DPF output, \est{3.8--4.0$\times$} faster per gate than per-lane DPF tag trees; a freeze-before-challenge check of every opening with $t=3$ independent MAC lanes over $\F_{2^{61}-1}$; and a role-bound one-time resource ledger with a release guard, in a protected datapath beside the GPU L2 cache. We prove stand-alone static malicious security with abort in a protected-module model, with statistical error $Q(2/p)^t\approx 2^{-148}$ for $Q\le 2^{32}$ checked batches. Our DFA-calibrated model estimates that, against dealer-based malicious FSS modeled after the protocol family of Shark, \sys removes \est{21.8--563~GB} of per-query offline authenticated material and, mainly by generating it in-module, lowers LAN latency by \est{10.1--14.0$\times$} (\est{1.5--1.8$\times$} excluding offline distribution) and energy by \est{3.0--3.9$\times$}. Malicious security costs \est{2.5--3.5$\times$} LAN latency over semi-honest DFA and \est{0.145~mm$^2$} at 7~nm. We executed a specification and a functional CPU reference model; GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet.
\end{abstract}

\begin{IEEEkeywords}
Distributed point function, function secret sharing, hardware accelerator, malicious security, private information retrieval, secure inference, trusted hardware.
\end{IEEEkeywords}


==> qa/draft4/sections/01_introduction.tex <==
% ==================================================================
% Section I: Introduction (owner: sections/01_introduction.tex)
% Labels defined here: sec:intro
% Red (\est{}): model outputs, assumed parameters. Black: cited DFA
% values, design constants, analytical counts, executed tests.
% ==================================================================
\section{Introduction}\label{sec:intro}

\IEEEPARstart{P}{rivacy}-preserving computation is moving into deployments where data are both valuable and regulated: hospitals running diagnostic models on records they may not export, cloud providers serving proprietary models to clients who will not reveal their queries, and lookup services whose queries disclose a user's interests. Secure two-party computation (2PC) for private machine-learning (ML) inference~\cite{yao1986generate,goldreich2019play,mohassel2017secureml,rathee2020cryptflow2} and private information retrieval (PIR)~\cite{chor1998private,angel2018pir} address these settings with cryptographic rather than contractual guarantees. Function secret sharing (FSS)~\cite{boyle2015fss,boyle2016function} has become one of the most effective building blocks for both. In FSS-based private inference, the parties open a masked input $x+r$ and evaluate one-time keys for the gate function shifted by the mask, so that a nonlinear layer often costs a single online round~\cite{boyle2021function,gupta2023sigma,jawalkar2024orca}. In two-server PIR, the client splits a point function into two short keys and each server evaluates its key over the entire database~\cite{gilboa2014distributed,wang2017splinter,lam2023gpu}.

The price of this online efficiency is paid in distributed point function (DPF) work. Every comparison, lookup table and interval test in an FSS-compiled model is built from DPFs or from the distributed comparison functions (DCFs) derived from them~\cite{boyle2021function,storrier2023grotto,gupta2023sigma}, and each key is used once. A dealer must therefore generate, ship and store fresh keys for every nonlinear element of every query: 17.1~GB of offline material for a single BERT-Base inference~\cite{dfa2026trusted}, a cost that cannot always be hidden behind the online phase~\cite{huang2026beyond}. PIR, conversely, is dominated by full-domain DPF evaluation, which is AES-bound even on a modern GPU~\cite{lam2023gpu}. The distributed function accelerator (DFA)~\cite{dfa2026trusted} attacked both costs with a small DPF engine integrated next to the GPU L2 cache. In its trusted mode, a protected module in each server attests to its peer, establishes a shared key and plays the dealer locally: it generates its own party's key share on demand and consumes each correction word as soon as it is produced (\emph{generate-and-consume}, GaC), so keys are never distributed, stored or reread. For BERT-Base, trusted DFA reduces LAN latency from 18.8~s to 1.42~s and offline communication from 17.1~GB to 0.1~GB; for PIR, DFA in its untrusted mode (client-generated keys) raises throughput by $5.05\times$ for $2^{20}$ records~\cite{dfa2026trusted}.

\textbf{The semi-honest boundary.}
DFA, like Sigma~\cite{gupta2023sigma}, Orca~\cite{jawalkar2024orca} and most GPU-based FSS systems, is secure only against semi-honest adversaries: it assumes that both servers run the prescribed code. In a real deployment, however, the components easiest to subvert are those around the small protected module: the host operating system, the GPU driver and runtime, the GPU kernels, the direct memory access (DMA) buffers and the network stack. They hold the whole data path, and attacks on privileged software and firmware~\cite{xu2015controlled,butterworth2013bios,han2018bad} and GPU isolation designs~\cite{volos2018graviton,jang2019heterogeneous} alike treat them as potentially adversarial. With its module intact, a single compromised server host can still mount at least five classes of attacks against semi-honest trusted acceleration (\cref{fig:scenarios}):
(i)~\emph{additive errors} on shares, openings or GPU products, which bias results and leak through selective failure;
(ii)~\emph{replay or reset} of masks, counters or module state;
(iii)~\emph{check-to-use} buffer swaps;
(iv)~abuse of a naive ``authenticate'' command as a \emph{forgery oracle}; and
(v)~\emph{premature} output requests.
Remote attestation does not close these gaps. It proves which code and configuration run inside the module; it does not prove that the untrusted GPU used a valid key, computed the right product, or released an authorized result.

\textbf{Why existing malicious routes are costly.}
FSS can be made maliciously secure, but the known routes give back much of what trusted acceleration gained. Actively secure FSS inference such as Shark~\cite{gupta2025shark} keeps an external dealer that ships authenticated keys and correlated randomness. For dealer-based malicious FSS modeled after the protocol family of Shark (\cref{app:model}), we estimate \est{37.6~GB} of offline material per BERT-Base query, \est{2.2$\times$} the semi-honest 17.1~GB~\cite{dfa2026trusted}, and a LAN latency of \est{43.9~s} of which \est{37.6~s} is distribution. Dealer-free malicious preprocessing in the SPDZ family~\cite{damgard2012spdz,keller2016mascot,keller2018overdrive,cramer2018spdz2k} replaces the dealer by oblivious-transfer (OT) or homomorphic-encryption triple generation, and pseudorandom correlation generators (PCGs) with silent OT~\cite{boyle2019pcg,boyle2020pcg} compress the communication of authenticated triples at a substantial computational cost. Neither yields FSS keys: generating DPF keys without a dealer requires a secure two-party evaluation of key generation with a round per tree level~\cite{doerner2017scaling}, so dealer-free malicious FSS keeps a preprocessing cost far above its online cost. Two recent dealerless designs attack this cost from the hardware side and from the protocol side: KORD~\cite{peng2026kord} co-designs a dealerless key-generation protocol with paired, mutually attested chips that reconstruct FSS keys without a dealer, and VeriFSS~\cite{xue2026verifss} obtains active security for dealer-free two-party FSS by binding the generation transcript, the computed function and the evaluation shares to a single execution; \sys instead keeps a trusted local dealer and extends integrity from key generation to the untrusted GPU and the output release. Verifiable FSS (vFSS)~\cite{decastro2022vfss} lets servers check that client-generated DPF keys are well formed, but not that an untrusted GPU evaluates them, or the arithmetic around the gate, correctly. Finally, the direct way to authenticate an FSS output inside an accelerator, one additional DPF tree with payload $\Delta_j\beta$ per message authentication code (MAC) lane, multiplies pseudorandom generator (PRG) work by $1+t$ for $t$ lanes. One tree with a $(1+t)$-element payload avoids most of this cost, but it widens every output correction and exports tag shares whose hiding rests on DPF key privacy.

\textbf{Our key insight} is that a module that already plays the FSS dealer can also be the verifier. Because it knows every correlation it generates, it can (1)~generate \emph{authenticated} correlations (input masks, Beaver triples~\cite{beaver1991efficient} and DPF keys) locally at zero network cost, computing every triple product correctly inside its own boundary; (2)~authenticate its own FSS outputs with a fresh resharing epilogue instead of extra DPF trees, because it already holds the raw output shares and the MAC key material; and (3)~check every opening on bytes it has frozen before any challenge exists, so that the GPU remains a fast but untrusted linear-algebra engine whose results are only candidates until verified. What must be protected is thus not a single primitive but an integrity chain:
\begin{center}
\small
\emph{authorized input} $\rightarrow$ \emph{correlated preprocessing} $\rightarrow$ \emph{correct local evaluation} $\rightarrow$ \emph{authenticated arithmetic} $\rightarrow$ \emph{consistent opening} $\rightarrow$ \emph{authorized output release.}
\end{center}
Each link has a concrete failure mode under a malicious host, and each needs its own mechanism. \Cref{fig:flows} places the resulting execution flow next to the semi-honest GPU baseline, trusted DFA and dealer-based malicious FSS.

\textbf{This work.}
We present \sys (Verified Integrity-Gated On-demand Randomness DFA), the malicious-secure successor of trusted DFA. It keeps DFA's placement beside the GPU L2 cache, its local key generation and its generate-and-consume execution. Under \ProfT (\cref{sec:threat}) a malicious adversary statically corrupts at most one host, and every secret value on a host is an authenticated share over $\Fp$, $p=2^{61}-1$, with $t=3$ SPDZ-style MAC lanes~\cite{damgard2012spdz,damgard2013practical} (32~bytes per element and party). Three mechanisms carry the design; we claim their composition, not any of them as an unprecedented primitive. The \emph{fresh authentication epilogue} turns each raw DPF output share into a freshly padded authenticated tuple at three field multiplications and four pads (\cref{sec:proto-epilogue}). It matches the PRG cost of a single vector-payload tree, makes every exported tuple exactly uniform, and leaves no command that authenticates a host-supplied value. \emph{Freeze-before-challenge} \CheckOpen{} derives independent per-lane challenges only after both modules have frozen the exact submitted bytes, and later consumes exactly those bytes. A \emph{role-bound one-time ledger} labels all randomness by session, epoch, gate and purpose and poisons the epoch on any failure, and its \emph{release guard} lets no output leave a module before the corresponding check is \lstate{VERIFIED}.

\textbf{Scope and limits.}
\sys relocates trust to the modules rather than removing it. The modules see inputs under \ProfT, and both learn the PIR index, so PIR query privacy in \sys rests on module trust, unlike untrusted two-server DPF-PIR~\cite{lam2023gpu} and DFA's untrusted mode, which hide the index without trusted hardware. Physical attacks, leakage beyond the stipulated observable-trace model and rollback without a trusted monotonic service are out of scope, and security holds with abort, without fairness (\cref{sec:discussion}). Once the epilogue removes tag trees, the dominant cost of malicious security moves to four-lane authenticated linear algebra on the GPU and to the doubled round count (\cref{sec:analysis}).

\textbf{Why keep FSS inside a trusted module?}
Under \ProfT a module that has verified $c=x+r$ also holds $r$, so FSS adds no formal confidentiality over evaluating the gate directly (\cref{sec:proto-direct}). The end-to-end gains of \sys come from generating and consuming authenticated correlations inside the modules, not from FSS evaluation: in our model direct-only compilation (\est{3.82~s} for BERT-Base) is marginally faster than the compiler-selected default (\est{3.83~s}), which keeps an FSS realization for gate shapes marked FSS-portable, and nonlinear gates take only \est{3.4\%} of the latency. We keep a malicious FSS datapath for three reasons: the same compiled circuit, including masked-input FSS gates from existing toolchains~\cite{gupta2023sigma,jawalkar2024orca}, runs under the key-exporting \ProfU (specified, not evaluated or proven); PIR and small lookup tables are full-domain, data-independent scans that match the pipelined AES engines; and long-lived evaluation state holds only seeds and correction words, keeping input-dependent state short-lived as defense in depth, not as a formal claim. On FSS gates the epilogue is \est{3.8--4.0$\times$} faster than per-lane tag trees, although tag trees would raise the BERT-Base LAN latency by only \est{8\%}.

This paper makes the following contributions:
\begin{itemize}[leftmargin=*]
    \item \textbf{Malicious Threat Analysis.}
    We systematize how a malicious host or GPU attacks semi-honest trusted FSS acceleration into ten scenarios, S1 to S10 (\cref{fig:scenarios,tab:scenarios}), from share tampering to PIR snapshot substitution. For S1 to S8 we show why semi-honest trusted DFA fails and which \sys mechanism and theorem stop it; for S9 (input substitution) and S10 (denial of service and selective abort) we make explicit what the ideal functionality permits or does not prevent.

    \item \textbf{Protocol Co-Design.}
    We specify the three mechanisms above, the authenticated $\Fp$ representation and malicious generate-and-consume with explicit generator and evaluator states (\cref{sec:protocol}). On top of them we build authenticated lookup-table, interval, polynomial and direct protected gates, exact comparison and truncation, a refactoring rule that preserves the joint (not only the marginal) distribution of DFA's decoupled preprocessing, and versioned-snapshot PIR whose query privacy rests on module trust.

    \item \textbf{Hardware Architecture.}
    We design a protected datapath beside the GPU L2 cache (\cref{sec:arch}) with a ledger, page freezer, joint pseudorandom-function (PRF) sampler, DPF generation and evaluation contexts, a 128-lane Mersenne-61 field unit array, a check engine, a peer-channel controller and a release guard, whose 64 AES engines are time-shared among PRG expansion, challenge derivation and authenticated-encryption (AEAD) freezing. The additions cost \est{0.145~mm$^2$} and \est{0.508~W} at 7~nm, and the entire \sys occupies \est{0.046\%} of the A100 die.

    \item \textbf{Security Analysis.}
    We give ideal functionalities with explicit leakage and a hybrid proof with an explicit simulator of stand-alone static malicious security with abort under sequential composition (\cref{sec:security}, \cref{thm:main}), with advantage at most $\eps{setup}+\eps{prf}+\eps{channel}+\eps{bind}+\eps{trace}+Q(2/p)^t$, where the last term is about $2^{-148}$ for $Q\le 2^{32}$ checked batches. We show why shared challenges across lanes and the ring $\Z_{2^{64}}$ break this bound, and we separate what is proved from the implementation obligations that remain (\cref{tab:obligations}).

    \item \textbf{Evaluation.}
    With an analytical model calibrated on DFA (\cref{sec:eval}, \cref{tab:e2e}), we estimate that in-module generation of authenticated correlations cuts offline communication from \est{37.6~GB} to \est{under 1~MB} per BERT-Base query. Against dealer-based malicious FSS modeled after the protocol family of Shark, \sys is \est{11.4$\times$} faster on a LAN, or \est{1.6$\times$} excluding per-query offline distribution; with no authenticated-key blow-up the dealer-based pipeline still needs \est{22.4~s}, \est{5.8$\times$} that of \sys. Malicious security costs \est{2.7$\times$} LAN latency over semi-honest trusted DFA for BERT-Base, mostly for four-lane linear algebra, yet \sys stays \est{4.3--6.1$\times$} faster than the semi-honest GPU-only pipeline across four models. We executed a specification and a functional CPU reference model, which covers every algorithm except the optional Freivalds check and passes all 22 unit tests (\cref{sec:eval-attack}); GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet, and six injections of \cref{tab:attacks}, including the release guard, lack executed evidence.
\end{itemize}

Throughout, red values are outputs or assumed parameters of our analytical model (\cref{app:model}) that await measurement; black values are reproduced from DFA~\cite{dfa2026trusted}, are design constants or analytical counts, or come from executed reference tests.

\Cref{sec:bg,sec:threat,sec:analysis} give background, the threat model and where the cost of malicious FSS goes; \cref{sec:protocol,sec:arch,sec:security,sec:eval} present the protocol, architecture, security analysis and evaluation; \cref{sec:discussion,sec:related,sec:conclusion} discuss limitations, related work and conclusions, and the appendices give the ideal functionalities, proofs and performance model.


==> qa/draft4/sections/02_background.tex <==
% ==================================================================
% Section II: Background
% Owner labels: sec:bg, sec:bg-fss, sec:bg-pi, sec:bg-pir, sec:bg-dfa,
%               sec:bg-mal, fig:flows, eq:dpf, eq:pir
% ==================================================================
\section{Background}
\label{sec:bg}

This section reviews the primitives that \sys builds on and the semi-honest DFA design~\cite{dfa2026trusted} that it extends.
We write $P_0,P_1$ for the two computing parties, $b\in\{0,1\}$ for a party index, $\lambda$ for the seed length of the pseudorandom generator (PRG), and $\one[\cdot]$ for the indicator of a predicate.

% ==================================================================
\subsection{Function Secret Sharing, DPF, and DCF}
\label{sec:bg-fss}

\textbf{Function secret sharing.}
A two-party function secret sharing (FSS) scheme~\cite{boyle2015fss,boyle2016function} for a function class $\mathcal{F}$ with output group $\mathbb{G}$ consists of $\Gen(1^\lambda,\hat f)$, which maps a description of $f\in\mathcal{F}$ to a key pair $(k_0,k_1)$, and $\Eval(k_b,x)$, which returns party $b$'s share $y_b\in\mathbb{G}$.
Correctness requires $\Eval(k_0,x)+\Eval(k_1,x)=f(x)$ for every $x$; security requires that each key alone be simulatable from public information (domain, output group, function class), so that a single key hides $f$.

\textbf{Distributed point function.}
A distributed point function (DPF)~\cite{gilboa2014distributed,boyle2015fss,boyle2016function} shares the point function $f_{\alpha,\beta}$ with target $\alpha\in\bits{n}$ and payload $\beta\in\mathbb{G}$:
\begin{equation}\label{eq:dpf}
\Eval(k_0,x)+\Eval(k_1,x)=\beta\cdot\one[x=\alpha]\quad\text{for all } x\in\bits{n}.
\end{equation}
In this paper $\mathbb{G}=\Fp$ with $p=2^{61}-1$ (\cref{sec:proto-repr}), inputs are read most-significant bit first, and we use the tree-based construction of Boyle et al.~\cite{boyle2016function}.
Each node of a depth-$n$ binary tree carries a state $(s,t)$ of a $\lambda$-bit seed and a control bit; a fixed PRG $\PRG:\bits{\lambda}\rightarrow(\bits{\lambda}\times\bits{})^2$ expands a seed into the states of its two children, and $\Conv:\bits{\lambda}\rightarrow\Fp$ converts a leaf seed into a field element.
Generation walks the target path from two independent root seeds with control bits $t_0=0$ and $t_1=1$; each level's correction word $\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$ makes both parties' states identical on the child leaving the path and keeps them pseudorandom with opposite control bits on the child staying on it, and an output correction $\CWout$ makes the signed outputs $y_b=(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$ sum to $\beta$ at $x=\alpha$ and cancel elsewhere.
Party $b$'s key holds its root seed, its fixed control bit $t_b^{(0)}=b$, the $n$ correction words and $\CWout$, i.e., $O(\lambda n)$ bits; \cref{alg:gen,alg:eval} in \cref{sec:analysis-dpf} give the exact algorithms.

\textbf{Evaluation patterns and cost.}
Generation expands $2n$ states and a single-path $\Eval(k_b,x)$ expands $n$; a full-domain $\EvalAll(k_b)$ expands $2^n-1$ internal nodes, keeping only $O(n)$ pending siblings in a depth-first traversal.
The PRG dominates all patterns; DFA, GPU-DPF~\cite{lam2023gpu} and \sys instantiate it with AES-128.
Two properties matter later.
Keys are \emph{one-time}: each encodes one mask or query index, and reusing a mask reveals the difference of the two inputs it hides.
DPF key privacy holds for \emph{arbitrary} $(\alpha,\beta)$~\cite{boyle2016function}, so uniform targets come from the application's masking (\cref{sec:bg-pi}), whose joint distribution any refactoring of generation must preserve (\cref{sec:proto-refactor}).

\textbf{Distributed comparison function.}
A distributed comparison function (DCF) shares $f^{<}_{\alpha,\beta}(x)=\beta\cdot\one[x<\alpha]$.
We use this ``$<$'' orientation throughout; DFA~\cite{dfa2026trusted} uses ``$>$'', and we convert explicitly at interfaces via $\beta\cdot\one[x>\alpha]=\beta-f^{<}_{\alpha+1,\beta}(x)$, treating the threshold $2^n$ as a public constant.
Optimized DCFs evaluate with $O(n)$ PRG expansions~\cite{boyle2021function}, and DCFs can be assembled from DPFs~\cite{storrier2023grotto}.
\sys uses the conservative $O(n^2)$ DCF of \cref{alg:dcf}, which sums $n$ prefix DPFs and whose correctness \cref{thm:dcf} proves (\cref{app:proof-dpf}).

% ==================================================================
\subsection{FSS-Based Private Inference}
\label{sec:bg-pi}

\textbf{Two-party secure inference.}
Private inference runs a neural network with private input, and possibly private weights, as a secure two-party computation~\cite{yao1986generate,goldreich2019play,mohassel2017secureml,rathee2020cryptflow2,crypten2020,tan2021cryptgpu,watson2022piranha}.
With additive shares $x=x_0+x_1$, linear operations are local, and a multiplication consumes a Beaver triple $(a,b,c=ab)$~\cite{beaver1991efficient}: the parties open $d=x-a$ and $e=y-b$ and locally compute shares of $xy=c+db+ea+de$.
Nonlinear layers (ReLU, GeLU, Softmax, LayerNorm) dominate the cost; earlier systems use multi-round Boolean conversions for them~\cite{demmler2015aby,mohassel2018aby3,wagh2019securenn,wagh2020falcon}.

\textbf{Masked-input FSS gates.}
FSS-based systems~\cite{boyle2019preprocessing,boyle2021function,ryffel2020ariann,wagh2022pika,gupta2023sigma,jawalkar2024orca} evaluate each nonlinear gate $g$ in the masked-input paradigm.
Offline, a dealer samples a fresh uniform mask $r$, shares it, and generates FSS keys for the offset function $g_r(c)=g(c-r)$, often with an output mask.
Online, the parties open $c=x+r$, which is uniform and independent of $x$, and the outputs $\Eval(k_b,c)$ are shares of $g(x)$.
Comparisons and ReLU use DCFs; splines for GeLU, exponentials and inverse square roots use DCF-based interval selection plus low-degree polynomials; and small lookup tables (LUTs) use DPFs~\cite{gupta2023sigma,jawalkar2024orca}.
Each gate costs one opening round, so the online phase is round-efficient but compute-intensive.

\textbf{Offline cost and the dealer assumption.}
The price is paid offline.
Semi-honest FSS inference of BERT-Base with 128 tokens moves 17.1~GB of one-time key material per query and LLaMA2-7B moves 256~GB, more than 90\% of it DPF keys~\cite{dfa2026trusted}; this cost cannot always be hidden behind online work, and its energy and monetary cost is never hidden~\cite{huang2026beyond}.
Sigma, Orca, and related systems~\cite{gupta2023sigma,jawalkar2024orca,crypten2020} obtain keys from a trusted dealer and assume semi-honest computing parties.

% ==================================================================
\subsection{DPF-Based Private Information Retrieval}
\label{sec:bg-pir}

PIR lets a client retrieve record $D[\alpha]$ of an $N$-record database $D$ without revealing $\alpha$~\cite{chor1998private}.
Single-server schemes rely on homomorphic encryption and are computationally heavy~\cite{angel2018pir,henzinger2023one}; we focus on the faster two-server DPF-based schemes~\cite{gilboa2014distributed,boyle2016function}.
With $n=\lceil\log_2 N\rceil$, the client sends $k_b$ of $(k_0,k_1)\leftarrow\Gen(1^\lambda,\alpha,1)$ to server $P_b$, which returns
\begin{equation}\label{eq:pir}
y_b=\sum_{x=0}^{N-1}\Eval(k_b,x)\cdot D[x],\qquad b\in\{0,1\},
\end{equation}
and by \cref{eq:dpf} the client obtains $D[\alpha]=y_0+y_1$.
Keys have $O(\lambda\log N)$ bits, but each query costs $O(N)$ PRG expansions plus an $N$-term inner product per server, and the expansion dominates even on GPUs~\cite{lam2023gpu}.
Standard DPF-based PIR protects the index but not the answer: a malicious server can add an offset $\delta$ to $y_b$, so that the client accepts $D[\alpha]+\delta$, or answer from a stale database.
Conversely, a malicious client can submit a malformed key pair that reconstructs a combination of several records, which verifiable DPFs detect~\cite{decastro2022vfss}.
Authenticated PIR (APIR)~\cite{colombo2023apir} lets the client verify answers against a database digest at additional server cost.
\Cref{sec:proto-pir} gives our protected versioned-snapshot design, in which both modules learn $\alpha$: unlike untrusted two-server DPF-PIR, its query privacy rests on module trust.

% ==================================================================
\subsection{Trusted DFA}
\label{sec:bg-dfa}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_flows.pdf}
    \caption{Execution flows of two-party FSS-based private inference in four configurations, from left to right.
    (1)~GPU without DFA (semi-honest): a trusted party generates FSS keys offline and ships them over the network; each party stores them, rereads them and transfers them to its GPU.
    (2)~Trusted DFA (semi-honest)~\cite{dfa2026trusted}: after a one-time initialization with attestation and key exchange, each on-die module generates its party's keys locally and merges generation with evaluation (generate-and-consume), removing the offline phase.
    (3)~Dealer-based malicious FSS, modeled after the protocol family of Shark~\cite{gupta2025shark}: the dealer also issues authenticated keys and triples, so about \est{2.2$\times$} as much offline material (red: model estimate, \cref{app:model}) must be shipped, stored and reread, while the GPU runs authenticated general matrix multiplication (GEMM) and checks MACs online.
    (4)~\sys (malicious): the protected module (red dashed trusted boundary) keeps local generation and generate-and-consume, adds the fresh authentication epilogue, freeze-before-challenge \CheckOpen{} and the release guard, and exchanges authenticated shares $\authb{x}{b}$ with a GPU that runs authenticated linear algebra on one value lane and three MAC-tag lanes; the inter-party network carries opened values and check residuals, not keys.}
    \label{fig:flows}
\end{figure*}

\textbf{Hardware.}
DFA~\cite{dfa2026trusted} integrates 16 DPF units with four pipelined AES-128 engines each (64 in total) next to the L2 slices of a GPU; each 20-stage unit sustains one Gen or Eval iteration per cycle after warm-up.
An SC300-class control core~\cite{st33tpm12spi,arm_cortex_m3} handles attestation and key management, and a 16-lane vector unit~\cite{cavalcante2019ara} runs protocol-specific pre- and post-processing.
The design runs at 720~MHz in 28~nm, delivers about 290~GB/s of DPF output in Accel-Sim~\cite{khairy2020accel}, and traverses full-domain trees depth-first, needing $O(nm)$ state for $m$ units instead of $O(2^n)$~\cite{dfa2026trusted}.

\textbf{Untrusted and trusted modes.}
In the \emph{untrusted mode}, DFA only expands seeds for keys produced elsewhere, and the protocol is unchanged.
In the \emph{trusted mode}, each party's module replaces the dealer: the modules attest to each other and establish a key $K$ that the hosts never see, derive the same generation coins (including $\alpha$) from $K$ and a counter, and thus compute identical correction words while each evaluates only its own party's share.
\emph{Generate-and-consume} (GaC) runs the joint generation and the local evaluation in lockstep, consuming each correction word as soon as it is produced, so that neither key distribution nor key storage remains.
DFA also \emph{decouples} generation from protocol preprocessing: when the target is $a=g(r)$ for a bijection $g$, the module samples $a$ uniformly and recovers $r=g^{-1}(a)$.

\textbf{Limits of the semi-honest design.}
DFA argues that correct in-module generation leaves the semi-honest protocol unchanged; against a deviating host this argument fails in four places treated later: (i)~decoupled preprocessing must preserve joint, not only marginal, distributions (\cref{sec:proto-refactor}); (ii)~generator and evaluator state is left implicit (\cref{sec:analysis-dpf}); (iii)~attestation authenticates the module configuration, not that the GPU used a valid key, computed the right product or released an authorized result (\cref{sec:threat-scenarios}); and (iv)~the GPU lies outside the trusted computing base (TCB) and must never obtain module tags for its own results (\cref{sec:proto-epilogue}).

% ==================================================================
\subsection{Tools for Malicious Security}
\label{sec:bg-mal}

\textbf{Security with abort.}
We use the stand-alone real/ideal simulation paradigm, which is preserved under sequential composition~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}; we make no concurrent-composition claim.
A malicious adversary deviates arbitrarily; security with abort requires that it achieve nothing beyond an ideal world in which a trusted functionality computes the result and the adversary only chooses corrupted inputs and whether honest parties receive output, so fairness is not required.
Covert security~\cite{aumann2007covert} only deters cheating; we target full malicious security with abort.

\textbf{Information-theoretic MACs.}
SPDZ-style protocols~\cite{damgard2012spdz,damgard2013practical} authenticate each value of a field $\F$ under a global key $\Delta=\Delta_0+\Delta_1$ that no single party knows.
Party $b$ holds $\Delta_b$ and $\authb{x}{b}=(x_b,\gamma_b)$ with $x_0+x_1=x$ and $\gamma_0+\gamma_1=\Delta x$; linear operations act identically on values and tags, and multiplications consume authenticated triples.
To check openings $z_1,\dots,z_m$, the parties draw coefficients $\rho_i$ \emph{after} the values are fixed, compute $\sigma_b=\sum_i\rho_i(\gamma_{b,i}-\Delta_b z_i)$, and accept only if $\sigma_0+\sigma_1=0$.
A wrong opening passes only if its tag error matches $\Delta$ times the value error or cancels under the coefficients, which happens with probability less than $2/|\F|$.
\sys instantiates this with $t=3$ independent lanes over $\Fp$ (\cref{sec:proto-repr}).

\textbf{Authenticated preprocessing.}
Malicious protocols need authenticated masks and triples whose relations, such as $c=ab$, are actually correct; a valid MAC on a wrong triple does not make it correct.
Generating them without a trusted party is communication-heavy, with oblivious transfer in MASCOT~\cite{keller2016mascot} or somewhat homomorphic encryption in SPDZ and Overdrive~\cite{damgard2012spdz,keller2018overdrive}, all in MP-SPDZ~\cite{keller2020mpspdz}.
Pseudorandom correlation generators~\cite{boyle2019pcg,boyle2020pcg} compress this communication at a substantial computational cost, and a trusted dealer avoids generation but ships every authenticated share.

\textbf{Malicious and verifiable FSS.}
Malicious FSS gates additionally need well-formed keys and authenticated evaluation outputs that can enter MAC-checked arithmetic.
Verifiable FSS~\cite{decastro2022vfss} checks that a key pair shares a function of the declared class, not that a malicious party evaluates its own key correctly.
Shark~\cite{gupta2025shark} achieves active security for FSS-based inference with a dealer that issues authenticated FSS keys and correlated randomness, which enlarges the offline material relative to semi-honest FSS.
The direct way to authenticate a DPF output, a second \emph{tag tree} with payload $\Delta_j\beta$ per MAC key, multiplies DPF work by $1+t$ for $t$ lanes (\cref{sec:analysis-work}).

\textbf{Trusted hardware for secure computation.}
Slalom~\cite{tramer2018slalom} and DarKnight~\cite{hashemi2021darknight} outsource linear layers from a trusted execution environment (TEE) to untrusted GPUs and check the results, Slalom with Freivalds' algorithm~\cite{freivalds1977probabilistic}, which \sys uses only for a restricted subroutine (\cref{sec:proto-freivalds}).
PPMLAC~\cite{zhou2022ppmlac} and STAMP~\cite{huang2022efficient} use small trusted modules to generate correlated randomness or to execute nonlinear operations; STAMP also reports honest-majority malicious settings, and \cref{sec:related} compares these and other trusted-hardware designs.

\textbf{Implications.}
Each tool covers only part of the integrity chain of \cref{sec:intro}, at a cost that erodes trusted DFA's advantage (\cref{sec:analysis}); \sys therefore keeps the module as the dealer and also makes it the verifier (\cref{sec:protocol}).

\textbf{Scope.}
Throughout this paper, \emph{private inference} means two-party FSS-based private inference and \emph{PIR} means two-server DPF-based PIR, as in DFA~\cite{dfa2026trusted}.


==> qa/draft4/sections/03_threat_model.tex <==
% ==================================================================
% Section III: Threat Model and Security Goals
% Owner labels: sec:threat, sec:threat-model, sec:threat-scenarios,
%   sec:threat-goals, sec:threat-profileu, fig:threat, fig:scenarios,
%   tab:scenarios, fig:func, def:security, def:leakage
% ==================================================================
\section{Threat Model and Security Goals}\label{sec:threat}

The trusted mode of DFA moved the FSS dealer into a small protected module but kept the semi-honest model of the protocols it accelerates~\cite{dfa2026trusted}. This section states what changes when a host is malicious: we fix the system model (\cref{sec:threat-model}) and the adversary, derive ten attack scenarios (\cref{sec:threat-scenarios}), define security with explicit leakage (\cref{sec:threat-goals}), and delimit \ProfU (\cref{sec:threat-profileu}). Every link of the integrity chain of \cref{sec:intro} crosses memory, buses, or network paths that a corrupted host controls.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_threat.pdf}
    \caption{System model and trust boundary of \sys under \ProfT. Each party $P_b$ has an untrusted host (CPU, OS, driver, runtime, network interface card (NIC), DRAM) with its GPU, including the streaming multiprocessors (SMs) and high-bandwidth memory (HBM), and a protected module $T_b$ (red dashed TCB, contents in \cref{sec:threat-model}). The adversary statically corrupts at most one host (here that of $P_0$, red region) and may deviate arbitrarily, replay, and abort, but never corrupts $T_0$ or $T_1$. Hosts and GPUs hold only party-local authenticated shares; the protected peer channel between the modules and the authenticated confidential client channels are carried by the untrusted network.}
    \label{fig:threat}
\end{figure*}

\subsection{System Model and Trust Boundary}\label{sec:threat-model}

\textbf{Parties.}
\sys targets the two workloads of DFA~\cite{dfa2026trusted}: two-party FSS-based private inference and two-server DPF-based PIR (\cref{sec:bg}). Two computing parties $P_0$ and $P_1$ serve an external client that owns private inputs and receives outputs; a computing party may also own an input, typically the model weights. Each $P_b$ consists of an untrusted \emph{host~$b$} (every component outside the TCB in \cref{fig:threat}, including DMA engines and storage) and a \emph{protected module} $T_b$, the \sys extension placed next to the GPU L2 as in DFA (\cref{sec:arch-hw}).

\textbf{Trusted computing base.}
$T_b$ contains the session, identity (attestation), and joint-sampler keys and the global MAC keys $\Delta_1,\dots,\Delta_t$; the session role, counters, and one-time resource ledger; the DPF generator and evaluator states and the correction words; the protected table and reduction logic; the frozen check buffers, challenges, and residuals; and all release decisions. Everything else is outside, including every GPU and DMA buffer and every byte in transit between the parties. The GPU computes on party-local authenticated arrays and hands $T_b$ only \emph{candidate} shares (\cref{sec:proto-repr}). Host~$b$ may know its own MAC key shares $\Delta_{b,j}$, but no host ever holds a complete $\Delta_j$, the joint-sampler key, a complete mask (other than the input mask of a wire its party owns or the output mask of an output its party is authorized to receive), the peer's shares, or any challenge or residual.

\textbf{Modules as an ideal resource.}
Following~\cite{katz2007universally}, we model $T_0,T_1$ as an ideal resource $\mathcal{F}_{\mathsf{T}}$ (\cref{app:func-module}; ideal-module assumption in \cref{sec:sec-assump}): their code, keys, parser, arithmetic, state, and approved I/O paths are correct and confidential, and each module's externally observable trace (lengths, timing, host-visible memory and DMA activity, power, thermal, and clock telemetry) is simulatable from the command sequence issued by the host, $\mu$, public lengths, and the accept or abort outcomes, and is independent of the global MAC keys, challenges, and residuals given these. The real execution (\cref{def:security}) realizes their randomness, channels, and setup with concrete primitives. Availability is not assumed, \ProfT requires two physically independent modules, and only the on-die design (\cref{sec:arch-hw}) is a \ProfT target.

\textbf{Channels.}
Client channels are authenticated, confidential, and terminate inside the modules; the peer channel uses AEAD with independent directional keys and no nonce reuse and is established by the authenticated setup of \cref{sec:proto-setup}. The untrusted network carries both. We propose no new attestation or key-exchange protocol; the security of setup is the explicit assumption $\eps{setup}$.

\textbf{Trust is relocated, not removed.}
The modules jointly act as the dealer and can recover inputs from verified openings, and in PIR both modules learn the queried index $\alpha$. \sys thus moves trust from an external dealer and the hosts into the modules rather than hiding inputs from them (\cref{sec:discussion}); its PIR query privacy rests on module trust, unlike untrusted two-server DPF-PIR such as GPU-DPF~\cite{lam2023gpu} or DFA's untrusted mode~\cite{dfa2026trusted}, which hides $\alpha$ from each server without trusted hardware.

\subsection{Adversary Model}

Unlike DFA~\cite{dfa2026trusted}, Sigma~\cite{gupta2023sigma}, and Orca~\cite{jawalkar2024orca}, which assume that both hosts run the prescribed kernels, we consider a probabilistic polynomial-time (PPT) adversary $\Adv$ that statically and maliciously corrupts at most one host before the session starts (host~$0$ in \cref{fig:threat}, by symmetry), controlling its operating system, drivers, GPU kernels and results, host and GPU memory including DMA buffers, and outgoing network traffic. Concretely, $\Adv$ can
(i) modify any value share or tag and run arbitrary kernels in place of the prescribed ones;
(ii) invoke its module's commands in any order with malformed, replayed, or mislabeled arguments;
(iii) rewrite any host-visible buffer at any time, including while the module reads it;
(iv) replay, reorder, delay, or drop messages, reset its platform, and restore old host-side state;
(v) choose the inputs it owns arbitrarily; and
(vi) abort at any point, including after it has learned its own output.
It observes message lengths and timing, the frames exchanged with its module, and the module's external trace. The principal inference statement assumes an honest external client and gives no guarantee against client-server collusion; PIR has two separate regimes, (R1) one malicious server host and (R2) a malicious client only with two honest server hosts (\cref{fig:func}).

\textbf{Out of scope.}
Our theorems exclude corruption of either module (its code, keys, state, or arithmetic); physical attacks such as microprobing, optical fault injection, and power or electromagnetic analysis with measurement equipment~\cite{skorobogatov2017microprobing,skorobogatov2003optical,kocher1999differential,quadir2016survey}; leakage beyond the stipulated trace model; speculative-execution bugs inside the trusted boundary~\cite{van2018foreshadow}; faulty trusted arithmetic; adaptive corruption; and corruption of both hosts. Software-reachable fault and power channels are not physical attacks: the corrupted host controls the GPU driver, which sets clocks, voltage, and power limits and reads telemetry, an interface that Plundervolt exploited on CPUs~\cite{murdock2020plundervolt}. We therefore require isolation from dynamic voltage and frequency scaling (DVFS): host software cannot drive the module's clock or voltage outside its safe operating range (or the module detects glitches and aborts), and the telemetry is covered by the trace simulator. Rollback of module state is covered only by the reboot rule of \cref{sec:proto-ledger}. Availability and fairness are not provided.

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_scenarios.pdf}
    \caption{Malicious scenarios S1 to S8 against trusted FSS acceleration and the \sys mechanism that stops each. Corrupted hosts and GPUs are shaded red, $T_b$ is the red dashed TCB, red arrows with circled numbers are adversary actions, red crosses mark where \sys blocks them, and green text names the defense. S9 and S10, which no protocol can prevent, appear only in \cref{tab:scenarios}.}
    \label{fig:scenarios}
\end{figure*}

\subsection{Malicious Scenarios Against Trusted FSS Acceleration}\label{sec:threat-scenarios}

\Cref{fig:scenarios} and \cref{tab:scenarios} list what a corrupted host can do to a trusted FSS accelerator designed for semi-honest hosts and which \sys mechanism stops each action; the paragraphs below explain why the semi-honest design fails. The scenarios follow the integrity chain: S9 targets the authorized input; S4 and S7 the correlated preprocessing; S2 and S5 the correct local evaluation; S1 the authenticated arithmetic; S3 the consistent opening; and S6 the authorized output release. S8 carries S3 over to the PIR database, and S10 targets availability, which lies outside the chain. \Cref{sec:sec-scenarios,sec:eval-attack} map the scenarios to theorems and to injected tests.

\textbf{S1: Share and tag tampering.}
The corrupted GPU holds every intermediate share and can add an error vector $\bm{e}$ to value shares (and $\bm{d}_j$ to the tags of lane $j$); semi-honest trusted DFA passes it unchecked into the masked opening $x_i+r_i$ of the next FSS gate. Beyond biasing results, this causes \emph{selective failure}: whether $e_i$ flips a comparison depends on whether $x_i$ lies within $|e_i|$ of the threshold, so any observable output change leaks information about $x_i$ (\cref{tab:scenarios}, \cref{sec:proto-check}).

\textbf{S2: Forgery-oracle request.}
A tempting extension of DFA's trusted mode is a command that tags a value computed elsewhere, such as a nonlinear output computed by the GPU's streaming multiprocessors (SMs). This \emph{authenticate(host value)} entry point turns the module into a MAC oracle: the host submits any $y^*$, and every later check accepts it. Attestation certifies the module's code, not the provenance of what it signs (\cref{tab:scenarios}, \cref{sec:proto-epilogue}).

\textbf{S3: TOCTOU buffer swap.}
The module reads its inputs by DMA from host-controlled memory. Verifying a buffer and later rereading it, or trusting a host-reported digest, admits a time-of-check-to-time-of-use (TOCTOU) swap: the host changes the bytes after verification or chooses its error after the challenge is fixed. DMA completion is not evidence of authenticity, a problem semi-honest DFA never faced (\cref{tab:scenarios}, \cref{sec:proto-check}).

\textbf{S4: Replay and rollback.}
DFA derives keys and masks from the shared key $K$ and a counter that is an input of its generate-and-consume procedure~\cite{dfa2026trusted}. Replaying a counter yields the same mask $r$ for two gates, and the openings $x+r$ and $x'+r$ reveal $x-x'$; resetting the module and resuming an old session replays entire key streams (\cref{tab:scenarios}, \cref{sec:proto-ledger}).

\textbf{S5: Role and gate confusion.}
The host decides which module command runs for which gate: it can route the preprocessing of gate $g$ into gate $g'$, alter a table hash or tensor shape, or present party-$0$ material as party-$1$ material. If the role were a per-request argument, the host could obtain both parties' outputs of one joint draw and reconstruct the DPF target $\alpha$, which is exactly the mask of an honest input (\cref{tab:scenarios}, \cref{sec:proto-setup,sec:proto-ledger}).

\textbf{S6: Premature release.}
Semi-honest trusted DFA releases results as soon as they are computed; under a malicious host an early output may already be wrong, and the host may request it repeatedly or for an unauthorized recipient (\cref{tab:scenarios}, \cref{sec:proto-ledger}).

\textbf{S7: Malformed preprocessing.}
A MAC authenticates values, not relations: a triple $(\auth{a},\auth{b},\auth{c})$ with $c\neq ab$ carries valid tags, and multiplying with it yields $xy+\delta$ for a $\delta$ chosen by its producer; the same holds for a GPU-computed matrix product with $C\neq AB$ and for a malformed DPF key. DFA's attestation covers the module's own key generation, not correlations from elsewhere (\cref{tab:scenarios}, \cref{sec:proto-arith}).

\textbf{S8: Snapshot substitution in PIR.}
The PIR database resides in host memory, so a corrupted server host can modify a record, serve an older version, or hash one buffer while scanning another. Semi-honest PIR, including DFA-accelerated PIR, returns whatever the servers compute. Worse, a record modified only at position $i$ corrupts the answer only when $\alpha=i$, so the client's reaction leaks the queried index (\cref{tab:scenarios}, \cref{sec:proto-pir}).

\textbf{S9 and S10: Input substitution; denial of service and selective abort.}
S9, a corrupt owner choosing its input freely, is permitted and extracted by $\FC$; binding a specific model needs the commitment of \emph{Model provenance} below. S10 is not prevented: like SPDZ-style protocols~\cite{damgard2012spdz,keller2016mascot}, \sys provides security with abort, without fairness or guaranteed output delivery, and abort outcomes stay within the permitted leakage (\cref{def:leakage}, \cref{sec:discussion}).

\begin{table*}[t]
\centering
\caption{Malicious scenarios against trusted FSS acceleration. The ``effect'' column describes a semi-honest trusted DFA~\cite{dfa2026trusted}, or a naive malicious extension of it, when one host is corrupted. \cmark: prevented up to the error terms of \cref{thm:main}; \pmark: permitted by the ideal functionality; \xmark: not prevented.}
\label{tab:scenarios}
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabularx}{\textwidth}{c >{\raggedright\arraybackslash}p{1.75cm} >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}p{2.75cm}}
\hline
\textbf{ID} & \textbf{Scenario} & \textbf{Adversary action} & \textbf{Effect on semi-honest trusted DFA} & \textbf{\sys mechanism} & \textbf{Guarantee} \\
\hline
S1 & Share/tag tampering & GPU adds errors $\bm{e}$ to value shares (and $\bm{d}_j$ to tags) before an opening or FSS gate & Undetected; biases outputs and causes selective failure that leaks inputs & Authenticated shares with $t=3$ MAC lanes over $\Fp$; \CheckOpen{} before any protected gate or release & \cmark\ Wrong value accepted w.p.\ $\le (2/p)^t$ per batch (\cref{thm:mac-sound}) \\
\hline
S2 & Forgery-oracle request & Host submits $y^*$ and asks its module to authenticate it & No MACs; a naive authenticate command would sign any forgery & No \emph{authenticate(host value)} command; \Epilogue{} only on internally computed or verified results & \cmark\ Request rejected; outputs correctly authenticated (\cref{thm:epilogue}) \\
\hline
S3 & TOCTOU buffer swap & Host rewrites a DMA buffer after it is checked, or after the challenge is fixed & Module trusts DMA reads; a later reread consumes modified bytes & Freeze before challenge: bytes copied or AEAD-sealed, frozen roots agreed, only frozen bytes consumed & \cmark\ Modification ignored or abort; binding error $\eps{bind}$ \\
\hline
S4 & Replay and rollback & Replays a counter or mask request; resets the module and resumes old keys & Mask reuse: $x+r$ and $x'+r$ reveal $x-x'$; key streams replayed & Labels bound to session, epoch, gate, purpose; one-time ledger; epoch poisoning; erase-and-rekey after reboot & \cmark\ Reuse rejected before any accepted use \\
\hline
S5 & Role/gate confusion & Routes party-0 material as party-1, or gate $g$ material into gate $g'$; alters shapes or table hash & Host schedule trusted; requesting both roles' outputs exposes the target $\alpha$ & Roles fixed by authenticated setup; gate descriptors bound in the ledger and in PRF labels & \cmark\ Mismatched commands abort before preprocessing is issued; host-side reuse of issued shares fails \CheckOpen{} except w.p.\ $\le(2/p)^t$ (\cref{thm:mac-sound}) \\
\hline
S6 & Premature release & Requests outputs before verification, repeatedly, or for another recipient & Results released as soon as computed & Release guard: nothing before \lstate{VERIFIED}; bound certificates; epoch abort gates pending outputs & \cmark\ No candidate value leaves the modules \\
\hline
S7 & Malformed preprocessing & Injects a triple with valid tags but $c\neq ab$, a GPU-computed product with $C\neq AB$, or a wrong DPF key & Attestation silent on external correlations; MACs verify wrong triples & Triples and keys generated inside the TCB ($c=ab$ computed there); imports need a correctness proof & \cmark\ Never consumed; exact arithmetic (\cref{thm:arith}) \\
\hline
S8 & Snapshot substitution (PIR) & Swaps records or version after hashing, or scans a different buffer & Client reconstructs a wrong record; index-dependent failure leaks $\alpha$ & Module hashes the bytes it consumes in public order; quarantine until the commitment matches & \cmark\ Committed record or abort (\cref{thm:pir}) \\
\hline
S9 & Input substitution by a corrupt owner & Corrupted party supplies arbitrary weights or inputs & Same (allowed) & Input extraction by $\FC$; optional commitment-bound loader for model provenance & \pmark\ Allowed by the functionality \\
\hline
S10 & Denial of service/selective abort & Drops, delays, or reorders messages; aborts after learning its own output & Same (not prevented) & Bounded resources and abort; abort outcomes simulatable from permitted leakage & \xmark\ Not prevented (no fairness or availability) \\
\hline
\end{tabularx}
\end{table*}

\subsection{Security Goals and Ideal Functionalities}\label{sec:threat-goals}

\textbf{Goals.}
Against a corrupted host, \sys must provide \emph{privacy} (the host learns nothing beyond the permitted leakage and the outputs it is authorized to receive), \emph{correctness} (honest recipients obtain the circuit evaluated on the honest inputs and the corrupted party's extracted inputs, or abort), \emph{authorized release} (no value leaves the modules unless its opening was verified and bound to a release certificate), and \emph{one-time use} (no randomness is consumed twice). We formalize the first two as stand-alone real/ideal security with abort, preserved under sequential composition~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}, with an explicit leakage function; the last two are mechanisms that the proof relies on (\cref{sec:proto-ledger}). We claim neither universal nor concurrent composability, and concurrent sessions that share module state are not covered.

\textbf{Manifest.}
Every session fixes a public manifest $\mu$ (\cref{app:func-circuit}): the protocol version, session identities, roles, field, numeric encoding, the finite circuit $C$ with its gate and wire identifiers and tensor shapes, approved public tables, interval coefficients, authorized recipients, the input interface $\mathsf{In}_\nu$ and validation rules of every input wire $\nu$, and the public schedule, which places every input gate before every validity check, and both before the first output opening. The modules evaluate the validity predicates at the public boundaries declared in $\mu$; in $\Pi_{\mathsf{Input}}$ they compute $x^{*}=r+\varepsilon$ and abort unless $x^{*}\in\mathsf{In}_\nu$ (\cref{fig:arith}).

\begin{definition}[Permitted leakage]\label{def:leakage}
For a circuit execution under manifest $\mu$, the permitted leakage is
\[
\Leak_C=\bigl(\mu,\ \mathsf{len},\ \mathsf{sched},\ \mathsf{pub},\ \mathsf{status}\bigr),
\]
where $\mathsf{len}$ are the lengths of all public messages; $\mathsf{sched}$ is the public schedule of batches, checks, and interaction boundaries fixed by $\mu$; $\mathsf{pub}$ are the values that $\mu$ designates as authorized public openings; and $\mathsf{status}$ are the specified abort and validation outcomes, including every input-dependent validity bit declared in $\mu$, which is never silently excluded. For PIR, $\Leak_{\mathrm{PIR}}$ consists of the public descriptor $\mathsf{desc}_v=(\mathsf{id},v,N,\mathsf{enc},\mathsf{cm}_v)$ (database identifier, version, true length $N$, which also fixes the padded length, record encoding, and authorized snapshot commitment), the public scan length and order, message lengths and schedules, and the accept, reject, or abort outcome.
\end{definition}

Honest inputs, intermediate wire values, masks, MAC keys, DPF keys and correction words, raw FSS outputs, challenges, and residuals are not in $\Leak_C$. Masked openings such as $x+r$ are uniform given $\Leak_C$, and the simulator samples them (\cref{app:proof-main}). Module timing and access patterns are fixed by $\mu$ (full-domain scans have a declared order); the residual trace falls under $\eps{trace}$.

\begin{figure}[t]
\centering
\footnotesize
\fbox{\begin{minipage}{\dimexpr\columnwidth-2\fboxsep-2\fboxrule\relax}
\centering\underline{Functionality $\FC$}\par\smallskip
\raggedright
\textbf{Parameters.} Public manifest $\mu$ (circuit $C$ over $\Fp$, input owners and interfaces $\mathsf{In}_\nu$, validity predicates, authorized recipients, public schedule). Corrupted set $I$: at most one host; the client is honest.
\begin{enumerate}[leftmargin=*,nosep,topsep=2pt]
\item \textbf{Input.} Receive the authenticated input $x_\nu$ of every input wire $\nu$ from its designated owner. If the owner is corrupted, receive $x^{*}_\nu$ from $\Sim$ and set $x_\nu\gets x^{*}_\nu$ (extraction). If some $x_\nu$ is missing, malformed, or not in $\mathsf{In}_\nu$, send $\bot$ to every honest recipient and halt; this abort outcome is part of $\mathsf{status}$.
\item \textbf{Validate and evaluate.} Evaluate the validity predicates of $\mu$; their accept or abort outcome is part of $\mathsf{status}$. For accepted inputs, compute $\vec{y}=C(\vec{x})$ exactly in the declared finite arithmetic, including the specified comparisons and truncations.
\item \textbf{Deliver or abort.} Send $\Leak_C$ and the outputs of corrupted recipients to $\Sim$. At each public interaction boundary, $\Sim$ may send $\mathsf{abort}$ or $\mathsf{delay}$; on $\mathsf{abort}$, send $\bot$ to every honest recipient. Otherwise deliver each $y_i$ to its authorized recipient. A corrupted recipient may obtain its output before honest ones (no fairness).
\end{enumerate}
\end{minipage}}

\vspace{5pt}
\fbox{\begin{minipage}{\dimexpr\columnwidth-2\fboxsep-2\fboxrule\relax}
\centering\underline{Functionality $\FPIR$}\par\smallskip
\raggedright
\textbf{Parameters.} Public descriptor $\mathsf{desc}_v=(\mathsf{id},v,N,\mathsf{enc},\mathsf{cm}_v)$; the commitment $\mathsf{cm}_v$ fixes $D=(D[0],\dots,D[N-1])$. Corruption regimes, never combined: (R1) a malicious server host (at most one), client honest; (R2) a malicious client only, both server hosts honest.
\begin{enumerate}[leftmargin=*,nosep,topsep=2pt]
\item \textbf{Query.} Receive an index $\alpha$ with query identifier $\mathit{qid}$ from the client; in (R2), extract the corrupted client's index $\alpha^{*}$ and set $\alpha\gets\alpha^{*}$. If $\alpha\notin\{0,\dots,N-1\}$ or the request is inconsistent, return $\mathsf{reject}$ to the client and stop.
\item \textbf{Leak.} Send $\Leak_{\mathrm{PIR}}$ to $\Sim$; nothing about $\alpha$ is sent.
\item \textbf{Answer.} In (R1), if $\Sim$ sends $\mathsf{abort}$, send $\bot$ to the client; otherwise send $D[\alpha]$. In (R2), send $D[\alpha]$, and no other information about $D$, to the client.
\end{enumerate}
\end{minipage}}
\caption{Ideal functionalities for authenticated circuit evaluation (top) and versioned-snapshot PIR (bottom). Both provide security with abort. $\FPIR$ hides $\alpha$ from the corrupted host; both trusted modules learn it (\cref{sec:threat-model}). The full definitions, together with the ideal module resource $\mathcal{F}_{\mathsf{T}}$, are in \cref{app:func}.}
\label{fig:func}
\end{figure}

\begin{definition}[Static malicious security with abort]\label{def:security}
Let $\mathcal{F}\in\{\FC,\FPIR\}$ with leakage $\Leak$ as in \cref{def:leakage}, and let $\Pi$ be a protocol run by $P_0$ and $P_1$ in which each module executes the concrete module program correctly and confidentially: $\mathcal{F}_{\mathsf{T}}$ with its joint random function $R$ instantiated by $\PRF_K$, its peer and client channels by AEAD over the hosts' network, and \cmd{OPEN_SESSION} by attestation and authenticated key exchange.
For a PPT adversary $\Adv$ with auxiliary input $z$ that statically corrupts the set $I$, $\Real_{\Pi,\Adv(z),I}(\mu,\vec{x})$ is the joint distribution of the view of $\Adv$ (its inputs, randomness, received messages, and the external traces of the modules observable from corrupted hosts) and the outputs of the honest parties and client in an execution of $\Pi$ on manifest $\mu$ and input vector $\vec{x}$.
$\Ideal_{\mathcal{F},\Sim(z),I}(\mu,\vec{x})$ is the joint distribution of the output of a simulator $\Sim$ and the honest outputs in an execution in which $\Sim$ interacts only with $\mathcal{F}$: it submits the corrupted parties' inputs, receives $\Leak$ and the corrupted parties' outputs, and may abort or delay as $\mathcal{F}$ allows.
We say that $\Pi$ \emph{$\epsilon$-securely realizes $\mathcal{F}$ with leakage $\Leak$ against static malicious corruption with abort} if for every PPT adversary $\Adv$ and every set $I$ admitted by the corruption regime of $\mathcal{F}$ there exists a PPT simulator $\Sim$ such that for all $\mu$, $\vec{x}$, $z$ and every PPT distinguisher $\mathcal{D}$,
\begin{align*}
\Bigl|&\Pr\bigl[\mathcal{D}\bigl(\Real_{\Pi,\Adv(z),I}(\mu,\vec{x})\bigr)=1\bigr]\\
&\quad-\Pr\bigl[\mathcal{D}\bigl(\Ideal_{\mathcal{F},\Sim(z),I}(\mu,\vec{x})\bigr)=1\bigr]\Bigr|\le\epsilon .
\end{align*}
\end{definition}

\textbf{Remarks.}
The real world of \cref{def:security} contains the concrete module program; $\mathcal{F}_{\mathsf{T}}$ with ideal setup, channels, and randomness is the resource of hybrids $\Hyb{2}$ to $\Hyb{4}$ of the proof (\cref{app:proof-main}), and the simulator controls only this ideal representation of the trusted resources, never the honest party's prescribed inputs. The concrete $\epsilon$ is the bound $\eps{VIGOR}$ of \cref{thm:main}; correctness of protected code is a premise of $\mathcal{F}_{\mathsf{T}}$, and \cref{tab:obligations} lists what a chip must still establish.

\textbf{Model provenance.}
Computational correctness is not model provenance, and a public architecture hash in $\mu$ does not authenticate private weights. To bind a pre-approved model, $\mu$ must contain a commitment to the canonical quantized weight bytes, authorized by the client or an independent model authority rather than declared by the untrusted host, and the protected input loader hashes exactly those bytes before sharing them (\cref{sec:proto-arith}); a mismatch aborts. Otherwise the weights are the owner's freely chosen private input, and S9 is the intended behavior of $\FC$.

\subsection{The Stronger Profile U}\label{sec:threat-profileu}

\ProfT trusts the modules. When the hardware itself must be treated as adversarial, for example because the accelerator vendor or platform administrator is untrusted, \ProfU gives the accelerator neither the joint-sampler key nor any global MAC key. The circuit runs through an established malicious two-party backend, such as SPDZ-family protocols with MASCOT or SPDZ2k preprocessing~\cite{damgard2012spdz,keller2016mascot,cramer2018spdz2k,keller2020mpspdz} or dealer-based malicious FSS such as Shark~\cite{gupta2025shark}, and the accelerator is confined to party-local data, for instance expanding the DPF keys that the backend exports to its own party. The same DPF datapath therefore serves both profiles, but \ProfU gives up the local-dealer and generate-and-consume savings, and with exported keys it must add the backend's DPF privacy assumption to its bound (\cref{sec:sec-main}). \ProfU is a separate backend chosen at session start, not a fallback after a module compromise, which would not undo leaked secrets; a fresh session with fresh inputs and masks is required. The rest of this paper analyzes and evaluates \ProfT.


==> qa/draft4/sections/04_analysis.tex <==
% ======================================================================
% Section IV: Workload Analysis (owner: sections/04_analysis.tex)
% Labels defined here: sec:analysis, sec:analysis-cost, sec:analysis-dpf,
% sec:analysis-work, alg:gen, alg:eval, fig:gac, tab:gatecost, fig:motiv
% ======================================================================
\section{Workload Analysis: Where Malicious Security Costs Go}
\label{sec:analysis}

The DFA design~\cite{dfa2026trusted} was driven by one workload observation: in semi-honest FSS workloads, DPF generation, distribution and evaluation dominate both computation and communication, so a small DPF engine that also plays the dealer removes the dominant cost. Repeating this analysis for the adversary of \cref{sec:threat} changes the design target: handled naively, malicious security multiplies exactly the DPF work and key traffic that trusted DFA made small; handled carefully, it moves the cost from DPF to authenticated linear algebra on the GPU and to the extra round of every verified opening.

% ======================================================================
\subsection{Cost Sources in Malicious FSS}
\label{sec:analysis-cost}

We take as reference the masked-input paradigm of FSS-based inference~\cite{gupta2023sigma,jawalkar2024orca} (\cref{sec:bg-pi}): linear layers operate on additive shares, and every nonlinear gate opens a masked input $x+r$ and evaluates FSS keys prepared for the mask $r$. Making this pipeline secure against a malicious host (\cref{def:security}) adds the following costs, regardless of how they are implemented.

\textbf{(i) Authenticated representation.}
Every wire must carry information-theoretic MACs so that a host that changes its share is caught~\cite{damgard2012spdz,damgard2013practical}. In our representation (\cref{sec:proto-repr}), party $b$ holds $\authb{x}{b}=(x_b,\gamma_{b,1},\gamma_{b,2},\gamma_{b,3})$ over $\Fp$ with $p=2^{61}-1$ and $t=3$ independent MAC keys: four 64-bit words, or 32~B per element and party, instead of 8~B for a semi-honest share in $\Z_{2^{64}}$. Every linear layer is therefore computed on four lanes (the value and three tags), each lane uses exact Mersenne reduction instead of free 64-bit wraparound (\cref{sec:arch-field}), and every authenticated element that crosses PCIe or the host-module interface grows by the same factor of four. Only the peer link is spared, because checks exchange value shares and $t$ residuals rather than tags (\cref{sec:proto-check}).

\textbf{(ii) Verified openings.}
Opened values (masked gate inputs, the Beaver differences $d,e$ of each multiplication~\cite{beaver1991efficient}, and outputs) must be checked before anything depends on them. A sound check derives its challenge only after the checked bytes are fixed (\cref{thm:mac-sound}), so at least one extra exchange follows every checked batch, and a dependent nonlinear gate may not consume an unchecked opening. Batching amortizes challenge derivation and metadata but not this round, which lies on the critical path of every layer: a protocol with $R$ online rounds approaches $2R$.

\textbf{(iii) Correct preprocessing.}
Triples, masks and FSS keys must be \emph{correct}, not merely authenticated: a valid MAC on a triple with $c\neq ab$ does not make it correct. The options of \cref{sec:bg-mal} either ship more offline material from a dealer or replace the dealer by heavy interactive preprocessing, and neither removes offline data movement. Without a dealer, FSS keys require a secure two-party evaluation of DPF key generation, with one round per tree level~\cite{doerner2017scaling} before any malicious-security overhead.

\textbf{(iv) Authenticated FSS outputs.}
A DPF output share is a plain additive share. To re-enter authenticated arithmetic it needs $t$ tag shares, and the straightforward way to obtain them is a second DPF per MAC lane $j$ with the same target and payload $\Delta_j\beta$ (a \emph{tag tree}). This multiplies DPF keys, key bytes and PRG work by $1+t$, i.e., by four for $t=3$.

\textbf{(v) Key validity is not evaluation correctness.}
Verifiable FSS~\cite{decastro2022vfss} lets evaluators check that their keys are well formed, which protects against a malicious key generator. It does not constrain an evaluator that computes on valid keys and then adds an error to its output share, nor the arithmetic that consumes that share.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{charts/chart_motiv.pdf}
    \caption{Estimated BERT-Base latency breakdown on LAN (1~GB/s, 0.05~ms round-trip time) by cost source, for two semi-honest configurations of~\cite{dfa2026trusted} and three malicious ones (dealer-based malicious FSS, \sys without GaC, \sys); all splits come from our model (\cref{app:model}). The horizontal axis is broken between 7.5 and 15~s so that the 18.8~s semi-honest GPU bar and the \est{43.9~s} dealer-based bar fit.}
    \label{fig:motiv}
\end{figure}

\textbf{Observation 1: distribution still dominates dealer-based malicious FSS.}
\Cref{fig:motiv} splits the estimated BERT-Base LAN latency by cost source. Dealer-based malicious FSS, modeled after the protocol family of Shark~\cite{gupta2025shark} (\cref{sec:eval-method}), must move \est{37.6~GB} of authenticated keys and preprocessing per query, \est{2.2$\times$} the 17.1~GB of the semi-honest GPU baseline~\cite{dfa2026trusted}. At 1~GB/s, this distribution alone takes \est{37.6~s} of \est{43.9~s} (\est{86\%}), and moving the material from host memory into the GPU adds another \est{1.70~s}. Without an authenticated-key blow-up ($\psi_{\mathrm{key}}=1$, \cref{app:model}), it still takes \est{22.4~s}, \est{5.8$\times$} that of \sys.

\textbf{Observation 2: without distribution, DPF is no longer the bottleneck.}
Removing distribution, as trusted DFA did for the semi-honest case, exposes a different profile. In \sys, four-lane authenticated GEMM takes \est{2.60~s} of \est{3.83~s} (\est{68\%}), \est{5.0$\times$} our \est{0.52~s} estimate of the semi-honest GEMM; online communication takes \est{0.615~s} (\est{16\%}); and all nonlinear gates together take only \est{0.131~s} (\est{3.4\%}).

\textbf{Observation 3: on a WAN, verification rounds dominate.}
With a 70~ms round-trip time (RTT) the extra check round of source (ii) outweighs all computation: removing \CheckOpen, which is insecure and serves only as a lower bound, would cut the estimated BERT-Base WAN latency from \est{89.7~s} to \est{50.5~s} (\cref{tab:ablation}).

% ======================================================================
\subsection{Compute Pattern of Exact DPF}
\label{sec:analysis-dpf}

Malicious-security proofs reason about concrete states, so we fix the DPF computation exactly. \Cref{alg:gen,alg:eval} give the tree-based DPF~\cite{gilboa2014distributed,boyle2016function} in the form that \sys executes; the same algorithms serve \ProfU, where keys are exported to an external malicious backend (\cref{sec:threat-profileu}). The expansion function $\PRG:\bits{128}\to(\bits{128}\times\{0,1\})^2$ is fixed and AES-based as in DFA, $\Conv:\bits{128}\to\Fp$ is the fixed output conversion, the target $\alpha$ and the query $x$ have $n$ bits read most-significant first, and the payload is $\beta\in\Fp$.

\begin{algorithm}[t]
\caption{Exact DPF key generation ($\DPF.\Gen$)}
\label{alg:gen}
\begin{algorithmic}[1]
\algstretch
\Require target $\alpha=\alpha_1\cdots\alpha_n\in\bits{n}$ (MSB first), payload $\beta\in\Fp$
\Ensure keys $(k_0,k_1)$ with $\Eval(k_0,x)+\Eval(k_1,x)=\beta\cdot\one[x=\alpha]$
\State sample independent $s_0,s_1\getsr\bits{128}$; $t_0\gets 0$; $t_1\gets 1$
\State save the initial seeds $s_0^{(0)}\gets s_0$, $s_1^{(0)}\gets s_1$
\For{$i=1$ \textbf{to} $n$}
    \State $a\gets\alpha_i$; \ $\keep\gets a$; \ $\lose\gets 1-a$ \Comment{$L=0$, $R=1$}
    \State $(s_b^L,t_b^L,s_b^R,t_b^R)\gets\PRG(s_b)$ for $b\in\{0,1\}$
    \State $\sCW\gets s_0^{\lose}\oplus s_1^{\lose}$
    \State $\tCW{L}\gets t_0^L\oplus t_1^L\oplus a\oplus 1$; \ $\tCW{R}\gets t_0^R\oplus t_1^R\oplus a$
    \LineComment{both $b$, with the \emph{old} $t_b$; $\cdot$ is a conditional XOR}
    \State $(s_b,t_b)\gets\bigl(s_b^{\keep}\oplus t_b\cdot\sCW,\ t_b^{\keep}\oplus t_b\cdot\tCW{\keep}\bigr)$
    \State $\CW^{(i)}\gets(\sCW,\tCW{L},\tCW{R})$
\EndFor
\State $u_b\gets\Conv(s_b)$ for $b\in\{0,1\}$
\State $\CWout\gets(-1)^{t_1}\,(\beta-u_0+u_1)$
\LineComment{keys hold the initial roots, never the final states}
\State $k_b\gets\bigl(s_b^{(0)},\,b,\,\CW^{(1)},\ldots,\CW^{(n)},\,\CWout\bigr)$ for $b\in\{0,1\}$
\State \Return $(k_0,k_1)$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[t]
\caption{Exact DPF evaluation ($\DPF.\Eval$, $\DPF.\EvalAll$)}
\label{alg:eval}
\begin{algorithmic}[1]
\algstretch
\Require role $b$, key $k_b=(s_b^{(0)},b,\CW^{(1)},\ldots,\CW^{(n)},\CWout)$, query $x=x_1\cdots x_n$
\Ensure share $y_b\in\Fp$ (or all $2^n$ leaf shares for $\EvalAll$)
\Function{Eval}{$k_b,x$}
    \State $(s,t)\gets(s_b^{(0)},b)$ \Comment{root control bit $=$ role}
    \For{$i=1$ \textbf{to} $n$} \Comment{$\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$}
        \State $(s^L,t^L,s^R,t^R)\gets\PRG(s)$ \Comment{$t$: old evaluator bit}
        \State $(s^L,t^L)\gets(s^L\oplus t\cdot\sCW,\ t^L\oplus t\cdot\tCW{L})$
        \State $(s^R,t^R)\gets(s^R\oplus t\cdot\sCW,\ t^R\oplus t\cdot\tCW{R})$
        \State $(s,t)\gets(s^{L},t^{L})$ if $x_i=0$, else $(s^{R},t^{R})$
    \EndFor
    \State \Return $y_b\gets(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$
\EndFunction
\Function{EvalAll}{$k_b$}
    \State push $(s_b^{(0)},b,0,\langle\rangle)$ onto the stack \Comment{$\langle\rangle$: empty prefix}
    \While{the stack is not empty}
        \State pop $(s,t,i,\pi)$ \Comment{seed, bit, depth, prefix}
        \If{$i=n$}
            \State emit leaf $\pi$ with share $(-1)^b\bigl(\Conv(s)+t\cdot\CWout\bigr)$
        \Else
            \State expand $s$ as in lines 4--6 with $\CW^{(i+1)}$
            \State push $(s^R,t^R,i{+}1,\pi\|1)$
            \State push $(s^L,t^L,i{+}1,\pi\|0)$ \Comment{left first}
        \EndIf
    \EndWhile
\EndFunction
\end{algorithmic}
\end{algorithm}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_gac.pdf}
    \caption{Malicious-safe generate-and-consume inside module $T_b$ for a depth-2 tree. (a)~Joint generation: the two generator states $(s_0,t_0)$ and $(s_1,t_1)$ follow the target path $\alpha=01$ and emit $\CW^{(1)}$, $\CW^{(2)}$ and $\CWout$, which are consumed immediately instead of being stored as a key. (b)~Local evaluation of party $b$ on query $x=00$: a separate evaluator state $(\tilde s,\tilde t)$ follows $x$, applies each correction word at its own level, and leaves the target path at level~2, where only its own control bit $\tilde t$ is correct; grey nodes are never expanded. (c)~Leaf epilogue: the raw share $\tilde y_b$ is freshly reshared and authenticated with joint pads $\zeta,\kappa_1,\kappa_2,\kappa_3$ into the 32~B tuple $\authb{y}{b}$. The crossed-out inset is the tag-tree alternative, which needs $t=3$ extra DPF trees with payloads $\Delta_j\beta$ and four times the PRG work.}
    \label{fig:gac}
\end{figure*}

\textbf{High-level idea.}
\Cref{fig:gac}(a) shows $\Gen$ walking two states $(s_0,t_0)$ and $(s_1,t_1)$ down the target path. Since each state applies a correction only when its \emph{own} old control bit is set, exactly one of the two is corrected at each level; the corrections make the off-path states of both parties identical, so their signed outputs cancel, while $\CWout$ programs $\beta$ at the target leaf (\cref{thm:dpf-correct}). Correctness needs neither uniform targets nor computational hardness; uniform masks belong to the application protocol (\cref{sec:proto-refactor}).

\textbf{Explicit states.}
Three details that the simplified semi-honest listing~\cite{dfa2026trusted} leaves implicit are explicit in \cref{alg:gen,alg:eval}, because the malicious analysis depends on them. First, the root control bits are fixed by role, $t_0=0$ and $t_1=1$, rather than sampled, and the evaluator of party $b$ always starts from $(s_b^{(0)},b)$. Second, a key contains the \emph{initial} seed of its party, the correction words and $\CWout$; the generator's final states are never substituted for the roots. Third, the payload and the role enter only through $\CWout$ and the output sign $(-1)^b$, so both are bound inputs of the ledgered gate descriptor (\cref{sec:proto-ledger}) rather than host-supplied parameters.

\textbf{Generator versus evaluator state.}
Lines 5--6 of \cref{alg:eval} correct both children with the evaluator's own old control bit $t$. Along the target path this bit coincides with the generator's $t_b$, which invites reusing the generator's control register during generate-and-consume. The substitution is wrong as soon as the query leaves the path (level~2 in \cref{fig:gac}(b)): there the evaluator states of the two parties are identical and must apply identical corrections, whereas the generator bits $t_0$ and $t_1$ still differ, so one party would apply a correction that the other omits, and the off-path outputs would no longer cancel. Each module therefore keeps a separate evaluator state next to its two generator states (\cref{alg:gac}).

% ======================================================================
\subsection{Work Accounting}
\label{sec:analysis-work}

\begin{table*}[t]
\centering
\caption{Analytic Cost of One Single-Path DPF Gate of Depth $n$ with $t$ MAC Lanes}
\label{tab:gatecost}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{llccccccc}
\hline
\textbf{Design} & \textbf{Security} & \makecell{\textbf{PRG exp.}\\\textbf{per gate}} & \makecell{\textbf{Field ops per}\\\textbf{output, party}} & \makecell{\textbf{Offline bytes}\\\textbf{per gate}} & \makecell{\textbf{Bytes into GPU}\\\textbf{per party}} & \makecell{\textbf{Extra}\\\textbf{rounds}} & \makecell{\textbf{Auth.}\\\textbf{output}} & \makecell{\textbf{Verifies}\\\textbf{evaluation}} \\
\hline
Dealer-based FSS~\cite{gupta2023sigma,jawalkar2024orca} & SH & $4n$ & 0 & $2|k|$ & $|k|$ & 0 & \xmark & \xmark \\
Trusted DFA, GaC~\cite{dfa2026trusted} & SH & $6n$ & 0 & 0 & 8 & 0 & \xmark & \xmark \\
\makecell[l]{Dealer-based FSS, tag trees\\(counting bound)} & Mal. & $4n(1+t)$ & 0 & $2(1+t)|k|$ & $(1+t)|k|$ & 1 per batch & \cmark & \cmark\ (at opening) \\
vFSS-verified keys~\cite{decastro2022vfss} & Mal.\ key gen. & $4n$ + sketch & 0 & $2|k|+O(\lambda)$ & $|k|+O(\lambda)$ & 1 (sketch) & \xmark & \xmark\ (keys only) \\
Vector-payload tree, $t$ lanes$^{\dagger}$ & Mal. & $6n+O(t)$ & $t$ adds & 0 & 32 & 1 per batch & \cmark & \cmark \\
\sys, GaC + epilogue & Mal. & $6n$ & \makecell{3 mult.\\+ 4 pads} & 0 & 32 & 1 per batch & \cmark & \cmark \\
\hline
\end{tabular}

\vspace{3pt}
\parbox{\textwidth}{\footnotesize SH: semi-honest; Mal.: malicious. $|k|$ is the byte length of one party's key. PRG expansions are summed over all parties, dealer included. Bytes into the GPU are keys loaded by a GPU evaluator or output shares delivered by a module. Mask shares and Beaver triples of the surrounding arithmetic are omitted; with authentication, each such element costs 32~B per party instead of 8~B. Rounds are counted relative to the plain masked opening that every design performs. The evaluated dealer-based malicious FSS baseline assumes \est{2.2$\times$} the semi-honest offline bytes (\cref{app:model}), below this counting bound. $^{\dagger}$One in-module tree with payload $(\beta,\Delta_1\beta,\ldots,\Delta_t\beta)$; $O(t)$ counts extra leaf-conversion blocks.}
\end{table*}

\Cref{tab:gatecost} compares one single-path DPF gate at six design points. With 128-bit seeds, one party's key holds its root seed, $n$ correction words of $128+2$ bits and $\CWout$ as one canonical 64-bit word (the root control bit is the public role), so $|k|=\lceil(128+130n+64)/8\rceil$ bytes, or 1{,}016~B for $n=61$.

\textbf{Design-point comparison.}
Trusted DFA trades $1.5\times$ the dealer's PRG work for zero key bytes: each module expands $2n$ generator states and $n$ evaluator states for its own party, so the two modules perform $6n$ expansions where a dealer and two evaluators perform $4n$. Tag trees multiply PRG work, key bytes and key I/O by $1+t$, and verified keys authenticate neither the output nor its evaluation. \sys keeps DFA's $6n$ expansions and zero key bytes and adds only three field multiplications and four pads per output and party; it cannot avoid the 32~B authenticated tuple and the check round.

\textbf{Effect of the epilogue.}
Because the epilogue (\cref{fig:gac}(c)) leaves the per-gate PRG expansion count unchanged, the estimated single-path throughput of the DPF engine drops only from \est{113} to \est{106~M~gates/s} at $n=61$ relative to semi-honest trusted DFA, whereas per-lane tag trees fall to \est{26.7~M~gates/s}; the gap to per-lane tag trees stays at \est{3.8--4.0$\times$} for $n$ between 8 and 61 (\cref{fig:dpfthr}). The drop comes mainly from the assumed pipeline efficiency (\est{0.85} vs.\ \est{0.90}; \cref{app:model}); the two extra pad blocks ($6n{+}3$ vs.\ $6n{+}1$ AES blocks per gate) cost only 0.5\%. The vector-payload tree nearly matches the epilogue's PRG count, but it widens every output correction by $t$ field elements, covers only results linear in DPF evaluations, and exports pseudorandom tag shares whose hiding rests on DPF key privacy. The epilogue instead makes every exported tuple exactly uniform for its holder (\cref{thm:epilogue}) and applies unchanged to LUT, interval, direct and PIR results.

\textbf{Remaining costs we accept.}
\sys does not remove duplicated generation: $6n$ instead of $4n$ expansions is the price of eliminating $2|k|$ network bytes and $|k|$ bytes of key I/O per gate, a favorable trade because PRG expansion is the cheapest operation in the pipeline while bytes cross its slowest links. Two further costs remain. The conservative $O(n^2)$ DCF of \cref{alg:dcf} is the only DCF our proofs cover; its interval gate costs 22{,}692 AES blocks at $n=61$, against a projected \est{976} for an optimized DCF, so the compiler chooses among direct, LUT and interval gates by modeled cost, subject to an FSS-portability constraint (\cref{sec:proto-direct,sec:eval-micro}). A host-module link of $B$ bytes/s bounds the authenticated output stream at $B/32$ elements/s, which motivates the L2-adjacent placement (\cref{sec:arch-insight}).

\textbf{Implications.}
For sources (iii) and (iv) the semi-honest lesson still holds: distribution is the largest avoidable cost (Observation~1), so DFA's local generation and generate-and-consume must stay, and FSS outputs must be authenticated without multiplying DPF work. This leaves sources (i) and (ii) as the dominant costs (Observations~2 and~3). The analysis yields five design rules that structure the rest of the paper: (1)~authenticate FSS outputs by fresh resharing inside the module, never by extra trees and never by authenticating host values (S2; \cref{sec:proto-epilogue}); (2)~keep generation local and streamed, with separate generator and evaluator states (S7; \cref{sec:proto-gac}); (3)~make the unavoidable check round sound and batchable by freezing bytes before challenges are drawn (S1, S3, S8), and release no output before \lstate{VERIFIED} (S6; \cref{sec:proto-check,sec:proto-ledger}); (4)~bind every randomness draw to one session, gate, role and use, so that local generation does not open a replay path (S4, S5; \cref{sec:proto-ledger}); and (5)~leave four-lane exact linear algebra on the GPU while the module generates correct triples (S7) and verifies openings (\cref{sec:arch-insight}).


==> qa/draft4/sections/05a_protocol.tex <==
% ======================================================================
% Section V (part 1): VIGOR-DFA Protocol Design
% Owner: 05a_protocol.tex. Continues in 05b_protocol_gates.tex.
% ======================================================================
\section{\texorpdfstring{\sys}{VIGOR-DFA} Protocol Design}\label{sec:protocol}

This section specifies the protocol run by the two parties of \ProfT: the flow (\cref{sec:proto-overview}), the representation, joint randomness and lifecycle state (\cref{sec:proto-repr,sec:proto-setup,sec:proto-ledger}), and the mechanisms that move values through the integrity chain (\cref{sec:proto-gac,sec:proto-epilogue,sec:proto-check,sec:proto-arith}). Nonlinear gates, refactoring, GPU verification and PIR follow in \cref{sec:proto-gates,sec:proto-direct,sec:proto-refactor,sec:proto-freivalds,sec:proto-pir}; formal statements are collected in \cref{sec:security}.

% ======================================================================
\subsection{Overview}\label{sec:proto-overview}

\textbf{High-level idea.}
In trusted DFA the protected module replaces the dealer: it samples FSS keys locally and consumes each correction word as soon as it produces it~\cite{dfa2026trusted}. \sys turns the module from a dealer into a dealer that also verifies. Every wire carries an authenticated sharing with $t$ information-theoretic MAC lanes. The GPU performs all linear algebra on these sharings but only ever produces \emph{candidate} shares. Each module generates every correlation of its party, authenticates every FSS output it computes, checks every opening on frozen bytes and releases nothing before verification.

\textbf{Per-gate lifecycle.}
Every gate of the public circuit $C$ fixed by the manifest $\mu$ passes through the same module commands (\cref{tab:commands}). (1)~With \cmd{RESERVE_PREP}, $T_b$ reserves the gate's randomness labels in its one-time ledger and issues party-local authenticated preprocessing (masks, triples) to host~$b$. (2)~Host $b$'s GPU computes candidate authenticated shares with local linear operations. (3)~With \cmd{FREEZE_BATCH} and \cmd{CHECK_OPEN}, the two modules freeze the submitted bytes and verify the masked openings the gate needs. (4)~For a nonlinear gate, \cmd{EVAL_FSS} consumes the verified opening, runs generate-and-consume inside $T_b$ and returns a freshly authenticated share. (5)~\cmd{FINAL_OUTPUT} hands a masked output and a bound certificate to an authorized recipient. A failure in any step triggers \cmd{ABORT}, which poisons the epoch. Each mechanism below enforces one design rule of \cref{sec:analysis-work}; \cref{tab:notation} summarizes the notation.

\begin{table}[t]
\caption{Notation used in the protocol description}
\label{tab:notation}
\centering
\footnotesize
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{p{0.27\linewidth} p{0.63\linewidth}}
\hline
\textbf{Symbol} & \textbf{Meaning} \\
\hline
$P_b$; host $b$; $T_b$ & party $b\in\{0,1\}$; its untrusted host (CPU, OS, driver, GPU, memory, NIC); its protected module \\
$\mu$, $C$ & public manifest and the finite circuit it fixes \\
$p$, $\Fp$ & Mersenne prime $2^{61}-1$ and the protocol field \\
$t$ & number of MAC lanes ($t=3$) \\
$\Delta_j$; $\Delta_{b,j}$ & global MAC key of lane $j$ (modules only); host $b$'s additive share of it \\
$\auth{x}$; $\authb{x}{b}$ & authenticated sharing of $x$; party $b$'s tuple $(x_b,\gamma_{b,1},\dots,\gamma_{b,t})$ \\
$\gamma_{b,j}$ & tag share of party $b$ in lane $j$, $\gamma_{0,j}+\gamma_{1,j}=\Delta_j x$ \\
$K$ & session key shared by $T_0$ and $T_1$ after setup \\
$\ell$ & length-prefixed label (session, epoch, gate, purpose, logical draw, block) \\
$\PRF_K(\ell,\cdot)$ & joint draw: same label, same value in both modules \\
$\nu$; $\varepsilon$; $\upsilon$ & wire index; masked input difference $x-r$; masked output $y+o$ \\
$\mathsf{In}_\nu$; $\mathcal{V}$ & declared interface of input wire $\nu$; validity predicates of $\mu$ \\
$n$; $\lambda$ & DPF input length in bits; PRG seed length ($\lambda=128$) \\
$\alpha$, $\beta$, $x$ & DPF target, payload in $\Fp$, verified public query \\
$\CW^{(i)}$; $\CWout$ & level-$i$ correction word; output correction \\
$(s_c,t_c)$; $(\tilde s,\tilde t)$ & generator state of root $c\in\{0,1\}$; evaluator state of $T_b$ \\
$\tilde y_b$ & raw local output of the protected evaluator \\
$\zeta$; $\kappa_j$ & fresh common epilogue pads for the value; for lane $j$ \\
$m$; $h_b$; $\mathit{cid}$ & batch size; frozen root of $T_b$; check identifier \\
$\rho_{j,i}$; $\sigma_{b,j}$ & challenge of lane $j$ at batch position $i$; residual of $T_b$ in lane $j$ \\
$\bm{e}$; $\bm{d}_j$ & value-error vector; tag-error vector of lane $j$ in a checked batch \\
$Q$ & number of checked batches in one execution \\
$w$ & LUT input width (\cref{sec:proto-gates}) \\
\hline
\end{tabular}
\end{table}

% ======================================================================
\subsection{Authenticated Representation}\label{sec:proto-repr}

\textbf{Field and MAC lanes.}
All protocol arithmetic is over $\Fp$ with the Mersenne prime $p=2^{61}-1$. The modules hold $t=3$ independent global MAC keys $\Delta_1,\Delta_2,\Delta_3\getsr\Fp$, each additively split as $\Delta_j=\Delta_{0,j}+\Delta_{1,j}$; host~$b$ holds only $\Delta_{b,j}$, which it needs to add public values to its tags. Party $b$ holds an authenticated value $\auth{x}$ as
\begin{gather*}
\authb{x}{b}=(x_b,\gamma_{b,1},\gamma_{b,2},\gamma_{b,3}),\\
x_0+x_1=x,\qquad \gamma_{0,j}+\gamma_{1,j}=\Delta_j x\quad (j\in[t]),
\end{gather*}
which is the SPDZ representation~\cite{damgard2012spdz,damgard2013practical} with three independent lanes. A canonical wire occupies four 64-bit words, i.e., 32~B per party before metadata. Every element is encoded as an unsigned 64-bit integer smaller than $p$; the module parser rejects noncanonical encodings instead of reducing arbitrary integers modulo $p$, which keeps frozen bytes and checked field elements in one-to-one correspondence.

\textbf{Why three lanes over a 61-bit field.}
The Mersenne modulus lets the GPU compute exact products of canonical elements with native 64-bit multiplies and two folding steps (\cref{sec:arch-field}), so all $1+t$ lanes of authenticated linear algebra stay on standard integer datapaths. A single 61-bit tag is too weak: for $Q\le 2^{32}$ checked batches, $t=3$ is the smallest lane count whose statistical term $Q(2/p)^t$ falls below $2^{-128}$ (\cref{sec:sec-concrete}, \cref{tab:lanes}), and every lane is paid for in GPU work (\cref{sec:eval-ablation}).

\textbf{Why a field and not $\Z_{2^{64}}$.}
The soundness proof divides by a nonzero error coordinate and therefore needs a field (\cref{sec:sec-concrete}, \cref{app:proof-auth}). The encoding is thus not bit-identical to the $\Z_{2^{64}}$ arithmetic of FSS-compiled models~\cite{gupta2023sigma,jawalkar2024orca}. \sys fixes the numeric contract in the manifest (fixed-point scale, signed encoding, exact toward-zero truncation of \cref{sec:proto-gates}, magnitudes below $p/2$); a deployment that needs ring semantics must use a SPDZ2k-type backend~\cite{cramer2018spdz2k} with its own proof.

% ======================================================================
\subsection{Session Setup and Joint Randomness}\label{sec:proto-setup}

\textbf{Session setup.}
Each module authenticates its peer's identity, code and configuration measurement, role and freshness contribution. An authenticated key establishment then binds the ordered pair of identities, the roles 0 and 1, a fresh session identifier, the epoch, the manifest hash $\Hash(\mu)$, the field and tag parameters and the protocol version, and yields the session key $K$ known only to $T_0$ and $T_1$. Any failure aborts. We treat this step as an explicit setup assumption with error $\eps{setup}$ (\cref{thm:main}) and propose no new attestation protocol; attestation certifies what runs inside a module, not what the GPU computes (\cref{sec:bg-dfa}).

\textbf{Labels and joint draws.}
All module randomness is derived as $\PRF_K(\ell)$, or with an equivalent key derivation function (KDF)~\cite{krawczyk2010hkdf}, where $\ell$ is an unambiguous, length-prefixed encoding of $(\mathsf{session},\mathsf{epoch},\mathsf{gate},\mathsf{purpose},\mathsf{logical\_draw},\mathsf{block})$. A \emph{logical joint draw} uses the same label in both modules and thus yields the same value in $T_0$ and $T_1$ without communication; this is how both modules obtain identical DPF roots, correction words, masks, triples, pads and challenges. Distinct roots, pads, triple components, challenge lanes and rejection-sampling retries receive distinct labels. Two rules are easy to get wrong. The local role must \emph{not} be appended to a joint draw, since $T_0$ and $T_1$ would then generate two unrelated DPF instances whose outputs no longer add up; and the logical root-0 and root-1 draws of one DPF \emph{must} be different draws. Since labels name session, epoch and gate, the ledger detects replayed or misrouted material (S4, S5). A uniform element of $\Fp$ is obtained by rejection sampling: take 61 pseudorandom bits and reject the single value $p$, which occurs with probability $2^{-61}$; a bounded implementation aborts when its retry budget is exhausted instead of introducing a silent bias.

\textbf{Authenticated correlations.}
To share a protected value $v$, the joint sampler runs \AuthShare{}: it samples $v_0\getsr\Fp$ and sets $v_1=v-v_0$, independently samples $\gamma_{0,j}\getsr\Fp$ and sets $\gamma_{1,j}=\Delta_j v-\gamma_{0,j}$ for $j\in[t]$, and gives party $b$ only its tuple $\authb{v}{b}$. A multiplication triple samples $a,b\getsr\Fp$, computes $c=ab$ \emph{correctly inside the protected boundary} and authenticates all three values independently (S7); a matrix triple satisfies the actual equality $C=AB$ for its declared dimensions. Because both modules derive the same correlations from joint labels, preprocessing crosses no network link.

% ======================================================================
\subsection{One-Time Ledger and Release Guard}\label{sec:proto-ledger}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_ledger.pdf}
    \caption{Per-gate lifecycle enforced by the one-time ledger of $T_b$. Solid arrows are the only permitted transitions, each triggered by the named module command (\cref{tab:commands}). An accepted \cmd{CHECK_OPEN} only sets \lstate{VERIFIED}; \cmd{EVAL_FSS} consumes the opening of an FSS or direct gate, and an output gate, which runs no \cmd{EVAL_FSS}, is moved by \cmd{FINAL_OUTPUT} through \lstate{CONSUMED} to \lstate{RELEASED}. Any other transition or any failed check moves the gate to \lstate{ABORTED}, poisons the epoch and keeps the release guard closed.}
    \label{fig:ledger}
\end{figure}

\textbf{Ledger states.}
Each module keeps an authoritative protected ledger that binds every gate to its operation, predecessor and output wires, numeric type, table or model hash, public dimensions and allowed command sequence. A gate transaction moves only along
\lstate{NEW} $\rightarrow$ \lstate{RESERVED} $\rightarrow$ \lstate{PREPARED} $\rightarrow$ \lstate{FROZEN} $\rightarrow$ \lstate{VERIFIED} $\rightarrow$ \lstate{CONSUMED} $\rightarrow$ \lstate{RELEASED}
(\cref{fig:ledger}). Reservation burns the gate's randomness identifiers \emph{before} any preprocessing share is issued, so no label is ever issued twice. \lstate{PREPARED} lets the module issue the authorized party-local preprocessing exactly once; it is not permission to release an unchecked result. \lstate{CONSUMED} records the one-time use of verified openings and preprocessing, and \lstate{RELEASED} records that the result left the module under a certificate. Any invalid transition or failed check moves the gate to \lstate{ABORTED} and poisons the whole epoch: outstanding output responses are gated, no new challenge is derived, and aborted reservations never return to a free list.

\textbf{Freeze semantics.}
Before any checking challenge is drawn, $T_b$ copies the exact submitted value and tag bytes into protected storage, or spills them into AEAD-protected immutable pages~\cite{dworkin2007gcm} bound to sequence numbers, exact lengths, gate identifiers and a protected root. It hashes the complete descriptor and these bytes into a frozen root $h_b$, and the two modules agree on the ordered pair $(h_0,h_1)$. A host's claim that ``this buffer has hash $h$'' is not a freeze, and neither is DMA completion. After challenge generation, $T_b$ rereads only authenticated frozen pages and never verifies one buffer but consumes a later, host-modified one. This closes the time-of-check-to-time-of-use window (S3) that exists whenever checked data live in host or GPU memory.

\textbf{Release certificates and the guard.}
A release certificate binds the session, epoch, gate, recipients, output encoding or hash and terminal status. A missing peer acknowledgement can cause an abort, but it never authorizes output under a different transcript. The release guard is a small state machine in front of the module's output path (\cref{sec:arch-hw}); its enabling inputs originate from the protected checkers and the ledger, never from host-writable registers, so a host cannot open it by writing a status bit (S6). Resetting the guard is not a secure session reset.

\textbf{Reboot and rollback.}
After a reboot, either a separately justified trusted monotonic service preserves freshness~\cite{parno2011memoir,matetic2017rote}, or the old master key is irrecoverably erased and a freshly attested session is required. A host-controlled counter file is not anti-rollback protection, because the host can restore an old copy and replay old masks (S4).

% ======================================================================
\subsection{Malicious Generate-and-Consume}\label{sec:proto-gac}

\textbf{From semi-honest to malicious GaC.}
\Cref{alg:gac} interleaves \cref{alg:gen,alg:eval} with the three separate states of \cref{sec:analysis-dpf}: two generator states on the target path, started from $t_0=0$ and $t_1=1$, and an evaluator state on the query path, started from its own root seed and the fixed control bit $b$, never from a later generator state. Each correction word is computed from the expanded children of the two generator seeds and the target bit $\alpha_i$, applied to the generator states under their old bits $t_c$ and to both evaluator children under the evaluator's old bit $\tilde t$, and erased only after that use; $t\cdot s$ denotes a conditional XOR. The hardware keeps the two state sets in distinct contexts (\cref{sec:arch-pipe}), and the per-level work, which still duplicates generation in both modules, is accounted in \cref{tab:gatecost}.

\textbf{Inputs and outputs.}
The query $x$ is read from a verified masked opening of the same gate, never from unchecked host data: for instance the opened $c$ of an interval gate, whose prefix DPFs are queried at $c$ (\cref{alg:interval,alg:dcf}), whereas in a LUT gate the opened $u$ only permutes the table index while $\EvalAll$ visits every $a$ (\cref{alg:lut}). The target $\alpha$ and payload $\beta$ come from the gate's protected preprocessing record, so they are joint draws or joint functions of joint draws (\cref{sec:proto-refactor}). By \cref{thm:dpf-correct,thm:gac}, the raw outputs satisfy $\tilde y_0+\tilde y_1=\beta\cdot\one[x=\alpha]$, but $\tilde y_b$ never leaves the module: the epilogue lines of \cref{alg:gac} replace it with a freshly authenticated tuple. Since neither keys nor raw shares are exported, \cref{thm:main} needs no DPF key-privacy term. Gates that combine several DPF evaluations (interval prefixes, LUT and PIR scans) run only the (Gen) and (Eval) lines per constituent DPF and apply the ledger lines and one epilogue to their combined raw share, for PIR only its value pad (\cref{app:proof-dpf}). For full-domain uses such as LUT gates and PIR, the evaluator lines become the depth-first $\EvalAll$ traversal of \cref{alg:eval}; each $\CW^{(i)}$ then stays in protected registers until its last evaluator use, which costs $O(n)$ words and is covered by the same node-by-node coupling.

\begin{algorithm}[t]
\algstretch
\small
\caption{Malicious generate-and-consume with fresh authentication (\algname{GaC-Auth}) inside $T_b$}
\label{alg:gac}
\begin{algorithmic}[1]
\Require role $b\in\{0,1\}$; gate label $\ell$; public query $x\in\bits{n}$ from the gate's frozen, verified opening; target $\alpha\in\bits{n}$ and payload $\beta\in\Fp$ from the protected record of $\ell$; session key $K$; global keys $\Delta_1,\dots,\Delta_t$
\Ensure $\authb{y}{b}=(y_b,\gamma_{b,1},\dots,\gamma_{b,t})$ with $y_0+y_1=\beta\cdot\one[x=\alpha]$ and $\gamma_{0,j}+\gamma_{1,j}=\Delta_j(y_0+y_1)$
\If{gate $\ell$ is not \lstate{VERIFIED} in the ledger}
  \State \Abort{} and poison the epoch
\EndIf
\LineComment{Joint draws: identical labels in $T_0$ and $T_1$, no role appended}
\State $s_0\gets\PRF_K(\ell,\mathsf{root}_0)$;\ $s_1\gets\PRF_K(\ell,\mathsf{root}_1)$;\ $t_0\gets 0$;\ $t_1\gets 1$
\State $(\tilde s,\tilde t)\gets(s_b,b)$ \Comment{separate evaluator}
\For{$i=1$ \textbf{to} $n$}
  \LineComment{(Gen) both roots on the target path; updates use the old $t_c$}
  \State $(s_c^L,t_c^L,s_c^R,t_c^R)\gets\PRG(s_c)$ for $c\in\{0,1\}$
  \State $a\gets\alpha_i$;\ $\keep\gets a$;\ $\lose\gets 1-a$ \Comment{$L\equiv 0$, $R\equiv 1$}
  \State $\sCW\gets s_0^{\lose}\oplus s_1^{\lose}$
  \State $\tCW{L}\gets t_0^L\oplus t_1^L\oplus a\oplus 1$;\ \ $\tCW{R}\gets t_0^R\oplus t_1^R\oplus a$
  \State $(s_c,t_c)\gets\big(s_c^{\keep}\oplus t_c\cdot\sCW,\ t_c^{\keep}\oplus t_c\cdot\tCW{\keep}\big)$, $c\in\{0,1\}$
  \LineComment{(Eval) own query path; corrections use the old $\tilde t$}
  \State $(\hat s^L,\hat t^L,\hat s^R,\hat t^R)\gets\PRG(\tilde s)$
  \State $(\hat s^L,\hat t^L)\gets\big(\hat s^L\oplus\tilde t\cdot\sCW,\ \hat t^L\oplus\tilde t\cdot\tCW{L}\big)$
  \State $(\hat s^R,\hat t^R)\gets\big(\hat s^R\oplus\tilde t\cdot\sCW,\ \hat t^R\oplus\tilde t\cdot\tCW{R}\big)$
  \State $(\tilde s,\tilde t)\gets(\hat s^{x_i},\hat t^{x_i})$
  \State erase $\CW^{(i)}=(\sCW,\tCW{L},\tCW{R})$ \Comment{after its evaluator use}
\EndFor
\LineComment{(Gen) output correction from the final generator states}
\State $u_c\gets\Conv(s_c)$ for $c\in\{0,1\}$;\ \ $\CWout\gets(-1)^{t_1}(\beta-u_0+u_1)$
\LineComment{(Eval) raw share, never exported}
\State $\tilde y_b\gets(-1)^b\big(\Conv(\tilde s)+\tilde t\cdot\CWout\big)$; erase $s_c$, $t_c$, $\CWout$
\LineComment{(Epilogue) fresh uniform pads, distinct labels per output wire}
\State $\zeta\gets\PRF_K(\ell,\mathsf{pad}_0)$;\ \ $\kappa_j\gets\PRF_K(\ell,\mathsf{pad}_j)$ for $j\in[t]$
\State $y_b\gets\tilde y_b+(-1)^b\zeta$
\State $\gamma_{b,j}\gets\Delta_j\,y_b+(-1)^b\kappa_j$ for $j\in[t]$
\State mark $\ell$ \lstate{CONSUMED}; erase $\tilde y_b$, $\zeta$, $\kappa_1,\dots,\kappa_t$, $(\tilde s,\tilde t)$
\State \Return $\authb{y}{b}$ to the output FIFO behind the release guard
\end{algorithmic}
\end{algorithm}

% ======================================================================
\subsection{Fresh Authentication Epilogue}\label{sec:proto-epilogue}

\textbf{Construction.}
Let $\tilde y_0,\tilde y_1$ be raw local shares computed inside the two protected evaluators, with $\tilde y_0+\tilde y_1$ equal to the intended gate value. Both modules derive fresh common pads $\zeta,\kappa_1,\dots,\kappa_t\getsr\Fp$ from joint labels that are distinct for every output wire, and $T_b$ returns
\begin{equation*}
y_b=\tilde y_b+(-1)^b\zeta,\qquad \gamma_{b,j}=\Delta_j\,y_b+(-1)^b\kappa_j\quad (j\in[t]).
\end{equation*}
The pads cancel in $y_0+y_1$ and in $\gamma_{0,j}+\gamma_{1,j}=\Delta_j(y_0+y_1)$, so the result is an authenticated sharing of $\tilde y_0+\tilde y_1$, and each party's tuple is uniform on $\Fp^{1+t}$ whatever the gate value and the global keys (\cref{thm:epilogue}). Fresh pads make this hold jointly across outputs; correlations created by later arithmetic are handled by the circuit simulation of \cref{thm:main}.

\textbf{Why it replaces tag trees.}
Instead of $t$ further DPF trees with payloads $\Delta_j\beta$, the epilogue exploits the linearity of the MAC. Because $T_b$ knows the global $\Delta_j$, the tag of the reconstructed value is the sum of the per-party products $\Delta_j y_b$; the pad $\kappa_j$ hides $\Delta_j y_b$ from host $b$, which knows $y_b$ and could otherwise divide it out. The pad $\zeta$ rerandomizes the raw DPF share, so no host ever sees $\tilde y_b$. The cost is one raw DPF computation, three field multiplications and four fresh pads per party and output, and the output is a 32~B tuple.

\textbf{API restriction.}
The epilogue accepts only results computed inside the module, namely the DPF, DCF, LUT, interval and direct gates of \cref{sec:proto-gates,sec:proto-direct} and the PIR reductions of \cref{sec:proto-pir}, or results from an explicitly verified backend such as the frozen-operand Freivalds check of \cref{sec:proto-freivalds}. There is no \cmd{authenticate(host_value)} entry point. With one, the module would become a MAC oracle: a malicious host could obtain valid tags on any value it wishes to open, and \CheckOpen{} would accept the forgery with probability one (S2). Since the trusted boundary excludes the GPU SMs and memory, a malicious-secure extension must never compute an unchecked result on the GPU and ask the module to authenticate it.

% ======================================================================
\subsection{Freeze-Before-Challenge CheckOpen}\label{sec:proto-check}

\begin{algorithm}[t]
\algstretch
\small
\caption{Freeze-before-challenge authenticated opening (\CheckOpen) inside $T_b$}
\label{alg:checkopen}
\begin{algorithmic}[1]
\Require descriptor and nonempty ordered list of expected wires $(\nu_i)_{i\in[m]}$; host $b$'s tuples $(x_{b,i},\gamma_{b,j,i})_{i\in[m],\,j\in[t]}$; key shares $(\Delta_{b,j})_{j\in[t]}$ from the protected key store of $T_b$ (never from host input)
\Ensure verified openings $(z_i)_{i\in[m]}$ with bound certificates, or \Abort
\If{metadata, field encoding, gate order or length mismatch the ledger}
  \State \Abort{} and poison the epoch
\EndIf
\LineComment{Step 1: freeze, then agree on both roots}
\State copy the exact bytes into protected SRAM or sealed AEAD pages; $h_b\gets\Hash(\text{descriptor},\text{frozen bytes})$; mark \lstate{FROZEN}
\State exchange $(h_b,\mathit{cid})$ with $T_{1-b}$; \Abort{} unless both hold the same $(h_0,h_1)$ and $\mathit{cid}$
\LineComment{Step 2: reconstruct candidates inside the modules}
\State exchange the frozen value shares $(x_{b,i})_{i\in[m]}$ with $T_{1-b}$
\State $z_i\gets x_{0,i}+x_{1,i}$ for $i\in[m]$ \Comment{not exposed to the host}
\LineComment{Step 3: internal challenges, only after both freezes}
\State $\rho_{j,i}\gets\PRF_K(\mathsf{chk},h_0,h_1,\mathit{cid},j,i)$ for $j\in[t]$, $i\in[m]$
\LineComment{Step 4: per-lane residuals from frozen pages only}
\State $\sigma_{b,j}\gets\sum_{i=1}^{m}\rho_{j,i}\,(\gamma_{b,j,i}-\Delta_{b,j}z_i)$ for $j\in[t]$
\State exchange $(\sigma_{b,j})_{j\in[t]}$ with $T_{1-b}$
\LineComment{Step 5: decide and release}
\If{$\sigma_{0,j}+\sigma_{1,j}=0$ for every $j\in[t]$}
  \State agree on output digest and status; mark \lstate{VERIFIED}; record the checked material as used
  \State \Return $(z_i)_{i\in[m]}$ with certificates bound to session, epoch, gates and output hash
\Else
  \State release no candidate value; poison the epoch; return one generic failure status
\EndIf
\end{algorithmic}
\end{algorithm}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_checkopen.pdf}
    \caption{Freeze-before-challenge \CheckOpen{} between the two modules. Challenges $\rho_{j,i}$ are derived only after both frozen roots are agreed, and $T_b$ rereads only its frozen pages, so a host that overwrites its DMA buffer after the freeze changes nothing that is checked or consumed.}
    \label{fig:checkopen}
\end{figure}

\textbf{Role.}
Openings are the only places where a value produced by the untrusted GPU becomes public or feeds a protected gate: the masked differences of every multiplication, the masked inputs of every FSS gate and the masked outputs. \CheckOpen{} (\cref{alg:checkopen}, \cref{fig:checkopen}) is a SPDZ-style batched MAC check~\cite{damgard2012spdz,damgard2013practical} rebuilt for a verifier that reads its inputs from untrusted memory (S1, S3). All peer messages use the protected channel, and only an accepted batch releases $z$ with bound certificates.

\textbf{Independent challenge lanes.}
Let $\bm{e}$ be the value-error vector of a batch and $\bm{d}_j$ its tag-error vector in lane $j$, i.e., the differences between the submitted and the prescribed tuples. The freeze fixes $(\bm{e},\bm{d}_j)$ before any $\rho_{j,i}$ exists, so a host cannot place its errors in the kernel of a challenge (\cref{app:proof-auth}). Each lane has its own challenge vector $\bm{\rho}_j$. The complete residual of lane $j$ is $\inner{\bm{\rho}_j}{\bm{d}_j-\Delta_j\bm{e}}$, which for $\bm{e}\neq\bm{0}$ vanishes with probability below $2/p$; independence across lanes multiplies these bounds to $(2/p)^t$ (\cref{thm:mac-sound}). A shared vector collapses the product to one lane, and tag-only errors escape with probability $1/p$ without changing an opened value (\cref{sec:sec-concrete}, \cref{app:proof-auth}).

\textbf{Key hiding and failure handling.}
The bound relies on the hidden-key invariant of \cref{lem:hidden-key}: until the first accepted wrong opening, the honest key shares stay uniform given the corrupt host's view. \CheckOpen{} preserves it in three ways. Candidates, challenges and residuals never leave the modules. The zero tests of all lanes are aggregated into one generic failure status that exposes no residual, challenge, key or data-dependent diagnostic. A failure poisons the epoch and forbids retries with the same material, which rules out an adaptive key-learning sequence within an epoch.

\textbf{Traffic and batching.}
Per batch of $m$ elements, the modules exchange two vectors of $m$ field values and two vectors of $t$ residuals plus authenticated metadata. Tags never cross the peer link, but every local tag must be read by its module, so the host-to-module transfer of 32~B per element can remain the bottleneck (\cref{sec:arch-dse}). Because the value shares are frozen before they are sent, root agreement and value exchange can share one message, and our latency model charges two peer round trips per batch. Only independent openings are batched: a dependent nonlinear gate never consumes an unchecked masked opening, and a checkpoint precedes every input-dependent nonlinear output and every final release, since blindly delayed checking is not justified. Larger batches amortize metadata and round trips but increase staging memory and first-result latency (costs in \cref{sec:eval-check}).

% ======================================================================
\subsection{Inputs, Arithmetic, and Outputs}\label{sec:proto-arith}

\begin{figure*}[t]
\centering
\footnotesize
\setlength{\fboxsep}{4pt}
\fbox{%
\begin{minipage}[t]{0.472\textwidth}
\textbf{Input} $\Pi_{\mathsf{Input}}$\hfill\textit{input $x$ of endpoint $O$ for wire $\nu$}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: reserve label $\ell_\nu$; joint draw $r\getsr\Fp$ and $\authb{r}{b}\gets\AuthShare(r)$; issue $\authb{r}{b}$ to host $b$ once.
\item $T_0,T_1$: send the complete $r$ only to $O$ over its authenticated confidential channel.
\item $O$: send the canonical, authenticated $\varepsilon=x-r$ to $T_0$ and $T_1$.
\item $T_0,T_1$: confirm over the protected channel that both hold the same $\varepsilon$ and bind it to $\nu$; compute $x^*=r+\varepsilon$ and \Abort{} unless $x^*\in\mathsf{In}_\nu$. $T_b$ then hands the bound $\varepsilon$ to host $b$.
\item host $b$: $x_b\gets r_b+\one[b=0]\,\varepsilon$;\ \ $\gamma_{b,j}\gets\gamma_{r,b,j}+\Delta_{b,j}\,\varepsilon$ for $j\in[t]$.
\end{enumerate}
\textit{Extraction:} a corrupt owner's input is $x^*=r+\varepsilon$.
\textit{Validation:} at the public boundaries declared in $\mu$, after every input gate and before the first output opening, $T_0,T_1$ evaluate every predicate of $\mathcal{V}$ on the bound inputs and \Abort{} if one fails.
\textit{Committed inputs:} a protected loader verifies the authorized commitment over the frozen canonical stream, then runs \AuthShare{} on the exactly decoded values.

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Linear} $\Pi_{\mathsf{Lin}}$\hfill\textit{local, on host $b$'s GPU}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $\auth{x}+\auth{y}$: add the value shares and each of the $t$ tag shares.
\item $c\cdot\auth{x}$ for public $c$: multiply the value share and every tag share by $c$.
\item $\auth{x}+c$ for public $c$: $x_0\gets x_0+c$ (party~0 only); $\gamma_{b,j}\gets\gamma_{b,j}+\Delta_{b,j}\,c$ for both $b$ and all $j\in[t]$.
\item Tensors: apply steps 1 to 3 elementwise to the value array and to each of the $t$ tag arrays.
\end{enumerate}

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Output} $\Pi_{\mathsf{Out}}$\hfill\textit{private output $y$ for client $O$}
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: joint draw a fresh $\auth{o}$ as in step 1 of $\Pi_{\mathsf{Input}}$; send the complete $o$ only to $O$.
\item host $b$: $\auth{\upsilon}\gets\auth{y}+\auth{o}$ with $\Pi_{\mathsf{Lin}}$.
\item $\upsilon\gets\CheckOpen(\auth{\upsilon})$; the release guard opens only for a \mbox{\lstate{VERIFIED}} batch.
\item $T_b$: send $\upsilon$ and its release certificate (session, epoch, gate, recipients, output hash, status) to $O$.
\item $O$: verify both certificates for the same $\upsilon$ and output $y=\upsilon-o$; otherwise abort.
\end{enumerate}
\textit{Public outputs:} $y\gets\CheckOpen(\auth{y})$.
\textit{Never} hand $O$ both parties' tags: $\gamma_{0,j}+\gamma_{1,j}=\Delta_j y$ with a known $y\neq 0$ reveals $\Delta_j$.
\end{minipage}%
\hspace{0.01\textwidth}\vrule\hspace{0.01\textwidth}%
\begin{minipage}[t]{0.472\textwidth}
\textbf{Multiplication} $\Pi_{\mathsf{Mult}}$\hfill\textit{authenticated Beaver triples}

\textit{Scalar} $\auth{z}=\auth{x}\cdot\auth{y}$:
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep]
\item $T_0,T_1$: reserve a fresh triple $(\auth{a},\auth{b},\auth{c})$ from joint draws, with $c=ab$ computed inside the protected boundary; issue party $b$'s tuples to host $b$ once.
\item host $b$: $\auth{d}\gets\auth{x}-\auth{a}$ and $\auth{e}\gets\auth{y}-\auth{b}$ with $\Pi_{\mathsf{Lin}}$.
\item $(d,e)\gets\CheckOpen(\auth{d},\auth{e})$, batched with the independent openings of the layer.
\item host $b$: $z_b\gets c_b+d\,b_b+e\,a_b+\one[b=0]\,de$.
\item host $b$: $\gamma_{z,b,j}\gets\gamma_{c,b,j}+d\,\gamma_{b,b,j}+e\,\gamma_{a,b,j}+\Delta_{b,j}\,de$ for $j\in[t]$.
\end{enumerate}
\textit{Matrix} $\auth{Z}=\auth{X}\auth{Y}$ with declared dimensions:
\begin{enumerate}[label=\arabic*:,leftmargin=1.6em,labelsep=0.4em,nosep,start=6]
\item $T_0,T_1$: reserve $(\auth{A},\auth{B},\auth{C})$ with $C=AB$ computed inside the protected boundary; never expose both $A$ and $B$ to a GPU.
\item $D\gets\CheckOpen(\auth{X}-\auth{A})$;\ \ $E\gets\CheckOpen(\auth{Y}-\auth{B})$.
\item host $b$: $Z_b\gets C_b+D\,B_b+A_b\,E+\one[b=0]\,DE$.
\item host $b$: $\Gamma_{Z,b,j}\gets\Gamma_{C,b,j}+D\,\Gamma_{B,b,j}+\Gamma_{A,b,j}\,E+\Delta_{b,j}\,DE$ for $j\in[t]$, preserving the order of every matrix factor.
\end{enumerate}
\textit{Notation:} in $b_b$ and $\gamma_{b,b,j}$ the first $b$ names the triple's second component and the subscript names the party (implementations use named fields); $\Gamma_{\cdot,b,j}$ is party $b$'s lane-$j$ tag matrix.

\vspace{3pt}\hrule\vspace{3pt}
\textbf{Invariants shared by all four protocols}
\begin{itemize}[leftmargin=1.1em,nosep]
\item Every mask and triple is a one-time joint draw bound to session, epoch, gate and purpose, and is issued only from \mbox{\lstate{PREPARED}} (\cref{fig:ledger}).
\item Every opening is a \CheckOpen{} call on frozen bytes (\cref{alg:checkopen}); no opened value feeds a protected gate or a release before it is \mbox{\lstate{VERIFIED}}.
\item Outputs of host $b$'s GPU are candidate shares; no module ever authenticates them.
\end{itemize}
\end{minipage}}
\caption{Authenticated input, linear, multiplication and output protocols of \sys, written for party $P_b$. Steps labeled $T_0,T_1$ or $T_b$ run inside the protected modules; steps labeled host $b$ run on the untrusted GPU and yield only candidate shares until the next \CheckOpen. With honest messages the protocols realize their operations exactly; otherwise they select an allowed input, preserve the computation or abort, except with the probability bounded in \cref{thm:mac-sound} (\cref{thm:arith}).}
\label{fig:arith}
\end{figure*}

\Cref{fig:arith} specifies the four protocols that carry values between input owners, GPUs, modules and recipients; three points of rationale are not visible in the box.

\textbf{Inputs.}
The difference $\varepsilon$ is uniform for a uniform $r$, so the hosts learn nothing about $x$. Both modules bind one $\varepsilon$, so a corrupt owner cannot feed the two parties different inputs, and its input is extracted as $x^*=r+\varepsilon$ (S9, \cref{def:security}). Canonical encoding alone does not place $x^*$ in the declared interface; since the modules generated $r$, they compute $x^*$ and abort unless $x^*\in\mathsf{In}_\nu$. The validity predicates $\mathcal{V}$ of $\mu$ are evaluated inside the modules at public boundaries that the schedule of $\mu$ places after every input gate and before the first output opening; their accept or abort outcome is the $\mathsf{status}$ component of $\Leak_C$ (\cref{def:leakage}), and the simulator emulates the same abort (\cref{thm:main}). For committed inputs such as preapproved model weights, a host-declared hash does not suffice; the loader hashes exactly the bytes it shares. The modules thus see every input, which \ProfT permits (\cref{sec:threat-model}).

\textbf{Arithmetic.}
Multiplication follows Beaver~\cite{beaver1991efficient} with authenticated triples. An authenticated matrix product costs the GPU $2(1+t)$ plain products plus the public $DE$, which is why authenticated linear algebra, rather than DPF evaluation, dominates the malicious cost (\cref{sec:analysis-cost}).

\textbf{Outputs.}
The recipient accepts $\upsilon$ only with matching certificates from both modules, so integrity toward a client comes from these certificates, never from MAC tags.


==> qa/draft4/sections/05b_protocol_gates.tex <==
% ==================================================================
% Section V (part 2): authenticated nonlinear gates, direct gates and
% compilation, refactoring, verified GPU products, snapshot PIR.
% Continues the Section opened in 05a_protocol.tex (no \section here).
% ==================================================================

\subsection{Authenticated Nonlinear Gates}\label{sec:proto-gates}

Nonlinear layers of FSS-compiled models reduce to lookups in small public tables and piecewise functions selected by interval tests~\cite{boyle2021function,gupta2023sigma,jawalkar2024orca}. In the semi-honest DFA design, both parties evaluate a DPF or DCF key on a masked input and pass the raw output shares onward~\cite{dfa2026trusted}. A malicious host can shift the masked input before it selects the DPF path, and it can modify the raw outputs, which carry no MAC. \sys closes both gaps with one template (\cref{fig:gates}): (1)~mask the authenticated input with joint protected randomness (\cref{sec:proto-setup}); (2)~open the masked value with \CheckOpen{} (\cref{alg:checkopen}), so the value that selects the path is verified and frozen; (3)~evaluate the FSS gate inside $T_b$ with the (Gen) and (Eval) steps of generate-and-consume (\cref{alg:gac}); and (4)~authenticate and reshare the gate's combined raw share with one epilogue (\cref{sec:proto-epilogue}). The host sees only a uniform masked opening and fresh authenticated tuples, and no host-supplied value is ever authenticated, which defeats scenario S2 (\cref{tab:scenarios}).

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/fig_gates.pdf}
    \caption{Authenticated nonlinear gates in \sys. (a)~Small XOR-masked LUT (\cref{alg:lut}): the XOR-masked bit vector $u$ is opened by \CheckOpen{} and $T_b$ scans the full public domain in a fixed order. (b)~Shifted-interval indicator and Horner polynomial (\cref{alg:interval}): one field opening $c=x+r$ serves both translated thresholds $L$ and $H$, which derive from the same mask. (c)~Direct protected gate (\cref{sec:proto-direct}): the module recovers $x=c-r$ inside its boundary and returns a fresh sharing of $g(x)$. In all three cases the host submits only authenticated shares and receives only freshly authenticated outputs; raw FSS shares, DPF keys and, in (c), the plaintext $x$ never leave $T_b$.}
    \label{fig:gates}
\end{figure*}

\begin{algorithm}[t]
\algstretch
\caption{Authenticated small XOR-masked LUT (\algname{LUT-Auth}) for party $b$}
\label{alg:lut}
\begin{algorithmic}[1]
\Require authenticated bits $\authb{x_1}{b},\dots,\authb{x_w}{b}$ of an unsigned $w$-bit $x$, certified Boolean; approved public table $T\in\Fp^{2^w}$ bound in $\mu$ by its hash; gate identifier $\mathit{gid}$; role $b$
\Ensure $\authb{y}{b}$ with $y=T[x]$
\State $T_b$: \cmd{RESERVE_PREP} for $\mathit{gid}$; \Abort{} on any descriptor or table-hash mismatch
\LineComment{Joint preparation inside $T_b$ (same $r$ in $T_0$ and $T_1$)}
\State $r\getsr\bits{w}$ by one joint draw with label $(\mathit{gid},\textsf{mask})$
\State issue $\authb{r_i}{b}\gets\AuthShare(r_i)$ to host $b$ once, for $i=1,\dots,w$
\State bind the joint DPF generator of $(\alpha,\beta)=(r,1)$ to $\mathit{gid}$ \Comment{never resampled}
\LineComment{Masked opening (host $b$ with $T_b$)}
\For{$i=1$ \textbf{to} $w$} \Comment{independent: one batch}
  \State $\authb{u_i}{b}\gets\authb{x_i}{b}+\authb{r_i}{b}-2\,\authb{x_ir_i}{b}$ \Comment{$\Pi_{\mathsf{Mult}}$}
\EndFor
\State $u\gets\CheckOpen(\auth{u_1},\dots,\auth{u_w})$ \Comment{$u=x\oplus r$}
\If{some $u_i\notin\{0,1\}$ or $T_0,T_1$ hold different $u$}
  \State \Abort
\EndIf
\LineComment{Full-domain scan inside $T_b$ in fixed public order; $k_b$ is streamed by GaC and never materialized}
\State $\tilde y_b\gets 0$
\For{$a\in\bits{w}$ in lexicographic order} \Comment{$\EvalAll$, depth-first}
  \State $\tilde y_b\gets\tilde y_b+T[a\oplus u]\cdot\DPF.\Eval(k_b,a)$
\EndFor
\State $\authb{y}{b}\gets\Epilogue(\tilde y_b)$ \Comment{\cref{sec:proto-epilogue}}
\State \Return $\authb{y}{b}$
\end{algorithmic}
\end{algorithm}

\textbf{Small XOR-masked LUT.}
\Cref{alg:lut} evaluates an approved public table $T$ with $2^w$ field entries on a $w$-bit input given as authenticated, certified-Boolean bits. The sampler draws a fresh uniform $r\in\bits{w}$ once and uses it twice: for the authenticated bits $\auth{r_i}$ and as the target of the joint DPF for $(r,1)$. The parties open $u=x\oplus r$ in one \CheckOpen{} batch, both modules reject a non-Boolean or mismatching vector, and $T_b$ scans the full domain in a declared fixed order,
\begin{equation*}
    \tilde y_b=\sum_{a\in\bits{w}}T[a\oplus u]\cdot\DPF.\Eval(k_b,a).
\end{equation*}
By \cref{thm:dpf-correct}, the evaluations sum to one only at $a=r$, so $\tilde y_0+\tilde y_1=T[r\oplus u]=T[x]$; since XOR with a fixed $x$ is a bijection on $w$-bit strings, $u$ is uniform given $x$ (\cref{thm:lut}). In $\EvalAll$ mode the $w$ correction words stay in protected registers until their level is fully expanded, so no key is materialized outside $T_b$. Besides the $w$ XOR products (one batched multiplication round when the bits exist; otherwise bit decomposition is charged to the gate), the gate needs one batched opening, $2^w-1$ internal tree expansions and a $2^w$-term field reduction: small tables are practical, full-domain tables over 64-bit inputs are not (\cref{tab:gates}).

\begin{algorithm}[t]
\algstretch
\caption{Authenticated shifted intervals and piecewise polynomial (\algname{Interval-Auth}) for party $b$}
\label{alg:interval}
\begin{algorithmic}[1]
\Require $\authb{x}{b}$; public breakpoints $0=\tau_0<\tau_1<\dots<\tau_m=p$ with $m\ge2$; public coefficients $a_{i,j}\in\Fp$ of $P_i(x)=\sum_{j=0}^{d}a_{i,j}x^j$; gate identifier $\mathit{gid}$; role $b$
\Ensure $\authb{y}{b}$ with $y=P_i(x)$ for the unique $i$ such that $\tau_i\le x<\tau_{i+1}$
\State $T_b$: \cmd{RESERVE_PREP} for $\mathit{gid}$; $r\getsr\Fp$ by one joint draw (rejection sampling); issue $\authb{r}{b}\gets\AuthShare(r)$ once
\State $c\gets\CheckOpen(\auth{x}+\auth{r})$ \Comment{$c=x+r\bmod p$}
\LineComment{Indicators inside $T_b$; every endpoint and wrap bit derives from the same $r$}
\For{$i=0$ \textbf{to} $m-1$}
  \State $L_i\gets(\tau_i+r)\bmod p$;\; $H_i\gets(\tau_{i+1}+r)\bmod p$
  \State $\omega_i\gets\one[L_i>H_i]$ with a sharing $(\omega_{i,0},\omega_{i,1})$
  \State $\tilde s_{i,b}\gets\omega_{i,b}+\DCF_{H_i}(c)_b-\DCF_{L_i}(c)_b$ \Comment{GaC}
  \State $\authb{s_i}{b}\gets\Epilogue(\tilde s_{i,b})$ \Comment{$s_i=\one[\tau_i\le x<\tau_{i+1}]$}
\EndFor
\LineComment{Coefficient selection and Horner evaluation (host $b$, authenticated arithmetic)}
\For{$j=0$ \textbf{to} $d$}
  \State $\authb{\bar a_j}{b}\gets\sum_{i=0}^{m-1}a_{i,j}\,\authb{s_i}{b}$ \Comment{local, $\Pi_{\mathsf{Lin}}$}
\EndFor
\State $\authb{y}{b}\gets\authb{\bar a_d}{b}$
\For{$j=d-1$ \textbf{down to} $0$}
  \State $\authb{y}{b}\gets\authb{y\cdot x}{b}+\authb{\bar a_j}{b}$ \Comment{$\Pi_{\mathsf{Mult}}$}
  \State rescale exactly where $\mu$ specifies (\cref{alg:trunc})
\EndFor
\State \Return $\authb{y}{b}$
\end{algorithmic}
\end{algorithm}

\textbf{Shifted intervals.}
For a proper nonempty public interval $[a,b)\subsetneq[0,p)$ (here $a,b$ are endpoints, not party indices), \cref{alg:interval} opens $c=x+r\bmod p$ for a fresh field mask $r$, and $T_b$ derives from the same $r$
\begin{equation*}
    L=(a+r)\bmod p,\quad H=(b+r)\bmod p,\quad \omega=\one[L>H].
\end{equation*}
With conservative DCFs for thresholds $L$ and $H$ (\cref{alg:dcf}; orientation $\one[c<\theta]$, payload $1$, independent coins) and a sharing of the wrap bit $\omega$, the raw share $\tilde s_b=\omega_b+\DCF_H(c)_b-\DCF_L(c)_b$ goes to the epilogue. Translation by $r$ maps $[a,b)$ onto the circular half-open interval from $L$ to $H$ ($L\neq H$ since $0<b-a<p$): the indicator is $\one[c<H]-\one[c<L]$ if $L<H$ and $1+\one[c<H]-\one[c<L]$ if the interval wraps, so \cref{thm:dcf} gives $\tilde s_0+\tilde s_1=\one[a\le x<b]$ (\cref{thm:interval}). Empty and full intervals are public constants. A partition may share one mask and one opening if every endpoint, wrap bit and auxiliary share is derived jointly from that mask, while distinct DCFs keep independent coins. The conservative DCF evaluates $n(n+1)/2$ path levels per threshold; its cost, and that of a projected $O(n)$ DCF~\cite{boyle2021function,storrier2023grotto} that \cref{thm:dcf} does not cover, are in \cref{tab:gates}.

\textbf{Piecewise polynomials.}
Activation and normalization functions are approximated by low-degree polynomials on a public partition~\cite{gupta2023sigma,pang2024bolt,ma2023secretflow}. The parties select coefficients $\auth{\bar a_j}=\sum_i a_{i,j}\auth{s_i}$ locally ($\Pi_{\mathsf{Lin}}$, \cref{fig:arith}) and apply Horner's rule with $d$ authenticated products, independently of the number $m$ of pieces. Exactly one indicator of a disjoint exhaustive partition is one, so \cref{thm:arith} yields the active polynomial; rescaling is inserted where the manifest specifies it (\cref{alg:trunc}). Approximation error of the approved coefficients is distinct from the cryptographic correctness of \cref{thm:lut,thm:interval}, which concerns the declared finite arithmetic.

\textbf{Exact comparison, bit decomposition and truncation.}
The LUT input, exact threshold comparisons and toward-zero signed truncation need canonical bits, which \cref{alg:bitdec,alg:trunc} (\cref{app:proof-gates}) derive with authenticated arithmetic alone (\cref{thm:bitdec,thm:cmp-trunc})~\cite{damgard2006unconditionally,catrina2010improved,escudero2020edabits}.

\textbf{Why exact circuits are a fallback.}
Their carry chains cannot be shortened by batching: \cref{alg:bitdec} performs $2n=122$ dependent multiplications for $n=61$, hence $2n+1=123$ sequential verified openings, and exact signed truncation chains two decompositions and a comparator into 307 authenticated multiplications and 309 sequential rounds, \est{30.9~ms} on LAN (\cref{tab:gates}). At two round trips per verified opening (\cref{sec:proto-check}), the 123-round chain alone would take about \est{17.2~s} on WAN. A valid one-round candidate therefore always wins under the cost rule below, and exact circuits are used only when no such candidate meets the gate's contract, with their cost charged to any LUT whose input bits do not yet exist.

\subsection{Direct Protected Gates and Cost-Aware Compilation}\label{sec:proto-direct}

\textbf{The direct protected gate.}
After a verified opening $c=x+r$, each module holds $c$ and $r$ and can compute $x=c-r$ inside its boundary, evaluate an approved deterministic gate $g$, and return a fresh authenticated sharing of $g(x)$ through \AuthShare{} (\cref{fig:gates}(c)). This is secure (\cref{thm:arith}) in the same model and with the same output simulation as the FSS gates, since the host again receives a fresh, independently uniform value and tag tuple (\cref{thm:epilogue}), provided the module's observable trace while computing $g$ meets the same simulatability assumption ($\eps{trace}$ in \cref{thm:main}). Concretely, fetching $T[x]$ from host memory or running in $x$-dependent time would leak $x$, so approved direct gates run from protected memory in data-independent time. A direct gate needs one verified opening, two AES blocks and five field multiplications; our model estimates \est{1{,}800}~M gates/s, above every FSS realization in \cref{tab:gates}.

\textbf{Cost-aware selection.}
For each nonlinear gate shape, the compiler estimates a cost tuple (latency, bytes, protected memory, field operations, PRG calls) for the direct gate, a small XOR LUT, an interval or polynomial FSS gate, and a separately proven malicious backend. It rejects candidates that violate the gate's semantic and security contract (the exact finite function, encoding and rescaling fixed by $\mu$ under the profile in force) and selects the least modeled end-to-end cost among the rest, accounting for dependency depth and transport; only independent checks are batched (\cref{sec:proto-check}). One constraint applies: gate shapes that the manifest marks as FSS-portable keep an FSS realization, so that the same compiled circuit runs under \ProfU. The compiler-selected default is therefore not the unconstrained minimum, and direct-only compilation is marginally faster (\est{3.82~s} versus \est{3.83~s} for BERT-Base on LAN).

\textbf{Why FSS stays in the datapath.}
If the direct gate is at least as cheap under \ProfT, why keep DPF generation and evaluation in the module? (i)~\emph{Compatibility.} Sigma- and Orca-style toolchains~\cite{gupta2023sigma,jawalkar2024orca} compile nonlinear layers into masked-input FSS gates, and \ProfU (\cref{sec:threat-profileu}) runs the circuit through an established malicious backend whose DPF keys the accelerator evaluates as party-local data; there the direct candidate is invalid because the hardware is not trusted with $x$. One DPF datapath serves both profiles and the untrusted-mode DFA workloads. (ii)~\emph{Full-domain scans.} PIR and small-LUT gates are data-independent, fixed-order scans that the pipelined DPF units execute at one iteration per cycle (\cref{sec:arch-hw}), so both profiles reuse one engine; this is a reuse argument, not evidence that the DPF form is the fastest option under \ProfT (\cref{sec:proto-pir}). (iii)~\emph{Short-lived sensitive state.} FSS keeps long-running evaluation state pseudorandom (seeds and correction words), and index- or input-dependent state short-lived. We treat (iii) only as defense in depth against physical and microarchitectural threats that \ProfT excludes; no theorem depends on it, and since each module holds $c$ and $r$, FSS gains no formal confidentiality over the direct gate (\cref{sec:threat-model}). The evaluation reports direct-only, FSS-only and compiler-selected default configurations side by side (\cref{sec:eval-ablation}).

\subsection{Distribution-Preserving Refactoring}\label{sec:proto-refactor}

DFA decouples DPF generation from protocol preprocessing by sampling the target directly as a uniform value and recovering the mask $r$ through $g^{-1}$ when the protocol's transformation $g$ is a bijection~\cite{dfa2026trusted}. \sys draws every target from the joint sampler in the same way, with two refinements of the semi-honest argument. Since DPF key privacy holds for arbitrary targets (\cref{sec:bg-fss}), uniformity is required by the application, which publishes $c=x+r$ or $u=x\oplus r$; a refactoring must therefore preserve the \emph{joint} distribution of the preprocessing, not the uniformity of each target.

\textbf{Joint, not marginal, distributions.}
A gate's preprocessing contains correlated objects: the mask, its bits, DPF or DCF targets, wrap bits and auxiliary shares. If a gate needs targets $r$ and $r+1$, resampling each uniformly keeps the marginals but destroys their unit difference; drawing $L$ and $H$ of \cref{alg:interval} independently likewise yields a wrong indicator. The refactoring is valid exactly under the conditions of \cref{lem:bijection}: the map is a bijection for the fixed context \emph{and} all auxiliary material is regenerated from the recovered mask by the unchanged sampler. For example, \cref{alg:interval} may draw $L$ uniformly, set $r=L-a$ and derive $H$ and $\omega$ from that $r$, but may not draw $L$ and $H$ independently.

\textbf{Noninvertible maps and truncation.}
For unsigned truncation, the sampler $R'=2^hA+U$ of \cref{lem:noninv} makes the DFA rule (shift left, fill the low bits uniformly~\cite{dfa2026trusted}) exact; signed shifts, nonuniform masks and other moduli need their own samplers.

\subsection{Verified GPU Matrix Products}\label{sec:proto-freivalds}

Authenticated linear layers need no extra verification: a GPU deviation that changes a value is caught at the next \CheckOpen, before the result enters a protected gate or a release, except with the probability bounded in \cref{thm:mac-sound}. A module that must \emph{consume} a GPU-computed matrix before any opening, however, must not accept it on the host's word, which would reintroduce the forgery oracle of scenario S2. For this case \cref{alg:freivalds} (\cref{app:proof-gates}) is an optional frozen-operand Freivalds check~\cite{freivalds1977probabilistic}, in the spirit of Slalom~\cite{tramer2018slalom} but bound to the ledger.

\textbf{Permitted uses and check.}
The check applies only when exposing the operands to that GPU is already allowed, as in public-by-party-local matrix products; it never permits exposing global secret triple masks, which are generated inside the TCB (\cref{sec:proto-arith}). The module binds the exact operand bytes $A\in\Fp^{m\times k}$ and $B\in\Fp^{k\times n}$ to their authoritative records and freezes the claimed $C$ (\cref{sec:proto-ledger}); only then does it draw $s$ independent secret uniform $\bm{v}\in\Fp^{n}$, test $C\bm{v}\stackrel{?}{=}A(B\bm{v})$ inside the protected verifier, and consume only the verified frozen bytes of $C$ (\cmd{VERIFY_MATRIX} in \cref{tab:commands}). If the GPU also transforms tag arrays, their tag equations are verified too.

\textbf{Soundness and cost.}
\Cref{thm:freivalds} bounds acceptance of a wrong product by $p^{-s}$, and $Q_F$ calls add $Q_F/p^s$ to \cref{thm:main}. The check is disabled in all evaluated configurations; enabling it adds implementation obligations (\cref{tab:obligations}) and this error term.

\subsection{Versioned-Snapshot PIR}\label{sec:proto-pir}

In DPF-based two-server PIR (\cref{eq:pir}), a malicious server can return a wrong share, which the client silently reconstructs into a wrong record, or answer from a stale database. \Cref{alg:pir} and \cref{fig:pir} show the \sys countermeasures.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_pir.pdf}
    \caption{Versioned-snapshot PIR (\cref{alg:pir}). Both modules bind the same query, scan the same snapshot bytes in a public order, hash exactly the bytes they consume, and quarantine the DPF-weighted reduction until the hash matches the authorized commitment $\mathsf{cm}_v$. A host that swaps a record after hashing or serves an old version causes an abort, never a wrong accepted record (scenario S8). Both modules learn $\alpha$, so query privacy relies on module trust.}
    \label{fig:pir}
\end{figure}

\begin{algorithm}[t]
\algstretch
\caption{Versioned-snapshot protected PIR (\algname{PIR-Snap}) inside module $T_b$}
\label{alg:pir}
\begin{algorithmic}[1]
\Require from the client over its confidential channel: index $\alpha$, query identifier $\mathit{qid}$, descriptor $\mathsf{desc}_v=(\mathsf{id},v,N,\mathsf{enc},\mathsf{cm}_v)$; snapshot records $D[0],\dots,D[N-1]$ streamed by host $b$
\Ensure value share $y_b$ of $D[\alpha]$ and certificate $\mathsf{cert}_b$ for the client, or \Abort
\LineComment{Step 1: query binding}
\State exchange $(\alpha,\mathit{qid},\mathsf{desc}_v)$ with $T_{1-b}$ over the protected channel
\If{the bindings differ, $\alpha\ge N$, or $\mathsf{desc}_v$ is unauthorized}
  \State \Abort
\EndIf
\LineComment{Step 2: joint DPF and same-byte scan ($N\ge2$; $N=1$ is a constant-record case with the same checks)}
\State $n\gets\lceil\log_2N\rceil$; bind $N$ and $2^n$; $D[i]\gets0$ for $N\le i<2^n$
\State joint DPF generator for $(\alpha,1)$ under label $(\mathit{qid},\textsf{pir})$ \Comment{GaC}
\State $h\gets\Hash.\mathsf{init}(\mathsf{id},v,N,\mathsf{enc})$;\; $\tilde y_b\gets0$
\For{$i=0$ \textbf{to} $2^n-1$ in public order} \Comment{$\EvalAll$, depth-first}
  \If{$i<N$}
    \State read $D[i]$ into $T_b$; $h\gets\Hash.\mathsf{update}(h,D[i])$
  \EndIf
  \State $\tilde y_b\gets\tilde y_b+\DPF.\Eval(k_b,i)\cdot D[i]$ \Comment{per coordinate}
\EndFor
\LineComment{Step 3: snapshot check; the result is quarantined until here}
\If{$\Hash.\mathsf{final}(h)\neq\mathsf{cm}_v$}
  \State \Abort
\EndIf
\LineComment{Step 4: fresh resharing and certified release}
\State $y_b\gets\tilde y_b+(-1)^b\zeta$ with a fresh joint pad $\zeta$ per coordinate
\State $\mathsf{cert}_b\gets$ certificate on $(\mathsf{sid},\mathsf{ep},\mathit{qid},\mathsf{desc}_v,b,\Hash(y_b))$
\State \Return $(y_b,\mathsf{cert}_b)$ to the client \Comment{no MAC tags}
\end{algorithmic}
\end{algorithm}

\textbf{Protocol and snapshot binding.}
Both role-bound modules receive the same canonical query from the client, compare the binding over their protected channel, pad the snapshot to $2^n$ records while authorizing only $\alpha<N$, and run a joint DPF for $(\alpha,1)$ by generate-and-consume. Each scans the same canonical bytes in the same public order, applies the same DPF weights to every record coordinate, and hashes exactly the bytes it consumes. The commitment $\mathsf{cm}_v$ covers the database identifier, version, shape, record encoding and ordered data bytes, and the result stays quarantined behind the release guard (\cref{sec:proto-ledger}) until the hash matches it; a host that swaps a record after hashing or serves an old version therefore causes an abort (scenario S8 in \cref{tab:scenarios}). A Merkle realization~\cite{merkle1987digital} must authenticate every consumed leaf and its position against the same root. Offloading the reduction to the GPU would need \cref{alg:freivalds} or a separately proven authenticated reduction, never a signature on the GPU's claim, and would export the expanded share vector, so \sys reduces inside the module. Each module releases only a freshly reshared value share (the value half of the epilogue) with a bound certificate, and the client reconstructs $D[\alpha]=y_0+y_1$.

\textbf{Guarantees and regimes.}
In regime (R1) of $\FPIR$ (\cref{fig:func}), with one malicious server host and an honest client, the client obtains the committed record or an abort, and the host learns nothing about $\alpha$ beyond $\Leak_{\mathrm{PIR}}$ (\cref{def:leakage}). In regime (R2), a malicious client alone learns only the requested record and the public descriptor. We make no combined claim (\cref{thm:pir}). Both modules learn $\alpha$, so query privacy relies on module trust: unlike untrusted two-server DPF-PIR such as GPU-DPF~\cite{lam2023gpu} or DFA's untrusted mode~\cite{dfa2026trusted}, which hides $\alpha$ from each server without trusted hardware, \sys offers no query privacy against a compromised module.

\textbf{Scope and design choice.}
Authenticated PIR~\cite{colombo2023apir} provides integrity without trusted hardware at additional server cost and is our malicious-secure GPU baseline (\cref{sec:eval-pir}). Two alternatives bracket our design. Since the modules know $\alpha$ anyway, a module could select $D[\alpha]$ with a constant-time comparator during the same public-order scan; this needs no AES expansion and would be bound by snapshot bandwidth rather than by the AES array. If $\alpha$ must stay hidden from the modules, the client can generate the DPF keys as in untrusted-mode DFA, and each module evaluates its own key inside the boundary with the same hashing, quarantine, resharing and certificates; this adds a DPF key-privacy term and, against a malicious client, a key-verification step~\cite{boyle2016function,boneh2021lightweight,decastro2022vfss}. We keep joint generation for uniformity with the inference datapath (\cref{sec:proto-direct}) and as defense in depth. We model neither alternative, so \cref{tab:pir} does not show that our design is the best \ProfT PIR. Assuming a PIR efficiency of \est{0.93} relative to DFA (\cref{app:model}), our model gives \est{16{,}349} versus 17{,}580~queries/s at $N=2^{20}$~\cite{dfa2026trusted} (\cref{tab:pir}).


==> qa/draft4/sections/06_architecture.tex <==
% ======================================================================
% Section VI: Architecture and System Integration
% Labels defined here: sec:arch, sec:arch-insight, sec:arch-hw, sec:arch-pipe,
%   sec:arch-iface, sec:arch-field, sec:arch-deploy, sec:arch-dse,
%   fig:hw, fig:pipeline, tab:commands, lst:mersenne
% ======================================================================
\section{Architecture and System Integration}\label{sec:arch}

This section describes how \sys realizes the protected module $T_b$ of \cref{sec:protocol} next to the GPU and how the untrusted host drives it. We keep the organization of DFA~\cite{dfa2026trusted} wherever the malicious setting permits and add only the blocks that the integrity chain requires. Hardware sizes are design parameters; red values are estimates (\cref{sec:eval-hw,app:model}). That this hardware realizes the ideal resource $\mathcal{F}_{\mathsf{T}}$ of the proofs is an implementation obligation (\cref{tab:obligations}).

% ======================================================================
\subsection{Design Insights}\label{sec:arch-insight}

\textbf{Key insight.}
Malicious security moves the dominant cost from DPF to authenticated linear algebra on the GPU, while protected FSS evaluation, exposed triple generation and \CheckOpen{} stay small (\cref{sec:analysis-cost,fig:motiv}). The module therefore need not become a second GPU: it must hold exactly the state whose exposure or modification would break the integrity chain and inspect every byte that crosses its boundary. The GPU is a fast but untrusted engine for authenticated linear algebra, and the module is dealer, verifier and release authority at once.

\textbf{What must be protected.}
A block belongs inside the trusted boundary if it holds material that reveals both parties' views or authorizes a release. These are exactly the TCB items of \cref{sec:threat-model} (keys, sampler and counters, generator state and correction words, table and reduction logic, challenges and residuals, release decisions); everything else stays outside (\cref{fig:threat}).

\textbf{What stays on the GPU.}
Linear layers run as the matrix Beaver products of $\Pi_{\mathsf{Mult}}$ over the value lane and the $t=3$ tag lanes (\cref{fig:arith}), i.e., two dense products per lane, $2(1+t)$ in total, of the same public shape. A GPU result is a candidate share, never a certified value.

\textbf{Placement.}
An authenticated element costs 32~B per party at the module interface (\cref{sec:proto-repr}), so a link of bandwidth $B$ streams at most $B/32$ elements per second (\cref{sec:analysis-work}). The L2-adjacent placement of DFA delivers about 290~GB/s to the SMs~\cite{dfa2026trusted}, so we keep it: one DPF unit per L2 slice, a new protected core beside a designated L2 partition, and SM access through the DFA-mapped address range without a new network-on-chip (NoC) port.

% ======================================================================
\subsection{Hardware Design}\label{sec:arch-hw}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_hw.pdf}
    \caption{\sys hardware. Top: placement inside the GPU; as in DFA, one DPF unit sits next to each L2 slice and a designated slice hosts the VIGOR core. Bottom: logical organization of the protected module $T_b$ (red dashed trusted boundary). The 64 AES-128 engines are time-shared among PRG expansion, challenge derivation and AEAD sealing; the Mersenne-61 field unit array (eight lanes in each DPF unit) serves epilogues, triples, reductions and check residuals. SMs, L2, NoC, HBM and host DRAM stay outside the boundary.}
    \label{fig:hw}
\end{figure}

\Cref{fig:hw} shows the module (area and power in \cref{sec:eval-hw}). The trusted boundary encloses the 16 DPF units of DFA (\cref{sec:bg-dfa}), the vector processing unit (VPU), the new \emph{VIGOR core} and the on-die links between them. Only command frames with share batches, PIR database records, authenticated output tuples, sealed spill pages and sealed channel frames cross it, none carrying a module secret in the clear. The blocks follow the integrity chain: parser and ledger admit \emph{authorized input}; sampler and field unit array produce \emph{correlated preprocessing}; the DPF units perform \emph{correct local evaluation}; the epilogue yields \emph{authenticated arithmetic}; freezer, check engine and peer channel enforce \emph{consistent opening}; and the release guard gates \emph{authorized output release}.

\textbf{DPF units and sampler.}
The AES datapath is unchanged. Each pipeline context carries two generator states, a separate evaluator state, a depth-first search (DFS) stack and the conversion $\Conv$ into $\Fp$, exactly the state of \cref{alg:gac}; correction words are consumed and discarded inside the unit, and raw leaf shares $\tilde y_b$ go to the field unit array lanes of the same unit, never to SM-readable buffers. The joint PRF sampler implements the labeled derivation and bounded rejection sampling of \cref{sec:proto-setup} under the session key.

\textbf{Field unit array (FUA).}
The FUA consists of 128 Mersenne-61 multiply-accumulate lanes, each with a $61\times 61$-bit multiplier and the two-fold reduction of \cref{lst:mersenne}; its peak is 116~G multiply-accumulates per second at the 910~MHz 7~nm clock of DFA~\cite{dfa2026trusted}. It computes epilogues (three products per output), the triple products $c=ab$ and $C=AB$ with their \AuthShare{} tags (so matrix masks never reach the GPU), LUT and PIR reductions, interval sums and check residuals. The lanes sit in the DPF units, eight per unit (a design parameter), and the VIGOR core schedules them as one pool. Full-domain LUT and PIR reductions therefore run next to the leaves, and only per-query accumulators (three field elements per PIR query) travel to the core (\cref{sec:arch-dse}).

\textbf{Check engine and freezer.}
The check engine executes steps~3 and~4 of \cref{alg:checkopen}: it derives the $t$ challenge vectors only after both frozen roots are fixed, accumulates the residuals on FUA lanes (two products per lane and element) and evaluates all lanes over the full batch before emitting one generic status, so neither the status nor its latency reveals which lane or position failed. \cmd{FREEZE_BATCH} copies the exact submitted bytes into a 256~KB freeze SRAM (8{,}192 tuples of 32~B) and hashes them with their descriptor into the root $h_b$ that the modules exchange; larger batches spill to AES-GCM-sealed immutable HBM pages~\cite{dworkin2007gcm,mcgrew2004gcm} whose authoritative root and page counters stay inside, so after the challenge only authenticated frozen bytes are reread (\cref{sec:proto-ledger}).

\textbf{Ledger, release guard and control.}
A 32~KB ledger SRAM holds the authoritative state of every in-flight gate and the randomness identifiers burnt at reservation (\cref{fig:ledger}). The release guard opens for a gate only in state \lstate{VERIFIED}, and an epoch abort closes every outstanding response atomically (\cref{sec:proto-ledger}); the release multiplexer and output FIFO of \cref{fig:hw} belong to the release-guard logic. The peer-channel controller keeps independent directional keys, never repeats a nonce and enforces a per-session traffic and forgery budget. The SC300-class control core of DFA~\cite{st33tpm12spi,arm_cortex_m3} runs measured boot, attestation and the key establishment covered by $\eps{setup}$, and the 16-lane VPU of DFA~\cite{cavalcante2019ara} handles the remaining protocol logic, including the range check $x^*\in\mathsf{In}_\nu$ of $\Pi_{\mathsf{Input}}$ and the validity predicates of $\mu$ at the public boundaries that $\mu$ declares. Host software cannot drive the module's clock or voltage outside its safe operating range (DVFS isolation, \cref{app:func-module}).

\textbf{AES time-sharing.}
The 64 engines are the module's only AES resource. A slot arbiter per unit serves PRG expansion (two blocks per expansion, $6n+3$ per GaC output), challenge derivation (1.5 blocks per checked element: three 64-bit words for three 61-bit challenges) and AEAD keystream for sealing and the peer channel (two blocks per 32-byte tuple); one AEAD/GHASH block serves both the freezer and the peer-channel controller. Check and sealing requests take priority because they are short and on the critical path of the next round; PRG contexts fill all other slots. A per-slot purpose tag selects the key context, so the uses never share a key.

% ======================================================================
\subsection{Pipeline Scheduling and Memory}\label{sec:arch-pipe}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/fig_pipeline.pdf}
    \caption{Scheduling inside a DPF unit. (1)~Generator (g) and evaluator (e) expansions of at least $L$ independent contexts interleave to hide the $L$-cycle AES and correction feedback latency. (2)~AES slots are time-shared among PRG expansion, challenge derivation and AEAD sealing. (3)~Depth-first $\EvalAll$ keeps one pending sibling per level, i.e., $O(n)$ state per context.}
    \label{fig:pipeline}
\end{figure}

\textbf{Context interleaving.}
With an AES and correction feedback latency of $L$ cycles, one dependent path advances at most one level every $L$ cycles, so one issue per cycle needs at least $L$ independent contexts per unit (\cref{fig:pipeline}, panel~1). For the 20-stage DFA pipeline~\cite{dfa2026trusted} we therefore provision 20 contexts per unit, one per stage. The three expansions of a malicious GaC level issue back to back, because $\PRG(\tilde s)$ does not depend on $\CW^{(i)}$; only the correction waits for all three. A context (three 129-bit path states, the correction word in flight, target, query, payload and level) needs fewer than 100~B, so 20 contexts take less than 2~KB per unit, and a single gate with $n=61$ completes in \est{1.71~$\mu$s}.

\textbf{Separate old controls.}
Each unit keeps separate registers for the \emph{old} generator bits $t_0,t_1$ and the \emph{old} evaluator bit $\tilde t$ (\cref{sec:analysis-dpf}), captures all outputs of a transition before overwriting its inputs, and never substitutes generator states for evaluator roots; this is the schedule covered by \cref{thm:gac}. Planned RTL tests exercise signed final conversion, zero payloads, all-zero and all-one indices, $x=\alpha$ and divergence at every depth.

\textbf{Depth-first EvalAll.}
LUT and PIR gates evaluate the full domain. Depth-first traversal keeps one pending sibling per level ($O(n)$ states per traversal) and a complete tree needs $2^n-1$ internal expansions (panel~3). The 512 queries of a PIR batch walk the same public leaf order in lockstep, so each snapshot record is read and hashed once per batch and folded into 512 per-query accumulators. For $N=2^{20}$, 512 contexts with 20 pending siblings of 17~B occupy about 174~KB, or 11~KB per unit, which fits the traversal buffers of DFA~\cite{dfa2026trusted}.

\textbf{Pads and frozen buffers.}
The four pads of an output occupy two AES blocks and are drawn in step with the leaf, so no pad buffer beyond the pipeline depth is needed. A checked batch occupies the freeze SRAM until its verdict two peer round trips later, so batches beyond 8{,}192 elements, such as the 65{,}536-element batches of \cref{fig:checkperf}, spill to sealed pages.

% ======================================================================
\subsection{Command Interface and Host Integration}\label{sec:arch-iface}

\begin{table}[t]
\centering
\caption{Commands of the protected module $T_b$. Every command is a canonical frame bound to session, epoch, role and gate; the ledger state reached on success is given in parentheses. No command authenticates a host-supplied value.}
\label{tab:commands}
\footnotesize
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\linewidth}{l >{\raggedright\arraybackslash}X >{\raggedright\arraybackslash}X}
\hline
\textbf{Command} & \textbf{Required check} & \textbf{Allowed result} \\
\hline
\cmd{OPEN_SESSION}  & Authenticated identities, role, fresh epoch, manifest $\mu$ & Session capability \\
\cmd{RESERVE_PREP}  & Approved gate, unused randomness identifiers & Party-local authorized preprocessing, issued once (\lstate{PREPARED}) \\
\cmd{FREEZE_BATCH}  & Exact canonical bytes, dimensions, expected wire list & Frozen root $h_b$ and handle (\lstate{FROZEN}) \\
\cmd{CHECK_OPEN}    & Both frozen roots, independent challenge lanes, peer residuals & Verified prescribed opening or abort (\lstate{VERIFIED}) \\
\cmd{EVAL_FSS}      & Bound table or function, \lstate{VERIFIED} and unconsumed input opening, fixed role & Freshly reshared authenticated local output (\lstate{CONSUMED}) \\
\cmd{VERIFY_MATRIX} & Anchored operands, frozen candidate & Verified immutable result handle (\lstate{VERIFIED}) \\
\cmd{FINAL_OUTPUT}  & Authorized recipient, output mask, accepted check & Bound frame with $\upsilon=y+o$ and certificate (\lstate{CONSUMED}, then \lstate{RELEASED}) \\
\cmd{ABORT}         & Any integrity or lifecycle violation & Epoch invalidation, no candidate values (\lstate{ABORTED}) \\
\hline
\end{tabularx}
\end{table}

\textbf{Host responsibilities.}
Host $b$ schedules the public circuit, stores only party-local authenticated arrays (value and each MAC lane as separate coalesced arrays, serialized canonically only at the protected interface), runs the exact field kernels of \cref{sec:arch-field} and sends share batches to $T_b$. Its scheduling may be adversarial, so the ledger, not the host, decides whether operation, identity, shape and order are admissible, and a reused buffer always carries a fresh transaction identifier.

\textbf{Commands and frames.}
\Cref{tab:commands} lists the eight commands with the ledger state each reaches (\cref{fig:ledger}); since none of them authenticates a host value, the forgery-oracle path of scenario~S2 is closed (\cref{tab:scenarios}). A frame carries version, session identifier, epoch, role, opcode, gate identifier, ordered input and output identifiers, field identifier, tag count, dimensions, payload length, sequence number and payload, all length-prefixed with explicit endianness; frames between modules or from a client bind the header as AEAD associated data. The parser copies each frame into protected memory before checking it and rejects truncation, trailing bytes, duplicate identifiers, malformed dimensions, noncanonical field elements (values of at least $p$ are rejected, never reduced) and unexpected opcodes.

\textbf{Data races and aborts.}
Verification and consumption use the same immutable parsed bytes. Independent gate batches may overlap, but a dependent nonlinear gate never consumes an unchecked masked opening. Any integrity or lifecycle violation, such as an invalid transition or a failed check, triggers \cmd{ABORT}, which poisons the epoch, prevents new challenges and atomically keeps the release guard closed for every outstanding response (\cref{sec:proto-ledger}). \Cref{tab:attacks} maps each injected fault to the block that stops it.

% ======================================================================
\subsection{Exact Field Arithmetic on the GPU}\label{sec:arch-field}

GPU kernels must compute the finite circuit that the proofs reason about, so floating-point shortcuts are excluded. An authenticated GEMM applies the matrix Beaver combination of $\Pi_{\mathsf{Mult}}$ on each of the four lanes, i.e., two products per lane ($D\,B_b$ and $A_b\,E$ on the value lane, likewise on each tag lane), $2(1+t)=8$ products of the same shape, plus the public product $DE$ shared by all lanes (\cref{fig:arith}); \cref{lst:mersenne} gives the scalar multiplication at the core of every kernel.

\begin{figure}[t]
\centering
\scriptsize
\begin{tabular}{|l|}
\hline
\begin{minipage}{0.95\linewidth}
\vspace{2pt}
\begin{verbatim}
constexpr uint64_t P = (1ULL << 61) - 1;  // 2^61 - 1
// canonical a, b < P; returns canonical a*b mod P
__device__ uint64_t mul61(uint64_t a, uint64_t b) {
  uint64_t lo = a * b;              // low 64 bits
  uint64_t hi = __umul64hi(a, b);   // high bits, < 2^58
  uint64_t x  = (lo & P) + ((lo >> 61) | (hi << 3));
  x = (x & P) + (x >> 61);          // x <= 2^61
  return x >= P ? x - P : x;
}
\end{verbatim}
\vspace{-4pt}
\end{minipage}\\
\hline
\end{tabular}
\caption{Exact Mersenne-61 multiplication used by the GPU field kernels (CUDA). The first fold uses $2^{61}\equiv 1 \pmod p$; the second fold and the conditional subtraction return the canonical representative. No floating-point or Tensor-Core operation is involved.}
\label{lst:mersenne}
\end{figure}

\textbf{Correctness.}
For canonical $a,b<p=2^{61}-1$ the product is below $2^{122}$, so $\mathtt{hi}<2^{58}$ and $\mathtt{hi}\ll 3$ fits in 61 bits. Writing $ab=2^{64}\,\mathtt{hi}+\mathtt{lo}$ and using $2^{61}\equiv 1\pmod p$ gives $ab\equiv(\mathtt{lo}\bmod 2^{61})+\lfloor\mathtt{lo}/2^{61}\rfloor+2^{3}\,\mathtt{hi}\pmod p$. The last two terms occupy disjoint bit ranges (bits 0 to 2 and 3 to 60), so the bitwise OR equals their sum and the folded value is below $2^{62}$. The second fold yields at most $2^{61}=p+1$, and the conditional subtraction returns the canonical representative. The executed CPU check of this formula and the pending GPU conformance test are reported in \cref{sec:eval-attack}.

\textbf{Accumulation and numeric contract.}
A two-word 128-bit accumulator absorbs at most 64 unreduced products below $2^{122}$, so kernels fold at least once per 64 inner-dimension terms; random shares lie close to $p$ even for small plaintexts, so plaintext bounds never justify longer accumulation. The manifest $\mu$ fixes the scale $2^f$, signed encoding, toward-zero truncation (\cref{alg:trunc}), saturation, approximation coefficients and output decoding. For example, a dot product of length at most 4{,}096 with operand magnitudes at most $2^{20}$ stays within $|\cdot|\le 2^{52}$ before bias, which leaves room below $p/2$ only if bias and further accumulation are bounded too; the bound is recomputed per layer. FP16, BF16 and TF32 Tensor Cores never serve as exact field operations without a proven limb construction, and the exact finite circuit and a floating-point accuracy model remain separate references.

\textbf{GEMM cost assumption.}
Our model charges an exact Mersenne GEMM \est{1.25$\times$} the time of a wraparound 64-bit GEMM per lane ($\phi_{\mathrm{M}}$ in \cref{app:model}). This factor is an assumption, not a measurement: the kernel above additionally needs the high product word and a two-word accumulator per term, and the GPU test that would calibrate it has not run. Each $+0.25$ in $\phi_{\mathrm{M}}$ adds \est{0.52~s} to BERT-Base; with $\phi_{\mathrm{M}}=2$ its LAN latency would be \est{5.39~s}, i.e., \est{3.8$\times$} instead of \est{2.7$\times$} that of semi-honest trusted DFA.

% ======================================================================
\subsection{Deployment Targets}\label{sec:arch-deploy}

An on-die module cannot be added to a commercial A100, so we define three distinct experiments and never merge their timings. All three are planned (\cref{sec:eval-method}). \emph{(i) A100 software} runs the exact kernels, authenticated GEMM and host runtime on a real A100 with an emulated module. \emph{(ii) A ZCU102 prototype} (\texttt{xczu9eg-ffvb1156-2-e}~\cite{amd2023zcu102}) implements the datapath of \cref{fig:hw} at reduced scale (\est{4} DPF units, \est{16} AES engines, \est{32} FUA lanes at \est{250~MHz}, \cref{tab:fpga}) to validate streaming, freezing and release ordering; one board with an emulated peer shows functionality, not two independent trust boundaries, and an ARM process on it is not isolated from a malicious board administrator. \emph{(iii) The on-die projection} models integration next to the L2 slices with Accel-Sim~\cite{khairy2020accel} and synthesis, as in DFA; our headline numbers refer to it and currently come from the analytical model of \cref{app:model}. An external module uses staged transfer through host memory as its baseline, because GPUDirect RDMA needs platform and driver support and ordinarily a common PCIe root complex~\cite{nvidia2024gpudirect}; IOMMU protection is never disabled for a benchmark. In every target, freeze-before-challenge refers to immutable authenticated bytes, never to a GPU buffer that can change concurrently.

% ======================================================================
\subsection{Design-Space Comparison}\label{sec:arch-dse}

We compare the L2-adjacent organization of \sys with alternative homes for authentication, verification and randomness generation.

\textit{External protected module over PCIe.}
A discrete FPGA or security card~\cite{xu2025co} keeps the boundary off the GPU die but limits the interface to $B/32$ elements per second: \est{50~M} for the \est{1.6~GB/s} ZCU102 transport and \est{0.78~G} for \est{25~GB/s} of effective PCIe Gen4 bandwidth, against 9.1~G on the 290~GB/s on-die path of DFA~\cite{dfa2026trusted}. Because authenticated GEMM dominates, BERT-Base LAN latency rises only to \est{3.87~s} over PCIe and \est{4.59~s} with the ZCU102 link and lanes (\cref{tab:ablation}); the option suits prototyping but adds a second device per party and two device round trips per checked layer (\cref{app:model}).

\textit{Verification on the GPU SMs.}
In \ProfT the SMs belong to the malicious host: a corrupt checking kernel could see the challenges before choosing its errors, or simply report acceptance. Trusting them requires a GPU-wide TEE~\cite{volos2018graviton,jang2019heterogeneous,dhanuskodi2023confidential} covering SMs, caches, memory controllers and the driver interface, the large boundary that DFA and \sys avoid. The GPU therefore computes only products that the module verifies afterwards (\CheckOpen{} or the Freivalds check of \cref{sec:proto-freivalds}).

\textit{Tag DPF trees instead of the epilogue.}
One extra DPF tree per MAC lane (payload $\Delta_j\beta$) multiplies the PRG work of every gate by $1+t$ (\cref{tab:gatecost,fig:dpfthr}); the epilogue achieves the same with three multiplications and four pads (\cref{thm:epilogue}) at \est{3.8--4.0$\times$} the per-gate throughput of tag trees.

\textit{Software-only malicious backend.}
SPDZ-family preprocessing~\cite{keller2016mascot,keller2018overdrive,cramer2018spdz2k,keller2020mpspdz} needs inter-party communication that grows with the number of authenticated triples, and dealer-based malicious FSS, modeled after the protocol family of Shark~\cite{gupta2025shark}, ships authenticated keys and triples from an external dealer (\cref{tab:e2e}); both re-create the offline traffic that trusted DFA removed. Such a backend fits \ProfU, where the hardware itself is distrusted (\cref{sec:threat-profileu}); under \ProfT it pays for a trust assumption that the module already provides.

\textit{Dedicated check engines, a central FUA and per-slice checking.}
Checking needs only \est{2.8~ms} of module time per BERT-Base query against \est{131~ms} of protected FSS work, so dedicated AES engines for challenges and sealing would idle almost always. DPF units stay distributed because a single attachment point, a memory-channel path of about 180~GB/s, would cap DPF output at about 62\% of the 290~GB/s delivered bandwidth~\cite{dfa2026trusted}. The same limit rules out a central FUA: the raw 8-byte leaf shares of PIR at 16K entries alone would need \est{137~GB/s} (\est{76\%} of that path), so reductions stay in the units. Checks, by contrast, cost at most 3.5 AES blocks and six field multiplications per element and depend on the ledger, freeze SRAM and peer channel, which must be single points of authority; the VIGOR core therefore controls every check and holds one authoritative root per batch.


==> qa/draft4/sections/07_security.tex <==
% =====================================================================
% Section VII: Security Analysis
% File owner: sections/07_security.tex
% Labels defined here: sec:security, sec:sec-assump, sec:sec-main,
%   sec:sec-lemmas, sec:sec-scenarios, sec:sec-concrete, sec:sec-boundary,
%   thm:main, thm:dpf-correct, thm:gac, thm:dcf, thm:epilogue,
%   lem:hidden-key, thm:mac-sound, thm:arith, thm:bitdec, thm:cmp-trunc,
%   thm:lut, thm:interval, lem:bijection, lem:noninv, thm:freivalds,
%   thm:pir, tab:obligations, tab:lanes
% =====================================================================
\section{Security Analysis}
\label{sec:security}

We now show that \sys realizes the functionalities $\FC$ and $\FPIR$ of \cref{fig:func} with leakage $\Leak_C$ and $\Leak_{\mathrm{PIR}}$ (\cref{def:leakage}) against a malicious host and GPU, as stand-alone security with abort (\cref{def:security}) in the explicit-simulator style~\cite{canetti2000security,goldreich2004foundations,hazay2010efficient,lindell2017simulate}. Each link of the integrity chain, \emph{authorized input $\rightarrow$ correlated preprocessing $\rightarrow$ correct local evaluation $\rightarrow$ authenticated arithmetic $\rightarrow$ consistent opening $\rightarrow$ authorized output release}, is discharged by a named statement: input extraction (\cref{thm:arith}); in-module preprocessing and joint sampling (\cref{lem:bijection,lem:noninv}); exact DPF, DCF, FSS-gate and direct-gate correctness (\cref{thm:dpf-correct,thm:gac,thm:dcf,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval,thm:arith}); the epilogue and the arithmetic identities (\cref{thm:epilogue,thm:arith}); MAC-check soundness (\cref{lem:hidden-key,thm:mac-sound}); and gated release (\cref{thm:arith,thm:pir}). Full proofs are in \cref{app:proof-dpf,app:proof-auth,app:proof-gates,app:proof-main}.

% =====================================================================
\subsection{Assumptions and Error Terms}
\label{sec:sec-assump}

The theorem is proved in \ProfT (\cref{sec:threat}); we state module trust as an explicit ideal resource~\cite{katz2007universally}.

\begin{assumption}[Ideal protected module]
Corrupting host $b$ does not corrupt $T_b$; both modules are instances of the ideal resource $\mathcal{F}_{\mathsf{T}}$ (\cref{app:func-module}). The code, keys, parser, field arithmetic, ledger transitions, local memory, protected peer channel and approved I/O paths of each module are correct and confidential. Its externally observable trace (lengths, timing, host-visible memory and DMA activity, power, thermal and clock telemetry) is simulatable by a stipulated trace simulator from the command sequence issued by the host, $\mu$, the public lengths and the accept or abort outcomes, and is independent of the global MAC keys, challenges and residuals given these (all lanes are aggregated in data-independent time before one generic $\mathsf{status}$ is returned). Host software cannot drive the module's clock or voltage outside its safe operating range, or the module detects glitches and aborts (DVFS isolation); software-reachable undervolting~\cite{murdock2020plundervolt} is thus in scope (\cref{sec:threat}). Module state is fresh: a trusted monotonic service preserves freshness across reboots~\cite{parno2011memoir,matetic2017rote}, or the module irrecoverably erases its master key and requires a freshly attested session. Availability is not assumed.
\end{assumption}

\begin{assumption}[Setup, randomness, channels and bindings]
Each term bounds an idealization over the \emph{entire} admitted execution, not a single primitive call:
$\eps{setup}$, simulation of the authenticated setup of \cref{sec:proto-setup} by an ideal role-bound interface;
$\eps{prf}$, replacement of PRF/KDF outputs (AES-128, HKDF~\cite{krawczyk2010hkdf}) under distinct length-prefixed labels by independent coins, identical for the same joint label;
$\eps{channel}$, confidentiality and integrity of the AEAD channels~\cite{dworkin2007gcm,mcgrew2004gcm} with directional keys and nonrepeating nonces;
$\eps{bind}$, collisions or forgeries in manifests, snapshot commitments, frozen-page roots, certificates and session freshness~\cite{fips202,merkle1987digital};
$\eps{trace}$, the stipulated trace simulator.
\end{assumption}

Correctness of protected code, state and arithmetic is thus a \emph{premise}, not an estimated probability. The protocol contributes one statistical term, determined by the field $\Fp$ with $p=2^{61}-1$, the number $t$ of independent global keys $\Delta_j=\Delta_{0,j}+\Delta_{1,j}$ (host $b$ knows at most $\Delta_{b,j}$), and the number $Q$ of \CheckOpen{} batches. Exclusions and client assumptions are those of \cref{sec:threat}; the modules may see inputs (\cref{sec:discussion}).

% =====================================================================
\subsection{Main Theorem}
\label{sec:sec-main}

\begin{theorem}[Stand-alone static malicious security with abort]
\label{thm:main}
Under the assumptions of \cref{sec:sec-assump}, the protocols of \cref{sec:analysis-dpf,sec:protocol} (setup, ledger, exact DPF, generate-and-consume with the fresh authentication epilogue, conservative DCF, \AuthShare, \CheckOpen, $\Pi_{\mathsf{Input}}$ with the committed-input loader, $\Pi_{\mathsf{Lin}}$, $\Pi_{\mathsf{Mult}}$, $\Pi_{\mathsf{Out}}$, bit decomposition, comparison, truncation, LUT, interval and direct protected gates) realize $\FC$ with abort and leakage $\Leak_C$, and \cref{alg:pir} realizes $\FPIR$ with abort and leakage $\Leak_{\mathrm{PIR}}$ (\cref{def:security,def:leakage}), against a PPT adversary that statically corrupts at most one host or, for $\FPIR$ in regime (R2) of \cref{fig:func}, the client alone. With at most $Q$ \CheckOpen{} batches, the advantage of every PPT distinguisher in \cref{def:security} is at most
\begin{align*}
\eps{VIGOR}\le{}&\eps{setup}+\eps{prf}+\eps{channel}\\
&+\eps{bind}+\eps{trace}+Q\,(2/p)^{t}.
\end{align*}
If the Freivalds check (\cref{alg:freivalds}) is enabled for at most $Q_F$ calls with $s$ repetitions, the bound gains $Q_F/p^{s}$, and the binding obligations of \cref{thm:freivalds} apply.
\end{theorem}

\Cref{thm:main} is a stand-alone real/ideal statement about one admitted execution, preserved under sequential composition; we claim neither universal nor concurrent composability, and concurrent sessions that share module state are not covered (\cref{app:func}).

\textbf{What the bound omits.}
There is no DPF one-key-privacy term: keys never leave the modules, \cref{thm:dpf-correct} gives raw correctness and \cref{thm:epilogue} makes every exported tuple uniform. A key-exporting profile (\ProfU, \cref{sec:threat-profileu}, or verifiable FSS~\cite{decastro2022vfss}) must add its actual DPF or backend privacy assumption. The theorem does not prove that a concrete chip implements the ideal module (\cref{sec:sec-boundary}).

\textbf{Proof overview.}
The simulator $\Sim$ plays $\mathcal{F}_{\mathsf{T}}$ for both modules, keeps the global MAC keys internally, and tracks the ledger and, for every wire, the tuple a faithful corrupt party would hold; honest shares stay symbolic, so honest values are never needed. Five hybrids connect the real and ideal executions (\cref{app:proof-main}). In the real execution $\Hyb{0}$ the modules run the concrete module program: $\mathcal{F}_{\mathsf{T}}$ with its randomness $R$ instantiated by $\PRF_K$, peer and client channels by AEAD over the hosts' network, and \cmd{OPEN_SESSION} by attestation plus authenticated key exchange.
\begin{itemize}[leftmargin=*]
\item \textbf{$\Hyb{1}$ (ideal setup and channels).} Setup becomes the ideal role-bound interface, and protected-channel contents become ideal deliveries of the permitted lengths and schedules. Cost: $\eps{setup}+\eps{channel}$.
\item \textbf{$\Hyb{2}$ (ideal randomness and bindings).} PRF/KDF outputs become ideal coins, and any binding failure aborts; the ledger (\cref{fig:ledger}) then excludes label reuse, role swapping and post-challenge byte replacement. Streaming generate-and-consume is replaced by \cref{alg:gen} followed by \cref{alg:eval} (\cref{thm:gac}), and refactored samplers by their reference forms (\cref{lem:bijection,lem:noninv}); both replacements are exact. Cost: $\eps{prf}+\eps{bind}$.
\item \textbf{$\Hyb{3}$ (abort on an accepted wrong-value opening).} The experiment aborts at the first \CheckOpen{} batch accepted with $\bm{e}\ne\bm{0}$ (and, if \cref{alg:freivalds} is enabled, at the first accepted $C\ne AB$). It equals $\Hyb{2}$ until then; by \cref{lem:hidden-key,thm:mac-sound} the cost is $Q(2/p)^t$ (plus $Q_F/p^s$, \cref{thm:freivalds}).
\item \textbf{$\Hyb{4}$ (ideal execution).} Honest parties use $\FC$. $\Sim$ extracts corrupt inputs ($x^*=r+\varepsilon$ or the committed loader value) and aborts where the modules do (e.g., unless $x^*\in\mathsf{In}_\nu$), samples preprocessing tuples, epilogue and direct-gate outputs and every masked opening uniformly (the hidden preprocessing is defined afterwards), decides each check from $\inner{\bm{\rho}_j}{\bm{d}_j-\Delta_j\bm{e}}$ with its own keys and fresh challenges, delivers a corrupt recipient's output mask $o$ early and programs its opening $\upsilon=y+o$ after $\FC$ releases $y$, and appends the stipulated trace simulator. Since $\Hyb{3}$ accepts no wrong value, the trace-free views are identical (\cref{thm:arith,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval}); cost: $\eps{trace}$. PIR uses the simulator of \cref{thm:pir}.
\end{itemize}
The triangle inequality gives the bound. The adversary may still suppress delivery to honest parties: no fairness is added.

% =====================================================================
\subsection{Building Blocks}
\label{sec:sec-lemmas}

The statements refer to the exact algorithms of \cref{sec:analysis-dpf,sec:protocol}, which, unlike the semi-honest ones (\cref{sec:bg-dfa}), make root control bits, role inputs and separate generator and evaluator states explicit; each is followed by its proof idea.

\begin{theorem}[DPF correctness]
\label{thm:dpf-correct}
For all root seeds $s_0,s_1\in\bits{128}$ with root control bits $t_0=0$, $t_1=1$, every $n$, $\alpha,x\in\bits{n}$ and $\beta\in\Fp$, the keys of \cref{alg:gen} and the outputs $y_b$ of \cref{alg:eval} satisfy $y_0+y_1=\beta\cdot\one[x=\alpha]$. No uniform target and no hardness assumption is needed.
\end{theorem}

\noindent\textit{Proof idea.}
On the target prefix the control bits stay opposite; on a losing child $(s_0^{\lose}\oplus s_1^{\lose})\oplus((t_0\oplus t_1)\sCW)=0$ and the control bits cancel, so the states coincide and their signed outputs cancel. At the leaf $t_0-t_1=(-1)^{t_1}$, so $y_0+y_1=u_0-u_1+(-1)^{t_1}\CWout=\beta$ (\cref{app:proof-dpf}).

\begin{theorem}[Generate-and-consume equivalence]
\label{thm:gac}
For fixed roots, $\alpha$, $\beta$, role $b$ and query $x$, the raw share $\tilde{y}_b$ of \cref{alg:gac} equals the output of \cref{alg:eval} on the key $k_b$ that \cref{alg:gen} produces from the same inputs, node by node for every dependency-respecting depth-first order of $\EvalAll$.
\end{theorem}

\noindent\textit{Proof idea.}
Couple both executions: equal states before level $i$ give the same correction word, generator state and evaluator state after it. The theorem justifies scheduling only, not changes to expansion or correction (\cref{app:proof-dpf}).

\begin{theorem}[Conservative DCF]
\label{thm:dcf}
If \cref{alg:dcf} creates, for each $i=1,\dots,n$ (zero payloads included), an independent DPF with target $\alpha_1\cdots\alpha_{i-1}0$ and payload $\beta\alpha_i$, evaluated at $x_1\cdots x_i$, the shares sum to $\beta\cdot\one[x<\alpha]$, at a cost of $n(n+1)/2$ path levels.
\end{theorem}

\noindent\textit{Proof idea.}
If $x<\alpha$, exactly the prefix ending at their first differing bit ($x_i=0$, $\alpha_i=1$) contributes $\beta$; otherwise none does. \Cref{thm:dpf-correct} and linearity conclude (\cref{app:proof-dpf}).

\begin{theorem}[Epilogue correctness and local hiding]
\label{thm:epilogue}
For raw shares $\tilde{y}_0,\tilde{y}_1$ and fresh uniform pads $\zeta,\kappa_1,\dots,\kappa_t\in\Fp$, the outputs $y_b=\tilde{y}_b+(-1)^b\zeta$, $\gamma_{b,j}=\Delta_j y_b+(-1)^b\kappa_j$ form an authenticated sharing of $\tilde{y}_0+\tilde{y}_1$. For either fixed $b$, $(y_b,\gamma_{b,1},\dots,\gamma_{b,t})$ is uniform on $\Fp^{t+1}$ given the raw outputs and the keys, before conditioning on later prescribed openings, jointly across fresh outputs.
\end{theorem}

\noindent\textit{Proof idea.}
The pads cancel in the sums. For fixed $b$, $\zeta\mapsto y_b$ and each $\kappa_j\mapsto\gamma_{b,j}$ are bijections, so every tuple has probability $p^{-(t+1)}$ (\cref{app:proof-dpf}).

\begin{lemma}[Hidden-key invariant]
\label{lem:hidden-key}
In $\Hyb{2}$ with host $b$ corrupted, conditioned on its view and its shares $\Delta_{b,j}$, the honest shares $\Delta_{1-b,1},\dots,\Delta_{1-b,t}$ remain independent and uniform at every point up to the drawing of the challenges of the first check with a nonzero value error; that check either accepts (the event of \cref{thm:mac-sound}) or rejects and ends the execution.
\end{lemma}

\noindent\textit{Proof idea.}
Fresh tags are padded (\AuthShare, \cref{thm:epilogue}); linear updates are deterministic in the view; correct openings have zero residual; a tag-only error yields an outcome independent of $\Delta_j$; residuals and challenges stay inside the modules (\cref{app:proof-auth}).

\begin{theorem}[Wrong-value acceptance]
\label{thm:mac-sound}
Let a batch of $m$ positions submitted to \CheckOpen{} (\cref{alg:checkopen}) differ from the prescribed tuples by a value error $\bm{e}\in\Fp^m$ and tag errors $\bm{d}_1,\dots,\bm{d}_t\in\Fp^m$, fixed by the freeze. If $\bm{e}\ne\bm{0}$, no earlier batch with a nonzero value error has been accepted, and the lanes use independent uniform challenges $\bm{\rho}_j\in\Fp^m$ drawn after the freeze and hidden from the host, \CheckOpen{} accepts with probability at most $(2/p)^t$ in $\Hyb{2}$. Over at most $Q$ batches, an incorrect value is ever accepted with probability at most $Q(2/p)^t$.
\end{theorem}

\noindent\textit{Proof idea.}
Lane $j$ accepts iff $\inner{\bm{\rho}_j}{\bm{d}_j-\Delta_j\bm{e}}=0$. For $e_i\ne 0$ the vector vanishes only if $\Delta_j=d_{j,i}/e_i$ (probability $\le 1/p$ by \cref{lem:hidden-key}); otherwise the nonzero linear form vanishes with probability $1/p$~\cite{schwartz1980fast}. Each lane gives $1/p+(1-1/p)/p<2/p$, and lanes are independent. Apply the bound to the first wrong-value batch; a union bound over batches gives $Q(2/p)^t$, following the SPDZ MAC check~\cite{damgard2012spdz,damgard2013practical} (\cref{app:proof-auth}).

\begin{theorem}[Authenticated arithmetic and direct gates]
\label{thm:arith}
With correct modules and prescribed messages, the protocols of \cref{fig:arith} are exact: $\Pi_{\mathsf{Input}}$ yields $\auth{x}$ with $x=r+\varepsilon$ (or aborts unless $x\in\mathsf{In}_\nu$), $\Pi_{\mathsf{Lin}}$ preserves $\gamma_{0,j}+\gamma_{1,j}=\Delta_j x$, $\Pi_{\mathsf{Mult}}$ with a correct fresh triple yields $\auth{xy}$ (and $\auth{XY}$ with the factor order preserved), and $\Pi_{\mathsf{Out}}$ gives $y=\upsilon-o$ to its authorized recipient. A direct protected gate (\cref{sec:proto-direct}) for an approved deterministic $g$, evaluated from protected memory in data-independent time, outputs \AuthShare$(g(c-r))$, an authenticated sharing of $g(x)$ whose party-local tuple is uniform as in \cref{thm:epilogue}. Unless a nonzero value error is accepted or a binding fails, every deviation of a corrupt host selects a permitted input, leaves the computation unchanged, or causes abort.
\end{theorem}

\noindent\textit{Proof idea.}
With $d=x-a$, $e=y-b$ and $c=ab$: $c+db+ea+de=xy$~\cite{beaver1991efficient}, the tags follow scaled by $\Delta_j$, $Z=C+DB+AE+DE$ for matrices, and $\upsilon-o=(y+o)-o=y$ with $o$ uniform. A direct gate recomputes $x=c-r$ from a verified opening, and its trace falls under $\eps{trace}$. \CheckOpen{} and the ledger block changed or reused material; induct over gates (\cref{app:proof-auth}).

\begin{theorem}[Canonical bit decomposition]
\label{thm:bitdec}
For $p=2^n-1$ ($n=61$), \cref{alg:bitdec} returns authenticated bits (least significant first) of the canonical representative of $x$, using one masked opening $c=x+r\bmod p$ and $2n$ authenticated multiplications.
\end{theorem}

\noindent\textit{Proof idea.}
The first loop is a full subtractor giving $d=(c-r)\bmod 2^n$ and borrow $\one[c<r]$; with a borrow $x=c-r+p=d-1$ since $p=2^n-1$, which the second loop subtracts~\cite{damgard2006unconditionally} (\cref{app:proof-gates}).

\begin{theorem}[Exact comparison and signed truncation]
\label{thm:cmp-trunc}
From authenticated canonical bits of $x$ and a public $\theta\in[0,2^n)$, \cref{alg:trunc} returns authenticated $\one[x<\theta]$; for centered $z\in[-(p-1)/2,(p-1)/2]$ it returns $\mathrm{sgn}(z)\lfloor|z|/2^f\rfloor$, i.e., truncation toward zero.
\end{theorem}

\noindent\textit{Proof idea.}
The equality flag tracks the processed prefix, and $\mathit{lt}$ gains a term exactly at the first position with secret bit $0$ and threshold bit $1$. Negative values occupy the canonical upper half; $(1-2s)z$ is the magnitude without wrap, and shifting its bits floors~\cite{catrina2010improved}. Fixed-point products must stay below $p/2$ before truncation (\cref{app:proof-gates}).

\begin{theorem}[Authenticated LUT]
\label{thm:lut}
For an approved table $T$ of $2^w$ entries and certified authenticated bits of $x\in\bits{w}$, if the mask bits and the DPF target of the keys for $(r,1)$ come from the same fresh uniform $r$, \cref{alg:lut} outputs $\auth{T[x]}$ and the opened $u=x\oplus r$ is uniform given $x$.
\end{theorem}

\noindent\textit{Proof idea.}
By \cref{thm:dpf-correct}, $\tilde{y}_0+\tilde{y}_1=\sum_a T[a\oplus u]\one[a=r]=T[x]$, and XOR by fixed $x$ is a bijection; independent resampling of the target would break the identity (\cref{app:proof-gates}).

\begin{theorem}[Intervals and piecewise polynomials]
\label{thm:interval}
For a proper nonempty public $[a,b)\subset[0,p)$, \cref{alg:interval} outputs $\auth{\one[a\le x<b]}$; for a disjoint exhaustive partition, Horner evaluation of the selected coefficients outputs $P_{i^\star}(x)$ for the interval containing $x$, in the declared finite arithmetic.
\end{theorem}

\noindent\textit{Proof idea.}
Adding $r$ maps $[a,b)$ to the circular interval from $L$ to $H$; the indicator is $\one[c<H]-\one[c<L]$ if $L<H$ and $1+\one[c<H]-\one[c<L]$ if $L>H$, which is the raw share by \cref{thm:dcf}. Exactly one indicator is one, and Horner with \cref{thm:arith} gives the polynomial; no equality to an unapproximated real function is claimed (\cref{app:proof-gates}).

The next two lemmas state when the semi-honest decoupling, which samples DPF targets directly~\cite{dfa2026trusted}, remains valid: joint distributions with all auxiliary material must match, not only marginals (\cref{sec:proto-refactor}).

\begin{lemma}[Bijection with correlated auxiliary material]
\label{lem:bijection}
Fix $Z=z$, $R$ uniform on a finite $\mathcal{R}$, a bijection $g_z:\mathcal{R}\to\mathcal{A}$, independent coins $W$ and an auxiliary sampler $J$. Then $(R,g_z(R),J(z,R,W))$ and $(g_z^{-1}(A),A,J(z,g_z^{-1}(A),W))$ with $A$ uniform on $\mathcal{A}$ are identically distributed.
\end{lemma}

\noindent\textit{Proof idea.}
Each pair $(r,a)$ has probability $1/|\mathcal{R}|$ in both experiments if $a=g_z(r)$ and zero otherwise; the same $J$ preserves equality. Independently resampling correlated targets such as $(r,r+1)$ breaks it (\cref{app:proof-gates}).

\begin{lemma}[Noninvertible transformations]
\label{lem:noninv}
For any $g$, sampling $A$ from the law of $g(R)$ and $R'$ from $R\mid g(R)=A$ reproduces $(R,g(R))$ and everything derived from $R'$. For unsigned truncation of a uniform $\ell$-bit mask by $h$ bits, $R'=2^hA+U$ with $A$, $U$ uniform on $\ell-h$ and $h$ bits.
\end{lemma}

\noindent\textit{Proof idea.}
$\Pr[A=a]\Pr[R=r\mid g(R)=a]=\Pr[R=r,g(R)=a]$; each truncated mask has probability $2^{-\ell}$. Signed shifts and other moduli need their own samplers (\cref{app:proof-gates}).

\begin{theorem}[Frozen-operand matrix check]
\label{thm:freivalds}
Let the module bind $A\in\Fp^{m\times k}$, $B\in\Fp^{k\times n}$, whose exposure to the GPU is already permitted, and freeze a claimed $C$. If $C\ne AB$, \cref{alg:freivalds} with $s$ secret uniform $\bm{v}\in\Fp^n$ drawn after the freeze accepts with probability at most $p^{-s}$, and over $Q_F$ calls an incorrect product is consumed with probability at most $Q_F/p^s$.
\end{theorem}

\noindent\textit{Proof idea.}
A nonzero row $\bm{e}$ of $C-AB$ gives $\inner{\bm{e}}{\bm{v}}=0$ for a $1/p$ fraction of $\bm{v}$~\cite{freivalds1977probabilistic,tramer2018slalom}; repetitions multiply; freezing fixes $C$ before $v$, and binding ties the verified bytes to the consumed ones (\cref{app:proof-gates}).

\begin{theorem}[Versioned-snapshot PIR]
\label{thm:pir}
With correct modules and binding snapshot and query interfaces: (R1) with an honest client and at most one malicious server host, \cref{alg:pir} gives the client the record $D[\alpha]$ of the snapshot committed by $\mathsf{cm}_v$ or abort, and the corrupt host's view is simulatable without $\alpha$; (R2) with a malicious client alone, accepted requests reveal nothing about the database beyond the requested records and the public descriptor $\mathsf{desc}_v$. Both modules learn $\alpha$, so the query privacy of (R1) rests on module trust, unlike untrusted two-server DPF-PIR (GPU-DPF~\cite{lam2023gpu}, untrusted-mode DFA~\cite{dfa2026trusted}), which hides $\alpha$ without trusted hardware.
\end{theorem}

\noindent\textit{Proof idea.}
\Cref{thm:dpf-correct} gives $y_0+y_1=\sum_i(\DPF_0(i)+\DPF_1(i))D[i]=D[\alpha]$; hashing the consumed bytes, comparing queries and role-bound certificates prevent substitution ($\eps{bind}$); results are freshly reshared (\cref{thm:epilogue}). For a malicious client the simulator extracts the index and reshares the ideal record (\cref{app:proof-pir}).

\textbf{Batched execution.}
The PIR configuration of \cref{tab:pir} processes $B=512$ queries per scan as one admitted execution whose manifest lists the $B$ query identifiers $\mathit{qid}$. Each query has its own joint DPF and pad labels, so the simulation of \cref{app:proof-pir} applies query by query. $B$ is part of the public schedule in $\Leak_{\mathrm{PIR}}$, and one abort (e.g., a snapshot mismatch) denies all $B$ queries, which security with abort permits.

% =====================================================================
\subsection{Scenario-by-Scenario Analysis}
\label{sec:sec-scenarios}

We map the scenarios of \cref{fig:scenarios,tab:scenarios} to the statements above; \cref{tab:attacks} lists the corresponding injections.

\begin{itemize}[leftmargin=*]
\item \textbf{S1: Share and tag tampering.} Freeze (S3) and \cref{thm:mac-sound,lem:hidden-key}: a wrong value passes with probability at most $(2/p)^t$ per batch; only the abort bit is revealed.
\item \textbf{S2: Forgery-oracle request.} No command (\cref{tab:commands}) tags a host value; the epilogue tags only protected results (\cref{thm:epilogue}); chosen values enter by input extraction.
\item \textbf{S3: TOCTOU buffer swap.} Freeze-before-challenge realizes the premise of \cref{thm:mac-sound} that errors precede challenges; tampered spill pages abort ($\eps{bind}$).
\item \textbf{S4: Replay and rollback.} Ledger and label binding ($\eps{bind}$) reject reused material; resuming old keys is excluded by the freshness clause.
\item \textbf{S5: Role/gate confusion.} Role-bound keys, joint labels and ledger descriptors turn misrouting into a mismatch and abort ($\eps{bind}$).
\item \textbf{S6: Premature release.} The release guard opens only \lstate{VERIFIED} entries; private outputs are opened as $\upsilon=y+o$, uniform to every host that is not the authorized recipient (\cref{thm:arith}).
\item \textbf{S7: Malformed preprocessing.} Triples and keys are correct because they are generated inside the boundary (\cref{thm:arith}), not because a MAC check certifies them; GPU products need \cref{thm:freivalds}, and correlated targets need \cref{lem:bijection,lem:noninv}.
\item \textbf{S8: Snapshot substitution.} Same-byte hashing and quarantine give the committed record or abort (\cref{thm:pir}).
\item \textbf{S9: Input substitution.} Permitted by $\FC$ and extracted; model provenance requires the committed-input loader.
\item \textbf{S10: Denial of service and selective abort.} Not prevented; aborts occur at public boundaries and are simulatable, and abort and validation outcomes ($\mathsf{status}$) are part of $\Leak_C$.
\end{itemize}

% =====================================================================
\subsection{Concrete Security}
\label{sec:sec-concrete}

Since $2/p\approx 2^{-60}$ for $p=2^{61}-1$, we have $\log_2 Q(2/p)^t\approx\log_2 Q-60t$. For a budget of $Q\le 2^{32}$ checked batches, \cref{tab:lanes} gives the statistical term.

\begin{table}[t]
\centering
\caption{Statistical term and BERT-Base LAN latency versus the number $t$ of MAC lanes ($Q\le 2^{32}$). Latencies are model estimates}
\label{tab:lanes}
\footnotesize
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{c c c c}
\hline
$t$ & $(2/p)^t$ per batch & $Q(2/p)^t$ & BERT-Base LAN (s)\\
\hline
1 & $\approx 2^{-60}$ & $\approx 2^{-28}$ & \est{2.53}\\
2 & $\approx 2^{-120}$ & $\approx 2^{-88}$ & \est{3.18}\\
3 & $\approx 2^{-180}$ & $\approx 2^{-148}$ & \est{3.83}\\
\hline
\end{tabular}
\end{table}

One lane is inadequate. Since the primitives target 128-bit computational security, $t=3$ is the smallest $t$ whose statistical term falls below $2^{-128}$; beyond it the primitives, not the MAC, limit the bound. Extra lanes barely change \CheckOpen{} itself (\est{0.648~ms} for $t=1$ versus \est{0.652~ms} for $t=3$ at $m=65{,}536$ on LAN, \cref{fig:checkperf}); their cost is one more authenticated GEMM lane per key (last column of \cref{tab:lanes}; \cref{sec:eval-ablation}).

\textbf{Tag-only errors.}
The bound concerns wrong \emph{values}: an error in a single tag lane escapes with probability $1/p$ without changing the opened value.

\textbf{Independent challenges.}
With one shared vector $\bm{\rho}$, an adversary submitting $\bm{d}_j=\bm{0}$ and any $\bm{e}\ne\bm{0}$ makes every lane residual $-\Delta_j\inner{\bm{\rho}}{\bm{e}}$, and all lanes vanish together with probability $1/p$. The product bound then collapses to one lane, so shared challenges are rejected (injection~8, \cref{tab:attacks}).

\textbf{Field, not ring.}
The step $\Delta_j=d_{j,i}/e_i$ needs a field. Over $\Z_{2^{64}}$, $e_i=2^{63}$ gives $\Delta_j e_i\equiv 0$ for every even $\Delta_j$, so one lane accepts with probability at least $1/2$; ring arithmetic needs a SPDZ2k-type backend~\cite{cramer2018spdz2k} with its own proof.

\textbf{Matrix checks.}
With $s=3$, each Freivalds call accepts a wrong product with probability at most $p^{-3}\approx 2^{-183}$, so $Q_F\le 2^{32}$ calls add at most $Q_F/p^{3}\approx 2^{-151}$ to the bound of \cref{thm:main}. Rejection sampling rejects one value with probability $2^{-61}$ per draw and retries under a fresh label; exhaustion affects only availability.

% =====================================================================
\subsection{Proof Boundary and Implementation Obligations}
\label{sec:sec-boundary}

\Cref{thm:main} concerns the abstract protocol in the protected-module model; \cref{tab:obligations} separates what this paper establishes from what a deployment must still provide. We executed a specification and a functional CPU reference model; its tests (\cref{sec:eval-attack}) check conformance on finite cases and are neither a machine-checked proof nor evidence for the statistical bound. GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet.

\begin{table}[t]
\centering
\caption{Proof boundary: what this paper establishes and what a deployment must still provide}
\label{tab:obligations}
\footnotesize
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{\columnwidth}{>{\raggedright\arraybackslash}p{1.8cm}>{\raggedright\arraybackslash}X>{\raggedright\arraybackslash}X}
\hline
\textbf{Obligation} & \textbf{Established here} & \textbf{Still required}\\
\hline
DPF/DCF, GaC, field, Boolean, LUT algebra & Explicit algorithms; \cref{thm:dpf-correct,thm:gac,thm:dcf,thm:bitdec,thm:cmp-trunc,thm:lut,thm:interval}; CPU reference tests & Constant-time, bit-exact CUDA and RTL refinement\\
\hline
Wrong-value authentication & \Cref{lem:hidden-key,thm:mac-sound}, independent lanes & Correct freeze, entropy, parser and check engine\\
\hline
End-to-end privacy and correctness & \Cref{thm:main} in the protected-module model & Realization of every module and trace assumption\\
\hline
PIR & \Cref{thm:pir} for the specified snapshot and regimes & Secure query channel, same-byte scan, certificates\\
\hline
GPU matrix verification & \Cref{thm:freivalds} & Protected verifier, bound input/result integration\\
\hline
Physical leakage and faults & Not claimed & Threat-specific engineering and evidence\\
\hline
Software-controlled DVFS and power telemetry & Required isolation specified & Isolated or monitored voltage and clock domain; telemetry filtering\\
\hline
Rollback protection & Required semantics specified (\cref{sec:proto-ledger}) & Monotonic service or erase-and-rekey lifecycle\\
\hline
Machine-checked proof & Not claimed & Future Lean, Coq or EasyCrypt development\\
\hline
\end{tabularx}
\end{table}

\textbf{Relation to the semi-honest design.}
The DFA analysis~\cite{dfa2026trusted} shows that its transformations preserve semi-honest security; \cref{thm:main} tolerates a malicious host and GPU by placing more integrity and lifecycle responsibility inside the boundary.


==> qa/draft4/sections/08_evaluation.tex <==
% =====================================================================
% Section VIII: Evaluation
% Numbers: model/numbers.md (red via \est{}), DFA paper (black + cite),
% executed CPU reference tests (black).
% =====================================================================
\section{Evaluation}\label{sec:eval}

We evaluate the cost of the protected gates and verified openings of \sys (\cref{sec:eval-micro,sec:eval-check}), end-to-end inference against semi-honest trusted DFA and dealer-based malicious FSS (\cref{sec:eval-e2e}), PIR (\cref{sec:eval-pir}), attack coverage and silicon cost (\cref{sec:eval-attack,sec:eval-hw}), and ablations and scaling (\cref{sec:eval-ablation,sec:eval-scale}).

% =====================================================================
\subsection{Evaluation Methodology}\label{sec:eval-method}

\textbf{Evidence status.}
We distinguish three kinds of numbers.
Black numbers cited to~\cite{dfa2026trusted} are copied from the semi-honest DFA paper; its end-to-end rows combine measured A100 execution with simulated DFA hardware.
Black numbers without a citation are analytical (operation counts, design constants and security parameters such as $p=2^{61}-1$, $t=3$ and $Q(2/p)^t$) or counts from the executed CPU reference tests of \cref{sec:eval-attack}.
Red marks assumed model parameters and outputs of the analytical performance model of \cref{app:model}; they are placeholders to be replaced by measurements.
We executed a specification and a functional CPU reference model; GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet.
Every conclusion drawn from a red number is therefore conditional on the model assumptions, and we name the dominant assumption wherever a conclusion depends on it.

\textbf{Hardware cost.}
The DFA blocks that \sys reuses (16 DPF units with 64 AES-128 engines, SRAM buffers, a 16-lane Ara VPU~\cite{cavalcante2019ara} and an SC300-class control core~\cite{st33tpm12spi,arm_cortex_m3}) keep the TSMC 28~nm synthesis results of~\cite{dfa2026trusted}, which use a pipelined open-source AES-128 core~\cite{opencores_aes128_pipeline}.
For the blocks that \sys adds (\cref{sec:arch-hw}), namely the Mersenne-61 field unit array (FUA), the check engine, the AEAD/GHASH block shared by the freezer and the peer-channel controller, the ledger with release guard and parser, and the ledger and freeze SRAMs, this paper reports pre-synthesis component estimates at the DFA clock (720~MHz at 28~nm, 910~MHz at 7~nm); they will be replaced by synthesis in the same 28~nm flow.
As in DFA, we scale to 7~nm with DeepScaleTool~\cite{sarangi2021deepscaletool}.
Separately, we size a functional prototype on a ZCU102 board (XCZU9EG, ffvb1156, speed grade $-2$)~\cite{amd2023zcu102} for Vivado implementation; its resource and power figures are pre-implementation estimates and will be reported separately from measured board energy.

\textbf{System-level performance.}
The target methodology for headline numbers is that of DFA: the module sits next to the GPU L2 slices, where DFA delivers about 290~GB/s~\cite{dfa2026trusted}, its DPF and FSS work is modeled as a stream consumed by GPU kernels in Accel-Sim~\cite{khairy2020accel}, and non-FSS work comes from real GPU execution.
The three experiments of \cref{sec:arch-deploy} (A100 software, ZCU102 prototype, Accel-Sim on-die study) are never merged.
Until they are measured, every \sys row comes from a decomposition of DFA's trusted-mode rows into GPU linear algebra, other GPU work, module FSS work, CPU-GPU transfers, online bytes and online rounds, transformed for four authenticated lanes, exact Mersenne GEMM and doubled rounds; all constants are in \cref{app:model} and \cref{tab:model-params}.
The decomposition parameters are fitted to the LAN and WAN latencies of~\cite{dfa2026trusted} (largest deviation \est{0.42\%}, ResNet-50 LAN).
Two published latencies per model cannot identify five parameters, so the fit is a consistency constraint, not a validation; the split between GPU linear algebra, other GPU work, bytes and rounds, on which every malicious factor acts, is itself an assumption to be replaced by profiling the A100 baseline.
Because authenticated GEMM dominates every malicious row, the most influential factor is the assumed \est{1.25$\times$} cost of exact 61-bit Mersenne GEMM over wraparound $\Z_{2^{64}}$ GEMM per lane; Tensor Cores are not used for field arithmetic (\cref{sec:arch-field}).

\textbf{Baselines.}
For private inference we compare five configurations per model.
\emph{GPU (SH)} and \emph{GPU+Trusted DFA (SH)} are the semi-honest rows of~\cite{dfa2026trusted}, which build on Orca~\cite{jawalkar2024orca} for CNNs and Sigma~\cite{gupta2023sigma} for Transformers.
\emph{Dealer-based malicious FSS} is modeled after the protocol family of Shark~\cite{gupta2025shark}: an external dealer ships authenticated keys and preprocessing, which we model with assumed factors (\cref{app:model}) of \est{2.2$\times$} the semi-honest key and preprocessing volume, \est{2.0$\times$} the GPU FSS evaluation work and \est{2.4$\times$} the semi-honest GPU energy, while charging exactly the same authenticated linear algebra, online bytes and doubled rounds as \sys.
The comparison therefore isolates preprocessing and key handling; it does not equalize trust.
The dealer of this protocol family is an input-independent third party that can run offline and away from both servers, and it never sees an input or an opening, so breaking privacy requires its masks together with a server's view.
The \sys modules sit inside the adversary's platform and see every input and opening (\cref{sec:threat-model}), so extracting the secrets of either module suffices.
The speedups below are therefore obtained under a stronger hardware-confidentiality assumption; a deployment that cannot accept it must use \ProfU, which we do not evaluate.
The row models the protocol family, not the Shark artifact, and we make no performance claim against Shark itself until a matching artifact has been run.
We do not model a dealer-free (MASCOT, SPDZ2k or PCG-based) malicious baseline~\cite{keller2016mascot,cramer2018spdz2k,boyle2019pcg}; \cref{sec:analysis-cost} explains why its FSS keys remain costly.
\emph{GPU+\sys w/o GaC} generates authenticated material locally but, like the corresponding DFA ablation, spills it to host memory through the AEAD spill path and rereads it.
\emph{GPU+\sys} is the compiler-selected default.
For PIR we compare GPU-DPF~\cite{lam2023gpu} and GPU+DFA, both semi-honest and taken from~\cite{dfa2026trusted}, a GPU-DPF variant that adds authenticated PIR in the style of Colombo et al.~\cite{colombo2023apir} (assumed to reach \est{0.45$\times$} the GPU-DPF throughput at \est{350~W}), and GPU+\sys.

\textbf{Workloads.}
We run ResNet-50~\cite{he2016deep}, BERT-Base~\cite{devlin2019bert}, GPT-Neo~\cite{brown2020language} and LLaMA2-7B~\cite{touvron2023llama}, with 128 input tokens for the Transformer models, as in~\cite{dfa2026trusted}.
LAN is 1~GB/s with a 0.05~ms round-trip time (RTT) and WAN is 70~MB/s with a 70~ms RTT, following~\cite{gupta2023sigma,jawalkar2024orca,huang2026beyond}.
Malicious configurations use $\Fp$ with $p=2^{61}-1$ and $t=3$ MAC lanes; semi-honest rows use $\Z_{2^{64}}$ as in their sources.
Unless stated otherwise, the compiler selects among direct, LUT and interval gates by modeled cost subject to the FSS-portability constraint (\cref{sec:proto-direct,app:model}).
PIR databases hold 16K to 4M entries of 128 bits (\cref{tab:pir}), served in batches of 512 queries; \cref{fig:scale} extrapolates the model to 16M ($2^{24}$) entries.
We do not report inference accuracy; exact finite-reference agreement and model accuracy will be reported once bit-exact GPU conformance is established.

\textbf{Measurement protocol.}
The replacement measurements will use 5 warm-up runs and 30 measured repetitions, report the median and the 95th percentile with bootstrap confidence intervals, keep raw per-run records, and fix random seeds only for public synthetic inputs, since randomness used for security must remain fresh.
We will report per-stage service times (cold and amortized setup, preprocessing, online arithmetic, nonlinear evaluation, checking, transfers and final release) next to the critical-path wall time, counting both parties and any external preprocessing service.
Network conditions are shaped on dedicated interfaces with Linux traffic control, recording achieved throughput and RTT.
GPU energy integrates sampled GPU power, board energy is measured at the rail or the wall, and every energy figure is cross-checked against average power times latency (or throughput times energy per query).

% =====================================================================
\subsection{Microbenchmarks}\label{sec:eval-micro}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_dpfthr.pdf}
\caption{Single-path DPF gate throughput per module (M gates/s, log scale) at 28~nm, 720~MHz and 64 AES-128 engines, for input length $n$: semi-honest trusted DFA, \sys (GaC with fresh authentication epilogue), and a malicious variant with per-lane tag trees ($t=3$ extra trees). Model estimates.}
\label{fig:dpfthr}
\end{figure}

\textbf{DPF gate throughput.}
\sys sustains \est{106} against \est{113}~M~gates/s for trusted DFA at $n=61$ and stays \est{6--9\%} below it for all $n$, because the epilogue adds two AES blocks per gate and we assume a pipeline efficiency of \est{0.85} (\est{0.90} for trusted DFA; \cref{app:model}).
It is \est{3.8--4.0$\times$} faster than per-lane tag trees for all $n$, approaching the factor $1+t=4$ by which tag trees multiply DPF work (\cref{fig:dpfthr,tab:gatecost}), with a single-gate latency of \est{1.71~$\mu$s} at $n=61$.
These are DPF gate rates: complete gates also include input masking, a verified opening and the surrounding arithmetic (\cref{sec:eval-e2e}).

\begin{table}[t]
\centering
\caption{Authenticated Nonlinear Gate Options per Module}
\label{tab:gates}
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l r r r r r}
\hline
\textbf{Gate} & \makecell{\textbf{Online}\\\textbf{rounds}} & \makecell{\textbf{AES}\\\textbf{blocks}} & \makecell{\textbf{Field}\\\textbf{mults}} & \makecell{\textbf{Thr.}\\\textbf{(M/s)}} & \makecell{\textbf{LAN lat.}\\\textbf{(ms)}} \\
\hline
Direct protected gate & 1 & 2 & 5 & \est{1{,}800} & \est{0.100} \\
LUT, $w=8$ & 1 & 542 & 268 & \est{72.3} & \est{0.100} \\
LUT, $w=12$ & 1 & 8{,}238 & 4{,}112 & \est{4.75} & \est{0.100} \\
LUT, $w=16$ & 1 & 131{,}134 & 65{,}556 & \est{0.30} & \est{0.104} \\
Interval, conservative DCF & 1 & 22{,}692 & 8 & \est{1.73} & \est{0.100} \\
Interval, optimized DCF$^{\ast}$ & 1 & \est{976} & 8 & \est{40.1} & \est{0.100} \\
Bit decomposition & 123 & n/m & 122 & n/a & \est{12.3} \\
Exact signed truncation & 309 & n/m & 307 & n/a & \est{30.9} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize $n=61$; 28~nm, 720~MHz, 64 AES engines, 128 field lanes. Rounds, AES blocks and field multiplications are analytical counts per gate; throughput and LAN latency are model estimates. The direct-gate throughput is an assumed rate for evaluating $g$ in the module, not derived from the AES and FUA peak rates. One online round is one \CheckOpen, i.e., two inter-module round trips; rounds include masked openings. LUT rows assume that the multiplication round of the $w$ XOR products batches with the preceding layer's openings (\cref{app:model}); otherwise they need one more round. n/a: round-bound, throughput not meaningful; n/m: not modeled (the AES work of the round-bound gates is negligible next to their round trips).
$^{\ast}$Projected $O(n)$ DCF; not covered by \cref{thm:dcf}.}
\end{table}

\textbf{Nonlinear gates.}
\Cref{tab:gates} compares the authenticated gate options of \cref{sec:proto-gates}.
All gates with one online round pay the two-round-trip floor of one \CheckOpen{} (0.1~ms on LAN; a LUT whose XOR products cannot batch with the preceding layer pays a second round) and differ only in throughput, which favors the direct gate (an assumed \est{1{,}800}~M~gates/s) and small LUTs (LUT work grows as $2^w$) and penalizes the conservative DCF (\est{1.73}~M~gates/s); the optimized DCF would reach \est{40.1}~M~gates/s but lies outside our proofs.
Bit decomposition and exact signed truncation are round-bound (123 and 309 rounds, \est{12.3~ms} and \est{30.9~ms} on LAN), so the compiler uses them only as a fallback when no table or interval formulation of the gate exists.

% =====================================================================
\subsection{Cost of Verified Openings}\label{sec:eval-check}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_checkopen.pdf}
\caption{\CheckOpen{} cost versus batch size $m$ (64 to 65{,}536 elements): (a)~LAN latency for $t=1,2,3$ MAC lanes (the curves overlap); (b)~throughput on LAN and WAN for $t=3$ (log scale). Model estimates.}
\label{fig:checkperf}
\end{figure}

\Cref{fig:checkperf} sweeps the \CheckOpen{} batch size $m$ from 64 to 65{,}536 elements, and three observations guide the compiler.
First, the number of MAC lanes barely matters for cost: even at $m=65{,}536$, moving from $t=1$ to $t=3$ raises LAN latency only from \est{0.648~ms} to \est{0.652~ms}, while the statistical term improves from $2^{-28}$ to $2^{-148}$ at $Q=2^{32}$ (\cref{thm:mac-sound}).
Second, on LAN the two round trips (0.1~ms) dominate up to a few thousand elements (\est{0.101~ms} to \est{0.135~ms} between $m=64$ and $m=4{,}096$); beyond that the 8-byte value share per element on the peer link dominates (\est{0.52~ms} of \est{0.652~ms} at $m=65{,}536$), throughput saturates near \est{100}~M~elements/s, and the protected work stays below \est{5\%} of the check latency.
Third, on WAN the two 70~ms round trips set a floor of 140~ms per check, so throughput is only \est{0.44}~M~elements/s even at $m=65{,}536$; batching independent openings (\cref{sec:proto-check}) is therefore essential, and the round count, rather than bandwidth or module work, is the WAN price of malicious security (\cref{sec:eval-ablation}).

% =====================================================================
\subsection{End-to-End Private Inference}\label{sec:eval-e2e}

\begin{table*}[t]
\centering
\caption{End-to-End Private Inference per Query}
\label{tab:e2e}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l l c r r r r r r}
\hline
\textbf{Model} & \textbf{Method} & \textbf{Security} & \makecell{\textbf{Offline}\\\textbf{comm. (GB)}} & \makecell{\textbf{CPU-GPU}\\\textbf{(GB)}} & \makecell{\textbf{Module-GPU}\\\textbf{(GB/party)}} & \makecell{\textbf{LAN}\\\textbf{latency (s)}} & \makecell{\textbf{WAN}\\\textbf{latency (s)}} & \makecell{\textbf{GPU+module}\\\textbf{energy (J)}} \\
\hline
\multirow{5}{*}{ResNet-50}
 & GPU~\cite{dfa2026trusted} & SH & 9.9 & 10.2 & n/a & 10.9 & 162 & 71.0 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.02 & 0.34 & n/r & 0.73 & 18.0 & 11.9 \\
 & Dealer-based malicious FSS & Mal & \est{21.8} & \est{22.4} & n/a & \est{25.1} & \est{346} & \est{170} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{38.0} & \est{1.22} & \est{2.97} & \est{34.7} & \est{48.6} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{0.44} & \est{1.22} & \est{1.79} & \est{33.6} & \est{43.6} \\
\hline
\multirow{5}{*}{BERT-Base}
 & GPU~\cite{dfa2026trusted} & SH & 17.1 & 19.3 & n/a & 18.8 & 296 & 121 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.1 & 2.55 & n/r & 1.42 & 46.4 & 18.2 \\
 & Dealer-based malicious FSS & Mal & \est{37.6} & \est{42.5} & n/a & \est{43.9} & \est{630} & \est{290} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{68.6} & \est{1.66} & \est{5.87} & \est{91.8} & \est{82.2} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{3.31} & \est{1.66} & \est{3.83} & \est{89.7} & \est{73.7} \\
\hline
\multirow{5}{*}{GPT-Neo}
 & GPU~\cite{dfa2026trusted} & SH & 76.4 & 80.4 & n/a & 83.6 & 1{,}140 & 587 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.24 & 4.27 & n/r & 5.93 & 101 & 114 \\
 & Dealer-based malicious FSS & Mal & \est{168} & \est{177} & n/a & \est{197} & \est{2{,}611} & \est{1{,}409} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{296} & \est{9.92} & \est{28.6} & \est{209} & \est{522} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{5.55} & \est{9.92} & \est{19.5} & \est{200} & \est{477} \\
\hline
\multirow{5}{*}{LLaMA2-7B}
 & GPU~\cite{dfa2026trusted} & SH & 256 & 268 & n/a & 279 & 3{,}695 & 1{,}879 \\
 & GPU+Trusted DFA~\cite{dfa2026trusted} & SH & 0.81 & 12.8 & n/r & 18.0 & 193 & 303 \\
 & Dealer-based malicious FSS & Mal & \est{563} & \est{590} & n/a & \est{661} & \est{8{,}467} & \est{4{,}510} \\
 & GPU+\sys w/o GaC & Mal & \est{$<$0.001} & \est{994} & \est{33.3} & \est{93.6} & \est{418} & \est{1{,}483} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & Mal & \est{$<$0.001} & \est{16.6} & \est{33.3} & \est{63.1} & \est{387} & \est{1{,}343} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\textwidth}{\footnotesize SH: semi-honest; Mal: static malicious security with abort. Latency is end to end, including offline distribution where present. Energy is GPU plus module energy summed over both computing parties (and the dealer when present). Module-GPU is the authenticated tuple stream per party on the on-die path; n/a: no module; n/r: not reported in~\cite{dfa2026trusted}. SH rows are copied from~\cite{dfa2026trusted}; red values are model estimates.}
\end{table*}

\Cref{tab:e2e} reports per-query results for the four models.
The semi-honest rows are context, not same-security competitors.

\textbf{Comparison with dealer-based malicious FSS.}
The modeled dealer-based baseline pays for malicious security mainly offline: its dealer ships \est{21.8--563~GB} of authenticated keys and preprocessing per query, which each party then stages through CPU-GPU transfers, whereas \sys generates the authenticated correlations inside the modules and ships none of them (\est{$<$0.001~GB} of session setup).
Across the four models this yields \est{10.1--14.0$\times$} lower LAN latency, \est{7.0--21.9$\times$} lower WAN latency and \est{3.0--3.9$\times$} lower energy than the modeled baseline (\est{11.4$\times$}, \est{7.0$\times$} and \est{3.9$\times$} for BERT-Base); the energy ratio rests on the assumed \est{2.4$\times$} energy factor of the baseline.
These latency ratios include the per-query offline distribution; excluding it, \sys is \est{1.5--1.8$\times$} faster on LAN (\est{1.6$\times$} for BERT-Base), and with no authenticated-key blow-up ($\psi_{\mathrm{key}}=1$) the baseline still needs \est{22.4~s} for BERT-Base (\est{5.8$\times$}).
The end-to-end gains thus come mainly from generating authenticated correlations inside the modules; the epilogue's advantage (\est{3.8--4.0$\times$} over per-lane tag trees) is per gate.
The WAN gain is largest for LLaMA2-7B (\est{21.9$\times$}), whose \est{563~GB} of authenticated material alone would occupy a 70~MB/s link for more than \est{2.2~hours}.

\textbf{Cost of malicious security.}
Relative to semi-honest trusted DFA, \sys raises LAN latency by \est{2.46--3.51$\times$} (\est{2.7$\times$} for BERT-Base) and WAN latency by \est{1.86--2.01$\times$}; these factors rest on the assumed Mersenne GEMM cost, and doubling it ($\mu_{\mathrm{M}}=2$) would give \est{5.39~s}, or \est{3.8$\times$}, for BERT-Base (\cref{sec:arch-field}).
It nevertheless remains \est{4.3--6.1$\times$} faster on LAN and \est{3.3--9.5$\times$} faster on WAN than the semi-honest GPU baseline, and it uses \est{1.2--1.6$\times$} less energy, although it tolerates a malicious host.
CPU-GPU traffic is assumed to grow by \est{1.3$\times$} over trusted DFA ($\phi_{\mathrm{cg}}$, \cref{app:model}) for canonical field words, residuals and certificates; the authenticated tuples themselves (\est{1.22} to \est{33.3~GB} per party) take the on-die module-GPU path and do not add to it.

\textbf{Generate-and-consume remains essential.}
Without GaC, the locally generated authenticated material must be spilled and reread, which inflates CPU-GPU traffic by \est{20.7--86$\times$} (\est{68.6~GB} instead of \est{3.31~GB} for BERT-Base) and LAN latency by \est{1.47--1.66$\times$}.
The authenticated representation makes materialization costlier than in the semi-honest case, where DFA reports 36.1~GB of CPU-GPU traffic and a 1.74$\times$ LAN penalty for BERT-Base without GaC~\cite{dfa2026trusted}.

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_bert.pdf}
\caption{BERT-Base bottleneck analysis for \sys (model estimates). (a)~Speedup over dealer-based malicious FSS versus network bandwidth, split into the part due to eliminated key and preprocessing distribution and the remainder. (b)~LAN latency versus host-module link bandwidth (\est{1.6}, \est{8}, \est{25} and 290~GB/s~\cite{dfa2026trusted}). (c)~Breakdown of the \est{3.83~s} LAN latency.}
\label{fig:bert}
\end{figure}

\textbf{Bottleneck analysis.}
\Cref{fig:bert} decomposes the BERT-Base results.
(a)~The advantage over the dealer-based baseline depends on network bandwidth: \est{43.7$\times$} at 0.1~GB/s, \est{11.4$\times$} at 1~GB/s and \est{2.9$\times$} at 10~GB/s.
At 1~GB/s, \est{9.8$\times$} of the \est{11.4$\times$} comes from eliminated key and preprocessing distribution; at 10~GB/s, \est{1.7$\times$} of the \est{2.9$\times$} comes from lower key I/O and cheaper FSS evaluation and outweighs the distribution share.
Faster networks shrink the advantage but do not remove it, and, as observed for the semi-honest case~\cite{dfa2026trusted,huang2026beyond}, the energy and monetary cost of moving tens of gigabytes per query persists at any bandwidth.
(b)~Moving the module off die costs little for BERT-Base: LAN latency is \est{3.83~s} on die (290~GB/s), \est{3.87~s} over a \est{25~GB/s} PCIe-class link, \est{3.96~s} at \est{8~GB/s} and \est{4.46~s} at the \est{1.6~GB/s} of the ZCU102 prototype, because only \est{1.66~GB} of authenticated tuples per party cross the link.
(c)~The breakdown confirms Observation~2 of \cref{sec:analysis-cost}: authenticated GEMM accounts for \est{68\%} of the latency and \est{86\%} of the \est{2.41~s} added over trusted DFA, so the protected module is not the bottleneck; the tag lanes on the GPU and the doubled round count are, which motivates the compressed-check direction of \cref{sec:eval-scale}.

% =====================================================================
\subsection{Private Information Retrieval}\label{sec:eval-pir}

\begin{table}[t]
\centering
\caption{PIR Throughput and Energy per Query}
\label{tab:pir}
\footnotesize
\setlength{\tabcolsep}{2.0pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l l c c r r r}
\hline
\textbf{DB} & \textbf{Method} & \textbf{Integ.} & \makecell{\textbf{Index}\\\textbf{hidden}$^{\dagger}$} & \makecell{\textbf{Queries/s}\\\textbf{(k)}} & \makecell{\textbf{Energy/}\\\textbf{query (mJ)}} & \makecell{\textbf{Implied}\\\textbf{W}} \\
\hline
\multirow{4}{*}{16K}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & \cmark & 134 & 2.61 & 350 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & \cmark & 1{,}125 & 0.187 & 210 \\
 & GPU-DPF+APIR & \cmark & \cmark & \est{60.3} & \est{5.80} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \xmark & \est{1{,}046} & \est{0.180} & \est{188} \\
\hline
\multirow{4}{*}{1M}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & \cmark & 3.48 & 100 & 348 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & \cmark & 17.58 & 11.9 & 209 \\
 & GPU-DPF+APIR & \cmark & \cmark & \est{1.57} & \est{223} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \xmark & \est{16.35} & \est{11.5} & \est{188} \\
\hline
\multirow{4}{*}{4M}
 & GPU-DPF~\cite{dfa2026trusted} & \xmark & \cmark & 0.788 & 443 & 349 \\
 & GPU+DFA~\cite{dfa2026trusted} & \xmark & \cmark & 4.39 & 47.7 & 209 \\
 & GPU-DPF+APIR & \cmark & \cmark & \est{0.355} & \est{987} & \est{350} \\
\rowcolor{blue!6}\cellcolor{white} & GPU+\sys & \cmark & \xmark & \est{4.08} & \est{46.0} & \est{188} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize 128-bit entries, batch 512. SH rows are from~\cite{dfa2026trusted} with energy expressed in mJ; implied power is throughput times energy per query and serves as a unit cross-check. Integ.: the client obtains the committed record or abort against a malicious server host (R1). $^{\dagger}$Index hidden from each server without trusted hardware: GPU-DPF and GPU+DFA (untrusted mode, client-generated keys) and the APIR variant hide $\alpha$ from each server, whereas both \sys modules learn $\alpha$ and its query privacy relies on module trust. Red values are model estimates.}
\end{table}

\Cref{tab:pir} reports PIR throughput and energy per query.
Assuming a PIR efficiency of \est{0.93} relative to DFA ($\eta_{\mathrm{PIR}}$, \cref{app:model}), meant to cover snapshot hashing, the in-module record reduction and fresh resharing with bound certificates, \sys reaches \est{1{,}046}, \est{16.35} and \est{4.08}~k~queries/s, a consequence of this assumption to be replaced by the Accel-Sim study, not a result.
The integrity guarantee does not depend on the model: in regime (R1), with one malicious server host, an honest client receives the committed record or abort (\cref{thm:pir}).
Query privacy, however, is weaker than in untrusted two-server DPF-PIR: both modules learn $\alpha$, so privacy against the hosts relies on module trust, whereas GPU-DPF and untrusted-mode DFA hide $\alpha$ from each server without trusted hardware (\cref{app:func-pir}); the two \ProfT alternatives of \cref{sec:proto-pir} are not modeled.
Energy per query is \est{3--4\%} below DFA's (\est{0.180~mJ} vs.\ 0.187~mJ at 16K entries) only because we assume an average power of \est{188~W} ($P_{\mathrm{PIR}}$), with the record reduction moved from the SMs into the protected path; this is the least certain PIR value and among the first we will measure.
Likewise, the authenticated GPU baseline is an assumed \est{0.45$\times$} of GPU-DPF throughput at \est{350~W}, so the \est{10.4--17.4$\times$} higher throughput and \est{19--32$\times$} lower energy per query of \sys against it follow from these assumptions; against semi-honest GPU-DPF, \sys is \est{4.7--7.8$\times$} faster under a weaker query-privacy model.

\textbf{Bottleneck analysis.}
As in DFA, full-domain PIR is bound by DPF expansion in the AES array rather than by memory; DFA sustains about 18.4~G~leaves/s (1{,}125~k queries/s $\times$ $2^{14}$ entries~\cite{dfa2026trusted}).
The additional protected work is amortized over a batch: each batch of 512 queries scans the snapshot once in public order, so the snapshot hash costs one pass per batch rather than one per query, and every record is weighted by the 512 DPF outputs of the batch in the FUA.
At 16K entries this reduction needs about \est{51~G} field multiply-accumulates/s, below the 92.16~G/s that the 128-lane FUA delivers even at the 28~nm clock of 720~MHz (116~G/s at 910~MHz; \cref{app:model}).
This capacity check shows only that the FUA is not saturated; it does not establish the size of the throughput loss.

% =====================================================================
\subsection{Security Validation}\label{sec:eval-attack}

\begin{table*}[t]
\centering
\caption{Attack and Fault Injections and Their Expected Outcomes}
\label{tab:attacks}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{c >{\raggedright\arraybackslash}p{4.3cm} >{\raggedright\arraybackslash}p{5.0cm} c >{\raggedright\arraybackslash}p{4.9cm}}
\hline
\textbf{\#} & \textbf{Injection} & \textbf{Mechanism} & \makecell{\textbf{Reference}\\\textbf{model}} & \textbf{Expected RTL/FPGA outcome} \\
\hline
1 & Change payload, query, role, gate id, table hash or shape (S5) & Ledger descriptor binding; role- and gate-bound PRF labels (\cref{sec:proto-ledger}) & \cmark & \est{Rejected at frame parse or authenticated computation fails; no preprocessing issued} \\
2 & Flip a control bit, root seed or correction word in a candidate engine & Conformance against the reference DPF (\cref{thm:dpf-correct}); unverified engine output is never authenticated & planned & \est{Reference mismatch flagged; engine output never authenticated or released} \\
3 & Change a GPU value share or tag (S1) & \CheckOpen{} with $t=3$ independent lanes (\cref{thm:mac-sound}) & \cmark & \est{Abort within one \CheckOpen{} (0.10--0.65~ms on LAN)}; acceptance at most $(2/p)^3$ per batch \\
4 & Triple with valid-looking tags but $c\neq ab$ (S7) & Triples computed inside the TCB; imported material needs a correctness proof & planned & \est{Never consumed; unproven import refused at reservation} \\
5 & Reuse a mask or counter; reset and resume old keys (S4) & One-time ledger, epoch poisoning, erase-and-rekey & \cmark & \est{Rejected before any accepted reuse} \\
6 & Modify a DMA buffer after freezing (S3) & Freeze-before-challenge; consume only frozen pages & \cmark & \est{Frozen authenticated bytes consumed, or abort} \\
7 & Swap only the last column of a GPU matrix product & Frozen-operand Freivalds over all columns, $s=3$ (\cref{thm:freivalds}) & planned & \est{Rejected}, except with probability at most $p^{-3}$ \\
8 & Reuse one challenge vector across MAC lanes & Independent per-lane challenges; configuration check (counterexample in \cref{app:proof-auth}) & planned & \est{Configuration refused at session setup} \\
9 & Change database bytes or version after hashing (S8) & Same-byte snapshot hash and certificate binding (\cref{thm:pir}) & \cmark & \est{Abort; quarantined result never released} \\
10 & Request output before the verification barrier (S6) & Release guard (\cref{sec:proto-ledger}) & planned & \est{Guard stays closed; no candidate values leave} \\
11 & Overflow or truncate with the wrong signed rule & Exact finite reference; numeric contract (\cref{thm:cmp-trunc}) & \cmark & \est{Mismatch detected; manifest rejected} \\
12 & Delay, drop or reorder packets (S10) & Bounded resources and abort & planned & \est{Abort; no fairness or availability claimed} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\textwidth}{\footnotesize Reference model: \cmark{} executed and passing in the CPU reference model; planned: no executed evidence yet. Red outcomes are expected on the RTL and FPGA implementations, not yet observed. Scenario IDs refer to \cref{tab:scenarios}.}
\end{table*}

\Cref{tab:attacks} lists the twelve attack and fault injections of our test plan, the mechanism that must stop each one, whether the executed CPU reference model already covers it, and the outcome we expect on the RTL and FPGA implementations.
The injections cover the scenarios of \cref{tab:scenarios} except S2, which the interface excludes by construction, and S9, which the functionality permits (its commitment-bound loader variant is covered by the model-provenance mechanism, not by an injection).
For S2, the command set of \cref{tab:commands} has no entry point that authenticates a host-supplied value, and row~2 checks the related requirement that even the module's own engine output is never authenticated before it conforms to the reference.

\textbf{Executed functional validation.}
The functional reference implements the ideal-module model in Python~3.10+ using only the standard library.
In the preparation environment it passes 22 unit tests with 0 failures and 0 errors.
The tests cover 21{,}840 exhaustive small-domain DPF target, query and payload cases (\cref{thm:dpf-correct}); 2{,}728 party-local comparisons between streaming GaC and materialized evaluation (\cref{thm:gac}); 1{,}364 DCF comparisons (\cref{thm:dcf}); 20{,}004 CPU checks of the GPU Mersenne multiplication formula of \cref{sec:arch-field} against arbitrary-precision arithmetic, including boundary operands; all 31 elements of a toy field with $p=31$ for bit decomposition (\cref{thm:bitdec}); 124 signed-truncation cases (\cref{thm:cmp-trunc}); all 16 inputs of a small LUT (\cref{thm:lut}); selected exhaustive toy intervals (\cref{thm:interval}); a small composed nonlinear and arithmetic pipeline; and PIR snapshot rejection.
Negative tests exercise noncanonical encodings, tag and value mutations, poisoned epochs, role, replay and ordering errors, immutable frozen objects, joint sampling, truncation fibers, and the ring zero-divisor counterexample that motivates the field representation (\cref{app:proof-auth}).

\textbf{Limits of this evidence.}
The toy field $p=31$ serves finite correctness tests only and provides no cryptographic security.
The reference expands seeds with SHAKE rather than the pinned AES-based PRG, so the equivalence tests must be rerun against the production PRG and output conversion.
The CUDA micro-test (65{,}536 products against a host 128-bit reference) is written but has not been compiled or run, and the RTL release guard is written but has not been simulated or synthesized; no GPU toolchain, Vivado or RTL simulator was available in that environment.
Rows marked ``planned'' in \cref{tab:attacks} therefore have no executed evidence yet.
These tests check that the implementation conforms to the algorithms; they do not measure a forgery probability.
Observing zero accepted forgeries in any finite campaign cannot support a bound such as $2^{-148}$; that bound comes from \cref{thm:mac-sound} together with the ledger rules.
Power and electromagnetic analysis, probing and fault injection require separate, threat-specific engineering evaluation (\cref{sec:discussion}).

% =====================================================================
\subsection{Hardware Cost}\label{sec:eval-hw}

\begin{table}[t]
\centering
\caption{Hardware Cost of One \sys Module}
\label{tab:hwcost}
\footnotesize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l r r r r}
\hline
\multirow{2}{*}{\textbf{Component}} & \multicolumn{2}{c}{\textbf{28~nm}} & \multicolumn{2}{c}{\textbf{7~nm}} \\
\cline{2-5}
 & \textbf{mm$^2$} & \textbf{mW} & \textbf{mm$^2$} & \textbf{mW} \\
\hline
\multicolumn{5}{l}{\textit{DFA blocks reused by \sys~\cite{dfa2026trusted}}} \\
16 DPF units (64 AES-128) & 1.73 & 29 & 0.054 & 11 \\
SRAM buffers & 3.06 & 585 & 0.096 & 219 \\
VPU (16-lane Ara) & 1.97 & 794 & 0.062 & 298 \\
All DFA (incl.\ control core) & 7.67 & 1{,}683.5 & 0.239 & 631 \\
\hline
\multicolumn{5}{l}{\textit{Blocks added by \sys}} \\
Field unit array (128 lanes) & \est{2.80} & \est{1{,}000} & \est{0.088} & \est{375} \\
Check engine & \est{0.18} & \est{45} & \est{0.006} & \est{17} \\
AEAD/GHASH (freezer, peer channel) & \est{0.21} & \est{60} & \est{0.007} & \est{23} \\
Ledger, guard, parser & \est{0.09} & \est{12} & \est{0.003} & \est{5} \\
Ledger SRAM (32~KB) & \est{0.25} & \est{35} & \est{0.008} & \est{13} \\
Freeze SRAM (256~KB) & \est{1.07} & \est{200} & \est{0.033} & \est{75} \\
\cline{1-5}
\sys additions & \est{4.60} & \est{1{,}352} & \est{0.145} & \est{508} \\
\hline
\rowcolor{blue!6}All \sys & \est{12.27} & \est{3{,}036} & \est{0.384} & \est{1{,}139} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize DFA blocks are synthesis results from~\cite{dfa2026trusted}; blocks added by \sys are pre-synthesis estimates (red). 7~nm values are scaled with DeepScaleTool~\cite{sarangi2021deepscaletool}. One AEAD/GHASH block serves the freezer and the peer-channel controller. The 128 FUA lanes sit eight per DPF unit (area unchanged). Not yet costed: the trusted on-die links between the DPF units, the VPU and the VIGOR core.}
\end{table}

\begin{table}[t]
\centering
\caption{Planned ZCU102 Functional Prototype}
\label{tab:fpga}
\footnotesize
\setlength{\tabcolsep}{6pt}
\renewcommand{\arraystretch}{1.08}
\begin{tabular}{l r r r}
\hline
\textbf{Resource} & \textbf{Used} & \textbf{Available} & \textbf{Utilization} \\
\hline
LUT & \est{168K} & 274K & \est{61\%} \\
Flip-flop & \est{201K} & 548K & \est{37\%} \\
BRAM36 & \est{412} & 912 & \est{45\%} \\
DSP & \est{356} & 2{,}520 & \est{14\%} \\
\hline
\multicolumn{4}{l}{Datapath: \est{4} DPF units (\est{16} AES-128), \est{32} field lanes, \est{250~MHz}} \\
\multicolumn{4}{l}{DPF throughput: \est{1.0}~G~expansions/s; board power: \est{9.8~W}} \\
\multicolumn{4}{l}{Host link: \est{1.6~GB/s}, i.e., \est{50}~M authenticated elements/s} \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\linewidth}{\footnotesize XCZU9EG-2FFVB1156~\cite{amd2023zcu102}: configuration and pre-implementation estimates (red). The DPF throughput assumes \est{50\%} of the \est{2.0}~G~expansions/s peak of \est{16} AES engines at \est{250~MHz} (one block per engine and cycle, two blocks per expansion).}
\end{table}

\Cref{tab:hwcost} reports the cost of one module; at 7~nm a complete module occupies \est{0.384~mm$^2$}, \est{0.046\%} of the 826~mm$^2$ A100 die~\cite{nvidia2020ampere}.
The FUA dominates the additions with \est{61\%} of the added area and \est{74\%} of the added power at 7~nm, followed by the 256~KB freeze SRAM with \est{23\%} of the added area, whereas the logic that enforces the security policy (ledger, release guard, parser and check engine) takes only \est{0.009~mm$^2$}, or \est{6\%} of the additions.
As in DFA, arithmetic and memory dominate the cost, not control.
No AES engines are added, because challenge derivation and AEAD freezing time-share the 64 engines with PRG expansion (\cref{sec:arch-hw}); for BERT-Base, checking occupies the AES array and the FUA for about \est{2.8~ms} per query, below \est{0.1\%} of its latency.

\Cref{tab:fpga} sizes the external ZCU102 prototype, which exists to check functional conformance and streaming behavior on one board with an emulated peer; security measurements need two independent protected devices (\cref{sec:arch-deploy}).
Its \est{1.6~GB/s} host link (\est{50}~M authenticated elements/s at 32 bytes each), its smaller FUA and its slower DPF engine make it a pessimistic functional point rather than a performance target; the ZCU102 row of \cref{tab:ablation} models only the link and the FUA.
It is not a \ProfT deployment target (\cref{sec:arch-deploy}).

% =====================================================================
\subsection{Ablation Study}\label{sec:eval-ablation}

\begin{table*}[t]
\centering
\caption{Ablation on BERT-Base}
\label{tab:ablation}
\footnotesize
\setlength{\tabcolsep}{5pt}
\renewcommand{\arraystretch}{1.1}
\begin{tabular}{l c r r r r >{\raggedright\arraybackslash}p{5.1cm}}
\hline
\textbf{Configuration} & \textbf{Secure} & \makecell{\textbf{LAN}\\\textbf{(s)}} & \makecell{\textbf{Rel.}\\\textbf{LAN}} & \makecell{\textbf{WAN}\\\textbf{(s)}} & \makecell{\textbf{Energy}\\\textbf{(J)}} & \textbf{Note} \\
\hline
\rowcolor{blue!6}Compiler-selected default ($t=3$, batched checks) & \cmark & \est{3.83} & \est{1.00$\times$} & \est{89.7} & \est{73.7} & Reference configuration \\
w/o GaC & \cmark & \est{5.87} & \est{1.53$\times$} & \est{91.8} & \est{82.2} & Authenticated material spilled and reread \\
Tag trees instead of epilogue & \cmark & \est{4.12} & \est{1.08$\times$} & \est{90.0} & \est{80.4} & $(1+t)\times$ DPF work; FSS share is small \\
$t=1$ MAC lane & \xmark & \est{2.53} & \est{0.66$\times$} & \est{88.4} & \est{43.2} & $Q(2/p)^t=2^{-28}$ at $Q=2^{32}$: inadequate \\
$t=2$ MAC lanes & \cmark & \est{3.18} & \est{0.83$\times$} & \est{89.1} & \est{58.4} & $2^{-88}$ at $Q=2^{32}$ \\
FSS-only gates, conservative DCF & \cmark & \est{15.29} & \est{3.99$\times$} & \est{101.2} & \est{342.2} & $O(n^2)$ DCF of \cref{thm:dcf} \\
FSS-only gates, optimized DCF & \pmark & \est{4.20} & \est{1.10$\times$} & \est{90.1} & \est{82.3} & Projected; not covered by \cref{thm:dcf} \\
Direct protected gates only & \cmark & \est{3.82} & \est{1.00$\times$} & \est{89.7} & \est{73.3} & \ProfT only; drops the FSS-portability constraint \\
Small check batches ($m=64$) & \cmark & \est{4.24} & \est{1.11$\times$} & \est{90.2} & \est{74.6} & Per-batch overhead not amortized \\
External PCIe module (\est{25~GB/s}) & \cmark & \est{3.87} & \est{1.01$\times$} & \est{89.8} & \est{73.8} & Link roofline $B/32$ elements/s \\
ZCU102 link and FUA (\est{1.6~GB/s}, \est{32} lanes, \est{250~MHz}) & \cmark & \est{4.59} & \est{1.20$\times$} & \est{90.5} & \est{75.4} & Prototype link and slower triple generation; on-die DPF and AES rates kept \\
No \CheckOpen{} & \xmark & \est{3.80} & \est{0.99$\times$} & \est{50.5} & \est{73.6} & Insecure; performance lower bound only \\
\hline
\end{tabular}

\vspace{2pt}
\parbox{\textwidth}{\footnotesize LAN 1~GB/s, WAN 70~MB/s. Each row changes one choice of the compiler-selected default. Rel.\ LAN is LAN latency relative to the compiler-selected default. Secure: \cmark{} covered by our theorems; \pmark{} projected construction outside our proofs; \xmark{} not secure (statistically inadequate, or no verification). All latency and energy values are model estimates.}
\end{table*}

\Cref{tab:ablation} changes one design choice at a time for BERT-Base, and three conclusions follow.

\textbf{Protocol mechanisms.}
Generate-and-consume and the check round are the mechanisms that matter.
Disabling GaC costs \est{1.53$\times$} LAN latency (\cref{sec:eval-e2e}), and the insecure lower bound without \CheckOpen{} shows that the doubled round count costs \est{39~s} of the \est{89.7~s} WAN latency, the dominant WAN cost of malicious security.

\textbf{MAC lanes.}
$t$ is a security knob, not a performance one: $t=1$ saves \est{34\%} of the LAN latency but bounds a wrong opening only by $2^{-28}$, so the choice of $t=3$ follows from \cref{sec:sec-concrete} (\cref{tab:lanes}).

\textbf{Gate selection and placement.}
Because FSS is a small part of the malicious latency, tag trees, direct-only gates, small check batches and off-die links change LAN latency by at most \est{20\%} (with the DPF engine kept at its on-die rate); the epilogue matters most for LUT-heavy compiled models, where the \est{3.8--4.0$\times$} gate-level gap over per-lane tag trees (\cref{sec:eval-micro}) carries over.
The exception is FSS-only compilation with the conservative DCF of \cref{thm:dcf} (\est{3.99$\times$}), which is why the compiler selects gates by cost.
Direct-only (\est{3.82~s}) is marginally faster than the default (\est{3.83~s}) because the default keeps an FSS realization for gate shapes that the manifest marks as FSS-portable, so that the same compiled circuit runs under \ProfU; this allowance costs about \est{0.014~s} of module time (\cref{app:model}), and direct-only drops it and runs only under \ProfT (\cref{sec:proto-direct}).
Ablations on staged versus local checks and on caching versus recomputing bit decompositions are part of the measurement plan but are not yet modeled.

% =====================================================================
\subsection{Scalability}\label{sec:eval-scale}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{charts/chart_scale.pdf}
\caption{Scalability (model estimates). (a)~LAN latency with $t=1,2,3$ MAC lanes, normalized to semi-honest trusted DFA, annotated with the statistical term $Q(2/p)^t$ at $Q=2^{32}$ ($2^{-28}$, $2^{-88}$, $2^{-148}$). (b)~PIR throughput (queries/s, log scale) for $2^{14}$ to $2^{24}$ entries from a scaling model fitted to \cref{tab:pir} (a constant leaf rate for DFA and \sys, a calibrated per-entry efficiency for GPU-DPF); it matches the table at $2^{14}$, $2^{20}$ and $2^{22}$ entries to within \est{0.2\%}, interpolates between them and extrapolates beyond $2^{22}$ entries.}
\label{fig:scale}
\end{figure}

\textbf{MAC lanes and model size.}
\Cref{fig:scale}(a) normalizes LAN latency to semi-honest trusted DFA.
With $t=3$ the overhead grows from \est{2.46$\times$} for ResNet-50 to \est{3.51$\times$} for LLaMA2-7B, because the share of linear algebra grows with model size and each MAC lane replicates it: every additional lane adds about \est{0.65~s} for BERT-Base and \est{13.0~s} for LLaMA2-7B.
Authenticated GEMM on the GPU, not the protected module, is the scaling bottleneck.

\textbf{Triple generation.}
Correct matrix triples must be computed inside the protected boundary (\cref{sec:proto-arith}), so FUA work scales with the model's multiply-accumulate count.
LLaMA2-7B needs about \est{7.18~s} of FUA time per query at 128 lanes and 910~MHz, which overlaps with the \est{52.0~s} of authenticated GEMM except for an assumed \est{10\%} non-overlapped fraction ($\eta_{\mathrm{trip}}$, \cref{app:model}), leaving about \est{0.72~s} exposed.
The \est{32}-lane prototype at \est{250~MHz} would need about \est{105~s} for the same triples, another reason it is only a functional prototype; the on-die FUA should scale with the linear-algebra throughput of the host GPU.
If triple generation ever dominates, the alternatives are an imported malicious preprocessing backend with its own proof, or restructuring public-by-secret operations; exposing global secret masks to the GPU is not an option.

\textbf{Host-module bandwidth.}
BERT-Base moves only \est{1.66~GB} per party, well inside the $B/32$ roofline of \cref{sec:arch-insight}, which is why \cref{fig:bert}(b) is nearly flat above \est{8~GB/s}.

\textbf{PIR.}
\Cref{fig:scale}(b) shows PIR throughput from $2^{14}$ to $2^{24}$ entries.
Like DFA, the per-query cost of \sys grows linearly with the number of entries, so throughput falls from \est{1.05}~M to \est{1{,}022}~queries/s, whereas GPU-DPF reaches its peak per-entry efficiency near $2^{20}$ entries~\cite{dfa2026trusted,lam2023gpu}.
At $2^{24}$ entries \sys is \est{5.2$\times$} faster than GPU-DPF, under the weaker query-privacy model of \cref{sec:eval-pir}, and \est{11.5$\times$} faster than the authenticated GPU baseline.
Larger records increase the per-entry field reduction linearly while the DPF expansion stays unchanged, so for very large records the FUA, not the AES array, becomes the limit.

\textbf{Beyond per-lane tags.}
Because the tag lanes dominate large models, the most promising direction is to compress MAC checking, for example with rank-1 compressed checks that avoid carrying $t$ full tag arrays through the GPU.
Such schemes are not covered by our proofs and need their own soundness analysis, so we leave them to future work.
Scaling the number of DPF units and FUA lanes is a second, orthogonal knob; DFA found DPF-unit scaling to be nearly linear until on-chip bandwidth, about 7~TB/s of aggregate L2 read bandwidth on A100~\cite{nvidia2020ampere}, becomes the limit~\cite{dfa2026trusted}.


==> qa/draft4/sections/09_discussion.tex <==
% ==================================================================
% Section IX: Discussion and Limitations
% Owner labels: sec:discussion
% ==================================================================
\section{Discussion and Limitations}
\label{sec:discussion}

\sys claims that, under \ProfT, one maliciously corrupted host, including its GPU, driver and network stack, cannot make an honest party accept a wrong value or release an unauthorized one, except with the probability bounded in \cref{thm:main}. We now state what this claim does not cover and which evidence is still missing.

\textbf{Trust relocation, not removal.}
\sys moves the dealer of dealer-based FSS into two protected modules; it does not remove the dealer assumption. Both modules hold the joint-sampler key and the global MAC keys $\Delta_1,\dots,\Delta_t$ (\cref{sec:proto-setup}), so extracting the secrets of either module voids privacy and integrity for every session whose keys it holds. \Cref{thm:main} is a stand-alone statement under sequential composition; concurrent sessions that share module state are not covered (\cref{app:func}). The boundary also grows relative to DFA~\cite{dfa2026trusted}: the ledger, freezer, check engine, field unit array and release guard add only \est{0.145~mm$^2$} at 7~nm (\cref{tab:hwcost}), but each of them is logic that must be verified (\cref{tab:obligations}).

\textbf{What the modules learn.}
The modules are not blind. $\Pi_{\mathsf{Input}}$ validates $x^{*}=r+\varepsilon$ inside them (\cref{fig:arith}); after a verified opening $c = x + r$, module $T_b$ knows $c$ and $r$, hence $x$; the committed-input loader and the direct gate (\cref{sec:proto-direct}) see inputs explicitly; and in PIR both modules learn the client's index $\alpha$ (\cref{alg:pir}). For inference this is inherent to generate-and-consume and already holds for trusted DFA~\cite{dfa2026trusted}. For PIR it is a regression: the query privacy of \sys relies on module trust, whereas untrusted two-server DPF-PIR, such as GPU-DPF~\cite{lam2023gpu} and untrusted-mode DFA~\cite{dfa2026trusted}, hides $\alpha$ without trusted hardware. Client-generated keys evaluated inside the modules would avoid this but need key verification~\cite{decastro2022vfss}; neither this variant nor a constant-time select under \ProfT is modeled (\cref{sec:proto-pir}), and \cref{tab:pir} rests on assuming a PIR efficiency of \est{0.93} relative to DFA. FSS gates keep only seeds, control bits and correction words in long-lived state, whereas a direct gate computes on $x$ itself; we treat this as defense in depth only, because the trace model of \cref{thm:main} makes both options equivalent.

\textbf{Why two parties under \ProfT?}
Because the modules see plaintext, a single server whose protected module verifies an untrusted GPU, as in Slalom~\cite{tramer2018slalom}, would rest on the same hardware trust. The two-party structure buys two things. First, a host that held a value together with its complete tag would learn the MAC key; splitting every tag between two hosts lets SPDZ-style MACs~\cite{damgard2012spdz} check all GPU linear algebra at the next opening, whereas a single server must check each GPU product itself, for example with a Freivalds check per layer (\cref{sec:proto-freivalds}). Second, it keeps the two-party deployment of the FSS toolchains that DFA targets, on which \ProfU relies for its security (\cref{sec:threat-profileu}). It adds no protection against module compromise. For PIR as specified in \cref{alg:pir}, one server with one module would give the same guarantees. GPU-wide TEEs~\cite{nvidia_h100_overview,dhanuskodi2023confidential} avoid the four-lane GEMM cost but place the whole GPU and its firmware in the TCB.

\textbf{Physical and microarchitectural attacks.}
Probing~\cite{skorobogatov2017microprobing}, optical and other fault injection~\cite{skorobogatov2003optical,quadir2016survey}, and power or electromagnetic analysis~\cite{kocher1999differential} are outside \cref{thm:main} and can extract keys from an unhardened module. Faults matter more in the malicious setting: the bound $Q(2/p)^t$ presumes a correct check engine, so one glitch that forces acceptance bypasses it, and a fault in the field unit array can yield a wrong triple that carries valid tags. Software-controlled undervolting, which has induced such faults in SGX enclaves~\cite{murdock2020plundervolt}, is not physical: \cref{thm:main} assumes DVFS isolation (host software cannot drive the module's clock or voltage outside its safe operating range) and simulatable telemetry (\cref{sec:sec-assump}), whose realization we have not evaluated. Conversely, the module has no out-of-order core, no shared cache hierarchy and no host-managed page tables, so the controlled-channel, cache, transient-execution and Rowhammer attacks studied on general-purpose TEEs~\cite{xu2015controlled,shinde2015preventing,gotzfried2017cache,brasser2017software,lee2017inferring,van2018foreshadow,kim2014flipping} target mechanisms it lacks, and each check returns one generic status only after all $t$ lanes are aggregated. Small security chips have still shipped with exploitable flaws~\cite{moghimi2020tpm,han2018bad,butterworth2013bios}: a small TCB makes hardening tractable, but it does not replace hardening.

\textbf{Rollback and lifecycle.}
Ledger and epoch state live in volatile protected SRAM, so every reset falls under the reboot rule of \cref{sec:proto-ledger}. Because every failure poisons its epoch and aborted reservations never return to a free list (\cref{fig:ledger}), recovery always costs a new setup. Neither a monotonic service nor an erase-and-rekey lifecycle is implemented yet (\cref{tab:obligations}).

\textbf{Availability and fairness.}
\sys provides security with abort, the standard target for two-party computation with a malicious participant~\cite{hazay2010efficient,lindell2017simulate}. A corrupt host can withhold or reorder traffic, stall its GPU or abort at any public interaction boundary, and a corrupt recipient may obtain its output first; fairness and guaranteed output delivery are not claimed (S10 in \cref{tab:scenarios}). Aborts are, however, not a side channel on honest inputs. Apart from the validity predicates, which the modules evaluate before the first output opening and whose outcomes are the $\mathsf{status}$ part of $\Leak_C$ (\cref{def:leakage}), every \CheckOpen{} outcome depends only on the adversary's own deviation $(\bm{e},\bm{d}_j)$, the protected keys and the fresh challenges (\cref{thm:mac-sound}), and the first failure ends the epoch, so selective-failure and key-learning strategies cannot be iterated (\cref{lem:hidden-key}). Persistent denial of service remains a matter of deployment policy.

\textbf{Field versus ring.}
Over $\Fp$ with $p = 2^{61}-1$, \sys is not bit-identical to the $\Z_{2^{64}}$ arithmetic of Sigma and Orca~\cite{gupta2023sigma,jawalkar2024orca}. Ring-compiled models must be re-encoded under the numeric contract of \cref{sec:arch-field}, with magnitudes below $p/2$ before truncation, and exact signed truncation needs 307 authenticated multiplications on sequential carry chains, i.e., 309 rounds or \est{30.9~ms} on LAN (\cref{alg:bitdec,alg:trunc}), the most round-intensive gate in \cref{tab:gates}. A ring deployment needs a SPDZ2k-style backend~\cite{cramer2018spdz2k}, which is a separate design with a separate proof (\cref{sec:sec-concrete}).

\textbf{\ProfU.}
\ProfU (\cref{sec:threat-profileu}) is specified but not evaluated; it forfeits the local-dealer and generate-and-consume savings and must add the backend's key-privacy and answer-integrity arguments outside \cref{thm:main}.

\textbf{Model provenance.}
\sys proves correct evaluation on the inputs actually supplied (S9 in \cref{tab:scenarios}). A committed model (\cref{sec:threat-goals}) establishes provenance, not quality; the gap between the finite-field circuit and a floating-point model is an approximation question separate from cryptographic correctness.

\textbf{Artifact status.}
We executed a specification and a functional CPU reference model; GPU and RTL conformance, the protected runtime and deployment measurements have not been run yet (\cref{sec:eval-method,sec:eval-attack}). Every red value therefore awaits the three separate experiments of \cref{sec:arch-deploy}, and security measurements need two independent protected devices.


==> qa/draft4/sections/10_related.tex <==
% ==================================================================
% Section X: Related Work
% Owner labels: sec:related, tab:related
% ==================================================================
\section{Related Work}
\label{sec:related}

\begin{table*}[t]
\centering
\caption{Comparison of \sys with Representative Related Work}
\label{tab:related}
\footnotesize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.12}
\begin{tabular}{l c c c c l c c l}
\hline
\textbf{Work} & \textbf{Adversary} & \makecell{\textbf{Trusted}\\\textbf{HW}} & \makecell{\textbf{Trusted comp.}\\\textbf{sees plaintext}} & \makecell{\textbf{Custom}\\\textbf{HW}} & \textbf{Offline material} & \makecell{\textbf{Auth.\ FSS}\\\textbf{outputs}} & \makecell{\textbf{Verified}\\\textbf{openings}} & \textbf{Workloads} \\
\hline
Sigma~\cite{gupta2023sigma} & SH & \xmark & \xmark & \xmark$^{\mathrm{g}}$ & Dealer keys & \xmark & \xmark & Inference \\
Orca~\cite{jawalkar2024orca} & SH & \xmark & \xmark & \xmark$^{\mathrm{g}}$ & Dealer keys & \xmark & \xmark & Training, inference \\
Shark~\cite{gupta2025shark} & Mal & \xmark & \xmark & \xmark & Dealer, authenticated keys & \cmark & \cmark & Inference \\
\hline
MASCOT, MP-SPDZ~\cite{keller2016mascot,keller2020mpspdz} & Mal & \xmark & n/a & \xmark & Interactive (OT-based) & n/a & \cmark & General circuits \\
vFSS~\cite{decastro2022vfss} & Mal$^{\mathrm{a}}$ & \xmark & n/a & \xmark & Client keys, verified & \xmark & n/a & Key validation \\
APIR~\cite{colombo2023apir} & Mal$^{\mathrm{b}}$ & \xmark & n/a & \xmark & None (client query) & n/a & \cmark$^{\mathrm{b}}$ & PIR \\
\hline
Slalom~\cite{tramer2018slalom} & Mal$^{\mathrm{c}}$ & \cmark & \cmark & \xmark$^{\mathrm{g}}$ & n/a & n/a & \cmark$^{\mathrm{c}}$ & Inference \\
Aramis~\cite{kumar2020cryptflow} & Mal & \cmark$^{\mathrm{d}}$ & \xmark$^{\mathrm{d}}$ & \xmark & n/a & n/a & n/a & Inference \\
STAMP, PPMLAC~\cite{huang2022efficient,zhou2022ppmlac} & SH, Mal$^{\mathrm{e}}$ & \cmark & \pmark$^{\mathrm{e}}$ & \cmark & In trusted HW & n/a & \pmark$^{\mathrm{e}}$ & ML \\
\hline
GPU-DPF~\cite{lam2023gpu} & SH$^{\mathrm{i}}$ & \xmark & n/a & \xmark$^{\mathrm{g}}$ & None (client query) & \xmark & \xmark & PIR \\
DFA~\cite{dfa2026trusted} & SH$^{\mathrm{i}}$ & \pmark$^{\mathrm{f}}$ & \cmark$^{\mathrm{f}}$ & \cmark & Dealer or local$^{\mathrm{f}}$ & \xmark & \xmark & Inference, PIR \\
\hline
\textbf{\sys (this work)} & Mal$^{\mathrm{h}}$ & \cmark & \cmark$^{\mathrm{h}}$ & \cmark & Local, none shipped & \cmark & \cmark & Inference, PIR \\
\hline
\end{tabular}

\vspace{3pt}
\begin{minipage}{0.98\textwidth}
\footnotesize
SH: semi-honest; Mal: malicious (active) adversary. \emph{Trusted HW}: security relies on trusted hardware. \emph{Trusted comp.\ sees plaintext}: a trusted dealer, enclave or module sees inputs or intermediate values (FSS dealers are input independent). \emph{Custom HW}: dedicated hardware beyond commodity CPUs and GPUs. \emph{Offline material}: source of the per-query correlated randomness or keys. \emph{Auth.\ FSS outputs}: FSS gate outputs carry MAC tags. \emph{Verified openings}: opened values or untrusted results are checked before use. \cmark: yes; \xmark: no; \pmark: partial, optional or configuration dependent; n/a: not applicable. Lettered notes qualify the headline setting of each work.
$^{\mathrm{a}}$\,Malicious client key generator; servers check that keys are well formed, not that they are evaluated correctly.
$^{\mathrm{b}}$\,The client detects answers that are inconsistent with a public database digest.
$^{\mathrm{c}}$\,An SGX enclave outsources to an untrusted co-located GPU and checks its matrix products with Freivalds' algorithm.
$^{\mathrm{d}}$\,Relies on SGX integrity, not confidentiality.
$^{\mathrm{e}}$\,Settings differ between the two works: STAMP reports semi-honest and honest-majority malicious variants and evaluates nonlinear operations on unmasked values in its trusted processor; PPMLAC's trusted chipset mainly generates correlated randomness.
$^{\mathrm{f}}$\,Trusted mode only; the untrusted mode ships dealer keys.
$^{\mathrm{g}}$\,Implemented on commodity GPUs.
$^{\mathrm{h}}$\,Static corruption of one host, security with abort, under \ProfT, where the modules see inputs, openings and PIR indices; \ProfU delegates to an established malicious backend.
$^{\mathrm{i}}$\,In two-server DPF-PIR (GPU-DPF, DFA's untrusted mode), neither server learns the queried index, without relying on trusted hardware; SH refers to result integrity.
\end{minipage}
\end{table*}

\Cref{tab:related} summarizes the closest lines of work.

\textbf{FSS-based secure computation.}
FSS~\cite{boyle2015fss} and its tree-based DPF instantiations~\cite{gilboa2014distributed,boyle2016function} underlie a family of low-round two-party protocols with preprocessing~\cite{boyle2019preprocessing}. AriaNN~\cite{ryffel2020ariann} and Pika~\cite{wagh2022pika} first demonstrated private inference with FSS, Boyle et al.~\cite{boyle2021function} built comparisons, splines and fixed-point truncation from DCFs, Grotto~\cite{storrier2023grotto} replaced DCF-heavy constructions with DPF-based ones in a $(2{+}1)$-party setting, and Orca~\cite{jawalkar2024orca} and Sigma~\cite{gupta2023sigma} brought FSS-based training and GPT-class inference to GPUs. These systems are semi-honest and assume a dealer whose key material dominates the offline cost~\cite{huang2026beyond}. DPFs also underlie PIR, anonymous messaging, private queries and analytics, private heavy hitters, set intersection and distributed ORAM~\cite{corrigan2015riposte,wang2017splinter,dauterman2020dory,dauterman2022waldo,boneh2021lightweight,mouris2024plasma,garimella2024computation,vadapalli2023duoram,doerner2017scaling,ji2023multi}. Secure inference without FSS realizes nonlinear layers through share conversions, garbled circuits or homomorphic encryption~\cite{mohassel2017secureml,mohassel2018aby3,wagh2019securenn,wagh2020falcon,rathee2020cryptflow2,pang2024bolt,lu2023bumblebee}, typically with more interaction per layer.

\textbf{Malicious and verifiable FSS.}
To our knowledge, Shark~\cite{gupta2025shark} is the most directly comparable system: actively secure two-party FSS inference in which a trusted dealer supplies authenticated key material. Its security is cryptographic once its input-independent dealer, which never sees an input or an opening, is trusted, whereas each \sys module sees every input and opening under \ProfT (\cref{sec:eval-method}). In exchange, \sys generates the authenticated correlations locally and removes the offline distribution that dominates the dealer-based malicious FSS baseline, modeled after the protocol family of Shark~\cite{gupta2025shark} (\cref{tab:e2e}). Verifiable FSS~\cite{corrigan2015riposte,boyle2016function,boneh2021lightweight,decastro2022vfss} addresses a different adversary, a client that may submit malformed keys, which the servers detect; \sys instead treats key generation, evaluation, authentication and release as separate obligations. VeriFSS~\cite{xue2026verifss} removes the dealer altogether: its dealer-free two-party FSS attains static malicious security with authenticated sharings and a cross-phase verification that binds key generation to evaluation, generating keys interactively between the two parties, whereas \sys generates them inside the modules.

\textbf{Malicious MPC preprocessing and MACs.}
Beyond the SPDZ-family tools of \cref{sec:bg-mal}, mixed-circuit preprocessing with edaBits~\cite{escudero2020edabits} and classical bit-decomposition and truncation protocols~\cite{damgard2006unconditionally,catrina2010improved} supply the conversions that nonlinear layers need, and honest-majority protocols~\cite{furukawa2017high,mohassel2018aby3,wagh2020falcon,dalskov2021fantastic} obtain malicious security from replicated sharing among three or four servers. \sys adopts, and does not claim as new, the SPDZ MAC algebra with $t$ independent keys over a Mersenne field. It replaces interactive preprocessing by correct generation inside the modules, in the spirit of hardware-assisted correlation generation~\cite{lu2021correlated,zhou2022ppmlac}, and checks openings on frozen bytes (\cref{sec:proto-check}).

\textbf{Trusted hardware for MPC and ML.}
Tamper-proof tokens are a classical setup assumption for universally composable computation~\cite{katz2007universally}, and commodity TEEs~\cite{costan2016intel,amd_sev,arm_trustzone,lee2020keystone} have been used to accelerate or simplify two-party computation and functional encryption~\cite{gupta2016using,choi2019hybrid,felsen2019secure,wuhybrid,fisch2017iron}. For ML, Ohrimenko et al.~\cite{ohrimenko2016oblivious} and Chiron~\cite{hunt2018chiron} execute learning tasks inside SGX enclaves; Slalom~\cite{tramer2018slalom} and DarKnight~\cite{hashemi2021darknight} outsource linear layers from an enclave to untrusted GPUs and verify them, with Freivalds' algorithm~\cite{freivalds1977probabilistic} and with redundant coded computation, respectively; and Aramis~\cite{kumar2020cryptflow} compiles semi-honest protocols into maliciously secure ones by relying on the integrity, but not the confidentiality, of SGX. GPU TEEs~\cite{volos2018graviton,jang2019heterogeneous} and confidential computing on H100~\cite{nvidia_h100_overview,dhanuskodi2023confidential} protect GPU computation from the host but place the whole GPU and its firmware in a TCB far larger than our module. Closest to our trust model, STAMP~\cite{huang2022efficient} and PPMLAC~\cite{zhou2022ppmlac} rely on a small security processor or a trusted chipset to execute nonlinear operations or generate correlated randomness, respectively, in the tradition of TPM-class security chips, secure coprocessors and smart cards~\cite{tpm2spec,googletitan,ibm4758,rankl2004smart}, and DFA~\cite{dfa2026trusted} uses a small module as a local FSS dealer. STAMP's nonlinear evaluation inside its trusted processor corresponds to our direct protected gate (\cref{sec:proto-direct}). Relative to it, \sys contributes a two-party setting with an untrusted GPU checked by MACs, freeze-before-challenge checking against host-controlled DMA, ledgered one-time randomness, and a malicious FSS and PIR datapath. Like Slalom and DarKnight, \sys keeps the GPU outside the boundary, but it uses Freivalds checks only for operands the GPU may already see (\cref{sec:proto-freivalds}).

\textbf{Hardware acceleration for private computation.}
GPU systems accelerate secret-sharing MPC~\cite{tan2021cryptgpu,watson2022piranha,crypten2020}, FSS~\cite{gupta2023sigma,jawalkar2024orca} and DPF-based PIR~\cite{lam2023gpu}. FPGA designs target secret-sharing MPC~\cite{wolfe2020secret,patel2020arithmetic,xu2025co}, Ironman~\cite{ironman2025} accelerates OT extension near memory, KORD~\cite{peng2026kord} co-designs dealerless FSS key generation with paired, mutually attested chips on an FPGA, and FPGA and ASIC designs speed up the polynomial kernels of homomorphic encryption~\cite{riazi2020heax,reagen2021cheetah,samardzic2021f1,samardzic2022craterlake,kim2022bts}. These accelerators make a fixed protocol faster and inherit its adversary model. DFA~\cite{dfa2026trusted} additionally used trust to change the dataflow; \sys uses the same small trusted module to change the adversary model, which is why \cref{sec:eval} compares against security-matched baselines rather than raw kernel throughput alone.

\textbf{PIR with integrity.}
Authenticated PIR~\cite{colombo2023apir} lets a client detect answers that are inconsistent with a public database digest without trusted hardware, at additional server cost that our APIR-based GPU baseline reflects (\cref{tab:pir}). PIR with secure coprocessors~\cite{smith2001practical} and enclave-based oblivious storage such as Snoopy~\cite{dauterman2021snoopy} instead trust hardware that learns the query and hides its accesses through oblivious scans. The versioned-snapshot PIR of \sys follows this trust model: both modules learn the queried index $\alpha$, so its query privacy rests on module trust, unlike untrusted two-server DPF-PIR (GPU-DPF~\cite{lam2023gpu}, DFA's untrusted mode), which hides $\alpha$ from each server without trusted hardware. It scans in two role-bound modules, binds the exact consumed bytes to an authorized commitment $\mathsf{cm}_v$, optionally a Merkle root~\cite{merkle1987digital}, and releases freshly reshared answers only after the snapshot hash matches (\cref{sec:proto-pir}).

\textbf{Positioning.}
Each ingredient of \sys, from information-theoretic MACs and trusted correlation generation to verified GPU work and DPF acceleration, has precedents; our contribution is their composition in one small trusted module, proven stand-alone secure with abort in the ideal-module model of \cref{sec:threat-model} (\cref{tab:related}).


==> qa/draft4/sections/11_conclusion.tex <==
% ==================================================================
% Section XI: Conclusion (owner: sections/11_conclusion.tex)
% Labels defined here: sec:conclusion
% ==================================================================
\section{Conclusion}\label{sec:conclusion}

We presented \sys, a trusted hardware accelerator that secures FSS-based private inference and DPF-based PIR against a malicious host and GPU while keeping the key-movement savings of trusted DFA. Since a module acting as FSS dealer can also be the verifier, \sys generates authenticated correlations internally, authenticates DPF outputs with a fresh resharing epilogue instead of extra DPF trees, checks every opening on frozen bytes with $t=3$ independent MAC lanes over $\F_{2^{61}-1}$, and releases nothing before a role-bound one-time ledger records a verified check. These mechanisms protect the chain from authorized input to authorized output release; we prove stand-alone static malicious security with abort in a protected-module model, with statistical error about $2^{-148}$ for $2^{32}$ checked batches. Both modules see inputs and learn the PIR index, so PIR query privacy rests on module trust, unlike untrusted two-server DPF-PIR~\cite{lam2023gpu}. Our model estimates that \sys is \est{10.1--14.0$\times$} faster on a LAN than dealer-based malicious FSS modeled after the protocol family of Shark~\cite{gupta2025shark}, mainly because in-module generation removes \est{21.8--563~GB} of per-query offline distribution (\est{1.5--1.8$\times$} excluding it). Malicious security costs \est{2.5--3.5$\times$} LAN latency over semi-honest DFA and \est{0.145~mm$^2$} at 7~nm (pre-synthesis).

We executed a specification and a functional CPU reference model; GPU/RTL conformance, the protected runtime and deployment measurements have not been run yet, so no \sys performance number is measured. Three directions follow. First, these measurements, synthesis and on-die simulation must replace the estimates. Second, a \ProfU backend would run the same compiled circuit when the hardware is adversarial, and a SPDZ2k-style backend would cover the ring $\Z_{2^{64}}$. Third, compressed MAC checks that avoid carrying all tag lanes through the GPU would cut the now-dominant authenticated linear algebra; a vetted DCF faster than our $O(n^2)$ one would help FSS-only configurations, not the compiler-selected default, where nonlinear gates take \est{3.4\%} of BERT-Base latency. Both need proofs this paper does not provide.

\section*{Acknowledgment}
Omitted for anonymous review.

